Neural Networks with Physics-Informed Architectures and Constraints for Dynamical Systems Modeling

Effective inclusion of physics-based knowledge into deep neural network models of dynamical systems can greatly improve data efficiency and generalization. Such a-priori knowledge might arise from physical principles (e.g., conservation laws) or from the system's design (e.g., the Jacobian matrix of a robot), even if large portions of the system dynamics remain unknown. We develop a framework to learn dynamics models from trajectory data while incorporating a-priori system knowledge as inductive bias. More specifically, the proposed framework uses physics-based side information to inform the structure of the neural network itself, and to place constraints on the values of the outputs and the internal states of the model. It represents the system's vector field as a composition of known and unknown functions, the latter of which are parametrized by neural networks. The physics-informed constraints are enforced via the augmented Lagrangian method during the model's training. We experimentally demonstrate the benefits of the proposed approach on a variety of dynamical systems -- including a benchmark suite of robotics environments featuring large state spaces, non-linear dynamics, external forces, contact forces, and control inputs. By exploiting a-priori system knowledge during training, the proposed approach learns to predict the system dynamics two orders of magnitude more accurately than a baseline approach that does not include prior knowledge, given the same training dataset.

==> algorithms/inner_loop.tex <==
\begin{algorithm}[H]
\caption{Train for fixed $\lambda \geq 0$ and $\mu \geq 0$}
\label{alg:inner_loop}
\textbf{Input}: $\nnParamsAll$, $\vectorField(\cdot)$, $\{\equalConstr_i(\cdot)\}_{i \in [\numEqualConstr]}$, $\{\inequalConstr_j(\cdot)\}_{j \in [\numInequalConstr]}$, $\dataset$, $\collocationPoints$\\
\textbf{Parameter}: $N_{\mathrm{trainBatch}}$, $N_{\mathrm{constrBatch}}$, $\lagrangeVar^\mathrm{eq}_{i,k}$, $\lagrangeVar^\mathrm{ineq}_{j,k}$, and $\mu$\\
\textbf{Output}: Updated model parameters $\nnParamsAll$.

\begin{algorithmic}[1] %[1] enables line numbers

    \WHILE{\textbf{not} SGDStoppingCriterion()}
        \STATE $\dataset_{batch} \gets Sample(\dataset, N_{trainBatch})$
        \STATE $\collocationPoints_{batch} \gets Sample(\collocationPoints, N_{constrBatch})$
        \STATE $\nnParamsAll \gets optimUpdate(\mathcal{L}, \nnParamsAll, \dataset_{batch}, \collocationPoints_{batch})$
    \ENDWHILE

\end{algorithmic}

\end{algorithm}

==> algorithms/outer_loop.tex <==
\begin{algorithm}[H]
\caption{Model Training}
\label{alg:algorithm}
\textbf{Input}: $\vectorField(\cdot)$, $\{\equalConstr_i(\cdot)\}_{i \in [\numEqualConstr]}$, $\{\inequalConstr_j(\cdot)\}_{j \in [\numInequalConstr]}$, $\dataset$, $\collocationPoints$\\
\textbf{Parameter}: $\constrTol$, $\constrPenalty_0$, $\constrPenalty_{mult}$, $N_{\mathrm{trainBatch}}$, $N_{\mathrm{constrBatch}}$\\
\textbf{Output}: Model parameters $\nnParamsAll$.

\begin{algorithmic}[1] %[1] enables line numbers

\STATE Initialize parameters \(\nnParamsAll\); $\lambda \gets 0$; $\constrPenalty \gets \constrPenalty_0$.

\WHILE{$\mathrm{Constraint \ violation \ sum} \geq \constrTol$} 
    \STATE $\nnParamsAll \gets \mathrm{Train}(\nnParamsAll, N_{\mathrm{trainBatch}}, N_{\mathrm{constrBatch}})$
    \STATE $\lagrangeVar^\mathrm{eq}_{i,k} \gets \lagrangeVar^\mathrm{eq}_{i,k} + 2 * \constrPenalty * \equalConstr_i(\state_k, \controlInput_k, \collectionUnknownTerms)$
    \STATE $\lagrangeVar^\mathrm{ineq}_{j,k} \gets (\lagrangeVar^\mathrm{ineq}_{j,k} + 2 * \constrPenalty * \inequalConstr_j(\state_k, \controlInput_k, \collectionUnknownTerms))_+$
    \STATE $\constrPenalty \gets \constrPenalty * \constrPenalty_{mult}$
\ENDWHILE

\end{algorithmic}

\end{algorithm}

==> figs/approach_illustration.tex <==
\begin{tikzpicture}[
    % title/.style={font=\fontsize{6}{6}\color{black!50}\ttfamily},
    % typetag/.style={rectangle, draw=black!50, font=\scriptsize\ttfamily, anchor=west}
    % title/.style={font=\fontsize{6}{6}\color{black!70}\ttfamily},
    title/.style={font=\fontsize{6}{6}\color{black}\ttfamily},
    typetag/.style={rectangle, draw=black!50, font=\scriptsize\ttfamily, anchor=west},
    emptytag/.style={rectangle, draw=black!0, font=\scriptsize\ttfamily, anchor=west},
    plustag/.style={circle, draw=black!50, font=\scriptsize\ttfamily, anchor=west},
    line/.style={thick, draw},
    Arr/.style={-{Latex[length=1.5mm]}},
]

%%%%%%%%%%%%%%% BRAX ENV BOX
% Draw a rectange for the Brax system
% \node (braxTitle) [title, fill=green!10, anchor=west] {Simulation Environment};
% \node (braxImage) [below= 0.8cm of braxTitle.west, emptytag, inner sep=0, fill=blue!0, xshift=0cm, yshift=0] {\includegraphics[width=2.0cm, height=1.5cm] {figs/ant_v3.png}};

\node (braxImage) [emptytag, inner sep=0, fill=blue!0, xshift=0cm, yshift=0] {\includegraphics[width=2.0cm, height=1.5cm] {figs/ant_v3.png}};

\begin{scope}[on background layer]
    \node (rect0) [draw=black!50,
        inner xsep=0.1mm,
        inner ysep=0mm,
        % rounded corners=0.15cm,
        % fill=green!10,
        fit={(braxImage)}] {};
  %you may also use align = center instead of text width = ...
\end{scope}

%%%%%%%%%%%%%%% SIDE INFO CONSTRAINTS BLOCK
% We will draw  the title of side information here
\node (sideInfoConstraints) [title, anchor=west, below= 10.5mm of rect0.west, yshift=0, xshift=20mm] { Physics-Informed Constraints};

\node (sideInfoConstr) [  draw=black!50,
        fill=yellow!30,
        below= 3mm of sideInfoConstraints.west,
        typetag,
        xshift=0mm,
        yshift=-1mm,
        inner xsep=1mm,
        inner ysep=1mm,] {$\textcolor{black}{\constr}\big( x, u, \textcolor{red}{\funk_1}(\cdot),\hdots,\textcolor{red}{\funk_\mathrm{d}}(\cdot)\big) \leq 0$};
        
\node (sideInfoConstrEg) [
    below= 7mm of sideInfoConstraints.west, 
    title, 
    % fill=yellow!10, 
    xshift=30mm,
    text width=6cm] {e.g., $\textcolor{red}{\mathcal{F}_{norm}}(q,\dot{q}, u) \geq 0$};
    
\node (sideInfoConstrEg2) [
    below= 11mm of sideInfoConstraints.west, 
    title, 
    % fill=yellow!10, 
    xshift=30mm,
    text width=6cm] { $||\textcolor{red}{\mathcal{F}_{tang}}(q,\dot{q}, u)|| \leq \mu * \textcolor{red}{\mathcal{F}_{norm}}(q,\dot{q}, u)$};
        
\begin{scope}[on background layer]
    \node (rect1b) [
        % draw=black!50,
        % fill=yellow!10,
        rounded corners=0.15cm,
        fit={(sideInfoConstraints) (sideInfoConstr) (sideInfoConstrEg)}] {};
\end{scope}

%%%%%%%%%%%%%%% SIDE INFO STRUCTURE BOX
% We will draw  the title of side information here
\node (sideInfoStructure) [title, right= 2.0cm of braxImage.north east, yshift=0.5mm, xshift=0mm] { Physics-Informed Structure};

% Draw a rectangle for the dynamics side information
\node (sideInfoF) [  draw=blue,
        fill=blue!30,
        below= 4mm of sideInfoStructure.west, 
        typetag, 
        xshift=0mm,
        inner xsep=1.1mm,
        inner ysep=1mm,] {$\dot{x} = \textcolor{blue}{\fknown}\big( x, u, \textcolor{red}{\funk_1}(\cdot),\hdots,\textcolor{red}{\funk_\mathrm{d}}(\cdot)\big)$};
        
\node (sideInfoStructureEg) [
        below= 6mm of sideInfoStructure.west,
        xshift=23mm,
        title, 
        % fill=blue!10, 
        xshift=8mm] {e.g., $\ddot{q} = M^{-1}(q)[C(q,\dot{q}) + \textcolor{red}{\tau}(q,\dot{q}, u) + J(q)\textcolor{red}{\mathcal{F}}(q,\dot{q},u)]$};
        
\begin{scope}[on background layer]
    \node (rect1) [
            % draw=black!50,
            % fill=blue!10,
            rounded corners=0.15cm,
            fit={(sideInfoStructure) (sideInfoF) (sideInfoStructureEg)}] {};
\end{scope}

%%%%%%%%%%%%%%% NEURAL ODE BOX
\node (neuralODE) [
    title, 
    fill=blue!10, 
    right= 9cm of braxImage.north east,
    yshift=-2mm] { Physics-Informed Neural ODE};

% Construct the first neural network
\node (inputx) [draw,
                below=of neuralODE.west,
                minimum width= 0.1mm,
                inner sep=0.2mm,
                plustag,
                ] {$x$};
                
\node (inputu) [draw,
                below= 6mm of inputx.west,
                minimum width= 0.1mm,
                inner sep=0.2mm,
                plustag,
                ] {$u$};

\node (rect2) [draw=black!50,
        rounded corners=0.1cm,
        fit={(inputx) (inputu)}] {};

% Neural network 1 label
\node (nn1) [right=of rect2, yshift=0.65cm, xshift=-1cm, align=center] {\includegraphics[width=2cm, height=1cm] {figs/nn_example.png}};
\node (nn1input1) [left=of nn1,xshift=13mm, yshift=1.325mm]{$\cdot$};
\node (nn1input2) [left=of nn1,xshift=13mm, yshift=-1.4mm]{$\cdot$};

% Neural network 2 label
\node (nn2) [below= 0.3cm of nn1, align=center] {\includegraphics[width=2cm, height=1cm] {figs/nn_example.png}};
\node (nn2input1) [left=of nn2,xshift=13mm, yshift=1.325mm]{$\cdot$};
\node (nn2input2) [left=of nn2,xshift=13mm, yshift=-1.4mm]{$\cdot$};

\path (nn1) -- (nn2) node [black, font=\small, midway, sloped] {$\dots$};
\path [line] (inputx)--(nn1input1.center);
\path [line] (inputu)--(nn1input2.center);
\path [line] (inputx)--(nn2input1.center);
\path [line] (inputu)--(nn2input2.center);

\node (g1node) [  draw=blue,
        fill=blue!30,
        right= -1mm of nn1, 
        typetag, ] {$\textcolor{red}{\funk_1}$};

\node (gdnode) [  draw=blue,
        fill=blue!30,
        right= -1mm of nn2, 
        typetag, ] {$\textcolor{red}{\funk_d}$};

\path (g1node) -- (gdnode) node [black, font=\small, midway, sloped] {$\dots$};

\node (knownfun) [  draw=blue,
        fill=blue!30,
        right= 1mm of g1node, 
        inner sep=0.2mm,
        yshift=-0.75cm,
        typetag, ] {$\textcolor{blue}{\fknown}\big(\cdots)$};
        
% \path (inputx) -- (nn1) node;

\begin{scope}[on background layer]
    \node (rect3) [draw=black!50,
            fill=blue!10,
            rounded corners=0.15cm,
            inner xsep=0.5mm,
            inner ysep=0mm,
            fit={(neuralODE) (rect2) (nn1) (nn2) (knownfun)}] {};
\end{scope}

\draw [arrows={->[scale=0.5]}, thick] (g1node.east) -- ++(0.55cm,0) -| (knownfun.north);
\draw [arrows={->[scale=0.5]}, thick] (gdnode.east) -- ++(0.55cm,0) -| (knownfun.south);

%%%%%%%%%%%%%%% CONSTRAINT ENFORCEMENT BOX

\node (constrIlluTitle) [title, fill=yellow!10, right= 10mm of sideInfoConstr.east, yshift=5.0mm, xshift=-0mm] {Enforce $\textcolor{black}{\constr}$ Throughout State Space};
\node (constrIllu) [below= 0.5mm of constrIlluTitle, inner xsep=0.1mm, inner ysep=0mm,] {\input{figs/constraints_illustration}};

\begin{scope}[on background layer]
    \node (rect4) [draw=black!80,
        fit={(constrIlluTitle) (constrIllu)},
        fill=yellow!10,
        inner xsep=0.1mm,
        inner ysep=0mm,
        rounded corners=0.15cm] {};
\end{scope}

%%%%%%%%%%%% ODE SOLVER BOX

\node (odeSolverTitle) [draw=gray,
        fill=gray!30,
        below= 2.25cm of rect3.east,
        yshift=-0.0cm,
        xshift=-15mm,
        typetag,
        xshift=0mm,
        inner xsep = 0mm,
        align = center,
        text width=1cm,
        minimum width=1.3cm,
        minimum height=1cm]{ODE\\Solver};

%%%%%%%%%%%% LOSS BOX

\node (LossTitle) [draw=black,
        fill=red!10,
        left= 29mm of odeSolverTitle.west,
        yshift=-0.0cm,
        typetag,
        xshift=0mm,
        inner xsep = 0mm,
        align = center,
        text width=1cm,
        minimum width=1.3cm,
        minimum height=1cm] {Loss \(\loss(\cdot)\)};

%%%%%%%%%%%% Connections

\path[
    every node/.style={font=\scriptsize\ttfamily},
    thick, 
    arrows={->[scale=0.5]}
    ] (20.5mm, -4.0mm) edge node[pos=0.15, fill=white] {Training data} (108mm, -4.0mm);
    % (rect3) edge (rect4);

\draw [arrows={->[scale=0.5]}, thick] (rect3.west)+(0.0mm, -10mm) -- node[font=\scriptsize\ttfamily, pos=0.55, below, text width=1.5cm] {$\funk_1(\cdot), ..., \funk_d(\cdot)$} (91mm, -17.5mm);

\draw [arrows={->[scale=0.5]}, thick] (sideInfoF.east) -- (108mm,4mm);

\draw [arrows={->[scale=0.5]}, thick] (sideInfoConstr.east) --  node[font=\scriptsize\ttfamily, below, pos=1.0, text width=1.5cm] {$\constr(\cdot)$} (47.0mm, -16.5mm);
% \node(contrPathLabel)[font=\scriptsize\ttfamily, right=1.1cm of rect1b.east, yshift=-1.2cm] {$\constr(\cdot)$};

\draw [arrows={->[scale=0.5]}, thick] (rect4.east)+(0.0mm, -8.3mm) -- node[font=\scriptsize\ttfamily, text width=2cm, below, pos=0.7] {Constraint violations} (LossTitle.west);

\draw [arrows={->[scale=0.5]}, thick] (rect3.east) -- node[font=\scriptsize\ttfamily, right, text width=0.5cm, yshift=-5mm, xshift=3mm] {Vector field} ++(0.5cm,0) |- (odeSolverTitle.east);

\draw [arrows={->[scale=0.5]}, thick] (odeSolverTitle.west) -- node[font=\scriptsize\ttfamily, below, text width=1.5cm] {Predicted next state} (LossTitle.east);
        
\end{tikzpicture}

==> figs/constraints_illustration.tex <==
% This file was created with tikzplotlib v0.9.12.
\begin{tikzpicture}
\tikzstyle{every node}=[font=\scriptsize\ttfamily]
\definecolor{color0}{rgb}{0.611534025374856,0.0664359861591696,0.154786620530565}
\definecolor{color1}{rgb}{0.853056516724337,0.408304498269896,0.32641291810842}
\definecolor{color2}{rgb}{0.976931949250288,0.767474048442907,0.663667820069204}
\definecolor{color3}{rgb}{0.965705497885429,0.967243367935409,0.968089196462899}
\definecolor{color4}{rgb}{0.713033448673588,0.843906189926952,0.910726643598616}
\definecolor{color5}{rgb}{0.29919261822376,0.599538638985006,0.777162629757785}
\definecolor{color6}{rgb}{0.0971164936562861,0.337716262975779,0.58800461361015}

\begin{axis}[
legend cell align={left},
legend columns=2,
legend style={at={(0.0,-0.025)}, 
                fill opacity=0.9, anchor=north west,
                draw opacity=1, text opacity=1, 
                draw=white!80!black
            },
% legend style={
%   fill opacity=0.8,
%   draw opacity=1,
%   text opacity=1,
%   at={(0.03,0.97)},
%   anchor=north west,
%   draw=white!80!black
% },
tick pos=left,
width=5.3cm,
height=2.8cm,
% width=5.85cm,
% height=3.0cm,
xmajorgrids,
xmin=-2.44986404635652, xmax=2.05013595364348,
xticklabels={,,}
ymajorgrids,
ymin=-2.85182560572801, ymax=2.14817439427199,
yticklabels={,,},
]
\addplot [draw=none, fill opacity=0.8, fill=color0, forget plot]
table{%
x  y
-1.94986404635652 -2.35416462626448
-1.44986404635652 -2.64903401586017
-0.949864046356524 -2.68951748658423
-0.449864046356524 -2.43745104940097
-0.371563457552893 -2.35182560572801
-0.311004671967729 -1.85182560572801
-0.449864046356524 -1.78745708016447
-0.899092035618981 -1.35182560572801
-0.949864046356524 -1.3190719845487
-1.42401981342171 -0.851825605728012
-1.44986404635652 -0.791543906019143
-1.82808478867862 -0.351825605728012
-1.86493817321396 0.148174394271988
-1.6471029154035 0.648174394271988
-1.44986404635652 0.821934600464166
-0.983160009087089 1.14817439427199
-0.949864046356524 1.17448111767971
-0.449864046356524 1.47503808532056
0.0501359536434758 1.52933980178775
0.550135953643476 1.49038837571411
1.05013595364348 1.21287762528535
1.13844632066377 1.14817439427199
1.53948944129687 0.648174394271988
1.55013595364348 0.427521032564775
1.61290748225476 0.148174394271988
1.55013595364348 0.0658812072378536
1.50834026388732 -0.351825605728012
1.41074556169161 -0.851825605728012
1.30158235178746 -1.35182560572801
1.55013595364348 -1.69854222265406
2.05013595364348 -1.713915884788
2.05013595364348 -1.35182560572801
2.05013595364348 -0.851825605728012
2.05013595364348 -0.351825605728012
2.05013595364348 0.148174394271988
2.05013595364348 0.648174394271988
2.05013595364348 1.14817439427199
2.05013595364348 1.44841319917069
1.94352454058394 1.64817439427199
1.56257961538885 2.14817439427199
1.55013595364348 2.14817439427199
1.05013595364348 2.14817439427199
0.550135953643476 2.14817439427199
0.0501359536434758 2.14817439427199
-0.449864046356524 2.14817439427199
-0.949864046356524 2.14817439427199
-1.44986404635652 2.14817439427199
-1.79406596272788 2.14817439427199
-1.94986404635652 2.00463645042387
-2.24691928397388 1.64817439427199
-2.44986404635652 1.28036339202376
-2.44986404635652 1.14817439427199
-2.44986404635652 0.648174394271988
-2.44986404635652 0.148174394271988
-2.44986404635652 -0.351825605728012
-2.44986404635652 -0.851825605728012
-2.44986404635652 -1.35182560572801
-2.44986404635652 -1.54336622833048
-2.30838075939904 -1.85182560572801
-1.95225198409933 -2.35182560572801
-1.94986404635652 -2.35416462626448
};
\addplot [draw=none, fill opacity=0.8, fill=color1, forget plot]
table{%
x  y
-1.94986404635652 -2.85182560572801
-1.44986404635652 -2.85182560572801
-0.949864046356524 -2.85182560572801
-0.449864046356524 -2.85182560572801
0.0501359536434758 -2.85182560572801
0.0574875400142759 -2.85182560572801
0.515399127540899 -2.35182560572801
0.550135953643476 -2.2342986727799
1.05013595364348 -2.2443246385385
1.50852492056687 -2.35182560572801
1.55013595364348 -2.36045359913171
2.05013595364348 -2.40766523675514
2.05013595364348 -2.35182560572801
2.05013595364348 -1.85182560572801
2.05013595364348 -1.713915884788
1.55013595364348 -1.69854222265406
1.30158235178746 -1.35182560572801
1.41074556169161 -0.851825605728012
1.50834026388732 -0.351825605728012
1.55013595364348 0.0658812072378536
1.61290748225476 0.148174394271988
1.55013595364348 0.427521032564775
1.53948944129687 0.648174394271988
1.13844632066377 1.14817439427199
1.05013595364348 1.21287762528535
0.550135953643476 1.49038837571411
0.0501359536434758 1.52933980178775
-0.449864046356524 1.47503808532056
-0.949864046356524 1.17448111767971
-0.983160009087089 1.14817439427199
-1.44986404635652 0.821934600464166
-1.6471029154035 0.648174394271988
-1.86493817321396 0.148174394271988
-1.82808478867862 -0.351825605728012
-1.44986404635652 -0.791543906019143
-1.42401981342171 -0.851825605728012
-0.949864046356524 -1.3190719845487
-0.899092035618981 -1.35182560572801
-0.449864046356524 -1.78745708016447
-0.311004671967729 -1.85182560572801
-0.371563457552893 -2.35182560572801
-0.449864046356524 -2.43745104940097
-0.949864046356524 -2.68951748658423
-1.44986404635652 -2.64903401586017
-1.94986404635652 -2.35416462626448
-1.95225198409933 -2.35182560572801
-2.30838075939904 -1.85182560572801
-2.44986404635652 -1.54336622833048
-2.44986404635652 -1.85182560572801
-2.44986404635652 -2.35182560572801
-2.44986404635652 -2.85182560572801
-1.94986404635652 -2.85182560572801

-0.588679351959038 -1.35182560572801
-0.949864046356524 -1.11882111202746
-1.22080773865843 -0.851825605728012
-1.44010653214624 -0.351825605728012
-1.44986404635652 -0.237189971016923
-1.53102991188118 0.148174394271988
-1.44986404635652 0.269759250528547
-1.31985034988364 0.648174394271988
-0.949864046356524 0.993160340131104
-0.469816998753579 1.14817439427199
-0.449864046356524 1.16080926697883
0.0501359536434758 1.27829936002577
0.496626409903306 1.14817439427199
0.550135953643476 1.13952068075061
1.05013595364348 0.894092001036142
1.28302847942902 0.648174394271988
1.40706637028201 0.148174394271988
1.35166341669758 -0.351825605728012
1.13820088548993 -0.851825605728012
1.05013595364348 -1.02579523885782
0.874038305654979 -1.35182560572801
0.550135953643476 -1.80381721474241
0.0501359536434758 -1.75064190177402
-0.449864046356524 -1.48643947151419
-0.588679351959038 -1.35182560572801
};
\addplot [draw=none, fill opacity=0.8, fill=color1, forget plot]
table{%
x  y
-2.24691928397388 1.64817439427199
-1.94986404635652 2.00463645042387
-1.79406596272788 2.14817439427199
-1.94986404635652 2.14817439427199
-2.44986404635652 2.14817439427199
-2.44986404635652 1.64817439427199
-2.44986404635652 1.28036339202376
-2.24691928397388 1.64817439427199
};
\addplot [draw=none, fill opacity=0.8, fill=color1, forget plot]
table{%
x  y
2.05013595364348 1.44841319917069
2.05013595364348 1.64817439427199
2.05013595364348 2.14817439427199
1.56257961538885 2.14817439427199
1.94352454058394 1.64817439427199
2.05013595364348 1.44841319917069
};
\addplot [draw=none, fill opacity=0.8, fill=color2, forget plot]
table{%
x  y
0.550135953643476 -2.85182560572801
1.05013595364348 -2.85182560572801
1.55013595364348 -2.85182560572801
2.05013595364348 -2.85182560572801
2.05013595364348 -2.40766523675514
1.55013595364348 -2.36045359913171
1.50852492056687 -2.35182560572801
1.05013595364348 -2.2443246385385
0.550135953643476 -2.2342986727799
0.515399127540899 -2.35182560572801
0.0574875400142759 -2.85182560572801
0.550135953643476 -2.85182560572801
};
\addplot [draw=none, fill opacity=0.8, fill=color2, forget plot]
table{%
x  y
-0.449864046356524 -1.48643947151419
0.0501359536434758 -1.75064190177402
0.550135953643476 -1.80381721474241
0.874038305654979 -1.35182560572801
1.05013595364348 -1.02579523885782
1.13820088548993 -0.851825605728012
1.35166341669758 -0.351825605728012
1.40706637028201 0.148174394271988
1.28302847942902 0.648174394271988
1.05013595364348 0.894092001036142
0.550135953643476 1.13952068075061
0.496626409903306 1.14817439427199
0.0501359536434758 1.27829936002577
-0.449864046356524 1.16080926697883
-0.469816998753579 1.14817439427199
-0.949864046356524 0.993160340131104
-1.31985034988364 0.648174394271988
-1.44986404635652 0.269759250528547
-1.53102991188118 0.148174394271988
-1.44986404635652 -0.237189971016923
-1.44010653214624 -0.351825605728012
-1.22080773865843 -0.851825605728012
-0.949864046356524 -1.11882111202746
-0.588679351959038 -1.35182560572801
-0.449864046356524 -1.48643947151419

-0.237620683780422 -1.35182560572801
-0.449864046356524 -1.26677725904593
-0.949864046356524 -0.918570239506223
-1.01759566389515 -0.851825605728012
-1.3051652459132 -0.351825605728012
-1.34523880714743 0.148174394271988
-1.14799865341099 0.648174394271988
-0.949864046356524 0.832920840749834
-0.449864046356524 1.0257035405469
0.0501359536434758 1.0824398087346
0.550135953643476 1.0002157436361
1.03259150837149 0.648174394271988
1.05013595364348 0.616606784971125
1.2560605874425 0.148174394271988
1.19498656950785 -0.351825605728012
1.05013595364348 -0.640485502665451
0.939862426419254 -0.851825605728012
0.583232113238505 -1.35182560572801
0.550135953643476 -1.39800985334046
0.0501359536434758 -1.52267967166661
-0.237620683780422 -1.35182560572801
};
\addplot [draw=none, fill opacity=0.8, fill=color3, forget plot]
table{%
x  y
0.0501359536434758 -1.52267967166661
0.550135953643476 -1.39800985334046
0.583232113238505 -1.35182560572801
0.939862426419254 -0.851825605728012
1.05013595364348 -0.640485502665451
1.19498656950785 -0.351825605728012
1.2560605874425 0.148174394271988
1.05013595364348 0.616606784971125
1.03259150837149 0.648174394271988
0.550135953643476 1.0002157436361
0.0501359536434758 1.0824398087346
-0.449864046356524 1.0257035405469
-0.949864046356524 0.832920840749834
-1.14799865341099 0.648174394271988
-1.34523880714743 0.148174394271988
-1.3051652459132 -0.351825605728012
-1.01759566389515 -0.851825605728012
-0.949864046356524 -0.918570239506223
-0.449864046356524 -1.26677725904593
-0.237620683780422 -1.35182560572801
0.0501359536434758 -1.52267967166661

-0.808844024741433 -0.851825605728012
-0.949864046356524 -0.706873071310166
-1.17022395968016 -0.351825605728012
-1.20701414719621 0.148174394271988
-0.976146956938335 0.648174394271988
-0.949864046356524 0.672681341368564
-0.449864046356524 0.898101935128969
0.0501359536434758 0.945963983330508
0.550135953643476 0.86091080652159
0.841680864399329 0.648174394271988
1.05013595364348 0.273102471961433
1.10505480460299 0.148174394271988
1.05013595364348 -0.265888619043896
1.03422906431598 -0.351825605728012
0.776947723366155 -0.851825605728012
0.550135953643476 -1.15734914384067
0.0501359536434758 -1.29809695738884
-0.449864046356524 -1.11292825602916
-0.808844024741433 -0.851825605728012
};
\addplot [draw=none, fill opacity=0.8, fill=color4, forget plot]
table{%
x  y
-0.449864046356524 -1.11292825602916
0.0501359536434758 -1.29809695738884
0.550135953643476 -1.15734914384067
0.776947723366155 -0.851825605728012
1.03422906431598 -0.351825605728012
1.05013595364348 -0.265888619043896
1.10505480460299 0.148174394271988
1.05013595364348 0.273102471961433
0.841680864399329 0.648174394271988
0.550135953643476 0.86091080652159
0.0501359536434758 0.945963983330508
-0.449864046356524 0.898101935128969
-0.949864046356524 0.672681341368564
-0.976146956938335 0.648174394271988
-1.20701414719621 0.148174394271988
-1.17022395968016 -0.351825605728012
-0.949864046356524 -0.706873071310166
-0.808844024741433 -0.851825605728012
-0.449864046356524 -1.11292825602916

-0.597322955484579 -0.851825605728012
-0.949864046356524 -0.489453482797831
-1.03528267344711 -0.351825605728012
-1.06878948724499 0.148174394271988
-0.949864046356524 0.400124300029099
-0.715314240921022 0.648174394271988
-0.449864046356524 0.770500329711043
0.0501359536434758 0.809488157926416
0.550135953643476 0.721605869407083
0.650770220427167 0.648174394271988
0.892187638454184 0.148174394271988
0.823490647328987 -0.351825605728012
0.614033020313057 -0.851825605728012
0.550135953643476 -0.937897232027566
0.0501359536434758 -1.08362495195285
-0.449864046356524 -0.959079253012399
-0.597322955484579 -0.851825605728012
};
\addplot [draw=none, fill opacity=0.8, fill=color5, forget plot]
table{%
x  y
-0.449864046356524 -0.959079253012399
0.0501359536434758 -1.08362495195285
0.550135953643476 -0.937897232027566
0.614033020313057 -0.851825605728012
0.823490647328987 -0.351825605728012
0.892187638454184 0.148174394271988
0.650770220427167 0.648174394271988
0.550135953643476 0.721605869407083
0.0501359536434758 0.809488157926416
-0.449864046356524 0.770500329711043
-0.715314240921022 0.648174394271988
-0.949864046356524 0.400124300029099
-1.06878948724499 0.148174394271988
-1.03528267344711 -0.351825605728012
-0.949864046356524 -0.489453482797831
-0.597322955484579 -0.851825605728012
-0.449864046356524 -0.959079253012399

-0.0551548813028045 -0.851825605728012
-0.449864046356524 -0.660129728927219
-0.735018949240088 -0.351825605728012
-0.845713685064629 0.148174394271988
-0.449864046356524 0.612034658327419
-0.357303701513763 0.648174394271988
0.0501359536434758 0.673012332522324
0.189091644451048 0.648174394271988
0.550135953643476 0.370297556021743
0.643963363657599 0.148174394271988
0.61275223034199 -0.351825605728012
0.550135953643476 -0.515999907733086
0.108800754017864 -0.851825605728012
0.0501359536434758 -0.869152946516858
-0.0551548813028045 -0.851825605728012
};
\addplot [draw=none, fill opacity=0.8, fill=color6, forget plot]
table{%
x  y
0.0501359536434758 -0.869152946516858
0.108800754017864 -0.851825605728012
0.550135953643476 -0.515999907733086
0.61275223034199 -0.351825605728012
0.643963363657599 0.148174394271988
0.550135953643476 0.370297556021743
0.189091644451048 0.648174394271988
0.0501359536434758 0.673012332522324
-0.357303701513763 0.648174394271988
-0.449864046356524 0.612034658327419
-0.845713685064629 0.148174394271988
-0.735018949240088 -0.351825605728012
-0.449864046356524 -0.660129728927219
-0.0551548813028045 -0.851825605728012
0.0501359536434758 -0.869152946516858
};
\addplot [draw=black, fill=blue, mark size=1pt, mark=*, only marks]
table{%
x  y
0.33752225331874 0.197215599662918
0.260077965357372 -0.406927805548534
-0.773609429793765 -0.212513547783295
-0.807079574249594 -0.380865556068029
-1.0205910920627 0.554601738061803
1.21402308025753 -0.00750315423552667
-1.05628487448876 -0.0824865078366188
-0.442280552428476 0.791419748748412
-0.409752816858336 -0.765731055588387
-0.585528746151917 0.284601639418142
0.73242037365367 0.753967323841675
0.60985187229186 0.232173856451722
-0.384486756723379 0.971418964692116
-1.10713613080998 -0.637211265145977
0.710197771775466 0.41754396299306
0.42445553982448 -1.47865265339901
0.540326693496342 -0.111359268813586
0.162613969058122 -0.181832134319311
-0.764294199801045 -0.0332403446358431
-0.0826362014312263 0.5631909059528
-0.0175515326578052 -0.84912994010713
-1.33428073110402 0.281345218895319
-0.0549592502901707 0.527424953403736
0.971422002312229 -0.269476308679372
-0.110244360797006 0.440228052752272
0.469401811362688 0.770603237194879
};
\addlegendentry{Training}
\addplot [draw=black, fill=red, mark size=1pt, mark=*, only marks]
table{%
x  y
-1.61490099633067 -0.741072910103641
0.287142882669433 2.02262720304501
-1.58856523177193 -0.803110885625336
-0.623983449298293 -1.93652964732585
-1.2405418624851 0.939444885393181
1.35407260107014 -0.769720325487996
-1.83769910459582 0.443816697159715
-0.765428478491238 -1.28950515507882
1.01551298232178 -0.541972483637455
1.56603301799072 -0.688597534702316
-1.03332383129373 0.849524554508094
-0.651914678744723 -1.46468158970865
0.0810731136748359 0.899802282864147
1.18865010038801 -0.739980958452245
1.55395518652147 -1.24199011248069
1.85121256073607 -0.00497500481773616
-0.389171170008798 1.22250793529749
1.60296587379039 0.604205195793129
-1.29848703826165 -0.0983469248924394
0.844105797736166 1.90774378297459
1.51105348805999 1.21666544960528
1.30539824445142 -1.5246576931366
-1.78357770670238 1.46776644856135
-0.077972864950725 -1.48563137737682
-1.94890625474126 0.926464116307055
-0.670106084565666 -2.35182560572801
1.26205437802023 1.08872015292522
-0.647447941667977 1.50066709495303
1.4921319124856 1.54360637568377
-1.32792377031717 0.083002609026316
0.40606432488658 1.46244545342365
1.1654875033266 0.420367176449525
-1.39691976001367 -1.16291726588525
-1.53382164587308 1.21058973257649
};
\addlegendentry{Unlabelled}
\addplot [draw=black, fill=red, forget plot, mark size=1pt, mark=*, only marks]
table{%
x  y
-1.18919052140229 1.0173422618081
1.86146485811385 1.22983792768625
0.732901091110239 -1.32784027183494
-1.02598963142284 -1.25200345428357
-1.94986404635652 -1.11164531070207
1.98413584116339 0.1150019145969
-0.225437938536809 1.3778895712398
1.67384249709114 -0.0400150659536265
-0.540831028697447 -1.45583732131862
0.238553355887223 1.6462348583095
0.290677752938808 -1.57114470390514
0.904528349207041 -1.27852393579202
-0.780714297973988 1.32218203431019
0.925638976557729 1.77824855581039
0.589189303449862 -1.8301536600317
-1.85060760097009 -1.32219895509989
};
\addplot [draw=black, fill=blue, forget plot, mark size=1pt, mark=*, only marks]
table{%
x  y
0.440304009157515 0.943608799128879
-0.969347691072044 -0.728792553962904
0.836887071549792 -0.542524638356252
0.421078225790276 -0.950756363125224
-0.647102455784015 -0.132485879001431
-0.806888775541198 -0.590378882138368
-0.176159089019397 1.37253857396961
-0.0787008638713176 0.754780205866068
0.372877527019 -0.656733964678869
1.24256422888301 -0.310609606127911
-0.0764451569750706 0.376737106094826
0.917285158870224 0.941922545575613
1.41852669557668 -0.246125819152755
-0.570326618188776 0.902761827769084
0.329109682743503 -0.884895230113077
-0.623655534584229 0.0597524918673479
0.0420013353840512 -1.1378377182301
-0.0501849415864134 -0.722268094294163
-0.25026012024578 0.802420320114215
0.309842560861943 0.471746720570786
0.133362529200736 -0.898586598985571
0.921338806365313 0.594024130338962
-0.762880574349996 -0.0702389129962407
0.450657848580996 -0.97869023698746
};
\end{axis}

\end{tikzpicture}


==> plots/fetch/constraint_loss_data.tex <==
\path [fill=color0, fill opacity=0.4, ultra thick]
(axis cs:0,237.925003051758)
--(axis cs:0,211.867477416992)
--(axis cs:100,261.10009765625)
--(axis cs:200,262.886291503906)
--(axis cs:300,264.170318603516)
--(axis cs:400,250.576416015625)
--(axis cs:500,42.0327339172363)
--(axis cs:600,8.49201679229736)
--(axis cs:700,6.70053720474243)
--(axis cs:800,5.01216506958008)
--(axis cs:900,5.6209602355957)
--(axis cs:1000,1.58914947509766)
--(axis cs:1100,2.20554208755493)
--(axis cs:1200,7.27553176879883)
--(axis cs:1300,18.8865242004395)
--(axis cs:1400,24.5383987426758)
--(axis cs:1500,25.6514453887939)
--(axis cs:1600,27.448802947998)
--(axis cs:1700,27.9536628723145)
--(axis cs:1800,36.5069351196289)
--(axis cs:1900,40.7017097473145)
--(axis cs:2000,51.571533203125)
--(axis cs:2100,57.1563720703125)
--(axis cs:2200,55.919921875)
--(axis cs:2300,49.2231636047363)
--(axis cs:2400,50.0492973327637)
--(axis cs:2500,49.9380569458008)
--(axis cs:2600,74.3858108520508)
--(axis cs:2700,95.0464477539062)
--(axis cs:2800,120.612426757812)
--(axis cs:2900,142.361602783203)
--(axis cs:3000,153.484115600586)
--(axis cs:3100,128.602340698242)
--(axis cs:3200,127.2255859375)
--(axis cs:3300,116.761131286621)
--(axis cs:3400,114.569725036621)
--(axis cs:3500,139.926849365234)
--(axis cs:3600,139.1123046875)
--(axis cs:3700,152.905471801758)
--(axis cs:3800,173.743255615234)
--(axis cs:3900,173.795211791992)
--(axis cs:4000,196.888641357422)
--(axis cs:4100,200.711715698242)
--(axis cs:4200,209.338851928711)
--(axis cs:4300,192.587890625)
--(axis cs:4400,196.642456054688)
--(axis cs:4500,201.365905761719)
--(axis cs:4600,235.114715576172)
--(axis cs:4700,267.549224853516)
--(axis cs:4800,287.324890136719)
--(axis cs:4900,305.640167236328)
--(axis cs:5000,286.992828369141)
--(axis cs:5100,279.767883300781)
--(axis cs:5200,266.716400146484)
--(axis cs:5300,279.102081298828)
--(axis cs:5400,269.178314208984)
--(axis cs:5500,268.493011474609)
--(axis cs:5600,296.209136962891)
--(axis cs:5700,270.897277832031)
--(axis cs:5800,253.700988769531)
--(axis cs:5900,245.279434204102)
--(axis cs:6000,244.083770751953)
--(axis cs:6100,250.990478515625)
--(axis cs:6200,267.476318359375)
--(axis cs:6300,289.775970458984)
--(axis cs:6400,320.691009521484)
--(axis cs:6500,367.428771972656)
--(axis cs:6600,371.674072265625)
--(axis cs:6700,380.967041015625)
--(axis cs:6800,390.760345458984)
--(axis cs:6900,384.492889404297)
--(axis cs:7000,377.940002441406)
--(axis cs:7100,380.7158203125)
--(axis cs:7200,357.402374267578)
--(axis cs:7300,348.420562744141)
--(axis cs:7400,338.81591796875)
--(axis cs:7500,347.926788330078)
--(axis cs:7600,349.229766845703)
--(axis cs:7700,351.05419921875)
--(axis cs:7800,373.931243896484)
--(axis cs:7900,339.962554931641)
--(axis cs:8000,301.172424316406)
--(axis cs:8100,286.989044189453)
--(axis cs:8200,266.140869140625)
--(axis cs:8300,249.476959228516)
--(axis cs:8400,241.918914794922)
--(axis cs:8500,243.216400146484)
--(axis cs:8600,227.677200317383)
--(axis cs:8700,240.705856323242)
--(axis cs:8800,232.158203125)
--(axis cs:8900,250.845336914062)
--(axis cs:9000,251.595260620117)
--(axis cs:9100,252.255874633789)
--(axis cs:9200,254.892929077148)
--(axis cs:9300,248.598831176758)
--(axis cs:9400,265.6015625)
--(axis cs:9500,259.362609863281)
--(axis cs:9600,263.972106933594)
--(axis cs:9700,269.340667724609)
--(axis cs:9800,267.110595703125)
--(axis cs:9900,252.569519042969)
--(axis cs:10000,242.525619506836)
--(axis cs:10100,248.816482543945)
--(axis cs:10200,258.380310058594)
--(axis cs:10300,268.520355224609)
--(axis cs:10400,267.990142822266)
--(axis cs:10500,292.061828613281)
--(axis cs:10600,287.885040283203)
--(axis cs:10700,305.611541748047)
--(axis cs:10800,332.221557617188)
--(axis cs:10900,331.977416992188)
--(axis cs:11000,333.077209472656)
--(axis cs:11100,325.018371582031)
--(axis cs:11200,297.157897949219)
--(axis cs:11300,289.728485107422)
--(axis cs:11400,294.464263916016)
--(axis cs:11500,311.208190917969)
--(axis cs:11600,338.119537353516)
--(axis cs:11700,329.016662597656)
--(axis cs:11800,321.089263916016)
--(axis cs:11900,310.486999511719)
--(axis cs:12000,289.543518066406)
--(axis cs:12100,245.758865356445)
--(axis cs:12200,233.767761230469)
--(axis cs:12300,224.598876953125)
--(axis cs:12400,226.233612060547)
--(axis cs:12500,220.864166259766)
--(axis cs:12600,227.955490112305)
--(axis cs:12700,238.660308837891)
--(axis cs:12800,242.254653930664)
--(axis cs:12900,243.898971557617)
--(axis cs:13000,239.410293579102)
--(axis cs:13100,234.766128540039)
--(axis cs:13200,228.69921875)
--(axis cs:13300,246.186050415039)
--(axis cs:13400,242.430404663086)
--(axis cs:13500,250.6484375)
--(axis cs:13600,245.861877441406)
--(axis cs:13700,227.515487670898)
--(axis cs:13800,235.252349853516)
--(axis cs:13900,228.483596801758)
--(axis cs:14000,228.192962646484)
--(axis cs:14100,246.778121948242)
--(axis cs:14200,247.583587646484)
--(axis cs:14300,268.993743896484)
--(axis cs:14400,269.806060791016)
--(axis cs:14500,263.996887207031)
--(axis cs:14600,232.641876220703)
--(axis cs:14700,211.809677124023)
--(axis cs:14800,210.583709716797)
--(axis cs:14900,215.782806396484)
--(axis cs:15000,208.26513671875)
--(axis cs:15100,202.674713134766)
--(axis cs:15200,223.060623168945)
--(axis cs:15300,234.86003112793)
--(axis cs:15400,252.891403198242)
--(axis cs:15500,252.021881103516)
--(axis cs:15600,252.737503051758)
--(axis cs:15700,243.077346801758)
--(axis cs:15800,240.858596801758)
--(axis cs:15900,240.606262207031)
--(axis cs:16000,253.314056396484)
--(axis cs:16100,247.667190551758)
--(axis cs:16200,245.511352539062)
--(axis cs:16300,239.692123413086)
--(axis cs:16400,239.402252197266)
--(axis cs:16500,268.3828125)
--(axis cs:16600,259.651550292969)
--(axis cs:16700,261.959381103516)
--(axis cs:16800,289.94921875)
--(axis cs:16900,310.45654296875)
--(axis cs:17000,297.407806396484)
--(axis cs:17100,309.493011474609)
--(axis cs:17200,296.561706542969)
--(axis cs:17300,286.059387207031)
--(axis cs:17400,271.989837646484)
--(axis cs:17500,257.9140625)
--(axis cs:17600,246.754531860352)
--(axis cs:17700,246.188720703125)
--(axis cs:17800,236.026473999023)
--(axis cs:17900,227.731918334961)
--(axis cs:18000,216.261016845703)
--(axis cs:18100,204.853118896484)
--(axis cs:18200,215.9599609375)
--(axis cs:18300,231.124389648438)
--(axis cs:18400,232.56591796875)
--(axis cs:18500,261.956451416016)
--(axis cs:18600,285.498809814453)
--(axis cs:18700,305.319702148438)
--(axis cs:18800,303.158935546875)
--(axis cs:18900,285.684265136719)
--(axis cs:19000,255.546615600586)
--(axis cs:19100,246.903244018555)
--(axis cs:19200,252.369934082031)
--(axis cs:19300,282.061706542969)
--(axis cs:19400,286.267913818359)
--(axis cs:19500,286.360931396484)
--(axis cs:19600,271.086700439453)
--(axis cs:19700,238.127166748047)
--(axis cs:19800,203.004486083984)
--(axis cs:19900,194.085052490234)
--(axis cs:20000,206.0341796875)
--(axis cs:20100,211.15234375)
--(axis cs:20200,221.022659301758)
--(axis cs:20300,225.532028198242)
--(axis cs:20400,230.149993896484)
--(axis cs:20500,213.61328125)
--(axis cs:20600,216.249435424805)
--(axis cs:20700,207.887634277344)
--(axis cs:20800,210.308471679688)
--(axis cs:20900,209.821426391602)
--(axis cs:21000,222.740509033203)
--(axis cs:21100,237.649780273438)
--(axis cs:21200,254.386932373047)
--(axis cs:21300,258.989898681641)
--(axis cs:21400,255.463623046875)
--(axis cs:21500,239.509536743164)
--(axis cs:21600,235.169494628906)
--(axis cs:21700,237.678115844727)
--(axis cs:21800,246.940628051758)
--(axis cs:21900,243.8486328125)
--(axis cs:22000,259.929412841797)
--(axis cs:22100,274.756469726562)
--(axis cs:22200,265.448913574219)
--(axis cs:22300,250.444488525391)
--(axis cs:22400,251.248199462891)
--(axis cs:22500,250.243957519531)
--(axis cs:22600,237.177780151367)
--(axis cs:22700,247.9453125)
--(axis cs:22800,252.951370239258)
--(axis cs:22900,260.182800292969)
--(axis cs:23000,258.938201904297)
--(axis cs:23100,257.724700927734)
--(axis cs:23200,263.081573486328)
--(axis cs:23300,266.703857421875)
--(axis cs:23400,263.668273925781)
--(axis cs:23500,261.455932617188)
--(axis cs:23600,284.378601074219)
--(axis cs:23700,285.6875)
--(axis cs:23800,285.6875)
--(axis cs:23900,285.6875)
--(axis cs:24000,285.6875)
--(axis cs:24100,285.6875)
--(axis cs:24200,285.932098388672)
--(axis cs:24300,285.873718261719)
--(axis cs:24400,285.6875)
--(axis cs:24500,285.769714355469)
--(axis cs:24600,285.6875)
--(axis cs:24700,285.6875)
--(axis cs:24800,285.6875)
--(axis cs:24900,285.6875)
--(axis cs:25000,285.6875)
--(axis cs:25100,285.6875)
--(axis cs:25200,285.6875)
--(axis cs:25300,285.6875)
--(axis cs:25400,285.6875)
--(axis cs:25500,285.6875)
--(axis cs:25600,285.6875)
--(axis cs:25700,285.6875)
--(axis cs:25800,285.6875)
--(axis cs:25900,285.6875)
--(axis cs:26000,285.6875)
--(axis cs:26100,285.6875)
--(axis cs:26200,285.6875)
--(axis cs:26300,285.6875)
--(axis cs:26400,285.6875)
--(axis cs:26500,285.6875)
--(axis cs:26600,285.6875)
--(axis cs:26700,285.6875)
--(axis cs:26800,274.797149658203)
--(axis cs:26900,269.342041015625)
--(axis cs:27000,268.369934082031)
--(axis cs:27100,272.777191162109)
--(axis cs:27200,285.6875)
--(axis cs:27300,285.6875)
--(axis cs:27400,285.6875)
--(axis cs:27500,285.6875)
--(axis cs:27600,285.6875)
--(axis cs:27700,285.6875)
--(axis cs:27800,285.6875)
--(axis cs:27900,285.6875)
--(axis cs:28000,285.6875)
--(axis cs:28100,285.6875)
--(axis cs:28200,285.6875)
--(axis cs:28300,285.6875)
--(axis cs:28400,285.6875)
--(axis cs:28500,285.6875)
--(axis cs:28600,285.6875)
--(axis cs:28700,285.6875)
--(axis cs:28800,285.6875)
--(axis cs:28900,285.6875)
--(axis cs:29000,285.6875)
--(axis cs:29100,285.6875)
--(axis cs:29200,285.6875)
--(axis cs:29300,285.6875)
--(axis cs:29400,285.6875)
--(axis cs:29500,285.6875)
--(axis cs:29600,285.6875)
--(axis cs:29700,285.6875)
--(axis cs:29800,285.6875)
--(axis cs:29900,285.6875)
--(axis cs:30000,285.6875)
--(axis cs:30100,285.6875)
--(axis cs:30200,285.6875)
--(axis cs:30300,285.6875)
--(axis cs:30400,285.6875)
--(axis cs:30500,285.6875)
--(axis cs:30600,285.6875)
--(axis cs:30700,285.6875)
--(axis cs:30800,285.6875)
--(axis cs:30900,285.6875)
--(axis cs:31000,285.6875)
--(axis cs:31100,285.6875)
--(axis cs:31200,285.6875)
--(axis cs:31300,285.6875)
--(axis cs:31400,285.6875)
--(axis cs:31500,285.6875)
--(axis cs:31600,285.6875)
--(axis cs:31700,285.6875)
--(axis cs:31800,285.6875)
--(axis cs:31900,285.6875)
--(axis cs:32000,285.6875)
--(axis cs:32100,285.6875)
--(axis cs:32200,285.6875)
--(axis cs:32300,285.6875)
--(axis cs:32400,285.6875)
--(axis cs:32500,285.6875)
--(axis cs:32600,285.6875)
--(axis cs:32700,285.6875)
--(axis cs:32800,285.6875)
--(axis cs:32900,285.6875)
--(axis cs:33000,285.6875)
--(axis cs:33100,285.6875)
--(axis cs:33200,285.6875)
--(axis cs:33300,285.6875)
--(axis cs:33400,285.6875)
--(axis cs:33500,285.6875)
--(axis cs:33600,285.6875)
--(axis cs:33700,285.6875)
--(axis cs:33800,285.6875)
--(axis cs:33900,285.6875)
--(axis cs:34000,285.6875)
--(axis cs:34100,285.6875)
--(axis cs:34200,285.6875)
--(axis cs:34300,285.6875)
--(axis cs:34300,423.303894042969)
--(axis cs:34300,423.303894042969)
--(axis cs:34200,426.1103515625)
--(axis cs:34100,447.194183349609)
--(axis cs:34000,454.480743408203)
--(axis cs:33900,453.176849365234)
--(axis cs:33800,449.891296386719)
--(axis cs:33700,440.137725830078)
--(axis cs:33600,417.440765380859)
--(axis cs:33500,400.848449707031)
--(axis cs:33400,403.414764404297)
--(axis cs:33300,397.858459472656)
--(axis cs:33200,402.381195068359)
--(axis cs:33100,395.231811523438)
--(axis cs:33000,418.085815429688)
--(axis cs:32900,426.741577148438)
--(axis cs:32800,443.639556884766)
--(axis cs:32700,447.576416015625)
--(axis cs:32600,451.904357910156)
--(axis cs:32500,428.763458251953)
--(axis cs:32400,411.598968505859)
--(axis cs:32300,385.782745361328)
--(axis cs:32200,380.465362548828)
--(axis cs:32100,372.159301757812)
--(axis cs:32000,376.937255859375)
--(axis cs:31900,390.487762451172)
--(axis cs:31800,393.432495117188)
--(axis cs:31700,393.844909667969)
--(axis cs:31600,406.589630126953)
--(axis cs:31500,415.806213378906)
--(axis cs:31400,407.352844238281)
--(axis cs:31300,409.271606445312)
--(axis cs:31200,400.725250244141)
--(axis cs:31100,378.241119384766)
--(axis cs:31000,362.846252441406)
--(axis cs:30900,374.049133300781)
--(axis cs:30800,385.992706298828)
--(axis cs:30700,388.165405273438)
--(axis cs:30600,407.340270996094)
--(axis cs:30500,405.955902099609)
--(axis cs:30400,420.927459716797)
--(axis cs:30300,420.116455078125)
--(axis cs:30200,421.469421386719)
--(axis cs:30100,405.439147949219)
--(axis cs:30000,395.42041015625)
--(axis cs:29900,360.395690917969)
--(axis cs:29800,341.53125)
--(axis cs:29700,336.831695556641)
--(axis cs:29600,324.767852783203)
--(axis cs:29500,317.884307861328)
--(axis cs:29400,314.407745361328)
--(axis cs:29300,314.092254638672)
--(axis cs:29200,308.791564941406)
--(axis cs:29100,325.811248779297)
--(axis cs:29000,349.921081542969)
--(axis cs:28900,380.364807128906)
--(axis cs:28800,384.231170654297)
--(axis cs:28700,400.120452880859)
--(axis cs:28600,421.600158691406)
--(axis cs:28500,426.593231201172)
--(axis cs:28400,399.029052734375)
--(axis cs:28300,403.903839111328)
--(axis cs:28200,394.860870361328)
--(axis cs:28100,372.686157226562)
--(axis cs:28000,346.086364746094)
--(axis cs:27900,344.776275634766)
--(axis cs:27800,346.005859375)
--(axis cs:27700,341.035919189453)
--(axis cs:27600,344.290985107422)
--(axis cs:27500,336.118835449219)
--(axis cs:27400,329.934692382812)
--(axis cs:27300,313.548065185547)
--(axis cs:27200,300.628784179688)
--(axis cs:27100,287.2578125)
--(axis cs:27000,287.2578125)
--(axis cs:26900,287.2578125)
--(axis cs:26800,287.2578125)
--(axis cs:26700,295.732971191406)
--(axis cs:26600,321.601257324219)
--(axis cs:26500,340.592132568359)
--(axis cs:26400,338.689880371094)
--(axis cs:26300,340.038909912109)
--(axis cs:26200,335.466339111328)
--(axis cs:26100,315.330261230469)
--(axis cs:26000,302.696563720703)
--(axis cs:25900,306.469696044922)
--(axis cs:25800,309.546752929688)
--(axis cs:25700,310.959197998047)
--(axis cs:25600,325.657867431641)
--(axis cs:25500,342.846374511719)
--(axis cs:25400,345.069213867188)
--(axis cs:25300,349.711120605469)
--(axis cs:25200,347.238037109375)
--(axis cs:25100,361.294708251953)
--(axis cs:25000,358.025665283203)
--(axis cs:24900,343.165710449219)
--(axis cs:24800,328.155792236328)
--(axis cs:24700,321.509490966797)
--(axis cs:24600,300.238403320312)
--(axis cs:24500,290.101135253906)
--(axis cs:24400,298.841796875)
--(axis cs:24300,289.376831054688)
--(axis cs:24200,288.927276611328)
--(axis cs:24100,292.501098632812)
--(axis cs:24000,307.531951904297)
--(axis cs:23900,300.203918457031)
--(axis cs:23800,302.109527587891)
--(axis cs:23700,298.977294921875)
--(axis cs:23600,286.972961425781)
--(axis cs:23500,287.259368896484)
--(axis cs:23400,287.260162353516)
--(axis cs:23300,287.260925292969)
--(axis cs:23200,287.26171875)
--(axis cs:23100,287.26171875)
--(axis cs:23000,284.798797607422)
--(axis cs:22900,282.794311523438)
--(axis cs:22800,285.949157714844)
--(axis cs:22700,287.26171875)
--(axis cs:22600,302.432037353516)
--(axis cs:22500,314.482055664062)
--(axis cs:22400,321.604400634766)
--(axis cs:22300,325.252960205078)
--(axis cs:22200,319.682037353516)
--(axis cs:22100,334.602355957031)
--(axis cs:22000,332.938323974609)
--(axis cs:21900,316.407043457031)
--(axis cs:21800,312.165740966797)
--(axis cs:21700,287.209899902344)
--(axis cs:21600,265.375)
--(axis cs:21500,275.420166015625)
--(axis cs:21400,273.435150146484)
--(axis cs:21300,266.299163818359)
--(axis cs:21200,281.853912353516)
--(axis cs:21100,287.825775146484)
--(axis cs:21000,297.366394042969)
--(axis cs:20900,306.028900146484)
--(axis cs:20800,301.384368896484)
--(axis cs:20700,287.578918457031)
--(axis cs:20600,293.21826171875)
--(axis cs:20500,279.391326904297)
--(axis cs:20400,273.23193359375)
--(axis cs:20300,271.995758056641)
--(axis cs:20200,279.98583984375)
--(axis cs:20100,282.037780761719)
--(axis cs:20000,290.362152099609)
--(axis cs:19900,297.908142089844)
--(axis cs:19800,321.540863037109)
--(axis cs:19700,312.855682373047)
--(axis cs:19600,322.525299072266)
--(axis cs:19500,329.427642822266)
--(axis cs:19400,330.453460693359)
--(axis cs:19300,318.516967773438)
--(axis cs:19200,322.565490722656)
--(axis cs:19100,326.964996337891)
--(axis cs:19000,319.727355957031)
--(axis cs:18900,338.8359375)
--(axis cs:18800,321.98583984375)
--(axis cs:18700,324.135162353516)
--(axis cs:18600,319.84765625)
--(axis cs:18500,322.227355957031)
--(axis cs:18400,328.284118652344)
--(axis cs:18300,307.211547851562)
--(axis cs:18200,295.89892578125)
--(axis cs:18100,297.737945556641)
--(axis cs:18000,299.992645263672)
--(axis cs:17900,294.327453613281)
--(axis cs:17800,304.335021972656)
--(axis cs:17700,331.684753417969)
--(axis cs:17600,349.946472167969)
--(axis cs:17500,333.514007568359)
--(axis cs:17400,323.348358154297)
--(axis cs:17300,332.954315185547)
--(axis cs:17200,331.974945068359)
--(axis cs:17100,318.535125732422)
--(axis cs:17000,317.773529052734)
--(axis cs:16900,332.32421875)
--(axis cs:16800,346.114471435547)
--(axis cs:16700,351.121490478516)
--(axis cs:16600,338.334228515625)
--(axis cs:16500,336.270812988281)
--(axis cs:16400,320.193572998047)
--(axis cs:16300,299.598480224609)
--(axis cs:16200,298.365783691406)
--(axis cs:16100,300.647644042969)
--(axis cs:16000,287.111328125)
--(axis cs:15900,279.617980957031)
--(axis cs:15800,289.385467529297)
--(axis cs:15700,282.564117431641)
--(axis cs:15600,302.230926513672)
--(axis cs:15500,310.106811523438)
--(axis cs:15400,305.464324951172)
--(axis cs:15300,290.171722412109)
--(axis cs:15200,276.847198486328)
--(axis cs:15100,255.845306396484)
--(axis cs:15000,243.896331787109)
--(axis cs:14900,261.492706298828)
--(axis cs:14800,295.735534667969)
--(axis cs:14700,320.909606933594)
--(axis cs:14600,326.273223876953)
--(axis cs:14500,316.463134765625)
--(axis cs:14400,302.500762939453)
--(axis cs:14300,306.286071777344)
--(axis cs:14200,333.935791015625)
--(axis cs:14100,340.712005615234)
--(axis cs:14000,336.438293457031)
--(axis cs:13900,331.115356445312)
--(axis cs:13800,321.774047851562)
--(axis cs:13700,313.203247070312)
--(axis cs:13600,295.786560058594)
--(axis cs:13500,273.373565673828)
--(axis cs:13400,265.134704589844)
--(axis cs:13300,249.544525146484)
--(axis cs:13200,255.209487915039)
--(axis cs:13100,259.443237304688)
--(axis cs:13000,270.556243896484)
--(axis cs:12900,293.8828125)
--(axis cs:12800,299.880859375)
--(axis cs:12700,326.412506103516)
--(axis cs:12600,318.673828125)
--(axis cs:12500,324.419525146484)
--(axis cs:12400,321.278900146484)
--(axis cs:12300,338.112884521484)
--(axis cs:12200,322.028076171875)
--(axis cs:12100,339.405975341797)
--(axis cs:12000,333.503356933594)
--(axis cs:11900,355.829895019531)
--(axis cs:11800,355.744140625)
--(axis cs:11700,380.437744140625)
--(axis cs:11600,361.261627197266)
--(axis cs:11500,358.161529541016)
--(axis cs:11400,350.674835205078)
--(axis cs:11300,356.474395751953)
--(axis cs:11200,348.189453125)
--(axis cs:11100,350.110931396484)
--(axis cs:11000,352.801696777344)
--(axis cs:10900,352.771484375)
--(axis cs:10800,344.261779785156)
--(axis cs:10700,364.205871582031)
--(axis cs:10600,401.819366455078)
--(axis cs:10500,444.548034667969)
--(axis cs:10400,461.614074707031)
--(axis cs:10300,474.380859375)
--(axis cs:10200,522.602355957031)
--(axis cs:10100,534.526245117188)
--(axis cs:10000,492.624206542969)
--(axis cs:9900,468.660949707031)
--(axis cs:9800,460.585144042969)
--(axis cs:9700,383.435943603516)
--(axis cs:9600,361.928527832031)
--(axis cs:9500,327.735168457031)
--(axis cs:9400,325.326568603516)
--(axis cs:9300,301.502502441406)
--(axis cs:9200,312.359161376953)
--(axis cs:9100,318.175964355469)
--(axis cs:9000,312.702911376953)
--(axis cs:8900,297.044006347656)
--(axis cs:8800,297.390197753906)
--(axis cs:8700,257.573120117188)
--(axis cs:8600,237.922271728516)
--(axis cs:8500,258.31640625)
--(axis cs:8400,287.350860595703)
--(axis cs:8300,290.197601318359)
--(axis cs:8200,333.932800292969)
--(axis cs:8100,365.895690917969)
--(axis cs:8000,381.023315429688)
--(axis cs:7900,363.215240478516)
--(axis cs:7800,388.418853759766)
--(axis cs:7700,448.563293457031)
--(axis cs:7600,502.245147705078)
--(axis cs:7500,526.680847167969)
--(axis cs:7400,533.376159667969)
--(axis cs:7300,523.060852050781)
--(axis cs:7200,509.383087158203)
--(axis cs:7100,477.540344238281)
--(axis cs:7000,497.174560546875)
--(axis cs:6900,525.52734375)
--(axis cs:6800,537.726196289062)
--(axis cs:6700,507.900207519531)
--(axis cs:6600,463.028503417969)
--(axis cs:6500,430.086059570312)
--(axis cs:6400,420.608032226562)
--(axis cs:6300,368.781890869141)
--(axis cs:6200,366.047302246094)
--(axis cs:6100,365.952545166016)
--(axis cs:6000,403.075103759766)
--(axis cs:5900,421.165222167969)
--(axis cs:5800,412.1591796875)
--(axis cs:5700,433.427124023438)
--(axis cs:5600,419.231781005859)
--(axis cs:5500,372.352722167969)
--(axis cs:5400,345.239074707031)
--(axis cs:5300,359.612609863281)
--(axis cs:5200,313.469635009766)
--(axis cs:5100,313.383087158203)
--(axis cs:5000,330.706390380859)
--(axis cs:4900,337.056304931641)
--(axis cs:4800,331.103881835938)
--(axis cs:4700,358.553955078125)
--(axis cs:4600,356.223663330078)
--(axis cs:4500,361.139068603516)
--(axis cs:4400,380.112731933594)
--(axis cs:4300,368.809509277344)
--(axis cs:4200,305.40673828125)
--(axis cs:4100,316.763366699219)
--(axis cs:4000,322.122833251953)
--(axis cs:3900,334.707702636719)
--(axis cs:3800,365.058410644531)
--(axis cs:3700,365.880920410156)
--(axis cs:3600,328.037231445312)
--(axis cs:3500,278.644287109375)
--(axis cs:3400,224.760604858398)
--(axis cs:3300,191.840270996094)
--(axis cs:3200,181.021011352539)
--(axis cs:3100,204.642532348633)
--(axis cs:3000,220.413558959961)
--(axis cs:2900,218.617645263672)
--(axis cs:2800,199.951293945312)
--(axis cs:2700,196.722106933594)
--(axis cs:2600,184.029632568359)
--(axis cs:2500,160.153564453125)
--(axis cs:2400,160.087005615234)
--(axis cs:2300,144.508728027344)
--(axis cs:2200,149.102935791016)
--(axis cs:2100,123.597869873047)
--(axis cs:2000,113.937240600586)
--(axis cs:1900,99.9110794067383)
--(axis cs:1800,93.7909088134766)
--(axis cs:1700,79.0804672241211)
--(axis cs:1600,73.0702285766602)
--(axis cs:1500,70.9086151123047)
--(axis cs:1400,94.2665328979492)
--(axis cs:1300,90.9848937988281)
--(axis cs:1200,100.095748901367)
--(axis cs:1100,104.388732910156)
--(axis cs:1000,96.9970092773438)
--(axis cs:900,62.9253273010254)
--(axis cs:800,60.1164665222168)
--(axis cs:700,56.8890686035156)
--(axis cs:600,63.3722305297852)
--(axis cs:500,100.656539916992)
--(axis cs:400,310.820098876953)
--(axis cs:300,322.988311767578)
--(axis cs:200,306.850463867188)
--(axis cs:100,286.942504882812)
--(axis cs:0,237.925003051758)
--cycle;

\path [fill=white!40.1960784313725!black, fill opacity=0.4, ultra thick]
(axis cs:0,0.00546552613377571)
--(axis cs:0,0.00483751576393843)
--(axis cs:100,0.00483698956668377)
--(axis cs:200,0.00271829543635249)
--(axis cs:300,0.000903920852579176)
--(axis cs:400,6.10426059211022e-06)
--(axis cs:500,0)
--(axis cs:600,0)
--(axis cs:700,0)
--(axis cs:800,0)
--(axis cs:900,1.67334255820606e-05)
--(axis cs:1000,8.72332602739334e-05)
--(axis cs:1100,8.72332602739334e-05)
--(axis cs:1200,0.000130596759845503)
--(axis cs:1300,0.000191313039977103)
--(axis cs:1400,0.000166424026247114)
--(axis cs:1500,0.000149114988744259)
--(axis cs:1600,0.000694442540407181)
--(axis cs:1700,0.000593376404140145)
--(axis cs:1800,0.000740136136300862)
--(axis cs:1900,0.000910972594283521)
--(axis cs:2000,0.00115554046351463)
--(axis cs:2100,0.000687542837113142)
--(axis cs:2200,0.0013356547569856)
--(axis cs:2300,0.000495161104481667)
--(axis cs:2400,0.000901719904504716)
--(axis cs:2500,0.000662741076666862)
--(axis cs:2600,0.000930432230234146)
--(axis cs:2700,0.00092057790607214)
--(axis cs:2800,0.00213234964758158)
--(axis cs:2900,0.00220429827459157)
--(axis cs:3000,0.00167833059094846)
--(axis cs:3100,0.00168134330306202)
--(axis cs:3200,0.00222564116120338)
--(axis cs:3300,0.00168862869031727)
--(axis cs:3400,0.00132358376868069)
--(axis cs:3500,0.00168128393124789)
--(axis cs:3600,0.00169371941592544)
--(axis cs:3700,0.00126785563770682)
--(axis cs:3800,0.00104487361386418)
--(axis cs:3900,0.00144222029484808)
--(axis cs:4000,0.00341570097953081)
--(axis cs:4100,0.00186446949373931)
--(axis cs:4200,0.00308691547252238)
--(axis cs:4300,0.002515465952456)
--(axis cs:4400,0.000986131140962243)
--(axis cs:4500,0.000595399062149227)
--(axis cs:4600,0.000737183494493365)
--(axis cs:4700,0.000612314732279629)
--(axis cs:4800,0.000978122581727803)
--(axis cs:4900,0.000997256487607956)
--(axis cs:5000,0.00105053244624287)
--(axis cs:5100,0.0010830641258508)
--(axis cs:5200,0.00166286085732281)
--(axis cs:5300,0.00133092363830656)
--(axis cs:5400,0.00143646053038538)
--(axis cs:5500,0.00201174290850759)
--(axis cs:5600,0.00213901605457067)
--(axis cs:5700,0.00149803597014397)
--(axis cs:5800,0.00236350880004466)
--(axis cs:5900,0.00192027376033366)
--(axis cs:6000,0.00150494265835732)
--(axis cs:6100,0.00276569416746497)
--(axis cs:6200,0.00299112359061837)
--(axis cs:6300,0.00239076768048108)
--(axis cs:6400,0.00338934501633048)
--(axis cs:6500,0.00337997521273792)
--(axis cs:6600,0.00196414301171899)
--(axis cs:6700,0.0019818632863462)
--(axis cs:6800,0.00218252534978092)
--(axis cs:6900,0.0013943666126579)
--(axis cs:7000,0.0027922778390348)
--(axis cs:7100,0.00435074558481574)
--(axis cs:7200,0.00452185655012727)
--(axis cs:7300,0.00533555448055267)
--(axis cs:7400,0.00214294088073075)
--(axis cs:7500,0.00293785729445517)
--(axis cs:7600,0.00284295971505344)
--(axis cs:7700,0.00272319605574012)
--(axis cs:7800,0.00262545933946967)
--(axis cs:7900,0.0018497024429962)
--(axis cs:8000,0.00130684673786163)
--(axis cs:8100,0.00141834549140185)
--(axis cs:8200,0.00184761837590486)
--(axis cs:8300,0.00211975281126797)
--(axis cs:8400,0.00209931377321482)
--(axis cs:8500,0.00178852677345276)
--(axis cs:8600,0.00241603259928524)
--(axis cs:8700,0.00189135072287172)
--(axis cs:8800,0.00188021757639945)
--(axis cs:8900,0.00384205020964146)
--(axis cs:9000,0.00416135555133224)
--(axis cs:9100,0.00387640669941902)
--(axis cs:9200,0.00507509708404541)
--(axis cs:9300,0.0036198329180479)
--(axis cs:9400,0.00233557214960456)
--(axis cs:9500,0.00245482753962278)
--(axis cs:9600,0.00192187773063779)
--(axis cs:9700,0.00183289649430662)
--(axis cs:9800,0.00195123453158885)
--(axis cs:9900,0.00113551015965641)
--(axis cs:10000,0.00103186967317015)
--(axis cs:10100,0.00237001175992191)
--(axis cs:10200,0.00203695590607822)
--(axis cs:10300,0.00358482031151652)
--(axis cs:10400,0.00296826963312924)
--(axis cs:10500,0.00314995343796909)
--(axis cs:10600,0.00276533956639469)
--(axis cs:10700,0.0026103975251317)
--(axis cs:10800,0.00124095077626407)
--(axis cs:10900,0.000994336558505893)
--(axis cs:11000,0.00172268750611693)
--(axis cs:11100,0.00222566118463874)
--(axis cs:11200,0.00243891472928226)
--(axis cs:11300,0.00285938964225352)
--(axis cs:11400,0.00296008097939193)
--(axis cs:11500,0.00243562995456159)
--(axis cs:11600,0.00163811119273305)
--(axis cs:11700,0.00220730691216886)
--(axis cs:11800,0.00183904636651278)
--(axis cs:11900,0.0022596896160394)
--(axis cs:12000,0.00233743595890701)
--(axis cs:12100,0.00299625401385128)
--(axis cs:12200,0.00432268995791674)
--(axis cs:12300,0.00276877102442086)
--(axis cs:12400,0.00276521313935518)
--(axis cs:12500,0.00378331495448947)
--(axis cs:12600,0.00338948960416019)
--(axis cs:12700,0.00293023604899645)
--(axis cs:12800,0.00308385118842125)
--(axis cs:12900,0.00309920916333795)
--(axis cs:13000,0.00258896639570594)
--(axis cs:13100,0.00249582529067993)
--(axis cs:13200,0.00244441628456116)
--(axis cs:13300,0.0023071407340467)
--(axis cs:13400,0.00345491315238178)
--(axis cs:13500,0.00344536988995969)
--(axis cs:13600,0.00355582241900265)
--(axis cs:13700,0.00340813770890236)
--(axis cs:13800,0.00353825464844704)
--(axis cs:13900,0.00303652859292924)
--(axis cs:14000,0.0030118846334517)
--(axis cs:14100,0.00288993725553155)
--(axis cs:14200,0.00419694511219859)
--(axis cs:14300,0.00325419893488288)
--(axis cs:14400,0.00293771037831903)
--(axis cs:14500,0.00266131572425365)
--(axis cs:14600,0.00294919102452695)
--(axis cs:14700,0.00174391525797546)
--(axis cs:14800,0.00249302503652871)
--(axis cs:14900,0.00234586698934436)
--(axis cs:15000,0.00203636894002557)
--(axis cs:15100,0.00197851657867432)
--(axis cs:15200,0.00426848279312253)
--(axis cs:15300,0.00371221313253045)
--(axis cs:15400,0.0042867548763752)
--(axis cs:15500,0.00355703826062381)
--(axis cs:15600,0.0035890459548682)
--(axis cs:15700,0.00240503158420324)
--(axis cs:15800,0.00283912662416697)
--(axis cs:15900,0.00273391371592879)
--(axis cs:16000,0.00262057385407388)
--(axis cs:16100,0.00256977090612054)
--(axis cs:16200,0.0023155331145972)
--(axis cs:16300,0.00133770704269409)
--(axis cs:16400,0.00251871347427368)
--(axis cs:16500,0.00263789901509881)
--(axis cs:16600,0.00264016096480191)
--(axis cs:16700,0.00350009673275054)
--(axis cs:16800,0.00352751603350043)
--(axis cs:16900,0.00253958068788052)
--(axis cs:17000,0.00244067911989987)
--(axis cs:17100,0.00252106273546815)
--(axis cs:17200,0.00220823707059026)
--(axis cs:17300,0.00235371547751129)
--(axis cs:17400,0.00304657546803355)
--(axis cs:17500,0.00237484718672931)
--(axis cs:17600,0.00309207942336798)
--(axis cs:17700,0.00294109573587775)
--(axis cs:17800,0.00393783301115036)
--(axis cs:17900,0.00330180791206658)
--(axis cs:18000,0.00333225727081299)
--(axis cs:18100,0.00196844339370728)
--(axis cs:18200,0.00179911847226322)
--(axis cs:18300,0.00223048916086555)
--(axis cs:18400,0.00258115539327264)
--(axis cs:18500,0.00278441328555346)
--(axis cs:18600,0.00270497403107584)
--(axis cs:18700,0.00227294093929231)
--(axis cs:18800,0.0031800998840481)
--(axis cs:18900,0.00359323644079268)
--(axis cs:19000,0.00362445856444538)
--(axis cs:19100,0.00341089186258614)
--(axis cs:19200,0.00401407293975353)
--(axis cs:19300,0.00493527669459581)
--(axis cs:19400,0.00239985249936581)
--(axis cs:19500,0.00246105180121958)
--(axis cs:19600,0.00270561757497489)
--(axis cs:19700,0.00278289546258748)
--(axis cs:19800,0.00273652328178287)
--(axis cs:19900,0.00338268000632524)
--(axis cs:20000,0.00305422442033887)
--(axis cs:20100,0.00426567438989878)
--(axis cs:20200,0.00390973314642906)
--(axis cs:20300,0.0044286185875535)
--(axis cs:20400,0.00576056260615587)
--(axis cs:20500,0.00591312628239393)
--(axis cs:20600,0.00502048386260867)
--(axis cs:20700,0.00496227154508233)
--(axis cs:20800,0.00416136672720313)
--(axis cs:20900,0.00327011034823954)
--(axis cs:21000,0.00346823898144066)
--(axis cs:21100,0.00350130931474268)
--(axis cs:21200,0.00474364450201392)
--(axis cs:21300,0.00519083021208644)
--(axis cs:21400,0.00467483140528202)
--(axis cs:21500,0.00501247914507985)
--(axis cs:21600,0.00463953753933311)
--(axis cs:21700,0.00341665185987949)
--(axis cs:21800,0.00322266737930477)
--(axis cs:21900,0.00306874443776906)
--(axis cs:22000,0.00245116301812232)
--(axis cs:22100,0.00254172482527792)
--(axis cs:22200,0.0025615612976253)
--(axis cs:22300,0.00225329003296793)
--(axis cs:22400,0.00237437034957111)
--(axis cs:22500,0.00276885414496064)
--(axis cs:22600,0.00316216051578522)
--(axis cs:22700,0.00391185563057661)
--(axis cs:22800,0.0043192645534873)
--(axis cs:22900,0.00515468325465918)
--(axis cs:23000,0.00535854138433933)
--(axis cs:23100,0.00508613279089332)
--(axis cs:23200,0.00438877008855343)
--(axis cs:23300,0.00392786599695683)
--(axis cs:23400,0.0036476687528193)
--(axis cs:23500,0.00331310811452568)
--(axis cs:23600,0.00459592789411545)
--(axis cs:23700,0.00440153665840626)
--(axis cs:23800,0.00555700063705444)
--(axis cs:23900,0.00501228636130691)
--(axis cs:24000,0.00479469262063503)
--(axis cs:24100,0.00347996759228408)
--(axis cs:24200,0.00362211838364601)
--(axis cs:24300,0.00509118940681219)
--(axis cs:24400,0.0051051820628345)
--(axis cs:24500,0.00565676670521498)
--(axis cs:24600,0.00599058857187629)
--(axis cs:24700,0.00592584628611803)
--(axis cs:24800,0.00345480465330184)
--(axis cs:24900,0.00403713714331388)
--(axis cs:25000,0.00415077293291688)
--(axis cs:25100,0.00442524719983339)
--(axis cs:25200,0.00480891577899456)
--(axis cs:25300,0.00457455916330218)
--(axis cs:25400,0.00417455192655325)
--(axis cs:25500,0.00359273934736848)
--(axis cs:25600,0.00308434548787773)
--(axis cs:25700,0.00300519471056759)
--(axis cs:25800,0.00407980522140861)
--(axis cs:25900,0.00405621435493231)
--(axis cs:26000,0.00423480663448572)
--(axis cs:26100,0.00418767239898443)
--(axis cs:26200,0.00416082050651312)
--(axis cs:26300,0.00323889055289328)
--(axis cs:26400,0.0030115032568574)
--(axis cs:26500,0.00272920029237866)
--(axis cs:26600,0.00368376052938402)
--(axis cs:26700,0.00373112084344029)
--(axis cs:26800,0.00444256421178579)
--(axis cs:26900,0.00435787718743086)
--(axis cs:27000,0.00463553983718157)
--(axis cs:27100,0.00424590660259128)
--(axis cs:27200,0.00462279887869954)
--(axis cs:27300,0.00447339378297329)
--(axis cs:27400,0.00480052269995213)
--(axis cs:27500,0.00465881079435349)
--(axis cs:27600,0.00447263568639755)
--(axis cs:27700,0.00361617328599095)
--(axis cs:27800,0.00284483167342842)
--(axis cs:27900,0.00326508423313498)
--(axis cs:28000,0.00357314571738243)
--(axis cs:28100,0.00316453236155212)
--(axis cs:28100,0.00972661748528481)
--(axis cs:28100,0.00972661748528481)
--(axis cs:28000,0.00967986043542624)
--(axis cs:27900,0.00971476547420025)
--(axis cs:27800,0.00976560357958078)
--(axis cs:27700,0.0096751693636179)
--(axis cs:27600,0.00959421973675489)
--(axis cs:27500,0.00958068296313286)
--(axis cs:27400,0.00957168359309435)
--(axis cs:27300,0.00959416013211012)
--(axis cs:27200,0.00958315655589104)
--(axis cs:27100,0.00961296819150448)
--(axis cs:27000,0.0095822736620903)
--(axis cs:26900,0.00960342213511467)
--(axis cs:26800,0.0095965713262558)
--(axis cs:26700,0.00966288521885872)
--(axis cs:26600,0.00966790225356817)
--(axis cs:26500,0.0097801461815834)
--(axis cs:26400,0.009745042771101)
--(axis cs:26300,0.00971783231943846)
--(axis cs:26200,0.00962056778371334)
--(axis cs:26100,0.00961813796311617)
--(axis cs:26000,0.00961394235491753)
--(axis cs:25900,0.00963029079139233)
--(axis cs:25800,0.00962806306779385)
--(axis cs:25700,0.00974581204354763)
--(axis cs:25600,0.00973621569573879)
--(axis cs:25500,0.00967771746218204)
--(axis cs:25400,0.00961932167410851)
--(axis cs:25300,0.00958658382296562)
--(axis cs:25200,0.00957118906080723)
--(axis cs:25100,0.00959794502705336)
--(axis cs:25000,0.00962148420512676)
--(axis cs:24900,0.0096321078017354)
--(axis cs:24800,0.00969300325959921)
--(axis cs:24700,0.00955609232187271)
--(axis cs:24600,0.00955805368721485)
--(axis cs:24500,0.00955090299248695)
--(axis cs:24400,0.00955691747367382)
--(axis cs:24300,0.00955743901431561)
--(axis cs:24200,0.00967452581971884)
--(axis cs:24100,0.0096901785582304)
--(axis cs:24000,0.00957203004509211)
--(axis cs:23900,0.00956068374216557)
--(axis cs:23800,0.00955010950565338)
--(axis cs:23700,0.00959984865039587)
--(axis cs:23600,0.00958504993468523)
--(axis cs:23500,0.00970917940139771)
--(axis cs:23400,0.0096717681735754)
--(axis cs:23300,0.00964275281876326)
--(axis cs:23200,0.00960088428109884)
--(axis cs:23100,0.00955763272941113)
--(axis cs:23000,0.00955055933445692)
--(axis cs:22900,0.00955520290881395)
--(axis cs:22800,0.00960665289312601)
--(axis cs:22700,0.00964434631168842)
--(axis cs:22600,0.00972689967602491)
--(axis cs:22500,0.00977513380348682)
--(axis cs:22400,0.00982604082673788)
--(axis cs:22300,0.00984209775924683)
--(axis cs:22200,0.00980161130428314)
--(axis cs:22100,0.00980418547987938)
--(axis cs:22000,0.00981598254293203)
--(axis cs:21900,0.00973813235759735)
--(axis cs:21800,0.00971978157758713)
--(axis cs:21700,0.00969735626131296)
--(axis cs:21600,0.00958204455673695)
--(axis cs:21500,0.00956072099506855)
--(axis cs:21400,0.00957965198904276)
--(axis cs:21300,0.00955413468182087)
--(axis cs:21200,0.00957519561052322)
--(axis cs:21100,0.00968784000724554)
--(axis cs:21000,0.00969153642654419)
--(axis cs:20900,0.00971422158181667)
--(axis cs:20800,0.00962056219577789)
--(axis cs:20700,0.00956303812563419)
--(axis cs:20600,0.00956036895513535)
--(axis cs:20500,0.00955578871071339)
--(axis cs:20400,0.00955240707844496)
--(axis cs:20300,0.00959772150963545)
--(axis cs:20200,0.00964460149407387)
--(axis cs:20100,0.00961128808557987)
--(axis cs:20000,0.00973989628255367)
--(axis cs:19900,0.00941066257655621)
--(axis cs:19800,0.00918510556221008)
--(axis cs:19700,0.00949182361364365)
--(axis cs:19600,0.00934605859220028)
--(axis cs:19500,0.00908891391009092)
--(axis cs:19400,0.00916974153369665)
--(axis cs:19300,0.00925514288246632)
--(axis cs:19200,0.00988036580383778)
--(axis cs:19100,0.0097278393805027)
--(axis cs:19000,0.0097913546487689)
--(axis cs:18900,0.0102973580360413)
--(axis cs:18800,0.0102973580360413)
--(axis cs:18700,0.0094796409830451)
--(axis cs:18600,0.00809080991894007)
--(axis cs:18500,0.00643750419840217)
--(axis cs:18400,0.00483478838577867)
--(axis cs:18300,0.00341312028467655)
--(axis cs:18200,0.00450510997325182)
--(axis cs:18100,0.00438620056957006)
--(axis cs:18000,0.00480936793610454)
--(axis cs:17900,0.0051271915435791)
--(axis cs:17800,0.0052429111674428)
--(axis cs:17700,0.00556178949773312)
--(axis cs:17600,0.0054587796330452)
--(axis cs:17500,0.00437994860112667)
--(axis cs:17400,0.00360985659062862)
--(axis cs:17300,0.00333795580081642)
--(axis cs:17200,0.00253121857531369)
--(axis cs:17100,0.00323015777394176)
--(axis cs:17000,0.00437927059829235)
--(axis cs:16900,0.00482456665486097)
--(axis cs:16800,0.00451077241450548)
--(axis cs:16700,0.00502599030733109)
--(axis cs:16600,0.00432963250204921)
--(axis cs:16500,0.00432313233613968)
--(axis cs:16400,0.00421633338555694)
--(axis cs:16300,0.00649840990081429)
--(axis cs:16200,0.0067102937027812)
--(axis cs:16100,0.00695659127086401)
--(axis cs:16000,0.0064244382083416)
--(axis cs:15900,0.00421866588294506)
--(axis cs:15800,0.00377162685617805)
--(axis cs:15700,0.00412330636754632)
--(axis cs:15600,0.00850956793874502)
--(axis cs:15500,0.0077411001548171)
--(axis cs:15400,0.00849411729723215)
--(axis cs:15300,0.00793438218533993)
--(axis cs:15200,0.00748604582622647)
--(axis cs:15100,0.00423459988087416)
--(axis cs:15000,0.00463910866528749)
--(axis cs:14900,0.00347792496904731)
--(axis cs:14800,0.00382573087699711)
--(axis cs:14700,0.00324236298911273)
--(axis cs:14600,0.00432484783232212)
--(axis cs:14500,0.00462356396019459)
--(axis cs:14400,0.00480239558964968)
--(axis cs:14300,0.00495634879916906)
--(axis cs:14200,0.00646419962868094)
--(axis cs:14100,0.0062364786863327)
--(axis cs:14000,0.00625646254047751)
--(axis cs:13900,0.00834075827151537)
--(axis cs:13800,0.011661565862596)
--(axis cs:13700,0.00999101530760527)
--(axis cs:13600,0.00961694680154324)
--(axis cs:13500,0.00936242006719112)
--(axis cs:13400,0.00742164626717567)
--(axis cs:13300,0.00408290978521109)
--(axis cs:13200,0.00319207459688187)
--(axis cs:13100,0.00568880699574947)
--(axis cs:13000,0.00653011118993163)
--(axis cs:12900,0.00654194178059697)
--(axis cs:12800,0.00595997367054224)
--(axis cs:12700,0.00567395612597466)
--(axis cs:12600,0.00709152920171618)
--(axis cs:12500,0.00655442243441939)
--(axis cs:12400,0.00599974580109119)
--(axis cs:12300,0.00597625970840454)
--(axis cs:12200,0.00698094163089991)
--(axis cs:12100,0.00429215282201767)
--(axis cs:12000,0.00400269031524658)
--(axis cs:11900,0.00513026677072048)
--(axis cs:11800,0.00548080494627357)
--(axis cs:11700,0.00671393517404795)
--(axis cs:11600,0.00662817480042577)
--(axis cs:11500,0.00740686897188425)
--(axis cs:11400,0.00728370808064938)
--(axis cs:11300,0.0071267606690526)
--(axis cs:11200,0.00680378079414368)
--(axis cs:11100,0.00791123695671558)
--(axis cs:11000,0.00648015318438411)
--(axis cs:10900,0.00594560708850622)
--(axis cs:10800,0.00588031858205795)
--(axis cs:10700,0.00509979343041778)
--(axis cs:10600,0.00481646927073598)
--(axis cs:10500,0.0055448180064559)
--(axis cs:10400,0.00537041295319796)
--(axis cs:10300,0.00728061003610492)
--(axis cs:10200,0.00598663184791803)
--(axis cs:10100,0.00617004372179508)
--(axis cs:10000,0.00780967809259892)
--(axis cs:9900,0.00796798430383205)
--(axis cs:9800,0.00408003805205226)
--(axis cs:9700,0.00583626981824636)
--(axis cs:9600,0.00585760734975338)
--(axis cs:9500,0.00495925499126315)
--(axis cs:9400,0.00532786967232823)
--(axis cs:9300,0.00661035813391209)
--(axis cs:9200,0.00717759039252996)
--(axis cs:9100,0.00727905612438917)
--(axis cs:9000,0.00665484368801117)
--(axis cs:8900,0.00668072886765003)
--(axis cs:8800,0.00563851278275251)
--(axis cs:8700,0.00501798512414098)
--(axis cs:8600,0.00510468473657966)
--(axis cs:8500,0.00419219303876162)
--(axis cs:8400,0.00486432481557131)
--(axis cs:8300,0.00449492828920484)
--(axis cs:8200,0.00402408232912421)
--(axis cs:8100,0.00349775003269315)
--(axis cs:8000,0.00522793829441071)
--(axis cs:7900,0.00482235988602042)
--(axis cs:7800,0.00791468936949968)
--(axis cs:7700,0.00621026521548629)
--(axis cs:7600,0.00635387748479843)
--(axis cs:7500,0.00843485537916422)
--(axis cs:7400,0.00953948777168989)
--(axis cs:7300,0.00693160388618708)
--(axis cs:7200,0.00729643041267991)
--(axis cs:7100,0.00712104002013803)
--(axis cs:7000,0.00513294991105795)
--(axis cs:6900,0.00635908730328083)
--(axis cs:6800,0.00402952311560512)
--(axis cs:6700,0.0038591306656599)
--(axis cs:6600,0.00424620695412159)
--(axis cs:6500,0.00622361246496439)
--(axis cs:6400,0.00481010926887393)
--(axis cs:6300,0.0035680322907865)
--(axis cs:6200,0.00423457426950336)
--(axis cs:6100,0.00370505452156067)
--(axis cs:6000,0.00199205987155437)
--(axis cs:5900,0.00228475616313517)
--(axis cs:5800,0.00276757567189634)
--(axis cs:5700,0.00265825679525733)
--(axis cs:5600,0.00391737837344408)
--(axis cs:5500,0.00302409683354199)
--(axis cs:5400,0.00277384370565414)
--(axis cs:5300,0.00252642622217536)
--(axis cs:5200,0.00240896106697619)
--(axis cs:5100,0.00128835497889668)
--(axis cs:5000,0.00151407637167722)
--(axis cs:4900,0.00186747591942549)
--(axis cs:4800,0.00207759882323444)
--(axis cs:4700,0.00173316267319024)
--(axis cs:4600,0.00303433928638697)
--(axis cs:4500,0.00283001735806465)
--(axis cs:4400,0.00580459740012884)
--(axis cs:4300,0.00590650178492069)
--(axis cs:4200,0.00566292461007833)
--(axis cs:4100,0.00550371734425426)
--(axis cs:4000,0.0055136363953352)
--(axis cs:3900,0.00547897256910801)
--(axis cs:3800,0.00506046507507563)
--(axis cs:3700,0.00447312230244279)
--(axis cs:3600,0.0045601618476212)
--(axis cs:3500,0.0050100376829505)
--(axis cs:3400,0.00476583791896701)
--(axis cs:3300,0.00342303281649947)
--(axis cs:3200,0.00376981263980269)
--(axis cs:3100,0.00458634970709682)
--(axis cs:3000,0.00273564527742565)
--(axis cs:2900,0.002783905249089)
--(axis cs:2800,0.00227103987708688)
--(axis cs:2700,0.00286986422725022)
--(axis cs:2600,0.00293836602941155)
--(axis cs:2500,0.00292103295214474)
--(axis cs:2400,0.00213274220004678)
--(axis cs:2300,0.00220579328015447)
--(axis cs:2200,0.00181057641748339)
--(axis cs:2100,0.00180232245475054)
--(axis cs:2000,0.00171651144046336)
--(axis cs:1900,0.00145908107515424)
--(axis cs:1800,0.00136423006188124)
--(axis cs:1700,0.000751428829971701)
--(axis cs:1600,0.0013703202130273)
--(axis cs:1500,0.00137883971910924)
--(axis cs:1400,0.00143318506889045)
--(axis cs:1300,0.00142068066634238)
--(axis cs:1200,0.00129664211999625)
--(axis cs:1100,0.000266197515884414)
--(axis cs:1000,0.000246120675001293)
--(axis cs:900,9.17654469958507e-05)
--(axis cs:800,7.33741326257586e-05)
--(axis cs:700,5.99576388538026e-10)
--(axis cs:600,5.99576388538026e-10)
--(axis cs:500,5.99576388538026e-10)
--(axis cs:400,0.000154673092765734)
--(axis cs:300,0.00116706255357713)
--(axis cs:200,0.00322034885175526)
--(axis cs:100,0.00546487607061863)
--(axis cs:0,0.00546552613377571)
--cycle;

\addplot [ultra thick, color0]
table {%
0 224.896194458008
100 272.092132568359
200 281.175018310547
300 288.550933837891
400 276.11962890625
500 71.3446426391602
600 32.4839477539062
700 31.3121242523193
800 32.5643119812012
900 34.2731437683105
1000 49.293083190918
1100 53.1637954711914
1200 53.6856422424316
1300 54.9357032775879
1400 59.402458190918
1500 48.5678939819336
1600 47.9450950622559
1700 50.6780242919922
1800 61.2941246032715
1900 67.5493927001953
2000 77.6405639648438
2100 86.8087692260742
2200 101.4970703125
2300 96.8659439086914
2400 105.068138122559
2500 105.04581451416
2600 129.207748413086
2700 145.884246826172
2800 160.281829833984
2900 180.489654541016
3000 186.948852539062
3100 164.702911376953
3200 152.406478881836
3300 149.977005004883
3400 164.423477172852
3500 199.915008544922
3700 252.624710083008
3800 259.022338867188
3900 246.61311340332
4000 259.505706787109
4100 265.581268310547
4200 261.547637939453
4300 280.943756103516
4400 288.377532958984
4500 283.536560058594
4600 295.669219970703
4700 312.109375
4800 307.619750976562
4900 321.348205566406
5000 308.849609375
5100 294.108306884766
5200 293.770080566406
5300 322.961151123047
5400 311.358764648438
5500 325.018127441406
5600 357.720489501953
5700 352.162139892578
5800 332.929992675781
5900 333.222381591797
6000 323.579437255859
6100 318.118377685547
6200 316.761871337891
6300 327.505249023438
6400 368.017608642578
6500 398.757385253906
6600 420.60498046875
6700 447.806976318359
6800 467.347900390625
6900 455.010040283203
7100 422.75927734375
7200 433.392700195312
7500 437.303863525391
7600 425.737396240234
7700 399.808868408203
7800 381.175109863281
7900 353.242401123047
8000 341.097961425781
8100 332.720245361328
8200 300.515167236328
8300 269.408081054688
8400 264.634826660156
8500 250.766403198242
8600 233.633331298828
8700 248.902206420898
8800 263.352508544922
8900 273.944671630859
9000 282.149017333984
9100 285.215911865234
9200 283.626068115234
9300 274.730987548828
9400 292.791961669922
9500 295.114776611328
9600 317.216766357422
9700 335.182189941406
9800 366.11474609375
9900 364.543975830078
10000 371.141326904297
10100 391.671295166016
10200 399.588989257812
10300 388.746398925781
10400 373.124176025391
10500 377.047027587891
10600 344.852142333984
10700 335.624847412109
10800 338.241607666016
10900 343.907043457031
11000 342.939514160156
11100 337.588989257812
11200 325.555999755859
11300 323.101409912109
11400 322.569549560547
11500 330.868530273438
11600 349.310729980469
11700 354.727264404297
11800 339.962646484375
11900 333.158355712891
12100 292.582458496094
12200 277.89794921875
12300 282.622161865234
12400 278.998077392578
12600 277.471405029297
12700 287.135406494141
12800 273.946014404297
12900 270.205413818359
13000 256.417388916016
13100 247.104644775391
13200 241.727355957031
13500 260.538604736328
13600 270.82421875
13700 270.359436035156
13800 274.620300292969
14000 278.190093994141
14100 285.719573974609
14200 286.774169921875
14300 284.7578125
14400 286.153442382812
14500 289.977416992188
14600 279.457489013672
14800 253.159637451172
14900 235.199996948242
15000 226.08073425293
15100 229.932525634766
15200 249.953979492188
15400 275.209350585938
15500 277.589782714844
15600 273.837463378906
15700 260.391906738281
15800 265.088500976562
15900 261.282012939453
16000 268.692474365234
16100 273.015625
16300 269.645263671875
16400 279.797973632812
16500 297.685394287109
16600 295.365692138672
16700 304.633575439453
16800 317.283813476562
16900 321.390380859375
17000 306.805145263672
17100 314.014129638672
17200 313.384704589844
17300 307.532623291016
17400 294.057464599609
17500 295.014831542969
17600 298.350433349609
17700 288.936767578125
17800 270.180786132812
17900 261.029663085938
18000 258.126770019531
18100 250.059936523438
18200 255.929382324219
18300 269.167999267578
18400 280.425079345703
18500 295.785461425781
18700 315.725067138672
18800 312.572326660156
18900 312.462524414062
19000 291.030792236328
19100 286.934173583984
19200 287.467712402344
19300 299.346282958984
19400 308.360656738281
19500 307.894287109375
19600 296.805999755859
19700 275.491424560547
19800 262.272735595703
19900 245.996673583984
20000 248.198135375977
20100 246.179458618164
20200 250.442260742188
20300 246.643035888672
20400 249.870010375977
20500 245.553161621094
20600 254.733871459961
20700 253.540313720703
20800 262.412719726562
20900 259.824157714844
21100 264.274780273438
21200 269.705230712891
21300 262.644470214844
21400 264.512969970703
21500 257.464874267578
21600 252.525024414062
21700 262.444000244141
21800 276.177368164062
21900 280.127807617188
22000 296.433898925781
22100 304.679382324219
22300 287.848785400391
22400 286.426300048828
22500 282.363006591797
22600 271.194976806641
22700 268.724029541016
23000 271.868469238281
23300 278.292419433594
23500 276.116729736328
23600 285.675811767578
23700 291.640625
23800 292.940368652344
23900 292.149749755859
24000 295.188842773438
24100 288.945648193359
24200 287.4296875
24300 287.625244140625
24400 291.584442138672
24500 287.935394287109
24600 292.164001464844
24700 300.981262207031
24800 303.734832763672
25000 316.108856201172
25100 317.463104248047
25200 311.640075683594
25300 312.664672851562
25500 309.82080078125
25700 296.609405517578
26000 293.183807373047
26100 298.420867919922
26200 306.763549804688
26300 308.65771484375
26500 308.887084960938
26600 301.019287109375
26700 290.292633056641
26800 281.649017333984
26900 279.385406494141
27000 278.982299804688
27100 280.810363769531
27200 292.326049804688
27400 304.471893310547
27600 310.419219970703
27700 309.070770263672
27800 311.129638671875
28000 311.163116455078
28100 322.181793212891
28200 331.367156982422
28300 335.113037109375
28400 333.093811035156
28500 344.511566162109
28600 342.443237304688
28700 333.545776367188
28800 326.964141845703
28900 325.362487792969
29000 312.751525878906
29100 302.763610839844
29200 295.7109375
29300 297.907867431641
29500 299.479095458984
29600 302.331268310547
29700 307.329071044922
29800 309.275970458984
29900 317.090515136719
30000 331.598999023438
30100 335.748870849609
30200 342.389099121094
30400 342.16455078125
30500 335.962951660156
30600 336.536468505859
30700 328.593719482422
30800 327.693725585938
31000 318.105804443359
31100 324.482757568359
31200 333.796356201172
31300 337.336456298828
31400 336.541656494141
31500 340.043273925781
31700 330.9462890625
31900 329.555694580078
32000 323.942749023438
32100 321.963592529297
32300 327.606842041016
32400 338.300476074219
32500 345.410339355469
32600 354.995910644531
32800 351.572418212891
32900 344.572845458984
33000 340.987487792969
33100 331.520904541016
33200 334.482238769531
33300 332.608856201172
33400 334.910339355469
33500 333.847320556641
33600 340.720275878906
33700 350.121887207031
33800 354.162017822266
34000 356.062957763672
34100 353.044830322266
34200 344.3115234375
34300 343.14892578125
};
\addplot [ultra thick, white!60.2745098039216!black]
table {%
0 0.00515152141451836
100 0.00515093328431249
200 0.00298795290291309
300 0.00103488506283611
400 8.00003545009531e-05
500 2.48352838294608e-10
700 2.48352838294608e-10
800 3.03927809000015e-05
900 5.78296749154106e-05
1000 0.000164446042617783
1100 0.000173289939993992
1200 0.000633029616437852
1300 0.000805997056886554
1400 0.000799804634880275
1500 0.000763977353926748
1600 0.000994294881820679
1700 0.000672402500640601
1800 0.00105218321550637
1900 0.00118502660188824
2000 0.00143602560274303
2100 0.00124493287876248
2200 0.00157311570364982
2300 0.00132322299759835
2400 0.00141520402394235
2500 0.00177029706537724
2600 0.00186610058881342
2700 0.0018952211830765
2800 0.00220169546082616
2900 0.00245455862022936
3000 0.00220698839984834
3100 0.00313384691253304
3200 0.00299772713333368
3300 0.00248759193345904
3400 0.00283817504532635
3500 0.00334566156379879
3600 0.0031269402243197
3700 0.0028704886790365
3800 0.00305266887880862
3900 0.00346059631556273
4000 0.00446466961875558
4100 0.00368409371003509
4200 0.0043749213218689
4300 0.00421098247170448
4400 0.00339536461979151
4500 0.00171270803548396
4600 0.00188576127402484
4700 0.00117273861542344
4800 0.00156451866496354
4900 0.0014323660871014
5000 0.00128230464179069
5100 0.00118127488531172
5200 0.00203591072931886
5300 0.00193080306053162
5400 0.00214729411527514
5500 0.00252287788316607
5600 0.00302819791249931
5700 0.00216047838330269
5800 0.00256554246880114
5900 0.00210251519456506
6000 0.00174850143957883
6100 0.00318082049489021
6200 0.00357732269912958
6300 0.00306223123334348
6400 0.00402462901547551
6500 0.00478911679238081
6600 0.00301301316358149
6700 0.00288524804636836
6800 0.00301765650510788
6900 0.00387672684155405
7000 0.00391104491427541
7100 0.00573589187115431
7200 0.00590914208441973
7300 0.00604609632864594
7400 0.00584121374413371
7500 0.00568635761737823
7600 0.00459841964766383
7700 0.0043972977437079
7800 0.00491735385730863
7900 0.00333603098988533
8000 0.00325876055285335
8100 0.00245804828591645
8200 0.00294238142669201
8300 0.00321975094266236
8400 0.00348181929439306
8500 0.0029171125497669
8600 0.00378416874445975
8700 0.00338901253417134
8800 0.00386511348187923
8900 0.00526138814166188
9000 0.00559398671612144
9100 0.00557773094624281
9200 0.00595642672851682
9300 0.00511509506031871
9400 0.00378898321650922
9500 0.00370704126544297
9600 0.00388974160887301
9700 0.00373165146447718
9800 0.0030156362336129
9900 0.00445743277668953
10000 0.00437084026634693
10100 0.00402471702545881
10200 0.00386106502264738
10300 0.00543271377682686
10400 0.0040701269172132
10500 0.00434738583862782
10600 0.0036601850297302
10700 0.00385509640909731
10900 0.00327993743121624
11000 0.00373714161105454
11100 0.00486401654779911
11200 0.00447667110711336
11300 0.00499307457357645
11400 0.00512189511209726
11500 0.00492125051096082
11600 0.00413314439356327
11700 0.00446062255650759
11800 0.00365992565639317
11900 0.00361040094867349
12000 0.00317006278783083
12100 0.00362234865315259
12200 0.00544229010120034
12300 0.00437251524999738
12400 0.00438247853890061
12500 0.00516886962577701
12600 0.00497969705611467
12700 0.00430209608748555
12800 0.00452191149815917
12900 0.0048200530000031
13000 0.00455953972414136
13100 0.00406061904504895
13200 0.002780357375741
13300 0.00315156020224094
13400 0.00543827889487147
13500 0.00640389462932944
13600 0.00663481885567307
13700 0.00669957743957639
13800 0.00759990839287639
13900 0.00568864308297634
14000 0.00463417312130332
14100 0.00454873917624354
14200 0.00533057097345591
14300 0.00398258771747351
14400 0.00376789621077478
14500 0.00364243914373219
14600 0.00363702024333179
14700 0.00249313982203603
14800 0.00315937818959355
14900 0.00291313091292977
15000 0.00316380569711328
15100 0.00301427231170237
15200 0.00587726524099708
15300 0.00580383464694023
15400 0.00639043701812625
15500 0.0056417933665216
15600 0.00600409274920821
15700 0.00332801719196141
15800 0.0033622863702476
15900 0.00347629003226757
16000 0.00452250754460692
16100 0.00462112482637167
16200 0.00445491820573807
16300 0.00390920741483569
16400 0.00333251827396452
16600 0.00348489615134895
16700 0.00426304340362549
16800 0.00409733178094029
16900 0.00383320590481162
17000 0.00329230213537812
17100 0.00287561002187431
17200 0.00239169597625732
17300 0.00284583563916385
17400 0.00332821626216173
17500 0.00337739684619009
17600 0.00427542999386787
17700 0.0042381682433188
17800 0.00459037162363529
17900 0.0042667118832469
18000 0.00406006863340735
18100 0.00305927218869328
18200 0.00310161500237882
18300 0.00280284858308733
18400 0.00369284930638969
18500 0.00470620766282082
18600 0.00539789255708456
18700 0.00587629107758403
18800 0.00682799005880952
18900 0.0071806930936873
19000 0.00670790579169989
19100 0.00656936643645167
19200 0.00694721844047308
19300 0.00673875119537115
19400 0.00578479655086994
19500 0.00577498227357864
19600 0.00602583680301905
19700 0.00613735895603895
19800 0.00596081325784326
19900 0.00639667036011815
20000 0.00639706011861563
20100 0.0069384821690619
20200 0.00677716778591275
20300 0.00701317004859447
20400 0.00760613149031997
20500 0.00765698868781328
20600 0.00729042617604136
20700 0.00726265506818891
20800 0.00689096376299858
20900 0.00649216584861279
21000 0.0065798875875771
21100 0.00659457314759493
21200 0.00715942168608308
21300 0.00737248314544559
21400 0.00712724169716239
21500 0.00728660076856613
21600 0.00711079221218824
21700 0.00655700406059623
21900 0.00640343734994531
22000 0.00613357266411185
22200 0.00618158746510744
22300 0.00604769308120012
22400 0.00610020384192467
22600 0.00644452963024378
22700 0.00677810190245509
22800 0.00696295686066151
22900 0.00735494261607528
23000 0.0074545512907207
23100 0.00732188392430544
23200 0.00699482904747128
23300 0.00678530987352133
23500 0.00651114387437701
23600 0.00709048705175519
23700 0.0070006912574172
23800 0.00753826089203358
23900 0.00728648481890559
24000 0.00718336226418614
24100 0.00658507319167256
24200 0.00664832023903728
24300 0.00732431607320905
24400 0.0073310500010848
24500 0.00757151562720537
24600 0.00768278678879142
24700 0.00766120571643114
24800 0.00657390477135777
24900 0.00683462060987949
25000 0.00688612693920732
25100 0.00701159564778209
25200 0.00719005381688476
25300 0.00708057172596455
25400 0.0068969358690083
25600 0.00641028210520744
25700 0.00637550232931972
25800 0.00685393344610929
25900 0.00684325210750103
26000 0.00692437263205647
26200 0.0068906950764358
26300 0.00647836271673441
26500 0.0062546725384891
26600 0.00667583104223013
26700 0.00669700372964144
26800 0.0070195677690208
26900 0.00698065059259534
27000 0.00710890674963593
27100 0.00692943762987852
27200 0.00710297748446465
27300 0.00703377509489655
27400 0.00718610361218452
27600 0.00703342771157622
27800 0.00630521681159735
27900 0.00648992462083697
28000 0.00662650121375918
28100 0.00644557364284992
};

==> plots/fetch/rel_err_data.tex <==
\path [fill=red, fill opacity=0.4, ultra thick]
(axis cs:0.00499999988824129,0.0981471371189214)
--(axis cs:0.00499999988824129,0.0693458930148139)
--(axis cs:0.00999999977648258,0.0768913576643062)
--(axis cs:0.0149999996647239,0.0805582154812716)
--(axis cs:0.0199999995529652,0.0845196110592269)
--(axis cs:0.0249999994412065,0.0910616688263388)
--(axis cs:0.0299999993294477,0.0960605583494559)
--(axis cs:0.034999999217689,0.0995347371251724)
--(axis cs:0.0399999991059303,0.102204599471983)
--(axis cs:0.0449999989941716,0.105266256553993)
--(axis cs:0.0499999988824129,0.107840601840457)
--(axis cs:0.0549999987706542,0.11024953719084)
--(axis cs:0.0599999986588955,0.112444513695491)
--(axis cs:0.0649999985471368,0.114894346999308)
--(axis cs:0.0699999984353781,0.117045373991443)
--(axis cs:0.0749999983236194,0.119135580434824)
--(axis cs:0.0799999982118607,0.121087367134153)
--(axis cs:0.0849999981001019,0.123097295652794)
--(axis cs:0.0899999979883432,0.124914798373905)
--(axis cs:0.0949999978765845,0.12671936290503)
--(axis cs:0.0949999978765845,0.173708148227355)
--(axis cs:0.0949999978765845,0.173708148227355)
--(axis cs:0.0899999979883432,0.169887707845062)
--(axis cs:0.0849999981001019,0.165865428211006)
--(axis cs:0.0799999982118607,0.161634229731955)
--(axis cs:0.0749999983236194,0.157497989129546)
--(axis cs:0.0699999984353781,0.153176988531972)
--(axis cs:0.0649999985471368,0.148494744088243)
--(axis cs:0.0599999986588955,0.143608795563009)
--(axis cs:0.0549999987706542,0.139183186266431)
--(axis cs:0.0499999988824129,0.134703444736652)
--(axis cs:0.0449999989941716,0.130206618772106)
--(axis cs:0.0399999991059303,0.125438398773785)
--(axis cs:0.034999999217689,0.121120112118062)
--(axis cs:0.0299999993294477,0.116526519213719)
--(axis cs:0.0249999994412065,0.111403463333061)
--(axis cs:0.0199999995529652,0.108039080407262)
--(axis cs:0.0149999996647239,0.105659266717689)
--(axis cs:0.00999999977648258,0.103238590486459)
--(axis cs:0.00499999988824129,0.0981471371189214)
--cycle;

\path [fill=blue, fill opacity=0.4, semithick]
(axis cs:0.00499999988824129,0.107661017009161)
--(axis cs:0.00499999988824129,0.0717935295594608)
--(axis cs:0.00999999977648258,0.0791429559398589)
--(axis cs:0.0149999996647239,0.082633985186815)
--(axis cs:0.0199999995529652,0.0858279470274601)
--(axis cs:0.0249999994412065,0.0908997272933962)
--(axis cs:0.0299999993294477,0.0950262346217573)
--(axis cs:0.034999999217689,0.0975840947294547)
--(axis cs:0.0399999991059303,0.0995622718393212)
--(axis cs:0.0449999989941716,0.101930340941758)
--(axis cs:0.0499999988824129,0.104326165341986)
--(axis cs:0.0549999987706542,0.106561425199056)
--(axis cs:0.0599999986588955,0.108732622693041)
--(axis cs:0.0649999985471368,0.110962928983815)
--(axis cs:0.0699999984353781,0.112719499580694)
--(axis cs:0.0749999983236194,0.114088040030336)
--(axis cs:0.0799999982118607,0.115226777357021)
--(axis cs:0.0849999981001019,0.116211217248537)
--(axis cs:0.0899999979883432,0.117000700562331)
--(axis cs:0.0949999978765845,0.117650844561737)
--(axis cs:0.0949999978765845,0.151035332992766)
--(axis cs:0.0949999978765845,0.151035332992766)
--(axis cs:0.0899999979883432,0.148929664656605)
--(axis cs:0.0849999981001019,0.146587404283663)
--(axis cs:0.0799999982118607,0.144086798508434)
--(axis cs:0.0749999983236194,0.141669759099066)
--(axis cs:0.0699999984353781,0.138967673053992)
--(axis cs:0.0649999985471368,0.135896518813627)
--(axis cs:0.0599999986588955,0.132572491157166)
--(axis cs:0.0549999987706542,0.12944179141955)
--(axis cs:0.0499999988824129,0.126136930206528)
--(axis cs:0.0449999989941716,0.122714632222974)
--(axis cs:0.0399999991059303,0.119439657402984)
--(axis cs:0.034999999217689,0.116923003908404)
--(axis cs:0.0299999993294477,0.114131433051035)
--(axis cs:0.0249999994412065,0.110510261602679)
--(axis cs:0.0199999995529652,0.108501492013911)
--(axis cs:0.0149999996647239,0.107866638583188)
--(axis cs:0.00999999977648258,0.107825004923656)
--(axis cs:0.00499999988824129,0.107661017009161)
--cycle;

\path [fill=green!50.1960784313725!black, fill opacity=0.4, ultra thick]
(axis cs:0.00499999988824129,0.0830617524482067)
--(axis cs:0.00499999988824129,0.0577385334961019)
--(axis cs:0.00999999977648258,0.0609472347238716)
--(axis cs:0.0149999996647239,0.062344939486539)
--(axis cs:0.0199999995529652,0.0645523857627769)
--(axis cs:0.0249999994412065,0.0688552481509171)
--(axis cs:0.0299999993294477,0.0721968693716407)
--(axis cs:0.034999999217689,0.0740155351438639)
--(axis cs:0.0399999991059303,0.0747251433342523)
--(axis cs:0.0449999989941716,0.076196688060175)
--(axis cs:0.0499999988824129,0.078265236166539)
--(axis cs:0.0549999987706542,0.0799868066050893)
--(axis cs:0.0599999986588955,0.0811944321399374)
--(axis cs:0.0649999985471368,0.0826790375067071)
--(axis cs:0.0699999984353781,0.0842147872536796)
--(axis cs:0.0749999983236194,0.0852262409253277)
--(axis cs:0.0799999982118607,0.0858964548859035)
--(axis cs:0.0849999981001019,0.0869284669749143)
--(axis cs:0.0899999979883432,0.0880689473886511)
--(axis cs:0.0949999978765845,0.0887728774389657)
--(axis cs:0.0949999978765845,0.123950443219074)
--(axis cs:0.0949999978765845,0.123950443219074)
--(axis cs:0.0899999979883432,0.122065787742204)
--(axis cs:0.0849999981001019,0.119591672074542)
--(axis cs:0.0799999982118607,0.117123474651583)
--(axis cs:0.0749999983236194,0.114965108071722)
--(axis cs:0.0699999984353781,0.112221726189995)
--(axis cs:0.0649999985471368,0.108807137019256)
--(axis cs:0.0599999986588955,0.105237598566073)
--(axis cs:0.0549999987706542,0.102156176573968)
--(axis cs:0.0499999988824129,0.0986413392759387)
--(axis cs:0.0449999989941716,0.0947838197919073)
--(axis cs:0.0399999991059303,0.0911599179141883)
--(axis cs:0.034999999217689,0.0883223634854195)
--(axis cs:0.0299999993294477,0.0853904199404792)
--(axis cs:0.0249999994412065,0.0822060938997066)
--(axis cs:0.0199999995529652,0.0802182975294789)
--(axis cs:0.0149999996647239,0.0799168495767018)
--(axis cs:0.00999999977648258,0.0798972512640844)
--(axis cs:0.00499999988824129,0.0830617524482067)
--cycle;

\path [fill=color0, fill opacity=0.4, ultra thick]
(axis cs:0.00499999988824129,0.0691418707714119)
--(axis cs:0.00499999988824129,0.0432468939969296)
--(axis cs:0.00999999977648258,0.0516324535170185)
--(axis cs:0.0149999996647239,0.0515130633290674)
--(axis cs:0.0199999995529652,0.0512873514591298)
--(axis cs:0.0249999994412065,0.0531749001829137)
--(axis cs:0.0299999993294477,0.0547475864476341)
--(axis cs:0.034999999217689,0.0563171018417981)
--(axis cs:0.0399999991059303,0.0571659570531023)
--(axis cs:0.0449999989941716,0.0586610050907562)
--(axis cs:0.0499999988824129,0.0600586372681437)
--(axis cs:0.0549999987706542,0.0612916019755903)
--(axis cs:0.0599999986588955,0.0622983017165615)
--(axis cs:0.0649999985471368,0.0635656407422943)
--(axis cs:0.0699999984353781,0.064995355484257)
--(axis cs:0.0749999983236194,0.0661467390966307)
--(axis cs:0.0799999982118607,0.066896883721782)
--(axis cs:0.0849999981001019,0.0678902986932688)
--(axis cs:0.0899999979883432,0.0688010277693822)
--(axis cs:0.0949999978765845,0.0693265017147747)
--(axis cs:0.0949999978765845,0.0930321786056807)
--(axis cs:0.0949999978765845,0.0930321786056807)
--(axis cs:0.0899999979883432,0.0919125371334513)
--(axis cs:0.0849999981001019,0.0902283378317776)
--(axis cs:0.0799999982118607,0.0886564630415355)
--(axis cs:0.0749999983236194,0.0875976061835957)
--(axis cs:0.0699999984353781,0.0861671861597333)
--(axis cs:0.0649999985471368,0.0842818920139673)
--(axis cs:0.0599999986588955,0.0822768049447333)
--(axis cs:0.0549999987706542,0.0810396972361705)
--(axis cs:0.0499999988824129,0.0796091263396972)
--(axis cs:0.0449999989941716,0.0775728662310419)
--(axis cs:0.0399999991059303,0.0749869548046289)
--(axis cs:0.034999999217689,0.0727956040974394)
--(axis cs:0.0299999993294477,0.0707275527701303)
--(axis cs:0.0249999994412065,0.0679617527078296)
--(axis cs:0.0199999995529652,0.0666160932079101)
--(axis cs:0.0149999996647239,0.0669410170690395)
--(axis cs:0.00999999977648258,0.0704492526822372)
--(axis cs:0.00499999988824129,0.0691418707714119)
--cycle;

\path [fill=white!40!black, fill opacity=0.4, ultra thick]
(axis cs:0.00499999988824129,0.0728660114739282)
--(axis cs:0.00499999988824129,0.0472793839221152)
--(axis cs:0.00999999977648258,0.0522475106476856)
--(axis cs:0.0149999996647239,0.0543423041579315)
--(axis cs:0.0199999995529652,0.0549865341125751)
--(axis cs:0.0249999994412065,0.0575579704268763)
--(axis cs:0.0299999993294477,0.0597066606806348)
--(axis cs:0.034999999217689,0.0611029359784349)
--(axis cs:0.0399999991059303,0.0618320840140064)
--(axis cs:0.0449999989941716,0.0631873537919674)
--(axis cs:0.0499999988824129,0.064806731440754)
--(axis cs:0.0549999987706542,0.0661392594038266)
--(axis cs:0.0599999986588955,0.0671212654631985)
--(axis cs:0.0649999985471368,0.0684943794472619)
--(axis cs:0.0699999984353781,0.0698058700151522)
--(axis cs:0.0749999983236194,0.0707865738041196)
--(axis cs:0.0799999982118607,0.0714254531301117)
--(axis cs:0.0849999981001019,0.0722892435519938)
--(axis cs:0.0899999979883432,0.0731936281646384)
--(axis cs:0.0949999978765845,0.073899063733729)
--(axis cs:0.0949999978765845,0.098851571947577)
--(axis cs:0.0949999978765845,0.098851571947577)
--(axis cs:0.0899999979883432,0.0974827054803171)
--(axis cs:0.0849999981001019,0.0955383551671605)
--(axis cs:0.0799999982118607,0.093652007236664)
--(axis cs:0.0749999983236194,0.0923510896217436)
--(axis cs:0.0699999984353781,0.0907468745546822)
--(axis cs:0.0649999985471368,0.0885441239818889)
--(axis cs:0.0599999986588955,0.0862765882982384)
--(axis cs:0.0549999987706542,0.0849457619405477)
--(axis cs:0.0499999988824129,0.0830950683301027)
--(axis cs:0.0449999989941716,0.0807032698346358)
--(axis cs:0.0399999991059303,0.0778895897794887)
--(axis cs:0.034999999217689,0.0758716613948973)
--(axis cs:0.0299999993294477,0.0730464991303921)
--(axis cs:0.0249999994412065,0.0692151823749083)
--(axis cs:0.0199999995529652,0.0667704042014442)
--(axis cs:0.0149999996647239,0.0689100804883708)
--(axis cs:0.00999999977648258,0.0732407344645434)
--(axis cs:0.00499999988824129,0.0728660114739282)
--cycle;

\addplot [ultra thick, red]
table {%
0.00499999523162842 0.0837465077638626
0.00999999046325684 0.0900649651885033
0.0149999856948853 0.0931087359786034
0.0199999809265137 0.0962793454527855
0.0249999761581421 0.101232580840588
0.0299999713897705 0.106293544173241
0.0349999666213989 0.110327422618866
0.0399999618530273 0.113821513950825
0.0449999570846558 0.117736451327801
0.0499999523162842 0.121272020041943
0.0549999475479126 0.124716356396675
0.059999942779541 0.128026649355888
0.065000057220459 0.131694540381432
0.0700000524520874 0.135111182928085
0.0750000476837158 0.138316780328751
0.0850000381469727 0.144481375813484
0.0900000333786011 0.147401243448257
0.0950000286102295 0.150213733315468
};
% \addlegendentry{No si.}
\addplot [ultra thick, blue]
table {%
0.00499999523162842 0.0897272750735283
0.00999999046325684 0.0934839844703674
0.0149999856948853 0.0952502936124802
0.0199999809265137 0.0971647277474403
0.0249999761581421 0.100705005228519
0.0299999713897705 0.104578822851181
0.0349999666213989 0.107253558933735
0.0399999618530273 0.109500974416733
0.0499999523162842 0.115231536328793
0.0549999475479126 0.118001617491245
0.059999942779541 0.120652556419373
0.065000057220459 0.123429708182812
0.0700000524520874 0.125843584537506
0.0750000476837158 0.127878904342651
0.0800000429153442 0.129656776785851
0.0850000381469727 0.131399273872375
0.0900000333786011 0.132965177297592
0.0950000286102295 0.134343087673187
};
\addplot [ultra thick, green!50.1960784313725!black]
table {%
0.00499999523162842 0.0704001411795616
0.00999999046325684 0.0704222470521927
0.0149999856948853 0.0711309015750885
0.0199999809265137 0.0723853409290314
0.0249999761581421 0.0755306631326675
0.0299999713897705 0.0787936374545097
0.0349999666213989 0.081168957054615
0.0399999618530273 0.0829425230622292
0.0449999570846558 0.0854902490973473
0.0499999523162842 0.0884532779455185
0.0549999475479126 0.0910714864730835
0.059999942779541 0.0932160168886185
0.065000057220459 0.0957430973649025
0.0700000524520874 0.0982182696461678
0.0750000476837158 0.100095674395561
0.0800000429153442 0.101509973406792
0.0850000381469727 0.103260084986687
0.0900000333786011 0.105067357420921
0.0950000286102295 0.106361664831638
};
% \addlegendentry{Si 2}
\addplot [ultra thick, color0]
table {%
0.00499999523162842 0.0561943836510181
0.00999999046325684 0.061040848493576
0.0149999856948853 0.0592270456254482
0.0199999809265137 0.0589517205953598
0.0249999761581421 0.0605683177709579
0.0299999713897705 0.0627375692129135
0.0349999666213989 0.0645563378930092
0.0399999618530273 0.0660764425992966
0.0449999570846558 0.0681169256567955
0.0499999523162842 0.0698338747024536
0.0549999475479126 0.071165643632412
0.059999942779541 0.0722875520586967
0.065000057220459 0.0739237666130066
0.0700000524520874 0.0755812674760818
0.0750000476837158 0.0768721699714661
0.0800000429153442 0.0777766704559326
0.0900000333786011 0.080356776714325
0.0950000286102295 0.0811793431639671
};
% \addlegendentry{si 3}
\addplot [ultra thick, white!40!black]
table {%
0.00499999523162842 0.0600726939737797
0.00999999046325684 0.0627441257238388
0.0149999856948853 0.0616261959075928
0.0199999809265137 0.060878474265337
0.0249999761581421 0.0633865743875504
0.0299999713897705 0.0663765668869019
0.0349999666213989 0.0684873014688492
0.0399999618530273 0.0698608309030533
0.0449999570846558 0.0719453096389771
0.0499999523162842 0.0739509016275406
0.0549999475479126 0.0755425170063972
0.059999942779541 0.0766989141702652
0.065000057220459 0.0785192474722862
0.0700000524520874 0.0802763700485229
0.0750000476837158 0.0815688446164131
0.0800000429153442 0.0825387313961983
0.0850000381469727 0.0839137956500053
0.0900000333786011 0.0853381603956223
0.0950000286102295 0.0863753259181976
};
% \addlegendentry{si 4}




% \path [fill=blue, fill opacity=0.4, ultra thick]
% (axis cs:0.00499999988824129,0.104644967318169)
% --(axis cs:0.00499999988824129,0.0735731940053169)
% --(axis cs:0.00999999977648258,0.0808920605276985)
% --(axis cs:0.0149999996647239,0.0836938807572603)
% --(axis cs:0.0199999995529652,0.0867695519978043)
% --(axis cs:0.0249999994412065,0.0923157700653139)
% --(axis cs:0.0299999993294477,0.0973650951179764)
% --(axis cs:0.034999999217689,0.101662286631509)
% --(axis cs:0.0399999991059303,0.105320288986683)
% --(axis cs:0.0449999989941716,0.108968955728221)
% --(axis cs:0.0499999988824129,0.112164199952017)
% --(axis cs:0.0549999987706542,0.114874582314576)
% --(axis cs:0.0599999986588955,0.117283901268746)
% --(axis cs:0.0649999985471368,0.119674390690466)
% --(axis cs:0.0699999984353781,0.121829861257787)
% --(axis cs:0.0749999983236194,0.123752504517181)
% --(axis cs:0.0799999982118607,0.1256384918868)
% --(axis cs:0.0849999981001019,0.127635494599139)
% --(axis cs:0.0899999979883432,0.129562600113302)
% --(axis cs:0.0949999978765845,0.13142408914452)
% --(axis cs:0.0999999977648258,0.133205876743766)
% --(axis cs:0.104999997653067,0.135073594172048)
% --(axis cs:0.109999997541308,0.136834793923856)
% --(axis cs:0.11499999742955,0.138437898607242)
% --(axis cs:0.119999997317791,0.139934224885507)
% --(axis cs:0.124999997206032,0.141429874370928)
% --(axis cs:0.129999997094274,0.142813579882247)
% --(axis cs:0.134999996982515,0.144077579317613)
% --(axis cs:0.139999996870756,0.145249019510009)
% --(axis cs:0.144999996758997,0.146419907406387)
% --(axis cs:0.149999996647239,0.147562421058272)
% --(axis cs:0.15499999653548,0.148690351919368)
% --(axis cs:0.159999996423721,0.149804332145281)
% --(axis cs:0.164999996311963,0.150995638410959)
% --(axis cs:0.169999996200204,0.152170440940089)
% --(axis cs:0.174999996088445,0.153359390460353)
% --(axis cs:0.179999995976686,0.154604749199006)
% --(axis cs:0.184999995864928,0.15597526650941)
% --(axis cs:0.189999995753169,0.157512710256331)
% --(axis cs:0.19499999564141,0.159211054828558)
% --(axis cs:0.199999995529652,0.161087170455919)
% --(axis cs:0.204999995417893,0.163058040021124)
% --(axis cs:0.209999995306134,0.165098760390318)
% --(axis cs:0.214999995194376,0.167214557386469)
% --(axis cs:0.219999995082617,0.169383305629256)
% --(axis cs:0.224999994970858,0.171670192782016)
% --(axis cs:0.229999994859099,0.174060459585118)
% --(axis cs:0.234999994747341,0.176524598007166)
% --(axis cs:0.239999994635582,0.179035766404665)
% --(axis cs:0.244999994523823,0.181571641720527)
% --(axis cs:0.249999994412065,0.184139903083795)
% --(axis cs:0.254999994300306,0.186705873531486)
% --(axis cs:0.259999994188547,0.189271209372746)
% --(axis cs:0.264999994076788,0.19184850312581)
% --(axis cs:0.26999999396503,0.194425657701666)
% --(axis cs:0.274999993853271,0.196978490692018)
% --(axis cs:0.279999993741512,0.199493515675635)
% --(axis cs:0.284999993629754,0.20196690511764)
% --(axis cs:0.289999993517995,0.204384454027888)
% --(axis cs:0.294999993406236,0.206762409183226)
% --(axis cs:0.299999993294477,0.209077914295185)
% --(axis cs:0.304999993182719,0.211398599946444)
% --(axis cs:0.30999999307096,0.21367382878454)
% --(axis cs:0.314999992959201,0.215896106155777)
% --(axis cs:0.319999992847443,0.218102084808151)
% --(axis cs:0.324999992735684,0.220279090268894)
% --(axis cs:0.329999992623925,0.222426757967953)
% --(axis cs:0.334999992512167,0.224562763561923)
% --(axis cs:0.339999992400408,0.226690720198322)
% --(axis cs:0.344999992288649,0.228828048873333)
% --(axis cs:0.34999999217689,0.230960049781846)
% --(axis cs:0.354999992065132,0.233086611026266)
% --(axis cs:0.359999991953373,0.235212454822518)
% --(axis cs:0.364999991841614,0.237378767508273)
% --(axis cs:0.369999991729856,0.239566018308699)
% --(axis cs:0.374999991618097,0.24175396638904)
% --(axis cs:0.379999991506338,0.243947285350089)
% --(axis cs:0.384999991394579,0.246147274598957)
% --(axis cs:0.389999991282821,0.248327282774095)
% --(axis cs:0.394999991171062,0.250508289601579)
% --(axis cs:0.399999991059303,0.252684933863462)
% --(axis cs:0.404999990947545,0.254852182536972)
% --(axis cs:0.409999990835786,0.257020699377944)
% --(axis cs:0.414999990724027,0.259148981080679)
% --(axis cs:0.419999990612268,0.261252144042803)
% --(axis cs:0.42499999050051,0.26334111823306)
% --(axis cs:0.429999990388751,0.265379620519107)
% --(axis cs:0.434999990276992,0.267365589339461)
% --(axis cs:0.439999990165234,0.269326258130468)
% --(axis cs:0.444999990053475,0.271266364461258)
% --(axis cs:0.449999989941716,0.273167769137577)
% --(axis cs:0.454999989829957,0.275033112195185)
% --(axis cs:0.459999989718199,0.276870047537394)
% --(axis cs:0.46499998960644,0.27870401345168)
% --(axis cs:0.469999989494681,0.280521795208296)
% --(axis cs:0.474999989382923,0.282334225868085)
% --(axis cs:0.479999989271164,0.284138345551925)
% --(axis cs:0.484999989159405,0.285920029945882)
% --(axis cs:0.489999989047647,0.28768411599039)
% --(axis cs:0.494999988935888,0.289442441096964)
% --(axis cs:0.494999988935888,0.385392018376879)
% --(axis cs:0.494999988935888,0.385392018376879)
% --(axis cs:0.489999989047647,0.383232416726784)
% --(axis cs:0.484999989159405,0.381038863322875)
% --(axis cs:0.479999989271164,0.378801498204892)
% --(axis cs:0.474999989382923,0.376548727245794)
% --(axis cs:0.469999989494681,0.374266103938028)
% --(axis cs:0.46499998960644,0.371958947572844)
% --(axis cs:0.459999989718199,0.36964654332137)
% --(axis cs:0.454999989829957,0.367348182077589)
% --(axis cs:0.449999989941716,0.365021707668885)
% --(axis cs:0.444999990053475,0.362655860991412)
% --(axis cs:0.439999990165234,0.360271672254737)
% --(axis cs:0.434999990276992,0.357880713618944)
% --(axis cs:0.429999990388751,0.355472420676185)
% --(axis cs:0.42499999050051,0.353020795716705)
% --(axis cs:0.419999990612268,0.350531423514041)
% --(axis cs:0.414999990724027,0.348029239996762)
% --(axis cs:0.409999990835786,0.345495137006861)
% --(axis cs:0.404999990947545,0.3429348168487)
% --(axis cs:0.399999991059303,0.340354493698975)
% --(axis cs:0.394999991171062,0.337789870303694)
% --(axis cs:0.389999991282821,0.335205801384271)
% --(axis cs:0.384999991394579,0.332578348947944)
% --(axis cs:0.379999991506338,0.32990961709774)
% --(axis cs:0.374999991618097,0.327249707679)
% --(axis cs:0.369999991729856,0.324563048667938)
% --(axis cs:0.364999991841614,0.321866331028157)
% --(axis cs:0.359999991953373,0.319158542574693)
% --(axis cs:0.354999992065132,0.316466704556033)
% --(axis cs:0.34999999217689,0.31374778768912)
% --(axis cs:0.344999992288649,0.311004144993009)
% --(axis cs:0.339999992400408,0.308250753258195)
% --(axis cs:0.334999992512167,0.305521583272315)
% --(axis cs:0.329999992623925,0.302744054759145)
% --(axis cs:0.324999992735684,0.299913996238354)
% --(axis cs:0.319999992847443,0.297069249928117)
% --(axis cs:0.314999992959201,0.294219340450701)
% --(axis cs:0.30999999307096,0.291342974674745)
% --(axis cs:0.304999993182719,0.288448772495865)
% --(axis cs:0.299999993294477,0.285541348061667)
% --(axis cs:0.294999993406236,0.28270302530654)
% --(axis cs:0.289999993517995,0.279841306072054)
% --(axis cs:0.284999993629754,0.276968977459032)
% --(axis cs:0.279999993741512,0.274060557995169)
% --(axis cs:0.274999993853271,0.271133796324603)
% --(axis cs:0.26999999396503,0.268170750674561)
% --(axis cs:0.264999994076788,0.265182288949878)
% --(axis cs:0.259999994188547,0.262184279507878)
% --(axis cs:0.254999994300306,0.25925803369192)
% --(axis cs:0.249999994412065,0.256331025477006)
% --(axis cs:0.244999994523823,0.253402034823111)
% --(axis cs:0.239999994635582,0.250508650220522)
% --(axis cs:0.234999994747341,0.247689148309062)
% --(axis cs:0.229999994859099,0.244880140444648)
% --(axis cs:0.224999994970858,0.242046699387587)
% --(axis cs:0.219999995082617,0.239186093521672)
% --(axis cs:0.214999995194376,0.236397313277547)
% --(axis cs:0.209999995306134,0.233639262380815)
% --(axis cs:0.204999995417893,0.230969664637113)
% --(axis cs:0.199999995529652,0.228355032460781)
% --(axis cs:0.19499999564141,0.22580687581028)
% --(axis cs:0.189999995753169,0.223264714471965)
% --(axis cs:0.184999995864928,0.220692950013391)
% --(axis cs:0.179999995976686,0.218100626073155)
% --(axis cs:0.174999996088445,0.215579089457809)
% --(axis cs:0.169999996200204,0.213054996818397)
% --(axis cs:0.164999996311963,0.210489730287167)
% --(axis cs:0.159999996423721,0.207904919033045)
% --(axis cs:0.15499999653548,0.205351943198339)
% --(axis cs:0.149999996647239,0.202773866407403)
% --(axis cs:0.144999996758997,0.200162856899296)
% --(axis cs:0.139999996870756,0.197499526284553)
% --(axis cs:0.134999996982515,0.194856788489981)
% --(axis cs:0.129999997094274,0.192131576628439)
% --(axis cs:0.124999997206032,0.189313496542394)
% --(axis cs:0.119999997317791,0.186420357989294)
% --(axis cs:0.11499999742955,0.18356440234626)
% --(axis cs:0.109999997541308,0.180589700072097)
% --(axis cs:0.104999997653067,0.17749141917182)
% --(axis cs:0.0999999977648258,0.174274378331976)
% --(axis cs:0.0949999978765845,0.171135413018651)
% --(axis cs:0.0899999979883432,0.1679158439598)
% --(axis cs:0.0849999981001019,0.164660100636731)
% --(axis cs:0.0799999982118607,0.161369633955076)
% --(axis cs:0.0749999983236194,0.158447923434911)
% --(axis cs:0.0699999984353781,0.155508515442735)
% --(axis cs:0.0649999985471368,0.152562822303125)
% --(axis cs:0.0599999986588955,0.149644851810824)
% --(axis cs:0.0549999987706542,0.147344385922198)
% --(axis cs:0.0499999988824129,0.144624422975886)
% --(axis cs:0.0449999989941716,0.141438255943546)
% --(axis cs:0.0399999991059303,0.137329900200645)
% --(axis cs:0.034999999217689,0.132848545513201)
% --(axis cs:0.0299999993294477,0.127554194425302)
% --(axis cs:0.0249999994412065,0.122188839704902)
% --(axis cs:0.0199999995529652,0.117637873483173)
% --(axis cs:0.0149999996647239,0.114162500857339)
% --(axis cs:0.00999999977648258,0.110827012774136)
% --(axis cs:0.00499999988824129,0.104644967318169)
% --cycle;

% \path [fill=red, fill opacity=0.4, ultra thick]
% (axis cs:0.00499999988824129,0.115323148725986)
% --(axis cs:0.00499999988824129,0.0777649893221378)
% --(axis cs:0.00999999977648258,0.0848498704497275)
% --(axis cs:0.0149999996647239,0.0876242482072469)
% --(axis cs:0.0199999995529652,0.0903150550499889)
% --(axis cs:0.0249999994412065,0.0948590644829372)
% --(axis cs:0.0299999993294477,0.0987825867679661)
% --(axis cs:0.034999999217689,0.101518560374524)
% --(axis cs:0.0399999991059303,0.103652610297194)
% --(axis cs:0.0449999989941716,0.105969880028875)
% --(axis cs:0.0499999988824129,0.107956286707888)
% --(axis cs:0.0549999987706542,0.109656123009977)
% --(axis cs:0.0599999986588955,0.111217858392856)
% --(axis cs:0.0649999985471368,0.113106333385324)
% --(axis cs:0.0699999984353781,0.114675728616817)
% --(axis cs:0.0749999983236194,0.115936028405548)
% --(axis cs:0.0799999982118607,0.116997216418278)
% --(axis cs:0.0849999981001019,0.118160586497656)
% --(axis cs:0.0899999979883432,0.119174678313352)
% --(axis cs:0.0949999978765845,0.120074064296149)
% --(axis cs:0.0999999977648258,0.120937919501056)
% --(axis cs:0.104999997653067,0.121911309847295)
% --(axis cs:0.109999997541308,0.122844218669428)
% --(axis cs:0.11499999742955,0.123683973411858)
% --(axis cs:0.119999997317791,0.124510987407826)
% --(axis cs:0.124999997206032,0.125438034955452)
% --(axis cs:0.129999997094274,0.12632974188517)
% --(axis cs:0.134999996982515,0.127174117710089)
% --(axis cs:0.139999996870756,0.127993114756346)
% --(axis cs:0.144999996758997,0.128889133139415)
% --(axis cs:0.149999996647239,0.129824534793162)
% --(axis cs:0.15499999653548,0.130766464833809)
% --(axis cs:0.159999996423721,0.131703411098832)
% --(axis cs:0.164999996311963,0.132769650062524)
% --(axis cs:0.169999996200204,0.133879472519765)
% --(axis cs:0.174999996088445,0.134964031838909)
% --(axis cs:0.179999995976686,0.136000339720473)
% --(axis cs:0.184999995864928,0.137086638445677)
% --(axis cs:0.189999995753169,0.138221114496175)
% --(axis cs:0.19499999564141,0.139378416511888)
% --(axis cs:0.199999995529652,0.140601278382238)
% --(axis cs:0.204999995417893,0.141873633248089)
% --(axis cs:0.209999995306134,0.143158456069269)
% --(axis cs:0.214999995194376,0.144433311498)
% --(axis cs:0.219999995082617,0.145735375410912)
% --(axis cs:0.224999994970858,0.147056177021314)
% --(axis cs:0.229999994859099,0.148393366880473)
% --(axis cs:0.234999994747341,0.149766533633098)
% --(axis cs:0.239999994635582,0.151182438867571)
% --(axis cs:0.244999994523823,0.152603374087243)
% --(axis cs:0.249999994412065,0.15402858502602)
% --(axis cs:0.254999994300306,0.155438285344679)
% --(axis cs:0.259999994188547,0.15681428323794)
% --(axis cs:0.264999994076788,0.158192472258403)
% --(axis cs:0.26999999396503,0.159540307337155)
% --(axis cs:0.274999993853271,0.160855012875347)
% --(axis cs:0.279999993741512,0.162117701960092)
% --(axis cs:0.284999993629754,0.16334837724874)
% --(axis cs:0.289999993517995,0.164537469557674)
% --(axis cs:0.294999993406236,0.165765728361017)
% --(axis cs:0.299999993294477,0.166912601846999)
% --(axis cs:0.304999993182719,0.168086855671557)
% --(axis cs:0.30999999307096,0.169226722341343)
% --(axis cs:0.314999992959201,0.170308198000797)
% --(axis cs:0.319999992847443,0.171380096410684)
% --(axis cs:0.324999992735684,0.17243664785745)
% --(axis cs:0.329999992623925,0.173457349164852)
% --(axis cs:0.334999992512167,0.174462804215311)
% --(axis cs:0.339999992400408,0.175472581807845)
% --(axis cs:0.344999992288649,0.176454656704429)
% --(axis cs:0.34999999217689,0.177412862818855)
% --(axis cs:0.354999992065132,0.178337525799806)
% --(axis cs:0.359999991953373,0.179250928049253)
% --(axis cs:0.364999991841614,0.180240352779148)
% --(axis cs:0.369999991729856,0.18122981942378)
% --(axis cs:0.374999991618097,0.182228511910347)
% --(axis cs:0.379999991506338,0.1832528188409)
% --(axis cs:0.384999991394579,0.184288305595684)
% --(axis cs:0.389999991282821,0.185307995045993)
% --(axis cs:0.394999991171062,0.186342496633504)
% --(axis cs:0.399999991059303,0.187361104642761)
% --(axis cs:0.404999990947545,0.188318019747563)
% --(axis cs:0.409999990835786,0.189283604460759)
% --(axis cs:0.414999990724027,0.190191776510701)
% --(axis cs:0.419999990612268,0.191065816054047)
% --(axis cs:0.42499999050051,0.191926409777511)
% --(axis cs:0.429999990388751,0.192748515305735)
% --(axis cs:0.434999990276992,0.193521901309966)
% --(axis cs:0.439999990165234,0.194260040597891)
% --(axis cs:0.444999990053475,0.194991816688482)
% --(axis cs:0.449999989941716,0.195757637184958)
% --(axis cs:0.454999989829957,0.196460982648037)
% --(axis cs:0.459999989718199,0.197146788064293)
% --(axis cs:0.46499998960644,0.197848506176417)
% --(axis cs:0.469999989494681,0.198537370176233)
% --(axis cs:0.474999989382923,0.199270514545252)
% --(axis cs:0.479999989271164,0.199982059127765)
% --(axis cs:0.484999989159405,0.200772436117638)
% --(axis cs:0.489999989047647,0.201595229414353)
% --(axis cs:0.494999988935888,0.202401563889188)
% --(axis cs:0.494999988935888,0.267334673739007)
% --(axis cs:0.494999988935888,0.267334673739007)
% --(axis cs:0.489999989047647,0.266392663090109)
% --(axis cs:0.484999989159405,0.265431700082125)
% --(axis cs:0.479999989271164,0.26449651625256)
% --(axis cs:0.474999989382923,0.263547774299235)
% --(axis cs:0.469999989494681,0.262567320963961)
% --(axis cs:0.46499998960644,0.261596730645664)
% --(axis cs:0.459999989718199,0.260611383168248)
% --(axis cs:0.454999989829957,0.259621167722351)
% --(axis cs:0.449999989941716,0.258617351136264)
% --(axis cs:0.444999990053475,0.257580110177751)
% --(axis cs:0.439999990165234,0.256514147628608)
% --(axis cs:0.434999990276992,0.255442177868827)
% --(axis cs:0.429999990388751,0.254355594624831)
% --(axis cs:0.42499999050051,0.253220909276357)
% --(axis cs:0.419999990612268,0.252051406436885)
% --(axis cs:0.414999990724027,0.250890784152269)
% --(axis cs:0.409999990835786,0.249696506193748)
% --(axis cs:0.404999990947545,0.248492273800554)
% --(axis cs:0.399999991059303,0.247235360401502)
% --(axis cs:0.394999991171062,0.245983897039866)
% --(axis cs:0.389999991282821,0.244681379229696)
% --(axis cs:0.384999991394579,0.243365549842991)
% --(axis cs:0.379999991506338,0.242016125684251)
% --(axis cs:0.374999991618097,0.240693186273677)
% --(axis cs:0.369999991729856,0.239328290483388)
% --(axis cs:0.364999991841614,0.237969106358381)
% --(axis cs:0.359999991953373,0.23654514483009)
% --(axis cs:0.354999992065132,0.235193980954573)
% --(axis cs:0.34999999217689,0.23381502229776)
% --(axis cs:0.344999992288649,0.232433165480359)
% --(axis cs:0.339999992400408,0.231069015293304)
% --(axis cs:0.334999992512167,0.229701997185493)
% --(axis cs:0.329999992623925,0.228373500181266)
% --(axis cs:0.324999992735684,0.227069038231186)
% --(axis cs:0.319999992847443,0.225790645756163)
% --(axis cs:0.314999992959201,0.224526033075727)
% --(axis cs:0.30999999307096,0.223262333390923)
% --(axis cs:0.304999993182719,0.221957139399408)
% --(axis cs:0.299999993294477,0.220580555586704)
% --(axis cs:0.294999993406236,0.219275543817263)
% --(axis cs:0.289999993517995,0.217955873914347)
% --(axis cs:0.284999993629754,0.216651929831597)
% --(axis cs:0.279999993741512,0.215340723840481)
% --(axis cs:0.274999993853271,0.214109186380535)
% --(axis cs:0.26999999396503,0.212878444754997)
% --(axis cs:0.264999994076788,0.211643588762323)
% --(axis cs:0.259999994188547,0.210439511097812)
% --(axis cs:0.254999994300306,0.20930654830538)
% --(axis cs:0.249999994412065,0.208188499089921)
% --(axis cs:0.244999994523823,0.207043877158112)
% --(axis cs:0.239999994635582,0.205969163880385)
% --(axis cs:0.234999994747341,0.204925208664335)
% --(axis cs:0.229999994859099,0.203932147593429)
% --(axis cs:0.224999994970858,0.202873637206446)
% --(axis cs:0.219999995082617,0.201803304814188)
% --(axis cs:0.214999995194376,0.200756940434422)
% --(axis cs:0.209999995306134,0.199689594290334)
% --(axis cs:0.204999995417893,0.19876871600107)
% --(axis cs:0.199999995529652,0.197834880456701)
% --(axis cs:0.19499999564141,0.196936268207326)
% --(axis cs:0.189999995753169,0.195942748293694)
% --(axis cs:0.184999995864928,0.194896809192459)
% --(axis cs:0.179999995976686,0.193810291666759)
% --(axis cs:0.174999996088445,0.192796912316492)
% --(axis cs:0.169999996200204,0.191724467277622)
% --(axis cs:0.164999996311963,0.19057212449875)
% --(axis cs:0.159999996423721,0.18939432956688)
% --(axis cs:0.15499999653548,0.188285607901092)
% --(axis cs:0.149999996647239,0.187143957677883)
% --(axis cs:0.144999996758997,0.185978488205353)
% --(axis cs:0.139999996870756,0.184764824252658)
% --(axis cs:0.134999996982515,0.183561875698163)
% --(axis cs:0.129999997094274,0.182276828459588)
% --(axis cs:0.124999997206032,0.180852493587045)
% --(axis cs:0.119999997317791,0.179334688886043)
% --(axis cs:0.11499999742955,0.177896907617686)
% --(axis cs:0.109999997541308,0.176234160408414)
% --(axis cs:0.104999997653067,0.174359363712783)
% --(axis cs:0.0999999977648258,0.172277012117884)
% --(axis cs:0.0949999978765845,0.170112583160872)
% --(axis cs:0.0899999979883432,0.167660647011338)
% --(axis cs:0.0849999981001019,0.164889582146963)
% --(axis cs:0.0799999982118607,0.161849751472089)
% --(axis cs:0.0749999983236194,0.158919588601636)
% --(axis cs:0.0699999984353781,0.155732267660274)
% --(axis cs:0.0649999985471368,0.152350414729004)
% --(axis cs:0.0599999986588955,0.148816315729496)
% --(axis cs:0.0549999987706542,0.145846369950568)
% --(axis cs:0.0499999988824129,0.142431785960871)
% --(axis cs:0.0449999989941716,0.139036829363225)
% --(axis cs:0.0399999991059303,0.135173732269162)
% --(axis cs:0.034999999217689,0.131664782662156)
% --(axis cs:0.0299999993294477,0.127698206181957)
% --(axis cs:0.0249999994412065,0.12378645301857)
% --(axis cs:0.0199999995529652,0.120456069490315)
% --(axis cs:0.0149999996647239,0.118911521950235)
% --(axis cs:0.00999999977648258,0.117899680506565)
% --(axis cs:0.00499999988824129,0.115323148725986)
% --cycle;

% \path [fill=green!50.1960784313725!black, fill opacity=0.4, ultra thick]
% (axis cs:0.00499999988824129,0.0905936145398397)
% --(axis cs:0.00499999988824129,0.0619344746316198)
% --(axis cs:0.00999999977648258,0.0643951706717472)
% --(axis cs:0.0149999996647239,0.0653294359239248)
% --(axis cs:0.0199999995529652,0.066889258578383)
% --(axis cs:0.0249999994412065,0.070217011365269)
% --(axis cs:0.0299999993294477,0.0738559794930689)
% --(axis cs:0.034999999217689,0.0770621182568461)
% --(axis cs:0.0399999991059303,0.0795285510342601)
% --(axis cs:0.0449999989941716,0.0819562772393401)
% --(axis cs:0.0499999988824129,0.0846317128454203)
% --(axis cs:0.0549999987706542,0.0866215792615274)
% --(axis cs:0.0599999986588955,0.0879249477371107)
% --(axis cs:0.0649999985471368,0.089615614995606)
% --(axis cs:0.0699999984353781,0.0915062668902724)
% --(axis cs:0.0749999983236194,0.0928340885431344)
% --(axis cs:0.0799999982118607,0.0935478286933084)
% --(axis cs:0.0849999981001019,0.0946570942411352)
% --(axis cs:0.0899999979883432,0.0960547828902234)
% --(axis cs:0.0949999978765845,0.0970455563206244)
% --(axis cs:0.0999999977648258,0.0976856848693922)
% --(axis cs:0.104999997653067,0.0988120199618261)
% --(axis cs:0.109999997541308,0.100077116232881)
% --(axis cs:0.11499999742955,0.10081090440166)
% --(axis cs:0.119999997317791,0.101369310139692)
% --(axis cs:0.124999997206032,0.102470062699565)
% --(axis cs:0.129999997094274,0.103678925529724)
% --(axis cs:0.134999996982515,0.104503430747126)
% --(axis cs:0.139999996870756,0.10527489014677)
% --(axis cs:0.144999996758997,0.106557498751393)
% --(axis cs:0.149999996647239,0.107900738740209)
% --(axis cs:0.15499999653548,0.10883821729714)
% --(axis cs:0.159999996423721,0.109888269938818)
% --(axis cs:0.164999996311963,0.111501055981534)
% --(axis cs:0.169999996200204,0.113144602110863)
% --(axis cs:0.174999996088445,0.114368129569538)
% --(axis cs:0.179999995976686,0.115903736671615)
% --(axis cs:0.184999995864928,0.117974529655571)
% --(axis cs:0.189999995753169,0.11995925349499)
% --(axis cs:0.19499999564141,0.12161329930135)
% --(axis cs:0.199999995529652,0.12374732758748)
% --(axis cs:0.204999995417893,0.126334951915038)
% --(axis cs:0.209999995306134,0.128740577060067)
% --(axis cs:0.214999995194376,0.130913732113491)
% --(axis cs:0.219999995082617,0.133632685206692)
% --(axis cs:0.224999994970858,0.136677889548922)
% --(axis cs:0.229999994859099,0.139437646968747)
% --(axis cs:0.234999994747341,0.142045095562463)
% --(axis cs:0.239999994635582,0.145220930955307)
% --(axis cs:0.244999994523823,0.148591642267018)
% --(axis cs:0.249999994412065,0.151690540837371)
% --(axis cs:0.254999994300306,0.154706347173512)
% --(axis cs:0.259999994188547,0.158191905295761)
% --(axis cs:0.264999994076788,0.161801702369791)
% --(axis cs:0.26999999396503,0.165162325427477)
% --(axis cs:0.274999993853271,0.168490306013928)
% --(axis cs:0.279999993741512,0.172220027384902)
% --(axis cs:0.284999993629754,0.176040929434169)
% --(axis cs:0.289999993517995,0.179646676320252)
% --(axis cs:0.294999993406236,0.183271356702235)
% --(axis cs:0.299999993294477,0.18720170566392)
% --(axis cs:0.304999993182719,0.19119806081624)
% --(axis cs:0.30999999307096,0.195065083762147)
% --(axis cs:0.314999992959201,0.19892778263886)
% --(axis cs:0.319999992847443,0.203016479622035)
% --(axis cs:0.324999992735684,0.207153527058704)
% --(axis cs:0.329999992623925,0.211187850040957)
% --(axis cs:0.334999992512167,0.21521023986656)
% --(axis cs:0.339999992400408,0.219360471671798)
% --(axis cs:0.344999992288649,0.223534655355488)
% --(axis cs:0.34999999217689,0.227639825365903)
% --(axis cs:0.354999992065132,0.231717608236221)
% --(axis cs:0.359999991953373,0.235873744249659)
% --(axis cs:0.364999991841614,0.240057808639197)
% --(axis cs:0.369999991729856,0.244180670116588)
% --(axis cs:0.374999991618097,0.248259982864188)
% --(axis cs:0.379999991506338,0.252382722043005)
% --(axis cs:0.384999991394579,0.256504301834792)
% --(axis cs:0.389999991282821,0.260562441872667)
% --(axis cs:0.394999991171062,0.264574062216608)
% --(axis cs:0.399999991059303,0.268600965216978)
% --(axis cs:0.404999990947545,0.272627398714064)
% --(axis cs:0.409999990835786,0.276605664682336)
% --(axis cs:0.414999990724027,0.280524440081107)
% --(axis cs:0.419999990612268,0.284431321079858)
% --(axis cs:0.42499999050051,0.288328906086199)
% --(axis cs:0.429999990388751,0.292179750519874)
% --(axis cs:0.434999990276992,0.295960383406113)
% --(axis cs:0.439999990165234,0.299711016105431)
% --(axis cs:0.444999990053475,0.303457807739307)
% --(axis cs:0.449999989941716,0.307180385472404)
% --(axis cs:0.454999989829957,0.310837229203332)
% --(axis cs:0.459999989718199,0.314452361436014)
% --(axis cs:0.46499998960644,0.318058200395016)
% --(axis cs:0.469999989494681,0.321645320655308)
% --(axis cs:0.474999989382923,0.325177329576675)
% --(axis cs:0.479999989271164,0.328657164928547)
% --(axis cs:0.484999989159405,0.33212724566744)
% --(axis cs:0.489999989047647,0.335585535055852)
% --(axis cs:0.494999988935888,0.339012015787009)
% --(axis cs:0.494999988935888,0.423174016440028)
% --(axis cs:0.494999988935888,0.423174016440028)
% --(axis cs:0.489999989047647,0.419759463528283)
% --(axis cs:0.484999989159405,0.416317490283102)
% --(axis cs:0.479999989271164,0.412858982173539)
% --(axis cs:0.474999989382923,0.409357781168524)
% --(axis cs:0.469999989494681,0.405791279764874)
% --(axis cs:0.46499998960644,0.402177130713504)
% --(axis cs:0.459999989718199,0.398556507571238)
% --(axis cs:0.454999989829957,0.394919299467151)
% --(axis cs:0.449999989941716,0.391190949706465)
% --(axis cs:0.444999990053475,0.387412097059352)
% --(axis cs:0.439999990165234,0.383616123636629)
% --(axis cs:0.434999990276992,0.379805317071009)
% --(axis cs:0.429999990388751,0.375919802399306)
% --(axis cs:0.42499999050051,0.371953023372403)
% --(axis cs:0.419999990612268,0.367963560465907)
% --(axis cs:0.414999990724027,0.363970716732445)
% --(axis cs:0.409999990835786,0.35989908220315)
% --(axis cs:0.404999990947545,0.355742462386361)
% --(axis cs:0.399999991059303,0.351545364876176)
% --(axis cs:0.394999991171062,0.347353337732869)
% --(axis cs:0.389999991282821,0.343109011586739)
% --(axis cs:0.384999991394579,0.338768689848453)
% --(axis cs:0.379999991506338,0.334387266326286)
% --(axis cs:0.374999991618097,0.329998260998805)
% --(axis cs:0.369999991729856,0.325577518838651)
% --(axis cs:0.364999991841614,0.321069897028989)
% --(axis cs:0.359999991953373,0.316507100068982)
% --(axis cs:0.354999992065132,0.311954876900811)
% --(axis cs:0.34999999217689,0.307406588197479)
% --(axis cs:0.344999992288649,0.302773026542977)
% --(axis cs:0.339999992400408,0.298087564223247)
% --(axis cs:0.334999992512167,0.293378937834227)
% --(axis cs:0.329999992623925,0.288746056057768)
% --(axis cs:0.324999992735684,0.284049694797799)
% --(axis cs:0.319999992847443,0.279261448915349)
% --(axis cs:0.314999992959201,0.274471284377216)
% --(axis cs:0.30999999307096,0.269775059475637)
% --(axis cs:0.304999993182719,0.265048965685354)
% --(axis cs:0.299999993294477,0.260192919307162)
% --(axis cs:0.294999993406236,0.255329638241039)
% --(axis cs:0.289999993517995,0.250674088490193)
% --(axis cs:0.284999993629754,0.245957231738513)
% --(axis cs:0.279999993741512,0.241119209438786)
% --(axis cs:0.274999993853271,0.236259484595615)
% --(axis cs:0.26999999396503,0.23166762701484)
% --(axis cs:0.264999994076788,0.227155098158826)
% --(axis cs:0.259999994188547,0.222385497861896)
% --(axis cs:0.254999994300306,0.217734842144771)
% --(axis cs:0.249999994412065,0.21357792776023)
% --(axis cs:0.244999994523823,0.209439746624466)
% --(axis cs:0.239999994635582,0.205044221603139)
% --(axis cs:0.234999994747341,0.200774445671174)
% --(axis cs:0.229999994859099,0.19720343831519)
% --(axis cs:0.224999994970858,0.193577620014021)
% --(axis cs:0.219999995082617,0.189537076352577)
% --(axis cs:0.214999995194376,0.185866844768108)
% --(axis cs:0.209999995306134,0.182953097505703)
% --(axis cs:0.204999995417893,0.180004656083975)
% --(axis cs:0.199999995529652,0.176574702263556)
% --(axis cs:0.19499999564141,0.173618403888439)
% --(axis cs:0.189999995753169,0.171530429454806)
% --(axis cs:0.184999995864928,0.16897502876134)
% --(axis cs:0.179999995976686,0.166068018225678)
% --(axis cs:0.174999996088445,0.163722713872973)
% --(axis cs:0.169999996200204,0.1619771403708)
% --(axis cs:0.164999996311963,0.159892748969577)
% --(axis cs:0.159999996423721,0.157498667698726)
% --(axis cs:0.15499999653548,0.155816834776973)
% --(axis cs:0.149999996647239,0.154719875326475)
% --(axis cs:0.144999996758997,0.153007838280282)
% --(axis cs:0.139999996870756,0.151022497238454)
% --(axis cs:0.134999996982515,0.149646427987025)
% --(axis cs:0.129999997094274,0.148754034290532)
% --(axis cs:0.124999997206032,0.147201628289117)
% --(axis cs:0.119999997317791,0.145505880028255)
% --(axis cs:0.11499999742955,0.144562323745085)
% --(axis cs:0.109999997541308,0.143760930331894)
% --(axis cs:0.104999997653067,0.142221298716994)
% --(axis cs:0.0999999977648258,0.14050204433664)
% --(axis cs:0.0949999978765845,0.139287454897502)
% --(axis cs:0.0899999979883432,0.13769892538765)
% --(axis cs:0.0849999981001019,0.135321896426039)
% --(axis cs:0.0799999982118607,0.132861408165901)
% --(axis cs:0.0749999983236194,0.130649481806007)
% --(axis cs:0.0699999984353781,0.12791689037287)
% --(axis cs:0.0649999985471368,0.12474647528303)
% --(axis cs:0.0599999986588955,0.121533834934194)
% --(axis cs:0.0549999987706542,0.119088036008425)
% --(axis cs:0.0499999988824129,0.116099491437273)
% --(axis cs:0.0449999989941716,0.113040665141123)
% --(axis cs:0.0399999991059303,0.110558637406503)
% --(axis cs:0.034999999217689,0.109022654615685)
% --(axis cs:0.0299999993294477,0.106104931973609)
% --(axis cs:0.0249999994412065,0.102545191119572)
% --(axis cs:0.0199999995529652,0.0997331082189722)
% --(axis cs:0.0149999996647239,0.0963579984910028)
% --(axis cs:0.00999999977648258,0.0926075090910755)
% --(axis cs:0.00499999988824129,0.0905936145398397)
% --cycle;

% \path [fill=color0, fill opacity=0.4, ultra thick]
% (axis cs:0.00499999988824129,0.0723257914846999)
% --(axis cs:0.00499999988824129,0.044429407423608)
% --(axis cs:0.00999999977648258,0.0539409375767771)
% --(axis cs:0.0149999996647239,0.053225250659491)
% --(axis cs:0.0199999995529652,0.0531345400969327)
% --(axis cs:0.0249999994412065,0.0551293052876465)
% --(axis cs:0.0299999993294477,0.0571697549564637)
% --(axis cs:0.034999999217689,0.0588305271295207)
% --(axis cs:0.0399999991059303,0.0599630955190938)
% --(axis cs:0.0449999989941716,0.0617028736620725)
% --(axis cs:0.0499999988824129,0.0634576459598399)
% --(axis cs:0.0549999987706542,0.0646482099618023)
% --(axis cs:0.0599999986588955,0.0654319256960148)
% --(axis cs:0.0649999985471368,0.0664430674285895)
% --(axis cs:0.0699999984353781,0.0677677144711779)
% --(axis cs:0.0749999983236194,0.0687458842516745)
% --(axis cs:0.0799999982118607,0.0694806170757633)
% --(axis cs:0.0849999981001019,0.070411033322479)
% --(axis cs:0.0899999979883432,0.071418889230684)
% --(axis cs:0.0949999978765845,0.0720862912562898)
% --(axis cs:0.0999999977648258,0.0727198262668881)
% --(axis cs:0.104999997653067,0.0735291859354889)
% --(axis cs:0.109999997541308,0.0743550325112774)
% --(axis cs:0.11499999742955,0.0748841847476781)
% --(axis cs:0.119999997317791,0.0753862491825369)
% --(axis cs:0.124999997206032,0.0761232292564328)
% --(axis cs:0.129999997094274,0.0768467600382069)
% --(axis cs:0.134999996982515,0.077428795486793)
% --(axis cs:0.139999996870756,0.0780102705271391)
% --(axis cs:0.144999996758997,0.0788065685103195)
% --(axis cs:0.149999996647239,0.0796340660563939)
% --(axis cs:0.15499999653548,0.0802784814557429)
% --(axis cs:0.159999996423721,0.0810320538343023)
% --(axis cs:0.164999996311963,0.0819777925142018)
% --(axis cs:0.169999996200204,0.0828753442214418)
% --(axis cs:0.174999996088445,0.0836859806752981)
% --(axis cs:0.179999995976686,0.0847211183128134)
% --(axis cs:0.184999995864928,0.0859697191411594)
% --(axis cs:0.189999995753169,0.0871684657718662)
% --(axis cs:0.19499999564141,0.0884106620521939)
% --(axis cs:0.199999995529652,0.0899353354768147)
% --(axis cs:0.204999995417893,0.0915776381551231)
% --(axis cs:0.209999995306134,0.0931094477164975)
% --(axis cs:0.214999995194376,0.0947679461792401)
% --(axis cs:0.219999995082617,0.0966536621453462)
% --(axis cs:0.224999994970858,0.0985770539479435)
% --(axis cs:0.229999994859099,0.100382971438614)
% --(axis cs:0.234999994747341,0.102384216571466)
% --(axis cs:0.239999994635582,0.104543701349481)
% --(axis cs:0.244999994523823,0.106716009165406)
% --(axis cs:0.249999994412065,0.108803642419831)
% --(axis cs:0.254999994300306,0.111045089737367)
% --(axis cs:0.259999994188547,0.113373893624675)
% --(axis cs:0.264999994076788,0.115722334162695)
% --(axis cs:0.26999999396503,0.118004115494962)
% --(axis cs:0.274999993853271,0.120463270142621)
% --(axis cs:0.279999993741512,0.12298102677754)
% --(axis cs:0.284999993629754,0.125502318493234)
% --(axis cs:0.289999993517995,0.128012918856024)
% --(axis cs:0.294999993406236,0.130686107903321)
% --(axis cs:0.299999993294477,0.133411083929857)
% --(axis cs:0.304999993182719,0.136173687226338)
% --(axis cs:0.30999999307096,0.138994660887709)
% --(axis cs:0.314999992959201,0.141929352248594)
% --(axis cs:0.319999992847443,0.144883022930397)
% --(axis cs:0.324999992735684,0.147866996680735)
% --(axis cs:0.329999992623925,0.150922012172414)
% --(axis cs:0.334999992512167,0.154015413803879)
% --(axis cs:0.339999992400408,0.157138003742365)
% --(axis cs:0.344999992288649,0.160320700672981)
% --(axis cs:0.34999999217689,0.163569127166642)
% --(axis cs:0.354999992065132,0.166803792500647)
% --(axis cs:0.359999991953373,0.17005880902664)
% --(axis cs:0.364999991841614,0.17337841714836)
% --(axis cs:0.369999991729856,0.176740578104524)
% --(axis cs:0.374999991618097,0.180065008068346)
% --(axis cs:0.379999991506338,0.183420187240154)
% --(axis cs:0.384999991394579,0.186842993798051)
% --(axis cs:0.389999991282821,0.19027679098263)
% --(axis cs:0.394999991171062,0.19365692335345)
% --(axis cs:0.399999991059303,0.197066645103535)
% --(axis cs:0.404999990947545,0.200532693225683)
% --(axis cs:0.409999990835786,0.203987211326878)
% --(axis cs:0.414999990724027,0.207390076622503)
% --(axis cs:0.419999990612268,0.210809042670906)
% --(axis cs:0.42499999050051,0.214265009620529)
% --(axis cs:0.429999990388751,0.217692004672694)
% --(axis cs:0.434999990276992,0.221060653173686)
% --(axis cs:0.439999990165234,0.22443459767659)
% --(axis cs:0.444999990053475,0.227842566772114)
% --(axis cs:0.449999989941716,0.231219303613149)
% --(axis cs:0.454999989829957,0.234539028396446)
% --(axis cs:0.459999989718199,0.237856219059607)
% --(axis cs:0.46499998960644,0.241199396628021)
% --(axis cs:0.469999989494681,0.244511696995495)
% --(axis cs:0.474999989382923,0.247775942063147)
% --(axis cs:0.479999989271164,0.251032512736893)
% --(axis cs:0.484999989159405,0.254305697231816)
% --(axis cs:0.489999989047647,0.257556838628418)
% --(axis cs:0.494999988935888,0.260755094948821)
% --(axis cs:0.494999988935888,0.341926402429029)
% --(axis cs:0.494999988935888,0.341926402429029)
% --(axis cs:0.489999989047647,0.338510900062983)
% --(axis cs:0.484999989159405,0.335035267459041)
% --(axis cs:0.479999989271164,0.331522407498773)
% --(axis cs:0.474999989382923,0.328003349630812)
% --(axis cs:0.469999989494681,0.324464654707762)
% --(axis cs:0.46499998960644,0.320864120864743)
% --(axis cs:0.459999989718199,0.317215283600589)
% --(axis cs:0.454999989829957,0.313567078846323)
% --(axis cs:0.449999989941716,0.30990457170794)
% --(axis cs:0.444999990053475,0.306189159276113)
% --(axis cs:0.439999990165234,0.30241491981555)
% --(axis cs:0.434999990276992,0.298633194248247)
% --(axis cs:0.429999990388751,0.294848089913116)
% --(axis cs:0.42499999050051,0.291014252387845)
% --(axis cs:0.419999990612268,0.287098815666206)
% --(axis cs:0.414999990724027,0.283173509660718)
% --(axis cs:0.409999990835786,0.279255053703552)
% --(axis cs:0.404999990947545,0.275307974699719)
% --(axis cs:0.399999991059303,0.27127141985542)
% --(axis cs:0.394999991171062,0.267225978365104)
% --(axis cs:0.389999991282821,0.26320793646448)
% --(axis cs:0.384999991394579,0.259174470227904)
% --(axis cs:0.379999991506338,0.25503223149251)
% --(axis cs:0.374999991618097,0.250877183710329)
% --(axis cs:0.369999991729856,0.246779445665621)
% --(axis cs:0.364999991841614,0.242696043935185)
% --(axis cs:0.359999991953373,0.238493908006504)
% --(axis cs:0.354999992065132,0.234279346372542)
% --(axis cs:0.34999999217689,0.230167962374849)
% --(axis cs:0.344999992288649,0.226099440006191)
% --(axis cs:0.339999992400408,0.221904005637417)
% --(axis cs:0.334999992512167,0.217678284378716)
% --(axis cs:0.329999992623925,0.213619485493408)
% --(axis cs:0.324999992735684,0.209624210894439)
% --(axis cs:0.319999992847443,0.205471327670699)
% --(axis cs:0.314999992959201,0.201280285624445)
% --(axis cs:0.30999999307096,0.197330456073162)
% --(axis cs:0.304999993182719,0.193441526603557)
% --(axis cs:0.299999993294477,0.18937817683882)
% --(axis cs:0.294999993406236,0.185264514245044)
% --(axis cs:0.289999993517995,0.181489606882163)
% --(axis cs:0.284999993629754,0.177750759890497)
% --(axis cs:0.279999993741512,0.173790036493232)
% --(axis cs:0.274999993853271,0.169789573569113)
% --(axis cs:0.26999999396503,0.166247751478426)
% --(axis cs:0.264999994076788,0.162768793100849)
% --(axis cs:0.259999994188547,0.159025680721607)
% --(axis cs:0.254999994300306,0.155347280358988)
% --(axis cs:0.249999994412065,0.152260099835455)
% --(axis cs:0.244999994523823,0.149190273958979)
% --(axis cs:0.239999994635582,0.145793489695186)
% --(axis cs:0.234999994747341,0.142542096644207)
% --(axis cs:0.229999994859099,0.139972099925327)
% --(axis cs:0.224999994970858,0.137322382463338)
% --(axis cs:0.219999995082617,0.134265362729042)
% --(axis cs:0.214999995194376,0.131470875989588)
% --(axis cs:0.209999995306134,0.129378018955632)
% --(axis cs:0.204999995417893,0.127174460606692)
% --(axis cs:0.199999995529652,0.124619924665411)
% --(axis cs:0.19499999564141,0.122422455832414)
% --(axis cs:0.189999995753169,0.120822463074719)
% --(axis cs:0.184999995864928,0.118911104789816)
% --(axis cs:0.179999995976686,0.116699219552803)
% --(axis cs:0.174999996088445,0.114935753558584)
% --(axis cs:0.169999996200204,0.113652990706122)
% --(axis cs:0.164999996311963,0.111993708139155)
% --(axis cs:0.159999996423721,0.110143421155643)
% --(axis cs:0.15499999653548,0.108778230390167)
% --(axis cs:0.149999996647239,0.107700326071263)
% --(axis cs:0.144999996758997,0.106186066160169)
% --(axis cs:0.139999996870756,0.104582624039567)
% --(axis cs:0.134999996982515,0.103534719472137)
% --(axis cs:0.129999997094274,0.102617021948427)
% --(axis cs:0.124999997206032,0.101249202477253)
% --(axis cs:0.119999997317791,0.0998579215377418)
% --(axis cs:0.11499999742955,0.0989267083577865)
% --(axis cs:0.109999997541308,0.0980004719223629)
% --(axis cs:0.104999997653067,0.0966184984930541)
% --(axis cs:0.0999999977648258,0.0952158256202922)
% --(axis cs:0.0949999978765845,0.0942467591825453)
% --(axis cs:0.0899999979883432,0.0931020253564953)
% --(axis cs:0.0849999981001019,0.0915806693264902)
% --(axis cs:0.0799999982118607,0.0902212214304113)
% --(axis cs:0.0749999983236194,0.089241773372161)
% --(axis cs:0.0699999984353781,0.0879697340637059)
% --(axis cs:0.0649999985471368,0.0863133557983032)
% --(axis cs:0.0599999986588955,0.0846183247504366)
% --(axis cs:0.0549999987706542,0.0837984260853516)
% --(axis cs:0.0499999988824129,0.0825995808862086)
% --(axis cs:0.0449999989941716,0.0811211853611831)
% --(axis cs:0.0399999991059303,0.0795671275704294)
% --(axis cs:0.034999999217689,0.0787810339459002)
% --(axis cs:0.0299999993294477,0.0769930293466132)
% --(axis cs:0.0249999994412065,0.0748628587053995)
% --(axis cs:0.0199999995529652,0.0735565321982417)
% --(axis cs:0.0149999996647239,0.0748216554187491)
% --(axis cs:0.00999999977648258,0.0777360300409083)
% --(axis cs:0.00499999988824129,0.0723257914846999)
% --cycle;

% \path [fill=white!50.1960784313725!black, fill opacity=0.4, ultra thick]
% (axis cs:0.00499999988824129,0.0717130428605083)
% --(axis cs:0.00499999988824129,0.0479423620231686)
% --(axis cs:0.00999999977648258,0.0545217469628543)
% --(axis cs:0.0149999996647239,0.0550003746788291)
% --(axis cs:0.0199999995529652,0.0544554062637262)
% --(axis cs:0.0249999994412065,0.0563242272400719)
% --(axis cs:0.0299999993294477,0.0585527093342239)
% --(axis cs:0.034999999217689,0.0598958804710367)
% --(axis cs:0.0399999991059303,0.0609020837733752)
% --(axis cs:0.0449999989941716,0.0622297278214893)
% --(axis cs:0.0499999988824129,0.0635801774965467)
% --(axis cs:0.0549999987706542,0.0644275561573345)
% --(axis cs:0.0599999986588955,0.0650691824181672)
% --(axis cs:0.0649999985471368,0.0661175948923066)
% --(axis cs:0.0699999984353781,0.0674021507333243)
% --(axis cs:0.0749999983236194,0.0682795717863606)
% --(axis cs:0.0799999982118607,0.0689160373934828)
% --(axis cs:0.0849999981001019,0.0698269230203977)
% --(axis cs:0.0899999979883432,0.0709013929213666)
% --(axis cs:0.0949999978765845,0.0718145240580949)
% --(axis cs:0.0999999977648258,0.0725894509359476)
% --(axis cs:0.104999997653067,0.0735822090961512)
% --(axis cs:0.109999997541308,0.0745890059825799)
% --(axis cs:0.11499999742955,0.0753541678872109)
% --(axis cs:0.119999997317791,0.0760601799340242)
% --(axis cs:0.124999997206032,0.0769474359961481)
% --(axis cs:0.129999997094274,0.0778587237631285)
% --(axis cs:0.134999996982515,0.0786547537650245)
% --(axis cs:0.139999996870756,0.0793650287638424)
% --(axis cs:0.144999996758997,0.0802308613670677)
% --(axis cs:0.149999996647239,0.0811935689325096)
% --(axis cs:0.15499999653548,0.0820134393549197)
% --(axis cs:0.159999996423721,0.0827706081734575)
% --(axis cs:0.164999996311963,0.0837738538613493)
% --(axis cs:0.169999996200204,0.0848324726039726)
% --(axis cs:0.174999996088445,0.0857808426125378)
% --(axis cs:0.179999995976686,0.0867567227984275)
% --(axis cs:0.184999995864928,0.0880742980425841)
% --(axis cs:0.189999995753169,0.0894710984513577)
% --(axis cs:0.19499999564141,0.0908225610703488)
% --(axis cs:0.199999995529652,0.0923327849656376)
% --(axis cs:0.204999995417893,0.0941165061536277)
% --(axis cs:0.209999995306134,0.0959291803023438)
% --(axis cs:0.214999995194376,0.0976681712591969)
% --(axis cs:0.219999995082617,0.099592106606057)
% --(axis cs:0.224999994970858,0.101733079106683)
% --(axis cs:0.229999994859099,0.103862121802528)
% --(axis cs:0.234999994747341,0.10585240012953)
% --(axis cs:0.239999994635582,0.108132051708598)
% --(axis cs:0.244999994523823,0.110536660945738)
% --(axis cs:0.249999994412065,0.112951932752745)
% --(axis cs:0.254999994300306,0.115204100610966)
% --(axis cs:0.259999994188547,0.117763382724385)
% --(axis cs:0.264999994076788,0.120400274598243)
% --(axis cs:0.26999999396503,0.123051609098941)
% --(axis cs:0.274999993853271,0.125579609739125)
% --(axis cs:0.279999993741512,0.128408085479573)
% --(axis cs:0.284999993629754,0.131261065036432)
% --(axis cs:0.289999993517995,0.134129989205288)
% --(axis cs:0.294999993406236,0.13688267540486)
% --(axis cs:0.299999993294477,0.139913443167068)
% --(axis cs:0.304999993182719,0.142999359302441)
% --(axis cs:0.30999999307096,0.146096264125586)
% --(axis cs:0.314999992959201,0.149126074335531)
% --(axis cs:0.319999992847443,0.152378719109889)
% --(axis cs:0.324999992735684,0.155682578173698)
% --(axis cs:0.329999992623925,0.15897858085942)
% --(axis cs:0.334999992512167,0.162239120484111)
% --(axis cs:0.339999992400408,0.165653774406453)
% --(axis cs:0.344999992288649,0.169117883750487)
% --(axis cs:0.34999999217689,0.172558855076731)
% --(axis cs:0.354999992065132,0.175973118870107)
% --(axis cs:0.359999991953373,0.179484344402664)
% --(axis cs:0.364999991841614,0.183032952829621)
% --(axis cs:0.369999991729856,0.18656258677443)
% --(axis cs:0.374999991618097,0.190071425919554)
% --(axis cs:0.379999991506338,0.193633851851779)
% --(axis cs:0.384999991394579,0.197228757175838)
% --(axis cs:0.389999991282821,0.200806622830147)
% --(axis cs:0.394999991171062,0.204351485806873)
% --(axis cs:0.399999991059303,0.207929588215637)
% --(axis cs:0.404999990947545,0.211528693336554)
% --(axis cs:0.409999990835786,0.215119514108756)
% --(axis cs:0.414999990724027,0.218666949895898)
% --(axis cs:0.419999990612268,0.222214109143622)
% --(axis cs:0.42499999050051,0.225766267661877)
% --(axis cs:0.429999990388751,0.229314162847539)
% --(axis cs:0.434999990276992,0.232810772764882)
% --(axis cs:0.439999990165234,0.236291532488447)
% --(axis cs:0.444999990053475,0.239765927455225)
% --(axis cs:0.449999989941716,0.243247528144637)
% --(axis cs:0.454999989829957,0.246680589819622)
% --(axis cs:0.459999989718199,0.250073234763564)
% --(axis cs:0.46499998960644,0.253462744299809)
% --(axis cs:0.469999989494681,0.25685844865005)
% --(axis cs:0.474999989382923,0.260207185306575)
% --(axis cs:0.479999989271164,0.263519132805804)
% --(axis cs:0.484999989159405,0.266830835836301)
% --(axis cs:0.489999989047647,0.270152339463855)
% --(axis cs:0.494999988935888,0.273426411991371)
% --(axis cs:0.494999988935888,0.349083688898173)
% --(axis cs:0.494999988935888,0.349083688898173)
% --(axis cs:0.489999989047647,0.345670997645619)
% --(axis cs:0.484999989159405,0.342226387022885)
% --(axis cs:0.479999989271164,0.33874835703001)
% --(axis cs:0.474999989382923,0.335247415517636)
% --(axis cs:0.469999989494681,0.331701272603454)
% --(axis cs:0.46499998960644,0.328122944434829)
% --(axis cs:0.459999989718199,0.324506155452288)
% --(axis cs:0.454999989829957,0.320888767586842)
% --(axis cs:0.449999989941716,0.317223707342547)
% --(axis cs:0.444999990053475,0.313515463006913)
% --(axis cs:0.439999990165234,0.309774295233777)
% --(axis cs:0.434999990276992,0.306025274830068)
% --(axis cs:0.429999990388751,0.302226545148903)
% --(axis cs:0.42499999050051,0.29837651404755)
% --(axis cs:0.419999990612268,0.294491827579123)
% --(axis cs:0.414999990724027,0.290596686974282)
% --(axis cs:0.409999990835786,0.286672087604551)
% --(axis cs:0.404999990947545,0.282690339648468)
% --(axis cs:0.399999991059303,0.278674479889772)
% --(axis cs:0.394999991171062,0.274638871434317)
% --(axis cs:0.389999991282821,0.270589285872698)
% --(axis cs:0.384999991394579,0.266487781900841)
% --(axis cs:0.379999991506338,0.262365852605217)
% --(axis cs:0.374999991618097,0.258220544620302)
% --(axis cs:0.369999991729856,0.254079846352938)
% --(axis cs:0.364999991841614,0.249902609588789)
% --(axis cs:0.359999991953373,0.245721374016094)
% --(axis cs:0.354999992065132,0.24150687159973)
% --(axis cs:0.34999999217689,0.237330055455407)
% --(axis cs:0.344999992288649,0.233147742249853)
% --(axis cs:0.339999992400408,0.228981961207176)
% --(axis cs:0.334999992512167,0.224763729696106)
% --(axis cs:0.329999992623925,0.220613444180788)
% --(axis cs:0.324999992735684,0.216525358412039)
% --(axis cs:0.319999992847443,0.212433986269763)
% --(axis cs:0.314999992959201,0.208240605728379)
% --(axis cs:0.30999999307096,0.204141408887456)
% --(axis cs:0.304999993182719,0.200151170579539)
% --(axis cs:0.299999993294477,0.196131415591675)
% --(axis cs:0.294999993406236,0.192012039335615)
% --(axis cs:0.289999993517995,0.1880386661517)
% --(axis cs:0.284999993629754,0.184291709820745)
% --(axis cs:0.279999993741512,0.18039816794208)
% --(axis cs:0.274999993853271,0.176341350610355)
% --(axis cs:0.26999999396503,0.172505554402672)
% --(axis cs:0.264999994076788,0.1689867837134)
% --(axis cs:0.259999994188547,0.165278824728154)
% --(axis cs:0.254999994300306,0.161475135822998)
% --(axis cs:0.249999994412065,0.158038054083306)
% --(axis cs:0.244999994523823,0.154993651136215)
% --(axis cs:0.239999994635582,0.151595511597343)
% --(axis cs:0.234999994747341,0.148153450009759)
% --(axis cs:0.229999994859099,0.145255843126663)
% --(axis cs:0.224999994970858,0.142697694914994)
% --(axis cs:0.219999995082617,0.139637457711652)
% --(axis cs:0.214999995194376,0.136618011644152)
% --(axis cs:0.209999995306134,0.134338425813371)
% --(axis cs:0.204999995417893,0.132196205095746)
% --(axis cs:0.199999995529652,0.129554138709648)
% --(axis cs:0.19499999564141,0.12709280731082)
% --(axis cs:0.189999995753169,0.125415317579282)
% --(axis cs:0.184999995864928,0.123567233546952)
% --(axis cs:0.179999995976686,0.121274711674759)
% --(axis cs:0.174999996088445,0.119327692575696)
% --(axis cs:0.169999996200204,0.118109646300884)
% --(axis cs:0.164999996311963,0.116463362822477)
% --(axis cs:0.159999996423721,0.114493584065053)
% --(axis cs:0.15499999653548,0.112963372538152)
% --(axis cs:0.149999996647239,0.111993262722908)
% --(axis cs:0.144999996758997,0.110506304616588)
% --(axis cs:0.139999996870756,0.108849474354826)
% --(axis cs:0.134999996982515,0.107768637398986)
% --(axis cs:0.129999997094274,0.107013481427831)
% --(axis cs:0.124999997206032,0.105702644121307)
% --(axis cs:0.119999997317791,0.10433527759536)
% --(axis cs:0.11499999742955,0.10353048258254)
% --(axis cs:0.109999997541308,0.102744199304688)
% --(axis cs:0.104999997653067,0.101416892564622)
% --(axis cs:0.0999999977648258,0.100046001683656)
% --(axis cs:0.0949999978765845,0.0991062162541207)
% --(axis cs:0.0899999979883432,0.0979210694992463)
% --(axis cs:0.0849999981001019,0.0962776138187348)
% --(axis cs:0.0799999982118607,0.0946657160670327)
% --(axis cs:0.0749999983236194,0.0933097306728568)
% --(axis cs:0.0699999984353781,0.0916069767012315)
% --(axis cs:0.0649999985471368,0.0896009924358052)
% --(axis cs:0.0599999986588955,0.0876074121237368)
% --(axis cs:0.0549999987706542,0.0865720318094755)
% --(axis cs:0.0499999988824129,0.0850385253058287)
% --(axis cs:0.0449999989941716,0.0835224054091462)
% --(axis cs:0.0399999991059303,0.0815473239455492)
% --(axis cs:0.034999999217689,0.0802732282341523)
% --(axis cs:0.0299999993294477,0.077842820206363)
% --(axis cs:0.0249999994412065,0.075286150444266)
% --(axis cs:0.0199999995529652,0.0739858239094146)
% --(axis cs:0.0149999996647239,0.0748448027177378)
% --(axis cs:0.00999999977648258,0.077868551452679)
% --(axis cs:0.00499999988824129,0.0717130428605083)
% --cycle;

% \addplot [ultra thick, blue]
% table {%
% 0.00499999523162842 0.0891090780496597
% 0.00999999046325684 0.0958595350384712
% 0.0149999856948853 0.098928190767765
% 0.0199999809265137 0.102203704416752
% 0.0299999713897705 0.112459667026997
% 0.0349999666213989 0.117255419492722
% 0.0399999618530273 0.121325097978115
% 0.0449999570846558 0.125203624367714
% 0.0499999523162842 0.128394305706024
% 0.0549999475479126 0.131109476089478
% 0.059999942779541 0.133464381098747
% 0.065000057220459 0.136118590831757
% 0.0700000524520874 0.138669177889824
% 0.0850000381469727 0.146147802472115
% 0.0900000333786011 0.148739218711853
% 0.0950000286102295 0.151279717683792
% 0.110000014305115 0.158712238073349
% 0.115000009536743 0.161001145839691
% 0.125 0.165371686220169
% 0.129999995231628 0.167472586035728
% 0.134999990463257 0.16946716606617
% 0.144999980926514 0.173291370272636
% 0.154999971389771 0.177021160721779
% 0.184999942779541 0.188334137201309
% 0.194999933242798 0.192508980631828
% 0.205000042915344 0.197013854980469
% 0.215000033378601 0.201805919408798
% 0.225000023841858 0.206858426332474
% 0.254999995231628 0.222981944680214
% 0.269999980926514 0.231298178434372
% 0.279999971389771 0.236777037382126
% 0.289999961853027 0.242112904787064
% 0.299999952316284 0.247309640049934
% 0.309999942779541 0.252508372068405
% 0.319999933242798 0.257585674524307
% 0.329999923706055 0.262585371732712
% 0.345000028610229 0.269916087388992
% 0.360000014305115 0.277185469865799
% 0.375 0.284501850605011
% 0.389999985694885 0.291766494512558
% 0.404999971389771 0.298893481492996
% 0.414999961853027 0.303589135408401
% 0.424999952316284 0.308180928230286
% 0.434999942779541 0.312623143196106
% 0.450000047683716 0.319094717502594
% 0.465000033378601 0.325331509113312
% 0.480000019073486 0.33146995306015
% 0.495000004768372 0.337417215108871
% };
% \addlegendentry{No si.}
% \addplot [ultra thick, red]
% table {%
% 0.00499999523162842 0.0965440645813942
% 0.00999999046325684 0.101374782621861
% 0.0149999856948853 0.103267908096313
% 0.0199999809265137 0.105385564267635
% 0.0249999761581421 0.109322763979435
% 0.0299999713897705 0.113240383565426
% 0.0349999666213989 0.116591677069664
% 0.0399999618530273 0.119413174688816
% 0.0449999570846558 0.122503362596035
% 0.0499999523162842 0.125194042921066
% 0.0549999475479126 0.127751260995865
% 0.059999942779541 0.130017086863518
% 0.065000057220459 0.132728382945061
% 0.0700000524520874 0.135204002261162
% 0.0750000476837158 0.137427806854248
% 0.0800000429153442 0.139423504471779
% 0.0850000381469727 0.141525059938431
% 0.0900000333786011 0.143417656421661
% 0.0950000286102295 0.145093321800232
% 0.105000019073486 0.148135304450989
% 0.110000014305115 0.149539217352867
% 0.115000009536743 0.150790438055992
% 0.120000004768372 0.151922807097435
% 0.125 0.153145298361778
% 0.129999995231628 0.154303312301636
% 0.134999990463257 0.155367985367775
% 0.144999980926514 0.157433807849884
% 0.190000057220459 0.167081922292709
% 0.210000038146973 0.171424046158791
% 0.245000004768372 0.179823651909828
% 0.254999995231628 0.18237242102623
% 0.284999966621399 0.190000176429749
% 0.309999942779541 0.196244537830353
% 0.329999923706055 0.200915440917015
% 0.355000019073486 0.206765726208687
% 0.365000009536743 0.209104746580124
% 0.389999985694885 0.214994698762894
% 0.399999976158142 0.217298209667206
% 0.409999966621399 0.21949003636837
% 0.419999957084656 0.221558630466461
% 0.429999947547913 0.223552018404007
% 0.444999933242798 0.226285979151726
% 0.454999923706055 0.228041112422943
% 0.495000004768372 0.234868139028549
% };
% \addlegendentry{Si 1}
% \addplot [ultra thick, green!50.1960784313725!black]
% table {%
% 0.00499999523162842 0.0762640386819839
% 0.0149999856948853 0.0808437243103981
% 0.0199999809265137 0.0833111777901649
% 0.0249999761581421 0.0863811075687408
% 0.0299999713897705 0.0899804532527924
% 0.0349999666213989 0.0930423885583878
% 0.0399999618530273 0.0950435847043991
% 0.0449999570846558 0.0974984765052795
% 0.0499999523162842 0.100365601480007
% 0.0549999475479126 0.102854825556278
% 0.059999942779541 0.104729406535625
% 0.0700000524520874 0.109711572527885
% 0.0750000476837158 0.111741788685322
% 0.0800000429153442 0.113204643130302
% 0.0850000381469727 0.114989511668682
% 0.0900000333786011 0.116876855492592
% 0.0950000286102295 0.118166506290436
% 0.100000023841858 0.119093850255013
% 0.110000014305115 0.121919028460979
% 0.120000004768372 0.123437598347664
% 0.129999995231628 0.126216486096382
% 0.134999990463257 0.12707494199276
% 0.139999985694885 0.128148689866066
% 0.144999980926514 0.129782646894455
% 0.149999976158142 0.131310299038887
% 0.154999971389771 0.132327526807785
% 0.159999966621399 0.133693471550941
% 0.164999961853027 0.135696887969971
% 0.169999957084656 0.13756088912487
% 0.174999952316284 0.139045402407646
% 0.179999947547913 0.140985891222954
% 0.184999942779541 0.143474742770195
% 0.190000057220459 0.145744830369949
% 0.194999933242798 0.14761583507061
% 0.200000047683716 0.150161013007164
% 0.205000042915344 0.153169795870781
% 0.210000038146973 0.155846834182739
% 0.215000033378601 0.158390268683434
% 0.220000028610229 0.161584883928299
% 0.225000023841858 0.165127739310265
% 0.230000019073486 0.168320551514626
% 0.235000014305115 0.171409741044044
% 0.245000004768372 0.179015681147575
% 0.254999995231628 0.186220556497574
% 0.264999985694885 0.194478422403336
% 0.274999976158142 0.202374890446663
% 0.284999966621399 0.210999056696892
% 0.305000066757202 0.228123500943184
% 0.319999933242798 0.241139009594917
% 0.325000047683716 0.245601564645767
% 0.335000038146973 0.254294574260712
% 0.345000028610229 0.263153791427612
% 0.355000019073486 0.271836221218109
% 0.365000009536743 0.280563831329346
% 0.375 0.289129078388214
% 0.384999990463257 0.29763650894165
% 0.394999980926514 0.305963665246964
% 0.404999971389771 0.314184933900833
% 0.414999961853027 0.322247594594955
% 0.424999952316284 0.330140948295593
% 0.434999942779541 0.337882846593857
% 0.444999933242798 0.345434993505478
% 0.454999923706055 0.352878302335739
% 0.470000028610229 0.363718301057816
% 0.480000019073486 0.370758056640625
% 0.495000004768372 0.381092995405197
% };
% \addlegendentry{Si 2}
% \addplot [ultra thick, color0]
% table {%
% 0.00499999523162842 0.058377593755722
% 0.00999999046325684 0.0658384785056114
% 0.0149999856948853 0.0640234425663948
% 0.0199999809265137 0.0633455291390419
% 0.0249999761581421 0.0649960860610008
% 0.0299999713897705 0.0670813769102097
% 0.0349999666213989 0.0688057765364647
% 0.0399999618530273 0.0697651132941246
% 0.0449999570846558 0.071412019431591
% 0.0499999523162842 0.0730286166071892
% 0.0549999475479126 0.0742233172059059
% 0.059999942779541 0.0750251188874245
% 0.065000057220459 0.0763782113790512
% 0.0700000524520874 0.077868714928627
% 0.0750000476837158 0.0789938271045685
% 0.0800000429153442 0.0798509269952774
% 0.0850000381469727 0.0809958502650261
% 0.0900000333786011 0.0822604671120644
% 0.0950000286102295 0.0831665322184563
% 0.100000023841858 0.0839678272604942
% 0.110000014305115 0.0861777439713478
% 0.120000004768372 0.0876220911741257
% 0.129999995231628 0.0897318795323372
% 0.134999990463257 0.090481773018837
% 0.139999985694885 0.0912964418530464
% 0.149999976158142 0.0936672016978264
% 0.154999971389771 0.09452835470438
% 0.159999966621399 0.095587745308876
% 0.164999961853027 0.096985749900341
% 0.169999957084656 0.0982641652226448
% 0.174999952316284 0.0993108674883842
% 0.179999947547913 0.100710168480873
% 0.184999942779541 0.102440416812897
% 0.190000057220459 0.103995457291603
% 0.194999933242798 0.105416551232338
% 0.200000047683716 0.107277646660805
% 0.205000042915344 0.109376065433025
% 0.215000033378601 0.113119408488274
% 0.220000028610229 0.115459501743317
% 0.225000023841858 0.117949709296227
% 0.235000014305115 0.122463181614876
% 0.245000004768372 0.127953127026558
% 0.254999995231628 0.13319618999958
% 0.264999985694885 0.139245584607124
% 0.274999976158142 0.145126432180405
% 0.284999966621399 0.151626512408257
% 0.294999957084656 0.157975301146507
% 0.305000066757202 0.164807602763176
% 0.329999923706055 0.182270720601082
% 0.345000028610229 0.19321009516716
% 0.360000014305115 0.204276353120804
% 0.370000004768372 0.211759999394417
% 0.384999990463257 0.223008751869202
% 0.394999980926514 0.230441465973854
% 0.404999971389771 0.23792028427124
% 0.414999961853027 0.24528181552887
% 0.424999952316284 0.252639621496201
% 0.434999942779541 0.259846895933151
% 0.444999933242798 0.267015844583511
% 0.454999923706055 0.274053037166595
% 0.465000033378601 0.281031757593155
% 0.475000023841858 0.287889689207077
% 0.485000014305115 0.29467049241066
% 0.495000004768372 0.301340788602829
% };
% \addlegendentry{Si 3}
% \addplot [ultra thick, white!50.1960784313725!black]
% table {%
% 0.00499999523162842 0.0598277002573013
% 0.00999999046325684 0.0661951526999474
% 0.0149999856948853 0.0649225860834122
% 0.0199999809265137 0.0642206072807312
% 0.0249999761581421 0.065805196762085
% 0.0299999713897705 0.0681977644562721
% 0.0349999666213989 0.0700845494866371
% 0.0399999618530273 0.0712246969342232
% 0.0449999570846558 0.0728760734200478
% 0.0499999523162842 0.0743093490600586
% 0.0549999475479126 0.0754997953772545
% 0.059999942779541 0.0763383060693741
% 0.065000057220459 0.0778592899441719
% 0.0700000524520874 0.0795045644044876
% 0.0750000476837158 0.0807946473360062
% 0.0800000429153442 0.0817908719182014
% 0.0850000381469727 0.0830522626638412
% 0.0900000333786011 0.0844112187623978
% 0.0950000286102295 0.0854603871703148
% 0.100000023841858 0.0863177254796028
% 0.110000014305115 0.0886666104197502
% 0.120000004768372 0.0901977196335793
% 0.129999995231628 0.0924361050128937
% 0.134999990463257 0.0932116881012917
% 0.139999985694885 0.0941072404384613
% 0.144999980926514 0.0953686013817787
% 0.149999976158142 0.0965934246778488
% 0.154999971389771 0.0974884107708931
% 0.159999966621399 0.0986321046948433
% 0.164999961853027 0.100118592381477
% 0.169999957084656 0.101471051573753
% 0.174999952316284 0.102554246783257
% 0.179999947547913 0.104015700519085
% 0.184999942779541 0.105820775032043
% 0.190000057220459 0.107443206012249
% 0.194999933242798 0.108957692980766
% 0.200000047683716 0.1109434440732
% 0.205000042915344 0.113156363368034
% 0.215000033378601 0.117143116891384
% 0.225000023841858 0.122215390205383
% 0.235000014305115 0.127002909779549
% 0.245000004768372 0.132765144109726
% 0.254999995231628 0.138339638710022
% 0.264999985694885 0.14469350874424
% 0.274999976158142 0.150960490107536
% 0.279999971389771 0.154403120279312
% 0.284999966621399 0.157776355743408
% 0.294999957084656 0.164447352290154
% 0.305000066757202 0.171575248241425
% 0.325000047683716 0.186103954911232
% 0.340000033378601 0.197317898273468
% 0.350000023841858 0.204944476485252
% 0.365000009536743 0.21646773815155
% 0.375 0.224145993590355
% 0.384999990463257 0.231858253479004
% 0.394999980926514 0.239495187997818
% 0.404999971389771 0.247109532356262
% 0.414999961853027 0.254631787538528
% 0.424999952316284 0.262071371078491
% 0.434999942779541 0.269418001174927
% 0.444999933242798 0.276640653610229
% 0.454999923706055 0.283784717321396
% 0.465000033378601 0.290792852640152
% 0.475000023841858 0.297727286815643
% 0.485000014305115 0.304528564214706
% 0.495000004768372 0.311255037784576
% };
% \addlegendentry{Si 4}

==> plots/fetch/traj_err_data.tex <==
\path [fill=red, fill opacity=0.4, ultra thick]
(axis cs:1,0.450832588657663)
--(axis cs:1,0.342277254094566)
--(axis cs:10,0.193951732104943)
--(axis cs:25,0.150299187024981)
--(axis cs:75,0.139574592806006)
--(axis cs:200,0.127053163665148)
--(axis cs:500,0.12671936290503)
--(axis cs:500,0.173708148227355)
--(axis cs:500,0.173708148227355)
--(axis cs:200,0.153499872891358)
--(axis cs:75,0.175308678055132)
--(axis cs:25,0.200064418380496)
--(axis cs:10,0.242821759343827)
--(axis cs:1,0.450832588657663)
--cycle;

\path [fill=blue, fill opacity=0.4, ultra thick]
(axis cs:1,0.451926405471201)
--(axis cs:1,0.342860865771516)
--(axis cs:10,0.199300593840028)
--(axis cs:25,0.154742646005381)
--(axis cs:75,0.128719010454512)
--(axis cs:200,0.124852794858849)
--(axis cs:500,0.117650844561737)
--(axis cs:500,0.151035332992766)
--(axis cs:500,0.151035332992766)
--(axis cs:200,0.159252187683108)
--(axis cs:75,0.173533777632331)
--(axis cs:25,0.203620894570686)
--(axis cs:10,0.242294546775482)
--(axis cs:1,0.451926405471201)
--cycle;

\path [fill=green!50.1960784313725!black, fill opacity=0.4, ultra thick]
(axis cs:1,0.470060717754753)
--(axis cs:1,0.349116601596732)
--(axis cs:10,0.128702420635964)
--(axis cs:25,0.103147952468473)
--(axis cs:75,0.0909859729168512)
--(axis cs:200,0.0821552220450362)
--(axis cs:500,0.0887728774389657)
--(axis cs:500,0.123950443219074)
--(axis cs:500,0.123950443219074)
--(axis cs:200,0.105308444634118)
--(axis cs:75,0.1225136292467)
--(axis cs:25,0.146719670927311)
--(axis cs:10,0.183442881853881)
--(axis cs:1,0.470060717754753)
--cycle;

\path [fill=color0, fill opacity=0.4, ultra thick]
(axis cs:1,0.460758098853286)
--(axis cs:1,0.332549681437606)
--(axis cs:10,0.104416636058916)
--(axis cs:25,0.0929826811626782)
--(axis cs:75,0.0840021843585121)
--(axis cs:200,0.0737448759121545)
--(axis cs:500,0.0693265017147747)
--(axis cs:500,0.0930321786056807)
--(axis cs:500,0.0930321786056807)
--(axis cs:200,0.0942462047210047)
--(axis cs:75,0.107495555657725)
--(axis cs:25,0.119711127995211)
--(axis cs:10,0.131280766537419)
--(axis cs:1,0.460758098853286)
--cycle;

\path [fill=white!40!black, fill opacity=0.4, ultra thick]
(axis cs:1,0.457690971213657)
--(axis cs:1,0.329526233032621)
--(axis cs:10,0.103653766848593)
--(axis cs:25,0.0935290442563888)
--(axis cs:75,0.0827389188560648)
--(axis cs:200,0.075193272762717)
--(axis cs:500,0.073899063733729)
--(axis cs:500,0.098851571947577)
--(axis cs:500,0.098851571947577)
--(axis cs:200,0.0969252035812792)
--(axis cs:75,0.100867508333778)
--(axis cs:25,0.134153717115168)
--(axis cs:10,0.131659006313328)
--(axis cs:1,0.457690971213657)
--cycle;

\addplot [ultra thick, red, mark=*, mark size=1.5, mark options={solid}]
table {%
1 0.396554887294769
10 0.218386724591255
25 0.175181820988655
75 0.157441630959511
200 0.140276536345482
500 0.150213733315468
};
% \addlegendentry{No si.}
\addplot [semithick, blue, mark=*, mark size=1.5, mark options={solid}]
table {%
1 0.397393703460693
10 0.220797553658485
25 0.17918173968792
75 0.15112641453743
200 0.142052501440048
500 0.134343087673187
};
\addplot [ultra thick, green!50.1960784313725!black, mark=asterisk, mark size=1.5, mark options={solid}]
table {%
1 0.409588694572449
10 0.156072616577148
25 0.124933794140816
75 0.106749795377254
200 0.0937318354845047
500 0.106361664831638
};
% \addlegendentry{Si 2}
\addplot [ultra thick, color0, mark=*, mark size=1.5, mark options={solid}]
table {%
1 0.396653860807419
10 0.117848709225655
25 0.106346897780895
75 0.0957488790154457
200 0.0839955359697342
500 0.0811793431639671
};
% \addlegendentry{si 3}
\addplot [ultra thick, white!40!black, mark=*, mark size=1.5, mark options={solid}]
table {%
1 0.393608659505844
10 0.117656394839287
25 0.113841384649277
75 0.0918032079935074
200 0.0860592424869537
500 0.0863753259181976
};
% \addlegendentry{si 4}

==> supp_mat/ant_plots/constraint_loss_data.tex <==
\definecolor{color0}{rgb}{1,0,1}


\path [fill=color0, fill opacity=0.4, semithick]
(axis cs:0,8.41387367248535)
--(axis cs:0,7.63184022903442)
--(axis cs:100,7.63175487518311)
--(axis cs:200,7.61650228500366)
--(axis cs:300,0.0006866455078125)
--(axis cs:400,0.000645446765702218)
--(axis cs:500,0.000576019287109375)
--(axis cs:600,0.000528717064298689)
--(axis cs:700,0.000510406505782157)
--(axis cs:800,0.000514984130859375)
--(axis cs:900,0.0408084243535995)
--(axis cs:1000,0.0459358505904675)
--(axis cs:1100,0.160048678517342)
--(axis cs:1200,0.201066821813583)
--(axis cs:1300,0.473329156637192)
--(axis cs:1400,0.406928241252899)
--(axis cs:1500,0.51608282327652)
--(axis cs:1600,0.690039813518524)
--(axis cs:1700,0.666200697422028)
--(axis cs:1800,1.13009893894196)
--(axis cs:1900,1.4127676486969)
--(axis cs:2000,1.67491173744202)
--(axis cs:2100,1.91194152832031)
--(axis cs:2200,2.33479690551758)
--(axis cs:2300,2.6640031337738)
--(axis cs:2400,2.73953890800476)
--(axis cs:2500,2.79550743103027)
--(axis cs:2600,3.30379939079285)
--(axis cs:2700,3.47955751419067)
--(axis cs:2800,3.56284022331238)
--(axis cs:2900,3.95066022872925)
--(axis cs:3000,4.05537939071655)
--(axis cs:3100,3.70586371421814)
--(axis cs:3200,4.09778451919556)
--(axis cs:3300,4.16625499725342)
--(axis cs:3400,4.67464876174927)
--(axis cs:3500,4.82595825195312)
--(axis cs:3600,5.86706829071045)
--(axis cs:3700,6.20315456390381)
--(axis cs:3800,6.64736318588257)
--(axis cs:3900,6.87308120727539)
--(axis cs:4000,6.55149078369141)
--(axis cs:4100,6.26373434066772)
--(axis cs:4200,5.97647094726562)
--(axis cs:4300,5.79604244232178)
--(axis cs:4400,6.80171871185303)
--(axis cs:4500,7.44239521026611)
--(axis cs:4600,8.22664833068848)
--(axis cs:4700,8.28733825683594)
--(axis cs:4800,7.99957466125488)
--(axis cs:4900,7.83669900894165)
--(axis cs:5000,7.97837972640991)
--(axis cs:5100,7.4248194694519)
--(axis cs:5200,7.04610109329224)
--(axis cs:5300,7.18055152893066)
--(axis cs:5400,8.01148128509521)
--(axis cs:5500,8.35300922393799)
--(axis cs:5600,7.4183931350708)
--(axis cs:5700,7.456298828125)
--(axis cs:5800,8.8077392578125)
--(axis cs:5900,8.00116539001465)
--(axis cs:6000,7.66686296463013)
--(axis cs:6100,7.48223161697388)
--(axis cs:6200,7.62960767745972)
--(axis cs:6300,6.42214202880859)
--(axis cs:6400,5.85565423965454)
--(axis cs:6500,5.71112155914307)
--(axis cs:6600,5.8490743637085)
--(axis cs:6700,6.07038021087646)
--(axis cs:6800,6.13049983978271)
--(axis cs:6900,6.20547103881836)
--(axis cs:7000,5.73598527908325)
--(axis cs:7100,6.1784291267395)
--(axis cs:7200,5.76655864715576)
--(axis cs:7300,5.90010356903076)
--(axis cs:7400,5.92307138442993)
--(axis cs:7500,5.97251605987549)
--(axis cs:7600,4.95956611633301)
--(axis cs:7700,4.96305322647095)
--(axis cs:7800,4.73349046707153)
--(axis cs:7900,5.86385869979858)
--(axis cs:8000,5.85897731781006)
--(axis cs:8100,6.18974018096924)
--(axis cs:8200,5.71666812896729)
--(axis cs:8300,5.46551179885864)
--(axis cs:8400,4.82412910461426)
--(axis cs:8500,4.61865043640137)
--(axis cs:8600,4.79533672332764)
--(axis cs:8700,4.90513324737549)
--(axis cs:8800,5.10430908203125)
--(axis cs:8900,5.26723718643188)
--(axis cs:9000,5.21361875534058)
--(axis cs:9100,4.95327186584473)
--(axis cs:9200,4.9489164352417)
--(axis cs:9300,4.62161874771118)
--(axis cs:9400,3.87828803062439)
--(axis cs:9500,4.17340421676636)
--(axis cs:9600,3.99137926101685)
--(axis cs:9700,4.10009765625)
--(axis cs:9800,4.01424741744995)
--(axis cs:9900,3.7936224937439)
--(axis cs:10000,4.1210618019104)
--(axis cs:10100,4.42196035385132)
--(axis cs:10200,4.72764158248901)
--(axis cs:10300,4.63932991027832)
--(axis cs:10400,4.51777362823486)
--(axis cs:10500,4.26390647888184)
--(axis cs:10600,4.31695890426636)
--(axis cs:10700,4.24930906295776)
--(axis cs:10800,4.24373769760132)
--(axis cs:10900,4.32976007461548)
--(axis cs:11000,4.87548589706421)
--(axis cs:11100,4.59371328353882)
--(axis cs:11200,4.25072431564331)
--(axis cs:11300,4.12395048141479)
--(axis cs:11400,3.90697336196899)
--(axis cs:11500,3.55652904510498)
--(axis cs:11600,3.91560053825378)
--(axis cs:11700,3.84647226333618)
--(axis cs:11800,3.97954058647156)
--(axis cs:11900,4.12263059616089)
--(axis cs:12000,4.18025684356689)
--(axis cs:12100,4.27630233764648)
--(axis cs:12200,4.00827074050903)
--(axis cs:12300,3.52186250686646)
--(axis cs:12400,3.44220876693726)
--(axis cs:12500,3.59850907325745)
--(axis cs:12600,3.50187873840332)
--(axis cs:12700,3.61796474456787)
--(axis cs:12800,3.6900646686554)
--(axis cs:12900,3.57481336593628)
--(axis cs:13000,3.41230940818787)
--(axis cs:13100,3.52352380752563)
--(axis cs:13200,4.04837656021118)
--(axis cs:13300,3.84902262687683)
--(axis cs:13400,3.81728410720825)
--(axis cs:13500,3.46647214889526)
--(axis cs:13600,3.44792485237122)
--(axis cs:13700,3.38343596458435)
--(axis cs:13800,3.56418061256409)
--(axis cs:13900,3.58167886734009)
--(axis cs:14000,3.65338897705078)
--(axis cs:14100,3.59256720542908)
--(axis cs:14200,3.38715076446533)
--(axis cs:14300,3.14019060134888)
--(axis cs:14400,3.08116674423218)
--(axis cs:14500,3.36102485656738)
--(axis cs:14600,3.17252254486084)
--(axis cs:14700,2.88228535652161)
--(axis cs:14800,2.9154691696167)
--(axis cs:14900,2.92670202255249)
--(axis cs:15000,2.82349634170532)
--(axis cs:15100,3.15548276901245)
--(axis cs:15200,3.28294801712036)
--(axis cs:15300,3.16390371322632)
--(axis cs:15400,3.13470935821533)
--(axis cs:15500,3.0826473236084)
--(axis cs:15600,3.03697514533997)
--(axis cs:15700,2.75079202651978)
--(axis cs:15800,2.67040848731995)
--(axis cs:15900,2.87613081932068)
--(axis cs:16000,3.01404690742493)
--(axis cs:16100,3.03815579414368)
--(axis cs:16200,3.16276431083679)
--(axis cs:16300,3.22609996795654)
--(axis cs:16400,2.90699791908264)
--(axis cs:16500,2.80696487426758)
--(axis cs:16600,2.83980226516724)
--(axis cs:16700,2.82849931716919)
--(axis cs:16800,2.76139259338379)
--(axis cs:16900,2.87691450119019)
--(axis cs:17000,2.67355394363403)
--(axis cs:17100,2.77340364456177)
--(axis cs:17200,2.83211040496826)
--(axis cs:17300,2.79898285865784)
--(axis cs:17400,2.65877461433411)
--(axis cs:17500,2.75625777244568)
--(axis cs:17600,2.57911920547485)
--(axis cs:17700,2.55428004264832)
--(axis cs:17800,2.57290077209473)
--(axis cs:17900,2.61156129837036)
--(axis cs:18000,2.8154182434082)
--(axis cs:18100,2.75100207328796)
--(axis cs:18200,2.75727820396423)
--(axis cs:18300,2.80413389205933)
--(axis cs:18400,2.81148767471313)
--(axis cs:18500,2.67538070678711)
--(axis cs:18600,2.71283292770386)
--(axis cs:18700,2.70105624198914)
--(axis cs:18800,2.73266577720642)
--(axis cs:18900,2.84857606887817)
--(axis cs:19000,2.97241306304932)
--(axis cs:19100,2.93081259727478)
--(axis cs:19200,2.88247776031494)
--(axis cs:19300,2.7573082447052)
--(axis cs:19400,2.60763835906982)
--(axis cs:19500,2.39734172821045)
--(axis cs:19600,2.92694473266602)
--(axis cs:19700,3.15997314453125)
--(axis cs:19800,3.29364013671875)
--(axis cs:19900,3.36518096923828)
--(axis cs:20000,3.314208984375)
--(axis cs:20100,2.80626392364502)
--(axis cs:20200,2.81702423095703)
--(axis cs:20300,2.69749307632446)
--(axis cs:20400,2.66385507583618)
--(axis cs:20500,2.58675527572632)
--(axis cs:20600,2.58428955078125)
--(axis cs:20700,2.6683349609375)
--(axis cs:20800,2.76310396194458)
--(axis cs:20900,2.61253666877747)
--(axis cs:21000,2.41082763671875)
--(axis cs:21100,2.66192102432251)
--(axis cs:21200,2.50179696083069)
--(axis cs:21300,2.41188097000122)
--(axis cs:21400,2.60182976722717)
--(axis cs:21500,2.59817314147949)
--(axis cs:21600,2.50177264213562)
--(axis cs:21700,2.51591777801514)
--(axis cs:21800,2.39096879959106)
--(axis cs:21900,2.56327128410339)
--(axis cs:22000,2.82365465164185)
--(axis cs:22100,2.74634003639221)
--(axis cs:22200,2.62802648544312)
--(axis cs:22300,2.70856642723083)
--(axis cs:22400,2.43293166160583)
--(axis cs:22500,2.2135009765625)
--(axis cs:22600,2.2135009765625)
--(axis cs:22700,2.2135009765625)
--(axis cs:22800,2.13381338119507)
--(axis cs:22900,2.2135009765625)
--(axis cs:23000,2.24750375747681)
--(axis cs:23100,2.2135009765625)
--(axis cs:23200,2.31971621513367)
--(axis cs:23300,2.36542558670044)
--(axis cs:23400,2.36827898025513)
--(axis cs:23500,2.39692306518555)
--(axis cs:23600,2.39892315864563)
--(axis cs:23700,2.39850544929504)
--(axis cs:23800,2.35869312286377)
--(axis cs:23900,2.37741088867188)
--(axis cs:24000,2.29563474655151)
--(axis cs:24100,2.36462664604187)
--(axis cs:24200,2.36767339706421)
--(axis cs:24300,2.36420607566833)
--(axis cs:24400,2.28696727752686)
--(axis cs:24500,2.33148527145386)
--(axis cs:24600,2.28137564659119)
--(axis cs:24700,2.2135009765625)
--(axis cs:24800,2.2268373966217)
--(axis cs:24900,2.32068347930908)
--(axis cs:25000,2.33114004135132)
--(axis cs:25100,2.24976658821106)
--(axis cs:25200,2.24396705627441)
--(axis cs:25300,2.27048325538635)
--(axis cs:25400,2.2135009765625)
--(axis cs:25500,2.23799514770508)
--(axis cs:25600,2.28055095672607)
--(axis cs:25700,2.34997367858887)
--(axis cs:25800,2.27198553085327)
--(axis cs:25900,2.34653210639954)
--(axis cs:26000,2.24043440818787)
--(axis cs:26100,2.29117441177368)
--(axis cs:26200,2.21348881721497)
--(axis cs:26300,2.21348881721497)
--(axis cs:26400,2.23614454269409)
--(axis cs:26500,2.30545949935913)
--(axis cs:26600,2.21348881721497)
--(axis cs:26700,2.35226941108704)
--(axis cs:26800,2.35150980949402)
--(axis cs:26900,2.2135009765625)
--(axis cs:27000,2.2135009765625)
--(axis cs:27100,2.2135009765625)
--(axis cs:27200,1.72744524478912)
--(axis cs:27300,1.82268071174622)
--(axis cs:27400,1.77955937385559)
--(axis cs:27500,1.87575685977936)
--(axis cs:27600,2.01076650619507)
--(axis cs:27700,2.2135009765625)
--(axis cs:27800,2.2135009765625)
--(axis cs:27900,2.23010492324829)
--(axis cs:28000,2.2135009765625)
--(axis cs:28100,2.2135009765625)
--(axis cs:28200,2.2135009765625)
--(axis cs:28300,2.2135009765625)
--(axis cs:28400,2.2135009765625)
--(axis cs:28500,2.2135009765625)
--(axis cs:28600,2.2135009765625)
--(axis cs:28700,2.2135009765625)
--(axis cs:28800,2.20939946174622)
--(axis cs:28900,2.08012700080872)
--(axis cs:29000,2.2135009765625)
--(axis cs:29100,2.2135009765625)
--(axis cs:29200,2.04013681411743)
--(axis cs:29300,2.2135009765625)
--(axis cs:29400,2.2135009765625)
--(axis cs:29500,2.20463871955872)
--(axis cs:29600,2.2135009765625)
--(axis cs:29700,2.30518078804016)
--(axis cs:29800,2.29588079452515)
--(axis cs:29900,2.23435521125793)
--(axis cs:30000,2.25114941596985)
--(axis cs:30100,2.28232741355896)
--(axis cs:30200,2.2135009765625)
--(axis cs:30300,2.2135009765625)
--(axis cs:30400,2.2135009765625)
--(axis cs:30500,2.22461986541748)
--(axis cs:30600,1.97709965705872)
--(axis cs:30700,2.19704580307007)
--(axis cs:30800,2.2135009765625)
--(axis cs:30900,2.16652822494507)
--(axis cs:31000,2.02177739143372)
--(axis cs:31100,2.12392568588257)
--(axis cs:31200,1.91191411018372)
--(axis cs:31300,2.10488271713257)
--(axis cs:31300,3.09048056602478)
--(axis cs:31300,3.09048056602478)
--(axis cs:31200,3.08254861831665)
--(axis cs:31100,3.09177398681641)
--(axis cs:31000,3.08596873283386)
--(axis cs:30900,3.09504318237305)
--(axis cs:30800,3.10142159461975)
--(axis cs:30700,3.0977189540863)
--(axis cs:30600,3.08425092697144)
--(axis cs:30500,3.14928960800171)
--(axis cs:30400,3.13775086402893)
--(axis cs:30300,3.11360430717468)
--(axis cs:30200,3.13546466827393)
--(axis cs:30100,3.18508791923523)
--(axis cs:30000,3.16388964653015)
--(axis cs:29900,3.1543333530426)
--(axis cs:29800,3.1960301399231)
--(axis cs:29700,3.20427584648132)
--(axis cs:29600,3.13989329338074)
--(axis cs:29500,3.09842967987061)
--(axis cs:29400,3.13490581512451)
--(axis cs:29300,3.10174989700317)
--(axis cs:29200,3.08681344985962)
--(axis cs:29100,3.10332918167114)
--(axis cs:29000,3.12042331695557)
--(axis cs:28900,3.08894801139832)
--(axis cs:28800,3.09888458251953)
--(axis cs:28700,3.14004182815552)
--(axis cs:28600,3.13656449317932)
--(axis cs:28500,3.13244724273682)
--(axis cs:28400,3.11653661727905)
--(axis cs:28300,3.14014625549316)
--(axis cs:28200,3.14000749588013)
--(axis cs:28100,3.1314709186554)
--(axis cs:28000,3.11426401138306)
--(axis cs:27900,3.15208911895752)
--(axis cs:27800,3.1072518825531)
--(axis cs:27700,3.10129165649414)
--(axis cs:27600,3.0855016708374)
--(axis cs:27500,3.08198595046997)
--(axis cs:27400,3.08178496360779)
--(axis cs:27300,3.08161497116089)
--(axis cs:27200,3.08284139633179)
--(axis cs:27100,3.10924100875854)
--(axis cs:27000,3.10985040664673)
--(axis cs:26900,3.13947892189026)
--(axis cs:26800,3.25757193565369)
--(axis cs:26700,3.2586681842804)
--(axis cs:26600,3.14334487915039)
--(axis cs:26500,3.20454216003418)
--(axis cs:26400,3.15530252456665)
--(axis cs:26300,3.1313271522522)
--(axis cs:26200,3.11738157272339)
--(axis cs:26100,3.19209384918213)
--(axis cs:26000,3.1576611995697)
--(axis cs:25900,3.25060343742371)
--(axis cs:25800,3.17749404907227)
--(axis cs:25700,3.25538110733032)
--(axis cs:25600,3.18373966217041)
--(axis cs:25500,3.15630865097046)
--(axis cs:25400,3.13173198699951)
--(axis cs:25300,3.17644047737122)
--(axis cs:25200,3.1596622467041)
--(axis cs:25100,3.1630585193634)
--(axis cs:25000,3.23119735717773)
--(axis cs:24900,3.21958303451538)
--(axis cs:24800,3.15040898323059)
--(axis cs:24700,3.13064455986023)
--(axis cs:24600,3.18436312675476)
--(axis cs:24500,3.23160076141357)
--(axis cs:24400,3.1887001991272)
--(axis cs:24300,3.27720046043396)
--(axis cs:24200,3.28309154510498)
--(axis cs:24100,3.27790236473083)
--(axis cs:24000,3.19582033157349)
--(axis cs:23900,3.30108833312988)
--(axis cs:23800,3.26832485198975)
--(axis cs:23700,3.314208984375)
--(axis cs:23600,3.314208984375)
--(axis cs:23500,3.314208984375)
--(axis cs:23400,3.28414630889893)
--(axis cs:23300,3.2792444229126)
--(axis cs:23200,3.21856474876404)
--(axis cs:23100,3.14069366455078)
--(axis cs:23000,3.16171646118164)
--(axis cs:22900,3.10882186889648)
--(axis cs:22800,3.09248566627502)
--(axis cs:22700,3.11488080024719)
--(axis cs:22600,3.12983751296997)
--(axis cs:22500,3.14250731468201)
--(axis cs:22400,3.18675446510315)
--(axis cs:22300,3.314208984375)
--(axis cs:22200,3.26563358306885)
--(axis cs:22100,3.25318837165833)
--(axis cs:22000,3.314208984375)
--(axis cs:21900,3.314208984375)
--(axis cs:21800,3.28464984893799)
--(axis cs:21700,3.42427968978882)
--(axis cs:21600,3.41652822494507)
--(axis cs:21500,3.39010000228882)
--(axis cs:21400,3.314208984375)
--(axis cs:21300,3.314208984375)
--(axis cs:21200,3.21886563301086)
--(axis cs:21100,3.26416921615601)
--(axis cs:21000,3.14879584312439)
--(axis cs:20900,3.20102143287659)
--(axis cs:20800,3.24071264266968)
--(axis cs:20700,3.20414972305298)
--(axis cs:20600,3.17280292510986)
--(axis cs:20500,3.18395662307739)
--(axis cs:20400,3.21115779876709)
--(axis cs:20300,3.27118396759033)
--(axis cs:20200,3.28809499740601)
--(axis cs:20100,3.31080961227417)
--(axis cs:20000,3.82589387893677)
--(axis cs:19900,3.87583494186401)
--(axis cs:19800,3.94293165206909)
--(axis cs:19700,4.06288003921509)
--(axis cs:19600,4.14494657516479)
--(axis cs:19500,3.79407262802124)
--(axis cs:19400,3.39671635627747)
--(axis cs:19300,3.314208984375)
--(axis cs:19200,3.314208984375)
--(axis cs:19100,3.33260488510132)
--(axis cs:19000,3.314208984375)
--(axis cs:18900,3.314208984375)
--(axis cs:18800,3.49779057502747)
--(axis cs:18700,3.47506093978882)
--(axis cs:18600,3.2810230255127)
--(axis cs:18500,3.23034048080444)
--(axis cs:18400,3.28388977050781)
--(axis cs:18300,3.28841972351074)
--(axis cs:18200,3.26759171485901)
--(axis cs:18100,3.30141520500183)
--(axis cs:18000,3.76045227050781)
--(axis cs:17900,3.74915647506714)
--(axis cs:17800,3.94078779220581)
--(axis cs:17700,3.97451186180115)
--(axis cs:17600,4.2712550163269)
--(axis cs:17500,3.86858773231506)
--(axis cs:17400,4.0525369644165)
--(axis cs:17300,4.10319852828979)
--(axis cs:17200,4.04108285903931)
--(axis cs:17100,3.77439880371094)
--(axis cs:17000,3.87755298614502)
--(axis cs:16900,3.74327564239502)
--(axis cs:16800,3.50828862190247)
--(axis cs:16700,3.92070341110229)
--(axis cs:16600,4.08161735534668)
--(axis cs:16500,4.04100036621094)
--(axis cs:16400,4.09148788452148)
--(axis cs:16300,3.87878322601318)
--(axis cs:16200,3.41092562675476)
--(axis cs:16100,3.23454594612122)
--(axis cs:16000,3.18770289421082)
--(axis cs:15900,3.10547709465027)
--(axis cs:15800,3.26482939720154)
--(axis cs:15700,3.26515007019043)
--(axis cs:15600,3.52773809432983)
--(axis cs:15500,3.52309799194336)
--(axis cs:15400,3.25101613998413)
--(axis cs:15300,3.34386563301086)
--(axis cs:15200,3.38904094696045)
--(axis cs:15100,3.55247592926025)
--(axis cs:15000,3.73790502548218)
--(axis cs:14900,4.18122482299805)
--(axis cs:14800,4.18799829483032)
--(axis cs:14700,4.01092004776001)
--(axis cs:14600,3.79857110977173)
--(axis cs:14500,3.51630258560181)
--(axis cs:14400,3.58951425552368)
--(axis cs:14300,3.8664665222168)
--(axis cs:14200,3.87329816818237)
--(axis cs:14100,3.73712038993835)
--(axis cs:14000,3.98779296875)
--(axis cs:13900,3.77278900146484)
--(axis cs:13800,3.57837319374084)
--(axis cs:13700,3.70303797721863)
--(axis cs:13600,4.10337448120117)
--(axis cs:13500,4.2605619430542)
--(axis cs:13400,4.31583738327026)
--(axis cs:13300,4.14130973815918)
--(axis cs:13200,4.17723369598389)
--(axis cs:13100,4.20536613464355)
--(axis cs:13000,4.16358661651611)
--(axis cs:12900,4.27867746353149)
--(axis cs:12800,4.34906005859375)
--(axis cs:12700,4.29407978057861)
--(axis cs:12600,4.61332225799561)
--(axis cs:12500,4.34491491317749)
--(axis cs:12400,4.58044767379761)
--(axis cs:12300,4.60934686660767)
--(axis cs:12200,4.61270761489868)
--(axis cs:12100,4.84897470474243)
--(axis cs:12000,5.19589900970459)
--(axis cs:11900,5.25280904769897)
--(axis cs:11800,5.12901210784912)
--(axis cs:11700,4.72062253952026)
--(axis cs:11600,4.10224914550781)
--(axis cs:11500,4.45362663269043)
--(axis cs:11400,4.50425004959106)
--(axis cs:11300,4.97426748275757)
--(axis cs:11200,5.25754308700562)
--(axis cs:11100,5.32016897201538)
--(axis cs:11000,5.45561742782593)
--(axis cs:10900,5.31862878799438)
--(axis cs:10800,5.73125314712524)
--(axis cs:10700,5.41918897628784)
--(axis cs:10600,5.30516004562378)
--(axis cs:10500,5.78970623016357)
--(axis cs:10400,5.549072265625)
--(axis cs:10300,5.19104862213135)
--(axis cs:10200,4.89783048629761)
--(axis cs:10100,5.01844549179077)
--(axis cs:10000,4.59472513198853)
--(axis cs:9900,4.82262182235718)
--(axis cs:9800,4.39368915557861)
--(axis cs:9700,4.33928680419922)
--(axis cs:9600,4.84047365188599)
--(axis cs:9500,4.48266649246216)
--(axis cs:9400,4.56843280792236)
--(axis cs:9300,4.77938652038574)
--(axis cs:9200,5.27684926986694)
--(axis cs:9100,5.19427394866943)
--(axis cs:9000,5.87347459793091)
--(axis cs:8900,6.28353261947632)
--(axis cs:8800,6.26194334030151)
--(axis cs:8700,6.47100353240967)
--(axis cs:8600,6.05547714233398)
--(axis cs:8500,6.39884281158447)
--(axis cs:8400,7.01039218902588)
--(axis cs:8300,7.22368478775024)
--(axis cs:8200,7.04433441162109)
--(axis cs:8100,7.83882284164429)
--(axis cs:8000,7.11802768707275)
--(axis cs:7900,6.52932739257812)
--(axis cs:7800,6.72937250137329)
--(axis cs:7700,6.78148698806763)
--(axis cs:7600,6.71542930603027)
--(axis cs:7500,6.76961517333984)
--(axis cs:7400,6.68923854827881)
--(axis cs:7300,6.94512557983398)
--(axis cs:7200,7.01997518539429)
--(axis cs:7100,6.62769556045532)
--(axis cs:7000,7.03955507278442)
--(axis cs:6900,6.6445779800415)
--(axis cs:6800,6.55258798599243)
--(axis cs:6700,6.53139877319336)
--(axis cs:6600,6.84446811676025)
--(axis cs:6500,6.78482055664062)
--(axis cs:6400,7.48538637161255)
--(axis cs:6300,7.81506061553955)
--(axis cs:6200,8.23427772521973)
--(axis cs:6100,8.15260791778564)
--(axis cs:6000,8.27439594268799)
--(axis cs:5900,8.78911972045898)
--(axis cs:5800,9.48759841918945)
--(axis cs:5700,9.54146194458008)
--(axis cs:5600,9.99423503875732)
--(axis cs:5500,9.70250797271729)
--(axis cs:5400,9.257248878479)
--(axis cs:5300,7.88515615463257)
--(axis cs:5200,9.0504846572876)
--(axis cs:5100,8.72604370117188)
--(axis cs:5000,8.58375263214111)
--(axis cs:4900,9.84212112426758)
--(axis cs:4800,10.8238315582275)
--(axis cs:4700,10.2401218414307)
--(axis cs:4600,10.0807847976685)
--(axis cs:4500,8.62196063995361)
--(axis cs:4400,8.96025657653809)
--(axis cs:4300,9.75087928771973)
--(axis cs:4200,8.8569278717041)
--(axis cs:4100,8.68159484863281)
--(axis cs:4000,9.64551734924316)
--(axis cs:3900,7.8516731262207)
--(axis cs:3800,7.34218692779541)
--(axis cs:3700,7.57635974884033)
--(axis cs:3600,8.10210037231445)
--(axis cs:3500,7.04123401641846)
--(axis cs:3400,6.58416604995728)
--(axis cs:3300,6.11940479278564)
--(axis cs:3200,4.95528507232666)
--(axis cs:3100,3.88849282264709)
--(axis cs:3000,4.70580434799194)
--(axis cs:2900,4.95373296737671)
--(axis cs:2800,4.2487587928772)
--(axis cs:2700,4.43647003173828)
--(axis cs:2600,4.61850214004517)
--(axis cs:2500,4.12643051147461)
--(axis cs:2400,3.53213047981262)
--(axis cs:2300,3.38777780532837)
--(axis cs:2200,3.15801095962524)
--(axis cs:2100,2.46476554870605)
--(axis cs:2000,2.34285092353821)
--(axis cs:1900,1.62428593635559)
--(axis cs:1800,1.25765812397003)
--(axis cs:1700,1.38605165481567)
--(axis cs:1600,1.219083070755)
--(axis cs:1500,1.09288311004639)
--(axis cs:1400,0.769291818141937)
--(axis cs:1300,0.79917311668396)
--(axis cs:1200,0.57192051410675)
--(axis cs:1100,0.390252649784088)
--(axis cs:1000,0.118704959750175)
--(axis cs:900,0.0854143053293228)
--(axis cs:800,0.0143444538116455)
--(axis cs:700,0.016373835504055)
--(axis cs:600,0.0186504330486059)
--(axis cs:500,0.0213629752397537)
--(axis cs:400,0.0237089712172747)
--(axis cs:300,0.0260407999157906)
--(axis cs:200,8.40727806091309)
--(axis cs:100,8.419264793396)
--(axis cs:0,8.41387367248535)
--cycle;

\path [fill=white!50.1960784313725!black, fill opacity=0.4, semithick]
(axis cs:0,0.0306430757045746)
--(axis cs:0,0.0231263339519501)
--(axis cs:100,0.0231263302266598)
--(axis cs:200,0.00338825769722462)
--(axis cs:300,0)
--(axis cs:400,0)
--(axis cs:500,0)
--(axis cs:600,0)
--(axis cs:700,0)
--(axis cs:800,0)
--(axis cs:900,0)
--(axis cs:1000,0)
--(axis cs:1100,0)
--(axis cs:1200,0)
--(axis cs:1300,0)
--(axis cs:1400,0)
--(axis cs:1500,0)
--(axis cs:1600,0)
--(axis cs:1700,1.56588976096828e-06)
--(axis cs:1800,3.1724571272207e-06)
--(axis cs:1900,3.1724571272207e-06)
--(axis cs:2000,0.000112820358481258)
--(axis cs:2100,8.82067834027112e-05)
--(axis cs:2200,7.22300610505044e-05)
--(axis cs:2300,1.94787971850019e-05)
--(axis cs:2400,8.87958449311554e-05)
--(axis cs:2500,0.000182356248842552)
--(axis cs:2600,0.000306989531964064)
--(axis cs:2700,0.000302503525745124)
--(axis cs:2800,1.30459666252136e-05)
--(axis cs:2900,5.82337361265672e-06)
--(axis cs:3000,5.8144332797383e-06)
--(axis cs:3100,5.82039365326636e-06)
--(axis cs:3200,2.0828843844356e-05)
--(axis cs:3300,2.64212485490134e-05)
--(axis cs:3400,9.18805599212646e-05)
--(axis cs:3500,0.000110789958853275)
--(axis cs:3600,4.8908590542851e-05)
--(axis cs:3700,0.00094863201957196)
--(axis cs:3800,0.001009761239402)
--(axis cs:3900,0.00104896200355142)
--(axis cs:4000,0.0024506589397788)
--(axis cs:4100,0.00314658577553928)
--(axis cs:4200,0.00347458105534315)
--(axis cs:4300,0.00319546647369862)
--(axis cs:4400,0.00316424574702978)
--(axis cs:4500,0.00714557524770498)
--(axis cs:4600,0.0119987698271871)
--(axis cs:4700,0.0118821710348129)
--(axis cs:4800,0.0131911281496286)
--(axis cs:4900,0.0133456820622087)
--(axis cs:5000,0.00327818980440497)
--(axis cs:5100,0.00317096407525241)
--(axis cs:5200,0.00236369064077735)
--(axis cs:5300,0.00223620235919952)
--(axis cs:5400,0.00132255558855832)
--(axis cs:5500,0.00246542389504611)
--(axis cs:5600,0.00219684233888984)
--(axis cs:5700,0.00213754782453179)
--(axis cs:5800,0.00194246170576662)
--(axis cs:5900,0.00271777180023491)
--(axis cs:6000,0.0035963177215308)
--(axis cs:6100,0.00313019147142768)
--(axis cs:6200,0.00308444094844162)
--(axis cs:6300,0.00359275727532804)
--(axis cs:6400,0.00157132698222995)
--(axis cs:6500,0.00141265976708382)
--(axis cs:6600,0.00134988618083298)
--(axis cs:6700,0.00121315126307309)
--(axis cs:6800,0.000655686832033098)
--(axis cs:6900,0.000920151243917644)
--(axis cs:7000,0.00143891246989369)
--(axis cs:7100,0.00151478894986212)
--(axis cs:7200,0.000719074159860611)
--(axis cs:7300,0.000892358482815325)
--(axis cs:7400,0.000644936983007938)
--(axis cs:7500,0.000911350653041154)
--(axis cs:7600,0.00115555943921208)
--(axis cs:7700,0.00121102214325219)
--(axis cs:7800,0.000859034073073417)
--(axis cs:7900,0.000390279281418771)
--(axis cs:8000,0.000365513551514596)
--(axis cs:8100,0.000537019979674369)
--(axis cs:8200,0.00053558946819976)
--(axis cs:8300,0.000778625137172639)
--(axis cs:8400,0.000749355531297624)
--(axis cs:8500,0.000982785248197615)
--(axis cs:8600,0.000862872577272356)
--(axis cs:8700,0.0010582268005237)
--(axis cs:8800,0.00137609243392944)
--(axis cs:8900,0.00177283282391727)
--(axis cs:9000,0.00162828562315553)
--(axis cs:9100,0.00159947900101542)
--(axis cs:9200,0.0015117364237085)
--(axis cs:9300,0.00127026706468314)
--(axis cs:9400,0.00101182307116687)
--(axis cs:9500,0.000744598684832454)
--(axis cs:9600,0.000785844633355737)
--(axis cs:9700,0.00117454468272626)
--(axis cs:9800,0.00135883805342019)
--(axis cs:9900,0.00137715239543468)
--(axis cs:10000,0.00114104757085443)
--(axis cs:10100,0.00118723465129733)
--(axis cs:10200,0.000624072563368827)
--(axis cs:10300,0.000584291410632432)
--(axis cs:10400,0.000676490366458893)
--(axis cs:10500,0.000428461207775399)
--(axis cs:10600,0.000492548220790923)
--(axis cs:10700,0.000626984518021345)
--(axis cs:10800,0.000534101389348507)
--(axis cs:10900,0.000474438042147085)
--(axis cs:11000,0.000811497797258198)
--(axis cs:11100,0.000749161234125495)
--(axis cs:11200,0.000624201842583716)
--(axis cs:11300,0.000784655567258596)
--(axis cs:11400,0.00103067851159722)
--(axis cs:11500,0.000682958227116615)
--(axis cs:11600,0.000660856545437127)
--(axis cs:11700,0.000593145727179945)
--(axis cs:11800,0.000511708436533809)
--(axis cs:11900,0.000276580336503685)
--(axis cs:12000,0.000406174804084003)
--(axis cs:12100,0.000514661893248558)
--(axis cs:12200,0.00186668639071286)
--(axis cs:12300,0.00206595659255981)
--(axis cs:12400,0.00165327789727598)
--(axis cs:12500,0.00199082773178816)
--(axis cs:12600,0.000628334295470268)
--(axis cs:12700,0.000941379112191498)
--(axis cs:12800,0.000940232130233198)
--(axis cs:12900,0.000790353398770094)
--(axis cs:13000,0.000453878659754992)
--(axis cs:13100,0.000493492814712226)
--(axis cs:13200,0.000401360273826867)
--(axis cs:13300,0.000313533295411617)
--(axis cs:13400,0.000267301395069808)
--(axis cs:13500,0.000303760141832754)
--(axis cs:13600,0.000240279536228627)
--(axis cs:13700,0.000322145235259086)
--(axis cs:13800,0.000351387250702828)
--(axis cs:13900,0.00041383015923202)
--(axis cs:14000,0.000455067143775523)
--(axis cs:14100,0.000467108708107844)
--(axis cs:14200,0.00050036096945405)
--(axis cs:14300,0.000778978108428419)
--(axis cs:14400,0.000757545232772827)
--(axis cs:14500,0.00068353780079633)
--(axis cs:14600,0.000523941591382027)
--(axis cs:14700,0.000588183291256428)
--(axis cs:14800,0.000549827178474516)
--(axis cs:14900,0.000472489977255464)
--(axis cs:15000,0.000554842583369464)
--(axis cs:15100,0.000717753544449806)
--(axis cs:15200,0.000561713124625385)
--(axis cs:15300,0.000371574104065076)
--(axis cs:15400,0.000343527499353513)
--(axis cs:15500,0.000393365626223385)
--(axis cs:15600,0.000342470419127494)
--(axis cs:15700,0.000349378591636196)
--(axis cs:15800,0.000234466788242571)
--(axis cs:15900,0.000353199255187064)
--(axis cs:16000,0.000216448301216587)
--(axis cs:16100,0.000228673685342073)
--(axis cs:16200,0.00043259741505608)
--(axis cs:16300,0.000683778547681868)
--(axis cs:16400,0.000549513089936227)
--(axis cs:16500,0.000457665300928056)
--(axis cs:16600,0.000638294208329171)
--(axis cs:16700,0.000621211540419608)
--(axis cs:16800,0.000504835217725486)
--(axis cs:16900,0.000512643018737435)
--(axis cs:17000,0.000468643673229963)
--(axis cs:17100,0.000401222700020298)
--(axis cs:17200,0.000566810369491577)
--(axis cs:17300,0.000435558147728443)
--(axis cs:17400,0.000510714598931372)
--(axis cs:17500,0.000539803295396268)
--(axis cs:17600,0.000478164030937478)
--(axis cs:17700,0.000323976622894406)
--(axis cs:17800,0.000367301050573587)
--(axis cs:17900,0.000446119112893939)
--(axis cs:18000,0.000352954433765262)
--(axis cs:18100,0.000381519610527903)
--(axis cs:18200,0.000446636695414782)
--(axis cs:18300,0.000484651332953945)
--(axis cs:18400,0.000417876231949776)
--(axis cs:18500,0.00042082933941856)
--(axis cs:18600,0.000271457422059029)
--(axis cs:18700,0.000233244893024676)
--(axis cs:18800,0.000262262299656868)
--(axis cs:18900,0.000411093875300139)
--(axis cs:19000,0.000394359783967957)
--(axis cs:19100,0.000331103801727295)
--(axis cs:19200,0.000337026314809918)
--(axis cs:19300,0.000283943169051781)
--(axis cs:19400,0.000171279913047329)
--(axis cs:19500,0.000237482279771939)
--(axis cs:19600,0.000282644061371684)
--(axis cs:19700,0.000309860508423299)
--(axis cs:19800,0.000291567121166736)
--(axis cs:19900,0.00019612887990661)
--(axis cs:20000,0.000228047501877882)
--(axis cs:20100,0.000378301367163658)
--(axis cs:20200,0.000356118194758892)
--(axis cs:20300,0.000432317901868373)
--(axis cs:20400,0.000396716583054513)
--(axis cs:20500,0.000451327534392476)
--(axis cs:20600,0.000298274244414642)
--(axis cs:20700,0.000231344951316714)
--(axis cs:20800,0.000247871328610927)
--(axis cs:20900,0.000193465384654701)
--(axis cs:21000,6.74217299092561e-05)
--(axis cs:21100,6.26023393124342e-05)
--(axis cs:21200,7.37353402655572e-05)
--(axis cs:21300,4.29153442382812e-06)
--(axis cs:21400,3.18690144922584e-05)
--(axis cs:21500,2.20899819396436e-05)
--(axis cs:21600,6.35610776953399e-05)
--(axis cs:21700,6.05004897806793e-05)
--(axis cs:21800,6.2726714531891e-05)
--(axis cs:21900,4.80856106150895e-05)
--(axis cs:22000,4.03893645852804e-05)
--(axis cs:22100,5.40213659405708e-05)
--(axis cs:22200,3.16277437377721e-05)
--(axis cs:22300,4.29153442382812e-06)
--(axis cs:22400,2.03393865376711e-05)
--(axis cs:22500,2.50051671173424e-05)
--(axis cs:22600,2.29529978241771e-05)
--(axis cs:22700,4.06062754336745e-05)
--(axis cs:22800,6.46154949208722e-05)
--(axis cs:22900,6.3784042140469e-05)
--(axis cs:23000,6.14208547631279e-05)
--(axis cs:23100,6.27589906798676e-05)
--(axis cs:23200,5.7519762776792e-05)
--(axis cs:23300,5.82901848247275e-05)
--(axis cs:23400,3.69577828678302e-05)
--(axis cs:23500,5.90596318943426e-05)
--(axis cs:23600,5.4344956879504e-05)
--(axis cs:23700,5.70487172808498e-05)
--(axis cs:23800,6.39140635030344e-05)
--(axis cs:23900,6.57892669551075e-05)
--(axis cs:24000,6.60006335237995e-05)
--(axis cs:24100,6.56504707876593e-05)
--(axis cs:24200,4.88411460537463e-05)
--(axis cs:24300,5.59390755370259e-05)
--(axis cs:24400,5.84973458899185e-05)
--(axis cs:24500,6.44797692075372e-05)
--(axis cs:24600,6.45109103061259e-05)
--(axis cs:24700,6.00662606302649e-05)
--(axis cs:24800,5.37101295776665e-05)
--(axis cs:24900,5.28728123754263e-05)
--(axis cs:25000,3.83493024855852e-05)
--(axis cs:25100,3.77686519641429e-05)
--(axis cs:25200,6.54003233648837e-05)
--(axis cs:25300,6.13825977779925e-05)
--(axis cs:25400,6.58081698929891e-05)
--(axis cs:25500,6.40425714664161e-05)
--(axis cs:25600,5.96754543948919e-05)
--(axis cs:25700,2.87913135252893e-05)
--(axis cs:25800,3.07034933939576e-05)
--(axis cs:25900,4.68004436697811e-05)
--(axis cs:26000,4.47649508714676e-05)
--(axis cs:26100,6.34065072517842e-05)
--(axis cs:26200,3.69256958947517e-05)
--(axis cs:26300,4.22230150434189e-05)
--(axis cs:26400,6.12229196121916e-05)
--(axis cs:26500,5.34377322765067e-05)
--(axis cs:26600,5.34143036929891e-05)
--(axis cs:26700,5.8580408222042e-05)
--(axis cs:26800,5.83185610594228e-05)
--(axis cs:26900,5.95040619373322e-05)
--(axis cs:27000,5.37692540092394e-05)
--(axis cs:27100,6.27976696705446e-05)
--(axis cs:27200,5.95026358496398e-05)
--(axis cs:27300,6.60377991152927e-05)
--(axis cs:27400,5.81265630898997e-05)
--(axis cs:27500,5.6546414270997e-05)
--(axis cs:27600,5.22584887221456e-05)
--(axis cs:27700,4.96001448482275e-05)
--(axis cs:27800,5.27006632182747e-05)
--(axis cs:27900,4.78716683574021e-05)
--(axis cs:28000,6.60478690406308e-05)
--(axis cs:28100,6.54564355500042e-05)
--(axis cs:28200,6.42421509837732e-05)
--(axis cs:28300,5.70849952055141e-05)
--(axis cs:28400,5.53303543711081e-05)
--(axis cs:28500,5.1965267630294e-05)
--(axis cs:28600,5.83600922254845e-05)
--(axis cs:28700,5.06074575241655e-05)
--(axis cs:28800,4.90575330331922e-05)
--(axis cs:28900,4.96456050314009e-05)
--(axis cs:29000,5.04830095451325e-05)
--(axis cs:29100,5.76744641875848e-05)
--(axis cs:29200,3.72101931134239e-05)
--(axis cs:29300,2.01639923034236e-05)
--(axis cs:29400,3.06696892948821e-05)
--(axis cs:29500,5.35946746822447e-05)
--(axis cs:29600,5.55465085199103e-05)
--(axis cs:29700,6.03445369051769e-05)
--(axis cs:29800,6.60401565255597e-05)
--(axis cs:29900,6.60672376397997e-05)
--(axis cs:30000,6.49206194793805e-05)
--(axis cs:30100,6.46524858893827e-05)
--(axis cs:30200,6.20311184320599e-05)
--(axis cs:30300,6.26942201051861e-05)
--(axis cs:30400,6.15386379649863e-05)
--(axis cs:30500,6.23490050202236e-05)
--(axis cs:30600,6.4222447690554e-05)
--(axis cs:30700,6.5939748310484e-05)
--(axis cs:30800,6.56483753118664e-05)
--(axis cs:30900,5.91143179917708e-05)
--(axis cs:31000,6.08108821325004e-05)
--(axis cs:31100,6.08914560871199e-05)
--(axis cs:31200,5.79154147999361e-05)
--(axis cs:31300,4.2945561290253e-05)
--(axis cs:31400,5.77535975025967e-05)
--(axis cs:31500,5.99377817707136e-05)
--(axis cs:31600,6.12288422416896e-05)
--(axis cs:31700,5.06207725265995e-05)
--(axis cs:31800,5.03953342558816e-05)
--(axis cs:31900,6.24826934654266e-05)
--(axis cs:32000,6.33380404906347e-05)
--(axis cs:32100,6.19651400484145e-05)
--(axis cs:32200,6.27229019301012e-05)
--(axis cs:32300,6.49468856863678e-05)
--(axis cs:32400,5.11507387273014e-05)
--(axis cs:32500,4.60196679341607e-05)
--(axis cs:32600,6.56460324535146e-05)
--(axis cs:32700,6.56132906442508e-05)
--(axis cs:32700,0.000429808569606394)
--(axis cs:32700,0.000429808569606394)
--(axis cs:32600,0.000428798317443579)
--(axis cs:32500,0.000289741234155372)
--(axis cs:32400,0.000296622514724731)
--(axis cs:32300,0.00034842491731979)
--(axis cs:32200,0.000311851501464844)
--(axis cs:32100,0.000302934640785679)
--(axis cs:32000,0.000320005405228585)
--(axis cs:31900,0.000308907037833706)
--(axis cs:31800,0.000296622514724731)
--(axis cs:31700,0.000296622514724731)
--(axis cs:31600,0.000296622514724731)
--(axis cs:31500,0.000296622514724731)
--(axis cs:31400,0.000296622514724731)
--(axis cs:31300,0.000284581969026476)
--(axis cs:31200,0.000296622514724731)
--(axis cs:31100,0.000296622514724731)
--(axis cs:31000,0.000296622514724731)
--(axis cs:30900,0.000296622514724731)
--(axis cs:30800,0.000369119632523507)
--(axis cs:30700,0.000384235376259312)
--(axis cs:30600,0.00045935669913888)
--(axis cs:30500,0.000486422970425338)
--(axis cs:30400,0.000496460183057934)
--(axis cs:30300,0.000481913419207558)
--(axis cs:30200,0.000490444363094866)
--(axis cs:30100,0.000342011451721191)
--(axis cs:30000,0.000347816938301548)
--(axis cs:29900,0.000401794910430908)
--(axis cs:29800,0.000394451606553048)
--(axis cs:29700,0.000296622514724731)
--(axis cs:29600,0.000296622514724731)
--(axis cs:29500,0.000296622514724731)
--(axis cs:29400,0.000269360200036317)
--(axis cs:29300,0.00026055402122438)
--(axis cs:29200,0.000276592385489494)
--(axis cs:29100,0.000296622514724731)
--(axis cs:29000,0.00060199317522347)
--(axis cs:28900,0.000608878443017602)
--(axis cs:28800,0.000613662705291063)
--(axis cs:28700,0.00060096278320998)
--(axis cs:28600,0.000531070225406438)
--(axis cs:28500,0.000296622514724731)
--(axis cs:28400,0.000296622514724731)
--(axis cs:28300,0.000296622514724731)
--(axis cs:28200,0.000334215175826102)
--(axis cs:28100,0.000362265098374337)
--(axis cs:28000,0.000395798677345738)
--(axis cs:27900,0.000623193220235407)
--(axis cs:27800,0.0005832928000018)
--(axis cs:27700,0.000609249749686569)
--(axis cs:27600,0.000587080779951066)
--(axis cs:27500,0.00054873077897355)
--(axis cs:27400,0.000296622514724731)
--(axis cs:27300,0.000394082075217739)
--(axis cs:27200,0.000296622514724731)
--(axis cs:27100,0.000312793243210763)
--(axis cs:27000,0.000296622514724731)
--(axis cs:26900,0.000296622514724731)
--(axis cs:26800,0.000296622514724731)
--(axis cs:26700,0.000296622514724731)
--(axis cs:26600,0.000296622514724731)
--(axis cs:26500,0.000296622514724731)
--(axis cs:26400,0.000296622514724731)
--(axis cs:26300,0.000283468660200015)
--(axis cs:26200,0.000276241102255881)
--(axis cs:26100,0.000472029991215095)
--(axis cs:26000,0.000647519191261381)
--(axis cs:25900,0.00063167919870466)
--(axis cs:25800,0.000750041857827455)
--(axis cs:25700,0.000763342482969165)
--(axis cs:25600,0.000517452484928071)
--(axis cs:25500,0.000330781942466274)
--(axis cs:25400,0.000423160498030484)
--(axis cs:25300,0.000296723854262382)
--(axis cs:25200,0.000360488891601562)
--(axis cs:25100,0.000699751428328454)
--(axis cs:25000,0.000695522932801396)
--(axis cs:24900,0.00058180937776342)
--(axis cs:24800,0.000574518868234009)
--(axis cs:24700,0.000513239065185189)
--(axis cs:24600,0.000454363413155079)
--(axis cs:24500,0.000454919063486159)
--(axis cs:24400,0.000529685232322663)
--(axis cs:24300,0.000554416445083916)
--(axis cs:24200,0.000615412835031748)
--(axis cs:24100,0.000369203102309257)
--(axis cs:24000,0.000389480584999546)
--(axis cs:23900,0.000375318515580148)
--(axis cs:23800,0.000328671943861991)
--(axis cs:23700,0.000296622514724731)
--(axis cs:23600,0.000296622514724731)
--(axis cs:23500,0.000296622514724731)
--(axis cs:23400,0.000276280508842319)
--(axis cs:23300,0.000296622514724731)
--(axis cs:23200,0.000296622514724731)
--(axis cs:23100,0.000312304502585903)
--(axis cs:23000,0.000297117221634835)
--(axis cs:22900,0.000326609617331997)
--(axis cs:22800,0.000341260427376255)
--(axis cs:22700,0.000678921118378639)
--(axis cs:22600,0.000803314382210374)
--(axis cs:22500,0.000789365149103105)
--(axis cs:22400,0.000820940418634564)
--(axis cs:22300,0.00108089949935675)
--(axis cs:22200,0.000743570388294756)
--(axis cs:22100,0.0005717757740058)
--(axis cs:22000,0.000680528813973069)
--(axis cs:21900,0.000621485174633563)
--(axis cs:21800,0.000311899173539132)
--(axis cs:21700,0.000296622514724731)
--(axis cs:21600,0.000360614067176357)
--(axis cs:21500,0.000295634556096047)
--(axis cs:21400,0.00038749334635213)
--(axis cs:21300,0.000431094085797668)
--(axis cs:21200,0.000564546906389296)
--(axis cs:21100,0.000764197495300323)
--(axis cs:21000,0.00084747385699302)
--(axis cs:20900,0.000939193763770163)
--(axis cs:20800,0.00085969822248444)
--(axis cs:20700,0.000763381132856011)
--(axis cs:20600,0.000505784526467323)
--(axis cs:20500,0.000552331213839352)
--(axis cs:20400,0.000587330316193402)
--(axis cs:20300,0.000609409820754081)
--(axis cs:20200,0.00058870913926512)
--(axis cs:20100,0.000691056251525879)
--(axis cs:20000,0.000680454424582422)
--(axis cs:19900,0.000585872097872198)
--(axis cs:19800,0.000657883239910007)
--(axis cs:19700,0.000681118399370462)
--(axis cs:19600,0.000626231369096786)
--(axis cs:19500,0.00055654050083831)
--(axis cs:19400,0.000800590612925589)
--(axis cs:19300,0.00083296443335712)
--(axis cs:19200,0.00098073307890445)
--(axis cs:19100,0.00107223936356604)
--(axis cs:19000,0.00111384829506278)
--(axis cs:18900,0.000817757856566459)
--(axis cs:18800,0.00056940910872072)
--(axis cs:18700,0.000532862497493625)
--(axis cs:18600,0.000586670299526304)
--(axis cs:18500,0.000433194625657052)
--(axis cs:18400,0.00109824188984931)
--(axis cs:18300,0.00133301073219627)
--(axis cs:18200,0.00139070826116949)
--(axis cs:18100,0.00125109124928713)
--(axis cs:18000,0.00129413651302457)
--(axis cs:17900,0.00144243822433054)
--(axis cs:17800,0.00143080821726471)
--(axis cs:17700,0.00127321726176888)
--(axis cs:17600,0.00129726529121399)
--(axis cs:17500,0.00138112728018314)
--(axis cs:17400,0.000745803117752075)
--(axis cs:17300,0.000646996486466378)
--(axis cs:17200,0.000789068173617125)
--(axis cs:17100,0.000868092523887753)
--(axis cs:17000,0.00080181349767372)
--(axis cs:16900,0.000768876052461565)
--(axis cs:16800,0.000770672399085015)
--(axis cs:16700,0.000682532670907676)
--(axis cs:16600,0.000894022348802537)
--(axis cs:16500,0.000839029671624303)
--(axis cs:16400,0.000665177183691412)
--(axis cs:16300,0.00100823643151671)
--(axis cs:16200,0.00103776156902313)
--(axis cs:16100,0.0011181925656274)
--(axis cs:16000,0.00206673704087734)
--(axis cs:15900,0.00188990391325206)
--(axis cs:15800,0.00145033316221088)
--(axis cs:15700,0.00137086154427379)
--(axis cs:15600,0.00147497223224491)
--(axis cs:15500,0.000702688354067504)
--(axis cs:15400,0.00086618063505739)
--(axis cs:15300,0.00109796668402851)
--(axis cs:15200,0.00104960205499083)
--(axis cs:15100,0.000806992873549461)
--(axis cs:15000,0.000869799812790006)
--(axis cs:14900,0.000799063825979829)
--(axis cs:14800,0.00118718715384603)
--(axis cs:14700,0.00101103784982115)
--(axis cs:14600,0.0011989347403869)
--(axis cs:14500,0.00120780104771256)
--(axis cs:14400,0.00131765019614249)
--(axis cs:14300,0.001236826996319)
--(axis cs:14200,0.00134775647893548)
--(axis cs:14100,0.00122826592996716)
--(axis cs:14000,0.000950384128373116)
--(axis cs:13900,0.000829899334348738)
--(axis cs:13800,0.000449379731435329)
--(axis cs:13700,0.000478802161524072)
--(axis cs:13600,0.000404360587708652)
--(axis cs:13500,0.000473129737656564)
--(axis cs:13400,0.000607198453508317)
--(axis cs:13300,0.000439059745986015)
--(axis cs:13200,0.000806813884992152)
--(axis cs:13100,0.00105686776805669)
--(axis cs:13000,0.00129044719506055)
--(axis cs:12900,0.00176306581124663)
--(axis cs:12800,0.00174810038879514)
--(axis cs:12700,0.00156978366430849)
--(axis cs:12600,0.00291052460670471)
--(axis cs:12500,0.00472676288336515)
--(axis cs:12400,0.00468807620927691)
--(axis cs:12300,0.00466108880937099)
--(axis cs:12200,0.00496246619150043)
--(axis cs:12100,0.00497586792334914)
--(axis cs:12000,0.0012787461746484)
--(axis cs:11900,0.00130064610857517)
--(axis cs:11800,0.000835507526062429)
--(axis cs:11700,0.00111468625254929)
--(axis cs:11600,0.000798213470261544)
--(axis cs:11500,0.00133719807490706)
--(axis cs:11400,0.00163503887597471)
--(axis cs:11300,0.0016118228668347)
--(axis cs:11200,0.0012613475555554)
--(axis cs:11100,0.00156088452786207)
--(axis cs:11000,0.00144863489549607)
--(axis cs:10900,0.000958719872869551)
--(axis cs:10800,0.00117983424570411)
--(axis cs:10700,0.00127160223200917)
--(axis cs:10600,0.00116684508975595)
--(axis cs:10500,0.000901373918168247)
--(axis cs:10400,0.000774584710597992)
--(axis cs:10300,0.00105199520476162)
--(axis cs:10200,0.00169135432224721)
--(axis cs:10100,0.00166051986161619)
--(axis cs:10000,0.00183544750325382)
--(axis cs:9900,0.00182968482840806)
--(axis cs:9800,0.00323178456164896)
--(axis cs:9700,0.00322102359496057)
--(axis cs:9600,0.00299980537965894)
--(axis cs:9500,0.00388824776746333)
--(axis cs:9400,0.00332495500333607)
--(axis cs:9300,0.00262635061517358)
--(axis cs:9200,0.00260999612510204)
--(axis cs:9100,0.0026292959228158)
--(axis cs:9000,0.00181044987402856)
--(axis cs:8900,0.00223683612421155)
--(axis cs:8800,0.00345804309472442)
--(axis cs:8700,0.00346140749752522)
--(axis cs:8600,0.00394976418465376)
--(axis cs:8500,0.00425735302269459)
--(axis cs:8400,0.00412781909108162)
--(axis cs:8300,0.00237380480393767)
--(axis cs:8200,0.00297504896298051)
--(axis cs:8100,0.00323183601722121)
--(axis cs:8000,0.00382241583429277)
--(axis cs:7900,0.00399987027049065)
--(axis cs:7800,0.00358116440474987)
--(axis cs:7700,0.0030046715401113)
--(axis cs:7600,0.00225143833085895)
--(axis cs:7500,0.00173270329833031)
--(axis cs:7400,0.0023513447958976)
--(axis cs:7300,0.00242571299895644)
--(axis cs:7200,0.00177385029383004)
--(axis cs:7100,0.00217148056253791)
--(axis cs:7000,0.00331671955063939)
--(axis cs:6900,0.00347181688994169)
--(axis cs:6800,0.00314376223832369)
--(axis cs:6700,0.00362760503776371)
--(axis cs:6600,0.00294733070768416)
--(axis cs:6500,0.00199420447461307)
--(axis cs:6400,0.00280755572021008)
--(axis cs:6300,0.005852778442204)
--(axis cs:6200,0.00725432299077511)
--(axis cs:6100,0.00679267989471555)
--(axis cs:6000,0.00780160585418344)
--(axis cs:5900,0.00955414958298206)
--(axis cs:5800,0.00543675059452653)
--(axis cs:5700,0.009016796015203)
--(axis cs:5600,0.0114225083962083)
--(axis cs:5500,0.0104024764150381)
--(axis cs:5400,0.00875507108867168)
--(axis cs:5300,0.00929964333772659)
--(axis cs:5200,0.00533171836286783)
--(axis cs:5100,0.00453941896557808)
--(axis cs:5000,0.0112622445449233)
--(axis cs:4900,0.0158562194555998)
--(axis cs:4800,0.0153893530368805)
--(axis cs:4700,0.0152548868209124)
--(axis cs:4600,0.0144877852872014)
--(axis cs:4500,0.0147397397086024)
--(axis cs:4400,0.00623001763597131)
--(axis cs:4300,0.00558767002075911)
--(axis cs:4200,0.0054984213784337)
--(axis cs:4100,0.00849147327244282)
--(axis cs:4000,0.00481600174680352)
--(axis cs:3900,0.00465850066393614)
--(axis cs:3800,0.00459417654201388)
--(axis cs:3700,0.00407146476209164)
--(axis cs:3600,0.000885947374626994)
--(axis cs:3500,0.00062057888135314)
--(axis cs:3400,0.000565089634619653)
--(axis cs:3300,0.000492898107040673)
--(axis cs:3200,0.000619693193584681)
--(axis cs:3100,0.000653818831779063)
--(axis cs:3000,0.000663258484564722)
--(axis cs:2900,0.000705189071595669)
--(axis cs:2800,0.0012213122099638)
--(axis cs:2700,0.00110361468978226)
--(axis cs:2600,0.00081557035446167)
--(axis cs:2500,0.000816366053186357)
--(axis cs:2400,0.00174612016417086)
--(axis cs:2300,0.00163894076831639)
--(axis cs:2200,0.00119736674241722)
--(axis cs:2100,0.0011970242485404)
--(axis cs:2000,0.00121557246893644)
--(axis cs:1900,0.000473798660095781)
--(axis cs:1800,0.000473849358968437)
--(axis cs:1700,5.85056550335139e-05)
--(axis cs:1600,5.32619742443785e-05)
--(axis cs:1500,3.74135709080292e-07)
--(axis cs:1400,3.74135709080292e-07)
--(axis cs:1300,0)
--(axis cs:1200,0)
--(axis cs:1100,0)
--(axis cs:1000,0)
--(axis cs:900,0)
--(axis cs:800,0)
--(axis cs:700,0)
--(axis cs:600,0)
--(axis cs:500,0)
--(axis cs:400,0)
--(axis cs:300,0)
--(axis cs:200,0.00881713815033436)
--(axis cs:100,0.0306430608034134)
--(axis cs:0,0.0306430757045746)
--cycle;

\addplot [ultra thick, color0]
table {%
0 8.02285671234131
200 8.01188850402832
300 0.0127649931237102
400 0.0116200773045421
500 0.010469563305378
600 0.00921935867518187
700 0.00822855811566114
800 0.00728759728372097
900 0.0631113722920418
1000 0.0823204144835472
1100 0.271043390035629
1200 0.386493742465973
1300 0.611946046352386
1400 0.572146594524384
1500 0.804482996463776
1600 0.954561531543732
1700 1.02612626552582
1800 1.1938784122467
1900 1.52497792243958
2000 2.00888156890869
2100 2.16211676597595
2200 2.74640417098999
2300 3.08615374565125
2400 3.15682768821716
2500 3.46096873283386
2600 3.97202110290527
2700 3.99569797515869
2800 3.90579962730408
2900 4.45219659805298
3000 4.38059186935425
3100 3.79717826843262
3200 4.46060276031494
3300 5.16678476333618
3400 5.62940692901611
3500 5.83866834640503
3600 6.95056390762329
3700 6.98970651626587
3800 6.95466709136963
3900 7.36237764358521
4000 8.09850406646729
4100 7.6254768371582
4200 7.51403903961182
4300 7.78181838989258
4400 7.91416215896606
4500 8.00523662567139
4600 9.00368595123291
4700 9.23652172088623
4800 9.4207935333252
5000 8.30564594268799
5100 8.07543182373047
5200 8.0482931137085
5300 7.57342767715454
5400 8.63436508178711
5500 8.94951248168945
5600 8.6783561706543
5700 8.45694828033447
5800 9.12291812896729
5900 8.3579626083374
6000 7.97651195526123
6100 7.81741952896118
6200 7.94464015960693
6300 7.11860179901123
6400 6.6705207824707
6500 6.29312562942505
6600 6.34677076339722
6700 6.30088996887207
6900 6.42502450942993
7000 6.38777112960815
7100 6.4030613899231
7200 6.291907787323
7300 6.36771774291992
7400 6.27017068862915
7500 6.34333992004395
7600 5.8374981880188
7700 5.87226963043213
7800 5.73143148422241
7900 6.20656204223633
8000 6.48850297927856
8100 6.95723485946655
8200 6.38050222396851
8300 6.3445987701416
8500 5.50874757766724
8600 5.3769588470459
8700 5.57762718200684
8800 5.6437463760376
8900 5.81199550628662
9000 5.54354763031006
9100 5.0737738609314
9200 5.1360878944397
9300 4.69922399520874
9400 4.24691152572632
9600 4.41592741012573
9700 4.21882104873657
9800 4.22069501876831
9900 4.3081226348877
10000 4.35789346694946
10100 4.68083906173706
10200 4.81273698806763
10400 5.03342294692993
10500 5.02680635452271
10600 4.81105947494507
10700 4.8342490196228
10800 4.90513467788696
10900 4.82419490814209
11000 5.16555070877075
11100 4.93984079360962
11300 4.57365751266479
11400 4.20561122894287
11500 4.00507783889771
11600 4.00209188461304
11800 4.55427646636963
11900 4.68771934509277
12000 4.68807744979858
12100 4.59658622741699
12200 4.34490537643433
12300 4.06560468673706
12400 4.01132822036743
12500 3.97171258926392
12600 4.0576000213623
12700 3.978187084198
12800 4.0494065284729
13000 3.81913685798645
13100 3.86444520950317
13200 4.10762071609497
13300 3.99516606330872
13400 4.06655979156494
13500 3.86351728439331
13600 3.73480677604675
13700 3.54323697090149
13800 3.57127714157104
13900 3.67723369598389
14000 3.83620977401733
14100 3.66484355926514
14200 3.63022398948669
14400 3.37823867797852
14500 3.43866372108459
14600 3.48554658889771
14700 3.44660234451294
14800 3.55173397064209
14900 3.55396342277527
15000 3.28070092201233
15100 3.35397934913635
15200 3.33599424362183
15300 3.25266146659851
15400 3.19286227226257
15500 3.3028724193573
15600 3.24873089790344
15700 3.00797080993652
15800 2.96761918067932
15900 2.99080348014832
16000 3.10087513923645
16100 3.14485287666321
16200 3.2868447303772
16300 3.55244183540344
16400 3.49924349784851
16500 3.42398285865784
16600 3.46071028709412
16700 3.37460112571716
16800 3.16508436203003
16900 3.3100950717926
17000 3.27555322647095
17100 3.27390098571777
17200 3.43659639358521
17300 3.45109057426453
17400 3.35565519332886
17500 3.31242275238037
17600 3.42518711090088
17700 3.26439547538757
17800 3.25684428215027
17900 3.18035864830017
18000 3.28793478012085
18100 3.0262086391449
18200 3.0124351978302
18300 3.04627728462219
18400 3.04768896102905
18500 2.95286083221436
18600 2.99692821502686
18700 3.10954618453979
18800 3.13004970550537
18900 3.11223936080933
19000 3.1609411239624
19100 3.16083979606628
19200 3.0992431640625
19300 3.05238389968872
19400 3.04624032974243
19500 3.09570693969727
19600 3.53594541549683
19700 3.57744526863098
19800 3.5685715675354
19900 3.62050771713257
20000 3.55332827568054
20100 3.05853652954102
20200 3.0525598526001
20300 2.98433804512024
20400 2.93479442596436
20500 2.86130833625793
20600 2.83131527900696
20700 2.92368102073669
20800 3.00190854072571
20900 2.90149736404419
21000 2.7432541847229
21100 2.96304559707642
21200 2.86033153533936
21300 2.88781356811523
21400 2.99364852905273
21500 3.04029512405396
21600 3.00837063789368
21700 3.01662135124207
21800 2.83780884742737
22000 3.09070611000061
22100 2.99976444244385
22200 2.94683027267456
22300 3.03568124771118
22400 2.80984306335449
22500 2.67645668983459
22600 2.65469980239868
22700 2.62380743026733
22800 2.55384135246277
22900 2.60882973670959
23000 2.7046103477478
23100 2.67352700233459
23200 2.76914072036743
23300 2.82233452796936
23400 2.82621216773987
23500 2.87126493453979
23700 2.87418627738953
23800 2.81350898742676
23900 2.83924961090088
24000 2.74572801589966
24100 2.82126402854919
24300 2.82070350646973
24400 2.73783349990845
24500 2.78154277801514
24600 2.73286890983582
24700 2.65618515014648
24800 2.68862295150757
24900 2.77013278007507
25000 2.78116869926453
25100 2.70641279220581
25200 2.70181441307068
25300 2.72346186637878
25400 2.65816259384155
25600 2.73214507102966
25700 2.80267786979675
25800 2.72473978996277
25900 2.79856824874878
26000 2.69904732704163
26100 2.74163413047791
26200 2.6294960975647
26300 2.65742564201355
26400 2.69572377204895
26500 2.75500106811523
26600 2.67778754234314
26700 2.80546879768372
26800 2.80454087257385
26900 2.67153382301331
27000 2.61150717735291
27100 2.60992836952209
27200 2.40514326095581
27300 2.45013070106506
27400 2.43067240715027
27600 2.51282548904419
27700 2.58704447746277
27800 2.60462236404419
27900 2.69109725952148
28000 2.62236309051514
28100 2.65769052505493
28200 2.67240357398987
28300 2.67263174057007
28400 2.62760424613953
28500 2.65944838523865
28700 2.67246079444885
28800 2.57903671264648
28900 2.53594589233398
29000 2.63609981536865
29100 2.59337568283081
29200 2.52261543273926
29400 2.66378593444824
29500 2.57744932174683
29600 2.67221665382385
29700 2.75472807884216
29800 2.7459557056427
29900 2.69434404373169
30000 2.70751976966858
30100 2.73370766639709
30200 2.66475415229797
30300 2.62080097198486
30400 2.66865205764771
30500 2.68695497512817
30600 2.50160312652588
30700 2.57491850852966
30800 2.58745908737183
30900 2.56474614143372
31000 2.51649570465088
31100 2.55054521560669
31200 2.4798743724823
31300 2.54419755935669
};
\addplot [ultra thick, white!40.2745098039216!black]
table {%
0 0.0268847029656172
100 0.0268846955150366
200 0.00610269932076335
nan nan
1400 1.54972013888255e-07
1500 1.54972013888255e-07
1600 2.21977625187719e-05
1700 3.00357660307782e-05
1800 0.000203554300242104
1900 0.000203399366000667
2000 0.000664196559228003
2100 0.000642615545075387
2200 0.000634798547253013
2300 0.000700054515618831
2400 0.000917457917239517
2500 0.000513201928697526
2600 0.000565209134947509
2700 0.000703059020452201
2800 0.00055936211720109
2900 0.00034209992736578
3000 0.000331256742356345
3100 0.000301200110698119
3200 0.000287021131953225
3300 0.000236117368331179
3400 0.000298633269267157
3500 0.000365684478310868
3600 0.000466565281385556
3700 0.00251004821620882
3800 0.00280196871608496
3900 0.00285373139195144
4000 0.00382519024424255
4100 0.00581903010606766
4200 0.00465607549995184
4300 0.0045601730234921
4400 0.00482929963618517
4500 0.011493188329041
4600 0.0131754269823432
4700 0.0135685270652175
4800 0.0142262782901525
4900 0.0146009512245655
5000 0.00723568117246032
5100 0.00383315328508615
5200 0.00382903730496764
5300 0.00532755767926574
5400 0.00469263503327966
5500 0.00575459841638803
5600 0.00620127096772194
5700 0.00502439634874463
5800 0.00367808970622718
5900 0.00613596057519317
6000 0.00552066043019295
6100 0.00489796372130513
6200 0.00516938045620918
6300 0.0047227693721652
6400 0.00218944088555872
6500 0.00170903571415693
6600 0.00214860774576664
6700 0.00233749183826149
6800 0.00177851272746921
6900 0.00219598459079862
7000 0.00237781601026654
7100 0.00186251744162291
7200 0.00124646199401468
7300 0.00165903591550887
7400 0.00149814074393362
7500 0.00132202717941254
7600 0.00170349888503551
7700 0.0021078463178128
7900 0.00202075252309442
8000 0.00201718253083527
8100 0.00179734430275857
8200 0.00167857413180172
8300 0.00157621479593217
8400 0.00239862804301083
8500 0.00246334099210799
8700 0.00217081094160676
8800 0.0023390231654048
8900 0.00198206841014326
9000 0.00171642517670989
9100 0.00211438746191561
9200 0.00206086575053632
9300 0.00194830901455134
9400 0.00216838950291276
9500 0.00231642299331725
9600 0.00189282547216862
9700 0.00219778390601277
9800 0.00229531084187329
9900 0.00160341849550605
10000 0.00148849666584283
10100 0.00145295029506087
10200 0.00114528916310519
10300 0.000818143365904689
10400 0.000725537480320781
10500 0.000664917461108416
10600 0.000829696655273438
10700 0.000949293549638242
10800 0.000856967933941633
10900 0.000716579204890877
11000 0.00113006634637713
11100 0.00115502288099378
11200 0.000955913681536913
11300 0.00125864939764142
11400 0.00138044147752225
11600 0.00074049411341548
11700 0.000853915873449296
11800 0.000673608097713441
11900 0.000788612989708781
12000 0.000905076507478952
12100 0.00274526537396014
12200 0.00323062739335001
12300 0.00324807642027736
12400 0.00311931385658681
12500 0.00335879577323794
12600 0.00171405216678977
12700 0.00125861004926264
12800 0.00134416634682566
12900 0.00127670983783901
13000 0.000872162752784789
13100 0.000775180116761476
13200 0.00060408707940951
13300 0.000380297453375533
13400 0.000452913896879181
13500 0.000389941415050998
13600 0.0003223201201763
13700 0.000395236536860466
13800 0.000399585493141785
13900 0.000625393760856241
14100 0.000847687479108572
14300 0.00100790231954306
14400 0.00101918180007488
14500 0.000945669191423804
14600 0.000861438049469143
14700 0.000820328656118363
14800 0.00086850713705644
14900 0.000635776785202324
15000 0.000712321256287396
15200 0.000814586703199893
15300 0.000734770263079554
15400 0.000612974225077778
15500 0.000548026990145445
15600 0.00087379600154236
15700 0.000787369324825704
15800 0.000753086933400482
15900 0.00102836079895496
16000 0.00105289230123162
16100 0.000673433183692396
16200 0.000735179404728115
16300 0.000837415456771851
16400 0.000598740472923964
16500 0.00064834754448384
16600 0.000758272595703602
16700 0.000647765526082367
16800 0.000637753983028233
16900 0.000647423847112805
17000 0.000635228701867163
17100 0.000601404870394617
17200 0.000677939329762012
17300 0.00054673757404089
17400 0.000643368461169302
17500 0.000960465404205024
17600 0.000914510223083198
17700 0.000798596767708659
17800 0.000899054750334471
17900 0.000944278901442885
18000 0.000823545444291085
18100 0.000816305284388363
18200 0.000918672594707459
18300 0.000894757220521569
18400 0.00074328196933493
18500 0.000427554012276232
18600 0.000425680365879089
18700 0.000381495628971606
18800 0.000422847253503278
18900 0.000618425896391273
19000 0.000754104228690267
19100 0.000691882858518511
19200 0.000658879755064845
19300 0.000558453903067857
19400 0.000483610201627016
19500 0.000410616339650005
19600 0.000454437627922744
19700 0.000495489570312202
19800 0.000474725296953693
19900 0.00039100056164898
20000 0.000454251043265685
20100 0.000539151893462986
20200 0.000491074693854898
20300 0.000533568905666471
20400 0.000482579052913934
20500 0.000501829315908253
20600 0.000402029399992898
20700 0.000497362925671041
20800 0.000553784717340022
20900 0.00056632945779711
21000 0.000457447749795392
21100 0.000413399975514039
21200 0.000319141137879342
21300 0.000213207793422043
21400 0.000209681165870279
21500 0.00015886225446593
21600 0.000217026521568187
21700 0.000196351655176841
21800 0.000204271083930507
21900 0.00033478534896858
22000 0.000360459031071514
22100 0.000312898540869355
22200 0.000387599051464349
22300 0.00053043570369482
22400 0.000420639873482287
22500 0.000407185201765969
22600 0.000413133617257699
22700 0.000359763740561903
22800 0.000214058178244159
22900 0.000209174482733943
23000 0.000199343805434182
23100 0.000204406140255742
23200 0.000188332793186419
23300 0.000190216320334002
23400 0.000156619178596884
23500 0.000192214982234873
23600 0.00018151402764488
23700 0.000187232115422376
23800 0.000209861973416992
23900 0.000225410884013399
24000 0.000230131539865397
24100 0.000223372422624379
24200 0.000332126946887001
24300 0.000305177731206641
24400 0.000294091354589909
24500 0.000259699387243018
24600 0.000259437190834433
24700 0.000286652648355812
24800 0.000314114469802007
24900 0.000317341124173254
25000 0.00036693611764349
25100 0.000368760025594383
25200 0.000220467671169899
25300 0.000199212634470314
25400 0.000244484341237694
25500 0.00021056535479147
25700 0.000396066898247227
25800 0.000390372588299215
25900 0.000339239835739136
26000 0.000346142100170255
26100 0.000267718191025779
26200 0.000156583424541168
26300 0.000162845870363526
26400 0.000198672234546393
26500 0.000179781505721621
26600 0.000179737791768275
26700 0.000190955397556536
26800 0.000190287857549265
26900 0.00019343095482327
27000 0.000180405360879377
27100 0.00020456915081013
27200 0.000193427025806159
27300 0.000231665311730467
27400 0.000189806989510544
27500 0.000302638625726104
27600 0.000319669634336606
27700 0.000329424918163568
27800 0.000317996658850461
27900 0.000335532356984913
28000 0.000232237565796822
28100 0.000221059715840966
28200 0.000211709731956944
28300 0.000187315599760041
28400 0.00018349286983721
28500 0.000177127119968645
28600 0.00029471522429958
28700 0.000325785193126649
28800 0.000331360060954466
29000 0.000326237990520895
29100 0.000188702368177474
29200 0.000156901282025501
29300 0.000140358970384113
29400 0.000150014966493472
29500 0.000180075556272641
29600 0.000183941883733496
29700 0.000195874818018638
29800 0.000231788581004366
29900 0.000234236285905354
30000 0.000216243613976985
30100 0.000214308514841832
30200 0.000276237726211548
30300 0.000272303877864033
30400 0.000278999475995079
30500 0.000274385965894908
30600 0.000261789537034929
30700 0.000228383141802624
30800 0.000223344584810548
30900 0.000192362043890171
31000 0.000197325163753703
31100 0.000197583474800922
31200 0.000189286496606655
31300 0.000163763790624216
31400 0.000188893071026541
31500 0.000194666790775955
31600 0.00019869209791068
31700 0.000174850240000524
31800 0.000174480694113299
31900 0.00020327368110884
32000 0.000206973098102026
32100 0.000201282848138362
32200 0.000204255164135247
32300 0.000216446351259947
32400 0.000175732391653582
32500 0.000167880454682745
32600 0.000247222167672589
32700 0.00024771096650511
};

==> supp_mat/ant_plots/relerr_data.tex <==
\definecolor{color0}{rgb}{1,0,1}
\path [fill=red, fill opacity=0.4,  ultra thick]
(axis cs:0.00499999988824129,0.0617737024119071)
--(axis cs:0.00499999988824129,0.0386343948381383)
--(axis cs:0.00999999977648258,0.0434856207657638)
--(axis cs:0.0149999996647239,0.0463247035673804)
--(axis cs:0.0199999995529652,0.0483650593141228)
--(axis cs:0.0249999994412065,0.0509652786796855)
--(axis cs:0.0299999993294477,0.0536652293125487)
--(axis cs:0.034999999217689,0.0561495114432288)
--(axis cs:0.0399999991059303,0.058535377160746)
--(axis cs:0.0449999989941716,0.0610025846955451)
--(axis cs:0.0499999988824129,0.0635675110653366)
--(axis cs:0.0549999987706542,0.0665719148415199)
--(axis cs:0.0599999986588955,0.0698230935670337)
--(axis cs:0.0649999985471368,0.0732127145130467)
--(axis cs:0.0699999984353781,0.076680764546631)
--(axis cs:0.0749999983236194,0.0800904369206006)
--(axis cs:0.0799999982118607,0.0834235957376939)
--(axis cs:0.0849999981001019,0.0866837948061991)
--(axis cs:0.0899999979883432,0.089940591470908)
--(axis cs:0.0949999978765845,0.0931625304480455)
--(axis cs:0.0999999977648258,0.0962032163588315)
--(axis cs:0.104999997653067,0.0993481992331271)
--(axis cs:0.109999997541308,0.102521379160813)
--(axis cs:0.11499999742955,0.105750852706632)
--(axis cs:0.119999997317791,0.109154367255317)
--(axis cs:0.124999997206032,0.112455173575764)
--(axis cs:0.129999997094274,0.115680917960176)
--(axis cs:0.134999996982515,0.11879441987693)
--(axis cs:0.139999996870756,0.121880881352344)
--(axis cs:0.144999996758997,0.124928204258747)
--(axis cs:0.149999996647239,0.127815518654646)
--(axis cs:0.15499999653548,0.130746953564645)
--(axis cs:0.159999996423721,0.133683888885195)
--(axis cs:0.164999996311963,0.136725370464057)
--(axis cs:0.169999996200204,0.139704476771666)
--(axis cs:0.174999996088445,0.142634763072111)
--(axis cs:0.179999995976686,0.145612147148451)
--(axis cs:0.184999995864928,0.148613778909054)
--(axis cs:0.189999995753169,0.151667725143722)
--(axis cs:0.19499999564141,0.154697313221166)
--(axis cs:0.199999995529652,0.157727027943181)
--(axis cs:0.204999995417893,0.160837235878736)
--(axis cs:0.209999995306134,0.163992122047044)
--(axis cs:0.214999995194376,0.167163613710579)
--(axis cs:0.219999995082617,0.170331076686798)
--(axis cs:0.224999994970858,0.173487800842013)
--(axis cs:0.229999994859099,0.176598341135)
--(axis cs:0.234999994747341,0.179626697633671)
--(axis cs:0.239999994635582,0.182591762963903)
--(axis cs:0.244999994523823,0.185502413489075)
--(axis cs:0.249999994412065,0.188356368506812)
--(axis cs:0.254999994300306,0.191194093350703)
--(axis cs:0.259999994188547,0.194027163271051)
--(axis cs:0.264999994076788,0.196791517211386)
--(axis cs:0.26999999396503,0.199505612598924)
--(axis cs:0.274999993853271,0.202157454431177)
--(axis cs:0.279999993741512,0.204760496561805)
--(axis cs:0.284999993629754,0.207312187808541)
--(axis cs:0.289999993517995,0.209760562399368)
--(axis cs:0.294999993406236,0.212144281082337)
--(axis cs:0.299999993294477,0.214497965567802)
--(axis cs:0.304999993182719,0.216870592968355)
--(axis cs:0.30999999307096,0.219252206614288)
--(axis cs:0.314999992959201,0.22162877843153)
--(axis cs:0.319999992847443,0.223979421489878)
--(axis cs:0.324999992735684,0.226307329827411)
--(axis cs:0.329999992623925,0.228614073395211)
--(axis cs:0.334999992512167,0.230875507534009)
--(axis cs:0.339999992400408,0.233131432749064)
--(axis cs:0.344999992288649,0.235372241343874)
--(axis cs:0.34999999217689,0.23761306000617)
--(axis cs:0.354999992065132,0.239900876972689)
--(axis cs:0.359999991953373,0.242216654237543)
--(axis cs:0.364999991841614,0.244564104473976)
--(axis cs:0.369999991729856,0.246932185041045)
--(axis cs:0.374999991618097,0.249304866490773)
--(axis cs:0.379999991506338,0.251654928110541)
--(axis cs:0.384999991394579,0.253985321218264)
--(axis cs:0.389999991282821,0.256253958112631)
--(axis cs:0.394999991171062,0.258485104298181)
--(axis cs:0.399999991059303,0.260695329009603)
--(axis cs:0.404999990947545,0.262907503413708)
--(axis cs:0.409999990835786,0.265113153140197)
--(axis cs:0.414999990724027,0.267313161258866)
--(axis cs:0.419999990612268,0.269495441318637)
--(axis cs:0.42499999050051,0.271639667740179)
--(axis cs:0.429999990388751,0.273736487343934)
--(axis cs:0.434999990276992,0.275785266992054)
--(axis cs:0.439999990165234,0.277796004009495)
--(axis cs:0.444999990053475,0.279770320078415)
--(axis cs:0.449999989941716,0.281718656846005)
--(axis cs:0.454999989829957,0.283686162439016)
--(axis cs:0.459999989718199,0.285664972824884)
--(axis cs:0.46499998960644,0.287660604024833)
--(axis cs:0.469999989494681,0.289655464443203)
--(axis cs:0.474999989382923,0.291645637668573)
--(axis cs:0.479999989271164,0.293638358205003)
--(axis cs:0.484999989159405,0.295605637606631)
--(axis cs:0.489999989047647,0.297555858444109)
--(axis cs:0.494999988935888,0.299483923885149)
--(axis cs:0.494999988935888,0.408135160747947)
--(axis cs:0.494999988935888,0.408135160747947)
--(axis cs:0.489999989047647,0.405369042214569)
--(axis cs:0.484999989159405,0.402580725792929)
--(axis cs:0.479999989271164,0.399767822106885)
--(axis cs:0.474999989382923,0.396927612244019)
--(axis cs:0.469999989494681,0.394054616752303)
--(axis cs:0.46499998960644,0.391155664016548)
--(axis cs:0.459999989718199,0.388227007698378)
--(axis cs:0.454999989829957,0.385282526471884)
--(axis cs:0.449999989941716,0.382313588749918)
--(axis cs:0.444999990053475,0.379328779761815)
--(axis cs:0.439999990165234,0.376296363963699)
--(axis cs:0.434999990276992,0.373211402072198)
--(axis cs:0.429999990388751,0.37008026503015)
--(axis cs:0.42499999050051,0.366901282428642)
--(axis cs:0.419999990612268,0.363679152027521)
--(axis cs:0.414999990724027,0.360412776408477)
--(axis cs:0.409999990835786,0.357115247647278)
--(axis cs:0.404999990947545,0.353808833669216)
--(axis cs:0.399999991059303,0.350475735441222)
--(axis cs:0.394999991171062,0.347127429543626)
--(axis cs:0.389999991282821,0.343748637587943)
--(axis cs:0.384999991394579,0.340326799113755)
--(axis cs:0.379999991506338,0.336855353776043)
--(axis cs:0.374999991618097,0.333345773330427)
--(axis cs:0.369999991729856,0.329796675159466)
--(axis cs:0.364999991841614,0.32621781293793)
--(axis cs:0.359999991953373,0.322623901710979)
--(axis cs:0.354999992065132,0.319022585571172)
--(axis cs:0.34999999217689,0.315422751501785)
--(axis cs:0.344999992288649,0.311823616943571)
--(axis cs:0.339999992400408,0.308203871221326)
--(axis cs:0.334999992512167,0.304550892983541)
--(axis cs:0.329999992623925,0.300874427517793)
--(axis cs:0.324999992735684,0.297160520863679)
--(axis cs:0.319999992847443,0.293418198410825)
--(axis cs:0.314999992959201,0.289652175612808)
--(axis cs:0.30999999307096,0.285869247623621)
--(axis cs:0.304999993182719,0.282072047848234)
--(axis cs:0.299999993294477,0.278272815312022)
--(axis cs:0.294999993406236,0.274490231155299)
--(axis cs:0.289999993517995,0.270696193526931)
--(axis cs:0.284999993629754,0.26685631059534)
--(axis cs:0.279999993741512,0.262956843193831)
--(axis cs:0.274999993853271,0.258990901067306)
--(axis cs:0.26999999396503,0.254988593191714)
--(axis cs:0.264999994076788,0.250935364804135)
--(axis cs:0.259999994188547,0.246868080013771)
--(axis cs:0.254999994300306,0.24278172328789)
--(axis cs:0.249999994412065,0.238748962275888)
--(axis cs:0.244999994523823,0.234782046252347)
--(axis cs:0.239999994635582,0.230828023930697)
--(axis cs:0.234999994747341,0.226832639605465)
--(axis cs:0.229999994859099,0.22282753503284)
--(axis cs:0.224999994970858,0.218784380931633)
--(axis cs:0.219999995082617,0.214760584794117)
--(axis cs:0.214999995194376,0.210748773835704)
--(axis cs:0.209999995306134,0.206782368296719)
--(axis cs:0.204999995417893,0.202840543418733)
--(axis cs:0.199999995529652,0.198956018994436)
--(axis cs:0.19499999564141,0.195129973041087)
--(axis cs:0.189999995753169,0.191249444220504)
--(axis cs:0.184999995864928,0.187379394516117)
--(axis cs:0.179999995976686,0.183443380573956)
--(axis cs:0.174999996088445,0.179458475141181)
--(axis cs:0.169999996200204,0.175471499178514)
--(axis cs:0.164999996311963,0.171514805637874)
--(axis cs:0.159999996423721,0.167457562590159)
--(axis cs:0.15499999653548,0.163285026064156)
--(axis cs:0.149999996647239,0.159100525229166)
--(axis cs:0.144999996758997,0.154865081775968)
--(axis cs:0.139999996870756,0.150765180477677)
--(axis cs:0.134999996982515,0.146553456721385)
--(axis cs:0.129999997094274,0.142299380791709)
--(axis cs:0.124999997206032,0.13805956250568)
--(axis cs:0.119999997317791,0.133775760955203)
--(axis cs:0.11499999742955,0.129580956417735)
--(axis cs:0.109999997541308,0.125507261120458)
--(axis cs:0.104999997653067,0.121623126423221)
--(axis cs:0.0999999977648258,0.117867286760317)
--(axis cs:0.0949999978765845,0.114319856905295)
--(axis cs:0.0899999979883432,0.110769735975372)
--(axis cs:0.0849999981001019,0.107094243317592)
--(axis cs:0.0799999982118607,0.103440520031469)
--(axis cs:0.0749999983236194,0.0996080159229109)
--(axis cs:0.0699999984353781,0.0955980278974687)
--(axis cs:0.0649999985471368,0.0914758897416644)
--(axis cs:0.0599999986588955,0.0874558046686462)
--(axis cs:0.0549999987706542,0.0836088886616326)
--(axis cs:0.0499999988824129,0.0798962558828157)
--(axis cs:0.0449999989941716,0.0768822693034747)
--(axis cs:0.0399999991059303,0.0738924092412926)
--(axis cs:0.034999999217689,0.07111532128823)
--(axis cs:0.0299999993294477,0.0684187050106929)
--(axis cs:0.0249999994412065,0.0660313064522116)
--(axis cs:0.0199999995529652,0.0642612245318483)
--(axis cs:0.0149999996647239,0.0634354685896186)
--(axis cs:0.00999999977648258,0.0623114930311117)
--(axis cs:0.00499999988824129,0.0617737024119071)
--cycle;

\path [fill=blue, fill opacity=0.4,  ultra thick]
(axis cs:0.00499999988824129,0.0526193747049425)
--(axis cs:0.00499999988824129,0.0310973366713826)
--(axis cs:0.00999999977648258,0.0339492388112239)
--(axis cs:0.0149999996647239,0.036182282210723)
--(axis cs:0.0199999995529652,0.0378708938442561)
--(axis cs:0.0249999994412065,0.0395553478803725)
--(axis cs:0.0299999993294477,0.0409821504749312)
--(axis cs:0.034999999217689,0.0420611044872087)
--(axis cs:0.0399999991059303,0.0430092866668241)
--(axis cs:0.0449999989941716,0.0438696391735633)
--(axis cs:0.0499999988824129,0.0447943276652075)
--(axis cs:0.0549999987706542,0.0463075343712091)
--(axis cs:0.0599999986588955,0.0479935775812441)
--(axis cs:0.0649999985471368,0.0495751145144116)
--(axis cs:0.0699999984353781,0.0510763826441422)
--(axis cs:0.0749999983236194,0.0525536917157409)
--(axis cs:0.0799999982118607,0.0539424922309172)
--(axis cs:0.0849999981001019,0.0552895390207408)
--(axis cs:0.0899999979883432,0.0566554297432967)
--(axis cs:0.0949999978765845,0.0580229686885128)
--(axis cs:0.0999999977648258,0.0592947218005902)
--(axis cs:0.104999997653067,0.0606940577883012)
--(axis cs:0.109999997541308,0.0622356895312977)
--(axis cs:0.11499999742955,0.0639031110720842)
--(axis cs:0.119999997317791,0.0656740016070529)
--(axis cs:0.124999997206032,0.0671947153876068)
--(axis cs:0.129999997094274,0.0685690750852565)
--(axis cs:0.134999996982515,0.0698822555322579)
--(axis cs:0.139999996870756,0.0711097157497876)
--(axis cs:0.144999996758997,0.0723332816186881)
--(axis cs:0.149999996647239,0.0735066421822264)
--(axis cs:0.15499999653548,0.074832115004375)
--(axis cs:0.159999996423721,0.076173921511128)
--(axis cs:0.164999996311963,0.0776076806157524)
--(axis cs:0.169999996200204,0.0789867735193033)
--(axis cs:0.174999996088445,0.0802641055798187)
--(axis cs:0.179999995976686,0.0815566095666901)
--(axis cs:0.184999995864928,0.0827883947631297)
--(axis cs:0.189999995753169,0.0840688545702352)
--(axis cs:0.19499999564141,0.0852647506427675)
--(axis cs:0.199999995529652,0.0864509093500647)
--(axis cs:0.204999995417893,0.0877176448169466)
--(axis cs:0.209999995306134,0.0890721152511092)
--(axis cs:0.214999995194376,0.0903466159649498)
--(axis cs:0.219999995082617,0.0915216724221831)
--(axis cs:0.224999994970858,0.0926829123816157)
--(axis cs:0.229999994859099,0.0937087048819056)
--(axis cs:0.234999994747341,0.0946243086274077)
--(axis cs:0.239999994635582,0.0955138119607365)
--(axis cs:0.244999994523823,0.0963623462078922)
--(axis cs:0.249999994412065,0.097205161903519)
--(axis cs:0.254999994300306,0.098167702117953)
--(axis cs:0.259999994188547,0.0991108052454358)
--(axis cs:0.264999994076788,0.100045599293028)
--(axis cs:0.26999999396503,0.100993030857953)
--(axis cs:0.274999993853271,0.101960342895151)
--(axis cs:0.279999993741512,0.102946876685298)
--(axis cs:0.284999993629754,0.103946213609579)
--(axis cs:0.289999993517995,0.104931476148878)
--(axis cs:0.294999993406236,0.105882751696443)
--(axis cs:0.299999993294477,0.106776154327792)
--(axis cs:0.304999993182719,0.10767995318944)
--(axis cs:0.30999999307096,0.108645371427002)
--(axis cs:0.314999992959201,0.109656538683485)
--(axis cs:0.319999992847443,0.110597947170229)
--(axis cs:0.324999992735684,0.111540748833862)
--(axis cs:0.329999992623925,0.112407271093308)
--(axis cs:0.334999992512167,0.113236775055168)
--(axis cs:0.339999992400408,0.114007588920844)
--(axis cs:0.344999992288649,0.114735683059254)
--(axis cs:0.34999999217689,0.115470836212098)
--(axis cs:0.354999992065132,0.116276561662788)
--(axis cs:0.359999991953373,0.117048968160027)
--(axis cs:0.364999991841614,0.117836627165853)
--(axis cs:0.369999991729856,0.118613955889304)
--(axis cs:0.374999991618097,0.119326063757596)
--(axis cs:0.379999991506338,0.120026098974325)
--(axis cs:0.384999991394579,0.120684931117701)
--(axis cs:0.389999991282821,0.121344568162132)
--(axis cs:0.394999991171062,0.122043581189101)
--(axis cs:0.399999991059303,0.122716147244609)
--(axis cs:0.404999990947545,0.12343668959545)
--(axis cs:0.409999990835786,0.124179273216774)
--(axis cs:0.414999990724027,0.12493236773218)
--(axis cs:0.419999990612268,0.12573354097861)
--(axis cs:0.42499999050051,0.12653462587288)
--(axis cs:0.429999990388751,0.127288594811515)
--(axis cs:0.434999990276992,0.127995924978395)
--(axis cs:0.439999990165234,0.12867379603478)
--(axis cs:0.444999990053475,0.129328644296242)
--(axis cs:0.449999989941716,0.12993847428416)
--(axis cs:0.454999989829957,0.13053959851337)
--(axis cs:0.459999989718199,0.131166682794783)
--(axis cs:0.46499998960644,0.131820245165412)
--(axis cs:0.469999989494681,0.132454259856872)
--(axis cs:0.474999989382923,0.133123760022589)
--(axis cs:0.479999989271164,0.133748244080939)
--(axis cs:0.484999989159405,0.134347003271289)
--(axis cs:0.489999989047647,0.134946389251444)
--(axis cs:0.494999988935888,0.135532023953662)
--(axis cs:0.494999988935888,0.167496070424621)
--(axis cs:0.494999988935888,0.167496070424621)
--(axis cs:0.489999989047647,0.166873144861811)
--(axis cs:0.484999989159405,0.166253794509155)
--(axis cs:0.479999989271164,0.165597258170229)
--(axis cs:0.474999989382923,0.164954904839348)
--(axis cs:0.469999989494681,0.164295091429391)
--(axis cs:0.46499998960644,0.163621521697818)
--(axis cs:0.459999989718199,0.162919507847973)
--(axis cs:0.454999989829957,0.162219495634211)
--(axis cs:0.449999989941716,0.161493626384821)
--(axis cs:0.444999990053475,0.160769759119758)
--(axis cs:0.439999990165234,0.159985048955667)
--(axis cs:0.434999990276992,0.159176133575992)
--(axis cs:0.429999990388751,0.158361541846624)
--(axis cs:0.42499999050051,0.157520352560398)
--(axis cs:0.419999990612268,0.156669262945409)
--(axis cs:0.414999990724027,0.155861830147043)
--(axis cs:0.409999990835786,0.155038454912463)
--(axis cs:0.404999990947545,0.154192686154111)
--(axis cs:0.399999991059303,0.153418123095931)
--(axis cs:0.394999991171062,0.15270080498109)
--(axis cs:0.389999991282821,0.151949479348727)
--(axis cs:0.384999991394579,0.151136856566913)
--(axis cs:0.379999991506338,0.150264577956322)
--(axis cs:0.374999991618097,0.149311625814905)
--(axis cs:0.369999991729856,0.148318577775514)
--(axis cs:0.364999991841614,0.147311148653342)
--(axis cs:0.359999991953373,0.146304868082512)
--(axis cs:0.354999992065132,0.145324139587999)
--(axis cs:0.34999999217689,0.144329109954611)
--(axis cs:0.344999992288649,0.143339092556295)
--(axis cs:0.339999992400408,0.142345967791997)
--(axis cs:0.334999992512167,0.141331059905095)
--(axis cs:0.329999992623925,0.140272598125789)
--(axis cs:0.324999992735684,0.139220262718108)
--(axis cs:0.319999992847443,0.138121816661019)
--(axis cs:0.314999992959201,0.137003134375263)
--(axis cs:0.30999999307096,0.135874096683733)
--(axis cs:0.304999993182719,0.134796567201425)
--(axis cs:0.299999993294477,0.133771334562128)
--(axis cs:0.294999993406236,0.132795954446777)
--(axis cs:0.289999993517995,0.131779299924796)
--(axis cs:0.284999993629754,0.130781204442719)
--(axis cs:0.279999993741512,0.129748898463453)
--(axis cs:0.274999993853271,0.12869058438574)
--(axis cs:0.26999999396503,0.127570639602731)
--(axis cs:0.264999994076788,0.126445620228606)
--(axis cs:0.259999994188547,0.125329375140858)
--(axis cs:0.254999994300306,0.124228153464618)
--(axis cs:0.249999994412065,0.123136486183295)
--(axis cs:0.244999994523823,0.122107568015815)
--(axis cs:0.239999994635582,0.120990747080327)
--(axis cs:0.234999994747341,0.119891474725174)
--(axis cs:0.229999994859099,0.118768313637374)
--(axis cs:0.224999994970858,0.117566369338194)
--(axis cs:0.219999995082617,0.116341288685958)
--(axis cs:0.214999995194376,0.11501226435194)
--(axis cs:0.209999995306134,0.113690985060218)
--(axis cs:0.204999995417893,0.112461546008359)
--(axis cs:0.199999995529652,0.111220562275862)
--(axis cs:0.19499999564141,0.110029055283486)
--(axis cs:0.189999995753169,0.108791743013446)
--(axis cs:0.184999995864928,0.107467401857521)
--(axis cs:0.179999995976686,0.106027363849677)
--(axis cs:0.174999996088445,0.104396923394695)
--(axis cs:0.169999996200204,0.102532172632396)
--(axis cs:0.164999996311963,0.100615196223398)
--(axis cs:0.159999996423721,0.0986506384006741)
--(axis cs:0.15499999653548,0.0967804139929879)
--(axis cs:0.149999996647239,0.0949894214875905)
--(axis cs:0.144999996758997,0.0933082609950248)
--(axis cs:0.139999996870756,0.0918129291697952)
--(axis cs:0.134999996982515,0.0902305593588103)
--(axis cs:0.129999997094274,0.0885499242213941)
--(axis cs:0.124999997206032,0.0868354141314124)
--(axis cs:0.119999997317791,0.0850264685847652)
--(axis cs:0.11499999742955,0.0831249816389768)
--(axis cs:0.109999997541308,0.0811149623599219)
--(axis cs:0.104999997653067,0.0792845172555406)
--(axis cs:0.0999999977648258,0.0774500863596918)
--(axis cs:0.0949999978765845,0.0758083575577113)
--(axis cs:0.0899999979883432,0.0742380784036295)
--(axis cs:0.0849999981001019,0.0725960938504832)
--(axis cs:0.0799999982118607,0.0710435112617033)
--(axis cs:0.0749999983236194,0.069493944170823)
--(axis cs:0.0699999984353781,0.0679143732262967)
--(axis cs:0.0649999985471368,0.0662368304096269)
--(axis cs:0.0599999986588955,0.0646117180954672)
--(axis cs:0.0549999987706542,0.0629639464924578)
--(axis cs:0.0499999988824129,0.0614569718319637)
--(axis cs:0.0449999989941716,0.0604139589879028)
--(axis cs:0.0399999991059303,0.0593118746647139)
--(axis cs:0.034999999217689,0.0582805771435086)
--(axis cs:0.0299999993294477,0.0571039648423289)
--(axis cs:0.0249999994412065,0.0557440388530259)
--(axis cs:0.0199999995529652,0.0544130556218963)
--(axis cs:0.0149999996647239,0.0533854634776379)
--(axis cs:0.00999999977648258,0.0520667731047234)
--(axis cs:0.00499999988824129,0.0526193747049425)
--cycle;

\path [fill=green!50.1960784313725!black, fill opacity=0.4,  ultra thick]
(axis cs:0.00499999988824129,0.052718895552199)
--(axis cs:0.00499999988824129,0.0377331078152753)
--(axis cs:0.00999999977648258,0.0369656955212091)
--(axis cs:0.0149999996647239,0.0367581605636091)
--(axis cs:0.0199999995529652,0.0363011407317183)
--(axis cs:0.0249999994412065,0.0362236410377981)
--(axis cs:0.0299999993294477,0.0363950467741389)
--(axis cs:0.034999999217689,0.0365557089784092)
--(axis cs:0.0399999991059303,0.0367473719703522)
--(axis cs:0.0449999989941716,0.0370568317801841)
--(axis cs:0.0499999988824129,0.0373554066862359)
--(axis cs:0.0549999987706542,0.0381665723548695)
--(axis cs:0.0599999986588955,0.0390330240550067)
--(axis cs:0.0649999985471368,0.0399709037257261)
--(axis cs:0.0699999984353781,0.0410048164676835)
--(axis cs:0.0749999983236194,0.0420630589974076)
--(axis cs:0.0799999982118607,0.0432134828740296)
--(axis cs:0.0849999981001019,0.0444814106225752)
--(axis cs:0.0899999979883432,0.0459260373583237)
--(axis cs:0.0949999978765845,0.0473792116667108)
--(axis cs:0.0999999977648258,0.0484944313749903)
--(axis cs:0.104999997653067,0.0496640955058358)
--(axis cs:0.109999997541308,0.0509131824311269)
--(axis cs:0.11499999742955,0.0524747382207274)
--(axis cs:0.119999997317791,0.0539887758582393)
--(axis cs:0.124999997206032,0.0551941803139558)
--(axis cs:0.129999997094274,0.0561614460488332)
--(axis cs:0.134999996982515,0.0571562939019801)
--(axis cs:0.139999996870756,0.0581391504571925)
--(axis cs:0.144999996758997,0.059098714430652)
--(axis cs:0.149999996647239,0.0599811510417191)
--(axis cs:0.15499999653548,0.0609624217915652)
--(axis cs:0.159999996423721,0.0619952991765535)
--(axis cs:0.164999996311963,0.062986608996049)
--(axis cs:0.169999996200204,0.0640307493826392)
--(axis cs:0.174999996088445,0.0651888180223052)
--(axis cs:0.179999995976686,0.0663206369687)
--(axis cs:0.184999995864928,0.0673486207255038)
--(axis cs:0.189999995753169,0.0683345594855995)
--(axis cs:0.19499999564141,0.0691847302691938)
--(axis cs:0.199999995529652,0.0700243952077905)
--(axis cs:0.204999995417893,0.0709218646062806)
--(axis cs:0.209999995306134,0.0719295638585678)
--(axis cs:0.214999995194376,0.0729450742124562)
--(axis cs:0.219999995082617,0.0738575444656645)
--(axis cs:0.224999994970858,0.0747523619969923)
--(axis cs:0.229999994859099,0.0755023268230594)
--(axis cs:0.234999994747341,0.0762129826714816)
--(axis cs:0.239999994635582,0.0769105276482941)
--(axis cs:0.244999994523823,0.0776421109116743)
--(axis cs:0.249999994412065,0.0783477385630158)
--(axis cs:0.254999994300306,0.0791386514355303)
--(axis cs:0.259999994188547,0.0799236014679012)
--(axis cs:0.264999994076788,0.0807115036630291)
--(axis cs:0.26999999396503,0.0814604619679292)
--(axis cs:0.274999993853271,0.082230661580531)
--(axis cs:0.279999993741512,0.0829894577803765)
--(axis cs:0.284999993629754,0.0837593069924075)
--(axis cs:0.289999993517995,0.0846107964400881)
--(axis cs:0.294999993406236,0.0854144203639712)
--(axis cs:0.299999993294477,0.0862115832589468)
--(axis cs:0.304999993182719,0.0869860366988914)
--(axis cs:0.30999999307096,0.0878014362159858)
--(axis cs:0.314999992959201,0.0886041094560014)
--(axis cs:0.319999992847443,0.0893727819246501)
--(axis cs:0.324999992735684,0.0901561198227204)
--(axis cs:0.329999992623925,0.0909157993417313)
--(axis cs:0.334999992512167,0.0916533207996425)
--(axis cs:0.339999992400408,0.0923861682771991)
--(axis cs:0.344999992288649,0.0931119228350846)
--(axis cs:0.34999999217689,0.0938433622911745)
--(axis cs:0.354999992065132,0.0945798232893806)
--(axis cs:0.359999991953373,0.0953093613111109)
--(axis cs:0.364999991841614,0.0960005413085186)
--(axis cs:0.369999991729856,0.0966686306340884)
--(axis cs:0.374999991618097,0.0972949034634671)
--(axis cs:0.379999991506338,0.0979190047588376)
--(axis cs:0.384999991394579,0.0984921117827667)
--(axis cs:0.389999991282821,0.0990745993589496)
--(axis cs:0.394999991171062,0.0997007916945693)
--(axis cs:0.399999991059303,0.100283817880949)
--(axis cs:0.404999990947545,0.100887579139203)
--(axis cs:0.409999990835786,0.101506920335366)
--(axis cs:0.414999990724027,0.102141146196819)
--(axis cs:0.419999990612268,0.102782803899474)
--(axis cs:0.42499999050051,0.103448780108315)
--(axis cs:0.429999990388751,0.104122169924533)
--(axis cs:0.434999990276992,0.104773581867073)
--(axis cs:0.439999990165234,0.105398618483843)
--(axis cs:0.444999990053475,0.106010233220647)
--(axis cs:0.449999989941716,0.106550712868891)
--(axis cs:0.454999989829957,0.107085180387914)
--(axis cs:0.459999989718199,0.10763942678576)
--(axis cs:0.46499998960644,0.108198610777833)
--(axis cs:0.469999989494681,0.108774209822492)
--(axis cs:0.474999989382923,0.1093523200086)
--(axis cs:0.479999989271164,0.109919136160841)
--(axis cs:0.484999989159405,0.110453349926482)
--(axis cs:0.489999989047647,0.110959304015686)
--(axis cs:0.494999988935888,0.111470364318783)
--(axis cs:0.494999988935888,0.147809566878869)
--(axis cs:0.494999988935888,0.147809566878869)
--(axis cs:0.489999989047647,0.147165265913493)
--(axis cs:0.484999989159405,0.146518818170214)
--(axis cs:0.479999989271164,0.145868780126404)
--(axis cs:0.474999989382923,0.145188094793641)
--(axis cs:0.469999989494681,0.144460289159731)
--(axis cs:0.46499998960644,0.143675688247728)
--(axis cs:0.459999989718199,0.142851963461976)
--(axis cs:0.454999989829957,0.142031552357311)
--(axis cs:0.449999989941716,0.141223939323968)
--(axis cs:0.444999990053475,0.140449464608545)
--(axis cs:0.439999990165234,0.13962768669614)
--(axis cs:0.434999990276992,0.138807703592882)
--(axis cs:0.429999990388751,0.137946951326558)
--(axis cs:0.42499999050051,0.137030893720138)
--(axis cs:0.419999990612268,0.136070525652991)
--(axis cs:0.414999990724027,0.135122451857107)
--(axis cs:0.409999990835786,0.134162330554011)
--(axis cs:0.404999990947545,0.133229624358181)
--(axis cs:0.399999991059303,0.13235807260697)
--(axis cs:0.394999991171062,0.131532722510922)
--(axis cs:0.389999991282821,0.130685748588355)
--(axis cs:0.384999991394579,0.129764780508276)
--(axis cs:0.379999991506338,0.128806269175385)
--(axis cs:0.374999991618097,0.12778659584532)
--(axis cs:0.369999991729856,0.126736550375306)
--(axis cs:0.364999991841614,0.125660829455246)
--(axis cs:0.359999991953373,0.124588700971975)
--(axis cs:0.354999992065132,0.12353283668363)
--(axis cs:0.34999999217689,0.122471110528298)
--(axis cs:0.344999992288649,0.121399431281553)
--(axis cs:0.339999992400408,0.120298312542103)
--(axis cs:0.334999992512167,0.119176292546403)
--(axis cs:0.329999992623925,0.117990962741968)
--(axis cs:0.324999992735684,0.116758310209857)
--(axis cs:0.319999992847443,0.115507821880799)
--(axis cs:0.314999992959201,0.114270064064592)
--(axis cs:0.30999999307096,0.11304498690947)
--(axis cs:0.304999993182719,0.111809875519869)
--(axis cs:0.299999993294477,0.110642218764999)
--(axis cs:0.294999993406236,0.109574293173152)
--(axis cs:0.289999993517995,0.10850416055787)
--(axis cs:0.284999993629754,0.107445518601871)
--(axis cs:0.279999993741512,0.106337871462761)
--(axis cs:0.274999993853271,0.105210647221294)
--(axis cs:0.26999999396503,0.104126107316572)
--(axis cs:0.264999994076788,0.103026012673143)
--(axis cs:0.259999994188547,0.101909588738177)
--(axis cs:0.254999994300306,0.100775997795416)
--(axis cs:0.249999994412065,0.0996663047092603)
--(axis cs:0.244999994523823,0.0986338356557137)
--(axis cs:0.239999994635582,0.0975854516523093)
--(axis cs:0.234999994747341,0.0965874718418276)
--(axis cs:0.229999994859099,0.0955940564533365)
--(axis cs:0.224999994970858,0.0945267706247652)
--(axis cs:0.219999995082617,0.0933342863038472)
--(axis cs:0.214999995194376,0.0919979607567778)
--(axis cs:0.209999995306134,0.0907085850865772)
--(axis cs:0.204999995417893,0.0895458657716199)
--(axis cs:0.199999995529652,0.0884529784050906)
--(axis cs:0.19499999564141,0.0875097844299693)
--(axis cs:0.189999995753169,0.0865001331389798)
--(axis cs:0.184999995864928,0.0855113476946768)
--(axis cs:0.179999995976686,0.08441281374417)
--(axis cs:0.174999996088445,0.0832286309549483)
--(axis cs:0.169999996200204,0.0819301930641628)
--(axis cs:0.164999996311963,0.0806187077937302)
--(axis cs:0.159999996423721,0.0791820131384782)
--(axis cs:0.15499999653548,0.0778585177756963)
--(axis cs:0.149999996647239,0.0766918199212264)
--(axis cs:0.144999996758997,0.0755892440566562)
--(axis cs:0.139999996870756,0.0745777957379875)
--(axis cs:0.134999996982515,0.0735458667462993)
--(axis cs:0.129999997094274,0.0724576792130986)
--(axis cs:0.124999997206032,0.0714019036579891)
--(axis cs:0.119999997317791,0.070263986664306)
--(axis cs:0.11499999742955,0.0689995628219258)
--(axis cs:0.109999997541308,0.067667972004064)
--(axis cs:0.104999997653067,0.0664501397723544)
--(axis cs:0.0999999977648258,0.0652512157870276)
--(axis cs:0.0949999978765845,0.06425612001939)
--(axis cs:0.0899999979883432,0.0633739197377898)
--(axis cs:0.0849999981001019,0.0624519027335414)
--(axis cs:0.0799999982118607,0.0614485825723696)
--(axis cs:0.0749999983236194,0.0603248034365794)
--(axis cs:0.0699999984353781,0.0591008589157261)
--(axis cs:0.0649999985471368,0.0577349849541557)
--(axis cs:0.0599999986588955,0.0562794801426207)
--(axis cs:0.0549999987706542,0.0546483568531742)
--(axis cs:0.0499999988824129,0.0533165731197414)
--(axis cs:0.0449999989941716,0.0523996838979065)
--(axis cs:0.0399999991059303,0.0514783454370624)
--(axis cs:0.034999999217689,0.0506797539062065)
--(axis cs:0.0299999993294477,0.0499572190541666)
--(axis cs:0.0249999994412065,0.0492345243909933)
--(axis cs:0.0199999995529652,0.0488979719733486)
--(axis cs:0.0149999996647239,0.0488972698092922)
--(axis cs:0.00999999977648258,0.0493381801100289)
--(axis cs:0.00499999988824129,0.052718895552199)
--cycle;

\path [fill=color0, fill opacity=0.4,  ultra thick]
(axis cs:0.00499999988824129,0.0595510930340604)
--(axis cs:0.00499999988824129,0.0300202818007593)
--(axis cs:0.00999999977648258,0.0310168134931776)
--(axis cs:0.0149999996647239,0.0329953006419044)
--(axis cs:0.0199999995529652,0.0343035552914914)
--(axis cs:0.0249999994412065,0.035346875079192)
--(axis cs:0.0299999993294477,0.0362126929654623)
--(axis cs:0.034999999217689,0.0368225076933057)
--(axis cs:0.0399999991059303,0.0373999538996123)
--(axis cs:0.0449999989941716,0.0381428186906952)
--(axis cs:0.0499999988824129,0.038841351064881)
--(axis cs:0.0549999987706542,0.0399976245716592)
--(axis cs:0.0599999986588955,0.041243926362405)
--(axis cs:0.0649999985471368,0.0424949551236544)
--(axis cs:0.0699999984353781,0.0437978503609495)
--(axis cs:0.0749999983236194,0.0450259321669842)
--(axis cs:0.0799999982118607,0.0462072083624832)
--(axis cs:0.0849999981001019,0.0475949732550756)
--(axis cs:0.0899999979883432,0.0490447419366174)
--(axis cs:0.0949999978765845,0.0505394730013672)
--(axis cs:0.0999999977648258,0.0517392540918245)
--(axis cs:0.104999997653067,0.052949619942706)
--(axis cs:0.109999997541308,0.0543062293735136)
--(axis cs:0.11499999742955,0.0557246681590736)
--(axis cs:0.119999997317791,0.0571474673361895)
--(axis cs:0.124999997206032,0.0582820606220017)
--(axis cs:0.129999997094274,0.059361009467796)
--(axis cs:0.134999996982515,0.0603535019222607)
--(axis cs:0.139999996870756,0.0613254736787152)
--(axis cs:0.144999996758997,0.0621789648783962)
--(axis cs:0.149999996647239,0.063035138897664)
--(axis cs:0.15499999653548,0.0640705591137776)
--(axis cs:0.159999996423721,0.0651504613520995)
--(axis cs:0.164999996311963,0.0662206147004865)
--(axis cs:0.169999996200204,0.0672489282077532)
--(axis cs:0.174999996088445,0.0683143899887879)
--(axis cs:0.179999995976686,0.0693223428340648)
--(axis cs:0.184999995864928,0.0702427003469219)
--(axis cs:0.189999995753169,0.0711543658968916)
--(axis cs:0.19499999564141,0.0720255010310316)
--(axis cs:0.199999995529652,0.0728490582526284)
--(axis cs:0.204999995417893,0.0737247717856738)
--(axis cs:0.209999995306134,0.0747804473136059)
--(axis cs:0.214999995194376,0.0758655687036733)
--(axis cs:0.219999995082617,0.0768418974580681)
--(axis cs:0.224999994970858,0.0777605148871777)
--(axis cs:0.229999994859099,0.0785133344857671)
--(axis cs:0.234999994747341,0.0791413520570611)
--(axis cs:0.239999994635582,0.0797528225260116)
--(axis cs:0.244999994523823,0.0804081349272958)
--(axis cs:0.249999994412065,0.0811245039471131)
--(axis cs:0.254999994300306,0.0819469556894927)
--(axis cs:0.259999994188547,0.0828277268081686)
--(axis cs:0.264999994076788,0.083654619614595)
--(axis cs:0.26999999396503,0.0844781400730263)
--(axis cs:0.274999993853271,0.0853383768624859)
--(axis cs:0.279999993741512,0.0861788771280623)
--(axis cs:0.284999993629754,0.0870447750003041)
--(axis cs:0.289999993517995,0.0879005156014825)
--(axis cs:0.294999993406236,0.0887168765336798)
--(axis cs:0.299999993294477,0.0894937210773138)
--(axis cs:0.304999993182719,0.0902402800370128)
--(axis cs:0.30999999307096,0.0910383227878737)
--(axis cs:0.314999992959201,0.0918803911532729)
--(axis cs:0.319999992847443,0.0927113933289962)
--(axis cs:0.324999992735684,0.0935837370493458)
--(axis cs:0.329999992623925,0.0943775842578269)
--(axis cs:0.334999992512167,0.0951652306126641)
--(axis cs:0.339999992400408,0.0959167605192633)
--(axis cs:0.344999992288649,0.0966510237428317)
--(axis cs:0.34999999217689,0.097363345827986)
--(axis cs:0.354999992065132,0.0980713040932966)
--(axis cs:0.359999991953373,0.0987706892135327)
--(axis cs:0.364999991841614,0.0994284663922396)
--(axis cs:0.369999991729856,0.100119564745113)
--(axis cs:0.374999991618097,0.100773185274741)
--(axis cs:0.379999991506338,0.101400677171746)
--(axis cs:0.384999991394579,0.101969868308733)
--(axis cs:0.389999991282821,0.102523574442257)
--(axis cs:0.394999991171062,0.103069923187987)
--(axis cs:0.399999991059303,0.103561442325757)
--(axis cs:0.404999990947545,0.104105967707741)
--(axis cs:0.409999990835786,0.104682373802634)
--(axis cs:0.414999990724027,0.10526009812568)
--(axis cs:0.419999990612268,0.105817756640169)
--(axis cs:0.42499999050051,0.106363172403119)
--(axis cs:0.429999990388751,0.106906004983255)
--(axis cs:0.434999990276992,0.107425245038112)
--(axis cs:0.439999990165234,0.107937389316414)
--(axis cs:0.444999990053475,0.108447895114424)
--(axis cs:0.449999989941716,0.10890250254781)
--(axis cs:0.454999989829957,0.109353601757642)
--(axis cs:0.459999989718199,0.109838444350698)
--(axis cs:0.46499998960644,0.110340469382864)
--(axis cs:0.469999989494681,0.110839343263005)
--(axis cs:0.474999989382923,0.111350581117816)
--(axis cs:0.479999989271164,0.111828421197552)
--(axis cs:0.484999989159405,0.112309817996079)
--(axis cs:0.489999989047647,0.112789800435704)
--(axis cs:0.494999988935888,0.113280933710017)
--(axis cs:0.494999988935888,0.155025004017252)
--(axis cs:0.494999988935888,0.155025004017252)
--(axis cs:0.489999989047647,0.154415986431967)
--(axis cs:0.484999989159405,0.153814763070669)
--(axis cs:0.479999989271164,0.153183831062644)
--(axis cs:0.474999989382923,0.152533579907756)
--(axis cs:0.469999989494681,0.15183814905118)
--(axis cs:0.46499998960644,0.151129472396737)
--(axis cs:0.459999989718199,0.150402738064095)
--(axis cs:0.454999989829957,0.149684822999253)
--(axis cs:0.449999989941716,0.149009440635106)
--(axis cs:0.444999990053475,0.14837664241687)
--(axis cs:0.439999990165234,0.147735430771245)
--(axis cs:0.434999990276992,0.147098043175534)
--(axis cs:0.429999990388751,0.146411411622155)
--(axis cs:0.42499999050051,0.145644544947047)
--(axis cs:0.419999990612268,0.144814815093848)
--(axis cs:0.414999990724027,0.143970815458984)
--(axis cs:0.409999990835786,0.143129932530385)
--(axis cs:0.404999990947545,0.142338920777637)
--(axis cs:0.399999991059303,0.141614752253145)
--(axis cs:0.394999991171062,0.140934362974097)
--(axis cs:0.389999991282821,0.140218203122878)
--(axis cs:0.384999991394579,0.139484521433157)
--(axis cs:0.379999991506338,0.138743422456424)
--(axis cs:0.374999991618097,0.137961317096887)
--(axis cs:0.369999991729856,0.137159904603361)
--(axis cs:0.364999991841614,0.136302886437633)
--(axis cs:0.359999991953373,0.135443928635118)
--(axis cs:0.354999992065132,0.134582958919926)
--(axis cs:0.34999999217689,0.13372580690658)
--(axis cs:0.344999992288649,0.132881628368785)
--(axis cs:0.339999992400408,0.132001943175998)
--(axis cs:0.334999992512167,0.131055166413313)
--(axis cs:0.329999992623925,0.130038671771912)
--(axis cs:0.324999992735684,0.128945300458556)
--(axis cs:0.319999992847443,0.127837501037084)
--(axis cs:0.314999992959201,0.126663692346972)
--(axis cs:0.30999999307096,0.125476560239464)
--(axis cs:0.304999993182719,0.124358167191449)
--(axis cs:0.299999993294477,0.123240510417331)
--(axis cs:0.294999993406236,0.122137497905999)
--(axis cs:0.289999993517995,0.121015943317474)
--(axis cs:0.284999993629754,0.119920679999321)
--(axis cs:0.279999993741512,0.118853420358227)
--(axis cs:0.274999993853271,0.117706365549454)
--(axis cs:0.26999999396503,0.116537450132247)
--(axis cs:0.264999994076788,0.115356675905878)
--(axis cs:0.259999994188547,0.114161547996086)
--(axis cs:0.254999994300306,0.112985762239335)
--(axis cs:0.249999994412065,0.111815462192957)
--(axis cs:0.244999994523823,0.110729004536866)
--(axis cs:0.239999994635582,0.109663470814929)
--(axis cs:0.234999994747341,0.108567142558893)
--(axis cs:0.229999994859099,0.107426143407133)
--(axis cs:0.224999994970858,0.106180505289214)
--(axis cs:0.219999995082617,0.104825527837035)
--(axis cs:0.214999995194376,0.103401042128595)
--(axis cs:0.209999995306134,0.101959487319666)
--(axis cs:0.204999995417893,0.100650383202345)
--(axis cs:0.199999995529652,0.0994209713482763)
--(axis cs:0.19499999564141,0.098361740048939)
--(axis cs:0.189999995753169,0.097307926007516)
--(axis cs:0.184999995864928,0.0962421988944678)
--(axis cs:0.179999995976686,0.0950081278310623)
--(axis cs:0.174999996088445,0.0936060079625685)
--(axis cs:0.169999996200204,0.0920618083641348)
--(axis cs:0.164999996311963,0.0905883043418095)
--(axis cs:0.159999996423721,0.0889454424644368)
--(axis cs:0.15499999653548,0.087353996169412)
--(axis cs:0.149999996647239,0.0859385115258687)
--(axis cs:0.144999996758997,0.0846810324896661)
--(axis cs:0.139999996870756,0.0834436601275601)
--(axis cs:0.134999996982515,0.0822586707522688)
--(axis cs:0.129999997094274,0.0808685027602842)
--(axis cs:0.124999997206032,0.0795524759051839)
--(axis cs:0.119999997317791,0.0780323875900292)
--(axis cs:0.11499999742955,0.0764346674510186)
--(axis cs:0.109999997541308,0.0748612103861089)
--(axis cs:0.104999997653067,0.0735093025197297)
--(axis cs:0.0999999977648258,0.0722539483627002)
--(axis cs:0.0949999978765845,0.0711310994013347)
--(axis cs:0.0899999979883432,0.0699214691293731)
--(axis cs:0.0849999981001019,0.0687558147126072)
--(axis cs:0.0799999982118607,0.0674135867561973)
--(axis cs:0.0749999983236194,0.0660706817994639)
--(axis cs:0.0699999984353781,0.0646987731983761)
--(axis cs:0.0649999985471368,0.0631773754243814)
--(axis cs:0.0599999986588955,0.061542753570785)
--(axis cs:0.0549999987706542,0.0598703043130145)
--(axis cs:0.0499999988824129,0.0582889689567411)
--(axis cs:0.0449999989941716,0.0572128531721293)
--(axis cs:0.0399999991059303,0.0561137244087217)
--(axis cs:0.034999999217689,0.0550887981847704)
--(axis cs:0.0299999993294477,0.0540726289438272)
--(axis cs:0.0249999994412065,0.0530287337582108)
--(axis cs:0.0199999995529652,0.0523139013503611)
--(axis cs:0.0149999996647239,0.0522699403018091)
--(axis cs:0.00999999977648258,0.053899109590012)
--(axis cs:0.00499999988824129,0.0595510930340604)
--cycle;

\path [fill=white!40.1960784313725!black, fill opacity=0.4,  ultra thick]
(axis cs:0.00499999988824129,0.0529545799497653)
--(axis cs:0.00499999988824129,0.0312038001669311)
--(axis cs:0.00999999977648258,0.0329828352733945)
--(axis cs:0.0149999996647239,0.0337306814792541)
--(axis cs:0.0199999995529652,0.0342793857545032)
--(axis cs:0.0249999994412065,0.0349030112798684)
--(axis cs:0.0299999993294477,0.035459325748376)
--(axis cs:0.034999999217689,0.0360063947972291)
--(axis cs:0.0399999991059303,0.0364294274348439)
--(axis cs:0.0449999989941716,0.0368715405888783)
--(axis cs:0.0499999988824129,0.0373345191026861)
--(axis cs:0.0549999987706542,0.0382326045301381)
--(axis cs:0.0599999986588955,0.0393157875342971)
--(axis cs:0.0649999985471368,0.0404345785158834)
--(axis cs:0.0699999984353781,0.0416640861412512)
--(axis cs:0.0749999983236194,0.0426987374654352)
--(axis cs:0.0799999982118607,0.0439043727761008)
--(axis cs:0.0849999981001019,0.0451599485867482)
--(axis cs:0.0899999979883432,0.0465710772595344)
--(axis cs:0.0949999978765845,0.0480801649454283)
--(axis cs:0.0999999977648258,0.0494057867145579)
--(axis cs:0.104999997653067,0.0507333926199508)
--(axis cs:0.109999997541308,0.0521689904629692)
--(axis cs:0.11499999742955,0.0537334265371703)
--(axis cs:0.119999997317791,0.0552858123370435)
--(axis cs:0.124999997206032,0.0564672070474576)
--(axis cs:0.129999997094274,0.0575850150898703)
--(axis cs:0.134999996982515,0.0586332624154657)
--(axis cs:0.139999996870756,0.0596310308205395)
--(axis cs:0.144999996758997,0.0605536942015979)
--(axis cs:0.149999996647239,0.0614437803835035)
--(axis cs:0.15499999653548,0.0626066399984635)
--(axis cs:0.159999996423721,0.0636846269471315)
--(axis cs:0.164999996311963,0.0648662780180515)
--(axis cs:0.169999996200204,0.0658982173097551)
--(axis cs:0.174999996088445,0.0668486594276827)
--(axis cs:0.179999995976686,0.0677558626324211)
--(axis cs:0.184999995864928,0.0686034991517549)
--(axis cs:0.189999995753169,0.0694191134127702)
--(axis cs:0.19499999564141,0.0701958728869677)
--(axis cs:0.199999995529652,0.071003449006537)
--(axis cs:0.204999995417893,0.0719319727088631)
--(axis cs:0.209999995306134,0.0728471018669668)
--(axis cs:0.214999995194376,0.0738169252714612)
--(axis cs:0.219999995082617,0.0747691848328039)
--(axis cs:0.224999994970858,0.0756374506013282)
--(axis cs:0.229999994859099,0.0763538419026544)
--(axis cs:0.234999994747341,0.0770279647752655)
--(axis cs:0.239999994635582,0.0776266689716228)
--(axis cs:0.244999994523823,0.0782354630429417)
--(axis cs:0.249999994412065,0.0787875810430996)
--(axis cs:0.254999994300306,0.0794638745594941)
--(axis cs:0.259999994188547,0.0801231643085537)
--(axis cs:0.264999994076788,0.0807971571435175)
--(axis cs:0.26999999396503,0.0814424473992927)
--(axis cs:0.274999993853271,0.0822638589186071)
--(axis cs:0.279999993741512,0.0830075116818677)
--(axis cs:0.284999993629754,0.0837421799721872)
--(axis cs:0.289999993517995,0.0844660902571253)
--(axis cs:0.294999993406236,0.0851174411402231)
--(axis cs:0.299999993294477,0.0857053225003193)
--(axis cs:0.304999993182719,0.0863089057879772)
--(axis cs:0.30999999307096,0.0869749540853776)
--(axis cs:0.314999992959201,0.0876661967136234)
--(axis cs:0.319999992847443,0.08834002511412)
--(axis cs:0.324999992735684,0.0890421612515591)
--(axis cs:0.329999992623925,0.0897399808160124)
--(axis cs:0.334999992512167,0.0904577030570728)
--(axis cs:0.339999992400408,0.0911410325409065)
--(axis cs:0.344999992288649,0.0918223491135857)
--(axis cs:0.34999999217689,0.0925094408477035)
--(axis cs:0.354999992065132,0.0931837219769631)
--(axis cs:0.359999991953373,0.0938570975897268)
--(axis cs:0.364999991841614,0.0944903778733287)
--(axis cs:0.369999991729856,0.0951410798092192)
--(axis cs:0.374999991618097,0.0957489541382195)
--(axis cs:0.379999991506338,0.0963672390393603)
--(axis cs:0.384999991394579,0.0969292493034325)
--(axis cs:0.389999991282821,0.097440845803114)
--(axis cs:0.394999991171062,0.0979695287737239)
--(axis cs:0.399999991059303,0.098475454487788)
--(axis cs:0.404999990947545,0.0990281283236533)
--(axis cs:0.409999990835786,0.0996006293633884)
--(axis cs:0.414999990724027,0.100213928951601)
--(axis cs:0.419999990612268,0.100844861337555)
--(axis cs:0.42499999050051,0.101496392546154)
--(axis cs:0.429999990388751,0.10214414452493)
--(axis cs:0.434999990276992,0.102761055833271)
--(axis cs:0.439999990165234,0.10336931652991)
--(axis cs:0.444999990053475,0.103941218525504)
--(axis cs:0.449999989941716,0.104451620045599)
--(axis cs:0.454999989829957,0.104932144704778)
--(axis cs:0.459999989718199,0.105429661419737)
--(axis cs:0.46499998960644,0.105941538446454)
--(axis cs:0.469999989494681,0.106496948945569)
--(axis cs:0.474999989382923,0.107047768936896)
--(axis cs:0.479999989271164,0.107567433954485)
--(axis cs:0.484999989159405,0.108056426816364)
--(axis cs:0.489999989047647,0.108522742142544)
--(axis cs:0.494999988935888,0.108960797960616)
--(axis cs:0.494999988935888,0.145501110774923)
--(axis cs:0.494999988935888,0.145501110774923)
--(axis cs:0.489999989047647,0.144880602798415)
--(axis cs:0.484999989159405,0.144253787326272)
--(axis cs:0.479999989271164,0.143629541013539)
--(axis cs:0.474999989382923,0.142994945497227)
--(axis cs:0.469999989494681,0.142318685963942)
--(axis cs:0.46499998960644,0.141644420364127)
--(axis cs:0.459999989718199,0.140928607841573)
--(axis cs:0.454999989829957,0.140218138514097)
--(axis cs:0.449999989941716,0.139492472291318)
--(axis cs:0.444999990053475,0.138805508780883)
--(axis cs:0.439999990165234,0.138070790057575)
--(axis cs:0.434999990276992,0.137344297512875)
--(axis cs:0.429999990388751,0.136607522247375)
--(axis cs:0.42499999050051,0.135817684578986)
--(axis cs:0.419999990612268,0.134967946619136)
--(axis cs:0.414999990724027,0.134120095721887)
--(axis cs:0.409999990835786,0.133231712579616)
--(axis cs:0.404999990947545,0.132346735262191)
--(axis cs:0.399999991059303,0.13151012701284)
--(axis cs:0.394999991171062,0.130702788717121)
--(axis cs:0.389999991282821,0.129898844124022)
--(axis cs:0.384999991394579,0.129050110979797)
--(axis cs:0.379999991506338,0.128187971004958)
--(axis cs:0.374999991618097,0.127305883388324)
--(axis cs:0.369999991729856,0.126409377974926)
--(axis cs:0.364999991841614,0.125493446273932)
--(axis cs:0.359999991953373,0.124586709889861)
--(axis cs:0.354999992065132,0.123693394350026)
--(axis cs:0.34999999217689,0.122817259714568)
--(axis cs:0.344999992288649,0.121957692630587)
--(axis cs:0.339999992400408,0.121082514734666)
--(axis cs:0.334999992512167,0.12016666998318)
--(axis cs:0.329999992623925,0.119177783530429)
--(axis cs:0.324999992735684,0.118136846634319)
--(axis cs:0.319999992847443,0.11704608396683)
--(axis cs:0.314999992959201,0.115920093907405)
--(axis cs:0.30999999307096,0.114772739919011)
--(axis cs:0.304999993182719,0.113658113073141)
--(axis cs:0.299999993294477,0.112604472578433)
--(axis cs:0.294999993406236,0.111619326307123)
--(axis cs:0.289999993517995,0.110614443922421)
--(axis cs:0.284999993629754,0.109616401537881)
--(axis cs:0.279999993741512,0.108599591462912)
--(axis cs:0.274999993853271,0.107514961318312)
--(axis cs:0.26999999396503,0.106397091616674)
--(axis cs:0.264999994076788,0.105245519985923)
--(axis cs:0.259999994188547,0.104048096786195)
--(axis cs:0.254999994300306,0.102796531361236)
--(axis cs:0.249999994412065,0.101539173077055)
--(axis cs:0.244999994523823,0.10039703536593)
--(axis cs:0.239999994635582,0.0993933820184098)
--(axis cs:0.234999994747341,0.0984003632475762)
--(axis cs:0.229999994859099,0.0973930983792203)
--(axis cs:0.224999994970858,0.0963165370290274)
--(axis cs:0.219999995082617,0.0951037615394297)
--(axis cs:0.214999995194376,0.0938614245200703)
--(axis cs:0.209999995306134,0.0926326441679597)
--(axis cs:0.204999995417893,0.0914949870609047)
--(axis cs:0.199999995529652,0.0904590025254958)
--(axis cs:0.19499999564141,0.0895458645009159)
--(axis cs:0.189999995753169,0.0885571994941532)
--(axis cs:0.184999995864928,0.0874569864667143)
--(axis cs:0.179999995976686,0.0862761552414902)
--(axis cs:0.174999996088445,0.0850233995073671)
--(axis cs:0.169999996200204,0.0836488426690747)
--(axis cs:0.164999996311963,0.082224508737199)
--(axis cs:0.159999996423721,0.0807720654302749)
--(axis cs:0.15499999653548,0.0793902000754053)
--(axis cs:0.149999996647239,0.0782204196738345)
--(axis cs:0.144999996758997,0.0770962500771077)
--(axis cs:0.139999996870756,0.0759950792987211)
--(axis cs:0.134999996982515,0.0748953677048322)
--(axis cs:0.129999997094274,0.0736769399532037)
--(axis cs:0.124999997206032,0.0726083596535632)
--(axis cs:0.119999997317791,0.0714814618580268)
--(axis cs:0.11499999742955,0.0702394534175706)
--(axis cs:0.109999997541308,0.0689388911744563)
--(axis cs:0.104999997653067,0.0677887533123136)
--(axis cs:0.0999999977648258,0.066645140086752)
--(axis cs:0.0949999978765845,0.0657520651761476)
--(axis cs:0.0899999979883432,0.0649074166772428)
--(axis cs:0.0849999981001019,0.0640559791003478)
--(axis cs:0.0799999982118607,0.0629994846955665)
--(axis cs:0.0749999983236194,0.0618339719525378)
--(axis cs:0.0699999984353781,0.0605766642717604)
--(axis cs:0.0649999985471368,0.0591098516139143)
--(axis cs:0.0599999986588955,0.0576376869378847)
--(axis cs:0.0549999987706542,0.0561640832930698)
--(axis cs:0.0499999988824129,0.0547251719220504)
--(axis cs:0.0449999989941716,0.0536398036050619)
--(axis cs:0.0399999991059303,0.0524621172920365)
--(axis cs:0.034999999217689,0.0512733673034577)
--(axis cs:0.0299999993294477,0.0500858461625836)
--(axis cs:0.0249999994412065,0.0487786039099984)
--(axis cs:0.0199999995529652,0.0478305057979142)
--(axis cs:0.0149999996647239,0.04756326747567)
--(axis cs:0.00999999977648258,0.0481438195449914)
--(axis cs:0.00499999988824129,0.0529545799497653)
--cycle;

\addplot [ ultra thick, red]
table {%
0.00499999523162842 0.0502040535211563
0.00999999046325684 0.0528985634446144
0.0149999856948853 0.0548800900578499
0.0199999809265137 0.0563131421804428
0.0249999761581421 0.0584983006119728
0.0349999666213989 0.0636324137449265
0.0499999523162842 0.071731872856617
0.0700000524520874 0.0861394107341766
0.0750000476837158 0.0898492261767387
0.0800000429153442 0.0934320613741875
0.0850000381469727 0.0968890264630318
0.0900000333786011 0.100355163216591
0.0950000286102295 0.103741176426411
0.115000009536743 0.117665886878967
0.120000004768372 0.12146507948637
0.125 0.125257387757301
0.129999995231628 0.12899012863636
0.134999990463257 0.132673919200897
0.139999985694885 0.136323049664497
0.149999976158142 0.143458008766174
0.159999966621399 0.15057073533535
0.164999961853027 0.154120102524757
0.174999952316284 0.161046624183655
0.184999942779541 0.167996570467949
0.194999933242798 0.174913659691811
0.215000033378601 0.18895623087883
0.225000023841858 0.196136072278023
0.230000019073486 0.199712947010994
0.240000009536743 0.206709891557693
0.25 0.21355265378952
0.259999990463257 0.220447584986687
0.269999980926514 0.227247104048729
0.279999971389771 0.233858659863472
0.284999966621399 0.237084254622459
0.294999957084656 0.243317246437073
0.309999942779541 0.252560704946518
0.319999933242798 0.258698761463165
0.329999923706055 0.264744251966476
0.340000033378601 0.270667642354965
0.355000019073486 0.279461711645126
0.370000004768372 0.288364470005035
0.379999995231628 0.29425510764122
0.389999985694885 0.300001293420792
0.399999976158142 0.305585563182831
0.414999961853027 0.313862979412079
0.424999952316284 0.319270461797714
0.434999942779541 0.324498325586319
0.444999933242798 0.329549551010132
0.465000033378601 0.339408159255981
0.480000019073486 0.346703141927719
0.495000004768372 0.353809475898743
};
\addplot [ ultra thick, blue]
table {%
0.00499999523162842 0.0418583564460278
0.00999999046325684 0.0430080071091652
0.0149999856948853 0.0447838678956032
0.0199999809265137 0.0461419671773911
0.0249999761581421 0.0476496890187263
0.0299999713897705 0.0490430556237698
0.0349999666213989 0.0501708388328552
0.0449999570846558 0.0521417930722237
0.0499999523162842 0.0531256496906281
0.0549999475479126 0.0546357408165932
0.059999942779541 0.056302648037672
0.065000057220459 0.0579059682786465
0.0700000524520874 0.0594953745603561
0.0750000476837158 0.0610238127410412
0.0800000429153442 0.0624929927289486
0.0950000286102295 0.0669156610965729
0.100000023841858 0.0683723986148834
0.110000014305115 0.0716753304004669
0.120000004768372 0.0753502324223518
0.125 0.0770150646567345
0.129999995231628 0.0785594955086708
0.134999990463257 0.0800564140081406
0.139999985694885 0.0814613327383995
0.149999976158142 0.0842480286955833
0.159999966621399 0.0874122753739357
0.164999961853027 0.0891114324331284
0.169999957084656 0.0907594710588455
0.174999952316284 0.0923305153846741
0.179999947547913 0.0937919765710831
0.184999942779541 0.0951278880238533
0.190000057220459 0.0964302867650986
0.220000028610229 0.103931479156017
0.225000023841858 0.105124622583389
0.230000019073486 0.106238506734371
0.240000009536743 0.10825227946043
0.245000004768372 0.109234966337681
0.25 0.110170818865299
0.264999985694885 0.113245606422424
0.279999971389771 0.116347879171371
0.289999961853027 0.118355393409729
0.294999957084656 0.119339346885681
0.305000066757202 0.121238239109516
0.325000047683716 0.125380501151085
0.335000038146973 0.127283915877342
0.345000028610229 0.129037410020828
0.360000014305115 0.131676897406578
0.370000004768372 0.133466243743896
0.379999995231628 0.135145336389542
0.389999985694885 0.136647030711174
0.409999966621399 0.139608860015869
0.434999942779541 0.143586009740829
0.444999933242798 0.145049199461937
0.470000028610229 0.148374676704407
0.480000019073486 0.149672761559486
0.495000004768372 0.151514068245888
};
\addplot [ ultra thick, green!50.1960784313725!black]
table {%
0.00499999523162842 0.0452259927988052
0.00999999046325684 0.0431519411504269
0.0149999856948853 0.0428277067840099
0.0199999809265137 0.0425995513796806
0.0249999761581421 0.0427290834486485
0.0349999666213989 0.0436177328228951
0.0399999618530273 0.0441128611564636
0.0499999523162842 0.0453359931707382
0.0549999475479126 0.0464074648916721
0.059999942779541 0.0476562529802322
0.0700000524520874 0.0500528328120708
0.0800000429153442 0.0523310303688049
0.0950000286102295 0.0558176673948765
0.100000023841858 0.0568728186190128
0.110000014305115 0.0592905804514885
0.115000009536743 0.0607371516525745
0.120000004768372 0.0621263831853867
0.125 0.0632980242371559
0.139999985694885 0.0663584619760513
0.149999976158142 0.0683364868164062
0.154999971389771 0.069410465657711
0.174999952316284 0.0742087140679359
0.179999947547913 0.0753667205572128
0.184999942779541 0.0764299929141998
0.190000057220459 0.0774173513054848
0.194999933242798 0.0783472508192062
0.200000047683716 0.0792386755347252
0.205000042915344 0.0802338570356369
0.210000038146973 0.0813190639019012
0.215000033378601 0.0824715197086334
0.220000028610229 0.0835959166288376
0.225000023841858 0.0846395716071129
0.230000019073486 0.0855481848120689
0.25 0.0890070199966431
0.264999985694885 0.0918687731027603
0.289999961853027 0.0965574756264687
0.305000066757202 0.0993979722261429
0.315000057220459 0.101437076926231
0.329999923706055 0.104453399777412
0.340000033378601 0.106342226266861
0.350000023841858 0.108157239854336
0.360000014305115 0.109949015080929
0.370000004768372 0.111702598631382
0.379999995231628 0.113362640142441
0.389999985694885 0.114880159497261
0.399999976158142 0.116320930421352
0.409999966621399 0.117834605276585
0.429999947547913 0.121034547686577
0.440000057220459 0.122513145208359
0.444999933242798 0.123229838907719
0.460000038146973 0.125245705246925
0.470000028610229 0.126617267727852
0.480000019073486 0.127893954515457
0.495000004768372 0.129639953374863
};
\addplot [ ultra thick, color0]
table {%
0.00499999523162842 0.0447856895625591
0.00999999046325684 0.0424579605460167
0.0149999856948853 0.0426326207816601
0.0199999809265137 0.0433087311685085
0.0249999761581421 0.0441878028213978
0.0299999713897705 0.0451426617801189
0.0399999618530273 0.0467568337917328
0.0449999570846558 0.0476778410375118
0.0499999523162842 0.0485651604831219
0.0549999475479126 0.0499339699745178
0.059999942779541 0.0513933412730694
0.065000057220459 0.0528361611068249
0.0700000524520874 0.0542483106255531
0.0750000476837158 0.0555483140051365
0.0800000429153442 0.0568103939294815
0.0850000381469727 0.0581753849983215
0.0950000286102295 0.0608352944254875
0.100000023841858 0.0619966089725494
0.105000019073486 0.0632294714450836
0.110000014305115 0.0645837038755417
0.120000004768372 0.0675899162888527
0.125 0.0689172595739365
0.134999990463257 0.0713060945272446
0.139999985694885 0.0723845660686493
0.149999976158142 0.0744868293404579
0.154999971389771 0.0757122859358788
0.164999961853027 0.0784044563770294
0.174999952316284 0.0809601992368698
0.179999947547913 0.0821652337908745
0.184999942779541 0.0832424461841583
0.194999933242798 0.0851936116814613
0.200000047683716 0.0861350074410439
0.205000042915344 0.0871875733137131
0.210000038146973 0.0883699655532837
0.215000033378601 0.0896333158016205
0.220000028610229 0.0908337160944939
0.225000023841858 0.0919705033302307
0.230000019073486 0.0929697304964066
0.240000009536743 0.0947081297636032
0.25 0.0964699760079384
0.274999976158142 0.101522371172905
0.284999966621399 0.103482738137245
0.294999957084656 0.105427168309689
0.315000057220459 0.109272062778473
0.325000047683716 0.111264511942863
0.329999923706055 0.112208113074303
0.335000038146973 0.113110221922398
0.340000033378601 0.113959342241287
0.350000023841858 0.115544594824314
0.365000009536743 0.117865659296513
0.370000004768372 0.118639744818211
0.379999995231628 0.120072044432163
0.389999985694885 0.121370896697044
0.394999980926514 0.122002117335796
0.399999976158142 0.122588090598583
0.404999971389771 0.123222462832928
0.429999947547913 0.126658692955971
0.440000057220459 0.127836391329765
0.450000047683716 0.128955975174904
0.460000038146973 0.13012059032917
0.475000023841858 0.131942063570023
0.490000009536743 0.133602902293205
0.495000004768372 0.134152933955193
};
\addplot [ ultra thick, white!40.1960784313725!black]
table {%
0.00499999523162842 0.0420791953802109
0.00999999046325684 0.0405633263289928
0.0149999856948853 0.0406469739973545
0.0199999809265137 0.0410549491643906
0.0249999761581421 0.0418408066034317
0.0299999713897705 0.0427725873887539
0.0349999666213989 0.0436398759484291
0.0449999570846558 0.0452556721866131
0.0499999523162842 0.0460298508405685
0.0549999475479126 0.0471983402967453
0.0700000524520874 0.0511203818023205
0.0850000381469727 0.0546079725027084
0.0950000286102295 0.056916106492281
0.100000023841858 0.0580254606902599
0.110000014305115 0.0605539381504059
0.115000009536743 0.0619864352047443
0.120000004768372 0.0633836388587952
0.125 0.0645377933979034
0.134999990463257 0.0667643174529076
0.139999985694885 0.0678130462765694
0.149999976158142 0.0698321089148521
0.154999971389771 0.0709984302520752
0.159999966621399 0.072228342294693
0.164999961853027 0.0735453888773918
0.169999957084656 0.0747735202312469
0.174999952316284 0.0759360268712044
0.179999947547913 0.0770160183310509
0.184999942779541 0.0780302360653877
0.190000057220459 0.0789881646633148
0.200000047683716 0.0807312279939651
0.210000038146973 0.0827398672699928
0.220000028610229 0.0849364697933197
0.225000023841858 0.0859769806265831
0.230000019073486 0.0868734568357468
0.235000014305115 0.0877141579985619
0.245000004768372 0.0893162488937378
0.25 0.0901633873581886
0.259999990463257 0.092085637152195
0.264999985694885 0.093021348118782
0.269999980926514 0.0939197614789009
0.274999976158142 0.0948894172906876
0.279999971389771 0.0958035588264465
0.289999961853027 0.0975402593612671
0.294999957084656 0.0983683839440346
0.305000066757202 0.0999835059046745
0.325000047683716 0.103589504957199
0.335000038146973 0.105312176048756
0.345000028610229 0.106890007853508
0.370000004768372 0.110775224864483
0.379999995231628 0.112277619540691
0.389999985694885 0.113669835031033
0.404999971389771 0.115687429904938
0.429999947547913 0.119375847280025
0.440000057220459 0.120720073580742
0.444999933242798 0.121373362839222
0.480000019073486 0.125598475337029
0.490000009536743 0.126701638102531
0.495000004768372 0.127230957150459
};

==> supp_mat/ant_plots/train_test_loss_data.tex <==
\definecolor{color0}{rgb}{1,0,1}

\path [fill=red, fill opacity=0.4, ultra thick]
(axis cs:0,0.0544604100286961)
--(axis cs:0,0.0544556342065334)
--(axis cs:100,0.054262787103653)
--(axis cs:200,0.0538671836256981)
--(axis cs:300,0.053299356251955)
--(axis cs:400,0.0524099729955196)
--(axis cs:500,0.0512915588915348)
--(axis cs:600,0.0498612597584724)
--(axis cs:700,0.048358503729105)
--(axis cs:800,0.0468810349702835)
--(axis cs:900,0.0455310307443142)
--(axis cs:1000,0.0442750826478004)
--(axis cs:1100,0.0432932898402214)
--(axis cs:1200,0.0424183383584023)
--(axis cs:1300,0.0415273271501064)
--(axis cs:1400,0.0406446345150471)
--(axis cs:1500,0.0398341491818428)
--(axis cs:1600,0.0391616970300674)
--(axis cs:1700,0.0385490283370018)
--(axis cs:1800,0.0380383096635342)
--(axis cs:1900,0.0376506596803665)
--(axis cs:2000,0.0372785739600658)
--(axis cs:2100,0.0367969311773777)
--(axis cs:2200,0.0362707525491714)
--(axis cs:2300,0.0357639789581299)
--(axis cs:2400,0.0351036749780178)
--(axis cs:2500,0.0343529209494591)
--(axis cs:2600,0.0336244218051434)
--(axis cs:2700,0.0329313911497593)
--(axis cs:2800,0.0321676023304462)
--(axis cs:2900,0.0315744169056416)
--(axis cs:3000,0.0310739763081074)
--(axis cs:3100,0.0305582359433174)
--(axis cs:3200,0.0300906151533127)
--(axis cs:3300,0.0296397153288126)
--(axis cs:3400,0.0291373878717422)
--(axis cs:3500,0.0286697149276733)
--(axis cs:3600,0.0282844062894583)
--(axis cs:3700,0.0278869438916445)
--(axis cs:3800,0.0275154709815979)
--(axis cs:3900,0.0271617714315653)
--(axis cs:4000,0.0268238559365273)
--(axis cs:4100,0.0264994949102402)
--(axis cs:4200,0.0262080077081919)
--(axis cs:4300,0.0259157679975033)
--(axis cs:4400,0.0256689712405205)
--(axis cs:4500,0.025422491133213)
--(axis cs:4600,0.0251766443252563)
--(axis cs:4700,0.0248826667666435)
--(axis cs:4800,0.0246551185846329)
--(axis cs:4900,0.0243975836783648)
--(axis cs:5000,0.02416424266994)
--(axis cs:5100,0.0239365864545107)
--(axis cs:5200,0.0237438529729843)
--(axis cs:5300,0.0235683433711529)
--(axis cs:5400,0.0233610551804304)
--(axis cs:5500,0.0231598597019911)
--(axis cs:5600,0.023010179400444)
--(axis cs:5700,0.0228530038148165)
--(axis cs:5800,0.0226530227810144)
--(axis cs:5900,0.0224942173808813)
--(axis cs:6000,0.0224036760628223)
--(axis cs:6100,0.022212190553546)
--(axis cs:6200,0.0220252610743046)
--(axis cs:6300,0.0218626577407122)
--(axis cs:6400,0.0217299945652485)
--(axis cs:6500,0.0215557813644409)
--(axis cs:6600,0.0214070416986942)
--(axis cs:6700,0.0212934091687202)
--(axis cs:6800,0.0211514942348003)
--(axis cs:6900,0.0209446866065264)
--(axis cs:7000,0.0208285804837942)
--(axis cs:7100,0.0207280609756708)
--(axis cs:7200,0.0205901581794024)
--(axis cs:7300,0.0204629115760326)
--(axis cs:7400,0.0203637108206749)
--(axis cs:7500,0.0202481839805841)
--(axis cs:7600,0.0201098583638668)
--(axis cs:7700,0.0200173370540142)
--(axis cs:7800,0.0199753753840923)
--(axis cs:7900,0.0198731906712055)
--(axis cs:8000,0.0197667293250561)
--(axis cs:8100,0.019667761400342)
--(axis cs:8200,0.0195592604577541)
--(axis cs:8300,0.0194630138576031)
--(axis cs:8400,0.0193438455462456)
--(axis cs:8500,0.0192207656800747)
--(axis cs:8600,0.019170131534338)
--(axis cs:8700,0.0191291328519583)
--(axis cs:8800,0.0189835410565138)
--(axis cs:8900,0.0188969131559134)
--(axis cs:9000,0.01880769059062)
--(axis cs:9100,0.0187026020139456)
--(axis cs:9200,0.0185937248170376)
--(axis cs:9300,0.0185507107526064)
--(axis cs:9400,0.0184898860752583)
--(axis cs:9500,0.0184556003659964)
--(axis cs:9600,0.0183398947119713)
--(axis cs:9700,0.0182806253433228)
--(axis cs:9800,0.0181940011680126)
--(axis cs:9900,0.0180638488382101)
--(axis cs:10000,0.0179491955786943)
--(axis cs:10100,0.017841188237071)
--(axis cs:10200,0.0176926981657743)
--(axis cs:10300,0.0175967868417501)
--(axis cs:10400,0.0175317618995905)
--(axis cs:10500,0.0174021758139133)
--(axis cs:10600,0.0173880644142628)
--(axis cs:10700,0.0173646006733179)
--(axis cs:10800,0.0172961968928576)
--(axis cs:10900,0.0171888209879398)
--(axis cs:11000,0.0171309262514114)
--(axis cs:11100,0.0169935300946236)
--(axis cs:11200,0.0169182326644659)
--(axis cs:11300,0.0168725401163101)
--(axis cs:11400,0.016796637326479)
--(axis cs:11500,0.016751479357481)
--(axis cs:11600,0.0166537445038557)
--(axis cs:11700,0.0165449250489473)
--(axis cs:11800,0.0164618492126465)
--(axis cs:11900,0.0164309032261372)
--(axis cs:12000,0.0163197480142117)
--(axis cs:12100,0.0162341054528952)
--(axis cs:12200,0.0161963142454624)
--(axis cs:12300,0.01618174277246)
--(axis cs:12400,0.0160710904747248)
--(axis cs:12500,0.0160338543355465)
--(axis cs:12600,0.0159660317003727)
--(axis cs:12700,0.015897274017334)
--(axis cs:12800,0.0158267971128225)
--(axis cs:12900,0.0158129688352346)
--(axis cs:13000,0.0157561786472797)
--(axis cs:13100,0.0156633742153645)
--(axis cs:13200,0.0156288873404264)
--(axis cs:13300,0.0155679890885949)
--(axis cs:13400,0.015466975979507)
--(axis cs:13500,0.0153632434085011)
--(axis cs:13600,0.0152401765808463)
--(axis cs:13700,0.0151568911969662)
--(axis cs:13800,0.0151304304599762)
--(axis cs:13900,0.0151357362046838)
--(axis cs:14000,0.0151082603260875)
--(axis cs:14100,0.0150860194116831)
--(axis cs:14200,0.0150018809363246)
--(axis cs:14300,0.0149315511807799)
--(axis cs:14400,0.0148943904787302)
--(axis cs:14500,0.0148011669516563)
--(axis cs:14600,0.0147597370669246)
--(axis cs:14700,0.0147587619721889)
--(axis cs:14800,0.0147669324651361)
--(axis cs:14900,0.0146925253793597)
--(axis cs:15000,0.0146520137786865)
--(axis cs:15100,0.0145990373566747)
--(axis cs:15200,0.0145597932860255)
--(axis cs:15300,0.0145007641986012)
--(axis cs:15400,0.0144540788605809)
--(axis cs:15500,0.0144067155197263)
--(axis cs:15600,0.0143493665382266)
--(axis cs:15700,0.0142554761841893)
--(axis cs:15800,0.0142619730904698)
--(axis cs:15900,0.0142113519832492)
--(axis cs:16000,0.0141738196834922)
--(axis cs:16100,0.0141389593482018)
--(axis cs:16200,0.0141159929335117)
--(axis cs:16300,0.0140097886323929)
--(axis cs:16400,0.0140025140717626)
--(axis cs:16500,0.0139666171744466)
--(axis cs:16600,0.0139559656381607)
--(axis cs:16700,0.0138910617679358)
--(axis cs:16800,0.0138474320992827)
--(axis cs:16900,0.0137956654652953)
--(axis cs:17000,0.0137717258185148)
--(axis cs:17100,0.0136962793767452)
--(axis cs:17200,0.01372582744807)
--(axis cs:17300,0.0136330248787999)
--(axis cs:17400,0.0135961640626192)
--(axis cs:17500,0.0135835250839591)
--(axis cs:17600,0.0135486600920558)
--(axis cs:17700,0.0134784579277039)
--(axis cs:17800,0.0135223409160972)
--(axis cs:17900,0.0134405894204974)
--(axis cs:18000,0.0133964847773314)
--(axis cs:18100,0.0133821414783597)
--(axis cs:18200,0.0133144287392497)
--(axis cs:18300,0.0132715748623013)
--(axis cs:18400,0.01326759532094)
--(axis cs:18500,0.013171287253499)
--(axis cs:18600,0.0131280375644565)
--(axis cs:18700,0.0131670320406556)
--(axis cs:18800,0.0131124742329121)
--(axis cs:18900,0.0130656994879246)
--(axis cs:19000,0.0130478031933308)
--(axis cs:19100,0.0129994284361601)
--(axis cs:19200,0.0129510853439569)
--(axis cs:19300,0.0129520930349827)
--(axis cs:19400,0.0129182981327176)
--(axis cs:19500,0.012884110212326)
--(axis cs:19600,0.0128494678065181)
--(axis cs:19700,0.0128425601869822)
--(axis cs:19800,0.0128195835277438)
--(axis cs:19900,0.0128211388364434)
--(axis cs:20000,0.0127958301454782)
--(axis cs:20100,0.0128185274079442)
--(axis cs:20200,0.0127081871032715)
--(axis cs:20300,0.0126992203295231)
--(axis cs:20400,0.0126626091077924)
--(axis cs:20500,0.0126040503382683)
--(axis cs:20600,0.0125713516026735)
--(axis cs:20700,0.0125728696584702)
--(axis cs:20800,0.0125019447878003)
--(axis cs:20900,0.0124830706045032)
--(axis cs:21000,0.0124933244660497)
--(axis cs:21100,0.0124383922666311)
--(axis cs:21200,0.01238146238029)
--(axis cs:21300,0.0123946191743016)
--(axis cs:21400,0.0123699186369777)
--(axis cs:21500,0.0122704524546862)
--(axis cs:21600,0.0122605636715889)
--(axis cs:21700,0.0122461812570691)
--(axis cs:21800,0.0122376251965761)
--(axis cs:21900,0.0122387958690524)
--(axis cs:22000,0.0122581394389272)
--(axis cs:22100,0.0122813833877444)
--(axis cs:22200,0.0121810473501682)
--(axis cs:22300,0.0121277393773198)
--(axis cs:22400,0.012080860324204)
--(axis cs:22500,0.0120696211233735)
--(axis cs:22600,0.0119963428005576)
--(axis cs:22700,0.0120304087176919)
--(axis cs:22800,0.0120290163904428)
--(axis cs:22900,0.0119633991271257)
--(axis cs:23000,0.0119415419176221)
--(axis cs:23100,0.0119390795007348)
--(axis cs:23200,0.0119160618633032)
--(axis cs:23300,0.0119337383657694)
--(axis cs:23400,0.0119722811505198)
--(axis cs:23500,0.0119769787415862)
--(axis cs:23600,0.0119992168620229)
--(axis cs:23700,0.0119779221713543)
--(axis cs:23800,0.0119130099192262)
--(axis cs:23900,0.0118473377078772)
--(axis cs:24000,0.0118102850392461)
--(axis cs:24100,0.0118188504129648)
--(axis cs:24200,0.011789171025157)
--(axis cs:24300,0.0117522710934281)
--(axis cs:24400,0.011734020896256)
--(axis cs:24500,0.0117339137941599)
--(axis cs:24600,0.0116416933014989)
--(axis cs:24700,0.0116728991270065)
--(axis cs:24800,0.0116539001464844)
--(axis cs:24900,0.0116408346220851)
--(axis cs:25000,0.011630249209702)
--(axis cs:25100,0.0115809440612793)
--(axis cs:25200,0.0115015031769872)
--(axis cs:25300,0.0115537643432617)
--(axis cs:25400,0.0115228649228811)
--(axis cs:25500,0.0115791317075491)
--(axis cs:25600,0.0116032604128122)
--(axis cs:25700,0.0115549089387059)
--(axis cs:25800,0.0115009304136038)
--(axis cs:25900,0.0115269664674997)
--(axis cs:26000,0.0115234274417162)
--(axis cs:26100,0.0115083549171686)
--(axis cs:26100,0.0119591541588306)
--(axis cs:26100,0.0119591541588306)
--(axis cs:26000,0.0119519662111998)
--(axis cs:25900,0.0119433784857392)
--(axis cs:25800,0.011936510913074)
--(axis cs:25700,0.0119388094171882)
--(axis cs:25600,0.0119435833767056)
--(axis cs:25500,0.01193852070719)
--(axis cs:25400,0.0119404662400484)
--(axis cs:25300,0.0119446646422148)
--(axis cs:25200,0.0119415652006865)
--(axis cs:25100,0.0119485789909959)
--(axis cs:25000,0.0119504695758224)
--(axis cs:24900,0.0119587359949946)
--(axis cs:24800,0.0119654517620802)
--(axis cs:24700,0.0119749177247286)
--(axis cs:24600,0.0119625115767121)
--(axis cs:24500,0.0119722979143262)
--(axis cs:24400,0.0119829708710313)
--(axis cs:24300,0.0119849359616637)
--(axis cs:24200,0.0119915865361691)
--(axis cs:24100,0.012009721249342)
--(axis cs:24000,0.0120248794555664)
--(axis cs:23900,0.0120248794555664)
--(axis cs:23800,0.0120350839570165)
--(axis cs:23700,0.0120603926479816)
--(axis cs:23600,0.0120548652485013)
--(axis cs:23500,0.0120907733216882)
--(axis cs:23400,0.0121250152587891)
--(axis cs:23300,0.0121221542358398)
--(axis cs:23200,0.0121251102536917)
--(axis cs:23100,0.0121641159057617)
--(axis cs:23000,0.0121542932465672)
--(axis cs:22900,0.0121618267148733)
--(axis cs:22800,0.0122117958962917)
--(axis cs:22700,0.0122381234541535)
--(axis cs:22600,0.0122654503211379)
--(axis cs:22500,0.0123108746483922)
--(axis cs:22400,0.0123540451750159)
--(axis cs:22300,0.012373742647469)
--(axis cs:22200,0.0124011989682913)
--(axis cs:22100,0.0123969120904803)
--(axis cs:22000,0.0123847965151072)
--(axis cs:21900,0.0123737333342433)
--(axis cs:21800,0.0123680112883449)
--(axis cs:21700,0.012409414164722)
--(axis cs:21600,0.0124173481017351)
--(axis cs:21500,0.0124794915318489)
--(axis cs:21400,0.0125247500836849)
--(axis cs:21300,0.0125572141259909)
--(axis cs:21200,0.0125944409519434)
--(axis cs:21100,0.0126098366454244)
--(axis cs:21000,0.0126252938061953)
--(axis cs:20900,0.0126391900703311)
--(axis cs:20800,0.0126958461478353)
--(axis cs:20700,0.0126935001462698)
--(axis cs:20600,0.0127169769257307)
--(axis cs:20500,0.0127220153808594)
--(axis cs:20400,0.0127724651247263)
--(axis cs:20300,0.0127746928483248)
--(axis cs:20200,0.012856213375926)
--(axis cs:20100,0.0128957824781537)
--(axis cs:20000,0.0129368286579847)
--(axis cs:19900,0.0129301669076085)
--(axis cs:19800,0.0129576679319143)
--(axis cs:19700,0.0129804350435734)
--(axis cs:19600,0.013002417050302)
--(axis cs:19500,0.0130496025085449)
--(axis cs:19400,0.0130996704101562)
--(axis cs:19300,0.0131112094968557)
--(axis cs:19200,0.0131596568971872)
--(axis cs:19100,0.0131754353642464)
--(axis cs:19000,0.0131762679666281)
--(axis cs:18900,0.0131357405334711)
--(axis cs:18800,0.0132158044725657)
--(axis cs:18700,0.0132748605683446)
--(axis cs:18600,0.0133171081542969)
--(axis cs:18500,0.0133959772065282)
--(axis cs:18400,0.0135154724121094)
--(axis cs:18300,0.0135165210813284)
--(axis cs:18200,0.0135496230795979)
--(axis cs:18100,0.0135834449902177)
--(axis cs:18000,0.013546722009778)
--(axis cs:17900,0.013551140204072)
--(axis cs:17800,0.0135754263028502)
--(axis cs:17700,0.0136132687330246)
--(axis cs:17600,0.013629131950438)
--(axis cs:17500,0.0137187084183097)
--(axis cs:17400,0.0137523543089628)
--(axis cs:17300,0.0138086322695017)
--(axis cs:17200,0.0138773918151855)
--(axis cs:17100,0.013890934176743)
--(axis cs:17000,0.0139442440122366)
--(axis cs:16900,0.0139674190431833)
--(axis cs:16800,0.0139827728271484)
--(axis cs:16700,0.013984203338623)
--(axis cs:16600,0.0140440072864294)
--(axis cs:16500,0.0141013832762837)
--(axis cs:16400,0.0140979969874024)
--(axis cs:16300,0.0140926409512758)
--(axis cs:16200,0.0141599653288722)
--(axis cs:16100,0.0141788106411695)
--(axis cs:16000,0.0142360096797347)
--(axis cs:15900,0.0142741044983268)
--(axis cs:15800,0.0143489548936486)
--(axis cs:15700,0.0143393436446786)
--(axis cs:15600,0.0144090326502919)
--(axis cs:15500,0.0144206034019589)
--(axis cs:15400,0.0144716138020158)
--(axis cs:15300,0.0145261259749532)
--(axis cs:15200,0.0146220847964287)
--(axis cs:15100,0.0146814035251737)
--(axis cs:15000,0.0147329801693559)
--(axis cs:14900,0.0147829754278064)
--(axis cs:14800,0.0147873079404235)
--(axis cs:14700,0.014823580160737)
--(axis cs:14600,0.0148650435730815)
--(axis cs:14500,0.0148841384798288)
--(axis cs:14400,0.0149312755092978)
--(axis cs:14300,0.0149893751367927)
--(axis cs:14200,0.0150564378127456)
--(axis cs:14100,0.0151063445955515)
--(axis cs:14000,0.0151844741776586)
--(axis cs:13900,0.0151990409940481)
--(axis cs:13800,0.0152580263093114)
--(axis cs:13700,0.0153612140566111)
--(axis cs:13600,0.0154139995574951)
--(axis cs:13500,0.0154553409665823)
--(axis cs:13400,0.0155464736744761)
--(axis cs:13300,0.0156712662428617)
--(axis cs:13200,0.0157166477292776)
--(axis cs:13100,0.0157855004072189)
--(axis cs:13000,0.015837674960494)
--(axis cs:12900,0.0159115381538868)
--(axis cs:12800,0.0159089341759682)
--(axis cs:12700,0.0159742049872875)
--(axis cs:12600,0.0160312168300152)
--(axis cs:12500,0.0161022655665874)
--(axis cs:12400,0.0161391254514456)
--(axis cs:12300,0.0162517540156841)
--(axis cs:12200,0.0163264274597168)
--(axis cs:12100,0.0163723398000002)
--(axis cs:12000,0.0163866430521011)
--(axis cs:11900,0.0164893697947264)
--(axis cs:11800,0.0165151376277208)
--(axis cs:11700,0.0165887419134378)
--(axis cs:11600,0.0167105849832296)
--(axis cs:11500,0.0167687721550465)
--(axis cs:11400,0.0168108567595482)
--(axis cs:11300,0.0169003717601299)
--(axis cs:11200,0.017009686678648)
--(axis cs:11100,0.0170697756111622)
--(axis cs:11000,0.0171493533998728)
--(axis cs:10900,0.0172552578151226)
--(axis cs:10800,0.0173345487564802)
--(axis cs:10700,0.0174223240464926)
--(axis cs:10600,0.017500139772892)
--(axis cs:10500,0.0175880901515484)
--(axis cs:10400,0.0176221840083599)
--(axis cs:10300,0.017712926492095)
--(axis cs:10200,0.0178159978240728)
--(axis cs:10100,0.0178976263850927)
--(axis cs:10000,0.0179755203425884)
--(axis cs:9900,0.0181197952479124)
--(axis cs:9800,0.0182127691805363)
--(axis cs:9700,0.0182967185974121)
--(axis cs:9600,0.0184009186923504)
--(axis cs:9500,0.0184660032391548)
--(axis cs:9400,0.0185186844319105)
--(axis cs:9300,0.0185909271240234)
--(axis cs:9200,0.0186445564031601)
--(axis cs:9100,0.0187652036547661)
--(axis cs:9000,0.0188222415745258)
--(axis cs:8900,0.0189501885324717)
--(axis cs:8800,0.0190504547208548)
--(axis cs:8700,0.019168246537447)
--(axis cs:8600,0.0192687511444092)
--(axis cs:8500,0.0194073058664799)
--(axis cs:8400,0.0194907188415527)
--(axis cs:8300,0.0195724964141846)
--(axis cs:8200,0.0196840241551399)
--(axis cs:8100,0.0198117177933455)
--(axis cs:8000,0.0199092403054237)
--(axis cs:7900,0.0200229231268167)
--(axis cs:7800,0.0201691929250956)
--(axis cs:7700,0.0202890820801258)
--(axis cs:7600,0.0203902721405029)
--(axis cs:7500,0.0205122027546167)
--(axis cs:7400,0.0206296630203724)
--(axis cs:7300,0.0207211002707481)
--(axis cs:7200,0.0208144392818213)
--(axis cs:7100,0.0209157187491655)
--(axis cs:7000,0.021091153845191)
--(axis cs:6900,0.021198557689786)
--(axis cs:6800,0.0213660709559917)
--(axis cs:6700,0.0215334333479404)
--(axis cs:6600,0.0217078104615211)
--(axis cs:6500,0.0218086428940296)
--(axis cs:6400,0.022011237218976)
--(axis cs:6300,0.02210951782763)
--(axis cs:6200,0.0222347341477871)
--(axis cs:6100,0.0223589893430471)
--(axis cs:6000,0.0225149635225534)
--(axis cs:5900,0.0226863902062178)
--(axis cs:5800,0.0228119697421789)
--(axis cs:5700,0.0228954497724771)
--(axis cs:5600,0.0230821706354618)
--(axis cs:5500,0.0232521779835224)
--(axis cs:5400,0.0234648454934359)
--(axis cs:5300,0.0236899703741074)
--(axis cs:5200,0.0239703170955181)
--(axis cs:5100,0.0241235736757517)
--(axis cs:5000,0.0243731029331684)
--(axis cs:4900,0.0246245861053467)
--(axis cs:4800,0.0248805526643991)
--(axis cs:4700,0.0251049045473337)
--(axis cs:4600,0.0253956317901611)
--(axis cs:4500,0.025603998452425)
--(axis cs:4400,0.0258862152695656)
--(axis cs:4300,0.0261315330862999)
--(axis cs:4200,0.0264453180134296)
--(axis cs:4100,0.026761507615447)
--(axis cs:4000,0.0271197073161602)
--(axis cs:3900,0.0274217370897532)
--(axis cs:3800,0.0277978181838989)
--(axis cs:3700,0.0281137228012085)
--(axis cs:3600,0.0284902099519968)
--(axis cs:3500,0.0289130918681622)
--(axis cs:3400,0.0293532349169254)
--(axis cs:3300,0.029787415638566)
--(axis cs:3200,0.0302085392177105)
--(axis cs:3100,0.0307397656142712)
--(axis cs:3000,0.0312823168933392)
--(axis cs:2900,0.0318399704992771)
--(axis cs:2800,0.0324261635541916)
--(axis cs:2700,0.0331516452133656)
--(axis cs:2600,0.0338584668934345)
--(axis cs:2500,0.0346151106059551)
--(axis cs:2400,0.0353444591164589)
--(axis cs:2300,0.0359557159245014)
--(axis cs:2200,0.0365590080618858)
--(axis cs:2100,0.0370881333947182)
--(axis cs:2000,0.0374819412827492)
--(axis cs:1900,0.0378921739757061)
--(axis cs:1800,0.0383850336074829)
--(axis cs:1700,0.0389180555939674)
--(axis cs:1600,0.0394937992095947)
--(axis cs:1500,0.0401790514588356)
--(axis cs:1400,0.0409828312695026)
--(axis cs:1300,0.0418524779379368)
--(axis cs:1200,0.0427315831184387)
--(axis cs:1100,0.0436275228857994)
--(axis cs:1000,0.044728197157383)
--(axis cs:900,0.0459869876503944)
--(axis cs:800,0.0473590902984142)
--(axis cs:700,0.0488145910203457)
--(axis cs:600,0.0502175539731979)
--(axis cs:500,0.0514817722141743)
--(axis cs:400,0.0525183789432049)
--(axis cs:300,0.0533152855932713)
--(axis cs:200,0.0538861751556396)
--(axis cs:100,0.054278127849102)
--(axis cs:0,0.0544604100286961)
--cycle;

\path [fill=blue, fill opacity=0.4, ultra thick]
(axis cs:0,0.0544335320591927)
--(axis cs:0,0.054432176053524)
--(axis cs:100,0.0542495846748352)
--(axis cs:200,0.0538603290915489)
--(axis cs:300,0.0532742850482464)
--(axis cs:400,0.0523951910436153)
--(axis cs:500,0.0512865595519543)
--(axis cs:600,0.0498741120100021)
--(axis cs:700,0.0483564101159573)
--(axis cs:800,0.0468932762742043)
--(axis cs:900,0.0455633401870728)
--(axis cs:1000,0.0443078018724918)
--(axis cs:1100,0.0432846322655678)
--(axis cs:1200,0.0424345768988132)
--(axis cs:1300,0.0415556877851486)
--(axis cs:1400,0.0406647920608521)
--(axis cs:1500,0.0398291163146496)
--(axis cs:1600,0.0391828306019306)
--(axis cs:1700,0.0385722517967224)
--(axis cs:1800,0.0380669757723808)
--(axis cs:1900,0.0376584194600582)
--(axis cs:2000,0.0372646190226078)
--(axis cs:2100,0.0367649793624878)
--(axis cs:2200,0.0362177900969982)
--(axis cs:2300,0.0356799587607384)
--(axis cs:2400,0.0350086912512779)
--(axis cs:2500,0.034287117421627)
--(axis cs:2600,0.0335360057651997)
--(axis cs:2700,0.0328628718852997)
--(axis cs:2800,0.0321836248040199)
--(axis cs:2900,0.0316130146384239)
--(axis cs:3000,0.0310813430696726)
--(axis cs:3100,0.0305554866790771)
--(axis cs:3200,0.0300310850143433)
--(axis cs:3300,0.0295623950660229)
--(axis cs:3400,0.0290660616010427)
--(axis cs:3500,0.0286244861781597)
--(axis cs:3600,0.0282619949430227)
--(axis cs:3700,0.0279204603284597)
--(axis cs:3800,0.0275640245527029)
--(axis cs:3900,0.0272417049854994)
--(axis cs:4000,0.0269234739243984)
--(axis cs:4100,0.0266087632626295)
--(axis cs:4200,0.0262746028602123)
--(axis cs:4300,0.0259784460067749)
--(axis cs:4400,0.0256840698421001)
--(axis cs:4500,0.025422353297472)
--(axis cs:4600,0.0251768156886101)
--(axis cs:4700,0.0248997993767262)
--(axis cs:4800,0.0246410723775625)
--(axis cs:4900,0.0244234297424555)
--(axis cs:5000,0.0241819582879543)
--(axis cs:5100,0.023911451920867)
--(axis cs:5200,0.023717975243926)
--(axis cs:5300,0.0235067047178745)
--(axis cs:5400,0.0233240239322186)
--(axis cs:5500,0.0231068357825279)
--(axis cs:5600,0.0229784715920687)
--(axis cs:5700,0.0227612499147654)
--(axis cs:5800,0.0225841049104929)
--(axis cs:5900,0.0224048607051373)
--(axis cs:6000,0.022297715768218)
--(axis cs:6100,0.022106122225523)
--(axis cs:6200,0.0219367016106844)
--(axis cs:6300,0.0217886604368687)
--(axis cs:6400,0.0216727647930384)
--(axis cs:6500,0.0214779749512672)
--(axis cs:6600,0.0213423296809196)
--(axis cs:6700,0.0212131068110466)
--(axis cs:6800,0.021058265119791)
--(axis cs:6900,0.0209077894687653)
--(axis cs:7000,0.0208116676658392)
--(axis cs:7100,0.0206428822129965)
--(axis cs:7200,0.0205142125487328)
--(axis cs:7300,0.0203821882605553)
--(axis cs:7400,0.0202583931386471)
--(axis cs:7500,0.0200969353318214)
--(axis cs:7600,0.0200254842638969)
--(axis cs:7700,0.0199416987597942)
--(axis cs:7800,0.0198725201189518)
--(axis cs:7900,0.0197923127561808)
--(axis cs:8000,0.019678020849824)
--(axis cs:8100,0.0195372961461544)
--(axis cs:8200,0.0194431748241186)
--(axis cs:8300,0.0193353183567524)
--(axis cs:8400,0.0192584041506052)
--(axis cs:8500,0.019168758764863)
--(axis cs:8600,0.0191126521676779)
--(axis cs:8700,0.0189914871007204)
--(axis cs:8800,0.0188591480255127)
--(axis cs:8900,0.0187256205826998)
--(axis cs:9000,0.0186511036008596)
--(axis cs:9100,0.0185457225888968)
--(axis cs:9200,0.0184227023273706)
--(axis cs:9300,0.0183546524494886)
--(axis cs:9400,0.0182809066027403)
--(axis cs:9500,0.0182144083082676)
--(axis cs:9600,0.0181195940822363)
--(axis cs:9700,0.0180124081671238)
--(axis cs:9800,0.0179086569696665)
--(axis cs:9900,0.017798975110054)
--(axis cs:10000,0.0176953189074993)
--(axis cs:10100,0.0176235102117062)
--(axis cs:10200,0.0175520293414593)
--(axis cs:10300,0.0174635890871286)
--(axis cs:10400,0.0173541065305471)
--(axis cs:10500,0.0172543525695801)
--(axis cs:10600,0.0171952247619629)
--(axis cs:10700,0.0171174947172403)
--(axis cs:10800,0.0170639995485544)
--(axis cs:10900,0.0169872753322124)
--(axis cs:11000,0.0168898832052946)
--(axis cs:11100,0.0167966745793819)
--(axis cs:11200,0.0167413782328367)
--(axis cs:11300,0.0166730396449566)
--(axis cs:11400,0.0166212692856789)
--(axis cs:11500,0.0165572986006737)
--(axis cs:11600,0.0164825115352869)
--(axis cs:11700,0.0163666065782309)
--(axis cs:11800,0.0163099095225334)
--(axis cs:11900,0.0162454601377249)
--(axis cs:12000,0.0161346904933453)
--(axis cs:12100,0.0160410888493061)
--(axis cs:12200,0.0159886367619038)
--(axis cs:12300,0.0158777721226215)
--(axis cs:12400,0.0158244129270315)
--(axis cs:12500,0.015808392316103)
--(axis cs:12600,0.0157580859959126)
--(axis cs:12700,0.0156753528863192)
--(axis cs:12800,0.0156015632674098)
--(axis cs:12900,0.0155363623052835)
--(axis cs:13000,0.0154847735539079)
--(axis cs:13100,0.0154057005420327)
--(axis cs:13200,0.0153419924899936)
--(axis cs:13300,0.0153291122987866)
--(axis cs:13400,0.0152128096669912)
--(axis cs:13500,0.0151236429810524)
--(axis cs:13600,0.015059688128531)
--(axis cs:13700,0.0150268282741308)
--(axis cs:13800,0.014957713894546)
--(axis cs:13900,0.0148977460339665)
--(axis cs:14000,0.01487170252949)
--(axis cs:14100,0.0147934667766094)
--(axis cs:14200,0.0147208524867892)
--(axis cs:14300,0.0146452272310853)
--(axis cs:14400,0.0145756239071488)
--(axis cs:14500,0.014508455991745)
--(axis cs:14600,0.0144579643383622)
--(axis cs:14700,0.014405052177608)
--(axis cs:14800,0.0143630979582667)
--(axis cs:14900,0.0143644157797098)
--(axis cs:15000,0.0142960594967008)
--(axis cs:15100,0.0142386313527822)
--(axis cs:15200,0.0141917616128922)
--(axis cs:15300,0.0141233718022704)
--(axis cs:15400,0.0140844332054257)
--(axis cs:15500,0.014009271748364)
--(axis cs:15600,0.0139885367825627)
--(axis cs:15700,0.0139292981475592)
--(axis cs:15800,0.0139255244284868)
--(axis cs:15900,0.0138300377875566)
--(axis cs:16000,0.0137888630852103)
--(axis cs:16100,0.0137423677369952)
--(axis cs:16200,0.013752356171608)
--(axis cs:16300,0.0137053225189447)
--(axis cs:16400,0.0137010253965855)
--(axis cs:16500,0.0137208076193929)
--(axis cs:16600,0.0136511018499732)
--(axis cs:16700,0.0135561199858785)
--(axis cs:16800,0.0135262375697494)
--(axis cs:16900,0.0134382331743836)
--(axis cs:17000,0.0134098026901484)
--(axis cs:17100,0.0133632188662887)
--(axis cs:17200,0.0133196245878935)
--(axis cs:17300,0.0133143421262503)
--(axis cs:17400,0.0132740456610918)
--(axis cs:17500,0.0132473865523934)
--(axis cs:17600,0.0132341384887695)
--(axis cs:17700,0.0131863597780466)
--(axis cs:17800,0.0131292343139648)
--(axis cs:17900,0.0130986217409372)
--(axis cs:18000,0.0130372466519475)
--(axis cs:18100,0.0130224227905273)
--(axis cs:18200,0.0129850385710597)
--(axis cs:18300,0.0129268644377589)
--(axis cs:18400,0.0128796249628067)
--(axis cs:18500,0.0128180403262377)
--(axis cs:18600,0.0128370337188244)
--(axis cs:18700,0.0128092914819717)
--(axis cs:18800,0.0127866473048925)
--(axis cs:18900,0.0127832889556885)
--(axis cs:19000,0.0127441491931677)
--(axis cs:19100,0.0127102853730321)
--(axis cs:19200,0.0126736154779792)
--(axis cs:19300,0.0125960726290941)
--(axis cs:19400,0.0125647252425551)
--(axis cs:19500,0.0125095723196864)
--(axis cs:19600,0.0124355554580688)
--(axis cs:19700,0.0124140903353691)
--(axis cs:19800,0.0124387741088867)
--(axis cs:19900,0.0124377254396677)
--(axis cs:20000,0.0124164577573538)
--(axis cs:20100,0.0124020669609308)
--(axis cs:20200,0.0123092858120799)
--(axis cs:20300,0.0122746285051107)
--(axis cs:20400,0.012230608612299)
--(axis cs:20500,0.012207574211061)
--(axis cs:20600,0.0122112045064569)
--(axis cs:20700,0.0121787525713444)
--(axis cs:20800,0.012142944149673)
--(axis cs:20900,0.0121135106310248)
--(axis cs:21000,0.0120790479704738)
--(axis cs:21100,0.0120518682524562)
--(axis cs:21200,0.0120136570185423)
--(axis cs:21300,0.0119550349190831)
--(axis cs:21400,0.0119206691160798)
--(axis cs:21500,0.0119044575840235)
--(axis cs:21600,0.0118471728637815)
--(axis cs:21700,0.0118621876463294)
--(axis cs:21800,0.0118607524782419)
--(axis cs:21900,0.0118111614137888)
--(axis cs:22000,0.0117671964690089)
--(axis cs:22100,0.0117557924240828)
--(axis cs:22200,0.0117327310144901)
--(axis cs:22300,0.0116840796545148)
--(axis cs:22400,0.0116962529718876)
--(axis cs:22500,0.0116653814911842)
--(axis cs:22600,0.0116074196994305)
--(axis cs:22700,0.0116332052275538)
--(axis cs:22800,0.0115885734558105)
--(axis cs:22900,0.0115231517702341)
--(axis cs:23000,0.0115125775337219)
--(axis cs:23100,0.0115283606573939)
--(axis cs:23200,0.0114797987043858)
--(axis cs:23300,0.0114748952910304)
--(axis cs:23400,0.0114502180367708)
--(axis cs:23500,0.011414622887969)
--(axis cs:23600,0.0113980295136571)
--(axis cs:23700,0.0113910268992186)
--(axis cs:23800,0.0113622667267919)
--(axis cs:23900,0.011357975192368)
--(axis cs:24000,0.0113400230184197)
--(axis cs:24100,0.0113336816430092)
--(axis cs:24200,0.0112646101042628)
--(axis cs:24300,0.0112400809302926)
--(axis cs:24400,0.0112124439328909)
--(axis cs:24500,0.0111760143190622)
--(axis cs:24600,0.0111130774021149)
--(axis cs:24700,0.0110944975167513)
--(axis cs:24800,0.0110788950696588)
--(axis cs:24900,0.0110671268776059)
--(axis cs:25000,0.0110290525481105)
--(axis cs:25100,0.011013412848115)
--(axis cs:25200,0.0109880920499563)
--(axis cs:25300,0.010956522077322)
--(axis cs:25400,0.0109062027186155)
--(axis cs:25500,0.0109069822356105)
--(axis cs:25600,0.0108440211042762)
--(axis cs:25700,0.0108280181884766)
--(axis cs:25800,0.0108275879174471)
--(axis cs:25900,0.0108341220766306)
--(axis cs:26000,0.0108281131833792)
--(axis cs:26100,0.0108047481626272)
--(axis cs:26200,0.0108080413192511)
--(axis cs:26300,0.0107443304732442)
--(axis cs:26400,0.0107106622308493)
--(axis cs:26500,0.0106398211792111)
--(axis cs:26600,0.0106361387297511)
--(axis cs:26700,0.0105820652097464)
--(axis cs:26800,0.0105976108461618)
--(axis cs:26900,0.0105530740693212)
--(axis cs:27000,0.0106028560549021)
--(axis cs:27100,0.01062788721174)
--(axis cs:27200,0.0106025440618396)
--(axis cs:27300,0.0106082381680608)
--(axis cs:27400,0.0105803441256285)
--(axis cs:27500,0.0105407144874334)
--(axis cs:27600,0.0104920500889421)
--(axis cs:27700,0.0105308536440134)
--(axis cs:27800,0.010491942986846)
--(axis cs:27900,0.0104450732469559)
--(axis cs:28000,0.0104446904733777)
--(axis cs:28100,0.0104502430185676)
--(axis cs:28200,0.0104138376191258)
--(axis cs:28300,0.0103866392746568)
--(axis cs:28400,0.0103658782318234)
--(axis cs:28500,0.0103333117440343)
--(axis cs:28600,0.0102964034304023)
--(axis cs:28700,0.0102840242907405)
--(axis cs:28800,0.0102773820981383)
--(axis cs:28900,0.0102506531402469)
--(axis cs:29000,0.0102233570069075)
--(axis cs:29100,0.0102275386452675)
--(axis cs:29200,0.0102102616801858)
--(axis cs:29300,0.0102035067975521)
--(axis cs:29400,0.0101978303864598)
--(axis cs:29500,0.0102004054933786)
--(axis cs:29600,0.0101241115480661)
--(axis cs:29700,0.0101123806089163)
--(axis cs:29800,0.0100692752748728)
--(axis cs:29900,0.0100580947473645)
--(axis cs:30000,0.00999717693775892)
--(axis cs:30100,0.0100271226838231)
--(axis cs:30200,0.0100125409662724)
--(axis cs:30300,0.00998885650187731)
--(axis cs:30400,0.0099664218723774)
--(axis cs:30500,0.00996250100433826)
--(axis cs:30600,0.00992115773260593)
--(axis cs:30700,0.00990260019898415)
--(axis cs:30800,0.00987290777266026)
--(axis cs:30900,0.00985742546617985)
--(axis cs:31000,0.00986372958868742)
--(axis cs:31100,0.00986238848417997)
--(axis cs:31200,0.00987695250660181)
--(axis cs:31300,0.00990858115255833)
--(axis cs:31400,0.00989713333547115)
--(axis cs:31500,0.00988187827169895)
--(axis cs:31600,0.00985479354858398)
--(axis cs:31700,0.00983131490647793)
--(axis cs:31800,0.0098100658506155)
--(axis cs:31900,0.00980119686573744)
--(axis cs:32000,0.0098111480474472)
--(axis cs:32100,0.00981569290161133)
--(axis cs:32200,0.00981852784752846)
--(axis cs:32300,0.00978679116815329)
--(axis cs:32400,0.00975015573203564)
--(axis cs:32500,0.009734439663589)
--(axis cs:32600,0.00969409942626953)
--(axis cs:32700,0.009674072265625)
--(axis cs:32800,0.00960033945739269)
--(axis cs:32900,0.00961164012551308)
--(axis cs:33000,0.00957019906491041)
--(axis cs:33100,0.0095888739451766)
--(axis cs:33200,0.00958347320556641)
--(axis cs:33300,0.00957717932760715)
--(axis cs:33400,0.0095664020627737)
--(axis cs:33500,0.00954713858664036)
--(axis cs:33600,0.0095362663269043)
--(axis cs:33700,0.00953149795532227)
--(axis cs:33800,0.0095067024230957)
--(axis cs:33900,0.00947237014770508)
--(axis cs:34000,0.00947550870478153)
--(axis cs:34100,0.00946750678122044)
--(axis cs:34200,0.00943441409617662)
--(axis cs:34300,0.0094276424497366)
--(axis cs:34400,0.00939884223043919)
--(axis cs:34500,0.00938577670603991)
--(axis cs:34600,0.00939655303955078)
--(axis cs:34700,0.00938138924539089)
--(axis cs:34800,0.00937452353537083)
--(axis cs:34900,0.00935935974121094)
--(axis cs:35000,0.0093864444643259)
--(axis cs:35100,0.0093670841306448)
--(axis cs:35200,0.00936946831643581)
--(axis cs:35300,0.00936307944357395)
--(axis cs:35400,0.00935020484030247)
--(axis cs:35500,0.00930281262844801)
--(axis cs:35600,0.0093226432800293)
--(axis cs:35700,0.00929911714047194)
--(axis cs:35800,0.00930395163595676)
--(axis cs:35900,0.00928819738328457)
--(axis cs:36000,0.00925733521580696)
--(axis cs:36100,0.00925680436193943)
--(axis cs:36200,0.00926316436380148)
--(axis cs:36300,0.00921400170773268)
--(axis cs:36400,0.00921938940882683)
--(axis cs:36500,0.00924787390977144)
--(axis cs:36600,0.00920475646853447)
--(axis cs:36700,0.0091787064447999)
--(axis cs:36800,0.00921904947608709)
--(axis cs:36900,0.00919449981302023)
--(axis cs:37000,0.00914567429572344)
--(axis cs:37100,0.00913190841674805)
--(axis cs:37200,0.00915038865059614)
--(axis cs:37300,0.00911509525030851)
--(axis cs:37400,0.00910098385065794)
--(axis cs:37500,0.00910989940166473)
--(axis cs:37600,0.00913388933986425)
--(axis cs:37700,0.00909369345754385)
--(axis cs:37800,0.00910383928567171)
--(axis cs:37900,0.0091019831597805)
--(axis cs:38000,0.00908968411386013)
--(axis cs:38100,0.00904272776097059)
--(axis cs:38200,0.00901900418102741)
--(axis cs:38300,0.00901689566671848)
--(axis cs:38400,0.00899532716721296)
--(axis cs:38500,0.00898173451423645)
--(axis cs:38600,0.00900714099407196)
--(axis cs:38700,0.00908674672245979)
--(axis cs:38800,0.00906237680464983)
--(axis cs:38900,0.00905407965183258)
--(axis cs:39000,0.00903932470828295)
--(axis cs:39100,0.00901929475367069)
--(axis cs:39200,0.00893999356776476)
--(axis cs:39300,0.00893727131187916)
--(axis cs:39400,0.0089572612196207)
--(axis cs:39500,0.00893682986497879)
--(axis cs:39600,0.00891405995935202)
--(axis cs:39700,0.00891833938658237)
--(axis cs:39800,0.00891280639916658)
--(axis cs:39900,0.00888894032686949)
--(axis cs:40000,0.00889360066503286)
--(axis cs:40100,0.00888642575591803)
--(axis cs:40200,0.00887435674667358)
--(axis cs:40300,0.00884527992457151)
--(axis cs:40400,0.00882230885326862)
--(axis cs:40500,0.0088125579059124)
--(axis cs:40600,0.00879974383860826)
--(axis cs:40700,0.00878274161368608)
--(axis cs:40800,0.00874852947890759)
--(axis cs:40900,0.00875944271683693)
--(axis cs:41000,0.00874897837638855)
--(axis cs:41100,0.00875204335898161)
--(axis cs:41200,0.00873498991131783)
--(axis cs:41300,0.00874389242380857)
--(axis cs:41400,0.00873820669949055)
--(axis cs:41500,0.00874119997024536)
--(axis cs:41600,0.00873902998864651)
--(axis cs:41700,0.00873311888426542)
--(axis cs:41800,0.00873902998864651)
--(axis cs:41900,0.00871986616402864)
--(axis cs:42000,0.00870660506188869)
--(axis cs:42100,0.00867892988026142)
--(axis cs:42200,0.008676677942276)
--(axis cs:42300,0.0086832819506526)
--(axis cs:42400,0.00870413146913052)
--(axis cs:42500,0.00868688337504864)
--(axis cs:42600,0.00868965871632099)
--(axis cs:42700,0.00867720320820808)
--(axis cs:42800,0.00864903908222914)
--(axis cs:42900,0.00860601384192705)
--(axis cs:43000,0.00859019998461008)
--(axis cs:43100,0.00861037988215685)
--(axis cs:43200,0.00862129125744104)
--(axis cs:43300,0.00861293915659189)
--(axis cs:43400,0.00863310135900974)
--(axis cs:43500,0.00862407591193914)
--(axis cs:43600,0.0085749039426446)
--(axis cs:43700,0.00853749923408031)
--(axis cs:43800,0.00850390363484621)
--(axis cs:43900,0.0084768533706665)
--(axis cs:44000,0.00848947465419769)
--(axis cs:44100,0.00849755853414536)
--(axis cs:44200,0.00852383859455585)
--(axis cs:44300,0.00856842193752527)
--(axis cs:44400,0.00856337137520313)
--(axis cs:44500,0.00858696084469557)
--(axis cs:44600,0.00858033075928688)
--(axis cs:44700,0.00856744311749935)
--(axis cs:44800,0.00852421671152115)
--(axis cs:44900,0.00850964430719614)
--(axis cs:44900,0.00981760025024414)
--(axis cs:44900,0.00981760025024414)
--(axis cs:44800,0.00981760025024414)
--(axis cs:44700,0.00981760025024414)
--(axis cs:44600,0.00981760025024414)
--(axis cs:44500,0.00981760025024414)
--(axis cs:44400,0.00981760025024414)
--(axis cs:44300,0.00981760025024414)
--(axis cs:44200,0.00981760025024414)
--(axis cs:44100,0.00981760025024414)
--(axis cs:44000,0.00981760025024414)
--(axis cs:43900,0.00981760025024414)
--(axis cs:43800,0.00981760025024414)
--(axis cs:43700,0.00981760025024414)
--(axis cs:43600,0.00981760025024414)
--(axis cs:43500,0.00981760025024414)
--(axis cs:43400,0.00981700047850609)
--(axis cs:43300,0.00981760025024414)
--(axis cs:43200,0.00981760025024414)
--(axis cs:43100,0.00981760025024414)
--(axis cs:43000,0.00981760025024414)
--(axis cs:42900,0.00981760025024414)
--(axis cs:42800,0.00981454085558653)
--(axis cs:42700,0.00981021858751774)
--(axis cs:42600,0.00980831682682037)
--(axis cs:42500,0.00980873964726925)
--(axis cs:42400,0.00980611518025398)
--(axis cs:42300,0.00980929005891085)
--(axis cs:42200,0.00981029868125916)
--(axis cs:42100,0.00980995409190655)
--(axis cs:42000,0.00980573892593384)
--(axis cs:41900,0.00980373192578554)
--(axis cs:41800,0.00980084389448166)
--(axis cs:41700,0.00980173330754042)
--(axis cs:41600,0.00980084389448166)
--(axis cs:41500,0.00980051793158054)
--(axis cs:41400,0.00980096682906151)
--(axis cs:41300,0.00980011280626059)
--(axis cs:41200,0.00980145111680031)
--(axis cs:41100,0.00979889277368784)
--(axis cs:41000,0.00979935191571712)
--(axis cs:40900,0.00979778729379177)
--(axis cs:40800,0.0097994189709425)
--(axis cs:40700,0.00979432556778193)
--(axis cs:40600,0.00979181844741106)
--(axis cs:40500,0.00978993996977806)
--(axis cs:40400,0.0097885187715292)
--(axis cs:40300,0.00978519301861525)
--(axis cs:40200,0.00978103838860989)
--(axis cs:40100,0.00977933313697577)
--(axis cs:40000,0.00977832544595003)
--(axis cs:39900,0.00977897923439741)
--(axis cs:39800,0.00977565068751574)
--(axis cs:39700,0.00977488607168198)
--(axis cs:39600,0.00977547746151686)
--(axis cs:39500,0.00977235287427902)
--(axis cs:39400,0.00976959615945816)
--(axis cs:39300,0.00977229326963425)
--(axis cs:39200,0.00977192353457212)
--(axis cs:39100,0.00976154021918774)
--(axis cs:39000,0.00975905824452639)
--(axis cs:38900,0.00975727289915085)
--(axis cs:38800,0.00975628662854433)
--(axis cs:38700,0.00975347124040127)
--(axis cs:38600,0.00976307690143585)
--(axis cs:38500,0.00976635701954365)
--(axis cs:38400,0.00976459216326475)
--(axis cs:38300,0.00976184196770191)
--(axis cs:38200,0.00976157747209072)
--(axis cs:38100,0.00975864287465811)
--(axis cs:38000,0.0097531396895647)
--(axis cs:37900,0.00975177623331547)
--(axis cs:37800,0.00975157413631678)
--(axis cs:37700,0.00975269172340631)
--(axis cs:37600,0.00974841695278883)
--(axis cs:37500,0.00975091755390167)
--(axis cs:37400,0.0097518851980567)
--(axis cs:37300,0.00975036341696978)
--(axis cs:37200,0.00974679458886385)
--(axis cs:37100,0.00974861718714237)
--(axis cs:37000,0.00974724907428026)
--(axis cs:36900,0.0097429296001792)
--(axis cs:36800,0.00974114146083593)
--(axis cs:36700,0.00974422600120306)
--(axis cs:36600,0.00974214635789394)
--(axis cs:36500,0.00973946321755648)
--(axis cs:36400,0.00974111817777157)
--(axis cs:36300,0.00974148418754339)
--(axis cs:36200,0.00973879639059305)
--(axis cs:36100,0.00973905250430107)
--(axis cs:36000,0.00973903015255928)
--(axis cs:35900,0.00973811373114586)
--(axis cs:35800,0.00973799359053373)
--(axis cs:35700,0.00973800290375948)
--(axis cs:35600,0.00973809510469437)
--(axis cs:35500,0.00973799359053373)
--(axis cs:35400,0.00973860640078783)
--(axis cs:35300,0.00973900593817234)
--(axis cs:35200,0.00973924621939659)
--(axis cs:35100,0.00973915308713913)
--(axis cs:35000,0.00974002201110125)
--(axis cs:34900,0.00973888020962477)
--(axis cs:34800,0.00973945483565331)
--(axis cs:34700,0.00973976869136095)
--(axis cs:34600,0.00974058546125889)
--(axis cs:34500,0.00973998662084341)
--(axis cs:34400,0.00974072329699993)
--(axis cs:34300,0.00974283181130886)
--(axis cs:34200,0.0097479997202754)
--(axis cs:34100,0.0097534628584981)
--(axis cs:34000,0.00976626947522163)
--(axis cs:33900,0.00976164545863867)
--(axis cs:33800,0.00976221822202206)
--(axis cs:33700,0.00976445339620113)
--(axis cs:33600,0.00976430624723434)
--(axis cs:33500,0.00977353285998106)
--(axis cs:33400,0.00977737735956907)
--(axis cs:33300,0.00977974198758602)
--(axis cs:33200,0.00977542996406555)
--(axis cs:33100,0.00978298578411341)
--(axis cs:33000,0.00978099834173918)
--(axis cs:32900,0.00978724099695683)
--(axis cs:32800,0.00978576205670834)
--(axis cs:32700,0.00978967826813459)
--(axis cs:32600,0.00979689229279757)
--(axis cs:32500,0.00980173423886299)
--(axis cs:32400,0.00980805233120918)
--(axis cs:32300,0.00981394853442907)
--(axis cs:32200,0.00982570089399815)
--(axis cs:32100,0.00983877014368773)
--(axis cs:32000,0.00983702205121517)
--(axis cs:31900,0.00985331833362579)
--(axis cs:31800,0.00988580379635096)
--(axis cs:31700,0.0099287535995245)
--(axis cs:31600,0.00991843268275261)
--(axis cs:31500,0.00996512826532125)
--(axis cs:31400,0.00995264388620853)
--(axis cs:31300,0.00996849779039621)
--(axis cs:31200,0.009929527528584)
--(axis cs:31100,0.00993061345070601)
--(axis cs:31000,0.00988692883402109)
--(axis cs:30900,0.0099186897277832)
--(axis cs:30800,0.00994133017957211)
--(axis cs:30700,0.00996723212301731)
--(axis cs:30600,0.00999963656067848)
--(axis cs:30500,0.0100844949483871)
--(axis cs:30400,0.0100713726133108)
--(axis cs:30300,0.0100850341841578)
--(axis cs:30200,0.0100639341399074)
--(axis cs:30100,0.0101233161985874)
--(axis cs:30000,0.0100917937234044)
--(axis cs:29900,0.0101124988868833)
--(axis cs:29800,0.0101455114781857)
--(axis cs:29700,0.0101354792714119)
--(axis cs:29600,0.0101544018834829)
--(axis cs:29500,0.0102128060534596)
--(axis cs:29400,0.0102396458387375)
--(axis cs:29300,0.0102354511618614)
--(axis cs:29200,0.0102814668789506)
--(axis cs:29100,0.0102936252951622)
--(axis cs:29000,0.010263666510582)
--(axis cs:28900,0.0102819548919797)
--(axis cs:28800,0.0103355403989553)
--(axis cs:28700,0.010355013422668)
--(axis cs:28600,0.0104009350761771)
--(axis cs:28500,0.0104560265317559)
--(axis cs:28400,0.0104374885559082)
--(axis cs:28300,0.0104182744398713)
--(axis cs:28200,0.0104532698169351)
--(axis cs:28100,0.0104832882061601)
--(axis cs:28000,0.0104785915464163)
--(axis cs:27900,0.0105533748865128)
--(axis cs:27800,0.0105800963938236)
--(axis cs:27700,0.0106152836233377)
--(axis cs:27600,0.0106422612443566)
--(axis cs:27500,0.0107002258300781)
--(axis cs:27400,0.0107155852019787)
--(axis cs:27300,0.0107455253601074)
--(axis cs:27200,0.0107453344389796)
--(axis cs:27100,0.0107482140883803)
--(axis cs:27000,0.0107669522985816)
--(axis cs:26900,0.010798410512507)
--(axis cs:26800,0.0107461269944906)
--(axis cs:26700,0.0107617303729057)
--(axis cs:26600,0.0107875196263194)
--(axis cs:26500,0.0108062783256173)
--(axis cs:26400,0.01082525216043)
--(axis cs:26300,0.0108385263010859)
--(axis cs:26200,0.010894107632339)
--(axis cs:26100,0.0109390905126929)
--(axis cs:26000,0.0109749333932996)
--(axis cs:25900,0.0109571469947696)
--(axis cs:25800,0.0109552219510078)
--(axis cs:25700,0.0109237283468246)
--(axis cs:25600,0.0109124695882201)
--(axis cs:25500,0.0109326867386699)
--(axis cs:25400,0.010975981131196)
--(axis cs:25300,0.0110233183950186)
--(axis cs:25200,0.0110782776027918)
--(axis cs:25100,0.0111314402893186)
--(axis cs:25000,0.0111259380355477)
--(axis cs:24900,0.0111210821196437)
--(axis cs:24800,0.0111306188628078)
--(axis cs:24700,0.0111324712634087)
--(axis cs:24600,0.0111339837312698)
--(axis cs:24500,0.0111861554905772)
--(axis cs:24400,0.0112485243007541)
--(axis cs:24300,0.0112746423110366)
--(axis cs:24200,0.0113095743581653)
--(axis cs:24100,0.0113524440675974)
--(axis cs:24000,0.0113473823294044)
--(axis cs:23900,0.0113813653588295)
--(axis cs:23800,0.0114620383828878)
--(axis cs:23700,0.0114919431507587)
--(axis cs:23600,0.0115079907700419)
--(axis cs:23500,0.0115275271236897)
--(axis cs:23400,0.0115677919238806)
--(axis cs:23300,0.0115403588861227)
--(axis cs:23200,0.0115270856767893)
--(axis cs:23100,0.0115502355620265)
--(axis cs:23000,0.0115682603791356)
--(axis cs:22900,0.0115883247926831)
--(axis cs:22800,0.0116338850930333)
--(axis cs:22700,0.0116669228300452)
--(axis cs:22600,0.0116993905976415)
--(axis cs:22500,0.011736324056983)
--(axis cs:22400,0.0117433462291956)
--(axis cs:22300,0.0117527963593602)
--(axis cs:22200,0.0117894168943167)
--(axis cs:22100,0.0118451043963432)
--(axis cs:22000,0.0118656335398555)
--(axis cs:21900,0.011854974552989)
--(axis cs:21800,0.011913432739675)
--(axis cs:21700,0.01194451097399)
--(axis cs:21600,0.011992777697742)
--(axis cs:21500,0.0120187178254128)
--(axis cs:21400,0.0121123054996133)
--(axis cs:21300,0.012103752233088)
--(axis cs:21200,0.0120978355407715)
--(axis cs:21100,0.0120992418378592)
--(axis cs:21000,0.0121458228677511)
--(axis cs:20900,0.0121409082785249)
--(axis cs:20800,0.0121867768466473)
--(axis cs:20700,0.0122829936444759)
--(axis cs:20600,0.0122548015788198)
--(axis cs:20500,0.0122761065140367)
--(axis cs:20400,0.0123125072568655)
--(axis cs:20300,0.0123425479978323)
--(axis cs:20200,0.0123398872092366)
--(axis cs:20100,0.0124297142028809)
--(axis cs:20000,0.0124724106863141)
--(axis cs:19900,0.0124943275004625)
--(axis cs:19800,0.0125038232654333)
--(axis cs:19700,0.0125264618545771)
--(axis cs:19600,0.0125227924436331)
--(axis cs:19500,0.0125947585329413)
--(axis cs:19400,0.0126494700089097)
--(axis cs:19300,0.0127182956784964)
--(axis cs:19200,0.0127710346132517)
--(axis cs:19100,0.0128004103899002)
--(axis cs:19000,0.0128087922930717)
--(axis cs:18900,0.0128120575100183)
--(axis cs:18800,0.01285320520401)
--(axis cs:18700,0.01288185082376)
--(axis cs:18600,0.0129249505698681)
--(axis cs:18500,0.0129923932254314)
--(axis cs:18400,0.0130294803529978)
--(axis cs:18300,0.0130600640550256)
--(axis cs:18200,0.0130613837391138)
--(axis cs:18100,0.0131297605112195)
--(axis cs:18000,0.0131539581343532)
--(axis cs:17900,0.0131791587918997)
--(axis cs:17800,0.0132534941658378)
--(axis cs:17700,0.0133034186437726)
--(axis cs:17600,0.0133366109803319)
--(axis cs:17500,0.0133627345785499)
--(axis cs:17400,0.0133653841912746)
--(axis cs:17300,0.0134083516895771)
--(axis cs:17200,0.013502337038517)
--(axis cs:17100,0.0134558184072375)
--(axis cs:17000,0.0135493315756321)
--(axis cs:16900,0.0136361690238118)
--(axis cs:16800,0.0136342803016305)
--(axis cs:16700,0.0136768454685807)
--(axis cs:16600,0.0137632852420211)
--(axis cs:16500,0.0137732746079564)
--(axis cs:16400,0.0138300899416208)
--(axis cs:16300,0.0138827264308929)
--(axis cs:16200,0.0139306541532278)
--(axis cs:16100,0.0139421466737986)
--(axis cs:16000,0.0139581207185984)
--(axis cs:15900,0.0139944553375244)
--(axis cs:15800,0.0140493391081691)
--(axis cs:15700,0.0140560511499643)
--(axis cs:15600,0.0141534069553018)
--(axis cs:15500,0.0142648192122579)
--(axis cs:15400,0.0142949419096112)
--(axis cs:15300,0.014360242523253)
--(axis cs:15200,0.0144058167934418)
--(axis cs:15100,0.0144036412239075)
--(axis cs:15000,0.0144205363467336)
--(axis cs:14900,0.0144539996981621)
--(axis cs:14800,0.0144898723810911)
--(axis cs:14700,0.0145029770210385)
--(axis cs:14600,0.0145877758041024)
--(axis cs:14500,0.0146119892597198)
--(axis cs:14400,0.014730310998857)
--(axis cs:14300,0.0148157123476267)
--(axis cs:14200,0.0148933883756399)
--(axis cs:14100,0.0149639127776027)
--(axis cs:14000,0.0150173390284181)
--(axis cs:13900,0.0150119299069047)
--(axis cs:13800,0.0150462435558438)
--(axis cs:13700,0.0151396095752716)
--(axis cs:13600,0.015181771479547)
--(axis cs:13500,0.0152234509587288)
--(axis cs:13400,0.0153436157852411)
--(axis cs:13300,0.0154324052855372)
--(axis cs:13200,0.0154607770964503)
--(axis cs:13100,0.0155480857938528)
--(axis cs:13000,0.0156178520992398)
--(axis cs:12900,0.0156608354300261)
--(axis cs:12800,0.0156801957637072)
--(axis cs:12700,0.0157846454530954)
--(axis cs:12600,0.0158737972378731)
--(axis cs:12500,0.0159679260104895)
--(axis cs:12400,0.0160554368048906)
--(axis cs:12300,0.0161532387137413)
--(axis cs:12200,0.0161912459880114)
--(axis cs:12100,0.0162125881761312)
--(axis cs:12000,0.0162795092910528)
--(axis cs:11900,0.0163390878587961)
--(axis cs:11800,0.0164129436016083)
--(axis cs:11700,0.0164711978286505)
--(axis cs:11600,0.016582490876317)
--(axis cs:11500,0.0166755206882954)
--(axis cs:11400,0.0167262069880962)
--(axis cs:11300,0.0167422741651535)
--(axis cs:11200,0.0168737974017859)
--(axis cs:11100,0.0169166661798954)
--(axis cs:11000,0.016962630674243)
--(axis cs:10900,0.0170543827116489)
--(axis cs:10800,0.0171628128737211)
--(axis cs:10700,0.0172284189611673)
--(axis cs:10600,0.0173048358410597)
--(axis cs:10500,0.0174034386873245)
--(axis cs:10400,0.0174682922661304)
--(axis cs:10300,0.017548430711031)
--(axis cs:10200,0.0176105983555317)
--(axis cs:10100,0.0177533254027367)
--(axis cs:10000,0.0178423877805471)
--(axis cs:9900,0.0179459564387798)
--(axis cs:9800,0.0180930253118277)
--(axis cs:9700,0.0181863345205784)
--(axis cs:9600,0.0182542745023966)
--(axis cs:9500,0.0183899328112602)
--(axis cs:9400,0.0184973832219839)
--(axis cs:9300,0.0185294654220343)
--(axis cs:9200,0.0186066273599863)
--(axis cs:9100,0.0187499988824129)
--(axis cs:9000,0.0188134498894215)
--(axis cs:8900,0.0189013760536909)
--(axis cs:8800,0.0189830996096134)
--(axis cs:8700,0.0191060844808817)
--(axis cs:8600,0.0191610809415579)
--(axis cs:8500,0.0192514453083277)
--(axis cs:8400,0.0193099640309811)
--(axis cs:8300,0.0194547735154629)
--(axis cs:8200,0.0195495467633009)
--(axis cs:8100,0.0196616724133492)
--(axis cs:8000,0.0197633597999811)
--(axis cs:7900,0.0198562163859606)
--(axis cs:7800,0.0199846141040325)
--(axis cs:7700,0.0200949162244797)
--(axis cs:7600,0.0201998911798)
--(axis cs:7500,0.0203391071408987)
--(axis cs:7400,0.0204577445983887)
--(axis cs:7300,0.020592775195837)
--(axis cs:7200,0.02069091796875)
--(axis cs:7100,0.0207929126918316)
--(axis cs:7000,0.020945405587554)
--(axis cs:6900,0.0211072918027639)
--(axis cs:6800,0.0212579146027565)
--(axis cs:6700,0.0214105136692524)
--(axis cs:6600,0.0215893276035786)
--(axis cs:6500,0.0217418186366558)
--(axis cs:6400,0.02189726755023)
--(axis cs:6300,0.0220845192670822)
--(axis cs:6200,0.0222288463264704)
--(axis cs:6100,0.0224009975790977)
--(axis cs:6000,0.0225120577961206)
--(axis cs:5900,0.0227011889219284)
--(axis cs:5800,0.0228366442024708)
--(axis cs:5700,0.0229272488504648)
--(axis cs:5600,0.0230689588934183)
--(axis cs:5500,0.0232525579631329)
--(axis cs:5400,0.0234100855886936)
--(axis cs:5300,0.0236716121435165)
--(axis cs:5200,0.0239564217627048)
--(axis cs:5100,0.0241363178938627)
--(axis cs:5000,0.0244102627038956)
--(axis cs:4900,0.0246717222034931)
--(axis cs:4800,0.0248761884868145)
--(axis cs:4700,0.0251153223216534)
--(axis cs:4600,0.025427620857954)
--(axis cs:4500,0.0256318561732769)
--(axis cs:4400,0.0259376652538776)
--(axis cs:4300,0.0261977445334196)
--(axis cs:4200,0.026547908782959)
--(axis cs:4100,0.0268498193472624)
--(axis cs:4000,0.0272371061146259)
--(axis cs:3900,0.0275289546698332)
--(axis cs:3800,0.0279086977243423)
--(axis cs:3700,0.0282009057700634)
--(axis cs:3600,0.0285837352275848)
--(axis cs:3500,0.0289764702320099)
--(axis cs:3400,0.0294577870517969)
--(axis cs:3300,0.0298750400543213)
--(axis cs:3200,0.0303155612200499)
--(axis cs:3100,0.0307642351835966)
--(axis cs:3000,0.0312351882457733)
--(axis cs:2900,0.031732052564621)
--(axis cs:2800,0.0323612876236439)
--(axis cs:2700,0.0331559777259827)
--(axis cs:2600,0.033890638500452)
--(axis cs:2500,0.0346561186015606)
--(axis cs:2400,0.0353867933154106)
--(axis cs:2300,0.0359896793961525)
--(axis cs:2200,0.0364970974624157)
--(axis cs:2100,0.0370430052280426)
--(axis cs:2000,0.0374748520553112)
--(axis cs:1900,0.0378871001303196)
--(axis cs:1800,0.0384030789136887)
--(axis cs:1700,0.0389373302459717)
--(axis cs:1600,0.0395270250737667)
--(axis cs:1500,0.0402104370296001)
--(axis cs:1400,0.0409765765070915)
--(axis cs:1300,0.0417912527918816)
--(axis cs:1200,0.0426510572433472)
--(axis cs:1100,0.0435818210244179)
--(axis cs:1000,0.0446990989148617)
--(axis cs:900,0.0459758415818214)
--(axis cs:800,0.0473586320877075)
--(axis cs:700,0.0488137416541576)
--(axis cs:600,0.0502007082104683)
--(axis cs:500,0.0514562092721462)
--(axis cs:400,0.0525052286684513)
--(axis cs:300,0.0533110685646534)
--(axis cs:200,0.0538739748299122)
--(axis cs:100,0.0542582049965858)
--(axis cs:0,0.0544335320591927)
--cycle;

\path [fill=green!50.1960784313725!black, fill opacity=0.4, ultra thick]
(axis cs:0,0.0637036859989166)
--(axis cs:0,0.0636349767446518)
--(axis cs:100,0.0615603215992451)
--(axis cs:200,0.0590961202979088)
--(axis cs:300,0.0565544627606869)
--(axis cs:400,0.0542185232043266)
--(axis cs:500,0.0527046918869019)
--(axis cs:600,0.052056085318327)
--(axis cs:700,0.0517884381115437)
--(axis cs:800,0.0516378432512283)
--(axis cs:900,0.051479309797287)
--(axis cs:1000,0.051042702049017)
--(axis cs:1100,0.0501771159470081)
--(axis cs:1200,0.0489348508417606)
--(axis cs:1300,0.0474495440721512)
--(axis cs:1400,0.0455842725932598)
--(axis cs:1500,0.0437570475041866)
--(axis cs:1600,0.0418655760586262)
--(axis cs:1700,0.0397585742175579)
--(axis cs:1800,0.0369190648198128)
--(axis cs:1900,0.033805537968874)
--(axis cs:2000,0.030795119702816)
--(axis cs:2100,0.0282053463160992)
--(axis cs:2200,0.0261255018413067)
--(axis cs:2300,0.0245132707059383)
--(axis cs:2400,0.0232763905078173)
--(axis cs:2500,0.0221428163349628)
--(axis cs:2600,0.0210395399481058)
--(axis cs:2700,0.0200916286557913)
--(axis cs:2800,0.0192982442677021)
--(axis cs:2900,0.0186894182115793)
--(axis cs:3000,0.018135953694582)
--(axis cs:3100,0.0176824033260345)
--(axis cs:3200,0.017232982441783)
--(axis cs:3300,0.0168337393552065)
--(axis cs:3400,0.0164223331958055)
--(axis cs:3500,0.0160551816225052)
--(axis cs:3600,0.015727449208498)
--(axis cs:3700,0.0153868198394775)
--(axis cs:3800,0.0150002241134644)
--(axis cs:3900,0.0146481990814209)
--(axis cs:4000,0.0142989158630371)
--(axis cs:4100,0.0139313936233521)
--(axis cs:4200,0.0136183062568307)
--(axis cs:4300,0.0133459279313684)
--(axis cs:4400,0.0131141152232885)
--(axis cs:4500,0.0129212141036987)
--(axis cs:4600,0.0127708734944463)
--(axis cs:4700,0.0126023534685373)
--(axis cs:4800,0.0124559877440333)
--(axis cs:4900,0.0122753251343966)
--(axis cs:5000,0.0121081974357367)
--(axis cs:5100,0.011993714608252)
--(axis cs:5200,0.0118730310350657)
--(axis cs:5300,0.0117479087784886)
--(axis cs:5400,0.0116108180955052)
--(axis cs:5500,0.0114802848547697)
--(axis cs:5600,0.0113481674343348)
--(axis cs:5700,0.0112878559157252)
--(axis cs:5800,0.0111934188753366)
--(axis cs:5900,0.0111123975366354)
--(axis cs:6000,0.0110433055087924)
--(axis cs:6100,0.0109653947874904)
--(axis cs:6200,0.0108279697597027)
--(axis cs:6300,0.0107330400496721)
--(axis cs:6400,0.0106290513649583)
--(axis cs:6500,0.0105752069503069)
--(axis cs:6600,0.0104993423447013)
--(axis cs:6700,0.0103827137500048)
--(axis cs:6800,0.0103110717609525)
--(axis cs:6900,0.0102437743917108)
--(axis cs:7000,0.0101909032091498)
--(axis cs:7100,0.0101536978036165)
--(axis cs:7200,0.0100868744775653)
--(axis cs:7300,0.0100052990019321)
--(axis cs:7400,0.00998483877629042)
--(axis cs:7500,0.0099245086312294)
--(axis cs:7600,0.00982762966305017)
--(axis cs:7700,0.00982656609266996)
--(axis cs:7800,0.00977120362222195)
--(axis cs:7900,0.00968469679355621)
--(axis cs:8000,0.00964463874697685)
--(axis cs:8100,0.00961857009679079)
--(axis cs:8200,0.0095398910343647)
--(axis cs:8300,0.00952783972024918)
--(axis cs:8400,0.0094585120677948)
--(axis cs:8500,0.00942463893443346)
--(axis cs:8600,0.00938692130148411)
--(axis cs:8700,0.00931196194142103)
--(axis cs:8800,0.00928010977804661)
--(axis cs:8900,0.00923133175820112)
--(axis cs:9000,0.00919395219534636)
--(axis cs:9100,0.00914883613586426)
--(axis cs:9200,0.00909476261585951)
--(axis cs:9300,0.00905415881425142)
--(axis cs:9400,0.00900821667164564)
--(axis cs:9500,0.00897607766091824)
--(axis cs:9600,0.00891470909118652)
--(axis cs:9700,0.00887002982199192)
--(axis cs:9800,0.00882124807685614)
--(axis cs:9900,0.00877401046454906)
--(axis cs:10000,0.00874427333474159)
--(axis cs:10100,0.00871048588305712)
--(axis cs:10200,0.00866400729864836)
--(axis cs:10300,0.00862484890967607)
--(axis cs:10400,0.00858969707041979)
--(axis cs:10500,0.00855994131416082)
--(axis cs:10600,0.00851969514042139)
--(axis cs:10700,0.00850529689341784)
--(axis cs:10800,0.00846571940928698)
--(axis cs:10900,0.00847913883626461)
--(axis cs:11000,0.00841078720986843)
--(axis cs:11100,0.00840597786009312)
--(axis cs:11200,0.00838897936046124)
--(axis cs:11300,0.00835347175598145)
--(axis cs:11400,0.00828185118734837)
--(axis cs:11500,0.00827784556895494)
--(axis cs:11600,0.0082249641418457)
--(axis cs:11700,0.00817920360714197)
--(axis cs:11800,0.00819506403058767)
--(axis cs:11900,0.00818183459341526)
--(axis cs:12000,0.00817676912993193)
--(axis cs:12100,0.00812316592782736)
--(axis cs:12200,0.00811531767249107)
--(axis cs:12300,0.00805472396314144)
--(axis cs:12400,0.00801105424761772)
--(axis cs:12500,0.00797216966748238)
--(axis cs:12600,0.00797000527381897)
--(axis cs:12700,0.00795022211968899)
--(axis cs:12800,0.00794303510338068)
--(axis cs:12900,0.00794792175292969)
--(axis cs:13000,0.00792036391794682)
--(axis cs:13100,0.00788555666804314)
--(axis cs:13200,0.00785708427429199)
--(axis cs:13300,0.00781445484608412)
--(axis cs:13400,0.00776035943999887)
--(axis cs:13500,0.00774708157405257)
--(axis cs:13600,0.00775386998429894)
--(axis cs:13700,0.0077319392003119)
--(axis cs:13800,0.00771483406424522)
--(axis cs:13900,0.00768750580027699)
--(axis cs:14000,0.00769880134612322)
--(axis cs:14100,0.00765533465892076)
--(axis cs:14200,0.00760951219126582)
--(axis cs:14300,0.00758652854710817)
--(axis cs:14400,0.00756483059376478)
--(axis cs:14500,0.00749981077387929)
--(axis cs:14600,0.00749107683077455)
--(axis cs:14700,0.00751647725701332)
--(axis cs:14800,0.0074959802441299)
--(axis cs:14900,0.00748709868639708)
--(axis cs:15000,0.00748205184936523)
--(axis cs:15100,0.00743943825364113)
--(axis cs:15200,0.00739577645435929)
--(axis cs:15300,0.00737026613205671)
--(axis cs:15400,0.00732450466603041)
--(axis cs:15500,0.00732960691675544)
--(axis cs:15600,0.00734138488769531)
--(axis cs:15700,0.00732079707086086)
--(axis cs:15800,0.00730999745428562)
--(axis cs:15900,0.00729026785120368)
--(axis cs:16000,0.00725416000932455)
--(axis cs:16100,0.00720404461026192)
--(axis cs:16200,0.00717591494321823)
--(axis cs:16300,0.00715883914381266)
--(axis cs:16400,0.00721436971798539)
--(axis cs:16500,0.00719568924978375)
--(axis cs:16600,0.00719826994463801)
--(axis cs:16700,0.00718113174661994)
--(axis cs:16800,0.0071498267352581)
--(axis cs:16900,0.00709204701706767)
--(axis cs:17000,0.00711231352761388)
--(axis cs:17100,0.00710775004699826)
--(axis cs:17200,0.00712878024205565)
--(axis cs:17300,0.0071251867339015)
--(axis cs:17400,0.00711927423253655)
--(axis cs:17500,0.0071036284789443)
--(axis cs:17600,0.00706869876012206)
--(axis cs:17700,0.00706928502768278)
--(axis cs:17800,0.00703867571428418)
--(axis cs:17900,0.00702173914760351)
--(axis cs:18000,0.00699694408103824)
--(axis cs:18100,0.00699098501354456)
--(axis cs:18200,0.00695144524797797)
--(axis cs:18300,0.00691674137488008)
--(axis cs:18400,0.00689218798652291)
--(axis cs:18500,0.00688536372035742)
--(axis cs:18600,0.00688301911577582)
--(axis cs:18700,0.00689382385462523)
--(axis cs:18800,0.00690444838255644)
--(axis cs:18900,0.00690837763249874)
--(axis cs:19000,0.00689779920503497)
--(axis cs:19100,0.00688023492693901)
--(axis cs:19200,0.00687850220128894)
--(axis cs:19300,0.00687556760385633)
--(axis cs:19400,0.00686239078640938)
--(axis cs:19500,0.00684259226545691)
--(axis cs:19600,0.00682610226795077)
--(axis cs:19700,0.00682611484080553)
--(axis cs:19800,0.00678225141018629)
--(axis cs:19900,0.00678906450048089)
--(axis cs:20000,0.00676918029785156)
--(axis cs:20100,0.00673599867150187)
--(axis cs:20200,0.00670981407165527)
--(axis cs:20300,0.00672059040516615)
--(axis cs:20400,0.00669183721765876)
--(axis cs:20500,0.00669727334752679)
--(axis cs:20600,0.00670366268604994)
--(axis cs:20700,0.00664744386449456)
--(axis cs:20800,0.00663218507543206)
--(axis cs:20900,0.00660948734730482)
--(axis cs:21000,0.00661106128245592)
--(axis cs:21100,0.00661759357899427)
--(axis cs:21200,0.00663557043299079)
--(axis cs:21300,0.00658988952636719)
--(axis cs:21400,0.00658845901489258)
--(axis cs:21500,0.00655603408813477)
--(axis cs:21600,0.00654501933604479)
--(axis cs:21700,0.00655541429296136)
--(axis cs:21800,0.00655937194824219)
--(axis cs:21900,0.00655121821910143)
--(axis cs:22000,0.00654945382848382)
--(axis cs:22100,0.00650849333032966)
--(axis cs:22200,0.00648646336048841)
--(axis cs:22300,0.00649633398279548)
--(axis cs:22400,0.00645995140075684)
--(axis cs:22500,0.00646467227488756)
--(axis cs:22600,0.00647244462743402)
--(axis cs:22700,0.00646667461842299)
--(axis cs:22800,0.0064691542647779)
--(axis cs:22900,0.0064558507874608)
--(axis cs:23000,0.00646581640467048)
--(axis cs:23100,0.00642790785059333)
--(axis cs:23200,0.00640363711863756)
--(axis cs:23300,0.00639920216053724)
--(axis cs:23400,0.00635423650965095)
--(axis cs:23500,0.00636143703013659)
--(axis cs:23600,0.00638828286901116)
--(axis cs:23700,0.00638351449742913)
--(axis cs:23800,0.00635166186839342)
--(axis cs:23900,0.00634322175756097)
--(axis cs:24000,0.00631790142506361)
--(axis cs:24100,0.00630531320348382)
--(axis cs:24200,0.00628027925267816)
--(axis cs:24300,0.00627965945750475)
--(axis cs:24400,0.00627865782007575)
--(axis cs:24500,0.00632481556385756)
--(axis cs:24600,0.0063331127166748)
--(axis cs:24700,0.00630888948217034)
--(axis cs:24800,0.00628075608983636)
--(axis cs:24900,0.00627627363428473)
--(axis cs:25000,0.00624547014012933)
--(axis cs:25100,0.00621428480371833)
--(axis cs:25200,0.00622339267283678)
--(axis cs:25300,0.00621962547302246)
--(axis cs:25400,0.00617651920765638)
--(axis cs:25500,0.00613861065357924)
--(axis cs:25600,0.00611248007044196)
--(axis cs:25700,0.00609655398875475)
--(axis cs:25800,0.00611190777271986)
--(axis cs:25900,0.00613398570567369)
--(axis cs:26000,0.00615301122888923)
--(axis cs:26100,0.00614552479237318)
--(axis cs:26200,0.00616130838170648)
--(axis cs:26300,0.00610504159703851)
--(axis cs:26400,0.00611205119639635)
--(axis cs:26500,0.00609974842518568)
--(axis cs:26600,0.00612187385559082)
--(axis cs:26700,0.00609207153320312)
--(axis cs:26800,0.00610895175486803)
--(axis cs:26900,0.00609846133738756)
--(axis cs:27000,0.00608248729258776)
--(axis cs:27100,0.00608263025060296)
--(axis cs:27200,0.00608439464122057)
--(axis cs:27300,0.00606460589915514)
--(axis cs:27400,0.00604515057057142)
--(axis cs:27500,0.006012630648911)
--(axis cs:27600,0.00597839336842299)
--(axis cs:27700,0.0060126781463623)
--(axis cs:27800,0.00600185384973884)
--(axis cs:27900,0.00604710588231683)
--(axis cs:28000,0.00606708507984877)
--(axis cs:28100,0.00607876759022474)
--(axis cs:28200,0.00605406751856208)
--(axis cs:28300,0.00600781431421638)
--(axis cs:28400,0.00597372045740485)
--(axis cs:28500,0.00596423167735338)
--(axis cs:28600,0.00589852314442396)
--(axis cs:28700,0.00586962699890137)
--(axis cs:28800,0.00586962699890137)
--(axis cs:28900,0.00586962699890137)
--(axis cs:29000,0.00586962699890137)
--(axis cs:29100,0.00586962699890137)
--(axis cs:29200,0.00586962699890137)
--(axis cs:29300,0.00586962699890137)
--(axis cs:29400,0.00586962699890137)
--(axis cs:29500,0.00586962699890137)
--(axis cs:29600,0.00586962699890137)
--(axis cs:29700,0.00586962699890137)
--(axis cs:29800,0.00586962699890137)
--(axis cs:29900,0.00586962699890137)
--(axis cs:30000,0.00586962699890137)
--(axis cs:30100,0.00586962699890137)
--(axis cs:30200,0.00586962699890137)
--(axis cs:30300,0.00586962699890137)
--(axis cs:30400,0.00586962699890137)
--(axis cs:30400,0.00680618034675717)
--(axis cs:30400,0.00680618034675717)
--(axis cs:30300,0.00680519454181194)
--(axis cs:30200,0.00680339336395264)
--(axis cs:30100,0.00680307345464826)
--(axis cs:30000,0.00680376728996634)
--(axis cs:29900,0.00680395774543285)
--(axis cs:29800,0.00680351629853249)
--(axis cs:29700,0.00680292770266533)
--(axis cs:29600,0.00680841039866209)
--(axis cs:29500,0.00681035313755274)
--(axis cs:29400,0.00681691337376833)
--(axis cs:29300,0.0068219481036067)
--(axis cs:29200,0.00682665267959237)
--(axis cs:29100,0.00681893434375525)
--(axis cs:29000,0.00681679742410779)
--(axis cs:28900,0.00681161321699619)
--(axis cs:28800,0.00680893380194902)
--(axis cs:28700,0.00680827163159847)
--(axis cs:28600,0.00681248959153891)
--(axis cs:28500,0.00682251621037722)
--(axis cs:28400,0.00682880030944943)
--(axis cs:28300,0.00683867791667581)
--(axis cs:28200,0.00684615503996611)
--(axis cs:28100,0.00684823608025908)
--(axis cs:28000,0.00684164231643081)
--(axis cs:27900,0.00684214988723397)
--(axis cs:27800,0.0068357321433723)
--(axis cs:27700,0.00683506531640887)
--(axis cs:27600,0.00683228950947523)
--(axis cs:27500,0.00683529209345579)
--(axis cs:27400,0.00683677289634943)
--(axis cs:27300,0.00683995150029659)
--(axis cs:27200,0.00684288609772921)
--(axis cs:27100,0.00684427656233311)
--(axis cs:27000,0.00684519670903683)
--(axis cs:26900,0.00684589613229036)
--(axis cs:26800,0.00685000419616699)
--(axis cs:26700,0.00684454757720232)
--(axis cs:26600,0.00685066170990467)
--(axis cs:26500,0.00684921769425273)
--(axis cs:26400,0.00685421517118812)
--(axis cs:26300,0.00685153249651194)
--(axis cs:26200,0.0068633034825325)
--(axis cs:26100,0.00686630746349692)
--(axis cs:26000,0.0068733086809516)
--(axis cs:25900,0.00687126070261002)
--(axis cs:25800,0.00687388377264142)
--(axis cs:25700,0.0068721417337656)
--(axis cs:25600,0.00686814589425921)
--(axis cs:25500,0.00687062228098512)
--(axis cs:25400,0.00687291892245412)
--(axis cs:25300,0.00687442906200886)
--(axis cs:25200,0.00687346374616027)
--(axis cs:25100,0.00687964493408799)
--(axis cs:25000,0.00687833409756422)
--(axis cs:24900,0.00688449759036303)
--(axis cs:24800,0.00688654230907559)
--(axis cs:24700,0.00688771065324545)
--(axis cs:24600,0.00689282454550266)
--(axis cs:24500,0.00689405994489789)
--(axis cs:24400,0.00688763614743948)
--(axis cs:24300,0.00689318217337132)
--(axis cs:24200,0.00689812377095222)
--(axis cs:24100,0.00689811166375875)
--(axis cs:24000,0.00690383743494749)
--(axis cs:23900,0.0069077811203897)
--(axis cs:23800,0.00690534897148609)
--(axis cs:23700,0.00690628448501229)
--(axis cs:23600,0.00690426724031568)
--(axis cs:23500,0.00690383417531848)
--(axis cs:23400,0.00690954877063632)
--(axis cs:23300,0.00691248569637537)
--(axis cs:23200,0.00691372016444802)
--(axis cs:23100,0.00691669154912233)
--(axis cs:23000,0.00691855559125543)
--(axis cs:22900,0.00692102592438459)
--(axis cs:22800,0.00691938027739525)
--(axis cs:22700,0.00692318379878998)
--(axis cs:22600,0.00692597264423966)
--(axis cs:22500,0.00692754238843918)
--(axis cs:22400,0.00693544512614608)
--(axis cs:22300,0.00693489564582705)
--(axis cs:22200,0.00693235686048865)
--(axis cs:22100,0.00693506561219692)
--(axis cs:22000,0.00693991128355265)
--(axis cs:21900,0.00693983305245638)
--(axis cs:21800,0.00694178696721792)
--(axis cs:21700,0.00694312667474151)
--(axis cs:21600,0.00694181537255645)
--(axis cs:21500,0.00694055063650012)
--(axis cs:21400,0.00694113364443183)
--(axis cs:21300,0.0069435597397387)
--(axis cs:21200,0.00695066805928946)
--(axis cs:21100,0.00694889528676867)
--(axis cs:21000,0.0069519761018455)
--(axis cs:20900,0.00695595610886812)
--(axis cs:20800,0.00695722689852118)
--(axis cs:20700,0.0069634816609323)
--(axis cs:20600,0.00696854898706079)
--(axis cs:20500,0.00696797296404839)
--(axis cs:20400,0.00696876691654325)
--(axis cs:20300,0.00697500770911574)
--(axis cs:20200,0.00697367358952761)
--(axis cs:20100,0.00698158936575055)
--(axis cs:20000,0.00698174675926566)
--(axis cs:19900,0.00698623666539788)
--(axis cs:19800,0.00699233449995518)
--(axis cs:19700,0.00698935240507126)
--(axis cs:19600,0.00700141256675124)
--(axis cs:19500,0.00700892368331552)
--(axis cs:19400,0.00702034216374159)
--(axis cs:19300,0.0070073870010674)
--(axis cs:19200,0.00702235056087375)
--(axis cs:19100,0.00700930040329695)
--(axis cs:19000,0.0070216809399426)
--(axis cs:18900,0.00702619552612305)
--(axis cs:18800,0.00705757131800056)
--(axis cs:18700,0.00709705520421267)
--(axis cs:18600,0.00710719218477607)
--(axis cs:18500,0.00711969379335642)
--(axis cs:18400,0.00709490897133946)
--(axis cs:18300,0.00706820469349623)
--(axis cs:18200,0.00702619552612305)
--(axis cs:18100,0.00703792553395033)
--(axis cs:18000,0.00702776899561286)
--(axis cs:17900,0.00704736728221178)
--(axis cs:17800,0.00708571774885058)
--(axis cs:17700,0.00709848385304213)
--(axis cs:17600,0.00713456375524402)
--(axis cs:17500,0.00714769959449768)
--(axis cs:17400,0.00715639442205429)
--(axis cs:17300,0.00713947787880898)
--(axis cs:17200,0.00715031614527106)
--(axis cs:17100,0.00715222349390388)
--(axis cs:17000,0.00717884534969926)
--(axis cs:16900,0.00722551345825195)
--(axis cs:16800,0.00726496055722237)
--(axis cs:16700,0.007254000287503)
--(axis cs:16600,0.0072748507373035)
--(axis cs:16500,0.00731732649728656)
--(axis cs:16400,0.00730074429884553)
--(axis cs:16300,0.00733062066137791)
--(axis cs:16200,0.00735750887542963)
--(axis cs:16100,0.00734021980315447)
--(axis cs:16000,0.00733294477686286)
--(axis cs:15900,0.00735705671831965)
--(axis cs:15800,0.00733642559498549)
--(axis cs:15700,0.00735532958060503)
--(axis cs:15600,0.00736895576119423)
--(axis cs:15500,0.00739146396517754)
--(axis cs:15400,0.00744504481554031)
--(axis cs:15300,0.00748283043503761)
--(axis cs:15200,0.00747804576531053)
--(axis cs:15100,0.00753200892359018)
--(axis cs:15000,0.00751964747905731)
--(axis cs:14900,0.00752363912761211)
--(axis cs:14800,0.00752763403579593)
--(axis cs:14700,0.00754294404760003)
--(axis cs:14600,0.00756636029109359)
--(axis cs:14500,0.00759110460057855)
--(axis cs:14400,0.0076126460917294)
--(axis cs:14300,0.00764517672359943)
--(axis cs:14200,0.00766068836674094)
--(axis cs:14100,0.00768190901726484)
--(axis cs:14000,0.00771438889205456)
--(axis cs:13900,0.00772396707907319)
--(axis cs:13800,0.00780001655220985)
--(axis cs:13700,0.0077975750900805)
--(axis cs:13600,0.00783543009310961)
--(axis cs:13500,0.00790242943912745)
--(axis cs:13400,0.00794703885912895)
--(axis cs:13300,0.00789913721382618)
--(axis cs:13200,0.00796949397772551)
--(axis cs:13100,0.00797528587281704)
--(axis cs:13000,0.00796883553266525)
--(axis cs:12900,0.00801739562302828)
--(axis cs:12800,0.00802528951317072)
--(axis cs:12700,0.00807026773691177)
--(axis cs:12600,0.00809737108647823)
--(axis cs:12500,0.008087158203125)
--(axis cs:12400,0.00811796169728041)
--(axis cs:12300,0.0081805232912302)
--(axis cs:12200,0.00819945335388184)
--(axis cs:12100,0.00821065902709961)
--(axis cs:12000,0.00824675522744656)
--(axis cs:11900,0.00827126484364271)
--(axis cs:11800,0.0082700913771987)
--(axis cs:11700,0.00830178428441286)
--(axis cs:11600,0.00839497987180948)
--(axis cs:11500,0.00842467602342367)
--(axis cs:11400,0.00842657312750816)
--(axis cs:11300,0.0084508340805769)
--(axis cs:11200,0.00846203416585922)
--(axis cs:11100,0.00843081437051296)
--(axis cs:11000,0.00846766401082277)
--(axis cs:10900,0.00852099433541298)
--(axis cs:10800,0.00857131276279688)
--(axis cs:10700,0.00859530735760927)
--(axis cs:10600,0.00863382127135992)
--(axis cs:10500,0.00861503463238478)
--(axis cs:10400,0.00863938964903355)
--(axis cs:10300,0.00867146532982588)
--(axis cs:10200,0.0087111433967948)
--(axis cs:10100,0.00876222644001245)
--(axis cs:10000,0.0088041303679347)
--(axis cs:9900,0.00884761847555637)
--(axis cs:9800,0.00888233166188002)
--(axis cs:9700,0.00894193816930056)
--(axis cs:9600,0.00897412747144699)
--(axis cs:9500,0.00902276486158371)
--(axis cs:9400,0.00908310990780592)
--(axis cs:9300,0.00910678971558809)
--(axis cs:9200,0.00914421118795872)
--(axis cs:9100,0.00917877350002527)
--(axis cs:9000,0.0092154499143362)
--(axis cs:8900,0.00926203746348619)
--(axis cs:8800,0.00934122782200575)
--(axis cs:8700,0.00940224342048168)
--(axis cs:8600,0.00942602753639221)
--(axis cs:8500,0.0095024798065424)
--(axis cs:8400,0.00956587679684162)
--(axis cs:8300,0.00961537379771471)
--(axis cs:8200,0.0096556656062603)
--(axis cs:8100,0.00970613956451416)
--(axis cs:8000,0.00981700979173183)
--(axis cs:7900,0.00987306423485279)
--(axis cs:7800,0.0098628206178546)
--(axis cs:7700,0.00992436241358519)
--(axis cs:7600,0.00999546144157648)
--(axis cs:7500,0.0100149633362889)
--(axis cs:7400,0.0101019144058228)
--(axis cs:7300,0.0101523157209158)
--(axis cs:7200,0.0101942485198379)
--(axis cs:7100,0.010236781090498)
--(axis cs:7000,0.0102639170363545)
--(axis cs:6900,0.0103161102160811)
--(axis cs:6800,0.0104055153205991)
--(axis cs:6700,0.0104808509349823)
--(axis cs:6600,0.0105427661910653)
--(axis cs:6500,0.0106602907180786)
--(axis cs:6400,0.0107465982437134)
--(axis cs:6300,0.0108617544174194)
--(axis cs:6200,0.0109682800248265)
--(axis cs:6100,0.0109872091561556)
--(axis cs:6000,0.0110870404168963)
--(axis cs:5900,0.0112245623022318)
--(axis cs:5800,0.0113101406022906)
--(axis cs:5700,0.0114040626212955)
--(axis cs:5600,0.011522326618433)
--(axis cs:5500,0.0116109661757946)
--(axis cs:5400,0.0116998655721545)
--(axis cs:5300,0.011818116530776)
--(axis cs:5200,0.0119392452761531)
--(axis cs:5100,0.0121285384520888)
--(axis cs:5000,0.0122660491615534)
--(axis cs:4900,0.0124231390655041)
--(axis cs:4800,0.0125930495560169)
--(axis cs:4700,0.0127431964501739)
--(axis cs:4600,0.0128848413005471)
--(axis cs:4500,0.0130982156842947)
--(axis cs:4400,0.0132982013747096)
--(axis cs:4300,0.0135007658973336)
--(axis cs:4200,0.0137696610763669)
--(axis cs:4100,0.0140824858099222)
--(axis cs:4000,0.0144160836935043)
--(axis cs:3900,0.0147873442620039)
--(axis cs:3800,0.0151412114500999)
--(axis cs:3700,0.0155271738767624)
--(axis cs:3600,0.0158979017287493)
--(axis cs:3500,0.0163123495876789)
--(axis cs:3400,0.0166979525238276)
--(axis cs:3300,0.0170717183500528)
--(axis cs:3200,0.0174731034785509)
--(axis cs:3100,0.0178576372563839)
--(axis cs:3000,0.0182927809655666)
--(axis cs:2900,0.0188154391944408)
--(axis cs:2800,0.0194802042096853)
--(axis cs:2700,0.0203478150069714)
--(axis cs:2600,0.0214035753160715)
--(axis cs:2500,0.0224937796592712)
--(axis cs:2400,0.0235886592417955)
--(axis cs:2300,0.0249193906784058)
--(axis cs:2200,0.0267025306820869)
--(axis cs:2100,0.0289442576467991)
--(axis cs:2000,0.031578965485096)
--(axis cs:1900,0.0345292389392853)
--(axis cs:1800,0.0373213961720467)
--(axis cs:1700,0.0399247892200947)
--(axis cs:1600,0.0421821065247059)
--(axis cs:1500,0.0441334955394268)
--(axis cs:1400,0.0460115931928158)
--(axis cs:1300,0.0477711781859398)
--(axis cs:1200,0.0492039807140827)
--(axis cs:1100,0.0503541566431522)
--(axis cs:1000,0.0511730425059795)
--(axis cs:900,0.0515283420681953)
--(axis cs:800,0.0516600236296654)
--(axis cs:700,0.0518020577728748)
--(axis cs:600,0.0520781837403774)
--(axis cs:500,0.0527633503079414)
--(axis cs:400,0.0543137490749359)
--(axis cs:300,0.056662742048502)
--(axis cs:200,0.0592069700360298)
--(axis cs:100,0.0616600550711155)
--(axis cs:0,0.0637036859989166)
--cycle;

\path [fill=color0, fill opacity=0.4, ultra thick]
(axis cs:0,0.0487950257956982)
--(axis cs:0,0.048629354685545)
--(axis cs:100,0.0425903834402561)
--(axis cs:200,0.0358326621353626)
--(axis cs:300,0.0322679057717323)
--(axis cs:400,0.0296411383897066)
--(axis cs:500,0.0268500093370676)
--(axis cs:600,0.0239638518542051)
--(axis cs:700,0.0221002344042063)
--(axis cs:800,0.0210253950208426)
--(axis cs:900,0.0199772603809834)
--(axis cs:1000,0.0189599748700857)
--(axis cs:1100,0.0181993190199137)
--(axis cs:1200,0.0174159165471792)
--(axis cs:1300,0.0166514068841934)
--(axis cs:1400,0.0159712340682745)
--(axis cs:1500,0.0153839690610766)
--(axis cs:1600,0.0148046240210533)
--(axis cs:1700,0.014320963062346)
--(axis cs:1800,0.0139094097539783)
--(axis cs:1900,0.0135928550735116)
--(axis cs:2000,0.0132493302226067)
--(axis cs:2100,0.0130304284393787)
--(axis cs:2200,0.0127656832337379)
--(axis cs:2300,0.0126054286956787)
--(axis cs:2400,0.0123540880158544)
--(axis cs:2500,0.0121608413755894)
--(axis cs:2600,0.011988771148026)
--(axis cs:2700,0.0119153903797269)
--(axis cs:2800,0.0117283780127764)
--(axis cs:2900,0.0115924319252372)
--(axis cs:3000,0.0114399464800954)
--(axis cs:3100,0.0113275982439518)
--(axis cs:3200,0.011183762922883)
--(axis cs:3300,0.0110980747267604)
--(axis cs:3400,0.0109866783022881)
--(axis cs:3500,0.0108873844146729)
--(axis cs:3600,0.0107817053794861)
--(axis cs:3700,0.0106692845001817)
--(axis cs:3800,0.0106248613446951)
--(axis cs:3900,0.0105391638353467)
--(axis cs:4000,0.0104595050215721)
--(axis cs:4100,0.0104005625471473)
--(axis cs:4200,0.0103146806359291)
--(axis cs:4300,0.0102438535541296)
--(axis cs:4400,0.010179559700191)
--(axis cs:4500,0.010112164542079)
--(axis cs:4600,0.0100308721885085)
--(axis cs:4700,0.00996671337634325)
--(axis cs:4800,0.00991099141538143)
--(axis cs:4900,0.00983161572366953)
--(axis cs:5000,0.00978424865752459)
--(axis cs:5100,0.00970828905701637)
--(axis cs:5200,0.00964848976582289)
--(axis cs:5300,0.00956210121512413)
--(axis cs:5400,0.00952408835291862)
--(axis cs:5500,0.00950355548411608)
--(axis cs:5600,0.00945037603378296)
--(axis cs:5700,0.00940935779362917)
--(axis cs:5800,0.0093857403844595)
--(axis cs:5900,0.00934929586946964)
--(axis cs:6000,0.00929865427315235)
--(axis cs:6100,0.00925660040229559)
--(axis cs:6200,0.00918538589030504)
--(axis cs:6300,0.00912001170217991)
--(axis cs:6400,0.0090666376054287)
--(axis cs:6500,0.00904356595128775)
--(axis cs:6600,0.00901827123016119)
--(axis cs:6700,0.0089785810559988)
--(axis cs:6800,0.00892381649464369)
--(axis cs:6900,0.00889419391751289)
--(axis cs:7000,0.00887663848698139)
--(axis cs:7100,0.00886866543442011)
--(axis cs:7200,0.00884649716317654)
--(axis cs:7300,0.0088197709992528)
--(axis cs:7400,0.00877709407359362)
--(axis cs:7500,0.00875394325703382)
--(axis cs:7600,0.00869183707982302)
--(axis cs:7700,0.00870625954121351)
--(axis cs:7800,0.00868376810103655)
--(axis cs:7900,0.00864872243255377)
--(axis cs:8000,0.00859700888395309)
--(axis cs:8100,0.00856242142617702)
--(axis cs:8200,0.00850940681993961)
--(axis cs:8300,0.00848625972867012)
--(axis cs:8400,0.00845228787511587)
--(axis cs:8500,0.00843879766762257)
--(axis cs:8600,0.00842626113444567)
--(axis cs:8700,0.00839195679873228)
--(axis cs:8800,0.00836566742509604)
--(axis cs:8900,0.00833487696945667)
--(axis cs:9000,0.00833966769278049)
--(axis cs:9100,0.00828318577259779)
--(axis cs:9200,0.0082489000633359)
--(axis cs:9300,0.00820619240403175)
--(axis cs:9400,0.00819161627441645)
--(axis cs:9500,0.00814506970345974)
--(axis cs:9600,0.00811932049691677)
--(axis cs:9700,0.00811350345611572)
--(axis cs:9800,0.00805970560759306)
--(axis cs:9900,0.00802341289818287)
--(axis cs:10000,0.00800802744925022)
--(axis cs:10100,0.00798420887440443)
--(axis cs:10200,0.00796267949044704)
--(axis cs:10300,0.0079263923689723)
--(axis cs:10400,0.0079063419252634)
--(axis cs:10500,0.0078976396471262)
--(axis cs:10600,0.00789041537791491)
--(axis cs:10700,0.00789506454020739)
--(axis cs:10800,0.00783126801252365)
--(axis cs:10900,0.00783181190490723)
--(axis cs:11000,0.00779289705678821)
--(axis cs:11100,0.00774736423045397)
--(axis cs:11200,0.00773830432444811)
--(axis cs:11300,0.00773878116160631)
--(axis cs:11400,0.00768057256937027)
--(axis cs:11500,0.00766446581110358)
--(axis cs:11600,0.00764429569244385)
--(axis cs:11700,0.00761656742542982)
--(axis cs:11800,0.00758202094584703)
--(axis cs:11900,0.00758399954065681)
--(axis cs:12000,0.00758855324238539)
--(axis cs:12100,0.00756383547559381)
--(axis cs:12200,0.00754580507054925)
--(axis cs:12300,0.00753645459190011)
--(axis cs:12400,0.00748999183997512)
--(axis cs:12500,0.00746054155752063)
--(axis cs:12600,0.00742542650550604)
--(axis cs:12700,0.00741562899202108)
--(axis cs:12800,0.00741031160578132)
--(axis cs:12900,0.0074401618912816)
--(axis cs:13000,0.00741944322362542)
--(axis cs:13100,0.00740952510386705)
--(axis cs:13200,0.00739088049158454)
--(axis cs:13300,0.00735251884907484)
--(axis cs:13400,0.00730678020045161)
--(axis cs:13500,0.00729226740077138)
--(axis cs:13600,0.00727970292791724)
--(axis cs:13700,0.00726479012519121)
--(axis cs:13800,0.00724495621398091)
--(axis cs:13900,0.00724936369806528)
--(axis cs:14000,0.00725152622908354)
--(axis cs:14100,0.00721871387213469)
--(axis cs:14200,0.00717947306111455)
--(axis cs:14300,0.00717320898547769)
--(axis cs:14400,0.0071441913023591)
--(axis cs:14500,0.00710551673546433)
--(axis cs:14600,0.00713607203215361)
--(axis cs:14700,0.00710894074290991)
--(axis cs:14800,0.00711694406345487)
--(axis cs:14900,0.00711003970354795)
--(axis cs:15000,0.00710693653672934)
--(axis cs:15100,0.00706619722768664)
--(axis cs:15200,0.00702973082661629)
--(axis cs:15300,0.00701700802892447)
--(axis cs:15400,0.00700150290504098)
--(axis cs:15500,0.00701642408967018)
--(axis cs:15600,0.00699433730915189)
--(axis cs:15700,0.00697788083925843)
--(axis cs:15800,0.00698116468265653)
--(axis cs:15900,0.00697905430570245)
--(axis cs:16000,0.00693949498236179)
--(axis cs:16100,0.00692489137873054)
--(axis cs:16200,0.00691823940724134)
--(axis cs:16300,0.00688695115968585)
--(axis cs:16400,0.00687217712402344)
--(axis cs:16500,0.00686378497630358)
--(axis cs:16600,0.00686823157593608)
--(axis cs:16700,0.00686463294550776)
--(axis cs:16800,0.00685898680239916)
--(axis cs:16900,0.00687061669304967)
--(axis cs:17000,0.0068803308531642)
--(axis cs:17100,0.00685529690235853)
--(axis cs:17200,0.0068522454239428)
--(axis cs:17300,0.00681436061859131)
--(axis cs:17400,0.00680170068517327)
--(axis cs:17500,0.00678095826879144)
--(axis cs:17600,0.00678722839802504)
--(axis cs:17700,0.00676970463246107)
--(axis cs:17800,0.00677111139521003)
--(axis cs:17900,0.00673153391107917)
--(axis cs:18000,0.00671780109405518)
--(axis cs:18100,0.00668911915272474)
--(axis cs:18200,0.0066691399551928)
--(axis cs:18300,0.00664226990193129)
--(axis cs:18400,0.0066446540877223)
--(axis cs:18500,0.00663094501942396)
--(axis cs:18600,0.0066535472869873)
--(axis cs:18700,0.00663735857233405)
--(axis cs:18800,0.00665199756622314)
--(axis cs:18900,0.0066337650641799)
--(axis cs:19000,0.00662564625963569)
--(axis cs:19100,0.00658912677317858)
--(axis cs:19200,0.00659799575805664)
--(axis cs:19300,0.00657196063548326)
--(axis cs:19400,0.0065452097915113)
--(axis cs:19500,0.0065624238923192)
--(axis cs:19600,0.00655088433995843)
--(axis cs:19700,0.00655388832092285)
--(axis cs:19800,0.00654449453577399)
--(axis cs:19900,0.00655112275853753)
--(axis cs:20000,0.00652060518041253)
--(axis cs:20100,0.00651860237121582)
--(axis cs:20200,0.00651373853906989)
--(axis cs:20300,0.00651788711547852)
--(axis cs:20400,0.00651340465992689)
--(axis cs:20500,0.00646762829273939)
--(axis cs:20600,0.00647521018981934)
--(axis cs:20700,0.00644521694630384)
--(axis cs:20800,0.00643229484558105)
--(axis cs:20900,0.00641841907054186)
--(axis cs:21000,0.00641264906153083)
--(axis cs:21100,0.00638670939952135)
--(axis cs:21200,0.00641841907054186)
--(axis cs:21300,0.00644340505823493)
--(axis cs:21400,0.00646753329783678)
--(axis cs:21500,0.006439876742661)
--(axis cs:21600,0.00643353443592787)
--(axis cs:21700,0.00642824172973633)
--(axis cs:21800,0.00640988349914551)
--(axis cs:21900,0.00638389587402344)
--(axis cs:22000,0.00639939308166504)
--(axis cs:22100,0.00638508796691895)
--(axis cs:22200,0.00637631397694349)
--(axis cs:22300,0.00635781278833747)
--(axis cs:22400,0.00635724049061537)
--(axis cs:22500,0.0063323020003736)
--(axis cs:22600,0.00631151208654046)
--(axis cs:22700,0.00631580362096429)
--(axis cs:22800,0.00631403923034668)
--(axis cs:22900,0.0062711713835597)
--(axis cs:23000,0.00626158714294434)
--(axis cs:23100,0.00626249331980944)
--(axis cs:23200,0.00625009555369616)
--(axis cs:23300,0.0062402724288404)
--(axis cs:23400,0.0062397001311183)
--(axis cs:23500,0.0062244413420558)
--(axis cs:23600,0.00624947529286146)
--(axis cs:23700,0.00626001367345452)
--(axis cs:23800,0.00622797012329102)
--(axis cs:23900,0.00622858991846442)
--(axis cs:24000,0.00624403962865472)
--(axis cs:24100,0.00620822887867689)
--(axis cs:24200,0.00617251405492425)
--(axis cs:24300,0.00617852201685309)
--(axis cs:24400,0.0061799050308764)
--(axis cs:24500,0.0061952592805028)
--(axis cs:24600,0.00617904681712389)
--(axis cs:24700,0.00618939381092787)
--(axis cs:24800,0.00618629436939955)
--(axis cs:24900,0.00619616499170661)
--(axis cs:25000,0.00615673046559095)
--(axis cs:25100,0.00616712588816881)
--(axis cs:25200,0.00614318856969476)
--(axis cs:25300,0.00615339260548353)
--(axis cs:25400,0.00612487085163593)
--(axis cs:25500,0.00612589996308088)
--(axis cs:25600,0.00612058583647013)
--(axis cs:25700,0.00610326603055)
--(axis cs:25800,0.00607524299994111)
--(axis cs:25900,0.00609194999560714)
--(axis cs:26000,0.00609895773231983)
--(axis cs:26100,0.00608359789475799)
--(axis cs:26200,0.00609194999560714)
--(axis cs:26300,0.00609240913763642)
--(axis cs:26400,0.00607309071347117)
--(axis cs:26500,0.00606232881546021)
--(axis cs:26600,0.00606499053537846)
--(axis cs:26700,0.00604886654764414)
--(axis cs:26800,0.00604299595579505)
--(axis cs:26900,0.0060273939743638)
--(axis cs:27000,0.00600355491042137)
--(axis cs:27100,0.00601628236472607)
--(axis cs:27200,0.00603239145129919)
--(axis cs:27300,0.00603869277983904)
--(axis cs:27400,0.00603882735595107)
--(axis cs:27500,0.00603353884071112)
--(axis cs:27600,0.00602705590426922)
--(axis cs:27700,0.00602827221155167)
--(axis cs:27800,0.00602955650538206)
--(axis cs:27900,0.0060479617677629)
--(axis cs:28000,0.00604091212153435)
--(axis cs:28100,0.00601987820118666)
--(axis cs:28200,0.00600133696570992)
--(axis cs:28300,0.00600604387000203)
--(axis cs:28400,0.00597369764000177)
--(axis cs:28500,0.00598981138318777)
--(axis cs:28600,0.00598837155848742)
--(axis cs:28700,0.00599867384880781)
--(axis cs:28800,0.00597992585971951)
--(axis cs:28900,0.00599289406090975)
--(axis cs:29000,0.00596372643485665)
--(axis cs:29100,0.00598411727696657)
--(axis cs:29200,0.00597958220168948)
--(axis cs:29300,0.00595729425549507)
--(axis cs:29400,0.00595050305128098)
--(axis cs:29500,0.00598157569766045)
--(axis cs:29600,0.00594915030524135)
--(axis cs:29700,0.00592750543728471)
--(axis cs:29800,0.00594446295872331)
--(axis cs:29900,0.00591845624148846)
--(axis cs:30000,0.00588985299691558)
--(axis cs:30100,0.00588816264644265)
--(axis cs:30200,0.00587033992633224)
--(axis cs:30300,0.00586241390556097)
--(axis cs:30400,0.00589474523440003)
--(axis cs:30500,0.00589365419000387)
--(axis cs:30600,0.00589284533634782)
--(axis cs:30700,0.00589931523427367)
--(axis cs:30800,0.00588883180171251)
--(axis cs:30900,0.00587429851293564)
--(axis cs:31000,0.00586935039609671)
--(axis cs:31100,0.00586432591080666)
--(axis cs:31200,0.00586871337145567)
--(axis cs:31300,0.00586574152112007)
--(axis cs:31300,0.00685878470540047)
--(axis cs:31300,0.00685878470540047)
--(axis cs:31200,0.00685848388820887)
--(axis cs:31100,0.00685892906039953)
--(axis cs:31000,0.00685841962695122)
--(axis cs:30900,0.0068579213693738)
--(axis cs:30800,0.00685648526996374)
--(axis cs:30700,0.00685547525063157)
--(axis cs:30600,0.00685609551146626)
--(axis cs:30500,0.00685601774603128)
--(axis cs:30400,0.00685591297224164)
--(axis cs:30300,0.0068591246381402)
--(axis cs:30200,0.00685831857845187)
--(axis cs:30100,0.00685654999688268)
--(axis cs:30000,0.00685638515278697)
--(axis cs:29900,0.00685369037091732)
--(axis cs:29800,0.00685139885172248)
--(axis cs:29700,0.00685287499800324)
--(axis cs:29600,0.00685100303962827)
--(axis cs:29500,0.00684842746704817)
--(axis cs:29400,0.00685088988393545)
--(axis cs:29300,0.00685032922774553)
--(axis cs:29200,0.00684857694432139)
--(axis cs:29100,0.00684823840856552)
--(axis cs:29000,0.00684980908408761)
--(axis cs:28900,0.00684759952127934)
--(axis cs:28800,0.0068485508672893)
--(axis cs:28700,0.00684719253331423)
--(axis cs:28600,0.00684792548418045)
--(axis cs:28500,0.00684782117605209)
--(axis cs:28400,0.00684902630746365)
--(axis cs:28300,0.00684668822214007)
--(axis cs:28200,0.00684700766578317)
--(axis cs:28100,0.00684579182416201)
--(axis cs:28000,0.00684456247836351)
--(axis cs:27900,0.00684418855234981)
--(axis cs:27800,0.00684520602226257)
--(axis cs:27700,0.00684528145939112)
--(axis cs:27600,0.00684535410255194)
--(axis cs:27500,0.00684497505426407)
--(axis cs:27400,0.0068446765653789)
--(axis cs:27300,0.00684468448162079)
--(axis cs:27200,0.00684504024684429)
--(axis cs:27100,0.00684601906687021)
--(axis cs:27000,0.00684685632586479)
--(axis cs:26900,0.00684533454477787)
--(axis cs:26800,0.0068444493226707)
--(axis cs:26700,0.00684414245188236)
--(axis cs:26600,0.00684337224811316)
--(axis cs:26500,0.00684349145740271)
--(axis cs:26400,0.00684302998706698)
--(axis cs:26300,0.00684233894571662)
--(axis cs:26200,0.00684235384687781)
--(axis cs:26100,0.00684263044968247)
--(axis cs:26000,0.00684214849025011)
--(axis cs:25900,0.00684235384687781)
--(axis cs:25800,0.00684294337406754)
--(axis cs:25700,0.00684203580021858)
--(axis cs:25600,0.00684169214218855)
--(axis cs:25500,0.00684162322431803)
--(axis cs:25400,0.0068416353315115)
--(axis cs:25300,0.00684154685586691)
--(axis cs:25200,0.00684152776375413)
--(axis cs:25100,0.00684162555262446)
--(axis cs:25000,0.00684155989438295)
--(axis cs:24900,0.00684200879186392)
--(axis cs:24800,0.00684184534475207)
--(axis cs:24700,0.00684189330786467)
--(axis cs:24600,0.00684174662455916)
--(axis cs:24500,0.00684199202805758)
--(axis cs:24400,0.00684175733476877)
--(axis cs:24300,0.00684174057096243)
--(axis cs:24200,0.00684167444705963)
--(axis cs:24100,0.0068422588519752)
--(axis cs:24000,0.00684333546087146)
--(axis cs:23900,0.00684280740097165)
--(axis cs:23800,0.00684278830885887)
--(axis cs:23700,0.00684398785233498)
--(axis cs:23600,0.00684354593977332)
--(axis cs:23500,0.00684268260374665)
--(axis cs:23400,0.00684317760169506)
--(axis cs:23300,0.0068431980907917)
--(axis cs:23200,0.00684356968849897)
--(axis cs:23100,0.00684409961104393)
--(axis cs:23000,0.00684405863285065)
--(axis cs:22900,0.00684451125562191)
--(axis cs:22800,0.00684706494212151)
--(axis cs:22700,0.00684718927368522)
--(axis cs:22600,0.0068468889221549)
--(axis cs:22500,0.0068484335206449)
--(axis cs:22400,0.00685102120041847)
--(axis cs:22300,0.00685156462714076)
--(axis cs:22200,0.00685385940596461)
--(axis cs:22100,0.00685791065916419)
--(axis cs:22000,0.00686048809438944)
--(axis cs:21900,0.00685680378228426)
--(axis cs:21800,0.00686061894521117)
--(axis cs:21700,0.00686425669118762)
--(axis cs:21600,0.00686814822256565)
--(axis cs:21500,0.00687059108167887)
--(axis cs:21400,0.00687263533473015)
--(axis cs:21300,0.00686806859448552)
--(axis cs:21200,0.00686535751447082)
--(axis cs:21100,0.00685850949957967)
--(axis cs:21000,0.00686125038191676)
--(axis cs:20900,0.00686386320739985)
--(axis cs:20800,0.00686691189184785)
--(axis cs:20700,0.00687206024304032)
--(axis cs:20600,0.00687845330685377)
--(axis cs:20500,0.00687720300629735)
--(axis cs:20400,0.00688099442049861)
--(axis cs:20300,0.00688225077465177)
--(axis cs:20200,0.00688097160309553)
--(axis cs:20100,0.00688423356041312)
--(axis cs:20000,0.00688360305503011)
--(axis cs:19900,0.00688777305185795)
--(axis cs:19800,0.00688679981976748)
--(axis cs:19700,0.00688942521810532)
--(axis cs:19600,0.00689151789993048)
--(axis cs:19500,0.00689552025869489)
--(axis cs:19400,0.00689194351434708)
--(axis cs:19300,0.00690188352018595)
--(axis cs:19200,0.00691154366359115)
--(axis cs:19100,0.00690960139036179)
--(axis cs:19000,0.00691692670807242)
--(axis cs:18900,0.00692056957632303)
--(axis cs:18800,0.0069130090996623)
--(axis cs:18700,0.00690589565783739)
--(axis cs:18600,0.00690960418432951)
--(axis cs:18500,0.00690615642815828)
--(axis cs:18400,0.006911251693964)
--(axis cs:18300,0.00691266497597098)
--(axis cs:18200,0.00691762054339051)
--(axis cs:18100,0.00692132348194718)
--(axis cs:18000,0.00692610489204526)
--(axis cs:17900,0.00692688627168536)
--(axis cs:17800,0.00693369749933481)
--(axis cs:17700,0.00693205138668418)
--(axis cs:17600,0.00693516293540597)
--(axis cs:17500,0.00693432847037911)
--(axis cs:17400,0.00693860603496432)
--(axis cs:17300,0.00694237509742379)
--(axis cs:17200,0.00694820517674088)
--(axis cs:17100,0.00694858096539974)
--(axis cs:17000,0.00695458659902215)
--(axis cs:16900,0.0069570573978126)
--(axis cs:16800,0.00695490650832653)
--(axis cs:16700,0.00694778235629201)
--(axis cs:16600,0.00694995326921344)
--(axis cs:16500,0.00694509129971266)
--(axis cs:16400,0.00694220652803779)
--(axis cs:16300,0.00695037143304944)
--(axis cs:16200,0.00695663783699274)
--(axis cs:16100,0.0069870101287961)
--(axis cs:16000,0.00700664054602385)
--(axis cs:15900,0.00703346729278564)
--(axis cs:15800,0.00703204656019807)
--(axis cs:15700,0.00704294303432107)
--(axis cs:15600,0.0070369285531342)
--(axis cs:15500,0.007033821195364)
--(axis cs:15400,0.00705683277919888)
--(axis cs:15300,0.00708681717514992)
--(axis cs:15200,0.00712904939427972)
--(axis cs:15100,0.00713546294718981)
--(axis cs:15000,0.00714412052184343)
--(axis cs:14900,0.0071481941267848)
--(axis cs:14800,0.00716171273961663)
--(axis cs:14700,0.00715939421206713)
--(axis cs:14600,0.00714157614856958)
--(axis cs:14500,0.00719118909910321)
--(axis cs:14400,0.00720639247447252)
--(axis cs:14300,0.00725531578063965)
--(axis cs:14200,0.00726492423564196)
--(axis cs:14100,0.00726276729255915)
--(axis cs:14000,0.00726703740656376)
--(axis cs:13900,0.00729024410247803)
--(axis cs:13800,0.0072992448695004)
--(axis cs:13700,0.00733289727941155)
--(axis cs:13600,0.00736005324870348)
--(axis cs:13500,0.00740097695961595)
--(axis cs:13400,0.00742184510454535)
--(axis cs:13300,0.00747497379779816)
--(axis cs:13200,0.00748876994475722)
--(axis cs:13100,0.00750908674672246)
--(axis cs:13000,0.00752719352021813)
--(axis cs:12900,0.00753316236659884)
--(axis cs:12800,0.00752022257074714)
--(axis cs:12700,0.00753671303391457)
--(axis cs:12600,0.0075503122061491)
--(axis cs:12500,0.00755246868357062)
--(axis cs:12400,0.00757865095511079)
--(axis cs:12300,0.00760956248268485)
--(axis cs:12200,0.0076560340821743)
--(axis cs:12100,0.00769981788471341)
--(axis cs:12000,0.00771000003442168)
--(axis cs:11900,0.00771084753796458)
--(axis cs:11800,0.0077040153555572)
--(axis cs:11700,0.0077028046362102)
--(axis cs:11600,0.0077107478864491)
--(axis cs:11500,0.00776638835668564)
--(axis cs:11400,0.00778775382786989)
--(axis cs:11300,0.00781305134296417)
--(axis cs:11200,0.00781823322176933)
--(axis cs:11100,0.00783918891102076)
--(axis cs:11000,0.0078557226806879)
--(axis cs:10900,0.00793302804231644)
--(axis cs:10800,0.00796305760741234)
--(axis cs:10700,0.00800886563956738)
--(axis cs:10600,0.00803768821060658)
--(axis cs:10500,0.00805125664919615)
--(axis cs:10400,0.00803550519049168)
--(axis cs:10300,0.00806283950805664)
--(axis cs:10200,0.00807841867208481)
--(axis cs:10100,0.00810746848583221)
--(axis cs:10000,0.00810604821890593)
--(axis cs:9900,0.00814112648367882)
--(axis cs:9800,0.00817620288580656)
--(axis cs:9700,0.00818442087620497)
--(axis cs:9600,0.00819882191717625)
--(axis cs:9500,0.00823299121111631)
--(axis cs:9400,0.00825307331979275)
--(axis cs:9300,0.00825977325439453)
--(axis cs:9200,0.00825564842671156)
--(axis cs:9100,0.00830129161477089)
--(axis cs:9000,0.00835177861154079)
--(axis cs:8900,0.00838332064449787)
--(axis cs:8800,0.00840079784393311)
--(axis cs:8700,0.00844440422952175)
--(axis cs:8600,0.00846142135560513)
--(axis cs:8500,0.0084675308316946)
--(axis cs:8400,0.00850044842809439)
--(axis cs:8300,0.00852862559258938)
--(axis cs:8200,0.00855123810470104)
--(axis cs:8100,0.00861977320164442)
--(axis cs:8000,0.00861954689025879)
--(axis cs:7900,0.00867083016782999)
--(axis cs:7800,0.00869068410247564)
--(axis cs:7700,0.00873917900025845)
--(axis cs:7600,0.00876313541084528)
--(axis cs:7500,0.0088068749755621)
--(axis cs:7400,0.00885336101055145)
--(axis cs:7300,0.00890163984149694)
--(axis cs:7200,0.0089099109172821)
--(axis cs:7100,0.00894253794103861)
--(axis cs:7000,0.00897443294525146)
--(axis cs:6900,0.00900376215577126)
--(axis cs:6800,0.00904353521764278)
--(axis cs:6700,0.00908470805734396)
--(axis cs:6600,0.00910090561956167)
--(axis cs:6500,0.00914750061929226)
--(axis cs:6400,0.00919509865343571)
--(axis cs:6300,0.00921312812715769)
--(axis cs:6200,0.00926152523607016)
--(axis cs:6100,0.00927507970482111)
--(axis cs:6000,0.00933827273547649)
--(axis cs:5900,0.00941464304924011)
--(axis cs:5800,0.00947486516088247)
--(axis cs:5700,0.00950172636657953)
--(axis cs:5600,0.00954005774110556)
--(axis cs:5500,0.00959188025444746)
--(axis cs:5400,0.00963639654219151)
--(axis cs:5300,0.00970355793833733)
--(axis cs:5200,0.00977576896548271)
--(axis cs:5100,0.00985685549676418)
--(axis cs:5000,0.00987931620329618)
--(axis cs:4900,0.00993124302476645)
--(axis cs:4800,0.00996583886444569)
--(axis cs:4700,0.0100254779681563)
--(axis cs:4600,0.0100779226049781)
--(axis cs:4500,0.0101523566991091)
--(axis cs:4400,0.0101955411955714)
--(axis cs:4300,0.0102711115032434)
--(axis cs:4200,0.0103566171601415)
--(axis cs:4100,0.0104250544682145)
--(axis cs:4000,0.0105152726173401)
--(axis cs:3900,0.0106360139325261)
--(axis cs:3800,0.010682194493711)
--(axis cs:3700,0.0107612954452634)
--(axis cs:3600,0.0108530335128307)
--(axis cs:3500,0.0109247211366892)
--(axis cs:3400,0.0110286697745323)
--(axis cs:3300,0.0111628901213408)
--(axis cs:3200,0.0113132260739803)
--(axis cs:3100,0.0114332046359777)
--(axis cs:3000,0.0115463379770517)
--(axis cs:2900,0.0116647724062204)
--(axis cs:2800,0.0118211749941111)
--(axis cs:2700,0.0119809145107865)
--(axis cs:2600,0.0121162803843617)
--(axis cs:2500,0.0123082492500544)
--(axis cs:2400,0.0125016439706087)
--(axis cs:2300,0.0126613760367036)
--(axis cs:2200,0.0128647033125162)
--(axis cs:2100,0.0131368450820446)
--(axis cs:2000,0.0134150385856628)
--(axis cs:1900,0.0137205282226205)
--(axis cs:1800,0.0140944411978126)
--(axis cs:1700,0.0145047549158335)
--(axis cs:1600,0.015034407377243)
--(axis cs:1500,0.0155743416398764)
--(axis cs:1400,0.0162540432065725)
--(axis cs:1300,0.01698974147439)
--(axis cs:1200,0.0178048741072416)
--(axis cs:1100,0.0186079870909452)
--(axis cs:1000,0.0194399263709784)
--(axis cs:900,0.0204215664416552)
--(axis cs:800,0.0214774925261736)
--(axis cs:700,0.0224762018769979)
--(axis cs:600,0.0242088567465544)
--(axis cs:500,0.027130639180541)
--(axis cs:400,0.0299398619681597)
--(axis cs:300,0.0326264128088951)
--(axis cs:200,0.0363860614597797)
--(axis cs:100,0.0428013391792774)
--(axis cs:0,0.0487950257956982)
--cycle;

\path [fill=white!40.1960784313725!black, fill opacity=0.4, ultra thick]
(axis cs:0,0.0491982959210873)
--(axis cs:0,0.049132626503706)
--(axis cs:100,0.0430962294340134)
--(axis cs:200,0.0363682098686695)
--(axis cs:300,0.0321813933551311)
--(axis cs:400,0.0294917728751898)
--(axis cs:500,0.0267006009817123)
--(axis cs:600,0.0238281451165676)
--(axis cs:700,0.0221217013895512)
--(axis cs:800,0.0211009476333857)
--(axis cs:900,0.0200391244143248)
--(axis cs:1000,0.0190135780721903)
--(axis cs:1100,0.018229840323329)
--(axis cs:1200,0.0174305085092783)
--(axis cs:1300,0.0165961217135191)
--(axis cs:1400,0.0158965904265642)
--(axis cs:1500,0.01532275788486)
--(axis cs:1600,0.0147445248439908)
--(axis cs:1700,0.0142889143899083)
--(axis cs:1800,0.0139182126149535)
--(axis cs:1900,0.0135842338204384)
--(axis cs:2000,0.0132447788491845)
--(axis cs:2100,0.0130140380933881)
--(axis cs:2200,0.012761645950377)
--(axis cs:2300,0.0125689264386892)
--(axis cs:2400,0.0123534565791488)
--(axis cs:2500,0.0121830115094781)
--(axis cs:2600,0.0120224803686142)
--(axis cs:2700,0.0119075067341328)
--(axis cs:2800,0.0117439897730947)
--(axis cs:2900,0.0116162057965994)
--(axis cs:3000,0.0115119013935328)
--(axis cs:3100,0.0113889779895544)
--(axis cs:3200,0.0112512428313494)
--(axis cs:3300,0.0111356787383556)
--(axis cs:3400,0.0109908860176802)
--(axis cs:3500,0.0108609609305859)
--(axis cs:3600,0.0107248928397894)
--(axis cs:3700,0.0106415031477809)
--(axis cs:3800,0.0105662290006876)
--(axis cs:3900,0.0104771545156837)
--(axis cs:4000,0.0103706466034055)
--(axis cs:4100,0.0103115122765303)
--(axis cs:4200,0.0102346502244473)
--(axis cs:4300,0.010163658298552)
--(axis cs:4400,0.0101066147908568)
--(axis cs:4500,0.0100476108491421)
--(axis cs:4600,0.0100204711779952)
--(axis cs:4700,0.00994156487286091)
--(axis cs:4800,0.00988617539405823)
--(axis cs:4900,0.00979821756482124)
--(axis cs:5000,0.00974726025015116)
--(axis cs:5100,0.00966677814722061)
--(axis cs:5200,0.00961588229984045)
--(axis cs:5300,0.00954455137252808)
--(axis cs:5400,0.00952557288110256)
--(axis cs:5500,0.00947717949748039)
--(axis cs:5600,0.00941329170018435)
--(axis cs:5700,0.00941506028175354)
--(axis cs:5800,0.00939751323312521)
--(axis cs:5900,0.00935683492571115)
--(axis cs:6000,0.00929501000791788)
--(axis cs:6100,0.0092425849288702)
--(axis cs:6200,0.00916855875402689)
--(axis cs:6300,0.00912216678261757)
--(axis cs:6400,0.00907672196626663)
--(axis cs:6500,0.00904580112546682)
--(axis cs:6600,0.00900828558951616)
--(axis cs:6700,0.00897378940135241)
--(axis cs:6800,0.00893955212086439)
--(axis cs:6900,0.0089056259021163)
--(axis cs:7000,0.00889360066503286)
--(axis cs:7100,0.00887115020304918)
--(axis cs:7200,0.00887722987681627)
--(axis cs:7300,0.0088274534791708)
--(axis cs:7400,0.00879304111003876)
--(axis cs:7500,0.00875385571271181)
--(axis cs:7600,0.00868077296763659)
--(axis cs:7700,0.00862491130828857)
--(axis cs:7800,0.00861332379281521)
--(axis cs:7900,0.00858140364289284)
--(axis cs:8000,0.00855625048279762)
--(axis cs:8100,0.00853403843939304)
--(axis cs:8200,0.00848930142819881)
--(axis cs:8300,0.00844331737607718)
--(axis cs:8400,0.00844314135611057)
--(axis cs:8500,0.0084140794351697)
--(axis cs:8600,0.0083959000185132)
--(axis cs:8700,0.00837953109294176)
--(axis cs:8800,0.00834438763558865)
--(axis cs:8900,0.00829768180847168)
--(axis cs:9000,0.0082654133439064)
--(axis cs:9100,0.00823108945041895)
--(axis cs:9200,0.00821364019066095)
--(axis cs:9300,0.00818733032792807)
--(axis cs:9400,0.00816063489764929)
--(axis cs:9500,0.00814556702971458)
--(axis cs:9600,0.00812162738293409)
--(axis cs:9700,0.00807300396263599)
--(axis cs:9800,0.00803261063992977)
--(axis cs:9900,0.0080031817778945)
--(axis cs:10000,0.00800285954028368)
--(axis cs:10100,0.00795783288776875)
--(axis cs:10200,0.00793487299233675)
--(axis cs:10300,0.00790082477033138)
--(axis cs:10400,0.00789136905223131)
--(axis cs:10500,0.00785657204687595)
--(axis cs:10600,0.00784869492053986)
--(axis cs:10700,0.00782443396747112)
--(axis cs:10800,0.00780411204323173)
--(axis cs:10900,0.00778473308309913)
--(axis cs:11000,0.00773728685453534)
--(axis cs:11100,0.00771230226382613)
--(axis cs:11200,0.00772428046911955)
--(axis cs:11300,0.00772189116105437)
--(axis cs:11400,0.00769791612401605)
--(axis cs:11500,0.00767219066619873)
--(axis cs:11600,0.00764191150665283)
--(axis cs:11700,0.00758969783782959)
--(axis cs:11800,0.00757623743265867)
--(axis cs:11900,0.0075700324960053)
--(axis cs:12000,0.00758716836571693)
--(axis cs:12100,0.00757521670311689)
--(axis cs:12200,0.00759265432134271)
--(axis cs:12300,0.00756454421207309)
--(axis cs:12400,0.00751562789082527)
--(axis cs:12500,0.00748812826350331)
--(axis cs:12600,0.00744058145210147)
--(axis cs:12700,0.00742497015744448)
--(axis cs:12800,0.00740518048405647)
--(axis cs:12900,0.00739777088165283)
--(axis cs:13000,0.00736655527725816)
--(axis cs:13100,0.007316704839468)
--(axis cs:13200,0.00730377109721303)
--(axis cs:13300,0.00727003859356046)
--(axis cs:13400,0.00726979784667492)
--(axis cs:13500,0.00727691408246756)
--(axis cs:13600,0.00726385274901986)
--(axis cs:13700,0.00722099281847477)
--(axis cs:13800,0.00720012607052922)
--(axis cs:13900,0.00719556258991361)
--(axis cs:14000,0.00715773878619075)
--(axis cs:14100,0.00712947361171246)
--(axis cs:14200,0.00712584098801017)
--(axis cs:14300,0.0071299490518868)
--(axis cs:14400,0.00711811892688274)
--(axis cs:14500,0.00711890868842602)
--(axis cs:14600,0.00711896410211921)
--(axis cs:14700,0.00708145694807172)
--(axis cs:14800,0.00707411766052246)
--(axis cs:14900,0.00708451261743903)
--(axis cs:15000,0.00708606233820319)
--(axis cs:15100,0.00705220131203532)
--(axis cs:15200,0.00703921308740973)
--(axis cs:15300,0.00701575679704547)
--(axis cs:15400,0.00695932609960437)
--(axis cs:15500,0.00691783800721169)
--(axis cs:15600,0.00693326629698277)
--(axis cs:15700,0.00692059239372611)
--(axis cs:15800,0.00691557954996824)
--(axis cs:15900,0.00692317495122552)
--(axis cs:16000,0.00690956134349108)
--(axis cs:16100,0.00688606919720769)
--(axis cs:16200,0.00686616683378816)
--(axis cs:16300,0.00685786409303546)
--(axis cs:16400,0.00687220832332969)
--(axis cs:16500,0.00688349036499858)
--(axis cs:16600,0.00687645189464092)
--(axis cs:16700,0.0068903504870832)
--(axis cs:16800,0.0068669319152832)
--(axis cs:16900,0.00683695776388049)
--(axis cs:17000,0.00679626455530524)
--(axis cs:17100,0.00679817190393806)
--(axis cs:17200,0.00676906108856201)
--(axis cs:17300,0.00675816554576159)
--(axis cs:17400,0.00675151124596596)
--(axis cs:17500,0.00677290186285973)
--(axis cs:17600,0.00674161966890097)
--(axis cs:17700,0.00672448566183448)
--(axis cs:17800,0.00671280268579721)
--(axis cs:17900,0.00669991970062256)
--(axis cs:18000,0.00664999475702643)
--(axis cs:18100,0.00664889812469482)
--(axis cs:18200,0.0066505060531199)
--(axis cs:18300,0.00661106687039137)
--(axis cs:18400,0.00657129799947143)
--(axis cs:18500,0.00658774701878428)
--(axis cs:18600,0.00659332657232881)
--(axis cs:18700,0.00658155046403408)
--(axis cs:18800,0.0066035334020853)
--(axis cs:18900,0.0066056726500392)
--(axis cs:19000,0.00657343119382858)
--(axis cs:19100,0.00655139796435833)
--(axis cs:19200,0.00654098484665155)
--(axis cs:19300,0.00652728090062737)
--(axis cs:19400,0.00651273969560862)
--(axis cs:19500,0.00650787353515625)
--(axis cs:19600,0.00647808937355876)
--(axis cs:19700,0.00648327590897679)
--(axis cs:19800,0.00644602114334702)
--(axis cs:19900,0.00642811181023717)
--(axis cs:20000,0.00642998749390244)
--(axis cs:20100,0.00641488051041961)
--(axis cs:20200,0.00642308965325356)
--(axis cs:20300,0.00640921574085951)
--(axis cs:20400,0.00640395935624838)
--(axis cs:20500,0.00639859307557344)
--(axis cs:20600,0.006396877579391)
--(axis cs:20700,0.00636670086532831)
--(axis cs:20800,0.00639046309515834)
--(axis cs:20900,0.00638170260936022)
--(axis cs:21000,0.0063633918762207)
--(axis cs:21100,0.00636102957651019)
--(axis cs:21200,0.00633905967697501)
--(axis cs:21300,0.0063130808994174)
--(axis cs:21400,0.00632077641785145)
--(axis cs:21500,0.00631920993328094)
--(axis cs:21600,0.00632180133834481)
--(axis cs:21700,0.00632417760789394)
--(axis cs:21800,0.00631679408252239)
--(axis cs:21900,0.00631573330610991)
--(axis cs:22000,0.00631213188171387)
--(axis cs:22100,0.00629358272999525)
--(axis cs:22200,0.00628466624766588)
--(axis cs:22300,0.00628232955932617)
--(axis cs:22400,0.00626506097614765)
--(axis cs:22500,0.00627197651192546)
--(axis cs:22600,0.00627545453608036)
--(axis cs:22700,0.00626832060515881)
--(axis cs:22800,0.00626265536993742)
--(axis cs:22900,0.00627807900309563)
--(axis cs:23000,0.00626330124214292)
--(axis cs:23100,0.00624522846192122)
--(axis cs:23200,0.00623960606753826)
--(axis cs:23300,0.00624810950830579)
--(axis cs:23400,0.0062272297218442)
--(axis cs:23500,0.00621978519484401)
--(axis cs:23600,0.00622192258015275)
--(axis cs:23700,0.00623825564980507)
--(axis cs:23800,0.00622668955475092)
--(axis cs:23900,0.00622470583766699)
--(axis cs:24000,0.00620948290452361)
--(axis cs:24100,0.00621706293895841)
--(axis cs:24200,0.00620395503938198)
--(axis cs:24300,0.00621651764959097)
--(axis cs:24400,0.00621782569214702)
--(axis cs:24500,0.00621491670608521)
--(axis cs:24600,0.00620065163820982)
--(axis cs:24700,0.006169602740556)
--(axis cs:24800,0.00614321744069457)
--(axis cs:24900,0.00611946452409029)
--(axis cs:25000,0.00611034408211708)
--(axis cs:25100,0.00610245810821652)
--(axis cs:25200,0.00611995439976454)
--(axis cs:25300,0.00611498160287738)
--(axis cs:25400,0.00610325066372752)
--(axis cs:25500,0.0061086849309504)
--(axis cs:25600,0.00609581032767892)
--(axis cs:25700,0.00606576120480895)
--(axis cs:25800,0.00606416864320636)
--(axis cs:25900,0.00608102371916175)
--(axis cs:26000,0.00607087649405003)
--(axis cs:26100,0.00607871497049928)
--(axis cs:26200,0.00610943930223584)
--(axis cs:26300,0.00609516818076372)
--(axis cs:26400,0.00608719093725085)
--(axis cs:26500,0.00609641522169113)
--(axis cs:26600,0.00608465680852532)
--(axis cs:26700,0.0060420511290431)
--(axis cs:26800,0.00604402506724)
--(axis cs:26900,0.0060420511290431)
--(axis cs:27000,0.00605070497840643)
--(axis cs:27100,0.00609509274363518)
--(axis cs:27200,0.00609293766319752)
--(axis cs:27300,0.00608446728438139)
--(axis cs:27400,0.00606318330392241)
--(axis cs:27500,0.00605127448216081)
--(axis cs:27600,0.00602985825389624)
--(axis cs:27700,0.00603320170193911)
--(axis cs:27800,0.00603483524173498)
--(axis cs:27900,0.00605154037475586)
--(axis cs:28000,0.00604087393730879)
--(axis cs:28100,0.0060338475741446)
--(axis cs:28200,0.00601716199889779)
--(axis cs:28300,0.00599558930844069)
--(axis cs:28400,0.00596809014678001)
--(axis cs:28500,0.00595699856057763)
--(axis cs:28600,0.00594380544498563)
--(axis cs:28700,0.00595455849543214)
--(axis cs:28800,0.00596927152946591)
--(axis cs:28900,0.00596709968522191)
--(axis cs:29000,0.00596656557172537)
--(axis cs:29100,0.00594815285876393)
--(axis cs:29200,0.00592686794698238)
--(axis cs:29300,0.00590530410408974)
--(axis cs:29400,0.00591854937374592)
--(axis cs:29500,0.00590434949845076)
--(axis cs:29600,0.00589915690943599)
--(axis cs:29700,0.00590286031365395)
--(axis cs:29800,0.00591499963775277)
--(axis cs:29900,0.00589018315076828)
--(axis cs:30000,0.00589213101193309)
--(axis cs:30100,0.00588105525821447)
--(axis cs:30200,0.00588728068396449)
--(axis cs:30300,0.0058612278662622)
--(axis cs:30400,0.00585675705224276)
--(axis cs:30500,0.00585881993174553)
--(axis cs:30600,0.00584628619253635)
--(axis cs:30700,0.00583822093904018)
--(axis cs:30800,0.00585656613111496)
--(axis cs:30900,0.0058605782687664)
--(axis cs:31000,0.00582373281940818)
--(axis cs:31100,0.00583539251238108)
--(axis cs:31200,0.00583952059969306)
--(axis cs:31300,0.00584150850772858)
--(axis cs:31400,0.00582977291196585)
--(axis cs:31500,0.00582927605137229)
--(axis cs:31600,0.00580247212201357)
--(axis cs:31700,0.00578415207564831)
--(axis cs:31800,0.00577504793182015)
--(axis cs:31900,0.00577998254448175)
--(axis cs:32000,0.00581149710342288)
--(axis cs:32100,0.00581409689038992)
--(axis cs:32200,0.00582621805369854)
--(axis cs:32300,0.00583718903362751)
--(axis cs:32400,0.00581577979028225)
--(axis cs:32500,0.00578591134399176)
--(axis cs:32600,0.00580557016655803)
--(axis cs:32700,0.00578438164666295)
--(axis cs:32700,0.00639748573303223)
--(axis cs:32700,0.00639748573303223)
--(axis cs:32600,0.00639748573303223)
--(axis cs:32500,0.00639748573303223)
--(axis cs:32400,0.00639748573303223)
--(axis cs:32300,0.00639748573303223)
--(axis cs:32200,0.00639748573303223)
--(axis cs:32100,0.00639748573303223)
--(axis cs:32000,0.00639748573303223)
--(axis cs:31900,0.00639748573303223)
--(axis cs:31800,0.00639748573303223)
--(axis cs:31700,0.00639748573303223)
--(axis cs:31600,0.00639748573303223)
--(axis cs:31500,0.00639748573303223)
--(axis cs:31400,0.00639748573303223)
--(axis cs:31300,0.00639748573303223)
--(axis cs:31200,0.00639748573303223)
--(axis cs:31100,0.00639748573303223)
--(axis cs:31000,0.00639748573303223)
--(axis cs:30900,0.00639748573303223)
--(axis cs:30800,0.00639748573303223)
--(axis cs:30700,0.00639748573303223)
--(axis cs:30600,0.00639748573303223)
--(axis cs:30500,0.00639748573303223)
--(axis cs:30400,0.00639748573303223)
--(axis cs:30300,0.00639748573303223)
--(axis cs:30200,0.00639748573303223)
--(axis cs:30100,0.00639748573303223)
--(axis cs:30000,0.00639748573303223)
--(axis cs:29900,0.00639748573303223)
--(axis cs:29800,0.00639748573303223)
--(axis cs:29700,0.00639748573303223)
--(axis cs:29600,0.00639748573303223)
--(axis cs:29500,0.00639748573303223)
--(axis cs:29400,0.00639748573303223)
--(axis cs:29300,0.00639748573303223)
--(axis cs:29200,0.00639748573303223)
--(axis cs:29100,0.00639748573303223)
--(axis cs:29000,0.00639748573303223)
--(axis cs:28900,0.00639748573303223)
--(axis cs:28800,0.00639748573303223)
--(axis cs:28700,0.00639748573303223)
--(axis cs:28600,0.00639748573303223)
--(axis cs:28500,0.00639748573303223)
--(axis cs:28400,0.00639748573303223)
--(axis cs:28300,0.00639748573303223)
--(axis cs:28200,0.00639748573303223)
--(axis cs:28100,0.00639748573303223)
--(axis cs:28000,0.00639748573303223)
--(axis cs:27900,0.00639748573303223)
--(axis cs:27800,0.00639748573303223)
--(axis cs:27700,0.00639748573303223)
--(axis cs:27600,0.00639748573303223)
--(axis cs:27500,0.00639748573303223)
--(axis cs:27400,0.00639748573303223)
--(axis cs:27300,0.00639748573303223)
--(axis cs:27200,0.00639748573303223)
--(axis cs:27100,0.00639748573303223)
--(axis cs:27000,0.00639748573303223)
--(axis cs:26900,0.00639748573303223)
--(axis cs:26800,0.00639748573303223)
--(axis cs:26700,0.00639748573303223)
--(axis cs:26600,0.00639748573303223)
--(axis cs:26500,0.00639748573303223)
--(axis cs:26400,0.00639748573303223)
--(axis cs:26300,0.00639748573303223)
--(axis cs:26200,0.00639748573303223)
--(axis cs:26100,0.00639748573303223)
--(axis cs:26000,0.00639748573303223)
--(axis cs:25900,0.00639748573303223)
--(axis cs:25800,0.00639748573303223)
--(axis cs:25700,0.00639748573303223)
--(axis cs:25600,0.00639748573303223)
--(axis cs:25500,0.00639748573303223)
--(axis cs:25400,0.00639748573303223)
--(axis cs:25300,0.00639748573303223)
--(axis cs:25200,0.00639748573303223)
--(axis cs:25100,0.00639748573303223)
--(axis cs:25000,0.00639748573303223)
--(axis cs:24900,0.00639748573303223)
--(axis cs:24800,0.00639518303796649)
--(axis cs:24700,0.00639124168083072)
--(axis cs:24600,0.00638686306774616)
--(axis cs:24500,0.00638499576598406)
--(axis cs:24400,0.00638463022187352)
--(axis cs:24300,0.00638479460030794)
--(axis cs:24200,0.00638642068952322)
--(axis cs:24100,0.00638472614809871)
--(axis cs:24000,0.00638569379225373)
--(axis cs:23900,0.00638378970324993)
--(axis cs:23800,0.00638355500996113)
--(axis cs:23700,0.00638225674629211)
--(axis cs:23600,0.00638412544503808)
--(axis cs:23500,0.00638438807800412)
--(axis cs:23400,0.00638349168002605)
--(axis cs:23300,0.00638127280399203)
--(axis cs:23200,0.0063821142539382)
--(axis cs:23100,0.00638154614716768)
--(axis cs:23000,0.00638006860390306)
--(axis cs:22900,0.00637946743518114)
--(axis cs:22800,0.00638010911643505)
--(axis cs:22700,0.00637978501617908)
--(axis cs:22600,0.00637951772660017)
--(axis cs:22500,0.00637962622568011)
--(axis cs:22400,0.00637996103614569)
--(axis cs:22300,0.0063794506713748)
--(axis cs:22200,0.00637946417555213)
--(axis cs:22100,0.00637964671477675)
--(axis cs:22000,0.00638356572017074)
--(axis cs:21900,0.00638625491410494)
--(axis cs:21800,0.00638697482645512)
--(axis cs:21700,0.00639523100107908)
--(axis cs:21600,0.00640380615368485)
--(axis cs:21500,0.00640525389462709)
--(axis cs:21400,0.00642377696931362)
--(axis cs:21300,0.00642524287104607)
--(axis cs:21200,0.00642517162486911)
--(axis cs:21100,0.00641706166788936)
--(axis cs:21000,0.00641902908682823)
--(axis cs:20900,0.00642001815140247)
--(axis cs:20800,0.00642223376780748)
--(axis cs:20700,0.00643466040492058)
--(axis cs:20600,0.00643320102244616)
--(axis cs:20500,0.00645334459841251)
--(axis cs:20400,0.00646562222391367)
--(axis cs:20300,0.00647897645831108)
--(axis cs:20200,0.00648374855518341)
--(axis cs:20100,0.00651555042713881)
--(axis cs:20000,0.00648298254236579)
--(axis cs:19900,0.0065013887360692)
--(axis cs:19800,0.00649347295984626)
--(axis cs:19700,0.00651768920943141)
--(axis cs:19600,0.00651988806203008)
--(axis cs:19500,0.00655012438073754)
--(axis cs:19400,0.00654185470193624)
--(axis cs:19300,0.00657198904082179)
--(axis cs:19200,0.00658026989549398)
--(axis cs:19100,0.00661669857800007)
--(axis cs:19000,0.00663797836750746)
--(axis cs:18900,0.00664813350886106)
--(axis cs:18800,0.00664794445037842)
--(axis cs:18700,0.00664764456450939)
--(axis cs:18600,0.00666815089061856)
--(axis cs:18500,0.00666482467204332)
--(axis cs:18400,0.00666527729481459)
--(axis cs:18300,0.00666277389973402)
--(axis cs:18200,0.00668241688981652)
--(axis cs:18100,0.00668177986517549)
--(axis cs:18000,0.0067030880600214)
--(axis cs:17900,0.00674375845119357)
--(axis cs:17800,0.00678477250039577)
--(axis cs:17700,0.00678908824920654)
--(axis cs:17600,0.00679538259282708)
--(axis cs:17500,0.00680287461727858)
--(axis cs:17400,0.00679948320612311)
--(axis cs:17300,0.00683676358312368)
--(axis cs:17200,0.00683769304305315)
--(axis cs:17100,0.006861821282655)
--(axis cs:17000,0.00687120901420712)
--(axis cs:16900,0.00690071564167738)
--(axis cs:16800,0.00687693897634745)
--(axis cs:16700,0.00691852578893304)
--(axis cs:16600,0.00692334165796638)
--(axis cs:16500,0.00696012983098626)
--(axis cs:16400,0.00697999028488994)
--(axis cs:16300,0.00699863443151116)
--(axis cs:16200,0.00699602952226996)
--(axis cs:16100,0.00701111136004329)
--(axis cs:16000,0.00701030110940337)
--(axis cs:15900,0.00700525753200054)
--(axis cs:15800,0.00698770396411419)
--(axis cs:15700,0.00699450215324759)
--(axis cs:15600,0.00699610728770494)
--(axis cs:15500,0.0070111989043653)
--(axis cs:15400,0.00701088923960924)
--(axis cs:15300,0.0070389392785728)
--(axis cs:15200,0.00706464517861605)
--(axis cs:15100,0.00707654701545835)
--(axis cs:15000,0.00714007159695029)
--(axis cs:14900,0.00717012863606215)
--(axis cs:14800,0.00718042301014066)
--(axis cs:14700,0.00718468381091952)
--(axis cs:14600,0.00719122076407075)
--(axis cs:14500,0.00714716920629144)
--(axis cs:14400,0.00717273820191622)
--(axis cs:14300,0.00720708351582289)
--(axis cs:14200,0.00720734614878893)
--(axis cs:14100,0.00721867103129625)
--(axis cs:14000,0.00725096138194203)
--(axis cs:13900,0.0072467545978725)
--(axis cs:13800,0.00723483087494969)
--(axis cs:13700,0.00725872348994017)
--(axis cs:13600,0.00727500813081861)
--(axis cs:13500,0.00728882476687431)
--(axis cs:13400,0.00731306057423353)
--(axis cs:13300,0.00738604087382555)
--(axis cs:13200,0.00740401679649949)
--(axis cs:13100,0.00739669427275658)
--(axis cs:13000,0.00740659004077315)
--(axis cs:12900,0.00743050174787641)
--(axis cs:12800,0.00742949452251196)
--(axis cs:12700,0.00745323859155178)
--(axis cs:12600,0.00750535493716598)
--(axis cs:12500,0.00749921379610896)
--(axis cs:12400,0.00753927230834961)
--(axis cs:12300,0.0075694085098803)
--(axis cs:12200,0.00760670471936464)
--(axis cs:12100,0.00762266386300325)
--(axis cs:12000,0.00761704426258802)
--(axis cs:11900,0.00763342762365937)
--(axis cs:11800,0.00762685760855675)
--(axis cs:11700,0.00766760995611548)
--(axis cs:11600,0.00770571967586875)
--(axis cs:11500,0.00774653255939484)
--(axis cs:11400,0.00776670640334487)
--(axis cs:11300,0.00781777035444975)
--(axis cs:11200,0.00782269332557917)
--(axis cs:11100,0.00785706751048565)
--(axis cs:11000,0.00786595325917006)
--(axis cs:10900,0.0079128984361887)
--(axis cs:10800,0.0078978780657053)
--(axis cs:10700,0.00792603474110365)
--(axis cs:10600,0.00793793238699436)
--(axis cs:10500,0.00795359630137682)
--(axis cs:10400,0.00794408284127712)
--(axis cs:10300,0.00801607966423035)
--(axis cs:10200,0.00804389175027609)
--(axis cs:10100,0.00806787051260471)
--(axis cs:10000,0.00808532256633043)
--(axis cs:9900,0.00812030490487814)
--(axis cs:9800,0.00813080184161663)
--(axis cs:9700,0.00812826119363308)
--(axis cs:9600,0.00816431734710932)
--(axis cs:9500,0.00818273983895779)
--(axis cs:9400,0.00822431687265635)
--(axis cs:9300,0.00824671890586615)
--(axis cs:9200,0.0082556726410985)
--(axis cs:9100,0.00827992055565119)
--(axis cs:9000,0.0083168838173151)
--(axis cs:8900,0.0083491550758481)
--(axis cs:8800,0.008379140868783)
--(axis cs:8700,0.00841499213129282)
--(axis cs:8600,0.00843815784901381)
--(axis cs:8500,0.00845225434750319)
--(axis cs:8400,0.00847639422863722)
--(axis cs:8300,0.00851132813841105)
--(axis cs:8200,0.00852229632437229)
--(axis cs:8100,0.00856379978358746)
--(axis cs:8000,0.00858151912689209)
--(axis cs:7900,0.00862834416329861)
--(axis cs:7800,0.0086601497605443)
--(axis cs:7700,0.00868547149002552)
--(axis cs:7600,0.00871133990585804)
--(axis cs:7500,0.00877509173005819)
--(axis cs:7400,0.00883149541914463)
--(axis cs:7300,0.00888761878013611)
--(axis cs:7200,0.00891011673957109)
--(axis cs:7100,0.00892579555511475)
--(axis cs:7000,0.00891035329550505)
--(axis cs:6900,0.00894223060458899)
--(axis cs:6800,0.00898073520511389)
--(axis cs:6700,0.00903828628361225)
--(axis cs:6600,0.00908056367188692)
--(axis cs:6500,0.0091228699311614)
--(axis cs:6400,0.00915632210671902)
--(axis cs:6300,0.00918144918978214)
--(axis cs:6200,0.00920643843710423)
--(axis cs:6100,0.0092843733727932)
--(axis cs:6000,0.0093438858166337)
--(axis cs:5900,0.0093970512971282)
--(axis cs:5800,0.00943869072943926)
--(axis cs:5700,0.00948349945247173)
--(axis cs:5600,0.00951544009149075)
--(axis cs:5500,0.00956014357507229)
--(axis cs:5400,0.00960821378976107)
--(axis cs:5300,0.00968102924525738)
--(axis cs:5200,0.00975377392023802)
--(axis cs:5100,0.0098196417093277)
--(axis cs:5000,0.00987078901380301)
--(axis cs:4900,0.00991247408092022)
--(axis cs:4800,0.0099507812410593)
--(axis cs:4700,0.0100187119096518)
--(axis cs:4600,0.0100942766293883)
--(axis cs:4500,0.0101769212633371)
--(axis cs:4400,0.010251940228045)
--(axis cs:4300,0.0103331794962287)
--(axis cs:4200,0.0103941354900599)
--(axis cs:4100,0.0104318428784609)
--(axis cs:4000,0.0104827610775828)
--(axis cs:3900,0.0105607630684972)
--(axis cs:3800,0.0106485188007355)
--(axis cs:3700,0.0107548180967569)
--(axis cs:3600,0.0108531564474106)
--(axis cs:3500,0.0109605230391026)
--(axis cs:3400,0.011052024550736)
--(axis cs:3300,0.0111840963363647)
--(axis cs:3200,0.0113219618797302)
--(axis cs:3100,0.0114828739315271)
--(axis cs:3000,0.0116145275533199)
--(axis cs:2900,0.0117637319490314)
--(axis cs:2800,0.0118762822821736)
--(axis cs:2700,0.0120199583470821)
--(axis cs:2600,0.0121446456760168)
--(axis cs:2500,0.0123099749907851)
--(axis cs:2400,0.0125218098983169)
--(axis cs:2300,0.0126814544200897)
--(axis cs:2200,0.0128805637359619)
--(axis cs:2100,0.0131098432466388)
--(axis cs:2000,0.0133815044537187)
--(axis cs:1900,0.0136804804205894)
--(axis cs:1800,0.0140497973188758)
--(axis cs:1700,0.0144479628652334)
--(axis cs:1600,0.0149785010144114)
--(axis cs:1500,0.0155085325241089)
--(axis cs:1400,0.0161406192928553)
--(axis cs:1300,0.0167877674102783)
--(axis cs:1200,0.0175414141267538)
--(axis cs:1100,0.0183536950498819)
--(axis cs:1000,0.0191886592656374)
--(axis cs:900,0.0202075075358152)
--(axis cs:800,0.0212784055620432)
--(axis cs:700,0.0223503522574902)
--(axis cs:600,0.0239617880433798)
--(axis cs:500,0.0268660485744476)
--(axis cs:400,0.0296337939798832)
--(axis cs:300,0.0322838500142097)
--(axis cs:200,0.0364052802324295)
--(axis cs:100,0.0431578680872917)
--(axis cs:0,0.0491982959210873)
--cycle;

\addplot [ultra thick, red]
table {%
0 0.0544580146670341
100 0.0542704574763775
200 0.0538766831159592
300 0.0533064268529415
400 0.052464172244072
500 0.0513866692781448
600 0.0500394143164158
700 0.0485865473747253
800 0.0471253134310246
900 0.0457724444568157
1000 0.0445105321705341
1100 0.0434617474675179
1400 0.0408168621361256
1500 0.04001235216856
1600 0.0393390245735645
1700 0.0387342125177383
1800 0.0382256507873535
1900 0.0377788990736008
2000 0.0373917557299137
2100 0.0369442813098431
2200 0.036414872854948
2300 0.0358754359185696
2400 0.0352378450334072
2500 0.0344973541796207
2600 0.033745676279068
2700 0.0330415181815624
2800 0.0322929210960865
2900 0.0316906832158566
3200 0.030158843845129
3300 0.0297135636210442
3500 0.0287914033979177
3600 0.0283913724124432
3700 0.02801757119596
3800 0.0276709068566561
3900 0.027309313416481
4300 0.0260236486792564
4400 0.025777593255043
4500 0.025513244792819
4600 0.025288037955761
4700 0.0250044278800488
4800 0.0247754212468863
5100 0.0240313708782196
5200 0.0238579753786325
5300 0.0236291587352753
5500 0.0232081431895494
5600 0.0230461768805981
5700 0.0228742249310017
5900 0.0225903075188398
6000 0.0224648304283619
6200 0.0221300013363361
6300 0.0219860877841711
6400 0.0218684077262878
6500 0.0216822102665901
6600 0.0215574279427528
6700 0.0214134231209755
6900 0.021071620285511
7000 0.0209593120962381
7100 0.0208218917250633
7300 0.0205920059233904
7400 0.0204966869205236
7500 0.0203801915049553
7600 0.0202500633895397
7700 0.0201496779918671
7800 0.0200602654367685
7900 0.0199365317821503
8100 0.0197397377341986
8200 0.019621642306447
8500 0.0193140376359224
8600 0.0192248970270157
8700 0.0191471241414547
8800 0.0190169960260391
8900 0.0189204830676317
9000 0.0188152622431517
9100 0.0187287982553244
9200 0.018619142472744
9300 0.0185727756470442
9400 0.0185021888464689
9500 0.0184599217027426
9600 0.0183704067021608
9800 0.0182033833116293
9900 0.0180918220430613
10000 0.017962533980608
10100 0.0178694054484367
10200 0.0177543498575687
10300 0.0176588073372841
10500 0.0174989383667707
10700 0.0173934604972601
10800 0.0173153709620237
10900 0.0172220394015312
11000 0.0171412937343121
11100 0.0170316491276026
11200 0.0169676952064037
11400 0.0168036464601755
11500 0.0167601257562637
11600 0.0166821628808975
11700 0.0165668316185474
11800 0.0164874698966742
11900 0.0164590999484062
12000 0.0163531918078661
12100 0.0163032226264477
12300 0.0162204261869192
12400 0.0161084327846766
12500 0.016071904450655
12800 0.0158610977232456
12900 0.0158600956201553
13100 0.0157244391739368
13200 0.0156792141497135
13300 0.0156196299940348
13400 0.0155038507655263
13500 0.0154104707762599
13600 0.0153341311961412
13700 0.0152724115177989
13800 0.015203857794404
13900 0.0151695245876908
14000 0.0151463663205504
14100 0.0150967901572585
14300 0.0149604612961411
14400 0.0149099184200168
14500 0.014843606390059
14600 0.0148123884573579
14700 0.014791346155107
14800 0.0147771183401346
14900 0.0147377494722605
15200 0.0145905986428261
15300 0.0145134432241321
15500 0.0144136594608426
15600 0.0143792005255818
15700 0.0142927002161741
15800 0.0143054639920592
15900 0.014242728240788
16000 0.0142049146816134
16100 0.0141588868573308
16200 0.0141407484188676
16300 0.0140512157231569
16500 0.0140340011566877
16600 0.0139999855309725
16700 0.0139376325532794
16800 0.0139248026534915
17000 0.0138608627021313
17100 0.0138021148741245
17200 0.0138110164552927
17300 0.0137335127219558
17400 0.0136742601171136
17500 0.0136511167511344
17600 0.0135886501520872
17700 0.0135458642616868
17800 0.0135488845407963
17900 0.0134980846196413
18000 0.0134716043248773
18100 0.0134827913716435
18200 0.0134320259094238
18300 0.0133959129452705
18400 0.0133938463404775
18500 0.0132926935330033
18600 0.0132384318858385
18700 0.0132275894284248
18900 0.0131007190793753
19000 0.0131120374426246
19400 0.0130110448226333
19600 0.0129259433597326
19700 0.0129063623026013
19800 0.0128953913226724
19900 0.0128756519407034
20100 0.0128565458580852
20200 0.0127760553732514
20300 0.0127369575202465
20400 0.0127216642722487
20500 0.0126699768006802
20600 0.0126441633328795
20700 0.0126420669257641
20900 0.0125611303374171
21000 0.0125522930175066
21100 0.0125107131898403
21200 0.0124879516661167
21300 0.0124733308330178
21400 0.0124403312802315
21500 0.012374971061945
21600 0.0123389568179846
21700 0.0123277986422181
21800 0.0123084373772144
22000 0.012323890812695
22100 0.0123391458764672
22300 0.0122507391497493
22400 0.0122160920873284
22500 0.012190249748528
22600 0.0121308974921703
22700 0.0121342642232776
22800 0.0121204070746899
22900 0.0120781920850277
23000 0.0120641691610217
23100 0.0120582561939955
23200 0.0120221106335521
23400 0.0120556820183992
23500 0.012033874168992
23700 0.012019157409668
23900 0.011939812451601
24000 0.0119178453460336
24100 0.011914286762476
24300 0.0118686025962234
24400 0.0118584949523211
24500 0.0118426308035851
24600 0.0117985429242253
24700 0.0118239084258676
25100 0.0117551805451512
25200 0.0117189101874828
25300 0.0117401434108615
25400 0.0117234857752919
25500 0.0117299715057015
25600 0.0117471674457192
25800 0.0117098167538643
25900 0.0117299715057015
26000 0.0117376977577806
26100 0.0117337554693222
};
\addlegendentry{Baseline}
\addplot [ultra thick, blue,  ]
table {%
0 0.0544329546391964
100 0.0542538948357105
200 0.0538675598800182
300 0.0532926768064499
400 0.052450206130743
500 0.0513713844120502
600 0.0500374063849449
700 0.0485850796103477
800 0.0471259616315365
900 0.0457695946097374
1000 0.0445034466683865
1100 0.0434341281652451
1400 0.0408206805586815
1500 0.0400197766721249
1600 0.0393495000898838
1700 0.0387455262243748
1800 0.0382350236177444
1900 0.0377727597951889
2000 0.0373697355389595
2100 0.0369039922952652
2300 0.0358095169067383
2400 0.0351712740957737
2500 0.034451637417078
2600 0.033703401684761
2700 0.0330094210803509
2800 0.0322677753865719
2900 0.031666737049818
3200 0.0301722250878811
3400 0.0292610004544258
3500 0.0287890732288361
3600 0.0284040402621031
3700 0.0280440784990788
3800 0.0277284868061543
3900 0.0273853316903114
4000 0.0270802900195122
4100 0.0267292894423008
4200 0.0264112558215857
4300 0.0260820537805557
4500 0.0255271084606647
4600 0.0253022145479918
4700 0.0250189080834389
4800 0.0247778203338385
4900 0.0245504919439554
5000 0.0242961123585701
5100 0.0240184664726257
5200 0.0238253846764565
5300 0.0235891602933407
5400 0.0233670528978109
5500 0.0231796987354755
5600 0.0230237189680338
5700 0.0228442512452602
5800 0.022703455761075
5900 0.0225359611213207
6100 0.0222535580396652
6200 0.0220827739685774
6300 0.0219365898519754
6400 0.0218022502958775
6500 0.021622022613883
6700 0.0213265437632799
6800 0.0211580879986286
6900 0.0210130866616964
7000 0.0208878833800554
7100 0.0207185577601194
7200 0.0206089969724417
7400 0.0203615501523018
7500 0.0202243458479643
7600 0.0201126895844936
7900 0.0198242645710707
8000 0.0197166744619608
8100 0.0195994861423969
8400 0.0192834865301847
8500 0.0192055869847536
8600 0.0191373508423567
8700 0.019048785790801
8800 0.0189191177487373
8900 0.0188135001808405
9000 0.0187192130833864
9100 0.0186352077871561
9200 0.0185146667063236
9300 0.0184420589357615
9400 0.0183891449123621
9500 0.0183021686971188
9600 0.0181869361549616
9700 0.0180993713438511
9800 0.0180008392781019
9900 0.0178767703473568
10000 0.0177760943770409
10100 0.0176884178072214
10200 0.0175838023424149
10300 0.0175022631883621
10500 0.0173247996717691
10700 0.0171729549765587
10800 0.0171127952635288
11000 0.0169262569397688
11100 0.0168566722422838
11200 0.0168075859546661
11300 0.016707656905055
11400 0.0166737399995327
11500 0.0166164096444845
11600 0.0165324974805117
11700 0.0164189003407955
11800 0.0163614265620708
11900 0.0162894111126661
12100 0.0161133781075478
12200 0.0160762947052717
12600 0.0158159397542477
12800 0.0156408753246069
13000 0.0155513137578964
13200 0.015403619967401
13300 0.015382400713861
13500 0.0151735479012132
13600 0.0151207279413939
13700 0.0150832170620561
13800 0.0149945104494691
13900 0.014954837039113
14000 0.014944520778954
14100 0.0148839000612497
14200 0.0148148853331804
14400 0.0146529683843255
14500 0.0145602207630873
14600 0.0145228682085872
14700 0.0144540155306458
14800 0.0144231459125876
14900 0.0144092096015811
15000 0.0143582969903946
15100 0.0143211362883449
15200 0.0142987901344895
15500 0.0141370464116335
15600 0.0140709728002548
15700 0.0139926746487617
15800 0.0139889372512698
15900 0.0139181157574058
16000 0.0138871362432837
16100 0.0138452844694257
16200 0.0138457287102938
16300 0.0137940244749188
16400 0.0137655586004257
16500 0.0137470411136746
16600 0.0137071944773197
16700 0.013616481795907
16800 0.0135802607983351
16900 0.0135372001677752
17000 0.0134795680642128
17100 0.0134095177054405
17200 0.0134109826758504
17300 0.0133547456935048
17400 0.0133197139948606
17500 0.0133050614967942
17600 0.0132798822596669
17700 0.0132426582276821
17900 0.0131350196897984
18000 0.0130956033244729
18100 0.0130707416683435
18200 0.0130211841315031
18400 0.0129545535892248
18500 0.0129052177071571
18600 0.0128809930756688
18700 0.0128457378596067
19200 0.01272246055305
19500 0.0125521654263139
19600 0.0124807041138411
19700 0.0124702770262957
19900 0.0124641414731741
20100 0.0124177942052484
20200 0.0123245874419808
20300 0.0123109817504883
20500 0.0122418412938714
20600 0.0122330039739609
20700 0.0122308721765876
20800 0.012161954306066
20900 0.0121272085234523
21000 0.0121113145723939
21100 0.0120745319873095
21200 0.012055748142302
21300 0.012029392644763
21400 0.0120164854452014
21500 0.0119615877047181
21600 0.0119199752807617
21800 0.0118838623166084
21900 0.0118325548246503
22100 0.0118004474788904
22200 0.0117649706080556
22300 0.0117218345403671
22400 0.011719798669219
22500 0.0117008527740836
22600 0.0116551714017987
22700 0.0116476686671376
22800 0.0116086006164551
22900 0.0115527464076877
23100 0.0115398727357388
23200 0.0115034431219101
23400 0.0115090049803257
23500 0.0114686647430062
23600 0.0114504173398018
23700 0.0114414850249887
23800 0.011411857791245
23900 0.011369195766747
24000 0.0113437036052346
24100 0.0113436067476869
24200 0.0112866079434752
24400 0.011227416805923
24500 0.0111809717491269
24600 0.0111235324293375
24900 0.0110973352566361
25000 0.0110740661621094
25100 0.0110714277252555
25200 0.0110331848263741
25300 0.0109899202361703
25400 0.0109410928562284
25500 0.0109192216768861
25600 0.0108782453462481
25700 0.0108676897361875
25800 0.0108914040029049
26000 0.0108920074999332
26100 0.0108674364164472
26200 0.0108532253652811
26300 0.0107914274558425
26400 0.0107691138982773
26500 0.0107230478897691
26600 0.0107118282467127
26700 0.010670599527657
26800 0.0106612835079432
26900 0.0106664970517159
27100 0.0106880497187376
27200 0.0106755886226892
27300 0.0106816617771983
27400 0.0106479655951262
27500 0.0106235183775425
27600 0.0105671556666493
27700 0.0105658527463675
28000 0.0104643832892179
28100 0.0104667646810412
28200 0.0104305585846305
28300 0.0104024549946189
28400 0.010402106679976
28500 0.0103946691378951
28600 0.0103486683219671
28700 0.0103195197880268
28800 0.01030816975981
28900 0.0102663049474359
29000 0.0102435136213899
29100 0.01026058383286
29200 0.0102458642795682
29300 0.0102194789797068
29400 0.0102159501984715
29500 0.0102061601355672
29600 0.0101382881402969
29900 0.0100852968171239
30000 0.0100390752777457
30100 0.0100714368745685
30200 0.0100418729707599
30300 0.0100369453430176
30400 0.0100267101079226
30500 0.0100234961137176
30600 0.00996039807796478
30700 0.00993919372558594
30800 0.00990711897611618
31000 0.0098753310739994
31100 0.00989650189876556
31200 0.00990324188023806
31300 0.00993493385612965
31400 0.00992488674819469
31500 0.00991977192461491
31600 0.00988527853041887
31700 0.00988003239035606
31800 0.00984630454331636
31900 0.00982281379401684
32100 0.009826535359025
32200 0.00982211250811815
32400 0.00977910216897726
32700 0.00972226541489363
32800 0.00969304982572794
32900 0.0096994424238801
33000 0.00967560149729252
33100 0.00968592707067728
33200 0.00967127270996571
33300 0.00967772584408522
33400 0.00967035442590714
33500 0.00965776480734348
33600 0.0096351308748126
33700 0.00963487755507231
33900 0.00961408577859402
34000 0.00962088629603386
34100 0.00959625281393528
34200 0.00957676488906145
34300 0.00956204440444708
34400 0.00955244805663824
34500 0.00954809132963419
34600 0.00955168250948191
34900 0.00953928381204605
35000 0.00954831670969725
35100 0.00954186078161001
35400 0.00953623652458191
35500 0.00952040310949087
35600 0.00952704809606075
35700 0.00951855815947056
35800 0.00952081568539143
35900 0.00951315648853779
36000 0.00949818547815084
36200 0.00950098037719727
36300 0.00947774108499289
36400 0.00948025472462177
36500 0.00949367042630911
36600 0.00947344955056906
36700 0.00946146436035633
36800 0.00948009267449379
36900 0.00946871284395456
37000 0.0094464598223567
37100 0.00944026466459036
37200 0.00944859161973
37300 0.009432727470994
37400 0.00942643266171217
37500 0.00943040754646063
37600 0.00944115128368139
37700 0.00942319352179766
37800 0.00942770577967167
37900 0.00942688249051571
38000 0.00942141376435757
38100 0.00940068624913692
38200 0.00939029268920422
38300 0.00938936974853277
38500 0.0093740476295352
38600 0.00938510801643133
38700 0.00942011084407568
38800 0.0094093345105648
39100 0.00939041655510664
39200 0.00935596134513617
39300 0.00935477949678898
39400 0.00936342682689428
39600 0.00934477057307959
39700 0.00934661272913218
39800 0.00934422668069601
39900 0.0093339579179883
40000 0.0093359611928463
40200 0.00932769849896431
40400 0.00930541381239891
40700 0.00928853545337915
40800 0.00927397329360247
40900 0.00927861221134663
41000 0.00927416700869799
41100 0.00927546992897987
41200 0.00926822237670422
41300 0.00927200354635715
41800 0.00926993694156408
42100 0.00924444012343884
42300 0.00924628786742687
42400 0.00925512425601482
42500 0.00924781057983637
42600 0.00924898870289326
42700 0.00924370996654034
42800 0.00923179183155298
42900 0.00921360589563847
43000 0.0092069311067462
43200 0.0092200618237257
43300 0.00921652931720018
43400 0.00922504905611277
43500 0.00922123622149229
43600 0.00920047890394926
43900 0.00915918499231339
44200 0.00917895697057247
44300 0.00919774174690247
44400 0.00919561181217432
44500 0.00920556206256151
44700 0.00919733289629221
44800 0.00917911343276501
44900 0.00917297787964344
};
\addlegendentry{K1}
\addplot [ultra thick, green!39.2156862745098!black,  ]
table {%
0 0.0636693313717842
100 0.0616101957857609
200 0.0591515451669693
300 0.056608609855175
400 0.0542661361396313
500 0.052734013646841
600 0.0520671382546425
700 0.0517956167459488
900 0.0515038184821606
1000 0.0511078648269176
1100 0.0502656362950802
1200 0.049069419503212
1300 0.0476103611290455
1400 0.0457979328930378
1500 0.0439452715218067
1600 0.0420238375663757
1700 0.039841677993536
1800 0.0371202230453491
1900 0.0341668166220188
2000 0.0311870444566011
2100 0.0285581424832344
2200 0.0263693351298571
2300 0.0247243661433458
2400 0.0234325230121613
2500 0.022318297997117
2600 0.0212215557694435
2700 0.020207554101944
2800 0.0193783231079578
2900 0.0187454055994749
3000 0.0182127896696329
3100 0.0177700202912092
3300 0.0169527269899845
3700 0.0154489735141397
3800 0.0150637710466981
3900 0.0147127136588097
4100 0.0140069387853146
4200 0.0136939836665988
4300 0.0134233459830284
4400 0.013206503354013
4500 0.0130100520327687
4600 0.0128278592601418
4700 0.0126698100939393
4800 0.0125195998698473
4900 0.0123492330312729
5000 0.0121871251612902
5100 0.0120611265301704
5200 0.0119048850610852
5400 0.0116539718583226
5600 0.0114352470263839
5800 0.0112469913437963
5900 0.011168478988111
6000 0.0110651720315218
6100 0.0109744854271412
6200 0.0109028182923794
6400 0.0106938667595387
6500 0.0106177488341928
6600 0.0105210524052382
6700 0.010431781411171
6800 0.0103582944720984
6900 0.010279942303896
7000 0.0102274091914296
7100 0.0101952403783798
7300 0.0100831184536219
7400 0.0100454483181238
7500 0.009974280372262
7600 0.0099115464836359
7700 0.00987546611577272
7800 0.00981199648231268
7900 0.00977888237684965
8000 0.00973082426935434
8100 0.00966986082494259
8200 0.00959778111428022
8300 0.00957708526402712
8400 0.00951219629496336
8800 0.00930551066994667
8900 0.00924687180668116
9400 0.00904380716383457
9500 0.00899581983685493
9600 0.00894397217780352
9900 0.00881303194910288
10000 0.00877923890948296
10100 0.00873635802417994
10200 0.00868757534772158
10300 0.0086481561884284
10400 0.00861290562897921
10500 0.00858748517930508
10600 0.00857675820589066
10700 0.00854484178125858
10800 0.00851850584149361
10900 0.00850006751716137
11000 0.00843782350420952
11100 0.00841876491904259
11200 0.00842550583183765
11300 0.00839595962315798
11400 0.00834767054766417
11500 0.00834363419562578
11600 0.00830729864537716
11700 0.00824049208313227
11800 0.00823257956653833
11900 0.00823179725557566
12000 0.00821755640208721
12100 0.00817333906888962
12200 0.00816441979259253
12300 0.00812389049679041
12400 0.00806570239365101
12500 0.00803945679217577
12600 0.00803368631750345
12800 0.00798416137695312
12900 0.00797977484762669
13000 0.00794460158795118
13100 0.00793042220175266
13200 0.00791227072477341
13300 0.00785581395030022
13400 0.00785370077937841
13700 0.00776792969554663
13800 0.00775742484256625
13900 0.00770573597401381
14000 0.0077065946534276
14100 0.00766707956790924
14200 0.00763509841635823
14300 0.00761585449799895
14400 0.00758828921243548
14500 0.00754766492173076
14600 0.00752871995791793
14700 0.00752995582297444
14800 0.00751180574297905
15000 0.00749993417412043
15100 0.00748572265729308
15200 0.00743690924718976
15300 0.00742654642090201
15400 0.00738267740234733
15500 0.00735791493207216
15600 0.00735327554866672
15800 0.00732340756803751
15900 0.00732366042211652
16000 0.0072951945476234
16100 0.00727213080972433
16200 0.00726671097800136
16300 0.00724473176524043
16400 0.00725755747407675
16500 0.00725650973618031
16700 0.00721756694838405
16800 0.00720739457756281
16900 0.00716118654236197
17100 0.00713297631591558
17200 0.00714020850136876
17300 0.00713144894689322
17400 0.00713521614670753
17500 0.00712566496804357
17600 0.00710163218900561
17700 0.00708444835618138
17800 0.00706219812855124
17900 0.00703598791733384
18000 0.00701454468071461
18100 0.00701524550095201
18200 0.00699186138808727
18400 0.00699354661628604
18500 0.00700252875685692
18600 0.00699510565027595
18700 0.00699543952941895
18900 0.00697299838066101
19100 0.00694476626813412
19200 0.00695042638108134
19300 0.00694147683680058
19400 0.00694136647507548
19500 0.00692575657740235
19800 0.00688729155808687
19900 0.00688367011025548
20000 0.00686950609087944
20100 0.00685879262164235
20200 0.00683749513700604
20300 0.00684309052303433
20400 0.00682314159348607
20600 0.00682562170550227
20700 0.00680058822035789
20800 0.00678429659456015
21100 0.0067614708095789
21200 0.00676824478432536
21300 0.00674325507134199
21500 0.00673011131584644
21600 0.00673046242445707
21700 0.00673577003180981
21800 0.00673368852585554
21900 0.00672745518386364
22000 0.00672728149220347
22100 0.00670728739351034
22200 0.00669614318758249
22300 0.00670383777469397
22400 0.00669413991272449
22500 0.00668069580569863
22600 0.00667899427935481
22800 0.00666111428290606
22900 0.00666390871629119
23000 0.00665836501866579
23200 0.00663631642237306
23300 0.0066325357183814
23400 0.00661565503105521
23500 0.00660448195412755
23700 0.00661436608061194
23800 0.00660608476027846
23900 0.00660921912640333
24100 0.00657957326620817
24200 0.0065732947550714
24300 0.00656286720186472
24400 0.00654955022037029
24500 0.00657332735136151
24600 0.00657051336020231
24700 0.00655317166820168
24900 0.00654082233086228
25000 0.00651992158964276
25100 0.00651804637163877
25200 0.00650363089516759
25300 0.00650592008605599
25600 0.00646909046918154
25700 0.00647222343832254
25800 0.00647991336882114
25900 0.00648098066449165
26000 0.00649002427235246
26100 0.006472856272012
26200 0.00646788300946355
26300 0.00642827246338129
26400 0.00643660267814994
26500 0.00642102444544435
26600 0.00642681121826172
26700 0.00640597240999341
26800 0.00642410945147276
26900 0.00641056708991528
27200 0.00640031648799777
27600 0.00635887775570154
27700 0.00637125829234719
27800 0.00637151347473264
27900 0.00639513274654746
28000 0.00639564171433449
28100 0.0064159082248807
28200 0.00640672165900469
28300 0.00637998385354877
28400 0.00634904112666845
28500 0.00633005984127522
28600 0.00629455083981156
28700 0.00627932650968432
28800 0.00628113653510809
28900 0.00628820946440101
29000 0.00630086380988359
29100 0.00630574300885201
29200 0.0063220513984561
29400 0.00630113342776895
29500 0.00628493446856737
29600 0.00627970602363348
29700 0.00626357551664114
29900 0.00626678438857198
30200 0.00626503676176071
30400 0.00627341400831938
};
\addlegendentry{K2}
\addplot [ultra thick, color0]
table {%
0 0.0487121939659119
100 0.0426958575844765
200 0.0361093617975712
300 0.0324471592903137
400 0.0297905020415783
500 0.0269802305847406
600 0.0240863561630249
700 0.0222672522068024
800 0.0212216656655073
900 0.0201710388064384
1000 0.0191998947411776
1100 0.018395995721221
1200 0.0176032297313213
1300 0.0168205741792917
1400 0.016115939244628
1500 0.0154903875663877
1600 0.0149311581626534
1700 0.0144285233691335
1800 0.014001926407218
1900 0.0136566897854209
2000 0.0133321834728122
2100 0.0130836386233568
2200 0.0128151923418045
2300 0.0126295424997807
2400 0.0124217243865132
2600 0.0120522808283567
2700 0.0119481533765793
2800 0.011776078492403
2900 0.0116331242024899
3000 0.0114999925717711
3100 0.0113804014399648
3200 0.0112479450181127
3400 0.0110076749697328
3500 0.0109060537070036
3600 0.0108167929574847
3700 0.0107152890414
3900 0.0105875888839364
4000 0.0104880267754197
4400 0.0101884780451655
4500 0.0101322596892715
4600 0.0100543973967433
4900 0.00988142658025026
5100 0.0097825713455677
5300 0.0096328305080533
5400 0.00958024058490992
5500 0.00954202376306057
5600 0.0094934981316328
5700 0.00945554487407207
5800 0.00942911859601736
5900 0.00938197132200003
6000 0.00931846536695957
6100 0.00926584098488092
6200 0.00921857357025146
6300 0.0091642402112484
6700 0.00903058052062988
6800 0.00898326002061367
6900 0.0089489771053195
7000 0.00893018115311861
7100 0.00890559982508421
7200 0.00887713301926851
7300 0.00885740295052528
7400 0.00881237909197807
7500 0.00877890642732382
7600 0.00872748531401157
7700 0.00872165616601706
7800 0.00868722703307867
7900 0.00865977630019188
8000 0.00860852282494307
8100 0.0085899094119668
8200 0.00853032153099775
8300 0.00850744359195232
8400 0.00847636722028255
8500 0.00845384784042835
8600 0.00844127964228392
8700 0.00842215772718191
8800 0.00838591810315847
8900 0.0083590978756547
9000 0.00834658928215504
9100 0.00829213485121727
9200 0.00825258903205395
9300 0.00823508854955435
9400 0.00822235830128193
9500 0.00818688794970512
9600 0.00815774407237768
9700 0.00814289320260286
9800 0.00811795610934496
9900 0.00808227062225342
10000 0.00805432163178921
10100 0.00804061349481344
10200 0.00801081117242575
10300 0.00799286272376776
10400 0.00796616729348898
10500 0.0079668927937746
10600 0.00796158984303474
10700 0.00794385932385921
10800 0.00789716467261314
10900 0.00788242090493441
11000 0.00782430823892355
11100 0.00779139390215278
11200 0.00777262169867754
11300 0.00777482846751809
11400 0.00773416506126523
11500 0.0077108689583838
11600 0.00767653062939644
11800 0.00763432309031487
12000 0.00764265097677708
12100 0.00763182574883103
12200 0.00760032562538981
12300 0.00757300807163119
12400 0.00753432232886553
12500 0.00750650418922305
12600 0.00748786795884371
12800 0.00746526848524809
12900 0.00748158106580377
13000 0.00746500631794333
13100 0.00745733035728335
13200 0.00743938377127051
13300 0.00740501051768661
13400 0.0073643121868372
13500 0.00734662171453238
13600 0.00732228578999639
13700 0.00730225862935185
13800 0.00727209867909551
13900 0.00727183138951659
14000 0.00725928274914622
14200 0.00722460728138685
14300 0.00721531640738249
14400 0.00717562157660723
14500 0.00714835477992892
14600 0.00713882502168417
14700 0.00713416654616594
14800 0.00713934237137437
14900 0.0071297069080174
15000 0.0071255280636251
15200 0.00708035798743367
15300 0.0070519121363759
15400 0.00702916597947478
15500 0.00702512310817838
15600 0.00701563432812691
15800 0.00700660469010472
15900 0.00700762402266264
16000 0.00697306729853153
16300 0.00691866176202893
16400 0.00690600974485278
16500 0.00690390216186643
16600 0.00690909288823605
16700 0.0069062071852386
16800 0.00690694665536284
16900 0.00691383564844728
17000 0.00691629946231842
17100 0.00689756823703647
17200 0.00689606880769134
17300 0.00687453849241138
17400 0.00686330907046795
17500 0.00684899464249611
17600 0.00685212761163712
17700 0.00684131775051355
17800 0.00684560043737292
17900 0.00682157604023814
18000 0.00681652966886759
18100 0.00679939705878496
18200 0.00678672920912504
18300 0.00676972744986415
18400 0.00676731206476688
18500 0.00675238622352481
18600 0.00676473043859005
18700 0.00675232335925102
18800 0.00677275704219937
18900 0.00677716778591275
19000 0.00677128462120891
19100 0.00674824696034193
19200 0.00675428844988346
19400 0.00670174043625593
19500 0.00671362737193704
19600 0.00670165941119194
19700 0.00669604772701859
19800 0.00668724207207561
19900 0.00669057993218303
20000 0.00667594093829393
20100 0.00667756469920278
20200 0.00666732667014003
20300 0.00667160283774137
20400 0.00666739232838154
20500 0.00665140151977539
20600 0.00665585044771433
20700 0.00663461489602923
20800 0.00661878660321236
21100 0.00658990442752838
21200 0.00661287363618612
21300 0.00662310840561986
21400 0.00663873227313161
21700 0.00661026779562235
21900 0.00658456329256296
22000 0.00659688329324126
22100 0.00658799847587943
22200 0.00657478906214237
22300 0.00656673032790422
22400 0.00656498223543167
22600 0.00654835626482964
22800 0.0065492014400661
22900 0.00653491076081991
23000 0.00653171492740512
23100 0.00653201621025801
23300 0.00652461219578981
23400 0.00652441848069429
23500 0.00651933439075947
23600 0.00652767904102802
23700 0.00653119152411819
23800 0.00652050832286477
23900 0.00652071600779891
24000 0.00652586575597525
24200 0.00650202436372638
24500 0.00650960672646761
24600 0.00650420226156712
24700 0.00650765234604478
24800 0.00650661624968052
24900 0.00650990707799792
25000 0.00649676145985723
25100 0.00650022923946381
25200 0.00649224780499935
25300 0.00649564899504185
25400 0.00648325122892857
25500 0.00648376019671559
25600 0.00648113759234548
25700 0.00647264998406172
25800 0.0064590941183269
25900 0.00646715192124248
26000 0.00647055404260755
26100 0.00646311277523637
26200 0.00646715192124248
26300 0.00646737543866038
26400 0.00645805848762393
26500 0.00645290920510888
26600 0.00645418139174581
26700 0.00644650403410196
26800 0.00644372310489416
26900 0.0064363656565547
27000 0.00642520608380437
27300 0.00644168956205249
27800 0.00643737986683846
27900 0.00644607609137893
28000 0.00644273636862636
28200 0.00642417278140783
28300 0.00642636697739363
28400 0.006411362439394
28500 0.00641881441697478
28600 0.00641814852133393
28700 0.00642293179407716
28800 0.0064142388291657
28900 0.00642024539411068
29000 0.00640676729381084
29100 0.00641617923974991
29200 0.00641408003866673
29300 0.00640381034463644
29400 0.00640069600194693
29500 0.00641500297933817
29600 0.00640007760375738
29700 0.00639019114896655
29800 0.00639793137088418
30000 0.00637311907485127
30100 0.00637235678732395
30200 0.00636432971805334
30300 0.00636077020317316
30400 0.00637532724067569
30600 0.00637446995824575
30700 0.0063773961737752
31100 0.00636162608861923
31200 0.00636359956115484
31300 0.00636226171627641
};
\addlegendentry{K3}
\addplot [ultra thick, white!40.2745098039216!black,  ]
table {%
0 0.0491654649376869
100 0.0431270524859428
200 0.0363886058330536
300 0.0322390757501125
400 0.029566241428256
500 0.0267833285033703
600 0.0239019766449928
700 0.0222393739968538
800 0.0211947374045849
1000 0.0191011186689138
1100 0.0183004960417747
1200 0.017491614446044
1300 0.0166925191879272
1400 0.0160186029970646
1500 0.0154156452044845
1600 0.0148615119978786
1700 0.0143752349540591
1800 0.0139840040355921
1900 0.0136323571205139
2000 0.0133131425827742
2100 0.0130619397386909
2200 0.0128217302262783
2300 0.0126251894980669
2400 0.0124376341700554
2500 0.0122464932501316
2600 0.0120835639536381
2700 0.0119637316092849
2800 0.0118101360276341
3000 0.0115632163360715
3100 0.0114359250292182
3200 0.0112884668633342
3300 0.011163629591465
3400 0.0110217668116093
3500 0.0109107429161668
3600 0.0107890255749226
3700 0.0106936963275075
3900 0.010522898286581
4000 0.0104267029091716
4200 0.0103143937885761
4500 0.0101122660562396
4600 0.0100573729723692
4700 0.00998013559728861
4800 0.00991978775709867
4900 0.00985534675419331
5000 0.00980902370065451
5100 0.00974320992827415
5200 0.00968482624739408
5300 0.00960940588265657
5500 0.00951881427317858
5600 0.0094665763899684
5700 0.00944928172975779
5800 0.00941809918731451
5900 0.00937694031745195
6100 0.00926348101347685
6200 0.00918970163911581
6500 0.00908433645963669
6700 0.00900416541844606
6800 0.00895731337368488
6900 0.00892392732203007
7000 0.00890197791159153
7200 0.008890968747437
7300 0.0088575342670083
7500 0.00876447465270758
7600 0.00869392044842243
7700 0.00865115225315094
7800 0.00863513350486755
7900 0.00860566459596157
8000 0.00856986735016108
8100 0.00854891911149025
8200 0.0085081160068512
8300 0.00847732182592154
8400 0.00845758896321058
8500 0.00843316502869129
8600 0.00841703172773123
8700 0.00839633774012327
8900 0.00832046195864677
9000 0.00829114764928818
9100 0.00825550686568022
9300 0.00821702461689711
9600 0.00814297422766685
9700 0.00810384564101696
9900 0.00806174520403147
10000 0.00805004313588142
10300 0.00795845221728086
10400 0.007919667288661
10600 0.0078977020457387
10700 0.00788183230906725
10800 0.00785555131733418
10900 0.00785235594958067
11000 0.00780161889269948
11100 0.00778468558564782
11200 0.00777348829433322
11300 0.00776983192190528
11400 0.00773034011945128
11500 0.00770722096785903
11600 0.00766965607181191
11700 0.00762546854093671
11800 0.007601547986269
12200 0.00759883597493172
12300 0.00756706530228257
12500 0.00749367056414485
12600 0.0074729691259563
12700 0.00743910623714328
12800 0.0074173379689455
12900 0.00741233956068754
13000 0.00738657312467694
13100 0.00735669955611229
13200 0.00735389301553369
13300 0.00732952076941729
13400 0.00729143479838967
13500 0.00728286989033222
13600 0.00726943230256438
13700 0.00723985722288489
13800 0.00721747940406203
13900 0.00722115766257048
14000 0.00720434868708253
14100 0.00717652728781104
14300 0.00716931745409966
14400 0.00714542763307691
14500 0.00713379448279738
14600 0.00715325772762299
14700 0.00713306991383433
14800 0.0071240495890379
14900 0.00712234852835536
15000 0.00710995309054852
15100 0.00706437323242426
15200 0.00705174589529634
15300 0.00702734850347042
15400 0.00698553072288632
15500 0.00696639018133283
15600 0.00696740765124559
15700 0.00695754634216428
15800 0.00695163989439607
15900 0.00696130562573671
16000 0.00695728277787566
16100 0.00694859120994806
16200 0.0069310967810452
16300 0.00693143159151077
16400 0.00692609883844852
16500 0.00692749815061688
16600 0.00690179551020265
16700 0.00690514175221324
16800 0.00687147118151188
16900 0.00686961924657226
17000 0.00683229090645909
17100 0.00682808784767985
17200 0.00680337753146887
17300 0.00679746409878135
17400 0.00677926652133465
17500 0.00678788777440786
17700 0.00675950758159161
17800 0.00674878805875778
17900 0.0067204306833446
18000 0.00667623756453395
18100 0.00666326470673084
18200 0.00666646286845207
18300 0.00663827266544104
18400 0.00662212306633592
18500 0.00662872800603509
18600 0.00663073733448982
18700 0.00661459844559431
18800 0.00662781484425068
18900 0.00662665441632271
19200 0.00656062643975019
19300 0.00654842099174857
19400 0.00652729533612728
19500 0.00652823410928249
19600 0.00649898778647184
19700 0.0065004825592041
19800 0.00647363811731339
20000 0.00646058702841401
20100 0.00646686414256692
20300 0.00644265860319138
20600 0.00641530239954591
20700 0.00640068203210831
20800 0.00640780152752995
21000 0.00639104750007391
21100 0.00638904422521591
21200 0.00638211378827691
21300 0.0063691632822156
21400 0.00637227622792125
21500 0.00636223005130887
21600 0.00636280281469226
21700 0.00635970523580909
21800 0.00635188585147262
21900 0.00635099364444613
22000 0.00634702015668154
22100 0.00633440166711807
22300 0.00633064704015851
22400 0.00632250960916281
22600 0.00632748520001769
22800 0.00632138177752495
22900 0.00632877415046096
23100 0.00631338777020574
23200 0.00631086155772209
23300 0.00631469069048762
23400 0.00630536209791899
23500 0.00630208477377892
23600 0.00630302261561155
23700 0.00631025526672602
23800 0.0063051232136786
23900 0.00630424777045846
24000 0.00629758881404996
24100 0.00630089500918984
24200 0.00629518646746874
24300 0.00630065612494946
24500 0.00629995763301849
24600 0.00629375595599413
24900 0.00625915499404073
25100 0.00625198800116777
25200 0.006259361281991
25300 0.00625726534053683
25400 0.0062523209489882
25500 0.00625461060553789
25600 0.00624918797984719
25700 0.00623656855896115
25800 0.00623590126633644
25900 0.00624297466129065
26000 0.00623871572315693
26100 0.00624200468882918
26200 0.00625492632389069
26400 0.00624556606635451
26500 0.00624944502487779
26600 0.00624449970200658
26700 0.00622663414105773
27000 0.00623025838285685
27100 0.00624888576567173
27300 0.00624442100524902
27400 0.00623548682779074
27500 0.00623049819841981
27600 0.00622153282165527
27800 0.00622361665591598
27900 0.00623060762882233
28200 0.00621622381731868
28500 0.00619111023843288
28600 0.00618561031296849
28800 0.0061962278559804
29000 0.00619509862735868
29300 0.00616957247257233
29400 0.00617508869618177
29500 0.00616917619481683
29600 0.00616701599210501
29700 0.00616855639964342
29800 0.00617361115291715
29900 0.00616327952593565
30000 0.00616409117355943
30100 0.00615948066115379
30200 0.00616207160055637
30300 0.00615123240277171
30400 0.00614937208592892
30500 0.00615022936835885
30700 0.00614166306331754
30800 0.00614929106086493
30900 0.00615096231922507
31000 0.00613563740625978
31100 0.00614048633724451
31300 0.00614302838221192
31400 0.00613815058022738
31500 0.00613794149830937
31600 0.0061268019489944
31700 0.00611918838694692
31800 0.00611540349200368
31900 0.00611745519563556
32000 0.00613055331632495
32100 0.0061316336505115
32300 0.00614123465493321
32400 0.00613233400508761
32500 0.00611991714686155
32600 0.00612808996811509
32700 0.00611928245052695
};
\addlegendentry{K4}

==> supp_mat/ant_plots/traj_err_data.tex <==
\definecolor{color0}{rgb}{1,0,1}

\path [fill=red, fill opacity=0.4, ultra thick]
(axis cs:1,0.383586272763004)
--(axis cs:1,0.341202610256376)
--(axis cs:10,0.367361768217054)
--(axis cs:25,0.319796351289705)
--(axis cs:75,0.327496231149024)
--(axis cs:200,0.302293175970288)
--(axis cs:500,0.299483923885149)
--(axis cs:500,0.408135160747947)
--(axis cs:500,0.408135160747947)
--(axis cs:200,0.407625694391887)
--(axis cs:75,0.436331474775788)
--(axis cs:25,0.425815033510392)
--(axis cs:10,0.442076923031832)
--(axis cs:1,0.383586272763004)
--cycle;

\path [fill=blue, fill opacity=0.4, ultra thick]
(axis cs:1,0.378788589702575)
--(axis cs:1,0.334688626313886)
--(axis cs:10,0.247467385134213)
--(axis cs:25,0.191879685682561)
--(axis cs:75,0.168319706635742)
--(axis cs:200,0.130946656629393)
--(axis cs:500,0.135532023953662)
--(axis cs:500,0.167496070424621)
--(axis cs:500,0.167496070424621)
--(axis cs:200,0.175287994115066)
--(axis cs:75,0.203453582057347)
--(axis cs:25,0.236824416902666)
--(axis cs:10,0.298414471136665)
--(axis cs:1,0.378788589702575)
--cycle;

\path [fill=green!50.1960784313725!black, fill opacity=0.4, ultra thick]
(axis cs:1,0.605682180861764)
--(axis cs:1,0.531938436029615)
--(axis cs:10,0.156418200779452)
--(axis cs:25,0.128638107683799)
--(axis cs:75,0.10911213326964)
--(axis cs:200,0.115090025036464)
--(axis cs:500,0.111470364318783)
--(axis cs:500,0.147809566878869)
--(axis cs:500,0.147809566878869)
--(axis cs:200,0.153399032182911)
--(axis cs:75,0.140587884401561)
--(axis cs:25,0.165873101743983)
--(axis cs:10,0.2024450106049)
--(axis cs:1,0.605682180861764)
--cycle;

\path [fill=color0, fill opacity=0.4, ultra thick]
(axis cs:1,0.599461083321354)
--(axis cs:1,0.527050921055466)
--(axis cs:10,0.379342079288971)
--(axis cs:25,0.146077175817807)
--(axis cs:75,0.122862885020942)
--(axis cs:200,0.112970145249631)
--(axis cs:500,0.113280933710017)
--(axis cs:500,0.155025004017252)
--(axis cs:500,0.155025004017252)
--(axis cs:200,0.143993104548496)
--(axis cs:75,0.158711252659485)
--(axis cs:25,0.183024958214832)
--(axis cs:10,0.448118709653378)
--(axis cs:1,0.599461083321354)
--cycle;

\path [fill=white!50.1960784313725!black, fill opacity=0.4, ultra thick]
(axis cs:1,0.603132169970756)
--(axis cs:1,0.530037687536275)
--(axis cs:10,0.386128986556324)
--(axis cs:25,0.146518969815949)
--(axis cs:75,0.126070911216527)
--(axis cs:200,0.114498525452292)
--(axis cs:500,0.108960797960616)
--(axis cs:500,0.145501110774923)
--(axis cs:500,0.145501110774923)
--(axis cs:200,0.149259511014837)
--(axis cs:75,0.154341881685116)
--(axis cs:25,0.181061946002654)
--(axis cs:10,0.460149184044299)
--(axis cs:1,0.603132169970756)
--cycle;

\addplot [ ultra thick, red, mark=*, mark size=1.5, mark options={solid}]
table {%
1 0.362394481897354
10 0.404719293117523
25 0.372805684804916
75 0.381913870573044
200 0.354959458112717
500 0.353809475898743
};
\addplot [ ultra thick, blue, mark=*, mark size=1.5, mark options={solid}]
table {%
1 0.356738537549973
10 0.272940933704376
25 0.214352056384087
75 0.185886666178703
200 0.153117299079895
500 0.151514068245888
};
\addplot [ ultra thick, green!50.1960784313725!black, mark=*, mark size=1.5, mark options={solid}]
table {%
1 0.568810284137726
10 0.179431572556496
25 0.147255569696426
75 0.124850012362003
200 0.13424451649189
500 0.129639953374863
};
\addplot [ ultra thick, color0, mark=*, mark size=1.5, mark options={solid}]
table {%
1 0.563256025314331
10 0.413730323314667
25 0.164551079273224
75 0.140787035226822
200 0.128481641411781
500 0.134152933955193
};
\addplot [ ultra thick, white!50.1960784313725!black, mark=*, mark size=1.5, mark options={solid}]
table {%
1 0.566584944725037
10 0.423139154911041
25 0.163790449500084
75 0.140206411480904
200 0.131879016757011
500 0.127230957150459
};


==> supp_mat/double_pend/error_vs_time_data.tex <==
\definecolor{color0}{rgb}{1,0,1}

\path [fill=red, fill opacity=0.4, ultra thick]
(axis cs:0.01,0.0101700500701365)
--(axis cs:0.01,0.00701536951257345)
--(axis cs:0.02,0.00980580248473079)
--(axis cs:0.03,0.0124468241376909)
--(axis cs:0.04,0.0149700209127562)
--(axis cs:0.05,0.0173889602233553)
--(axis cs:0.06,0.019709915139098)
--(axis cs:0.07,0.0219357885475528)
--(axis cs:0.08,0.0240677567493695)
--(axis cs:0.09,0.0261056926360533)
--(axis cs:0.1,0.0280485774465258)
--(axis cs:0.11,0.0298950133783)
--(axis cs:0.12,0.0316436507092191)
--(axis cs:0.13,0.033293204228407)
--(axis cs:0.14,0.0348425974963624)
--(axis cs:0.15,0.0362910856920826)
--(axis cs:0.16,0.0376383269402774)
--(axis cs:0.17,0.0388847121434407)
--(axis cs:0.18,0.0400316231675373)
--(axis cs:0.19,0.0410818637534183)
--(axis cs:0.2,0.0420400088929378)
--(axis cs:0.21,0.0429128212873142)
--(axis cs:0.22,0.0437094850591583)
--(axis cs:0.23,0.04444163602413)
--(axis cs:0.24,0.0451231416248391)
--(axis cs:0.25,0.0457695137683184)
--(axis cs:0.26,0.0463966792899072)
--(axis cs:0.27,0.047019921561732)
--(axis cs:0.28,0.0476530036660243)
--(axis cs:0.29,0.0483074685652342)
--(axis cs:0.3,0.0489921902922463)
--(axis cs:0.31,0.0497132941749416)
--(axis cs:0.32,0.050474443898869)
--(axis cs:0.33,0.0512773573234808)
--(axis cs:0.34,0.0521224717466439)
--(axis cs:0.35,0.0530097559704964)
--(axis cs:0.36,0.0539392613480847)
--(axis cs:0.37,0.0549115261977633)
--(axis cs:0.38,0.0559275695593664)
--(axis cs:0.39,0.0569887308338322)
--(axis cs:0.4,0.0580963877090027)
--(axis cs:0.41,0.0592517168422132)
--(axis cs:0.42,0.0604554143518914)
--(axis cs:0.43,0.0617077239886599)
--(axis cs:0.44,0.063008418018531)
--(axis cs:0.45,0.0643568340075879)
--(axis cs:0.46,0.0657519801640875)
--(axis cs:0.47,0.0671926691064594)
--(axis cs:0.48,0.068677627412142)
--(axis cs:0.49,0.0702055366734654)
--(axis cs:0.5,0.0717750608358346)
--(axis cs:0.51,0.0733848242017641)
--(axis cs:0.52,0.0750334630241943)
--(axis cs:0.53,0.0767196324040008)
--(axis cs:0.54,0.0784420326830346)
--(axis cs:0.55,0.0801993639529641)
--(axis cs:0.56,0.0819903379464451)
--(axis cs:0.57,0.0838136873045568)
--(axis cs:0.58,0.0856681598718124)
--(axis cs:0.59,0.0875525218430413)
--(axis cs:0.6,0.0894655378724331)
--(axis cs:0.61,0.0914059863829636)
--(axis cs:0.62,0.0933726818154818)
--(axis cs:0.63,0.0953644664301272)
--(axis cs:0.64,0.0973802100364209)
--(axis cs:0.65,0.0994187926087443)
--(axis cs:0.66,0.101479087271332)
--(axis cs:0.67,0.103559986800133)
--(axis cs:0.68,0.105660404960312)
--(axis cs:0.69,0.107779289842451)
--(axis cs:0.7,0.109915629667094)
--(axis cs:0.71,0.112068463361257)
--(axis cs:0.72,0.114236863447596)
--(axis cs:0.73,0.116419955186152)
--(axis cs:0.74,0.118616924156016)
--(axis cs:0.75,0.12082698755848)
--(axis cs:0.76,0.123049403255985)
--(axis cs:0.77,0.125283478076146)
--(axis cs:0.78,0.127528549653454)
--(axis cs:0.79,0.129784002367015)
--(axis cs:0.8,0.132049232583361)
--(axis cs:0.81,0.134323650398087)
--(axis cs:0.82,0.136606671588551)
--(axis cs:0.83,0.138897700990988)
--(axis cs:0.84,0.141196121837432)
--(axis cs:0.85,0.143501296895721)
--(axis cs:0.86,0.14581255915531)
--(axis cs:0.87,0.148129188660111)
--(axis cs:0.88,0.150450427818255)
--(axis cs:0.89,0.152775463185007)
--(axis cs:0.9,0.15510340764533)
--(axis cs:0.91,0.157433335453624)
--(axis cs:0.92,0.159764236776131)
--(axis cs:0.93,0.162095053867944)
--(axis cs:0.94,0.164424687003626)
--(axis cs:0.95,0.166752027468528)
--(axis cs:0.96,0.169075995187867)
--(axis cs:0.97,0.171395571807891)
--(axis cs:0.98,0.173709818693998)
--(axis cs:0.99,0.176017913147561)
--(axis cs:1,0.17831918047603)
--(axis cs:1.01,0.180613115879911)
--(axis cs:1.02,0.182899405375072)
--(axis cs:1.03,0.185177895918243)
--(axis cs:1.04,0.187448619869797)
--(axis cs:1.05,0.189711751367452)
--(axis cs:1.06,0.191967607101214)
--(axis cs:1.07,0.194216604737458)
--(axis cs:1.08,0.196459254080909)
--(axis cs:1.09,0.198696138115839)
--(axis cs:1.1,0.200927871279053)
--(axis cs:1.11,0.203155093871172)
--(axis cs:1.12,0.205378461273777)
--(axis cs:1.13,0.207598616456441)
--(axis cs:1.14,0.209816201935407)
--(axis cs:1.15,0.2120318316294)
--(axis cs:1.16,0.214246080036114)
--(axis cs:1.17,0.216459496664066)
--(axis cs:1.18,0.218672590964395)
--(axis cs:1.19,0.220885846431094)
--(axis cs:1.2,0.223099731563249)
--(axis cs:1.21,0.225314685897965)
--(axis cs:1.22,0.227531116035107)
--(axis cs:1.23,0.229749397815893)
--(axis cs:1.24,0.231969881628625)
--(axis cs:1.25,0.234192886665064)
--(axis cs:1.26,0.236418714941171)
--(axis cs:1.27,0.238647662590584)
--(axis cs:1.28,0.240880005808665)
--(axis cs:1.29,0.243116011786704)
--(axis cs:1.3,0.245355943573334)
--(axis cs:1.31,0.247600064124004)
--(axis cs:1.32,0.249848617930775)
--(axis cs:1.33,0.252101826383988)
--(axis cs:1.34,0.254359878438271)
--(axis cs:1.35,0.256622918539883)
--(axis cs:1.36,0.258891016305523)
--(axis cs:1.37,0.261164184985139)
--(axis cs:1.38,0.263442327011828)
--(axis cs:1.39,0.265725242977678)
--(axis cs:1.4,0.268012626571188)
--(axis cs:1.41,0.270304039856413)
--(axis cs:1.42,0.272598901372121)
--(axis cs:1.43,0.274896488834787)
--(axis cs:1.44,0.277195953690686)
--(axis cs:1.45,0.279496334897453)
--(axis cs:1.46,0.281796584550524)
--(axis cs:1.47,0.284095604566437)
--(axis cs:1.48,0.286392273189468)
--(axis cs:1.49,0.288685483626368)
--(axis cs:1.49,0.358156810349748)
--(axis cs:1.49,0.358156810349748)
--(axis cs:1.48,0.355841324988984)
--(axis cs:1.47,0.353524643952306)
--(axis cs:1.46,0.351207166226379)
--(axis cs:1.45,0.348889226557106)
--(axis cs:1.44,0.346571079371207)
--(axis cs:1.43,0.34425291557756)
--(axis cs:1.42,0.341934877814502)
--(axis cs:1.41,0.339617040273853)
--(axis cs:1.4,0.337299441995139)
--(axis cs:1.39,0.334982067496876)
--(axis cs:1.38,0.33266485928429)
--(axis cs:1.37,0.330347712619472)
--(axis cs:1.36,0.328030484126551)
--(axis cs:1.35,0.325712969670478)
--(axis cs:1.34,0.323394918017615)
--(axis cs:1.33,0.321076014010097)
--(axis cs:1.32,0.318755910598902)
--(axis cs:1.31,0.31643418746642)
--(axis cs:1.3,0.314110363179702)
--(axis cs:1.29,0.3117838850196)
--(axis cs:1.28,0.309454148014519)
--(axis cs:1.27,0.30712047561167)
--(axis cs:1.26,0.304782122282665)
--(axis cs:1.25,0.30243826918296)
--(axis cs:1.24,0.300088031793134)
--(axis cs:1.23,0.297730444381768)
--(axis cs:1.22,0.295364494746899)
--(axis cs:1.21,0.292989111046704)
--(axis cs:1.2,0.290603166587053)
--(axis cs:1.19,0.288205492671867)
--(axis cs:1.18,0.285794893376554)
--(axis cs:1.17,0.283370141422132)
--(axis cs:1.16,0.280930010901038)
--(axis cs:1.15,0.278473282338983)
--(axis cs:1.14,0.275998770109278)
--(axis cs:1.13,0.273505333457621)
--(axis cs:1.12,0.270991901354518)
--(axis cs:1.11,0.268457516450262)
--(axis cs:1.1,0.265901349708921)
--(axis cs:1.09,0.263322759277471)
--(axis cs:1.08,0.260721318660275)
--(axis cs:1.07,0.258096871882383)
--(axis cs:1.06,0.255449549571056)
--(axis cs:1.05,0.252779826156774)
--(axis cs:1.04,0.250088510887996)
--(axis cs:1.03,0.247376756016718)
--(axis cs:1.02,0.244646015441975)
--(axis cs:1.01,0.241897998361717)
--(axis cs:1,0.239134589644229)
--(axis cs:0.99,0.236357747501751)
--(axis cs:0.98,0.233569414073723)
--(axis cs:0.97,0.230771415831414)
--(axis cs:0.96,0.227965404631724)
--(axis cs:0.95,0.225152810718767)
--(axis cs:0.94,0.222334797666422)
--(axis cs:0.93,0.21951226686051)
--(axis cs:0.92,0.216685887075345)
--(axis cs:0.91,0.213856093198766)
--(axis cs:0.9,0.211023141955213)
--(axis cs:0.89,0.208187135095636)
--(axis cs:0.88,0.205348065121381)
--(axis cs:0.87,0.202505829196741)
--(axis cs:0.86,0.199660303391903)
--(axis cs:0.85,0.196811303854618)
--(axis cs:0.84,0.19395866812577)
--(axis cs:0.83,0.191102255932378)
--(axis cs:0.82,0.188241966569533)
--(axis cs:0.81,0.185377758562127)
--(axis cs:0.8,0.182509646271428)
--(axis cs:0.79,0.1796377324085)
--(axis cs:0.78,0.176762183786096)
--(axis cs:0.77,0.173883266445635)
--(axis cs:0.76,0.171001315925014)
--(axis cs:0.75,0.168116771356335)
--(axis cs:0.74,0.165230157931981)
--(axis cs:0.73,0.162342109994998)
--(axis cs:0.72,0.159453347223909)
--(axis cs:0.71,0.156564694411489)
--(axis cs:0.7,0.153677072657589)
--(axis cs:0.69,0.15079151338914)
--(axis cs:0.68,0.147909154585952)
--(axis cs:0.67,0.145031242866924)
--(axis cs:0.66,0.142159122402216)
--(axis cs:0.65,0.139294251963748)
--(axis cs:0.64,0.136438202758167)
--(axis cs:0.63,0.133592654163888)
--(axis cs:0.62,0.130759405086203)
--(axis cs:0.61,0.12794038022757)
--(axis cs:0.6,0.125137639931766)
--(axis cs:0.59,0.122353371259742)
--(axis cs:0.58,0.119589893467614)
--(axis cs:0.57,0.116849653963352)
--(axis cs:0.56,0.114135249547499)
--(axis cs:0.55,0.111449435574712)
--(axis cs:0.54,0.108795134244876)
--(axis cs:0.53,0.106175447922277)
--(axis cs:0.52,0.103593675263206)
--(axis cs:0.51,0.101053329723522)
--(axis cs:0.5,0.0985581528311232)
--(axis cs:0.49,0.0961121512675577)
--(axis cs:0.48,0.0937196332357306)
--(axis cs:0.47,0.0913852452233941)
--(axis cs:0.46,0.0891140083671152)
--(axis cs:0.45,0.0869113667990278)
--(axis cs:0.44,0.0847832359952379)
--(axis cs:0.43,0.0827360165215174)
--(axis cs:0.42,0.0807766045565161)
--(axis cs:0.41,0.0789123319381027)
--(axis cs:0.4,0.0771507977180858)
--(axis cs:0.39,0.0754995786800967)
--(axis cs:0.38,0.0739656899116144)
--(axis cs:0.37,0.0725549042078132)
--(axis cs:0.36,0.0712709733075355)
--(axis cs:0.35,0.0701147476176894)
--(axis cs:0.34,0.0690834242967357)
--(axis cs:0.33,0.0681700713361275)
--(axis cs:0.32,0.0673635141761238)
--(axis cs:0.31,0.0666485137375359)
--(axis cs:0.3,0.0660062033802069)
--(axis cs:0.29,0.0654146448149682)
--(axis cs:0.28,0.0648496934473549)
--(axis cs:0.27,0.064286170492216)
--(axis cs:0.26,0.0636991696284818)
--(axis cs:0.25,0.0630652696288356)
--(axis cs:0.24,0.0623634270214283)
--(axis cs:0.23,0.0615755849754163)
--(axis cs:0.22,0.0606868362433055)
--(axis cs:0.21,0.0596853501391177)
--(axis cs:0.2,0.0585620386049195)
--(axis cs:0.19,0.0573101582165936)
--(axis cs:0.18,0.0559247668860355)
--(axis cs:0.17,0.0544023694076317)
--(axis cs:0.16,0.0527404773011438)
--(axis cs:0.15,0.0509373256347582)
--(axis cs:0.14,0.0489917412448188)
--(axis cs:0.13,0.0469029964342839)
--(axis cs:0.12,0.0446705927300628)
--(axis cs:0.11,0.042294086099778)
--(axis cs:0.1,0.0397730420616839)
--(axis cs:0.09,0.0371069958640657)
--(axis cs:0.08,0.034295226272871)
--(axis cs:0.07,0.0313363646248865)
--(axis cs:0.06,0.0282282669817199)
--(axis cs:0.05,0.0249676113065844)
--(axis cs:0.04,0.0215486299643194)
--(axis cs:0.03,0.0179607619172408)
--(axis cs:0.02,0.0141832851451309)
--(axis cs:0.01,0.0101700500701365)
--cycle;

\path [fill=blue, fill opacity=0.4, ultra thick]
(axis cs:0.01,0.00112323182760268)
--(axis cs:0.01,0.000390862624956019)
--(axis cs:0.02,0.000547675323338917)
--(axis cs:0.03,0.000691097766777506)
--(axis cs:0.04,0.000816184369631479)
--(axis cs:0.05,0.000932564667534897)
--(axis cs:0.06,0.00106463019916385)
--(axis cs:0.07,0.00121442225101591)
--(axis cs:0.08,0.00137545005191573)
--(axis cs:0.09,0.00154410771827045)
--(axis cs:0.1,0.00171961149961205)
--(axis cs:0.11,0.00190389320527511)
--(axis cs:0.12,0.00210154284706295)
--(axis cs:0.13,0.0023170328832327)
--(axis cs:0.14,0.00255327017812378)
--(axis cs:0.15,0.00281211926166841)
--(axis cs:0.16,0.00309484681818376)
--(axis cs:0.17,0.00340063706568939)
--(axis cs:0.18,0.00372748656898652)
--(axis cs:0.19,0.0040734371660784)
--(axis cs:0.2,0.00443682641928937)
--(axis cs:0.21,0.00481614661395883)
--(axis cs:0.22,0.00520999250133833)
--(axis cs:0.23,0.00561709524540205)
--(axis cs:0.24,0.00603628065392102)
--(axis cs:0.25,0.00646648055869783)
--(axis cs:0.26,0.0069066199915263)
--(axis cs:0.27,0.00735563285330359)
--(axis cs:0.28,0.00781251470123112)
--(axis cs:0.29,0.00827649042151947)
--(axis cs:0.3,0.00874724659319398)
--(axis cs:0.31,0.00922505161971822)
--(axis cs:0.32,0.00971051303417376)
--(axis cs:0.33,0.010204502107229)
--(axis cs:0.34,0.0107079425805878)
--(axis cs:0.35,0.0112216053970157)
--(axis cs:0.36,0.0117460216745039)
--(axis cs:0.37,0.0122813117620533)
--(axis cs:0.38,0.012827522446051)
--(axis cs:0.39,0.0133847568838344)
--(axis cs:0.4,0.0139532664862385)
--(axis cs:0.41,0.0145333843374037)
--(axis cs:0.42,0.0151253989903719)
--(axis cs:0.43,0.0157293587524534)
--(axis cs:0.44,0.0163451129768677)
--(axis cs:0.45,0.0169723755654835)
--(axis cs:0.46,0.0176106437688661)
--(axis cs:0.47,0.0182592535793396)
--(axis cs:0.48,0.0189174196498552)
--(axis cs:0.49,0.0195841337902666)
--(axis cs:0.5,0.0202582143549897)
--(axis cs:0.51,0.0209383987935631)
--(axis cs:0.52,0.0216234041932187)
--(axis cs:0.53,0.0223119103340693)
--(axis cs:0.54,0.0230025501011941)
--(axis cs:0.55,0.0236939564540862)
--(axis cs:0.56,0.0243847487044521)
--(axis cs:0.57,0.0250735831778278)
--(axis cs:0.58,0.0257591424108205)
--(axis cs:0.59,0.0264400576990911)
--(axis cs:0.6,0.0271148869778234)
--(axis cs:0.61,0.0277821361237566)
--(axis cs:0.62,0.0284402813825012)
--(axis cs:0.63,0.0290877566691927)
--(axis cs:0.64,0.0297229575368492)
--(axis cs:0.65,0.0303442599386645)
--(axis cs:0.66,0.0309500318864892)
--(axis cs:0.67,0.0315386820515672)
--(axis cs:0.68,0.0321087185690765)
--(axis cs:0.69,0.0326588312795858)
--(axis cs:0.7,0.0331880290251911)
--(axis cs:0.71,0.0336958220710126)
--(axis cs:0.72,0.034182414977087)
--(axis cs:0.73,0.0346489113441002)
--(axis cs:0.74,0.0350975141248341)
--(axis cs:0.75,0.035531639967843)
--(axis cs:0.76,0.0359559430254809)
--(axis cs:0.77,0.0363761443451496)
--(axis cs:0.78,0.0367987164376841)
--(axis cs:0.79,0.0372304344331864)
--(axis cs:0.8,0.0376779135206471)
--(axis cs:0.81,0.0381471960349063)
--(axis cs:0.82,0.0386434557637386)
--(axis cs:0.83,0.0391708051548959)
--(axis cs:0.84,0.039732252612641)
--(axis cs:0.85,0.0403297575991028)
--(axis cs:0.86,0.0409643940193115)
--(axis cs:0.87,0.0416365230393467)
--(axis cs:0.88,0.0423459856130386)
--(axis cs:0.89,0.0430922399950236)
--(axis cs:0.9,0.0438744736636218)
--(axis cs:0.91,0.0446916826440689)
--(axis cs:0.92,0.0455427254973473)
--(axis cs:0.93,0.0464263331935536)
--(axis cs:0.94,0.0473411388113847)
--(axis cs:0.95,0.0482856685086629)
--(axis cs:0.96,0.0492583526219693)
--(axis cs:0.97,0.0502575156377388)
--(axis cs:0.98,0.0512813764510237)
--(axis cs:0.99,0.0523280602740425)
--(axis cs:1,0.0533955914430987)
--(axis cs:1.01,0.0544819080375713)
--(axis cs:1.02,0.055584881455677)
--(axis cs:1.03,0.0567023257086046)
--(axis cs:1.04,0.0578320180164231)
--(axis cs:1.05,0.058971721365533)
--(axis cs:1.06,0.0601192019272189)
--(axis cs:1.07,0.0612722214511191)
--(axis cs:1.08,0.0624285592127015)
--(axis cs:1.09,0.0635860180067926)
--(axis cs:1.1,0.0647424252962425)
--(axis cs:1.11,0.0658956407266312)
--(axis cs:1.12,0.0670435440459079)
--(axis cs:1.13,0.0681840364446624)
--(axis cs:1.14,0.0693149991364676)
--(axis cs:1.15,0.0704342897043326)
--(axis cs:1.16,0.0715396968592512)
--(axis cs:1.17,0.0726289492261564)
--(axis cs:1.18,0.073699719200063)
--(axis cs:1.19,0.0747495875876397)
--(axis cs:1.2,0.075776064327672)
--(axis cs:1.21,0.0767765865871431)
--(axis cs:1.22,0.0777485139614771)
--(axis cs:1.23,0.0786891021654161)
--(axis cs:1.24,0.079595513585611)
--(axis cs:1.25,0.0804647711421394)
--(axis cs:1.26,0.081293751769194)
--(axis cs:1.27,0.0820791695622273)
--(axis cs:1.28,0.0828175282578425)
--(axis cs:1.29,0.0835051274785759)
--(axis cs:1.3,0.0841380401090376)
--(axis cs:1.31,0.0847121387100107)
--(axis cs:1.32,0.0852231981879601)
--(axis cs:1.33,0.0856671538015378)
--(axis cs:1.34,0.0860406412654275)
--(axis cs:1.35,0.0863418874979533)
--(axis cs:1.36,0.0865718114367095)
--(axis cs:1.37,0.0867347430252594)
--(axis cs:1.38,0.0868384977038572)
--(axis cs:1.39,0.0868943452159211)
--(axis cs:1.4,0.0869167752027351)
--(axis cs:1.41,0.0869221994363794)
--(axis cs:1.42,0.0869265729167221)
--(axis cs:1.43,0.0869435365537514)
--(axis cs:1.44,0.0869842024174286)
--(axis cs:1.45,0.0870577600065079)
--(axis cs:1.46,0.0871714720592093)
--(axis cs:1.47,0.0873300393674262)
--(axis cs:1.48,0.087535222540199)
--(axis cs:1.49,0.08778626405545)
--(axis cs:1.49,0.112383269958444)
--(axis cs:1.49,0.112383269958444)
--(axis cs:1.48,0.112002245566529)
--(axis cs:1.47,0.111679784965737)
--(axis cs:1.46,0.111421155433828)
--(axis cs:1.45,0.111230103907043)
--(axis cs:1.44,0.111107457860928)
--(axis cs:1.43,0.111049834719887)
--(axis cs:1.42,0.111049368936689)
--(axis cs:1.41,0.111094832211034)
--(axis cs:1.4,0.111172580069064)
--(axis cs:1.39,0.111266072983714)
--(axis cs:1.38,0.11135540926434)
--(axis cs:1.37,0.11141885431843)
--(axis cs:1.36,0.111435666522079)
--(axis cs:1.35,0.111388002392972)
--(axis cs:1.34,0.111261962038174)
--(axis cs:1.33,0.111048650596296)
--(axis cs:1.32,0.11074430835388)
--(axis cs:1.31,0.11034917699172)
--(axis cs:1.3,0.109865934219338)
--(axis cs:1.29,0.109298470839942)
--(axis cs:1.28,0.108651164737564)
--(axis cs:1.27,0.107928511090496)
--(axis cs:1.26,0.107134951259796)
--(axis cs:1.25,0.10627478992209)
--(axis cs:1.24,0.105352199551069)
--(axis cs:1.23,0.104371212395328)
--(axis cs:1.22,0.103335745699791)
--(axis cs:1.21,0.102249604823824)
--(axis cs:1.2,0.101116510884896)
--(axis cs:1.19,0.0999401259404017)
--(axis cs:1.18,0.0987240491279761)
--(axis cs:1.17,0.0974718317285)
--(axis cs:1.16,0.0961869878198457)
--(axis cs:1.15,0.0948729839673384)
--(axis cs:1.14,0.0935332516555659)
--(axis cs:1.13,0.0921711633483992)
--(axis cs:1.12,0.0907900269164835)
--(axis cs:1.11,0.089393090956003)
--(axis cs:1.1,0.0879835165583067)
--(axis cs:1.09,0.0865644029437527)
--(axis cs:1.08,0.0851387986019108)
--(axis cs:1.07,0.083709742344111)
--(axis cs:1.06,0.0822803078268101)
--(axis cs:1.05,0.0808536022268366)
--(axis cs:1.04,0.0794327814592691)
--(axis cs:1.03,0.078021032353724)
--(axis cs:1.02,0.0766215544976105)
--(axis cs:1.01,0.0752375370819445)
--(axis cs:1,0.0738721374178527)
--(axis cs:0.99,0.0725284331795413)
--(axis cs:0.98,0.0712094150825152)
--(axis cs:0.97,0.0699179565908863)
--(axis cs:0.96,0.0686567888903057)
--(axis cs:0.95,0.0674284937826399)
--(axis cs:0.94,0.0662355063646037)
--(axis cs:0.93,0.065080115856022)
--(axis cs:0.92,0.0639644732092721)
--(axis cs:0.91,0.0628906189000946)
--(axis cs:0.9,0.0618604799869008)
--(axis cs:0.89,0.0608758982340057)
--(axis cs:0.88,0.0599386322157765)
--(axis cs:0.87,0.0590503519932535)
--(axis cs:0.86,0.0582126089431713)
--(axis cs:0.85,0.057426771161866)
--(axis cs:0.84,0.0566939203108107)
--(axis cs:0.83,0.0560146943175056)
--(axis cs:0.82,0.0553890769180333)
--(axis cs:0.81,0.0548161266446947)
--(axis cs:0.8,0.054293703388365)
--(axis cs:0.79,0.0538181965696469)
--(axis cs:0.78,0.0533843293545465)
--(axis cs:0.77,0.0529850703925575)
--(axis cs:0.76,0.0526117596501827)
--(axis cs:0.75,0.0522544991956887)
--(axis cs:0.74,0.0519027738490969)
--(axis cs:0.73,0.0515462366629979)
--(axis cs:0.72,0.0511754746956416)
--(axis cs:0.71,0.0507825910538021)
--(axis cs:0.7,0.0503615679175128)
--(axis cs:0.69,0.0499083205280651)
--(axis cs:0.68,0.0494205192700684)
--(axis cs:0.67,0.04889726175872)
--(axis cs:0.66,0.0483387211378166)
--(axis cs:0.65,0.0477458278189808)
--(axis cs:0.64,0.047120006169138)
--(axis cs:0.63,0.0464630136379676)
--(axis cs:0.62,0.0457768163498234)
--(axis cs:0.61,0.0450635035383928)
--(axis cs:0.6,0.0443252510025678)
--(axis cs:0.59,0.0435643263641232)
--(axis cs:0.58,0.042783050833315)
--(axis cs:0.57,0.04198377614698)
--(axis cs:0.56,0.0411688569088593)
--(axis cs:0.55,0.040340651693663)
--(axis cs:0.54,0.0395015404106392)
--(axis cs:0.53,0.0386538682277659)
--(axis cs:0.52,0.0377998440957724)
--(axis cs:0.51,0.0369414981454394)
--(axis cs:0.5,0.036080711720233)
--(axis cs:0.49,0.035219280632965)
--(axis cs:0.48,0.0343588235065396)
--(axis cs:0.47,0.0335007396543157)
--(axis cs:0.46,0.0326462011315243)
--(axis cs:0.45,0.0317961520501484)
--(axis cs:0.44,0.0309513267946135)
--(axis cs:0.43,0.0301123021972271)
--(axis cs:0.42,0.0292795440510969)
--(axis cs:0.41,0.0284535239636828)
--(axis cs:0.4,0.0276346337736426)
--(axis cs:0.39,0.0268230829306941)
--(axis cs:0.38,0.0260188871649575)
--(axis cs:0.37,0.0252218640829003)
--(axis cs:0.36,0.0244316683123175)
--(axis cs:0.35,0.0236478325756247)
--(axis cs:0.34,0.0228698912363656)
--(axis cs:0.33,0.022097374436487)
--(axis cs:0.32,0.021329820645567)
--(axis cs:0.31,0.0205661115595813)
--(axis cs:0.3,0.0198045026912443)
--(axis cs:0.29,0.0190431575477245)
--(axis cs:0.28,0.0182807038230337)
--(axis cs:0.27,0.0175164493334589)
--(axis cs:0.26,0.0167503411983803)
--(axis cs:0.25,0.0159829372106454)
--(axis cs:0.24,0.0152152874792558)
--(axis cs:0.23,0.0144487866613113)
--(axis cs:0.22,0.0136853485048857)
--(axis cs:0.21,0.0129270414051041)
--(axis cs:0.2,0.0121759190067088)
--(axis cs:0.19,0.011433903982436)
--(axis cs:0.18,0.0107029569554241)
--(axis cs:0.17,0.00998499615055175)
--(axis cs:0.16,0.00928183735937461)
--(axis cs:0.15,0.00859518663019253)
--(axis cs:0.14,0.00792702306120364)
--(axis cs:0.13,0.00727962523697065)
--(axis cs:0.12,0.00665504538645378)
--(axis cs:0.11,0.00605474549095041)
--(axis cs:0.1,0.00547936257081444)
--(axis cs:0.09,0.00492823989531453)
--(axis cs:0.08,0.00439971700703372)
--(axis cs:0.07,0.00389159127015809)
--(axis cs:0.06,0.00340126384760859)
--(axis cs:0.05,0.00292652256460163)
--(axis cs:0.04,0.00246684741876879)
--(axis cs:0.03,0.00201965697105396)
--(axis cs:0.02,0.00157618797505672)
--(axis cs:0.01,0.00112323182760268)
--cycle;

\path [fill=color0, fill opacity=0.4, ultra thick]
(axis cs:0.01,0.000533248698044085)
--(axis cs:0.01,0.000212942009494771)
--(axis cs:0.02,0.000293629287936698)
--(axis cs:0.03,0.000365162586290054)
--(axis cs:0.04,0.000427373785220157)
--(axis cs:0.05,0.000481787918360178)
--(axis cs:0.06,0.000533209397239513)
--(axis cs:0.07,0.000585509633992895)
--(axis cs:0.08,0.000640146485311864)
--(axis cs:0.09,0.000697374084793872)
--(axis cs:0.1,0.000757017316410774)
--(axis cs:0.11,0.000819904946464861)
--(axis cs:0.12,0.00088718740491867)
--(axis cs:0.13,0.000959355267182733)
--(axis cs:0.14,0.00103602080772871)
--(axis cs:0.15,0.00111614253436919)
--(axis cs:0.16,0.00119837837573656)
--(axis cs:0.17,0.00128147244049736)
--(axis cs:0.18,0.00136446677804016)
--(axis cs:0.19,0.00144655293342994)
--(axis cs:0.2,0.00152725524020904)
--(axis cs:0.21,0.00160626705782238)
--(axis cs:0.22,0.00168335851347813)
--(axis cs:0.23,0.00175828306402443)
--(axis cs:0.24,0.00183081230237102)
--(axis cs:0.25,0.0019007857574956)
--(axis cs:0.26,0.00196811055571339)
--(axis cs:0.27,0.00203271944085982)
--(axis cs:0.28,0.00209452363284045)
--(axis cs:0.29,0.00215347224982937)
--(axis cs:0.3,0.00221001588606194)
--(axis cs:0.31,0.00226520725946482)
--(axis cs:0.32,0.00232049443563777)
--(axis cs:0.33,0.00237687612849967)
--(axis cs:0.34,0.00243441133387117)
--(axis cs:0.35,0.0024922337088611)
--(axis cs:0.36,0.00254945264837)
--(axis cs:0.37,0.00260578999341849)
--(axis cs:0.38,0.00266170454396588)
--(axis cs:0.39,0.00271780127192051)
--(axis cs:0.4,0.00277442249107527)
--(axis cs:0.41,0.00283165986710451)
--(axis cs:0.42,0.00288949711093951)
--(axis cs:0.43,0.00294798053676083)
--(axis cs:0.44,0.00300723401353611)
--(axis cs:0.45,0.00306748008139248)
--(axis cs:0.46,0.00312899828906918)
--(axis cs:0.47,0.00319203489188414)
--(axis cs:0.48,0.00325676810277039)
--(axis cs:0.49,0.0033232637198665)
--(axis cs:0.5,0.00339152452605217)
--(axis cs:0.51,0.00346158479369152)
--(axis cs:0.52,0.00353358305401998)
--(axis cs:0.53,0.0036076006091798)
--(axis cs:0.54,0.00368359186426256)
--(axis cs:0.55,0.00376141412768531)
--(axis cs:0.56,0.00384097738952312)
--(axis cs:0.57,0.00392231047001072)
--(axis cs:0.58,0.00400547529731515)
--(axis cs:0.59,0.00409047986980614)
--(axis cs:0.6,0.00417730396116219)
--(axis cs:0.61,0.00426592315285722)
--(axis cs:0.62,0.00435632167829983)
--(axis cs:0.63,0.00444847660641092)
--(axis cs:0.64,0.00454235887805505)
--(axis cs:0.65,0.00463791307200394)
--(axis cs:0.66,0.00473506363870624)
--(axis cs:0.67,0.00483371897722357)
--(axis cs:0.68,0.00493378758822853)
--(axis cs:0.69,0.00503517486053477)
--(axis cs:0.7,0.00513777992374393)
--(axis cs:0.71,0.00524149596465715)
--(axis cs:0.72,0.00534621069013038)
--(axis cs:0.73,0.00545180030979165)
--(axis cs:0.74,0.00555813696695542)
--(axis cs:0.75,0.00566508234483802)
--(axis cs:0.76,0.00577248506478408)
--(axis cs:0.77,0.00588018158438993)
--(axis cs:0.78,0.00598800162194344)
--(axis cs:0.79,0.0060957891771548)
--(axis cs:0.8,0.00620340579603815)
--(axis cs:0.81,0.0063107137523868)
--(axis cs:0.82,0.00641760212952451)
--(axis cs:0.83,0.00652399142455819)
--(axis cs:0.84,0.00662981809812637)
--(axis cs:0.85,0.00673504157374346)
--(axis cs:0.86,0.00683964372009206)
--(axis cs:0.87,0.00694361202337281)
--(axis cs:0.88,0.0070469329149258)
--(axis cs:0.89,0.00714958274549273)
--(axis cs:0.9,0.0072515288595869)
--(axis cs:0.91,0.00735272141368291)
--(axis cs:0.92,0.00745310522861448)
--(axis cs:0.93,0.00755262511583565)
--(axis cs:0.94,0.00765123445583509)
--(axis cs:0.95,0.00774890544166914)
--(axis cs:0.96,0.00784565288523583)
--(axis cs:0.97,0.0079415486375926)
--(axis cs:0.98,0.00803672413180881)
--(axis cs:0.99,0.00813135000925251)
--(axis cs:1,0.00822561102842847)
--(axis cs:1.01,0.00831968912427039)
--(axis cs:1.02,0.00841372757811164)
--(axis cs:1.03,0.00850780785613205)
--(axis cs:1.04,0.008601930412219)
--(axis cs:1.05,0.00869601483911383)
--(axis cs:1.06,0.0087899104508846)
--(axis cs:1.07,0.00888343150908366)
--(axis cs:1.08,0.00897641519537249)
--(axis cs:1.09,0.00906875959146385)
--(axis cs:1.1,0.00916044123978111)
--(axis cs:1.11,0.0092514653934296)
--(axis cs:1.12,0.00934184054926068)
--(axis cs:1.13,0.00943157094928009)
--(axis cs:1.14,0.00952066012025932)
--(axis cs:1.15,0.00960909997568092)
--(axis cs:1.16,0.00969688016399388)
--(axis cs:1.17,0.00978399417370266)
--(axis cs:1.18,0.00987042912096598)
--(axis cs:1.19,0.00995615731884139)
--(axis cs:1.2,0.0100411437595123)
--(axis cs:1.21,0.0101253501982217)
--(axis cs:1.22,0.0102087250545588)
--(axis cs:1.23,0.0102912220760033)
--(axis cs:1.24,0.0103727879954403)
--(axis cs:1.25,0.0104533600537015)
--(axis cs:1.26,0.0105328785987318)
--(axis cs:1.27,0.0106112859137983)
--(axis cs:1.28,0.0106885390558398)
--(axis cs:1.29,0.0107645982531204)
--(axis cs:1.3,0.0108394291640047)
--(axis cs:1.31,0.0109130054121827)
--(axis cs:1.32,0.0109853145734954)
--(axis cs:1.33,0.0110563613899685)
--(axis cs:1.34,0.011126174592308)
--(axis cs:1.35,0.0111947946406291)
--(axis cs:1.36,0.0112622668619801)
--(axis cs:1.37,0.0113286403494989)
--(axis cs:1.38,0.0113939555642342)
--(axis cs:1.39,0.011458230230756)
--(axis cs:1.4,0.0115214622351401)
--(axis cs:1.41,0.0115836368284852)
--(axis cs:1.42,0.0116446966063241)
--(axis cs:1.43,0.0117045424144067)
--(axis cs:1.44,0.0117629977041631)
--(axis cs:1.45,0.011819810495201)
--(axis cs:1.46,0.0118746947817699)
--(axis cs:1.47,0.011927408813391)
--(axis cs:1.48,0.0119777325106373)
--(axis cs:1.49,0.0120254340172996)
--(axis cs:1.49,0.0205045290709664)
--(axis cs:1.49,0.0205045290709664)
--(axis cs:1.48,0.0204515209548821)
--(axis cs:1.47,0.0203927312958429)
--(axis cs:1.46,0.0203280966100604)
--(axis cs:1.45,0.0202577112879545)
--(axis cs:1.44,0.0201817540308462)
--(axis cs:1.43,0.0201004357163691)
--(axis cs:1.42,0.0200139687402044)
--(axis cs:1.41,0.0199225467780932)
--(axis cs:1.4,0.0198263421735203)
--(axis cs:1.39,0.0197254896136422)
--(axis cs:1.38,0.0196200976117088)
--(axis cs:1.37,0.0195102600554363)
--(axis cs:1.36,0.0193960656109216)
--(axis cs:1.35,0.0192776010493353)
--(axis cs:1.34,0.0191549565385618)
--(axis cs:1.33,0.019028231164579)
--(axis cs:1.32,0.0188975377387136)
--(axis cs:1.31,0.0187630028900491)
--(axis cs:1.3,0.0186247683346799)
--(axis cs:1.29,0.0184829943914907)
--(axis cs:1.28,0.0183378489109877)
--(axis cs:1.27,0.0181895114485138)
--(axis cs:1.26,0.0180381747867376)
--(axis cs:1.25,0.0178840441639651)
--(axis cs:1.24,0.0177273386782674)
--(axis cs:1.23,0.017568290881104)
--(axis cs:1.22,0.0174071484363317)
--(axis cs:1.21,0.0172441706681502)
--(axis cs:1.2,0.0170796217180379)
--(axis cs:1.19,0.0169137793501759)
--(axis cs:1.18,0.0167469419245163)
--(axis cs:1.17,0.0165794375005476)
--(axis cs:1.16,0.0164116243025004)
--(axis cs:1.15,0.0162438816386233)
--(axis cs:1.14,0.0160766099573002)
--(axis cs:1.13,0.0159102575626284)
--(axis cs:1.12,0.0157453227952065)
--(axis cs:1.11,0.0155823246503194)
--(axis cs:1.1,0.0154218069975938)
--(axis cs:1.09,0.0152643012174409)
--(axis cs:1.08,0.0151102551536626)
--(axis cs:1.07,0.0149599070313523)
--(axis cs:1.06,0.0148131734900339)
--(axis cs:1.05,0.0146696064488926)
--(axis cs:1.04,0.0145285189286766)
--(axis cs:1.03,0.0143891961394391)
--(axis cs:1.02,0.0142510257075252)
--(axis cs:1.01,0.0141135339928238)
--(axis cs:1,0.0139763976040177)
--(axis cs:0.99,0.0138394084940224)
--(axis cs:0.98,0.0137024410152266)
--(axis cs:0.97,0.0135653976008711)
--(axis cs:0.96,0.0134281267332284)
--(axis cs:0.95,0.0132903830739431)
--(axis cs:0.94,0.0131518147161415)
--(axis cs:0.93,0.0130119959223703)
--(axis cs:0.92,0.012870472615066)
--(axis cs:0.91,0.0127268413372586)
--(axis cs:0.9,0.0125808180888977)
--(axis cs:0.89,0.0124322624533375)
--(axis cs:0.88,0.0122811755303359)
--(axis cs:0.87,0.0121276600973771)
--(axis cs:0.86,0.0119719082270414)
--(axis cs:0.85,0.0118141468641213)
--(axis cs:0.84,0.0116546237741681)
--(axis cs:0.83,0.0114935828361924)
--(axis cs:0.82,0.0113312767434248)
--(axis cs:0.81,0.0111679528510222)
--(axis cs:0.8,0.0110038405813672)
--(axis cs:0.79,0.0108391535374779)
--(axis cs:0.78,0.0106740978830198)
--(axis cs:0.77,0.0105088735841173)
--(axis cs:0.76,0.010343676118837)
--(axis cs:0.75,0.0101787071443622)
--(axis cs:0.74,0.0100141749999706)
--(axis cs:0.73,0.00985028365463627)
--(axis cs:0.72,0.00968723164542309)
--(axis cs:0.71,0.00952520998045634)
--(axis cs:0.7,0.00936440547877524)
--(axis cs:0.69,0.00920500001953665)
--(axis cs:0.68,0.00904717519334336)
--(axis cs:0.67,0.00889111587177854)
--(axis cs:0.66,0.00873700473504183)
--(axis cs:0.65,0.00858502127283775)
--(axis cs:0.64,0.00843533361614606)
--(axis cs:0.63,0.00828809335598801)
--(axis cs:0.62,0.00814342860128524)
--(axis cs:0.61,0.00800144227764924)
--(axis cs:0.6,0.00786219871707595)
--(axis cs:0.59,0.00772569861413215)
--(axis cs:0.58,0.00759188640088205)
--(axis cs:0.57,0.00746068027847563)
--(axis cs:0.56,0.00733198669458961)
--(axis cs:0.55,0.00720578677809935)
--(axis cs:0.54,0.00708221714562532)
--(axis cs:0.53,0.00696156257343609)
--(axis cs:0.52,0.00684421317996972)
--(axis cs:0.51,0.00673059835153972)
--(axis cs:0.5,0.00662119482449696)
--(axis cs:0.49,0.00651651137027359)
--(axis cs:0.48,0.00641706689577763)
--(axis cs:0.47,0.00632331160632622)
--(axis cs:0.46,0.00623545900090003)
--(axis cs:0.45,0.00615324171407263)
--(axis cs:0.44,0.006075843305783)
--(axis cs:0.43,0.00600229835272606)
--(axis cs:0.42,0.00593177789337453)
--(axis cs:0.41,0.00586374114445191)
--(axis cs:0.4,0.00579822478973409)
--(axis cs:0.39,0.00573593776962688)
--(axis cs:0.38,0.00567821275361557)
--(axis cs:0.37,0.00562658585866593)
--(axis cs:0.36,0.00558187617058776)
--(axis cs:0.35,0.00554212638652181)
--(axis cs:0.34,0.00550183240510258)
--(axis cs:0.33,0.00545490821810086)
--(axis cs:0.32,0.00539732425694408)
--(axis cs:0.31,0.00532767470254839)
--(axis cs:0.3,0.00524572912301272)
--(axis cs:0.29,0.0051519000662861)
--(axis cs:0.28,0.00504697723649782)
--(axis cs:0.27,0.00493224006771007)
--(axis cs:0.26,0.00480949459071489)
--(axis cs:0.25,0.00468034853501086)
--(axis cs:0.24,0.00454604004182488)
--(axis cs:0.23,0.00440687129557459)
--(axis cs:0.22,0.0042626496223672)
--(axis cs:0.21,0.00411355975299538)
--(axis cs:0.2,0.00396004820126084)
--(axis cs:0.19,0.00380244883553344)
--(axis cs:0.18,0.00364098683309382)
--(axis cs:0.17,0.00347583541480076)
--(axis cs:0.16,0.00330723504247329)
--(axis cs:0.15,0.00313543134042431)
--(axis cs:0.14,0.00296068069855757)
--(axis cs:0.13,0.00278330484539286)
--(axis cs:0.12,0.00260382556685883)
--(axis cs:0.11,0.00242297760685044)
--(axis cs:0.1,0.00224117705422137)
--(axis cs:0.09,0.00205858830293313)
--(axis cs:0.08,0.00187510489113622)
--(axis cs:0.07,0.00169070273468436)
--(axis cs:0.06,0.00150548133238849)
--(axis cs:0.05,0.00131954151587513)
--(axis cs:0.04,0.00113217945430375)
--(axis cs:0.03,0.000941269242263489)
--(axis cs:0.02,0.000743093670191952)
--(axis cs:0.01,0.000533248698044085)
--cycle;

\addplot [ultra thick, red]
table {%
0.00999999046325684 0.00859271083027124
0.0199999809265137 0.0119945453479886
0.0299999713897705 0.0152037907391787
0.0399999618530273 0.0182593259960413
0.0499999523162842 0.0211782846599817
0.059999942779541 0.0239690896123648
0.0700000524520874 0.0266360752284527
0.0800000429153442 0.0291814878582954
0.0900000333786011 0.0316063389182091
0.100000023841858 0.0339108109474182
0.110000014305115 0.0360945463180542
0.120000004768372 0.0381571240723133
0.129999995231628 0.0400980971753597
0.139999985694885 0.0419171676039696
0.149999976158142 0.0436142012476921
0.159999966621399 0.0451893992722034
0.169999957084656 0.0466435439884663
0.180000066757202 0.047978188842535
0.190000057220459 0.0491960160434246
0.200000047683716 0.0503010228276253
0.210000038146973 0.0512990802526474
0.220000028610229 0.0521981567144394
0.230000019073486 0.053008608520031
0.240000009536743 0.0537432767450809
0.259999990463257 0.0550479330122471
0.309999942779541 0.058180894702673
0.330000042915344 0.0597237087786198
0.350000023841858 0.06156225502491
0.370000004768372 0.0637332051992416
0.389999985694885 0.0662441551685333
0.409999966621399 0.0690820142626762
0.430000066757202 0.0722218602895737
0.460000038146973 0.0774329900741577
0.559999942779541 0.09806277602911
0.589999914169312 0.104952953755856
0.620000004768372 0.112066030502319
0.649999976158142 0.119356513023376
0.680000066757202 0.126784786581993
0.710000038146973 0.134316578507423
0.740000009536743 0.141923531889915
0.769999980926514 0.149583384394646
0.799999952316284 0.157279446721077
0.829999923706055 0.164999976754189
0.860000014305115 0.172736436128616
0.889999985694885 0.180481284856796
0.920000076293945 0.188225090503693
0.950000047683716 0.195952415466309
0.980000019073486 0.203639581799507
1.00999999046326 0.211255550384521
1.03999996185303 0.218768551945686
1.07000005245209 0.226156696677208
1.11000001430511 0.235806286334991
1.14999997615814 0.245252534747124
1.19000005722046 0.254545629024506
1.24000000953674 0.266028940677643
1.28999996185303 0.277449935674667
1.35000002384186 0.291167914867401
1.4099999666214 0.304960519075394
1.47000002861023 0.318810164928436
1.49000000953674 0.323421210050583
};
\addplot [ultra thick, blue]
table {%
0.00999999046325684 0.000757047208026052
0.0199999809265137 0.00106193171814084
0.0299999713897705 0.00135537760797888
0.0399999618530273 0.00164151552598923
0.0499999523162842 0.00192954321391881
0.059999942779541 0.00223294692113996
0.0700000524520874 0.00255300709977746
0.0800000429153442 0.00288758357055485
0.0900000333786011 0.00323617458343506
0.100000023841858 0.00359948654659092
0.110000014305115 0.00397931830957532
0.129999995231628 0.00479832990095019
0.149999976158142 0.00570365320891142
0.169999957084656 0.00669281743466854
0.190000057220459 0.0077536697499454
0.210000038146973 0.0088715935125947
0.230000019073486 0.0100329406559467
0.25 0.011224708519876
0.269999980926514 0.0124360397458076
0.289999961853027 0.0136598246172071
0.309999942779541 0.0148955807089806
0.330000042915344 0.0161509364843369
0.350000023841858 0.0174347162246704
0.370000004768372 0.0187515877187252
0.389999985694885 0.0201039183884859
0.409999966621399 0.0214934516698122
0.430000066757202 0.0229208301752806
0.450000047683716 0.0243842639029026
0.470000028610229 0.0258799977600574
0.490000009536743 0.0274017080664635
0.509999990463257 0.0289399512112141
0.529999971389771 0.0304828882217407
0.549999952316284 0.0320173054933548
0.569999933242798 0.0335286743938923
0.589999914169312 0.0350021943449974
0.610000014305115 0.036422822624445
0.629999995231628 0.037775382399559
0.649999976158142 0.0390450395643711
0.670000076293945 0.0402179732918739
0.690000057220459 0.0412835814058781
0.710000038146973 0.0422392040491104
0.730000019073486 0.0430975742638111
0.759999990463257 0.0442838482558727
0.789999961853027 0.0455243140459061
0.809999942779541 0.0464816614985466
0.829999923706055 0.0475927479565144
0.850000023841858 0.048878263682127
0.870000004768372 0.0503434427082539
0.889999985694885 0.0519840680062771
0.910000085830688 0.0537911541759968
0.940000057220459 0.0567883178591728
0.980000019073486 0.0612454041838646
1.03999996185303 0.0686323940753937
1.07000005245209 0.0724909827113152
1.10000002384186 0.0763629749417305
1.12999999523163 0.0801775828003883
1.14999997615814 0.082653634250164
1.16999995708466 0.0850503891706467
1.19000005722046 0.0873448550701141
1.21000003814697 0.0895130857825279
1.23000001907349 0.0915301516652107
1.25 0.0933697894215584
1.26999998092651 0.0950038284063339
1.28999996185303 0.0964017882943153
1.30999994277954 0.0975306481122971
1.33000004291534 0.0983579084277153
1.35000002384186 0.0988649427890778
1.37000000476837 0.0990767851471901
1.39999997615814 0.0990446731448174
1.42999994754791 0.098996676504612
1.45000004768372 0.0991439297795296
1.47000002861023 0.0995048955082893
1.49000000953674 0.100084774196148
};
\addplot [ultra thick, color0]
table {%
0.00999999046325684 0.000373095303075388
0.0199999809265137 0.000518361513968557
0.0299999713897705 0.000653215975034982
0.0399999618530273 0.000779776542913169
0.0499999523162842 0.000900664716027677
0.059999942779541 0.00101934524718672
0.0700000524520874 0.00113810633774847
0.0800000429153442 0.0012576257577166
0.0900000333786011 0.00137798138894141
0.100000023841858 0.00149909756146371
0.110000014305115 0.00162144168280065
0.120000004768372 0.00174550630617887
0.129999995231628 0.0018713305471465
0.139999985694885 0.00199835002422333
0.149999976158142 0.00212578661739826
0.159999966621399 0.00225280621089041
0.169999957084656 0.0023786542005837
0.180000066757202 0.00250272662378848
0.190000057220459 0.00262450031004846
0.200000047683716 0.00274365162476897
0.210000038146973 0.00285991374403238
0.220000028610229 0.00297300447709858
0.230000019073486 0.00308257760480046
0.240000009536743 0.00318842544220388
0.25 0.0032905675470829
0.259999990463257 0.00338880228810012
0.269999980926514 0.00348248076625168
0.279999971389771 0.00357074965722859
0.289999961853027 0.00365268555469811
0.299999952316284 0.0037278716918081
0.309999942779541 0.00379644148051739
0.319999933242798 0.00385890994220972
0.330000042915344 0.00391589151695371
0.350000023841858 0.00401717890053988
0.370000004768372 0.00411618873476982
0.389999985694885 0.00422686897218227
0.419999957084656 0.00441063847392797
0.450000047683716 0.00461036060005426
0.470000028610229 0.00475767347961664
0.490000009536743 0.00491988658905029
0.519999980926514 0.00518889958038926
0.569999933242798 0.0056914952583611
0.710000038146973 0.00738335447385907
0.75 0.00792189314961433
0.779999971389771 0.00833105202764273
0.809999942779541 0.00873933266848326
0.839999914169312 0.00914222095161676
0.870000004768372 0.00953563489019871
0.899999976158142 0.00991617329418659
0.930000066757202 0.0102823097258806
0.960000038146973 0.0106368903070688
1 0.0111010037362576
1.05999994277954 0.0118015417829156
1.16999995708466 0.0131817171350121
1.21000003814697 0.0136847589164972
1.24000000953674 0.0140500627458096
1.26999998092651 0.0144003992900252
1.29999995231628 0.0147320991382003
1.33000004291534 0.0150422975420952
1.36000001430511 0.0153291653841734
1.38999998569489 0.0155918598175049
1.41999995708466 0.0158293340355158
1.45000004768372 0.0160387624055147
1.48000001907349 0.0162146259099245
1.49000000953674 0.0162649787962437
};

==> supp_mat/double_pend/error_vs_trajectory_count_data.tex <==
\definecolor{color0}{rgb}{1,0,1}

\path [fill=red, fill opacity=0.4, ultra thick]
(axis cs:1,0.358156810349748)
--(axis cs:1,0.288685483626368)
--(axis cs:5,0.0153974990861162)
--(axis cs:10,0.016051068814258)
--(axis cs:20,0.029675446614998)
--(axis cs:100,0.014277179006959)
--(axis cs:100,0.0283372811794607)
--(axis cs:100,0.0283372811794607)
--(axis cs:20,0.0418484036759897)
--(axis cs:10,0.0231407828796545)
--(axis cs:5,0.0233957937561589)
--(axis cs:1,0.358156810349748)
--cycle;

\path [fill=blue, fill opacity=0.4, ultra thick]
(axis cs:1,0.112383269958444)
--(axis cs:1,0.08778626405545)
--(axis cs:5,0.0130619439732912)
--(axis cs:10,0.0160178190904799)
--(axis cs:20,0.0173217215759679)
--(axis cs:100,0.0127757712234337)
--(axis cs:100,0.0171697606795847)
--(axis cs:100,0.0171697606795847)
--(axis cs:20,0.0226137352424347)
--(axis cs:10,0.0264860883282459)
--(axis cs:5,0.0162948465391275)
--(axis cs:1,0.112383269958444)
--cycle;

\path [fill=color0, fill opacity=0.4, ultra thick]
(axis cs:1,0.0205045290709664)
--(axis cs:1,0.0120254340172996)
--(axis cs:5,0.0135003245620557)
--(axis cs:10,0.0129304084580649)
--(axis cs:20,0.0130269641273556)
--(axis cs:100,0.0146339844868641)
--(axis cs:100,0.0220763006689502)
--(axis cs:100,0.0220763006689502)
--(axis cs:20,0.0228135113984045)
--(axis cs:10,0.019268864106573)
--(axis cs:5,0.0222284630625251)
--(axis cs:1,0.0205045290709664)
--cycle;

\addplot [ultra thick, red, mark=*, mark size=1.5, mark options={solid}]
table {%
1 0.323421210050583
5 0.0193966459482908
10 0.0195959247648716
20 0.0357619263231754
100 0.0213072281330824
};
\addlegendentry{Baseline}
\addplot [ultra thick, blue, mark=*, mark size=1.5, mark options={solid}]
table {%
1 0.100084774196148
5 0.0146783944219351
10 0.0212519560009241
20 0.0199677310883999
100 0.014972765929997
};
\addlegendentry{K1}
\addplot [ultra thick, color0, mark=*, mark size=1.5, mark options={solid}]
table {%
1 0.0162649787962437
5 0.0178643949329853
10 0.0160996317863464
20 0.0179202351719141
100 0.0183551404625177
};
\addlegendentry{K2}

==> supp_mat/double_pend/phi_1_dot_dynamics_data.tex <==
\addplot [ultra thick, green!50.1960784313725!black, dashed]
table {%
0 -0.480681180953979
0.0199999809265137 -0.534592866897583
0.0399999618530273 -0.585776567459106
0.059999942779541 -0.63373589515686
0.0800000429153442 -0.677995204925537
0.0900000333786011 -0.698596954345703
0.100000023841858 -0.718109369277954
0.110000014305115 -0.736482381820679
0.120000004768372 -0.753669261932373
0.129999995231628 -0.769626379013062
0.139999985694885 -0.784313678741455
0.149999976158142 -0.797694206237793
0.159999966621399 -0.809736251831055
0.169999957084656 -0.820409178733826
0.180000066757202 -0.829691648483276
0.190000057220459 -0.837563276290894
0.200000047683716 -0.844009399414062
0.210000038146973 -0.84902012348175
0.220000028610229 -0.852590560913086
0.230000019073486 -0.854719758033752
0.240000009536743 -0.855414390563965
0.25 -0.854681968688965
0.259999990463257 -0.852537393569946
0.269999980926514 -0.848999261856079
0.279999971389771 -0.84408974647522
0.289999961853027 -0.837838292121887
0.299999952316284 -0.830274105072021
0.309999942779541 -0.821432113647461
0.319999933242798 -0.811350345611572
0.330000042915344 -0.800071477890015
0.340000033378601 -0.787639260292053
0.350000023841858 -0.774100303649902
0.360000014305115 -0.759504437446594
0.370000004768372 -0.743903517723083
0.379999995231628 -0.727352380752563
0.399999976158142 -0.691623210906982
0.419999957084656 -0.652780294418335
0.440000057220459 -0.61131489276886
0.460000038146973 -0.567732810974121
0.490000009536743 -0.499534368515015
0.579999923706055 -0.291450500488281
0.600000023841858 -0.247876167297363
0.620000004768372 -0.206328868865967
0.639999985694885 -0.16722583770752
0.660000085830688 -0.130927562713623
0.680000066757202 -0.0977267026901245
0.690000057220459 -0.0823591947555542
0.700000047683716 -0.0678414106369019
0.710000038146973 -0.0541881322860718
0.720000028610229 -0.0414085388183594
0.730000019073486 -0.0295075178146362
0.740000009536743 -0.018484354019165
0.75 -0.00833356380462646
0.759999990463257 0.000954508781433105
0.769999980926514 0.00939404964447021
0.779999971389771 0.0170028209686279
0.789999961853027 0.0238025188446045
0.799999952316284 0.0298178195953369
0.809999942779541 0.0350759029388428
0.819999933242798 0.0396065711975098
0.829999923706055 0.0434415340423584
0.839999914169312 0.0466139316558838
0.850000023841858 0.0491580963134766
0.860000014305115 0.0511091947555542
0.870000004768372 0.0525029897689819
0.879999995231628 0.053375244140625
0.889999985694885 0.0537617206573486
0.910000085830688 0.0532193183898926
0.930000066757202 0.0511544942855835
0.950000047683716 0.0478354692459106
0.970000028610229 0.043519139289856
0.990000009536743 0.0384513139724731
1.01999998092651 0.0299577713012695
1.08000004291534 0.0126293897628784
1.10000002384186 0.00762367248535156
1.12000000476837 0.0034252405166626
1.13999998569489 0.000308036804199219
1.1599999666214 -0.00143933296203613
1.16999995708466 -0.00170552730560303
1.17999994754791 -0.00151526927947998
1.19000005722046 -0.000829815864562988
1.20000004768372 0.000390052795410156
1.21000003814697 0.00218319892883301
1.22000002861023 0.00458788871765137
1.23000001907349 0.00764179229736328
1.24000000953674 0.0113810300827026
1.25 0.0158402919769287
1.25999999046326 0.0210517644882202
1.26999998092651 0.027045726776123
1.27999997138977 0.0338486433029175
1.28999996185303 0.0414841175079346
1.29999995231628 0.0499718189239502
1.30999994277954 0.0593267679214478
1.32000005245209 0.0695595741271973
1.33000004291534 0.0806763172149658
1.3400000333786 0.0926774740219116
1.35000002384186 0.105558276176453
1.36000001430511 0.119308710098267
1.37000000476837 0.133913040161133
1.37999999523163 0.149350166320801
1.39999997615814 0.182612419128418
1.41999995708466 0.218823313713074
1.44000005722046 0.25763726234436
1.46000003814697 0.298645615577698
1.48000001907349 0.341387271881104
1.49000000953674 0.363253593444824
};
\addplot [ultra thick, red]
table {%
0 -0.480681180953979
0.0199999809265137 -0.533937335014343
0.0399999618530273 -0.584865212440491
0.059999942779541 -0.63304328918457
0.0800000429153442 -0.678117394447327
0.100000023841858 -0.719638586044312
0.110000014305115 -0.738881587982178
0.120000004768372 -0.757035493850708
0.129999995231628 -0.774103164672852
0.139999985694885 -0.790076971054077
0.149999976158142 -0.804876804351807
0.159999966621399 -0.818463325500488
0.169999957084656 -0.830866694450378
0.180000066757202 -0.842046737670898
0.190000057220459 -0.851926326751709
0.200000047683716 -0.860478520393372
0.210000038146973 -0.867661118507385
0.220000028610229 -0.873458623886108
0.230000019073486 -0.8778235912323
0.240000009536743 -0.880852937698364
0.25 -0.882518291473389
0.259999990463257 -0.882696866989136
0.269999980926514 -0.881384611129761
0.279999971389771 -0.878733515739441
0.289999961853027 -0.874793529510498
0.299999952316284 -0.869491100311279
0.309999942779541 -0.862787485122681
0.319999933242798 -0.854731798171997
0.330000042915344 -0.84534478187561
0.340000033378601 -0.83466362953186
0.350000023841858 -0.822812676429749
0.360000014305115 -0.80984902381897
0.370000004768372 -0.795789003372192
0.379999995231628 -0.780634999275208
0.389999985694885 -0.764451861381531
0.399999976158142 -0.747335076332092
0.419999957084656 -0.710529088973999
0.440000057220459 -0.670581579208374
0.460000038146973 -0.628018140792847
0.480000019073486 -0.583622694015503
0.509999990463257 -0.514552474021912
0.589999914169312 -0.327289938926697
0.610000014305115 -0.283124804496765
0.629999995231628 -0.241012930870056
0.649999976158142 -0.201382875442505
0.670000076293945 -0.16428279876709
0.690000057220459 -0.129839062690735
0.700000047683716 -0.113773465156555
0.710000038146973 -0.0986599922180176
0.720000028610229 -0.084526538848877
0.730000019073486 -0.0713659524917603
0.740000009536743 -0.0591596364974976
0.75 -0.0478278398513794
0.759999990463257 -0.0373440980911255
0.769999980926514 -0.0277142524719238
0.779999971389771 -0.0189712047576904
0.789999961853027 -0.011139988899231
0.799999952316284 -0.00418102741241455
0.809999942779541 0.00199210643768311
0.819999933242798 0.00741851329803467
0.829999923706055 0.0121356248855591
0.839999914169312 0.0161707401275635
0.850000023841858 0.0195292234420776
0.860000014305115 0.0222147703170776
0.870000004768372 0.0242235660552979
0.879999995231628 0.0256065130233765
0.889999985694885 0.0263971090316772
0.899999976158142 0.0266557931900024
0.920000076293945 0.0257819890975952
0.940000057220459 0.0234013795852661
0.960000038146973 0.0196982622146606
0.980000019073486 0.0149115324020386
1 0.00930929183959961
1.02999997138977 1.19209289550781e-05
1.0900000333786 -0.0188620090484619
1.11000001430511 -0.0244046449661255
1.12999999523163 -0.0291825532913208
1.14999997615814 -0.0329784154891968
1.16999995708466 -0.0356303453445435
1.19000005722046 -0.0368642807006836
1.20000004768372 -0.0368552207946777
1.21000003814697 -0.0363630056381226
1.22000002861023 -0.035355806350708
1.23000001907349 -0.0337735414505005
1.24000000953674 -0.031586766242981
1.25 -0.0287792682647705
1.25999999046326 -0.0253281593322754
1.26999998092651 -0.021185040473938
1.27999997138977 -0.0162997245788574
1.28999996185303 -0.0105917453765869
1.29999995231628 -0.00401866436004639
1.30999994277954 0.00346684455871582
1.32000005245209 0.0118309259414673
1.33000004291534 0.0210983753204346
1.3400000333786 0.0313328504562378
1.35000002384186 0.0425665378570557
1.36000001430511 0.0547809600830078
1.37000000476837 0.0679537057876587
1.37999999523163 0.0821197032928467
1.38999998569489 0.0973066091537476
1.39999997615814 0.113386034965515
1.4099999666214 0.130399823188782
1.42999994754791 0.167182564735413
1.45000004768372 0.207137584686279
1.47000002861023 0.24984872341156
1.49000000953674 0.295053243637085
};
\addplot [ultra thick, blue]
table {%
0 -0.480681180953979
0.0199999809265137 -0.53441333770752
0.0399999618530273 -0.585434198379517
0.059999942779541 -0.633220195770264
0.0800000429153442 -0.677313566207886
0.0900000333786011 -0.697839498519897
0.100000023841858 -0.717310786247253
0.110000014305115 -0.735682368278503
0.120000004768372 -0.752912998199463
0.129999995231628 -0.768963932991028
0.139999985694885 -0.783799886703491
0.149999976158142 -0.797390818595886
0.159999966621399 -0.809711694717407
0.169999957084656 -0.820731163024902
0.180000066757202 -0.830418109893799
0.190000057220459 -0.838746190071106
0.200000047683716 -0.845715403556824
0.210000038146973 -0.851304769515991
0.220000028610229 -0.855487704277039
0.230000019073486 -0.858273029327393
0.240000009536743 -0.859590530395508
0.25 -0.859293460845947
0.259999990463257 -0.857344746589661
0.269999980926514 -0.85369610786438
0.279999971389771 -0.848421931266785
0.289999961853027 -0.841752052307129
0.299999952316284 -0.83400547504425
0.309999942779541 -0.825271129608154
0.319999933242798 -0.815570473670959
0.330000042915344 -0.804920673370361
0.340000033378601 -0.793414950370789
0.350000023841858 -0.781076908111572
0.360000014305115 -0.767951488494873
0.370000004768372 -0.754027009010315
0.379999995231628 -0.739176273345947
0.389999985694885 -0.723389625549316
0.399999976158142 -0.706707835197449
0.419999957084656 -0.67083215713501
0.440000057220459 -0.631972551345825
0.460000038146973 -0.590606212615967
0.480000019073486 -0.547114610671997
0.509999990463257 -0.478955626487732
0.589999914169312 -0.293729662895203
0.610000014305115 -0.249775290489197
0.629999995231628 -0.207550883293152
0.649999976158142 -0.167373061180115
0.670000076293945 -0.129587292671204
0.690000057220459 -0.0945466756820679
0.710000038146973 -0.0625811815261841
0.720000028610229 -0.0478248596191406
0.730000019073486 -0.0339134931564331
0.740000009536743 -0.0208667516708374
0.75 -0.00870442390441895
0.759999990463257 0.00255918502807617
0.769999980926514 0.012919545173645
0.779999971389771 0.022374153137207
0.789999961853027 0.0309228897094727
0.799999952316284 0.0385514497756958
0.809999942779541 0.0452582836151123
0.819999933242798 0.0510549545288086
0.829999923706055 0.0559570789337158
0.839999914169312 0.0599836111068726
0.850000023841858 0.0631511211395264
0.860000014305115 0.0654876232147217
0.870000004768372 0.0670340061187744
0.879999995231628 0.067826509475708
0.889999985694885 0.0679111480712891
0.899999976158142 0.0673277378082275
0.910000085830688 0.0661189556121826
0.920000076293945 0.0643236637115479
0.930000066757202 0.0619925260543823
0.940000057220459 0.0591762065887451
0.960000038146973 0.0522409677505493
0.980000019073486 0.0438448190689087
1 0.0343871116638184
1.02999997138977 0.0190199613571167
1.07000005245209 -0.00167667865753174
1.0900000333786 -0.0112566947937012
1.11000001430511 -0.0198639631271362
1.12999999523163 -0.027069091796875
1.13999998569489 -0.0300222635269165
1.14999997615814 -0.0324832201004028
1.1599999666214 -0.0343992710113525
1.16999995708466 -0.0357130765914917
1.17999994754791 -0.0363837480545044
1.19000005722046 -0.03635573387146
1.20000004768372 -0.035542368888855
1.21000003814697 -0.0339163541793823
1.22000002861023 -0.0314515829086304
1.23000001907349 -0.0281262397766113
1.24000000953674 -0.0239143371582031
1.25 -0.0187770128250122
1.25999999046326 -0.0126882791519165
1.26999998092651 -0.00563549995422363
1.27999997138977 0.00239253044128418
1.28999996185303 0.0114148855209351
1.29999995231628 0.0214848518371582
1.30999994277954 0.0326372385025024
1.32000005245209 0.0448756217956543
1.33000004291534 0.0581732988357544
1.3400000333786 0.0724983215332031
1.35000002384186 0.0878150463104248
1.36000001430511 0.104088187217712
1.37000000476837 0.121287822723389
1.38999998569489 0.158351421356201
1.4099999666214 0.198709726333618
1.42999994754791 0.241916656494141
1.45000004768372 0.287535667419434
1.47000002861023 0.335330963134766
1.49000000953674 0.385026454925537
};
\addplot [ultra thick, color0]
table {%
0 -0.480681180953979
0.0199999809265137 -0.533701658248901
0.0399999618530273 -0.584283113479614
0.059999942779541 -0.632001161575317
0.0800000429153442 -0.67646336555481
0.100000023841858 -0.717246770858765
0.110000014305115 -0.736133575439453
0.120000004768372 -0.753963232040405
0.129999995231628 -0.77069890499115
0.139999985694885 -0.786286473274231
0.149999976158142 -0.800630569458008
0.159999966621399 -0.813700675964355
0.169999957084656 -0.825458288192749
0.180000066757202 -0.835871696472168
0.190000057220459 -0.844941377639771
0.200000047683716 -0.852668285369873
0.210000038146973 -0.858974933624268
0.220000028610229 -0.863850116729736
0.230000019073486 -0.867307662963867
0.240000009536743 -0.869389057159424
0.25 -0.869999408721924
0.259999990463257 -0.869152784347534
0.269999980926514 -0.866823434829712
0.279999971389771 -0.863102197647095
0.289999961853027 -0.858016490936279
0.299999952316284 -0.851571798324585
0.309999942779541 -0.843706727027893
0.319999933242798 -0.834464073181152
0.330000042915344 -0.823864936828613
0.340000033378601 -0.811999201774597
0.350000023841858 -0.798947095870972
0.360000014305115 -0.78480863571167
0.370000004768372 -0.76961624622345
0.379999995231628 -0.753389477729797
0.389999985694885 -0.736169576644897
0.399999976158142 -0.717990279197693
0.419999957084656 -0.678910374641418
0.440000057220459 -0.636818170547485
0.460000038146973 -0.59248948097229
0.480000019073486 -0.546636343002319
0.509999990463257 -0.475138664245605
0.600000023841858 -0.25812292098999
0.620000004768372 -0.21274995803833
0.639999985694885 -0.169509649276733
0.660000085830688 -0.128895998001099
0.680000066757202 -0.0913856029510498
0.690000057220459 -0.0738834142684937
0.700000047683716 -0.0572869777679443
0.710000038146973 -0.0416333675384521
0.720000028610229 -0.0269546508789062
0.730000019073486 -0.0132768154144287
0.740000009536743 -0.000560283660888672
0.75 0.011197566986084
0.759999990463257 0.0219912528991699
0.769999980926514 0.0318268537521362
0.779999971389771 0.0407054424285889
0.789999961853027 0.0486379861831665
0.799999952316284 0.0556635856628418
0.809999942779541 0.0618016719818115
0.819999933242798 0.0670711994171143
0.829999923706055 0.0714943408966064
0.839999914169312 0.075096607208252
0.850000023841858 0.0779038667678833
0.860000014305115 0.0799545049667358
0.870000004768372 0.0812857151031494
0.879999995231628 0.0819382667541504
0.889999985694885 0.0819520950317383
0.899999976158142 0.0813683271408081
0.910000085830688 0.0802266597747803
0.920000076293945 0.0785661935806274
0.930000066757202 0.0764211416244507
0.950000047683716 0.0708441734313965
0.970000028610229 0.0638073682785034
0.990000009536743 0.0556156635284424
1.01999998092651 0.0418750047683716
1.07000005245209 0.0173666477203369
1.10000002384186 0.00310146808624268
1.12000000476837 -0.00552034378051758
1.13999998569489 -0.0130362510681152
1.1599999666214 -0.0190213918685913
1.16999995708466 -0.0213571786880493
1.17999994754791 -0.0232093334197998
1.19000005722046 -0.0245348215103149
1.20000004768372 -0.0253103971481323
1.21000003814697 -0.0255151987075806
1.22000002861023 -0.0251109600067139
1.23000001907349 -0.0240498781204224
1.24000000953674 -0.0222867727279663
1.25 -0.0197802782058716
1.25999999046326 -0.0164929628372192
1.26999998092651 -0.0123827457427979
1.27999997138977 -0.00740730762481689
1.28999996185303 -0.00152742862701416
1.29999995231628 0.0053260326385498
1.30999994277954 0.0132150650024414
1.32000005245209 0.0221627950668335
1.33000004291534 0.0321886539459229
1.3400000333786 0.0433094501495361
1.35000002384186 0.0555286407470703
1.36000001430511 0.0688440799713135
1.37000000476837 0.0832511186599731
1.37999999523163 0.0987035036087036
1.38999998569489 0.115163207054138
1.39999997615814 0.132624864578247
1.4099999666214 0.151066541671753
1.42999994754791 0.190645694732666
1.45000004768372 0.233394145965576
1.47000002861023 0.278836250305176
1.49000000953674 0.326687574386597
};

==> supp_mat/double_pend/phi_1_dynamics_data.tex <==
\addplot [ultra thick, green!50.1960784313725!black, dashed]
table {%
0 0.226413011550903
0.00999999046325684 0.221436381340027
0.0199999809265137 0.216188311576843
0.0299999713897705 0.210675477981567
0.0399999618530273 0.204905271530151
0.0499999523162842 0.198884606361389
0.059999942779541 0.192622780799866
0.0700000524520874 0.186128497123718
0.0800000429153442 0.1794114112854
0.0900000333786011 0.172481656074524
0.110000014305115 0.158027529716492
0.129999995231628 0.142857789993286
0.149999976158142 0.127071261405945
0.169999957084656 0.110773086547852
0.190000057220459 0.0940735340118408
0.220000028610229 0.0685198307037354
0.289999961853027 0.00855779647827148
0.309999942779541 -0.00815403461456299
0.330000042915344 -0.0244852304458618
0.350000023841858 -0.0403393507003784
0.370000004768372 -0.0556273460388184
0.389999985694885 -0.0702682733535767
0.409999966621399 -0.0841906070709229
0.419999957084656 -0.0908617973327637
0.430000066757202 -0.0973308086395264
0.440000057220459 -0.103590965270996
0.450000047683716 -0.109636902809143
0.460000038146973 -0.115463256835938
0.470000028610229 -0.121065855026245
0.480000019073486 -0.12644100189209
0.490000009536743 -0.131585836410522
0.5 -0.136497735977173
0.509999990463257 -0.141175150871277
0.519999980926514 -0.145617127418518
0.529999971389771 -0.149823427200317
0.539999961853027 -0.153794288635254
0.549999952316284 -0.157530903816223
0.559999942779541 -0.16103458404541
0.569999933242798 -0.164308309555054
0.579999923706055 -0.167354702949524
0.589999914169312 -0.170177459716797
0.600000023841858 -0.172780871391296
0.610000014305115 -0.175169706344604
0.620000004768372 -0.17734968662262
0.629999995231628 -0.179325461387634
0.639999985694885 -0.181105494499207
0.649999976158142 -0.182695150375366
0.660000085830688 -0.184101819992065
0.670000076293945 -0.185333609580994
0.690000057220459 -0.187304019927979
0.710000038146973 -0.188672780990601
0.730000019073486 -0.189509391784668
0.75 -0.189884424209595
0.769999980926514 -0.189867973327637
0.789999961853027 -0.189528465270996
0.809999942779541 -0.188930511474609
0.839999914169312 -0.187682032585144
0.879999995231628 -0.185638785362244
0.950000047683716 -0.181968092918396
0.990000009536743 -0.180220603942871
1.01999998092651 -0.179185748100281
1.04999995231628 -0.178414940834045
1.08000004291534 -0.177907943725586
1.12000000476837 -0.177595496177673
1.16999995708466 -0.177590131759644
1.22000002861023 -0.177575588226318
1.25 -0.177283048629761
1.26999998092651 -0.176856637001038
1.28999996185303 -0.176172375679016
1.30999994277954 -0.175163269042969
1.33000004291534 -0.173759937286377
1.35000002384186 -0.1718909740448
1.37000000476837 -0.169486045837402
1.38999998569489 -0.166476368904114
1.39999997615814 -0.164724588394165
1.4099999666214 -0.162797331809998
1.41999995708466 -0.160688042640686
1.42999994754791 -0.158389568328857
1.44000005722046 -0.155895709991455
1.45000004768372 -0.153200626373291
1.46000003814697 -0.150299072265625
1.47000002861023 -0.147186517715454
1.48000001907349 -0.143858432769775
1.49000000953674 -0.140312194824219
};
\addlegendentry{True dynamics}
\addplot [ultra thick, red]
table {%
0 0.226413011550903
0.00999999046325684 0.222060441970825
0.0199999809265137 0.217421650886536
0.0299999713897705 0.212526082992554
0.0399999618530273 0.207375764846802
0.0499999523162842 0.201975345611572
0.059999942779541 0.196334719657898
0.0700000524520874 0.190466165542603
0.0800000429153442 0.184371113777161
0.0900000333786011 0.178027868270874
0.100000023841858 0.17143452167511
0.110000014305115 0.164601802825928
0.120000004768372 0.157552480697632
0.139999985694885 0.14286470413208
0.159999966621399 0.127473592758179
0.180000066757202 0.111520767211914
0.200000047683716 0.0951055288314819
0.230000019073486 0.0698764324188232
0.279999971389771 0.0271990299224854
0.309999942779541 0.00162887573242188
0.330000042915344 -0.0150630474090576
0.350000023841858 -0.0313287973403931
0.370000004768372 -0.0470895767211914
0.389999985694885 -0.0622299909591675
0.409999966621399 -0.0766987800598145
0.419999957084656 -0.0836714506149292
0.430000066757202 -0.0904203653335571
0.440000057220459 -0.0969357490539551
0.450000047683716 -0.103223562240601
0.460000038146973 -0.109289646148682
0.470000028610229 -0.115159869194031
0.480000019073486 -0.120819807052612
0.490000009536743 -0.126265645027161
0.5 -0.131484389305115
0.509999990463257 -0.136478662490845
0.519999980926514 -0.141255617141724
0.529999971389771 -0.145810127258301
0.539999961853027 -0.150143504142761
0.549999952316284 -0.154259324073792
0.559999942779541 -0.158154010772705
0.569999933242798 -0.161819458007812
0.579999923706055 -0.165292620658875
0.589999914169312 -0.168593645095825
0.600000023841858 -0.17169713973999
0.610000014305115 -0.174598336219788
0.620000004768372 -0.177281022071838
0.629999995231628 -0.179733037948608
0.639999985694885 -0.181948065757751
0.649999976158142 -0.183930516242981
0.660000085830688 -0.18569016456604
0.670000076293945 -0.18723475933075
0.680000066757202 -0.188575506210327
0.690000057220459 -0.189700961112976
0.710000038146973 -0.191463708877563
0.730000019073486 -0.19281792640686
0.75 -0.193803071975708
0.769999980926514 -0.194424033164978
0.789999961853027 -0.194701671600342
0.809999942779541 -0.194672584533691
0.829999923706055 -0.194268465042114
0.850000023841858 -0.193553447723389
0.879999995231628 -0.19214403629303
0.920000076293945 -0.189854741096497
0.970000028610229 -0.186944246292114
0.990000009536743 -0.186100959777832
1.00999999046326 -0.185535550117493
1.02999997138977 -0.185217976570129
1.05999994277954 -0.185116529464722
1.11000001430511 -0.185573101043701
1.16999995708466 -0.18627667427063
1.21000003814697 -0.187150001525879
1.25999999046326 -0.18818473815918
1.28999996185303 -0.188607811927795
1.30999994277954 -0.188452243804932
1.33000004291534 -0.187934160232544
1.35000002384186 -0.187088966369629
1.37000000476837 -0.18592357635498
1.38999998569489 -0.184400677680969
1.39999997615814 -0.183433294296265
1.4099999666214 -0.18228816986084
1.41999995708466 -0.180956959724426
1.42999994754791 -0.179429650306702
1.44000005722046 -0.177713990211487
1.45000004768372 -0.175803422927856
1.46000003814697 -0.173690676689148
1.47000002861023 -0.171362042427063
1.48000001907349 -0.16879940032959
1.49000000953674 -0.165973424911499
};
\addlegendentry{Baseline}
\addplot [ultra thick, blue]
table {%
0 0.226413011550903
0.00999999046325684 0.221606135368347
0.0199999809265137 0.216527581214905
0.0299999713897705 0.211183428764343
0.0399999618530273 0.205580472946167
0.0499999523162842 0.199726223945618
0.059999942779541 0.193628549575806
0.0700000524520874 0.187296390533447
0.0800000429153442 0.180738806724548
0.0900000333786011 0.173965692520142
0.110000014305115 0.159814119338989
0.129999995231628 0.144928216934204
0.149999976158142 0.129400610923767
0.169999957084656 0.113329529762268
0.190000057220459 0.0968180894851685
0.220000028610229 0.0714603662490845
0.299999952316284 0.00312185287475586
0.319999933242798 -0.0134710073471069
0.340000033378601 -0.0296758413314819
0.360000014305115 -0.04542076587677
0.379999995231628 -0.0606405735015869
0.399999976158142 -0.0752662420272827
0.419999957084656 -0.0892250537872314
0.440000057220459 -0.102450728416443
0.450000047683716 -0.108770489692688
0.460000038146973 -0.114886283874512
0.470000028610229 -0.120792388916016
0.480000019073486 -0.12648332118988
0.490000009536743 -0.131954550743103
0.5 -0.13720166683197
0.509999990463257 -0.142221450805664
0.519999980926514 -0.147010922431946
0.529999971389771 -0.151568293571472
0.539999961853027 -0.1558917760849
0.549999952316284 -0.159980654716492
0.559999942779541 -0.163835048675537
0.569999933242798 -0.167456388473511
0.579999923706055 -0.170847296714783
0.589999914169312 -0.174010038375854
0.600000023841858 -0.176947355270386
0.610000014305115 -0.179662823677063
0.620000004768372 -0.182160615921021
0.629999995231628 -0.184444904327393
0.639999985694885 -0.186520338058472
0.649999976158142 -0.188392281532288
0.660000085830688 -0.190065979957581
0.670000076293945 -0.191547513008118
0.680000066757202 -0.192843437194824
0.690000057220459 -0.193960428237915
0.700000047683716 -0.194905877113342
0.720000028610229 -0.196313381195068
0.740000009536743 -0.197130799293518
0.759999990463257 -0.197426438331604
0.779999971389771 -0.197271704673767
0.799999952316284 -0.196738719940186
0.819999933242798 -0.195900678634644
0.850000023841858 -0.194230675697327
0.899999976158142 -0.190916538238525
0.940000057220459 -0.188318967819214
0.970000028610229 -0.18664562702179
1 -0.185332894325256
1.02999997138977 -0.184453010559082
1.05999994277954 -0.18403959274292
1.0900000333786 -0.184088230133057
1.12000000476837 -0.184556484222412
1.14999997615814 -0.185364127159119
1.21000003814697 -0.187472939491272
1.24000000953674 -0.188407897949219
1.25999999046326 -0.1888347864151
1.27999997138977 -0.18901801109314
1.29999995231628 -0.18887996673584
1.32000005245209 -0.188338756561279
1.3400000333786 -0.187308311462402
1.36000001430511 -0.185705065727234
1.37000000476837 -0.184664249420166
1.37999999523163 -0.183451414108276
1.38999998569489 -0.182057499885559
1.39999997615814 -0.180474042892456
1.4099999666214 -0.178692579269409
1.41999995708466 -0.176705479621887
1.42999994754791 -0.174505591392517
1.44000005722046 -0.172086358070374
1.45000004768372 -0.169441938400269
1.46000003814697 -0.166566610336304
1.47000002861023 -0.16345489025116
1.48000001907349 -0.160101532936096
1.49000000953674 -0.156501889228821
};
\addlegendentry{K1}
\addplot [ultra thick, color0]
table {%
0 0.226413011550903
0.00999999046325684 0.221606135368347
0.0199999809265137 0.21653139591217
0.0299999713897705 0.211194396018982
0.0399999618530273 0.205601215362549
0.0499999523162842 0.199758291244507
0.059999942779541 0.193673133850098
0.0700000524520874 0.187353134155273
0.0800000429153442 0.180806398391724
0.0900000333786011 0.174041748046875
0.100000023841858 0.167068362236023
0.120000004768372 0.152534604072571
0.139999985694885 0.137287974357605
0.159999966621399 0.121418833732605
0.180000066757202 0.105027198791504
0.200000047683716 0.0882190465927124
0.230000019073486 0.0624641180038452
0.299999952316284 0.00182628631591797
0.319999933242798 -0.0151265859603882
0.340000033378601 -0.0317097902297974
0.360000014305115 -0.0478192567825317
0.379999995231628 -0.0633635520935059
0.399999976158142 -0.0782591104507446
0.419999957084656 -0.0924277305603027
0.430000066757202 -0.0992168188095093
0.440000057220459 -0.105798602104187
0.450000047683716 -0.11216676235199
0.460000038146973 -0.118315577507019
0.470000028610229 -0.124240398406982
0.480000019073486 -0.129938125610352
0.490000009536743 -0.135404467582703
0.5 -0.140635132789612
0.509999990463257 -0.14562714099884
0.519999980926514 -0.150378465652466
0.529999971389771 -0.154887557029724
0.539999961853027 -0.159152984619141
0.549999952316284 -0.163173913955688
0.559999942779541 -0.166950583457947
0.569999933242798 -0.170484066009521
0.579999923706055 -0.173775553703308
0.589999914169312 -0.176827192306519
0.600000023841858 -0.179641962051392
0.610000014305115 -0.182223200798035
0.620000004768372 -0.184575080871582
0.629999995231628 -0.186702609062195
0.639999985694885 -0.188611030578613
0.649999976158142 -0.190306067466736
0.660000085830688 -0.191794395446777
0.670000076293945 -0.19308340549469
0.680000066757202 -0.194180727005005
0.690000057220459 -0.195094585418701
0.700000047683716 -0.195833444595337
0.720000028610229 -0.196822643280029
0.740000009536743 -0.197224974632263
0.759999990463257 -0.197118639945984
0.779999971389771 -0.196580410003662
0.799999952316284 -0.195687055587769
0.819999933242798 -0.194512367248535
0.850000023841858 -0.192375779151917
0.899999976158142 -0.188345432281494
0.940000057220459 -0.185179591178894
0.970000028610229 -0.183057904243469
1 -0.181265354156494
1.02999997138977 -0.179868698120117
1.05999994277954 -0.178903818130493
1.0900000333786 -0.178382158279419
1.12000000476837 -0.178287267684937
1.14999997615814 -0.178567171096802
1.19000005722046 -0.179365515708923
1.26999998092651 -0.181196331977844
1.29999995231628 -0.181409597396851
1.32000005245209 -0.18122410774231
1.3400000333786 -0.180680632591248
1.36000001430511 -0.179692268371582
1.37999999523163 -0.178171277046204
1.38999998569489 -0.177184224128723
1.39999997615814 -0.176032662391663
1.4099999666214 -0.174706339836121
1.41999995708466 -0.173195719718933
1.42999994754791 -0.171491384506226
1.44000005722046 -0.169584989547729
1.45000004768372 -0.167468428611755
1.46000003814697 -0.16513454914093
1.47000002861023 -0.16257643699646
1.48000001907349 -0.159788012504578
1.49000000953674 -0.156763195991516
};
\addlegendentry{K2}

==> supp_mat/double_pend/phi_2_dot_dynamics_data.tex <==
\addplot [ultra thick, green!50.1960784313725!black, dashed]
table {%
0 -0.375052809715271
0.0199999809265137 -0.35399341583252
0.0399999618530273 -0.334224462509155
0.059999942779541 -0.316332697868347
0.0700000524520874 -0.308269381523132
0.0800000429153442 -0.300885796546936
0.0900000333786011 -0.29424774646759
0.100000023841858 -0.288418173789978
0.110000014305115 -0.283456802368164
0.120000004768372 -0.279419541358948
0.129999995231628 -0.276358604431152
0.139999985694885 -0.274320960044861
0.149999976158142 -0.273349285125732
0.159999966621399 -0.273480415344238
0.169999957084656 -0.274746417999268
0.180000066757202 -0.277171015739441
0.190000057220459 -0.280774235725403
0.200000047683716 -0.285568475723267
0.210000038146973 -0.291559100151062
0.220000028610229 -0.298745393753052
0.230000019073486 -0.307118773460388
0.240000009536743 -0.316665053367615
0.25 -0.327363014221191
0.259999990463257 -0.339184641838074
0.269999980926514 -0.35209596157074
0.279999971389771 -0.366056680679321
0.289999961853027 -0.381022095680237
0.299999952316284 -0.396940469741821
0.309999942779541 -0.413755893707275
0.330000042915344 -0.44983434677124
0.350000023841858 -0.488729000091553
0.370000004768372 -0.529859304428101
0.399999976158142 -0.594385385513306
0.460000038146973 -0.725439786911011
0.480000019073486 -0.767227411270142
0.5 -0.806927680969238
0.519999980926514 -0.843864440917969
0.529999971389771 -0.86108922958374
0.539999961853027 -0.87737512588501
0.549999952316284 -0.892645597457886
0.559999942779541 -0.906818866729736
0.569999933242798 -0.919820547103882
0.579999923706055 -0.931578755378723
0.589999914169312 -0.94202184677124
0.600000023841858 -0.951083421707153
0.610000014305115 -0.958698153495789
0.620000004768372 -0.964807629585266
0.629999995231628 -0.969357848167419
0.639999985694885 -0.972296476364136
0.649999976158142 -0.97357964515686
0.660000085830688 -0.973169803619385
0.670000076293945 -0.971033573150635
0.680000066757202 -0.967144966125488
0.690000057220459 -0.961483359336853
0.700000047683716 -0.954036235809326
0.710000038146973 -0.944798707962036
0.720000028610229 -0.933772563934326
0.730000019073486 -0.920961380004883
0.740000009536743 -0.906385183334351
0.75 -0.890064120292664
0.759999990463257 -0.872025728225708
0.769999980926514 -0.852305054664612
0.779999971389771 -0.830939650535583
0.789999961853027 -0.807975053787231
0.799999952316284 -0.783461570739746
0.809999942779541 -0.757452011108398
0.819999933242798 -0.730002164840698
0.829999923706055 -0.701175212860107
0.850000023841858 -0.639637231826782
0.870000004768372 -0.573366403579712
0.889999985694885 -0.502910971641541
0.910000085830688 -0.428828954696655
0.930000066757202 -0.351680755615234
0.960000038146973 -0.23142421245575
0.990000009536743 -0.107361912727356
1.0900000333786 0.310541868209839
1.12000000476837 0.43026065826416
1.13999998569489 0.506898164749146
1.1599999666214 0.580328583717346
1.17999994754791 0.649967312812805
1.20000004768372 0.715232372283936
1.22000002861023 0.775550961494446
1.23000001907349 0.803682088851929
1.24000000953674 0.830371856689453
1.25 0.85555899143219
1.25999999046326 0.879183053970337
1.26999998092651 0.901188492774963
1.27999997138977 0.921524286270142
1.28999996185303 0.940145015716553
1.29999995231628 0.957009553909302
1.30999994277954 0.972084283828735
1.32000005245209 0.985340714454651
1.33000004291534 0.996757984161377
1.3400000333786 1.0063214302063
1.35000002384186 1.01402401924133
1.36000001430511 1.01987266540527
1.37000000476837 1.02386713027954
1.37999999523163 1.0260261297226
1.38999998569489 1.02637195587158
1.39999997615814 1.02493739128113
1.4099999666214 1.02175486087799
1.41999995708466 1.01687121391296
1.42999994754791 1.01033282279968
1.44000005722046 1.00219297409058
1.45000004768372 0.992514371871948
1.46000003814697 0.981356978416443
1.47000002861023 0.968791961669922
1.48000001907349 0.954890608787537
1.49000000953674 0.939724683761597
};
\addplot [ultra thick, red]
table {%
0 -0.375052809715271
0.0299999713897705 -0.34479296207428
0.0499999523162842 -0.325867176055908
0.0700000524520874 -0.30856192111969
0.0800000429153442 -0.300646305084229
0.0900000333786011 -0.293282032012939
0.100000023841858 -0.286518573760986
0.110000014305115 -0.28044605255127
0.120000004768372 -0.275131464004517
0.129999995231628 -0.27057421207428
0.139999985694885 -0.266843795776367
0.149999976158142 -0.263944029808044
0.159999966621399 -0.261911869049072
0.169999957084656 -0.260740756988525
0.180000066757202 -0.260581970214844
0.190000057220459 -0.261608242988586
0.200000047683716 -0.263932943344116
0.210000038146973 -0.267612457275391
0.220000028610229 -0.272644281387329
0.230000019073486 -0.279072165489197
0.240000009536743 -0.286825656890869
0.25 -0.29586136341095
0.259999990463257 -0.306235909461975
0.269999980926514 -0.317941546440125
0.279999971389771 -0.330834150314331
0.289999961853027 -0.344872117042542
0.299999952316284 -0.360018730163574
0.309999942779541 -0.376288890838623
0.319999933242798 -0.393571615219116
0.340000033378601 -0.430786609649658
0.360000014305115 -0.470796346664429
0.379999995231628 -0.513087749481201
0.409999966621399 -0.579582691192627
0.490000009536743 -0.760274410247803
0.509999990463257 -0.802544593811035
0.529999971389771 -0.842248201370239
0.539999961853027 -0.860876798629761
0.549999952316284 -0.878507494926453
0.559999942779541 -0.895048856735229
0.569999933242798 -0.910327196121216
0.579999923706055 -0.924288749694824
0.589999914169312 -0.936930894851685
0.600000023841858 -0.948229789733887
0.610000014305115 -0.958139657974243
0.620000004768372 -0.966625452041626
0.629999995231628 -0.97360360622406
0.639999985694885 -0.979060411453247
0.649999976158142 -0.983085989952087
0.660000085830688 -0.985669374465942
0.670000076293945 -0.98673677444458
0.680000066757202 -0.986242532730103
0.690000057220459 -0.984138607978821
0.700000047683716 -0.980235576629639
0.710000038146973 -0.974430084228516
0.720000028610229 -0.966770648956299
0.730000019073486 -0.957227349281311
0.740000009536743 -0.945815086364746
0.75 -0.932609558105469
0.759999990463257 -0.917635917663574
0.769999980926514 -0.900911092758179
0.779999971389771 -0.882425308227539
0.789999961853027 -0.862182140350342
0.799999952316284 -0.840234756469727
0.809999942779541 -0.816640377044678
0.819999933242798 -0.791443228721619
0.829999923706055 -0.764711260795593
0.839999914169312 -0.736555337905884
0.850000023841858 -0.707006692886353
0.870000004768372 -0.643865346908569
0.889999985694885 -0.575729608535767
0.910000085830688 -0.503252506256104
0.930000066757202 -0.427269220352173
0.950000047683716 -0.348373770713806
0.980000019073486 -0.225610256195068
1.00999999046326 -0.0990240573883057
1.11000001430511 0.327710628509521
1.13999998569489 0.450340986251831
1.1599999666214 0.529210329055786
1.17999994754791 0.605208396911621
1.20000004768372 0.677639484405518
1.22000002861023 0.745837688446045
1.24000000953674 0.809105634689331
1.25 0.838767528533936
1.25999999046326 0.867063999176025
1.26999998092651 0.893930792808533
1.27999997138977 0.919314622879028
1.28999996185303 0.943103671073914
1.29999995231628 0.965176939964294
1.30999994277954 0.985450744628906
1.32000005245209 1.00395512580872
1.33000004291534 1.02058684825897
1.3400000333786 1.03518092632294
1.35000002384186 1.04772818088531
1.36000001430511 1.05824744701385
1.37000000476837 1.06683325767517
1.37999999523163 1.073481798172
1.38999998569489 1.07815301418304
1.39999997615814 1.08098721504211
1.4099999666214 1.08187830448151
1.41999995708466 1.0807683467865
1.42999994754791 1.07772707939148
1.44000005722046 1.07285761833191
1.45000004768372 1.0662556886673
1.46000003814697 1.05798184871674
1.47000002861023 1.04802083969116
1.48000001907349 1.036465883255
1.49000000953674 1.02337205410004
};
\addplot [ultra thick, blue]
table {%
0 -0.375052809715271
0.0199999809265137 -0.354439616203308
0.0399999618530273 -0.335317254066467
0.0499999523162842 -0.326518654823303
0.059999942779541 -0.318325757980347
0.0700000524520874 -0.310792446136475
0.0800000429153442 -0.303995490074158
0.0900000333786011 -0.297987341880798
0.100000023841858 -0.292775273323059
0.110000014305115 -0.28840959072113
0.120000004768372 -0.284934759140015
0.129999995231628 -0.282394170761108
0.139999985694885 -0.280826330184937
0.149999976158142 -0.28026270866394
0.159999966621399 -0.280729413032532
0.169999957084656 -0.282263040542603
0.180000066757202 -0.284902334213257
0.190000057220459 -0.288683891296387
0.200000047683716 -0.293604731559753
0.210000038146973 -0.299673557281494
0.220000028610229 -0.306903600692749
0.230000019073486 -0.315272569656372
0.240000009536743 -0.324841260910034
0.25 -0.335751533508301
0.259999990463257 -0.348031997680664
0.269999980926514 -0.361712574958801
0.279999971389771 -0.37670111656189
0.299999952316284 -0.409523010253906
0.319999933242798 -0.444836497306824
0.340000033378601 -0.482085943222046
0.370000004768372 -0.540358304977417
0.389999985694885 -0.580827951431274
0.419999957084656 -0.643582582473755
0.470000028610229 -0.748948454856873
0.5 -0.809882879257202
0.519999980926514 -0.848361015319824
0.539999961853027 -0.88438355922699
0.549999952316284 -0.901211738586426
0.559999942779541 -0.91693913936615
0.569999933242798 -0.931445121765137
0.579999923706055 -0.944803357124329
0.589999914169312 -0.956969976425171
0.600000023841858 -0.967820525169373
0.610000014305115 -0.977311134338379
0.620000004768372 -0.985439300537109
0.629999995231628 -0.992175221443176
0.639999985694885 -0.997470855712891
0.649999976158142 -1.00127410888672
0.660000085830688 -1.00353848934174
0.670000076293945 -1.00421047210693
0.680000066757202 -1.00323903560638
0.690000057220459 -1.00056374073029
0.700000047683716 -0.996142625808716
0.710000038146973 -0.989949107170105
0.720000028610229 -0.981957197189331
0.730000019073486 -0.972152471542358
0.740000009536743 -0.960522413253784
0.75 -0.947054862976074
0.759999990463257 -0.931743860244751
0.769999980926514 -0.91459846496582
0.779999971389771 -0.895631790161133
0.789999961853027 -0.874860048294067
0.799999952316284 -0.852285861968994
0.809999942779541 -0.827928781509399
0.819999933242798 -0.801822423934937
0.829999923706055 -0.774008512496948
0.839999914169312 -0.744529366493225
0.850000023841858 -0.713431119918823
0.860000014305115 -0.680772542953491
0.879999995231628 -0.611066102981567
0.899999976158142 -0.53601598739624
0.920000076293945 -0.456254005432129
0.940000057220459 -0.372455358505249
0.960000038146973 -0.28530216217041
0.990000009536743 -0.149757981300354
1.02999997138977 0.0361281633377075
1.08000004291534 0.26858651638031
1.11000001430511 0.403778553009033
1.12999999523163 0.490597486495972
1.14999997615814 0.573909044265747
1.16999995708466 0.652990341186523
1.19000005722046 0.727120876312256
1.21000003814697 0.795507907867432
1.22000002861023 0.827368378639221
1.23000001907349 0.857600092887878
1.24000000953674 0.886144757270813
1.25 0.912933230400085
1.25999999046326 0.937911510467529
1.26999998092651 0.961040735244751
1.27999997138977 0.982285499572754
1.28999996185303 1.00160574913025
1.29999995231628 1.0189266204834
1.30999994277954 1.03419637680054
1.32000005245209 1.04739475250244
1.33000004291534 1.05853724479675
1.3400000333786 1.06764805316925
1.35000002384186 1.07475459575653
1.36000001430511 1.07989060878754
1.37000000476837 1.08308219909668
1.37999999523163 1.08435726165771
1.38999998569489 1.08373987674713
1.39999997615814 1.08127665519714
1.4099999666214 1.07704019546509
1.41999995708466 1.07109928131104
1.42999994754791 1.0635232925415
1.44000005722046 1.05437934398651
1.45000004768372 1.04370725154877
1.46000003814697 1.03148508071899
1.47000002861023 1.01768612861633
1.48000001907349 1.00236880779266
1.49000000953674 0.985586047172546
};
\addplot [ultra thick, color0]
table {%
0 -0.375052809715271
0.0199999809265137 -0.355425119400024
0.0399999618530273 -0.336840867996216
0.059999942779541 -0.319757342338562
0.0800000429153442 -0.304588794708252
0.0900000333786011 -0.297880053520203
0.100000023841858 -0.291837811470032
0.110000014305115 -0.28652012348175
0.120000004768372 -0.281968474388123
0.129999995231628 -0.278219938278198
0.139999985694885 -0.275350451469421
0.149999976158142 -0.273462414741516
0.159999966621399 -0.272584915161133
0.169999957084656 -0.272766351699829
0.180000066757202 -0.274045586585999
0.190000057220459 -0.276425719261169
0.200000047683716 -0.279907703399658
0.210000038146973 -0.284570932388306
0.220000028610229 -0.290427684783936
0.230000019073486 -0.297469973564148
0.240000009536743 -0.305666923522949
0.25 -0.315110445022583
0.259999990463257 -0.325777769088745
0.269999980926514 -0.337688446044922
0.279999971389771 -0.350744009017944
0.289999961853027 -0.364902019500732
0.299999952316284 -0.380129218101501
0.309999942779541 -0.396454095840454
0.319999933242798 -0.413812398910522
0.340000033378601 -0.451374053955078
0.360000014305115 -0.491986989974976
0.379999995231628 -0.534942388534546
0.399999976158142 -0.579834222793579
0.440000057220459 -0.672948837280273
0.460000038146973 -0.71928083896637
0.490000009536743 -0.785741806030273
0.509999990463257 -0.827916502952576
0.529999971389771 -0.867523908615112
0.549999952316284 -0.904052257537842
0.559999942779541 -0.920892953872681
0.569999933242798 -0.936716794967651
0.579999923706055 -0.951441168785095
0.589999914169312 -0.964968681335449
0.600000023841858 -0.977202653884888
0.610000014305115 -0.988062143325806
0.620000004768372 -0.997481465339661
0.629999995231628 -1.00540602207184
0.639999985694885 -1.01176905632019
0.649999976158142 -1.01650047302246
0.660000085830688 -1.01947629451752
0.670000076293945 -1.02064990997314
0.680000066757202 -1.02004015445709
0.690000057220459 -1.01760029792786
0.700000047683716 -1.01327621936798
0.710000038146973 -1.00703191757202
0.720000028610229 -0.998838663101196
0.730000019073486 -0.988676786422729
0.740000009536743 -0.976596593856812
0.75 -0.962610483169556
0.759999990463257 -0.94672703742981
0.769999980926514 -0.928970575332642
0.779999971389771 -0.909358620643616
0.789999961853027 -0.887919902801514
0.799999952316284 -0.864713668823242
0.809999942779541 -0.839781522750854
0.819999933242798 -0.813165903091431
0.829999923706055 -0.784915089607239
0.839999914169312 -0.755081415176392
0.850000023841858 -0.723716020584106
0.870000004768372 -0.656666159629822
0.889999985694885 -0.584355354309082
0.910000085830688 -0.507404923439026
0.930000066757202 -0.426422834396362
0.950000047683716 -0.342018842697144
0.980000019073486 -0.210339784622192
1.00999999046326 -0.0744529962539673
1.11000001430511 0.382781505584717
1.13999998569489 0.513292193412781
1.1599999666214 0.596461772918701
1.17999994754791 0.675846099853516
1.20000004768372 0.750841617584229
1.22000002861023 0.82090950012207
1.24000000953674 0.885424852371216
1.25 0.915406346321106
1.25999999046326 0.943779826164246
1.26999998092651 0.970473289489746
1.27999997138977 0.995416164398193
1.28999996185303 1.01854228973389
1.29999995231628 1.03975772857666
1.30999994277954 1.05897724628448
1.32000005245209 1.07615685462952
1.33000004291534 1.09125804901123
1.3400000333786 1.10424113273621
1.35000002384186 1.11508738994598
1.36000001430511 1.12378740310669
1.37000000476837 1.13032913208008
1.37999999523163 1.13474428653717
1.38999998569489 1.13707137107849
1.39999997615814 1.137286901474
1.4099999666214 1.13539743423462
1.41999995708466 1.13148009777069
1.42999994754791 1.1256285905838
1.44000005722046 1.11791825294495
1.45000004768372 1.10841405391693
1.46000003814697 1.09718346595764
1.47000002861023 1.08432006835938
1.48000001907349 1.06974589824677
1.49000000953674 1.05349922180176
};


==> supp_mat/double_pend/phi_2_dynamics_data.tex <==
\addplot [ultra thick, green!50.1960784313725!black, dashed]
table {%
0 0.1720130443573
0.0199999809265137 0.16467559337616
0.0399999618530273 0.157750248908997
0.059999942779541 0.151204943656921
0.0900000333786011 0.142001271247864
0.120000004768372 0.13335919380188
0.220000028610229 0.105218172073364
0.240000009536743 0.0990309715270996
0.259999990463257 0.0924361944198608
0.279999971389771 0.0853438377380371
0.299999952316284 0.0776693820953369
0.319999933242798 0.0693362951278687
0.340000033378601 0.0602772235870361
0.360000014305115 0.0504356622695923
0.379999995231628 0.0397665500640869
0.399999976158142 0.0282371044158936
0.419999957084656 0.0158283710479736
0.440000057220459 0.00253379344940186
0.460000038146973 -0.0116386413574219
0.480000019073486 -0.0266677141189575
0.5 -0.0425183773040771
0.519999980926514 -0.0591415166854858
0.539999961853027 -0.0764749050140381
0.559999942779541 -0.0944430828094482
0.579999923706055 -0.112958073616028
0.610000014305115 -0.141533374786377
0.649999976158142 -0.180522561073303
0.700000047683716 -0.229218721389771
0.720000028610229 -0.248234748840332
0.740000009536743 -0.266770958900452
0.759999990463257 -0.284685373306274
0.779999971389771 -0.301839113235474
0.799999952316284 -0.318100929260254
0.819999933242798 -0.333346486091614
0.829999923706055 -0.340551495552063
0.839999914169312 -0.347459435462952
0.850000023841858 -0.354057192802429
0.860000014305115 -0.360333204269409
0.870000004768372 -0.366275548934937
0.879999995231628 -0.371873378753662
0.889999985694885 -0.377116560935974
0.899999976158142 -0.381995558738708
0.910000085830688 -0.386501550674438
0.920000076293945 -0.390627145767212
0.930000066757202 -0.394363522529602
0.940000057220459 -0.397705316543579
0.950000047683716 -0.400645971298218
0.960000038146973 -0.403180360794067
0.970000028610229 -0.405303835868835
0.980000019073486 -0.407012462615967
0.990000009536743 -0.408303260803223
1 -0.409173369407654
1.00999999046326 -0.409621000289917
1.01999998092651 -0.409644842147827
1.02999997138977 -0.409244537353516
1.03999996185303 -0.408419847488403
1.04999995231628 -0.407171845436096
1.05999994277954 -0.405501842498779
1.07000005245209 -0.403411984443665
1.08000004291534 -0.400905013084412
1.0900000333786 -0.397984266281128
1.10000002384186 -0.394654154777527
1.11000001430511 -0.390919208526611
1.12000000476837 -0.386785745620728
1.12999999523163 -0.382259011268616
1.13999998569489 -0.377346158027649
1.14999997615814 -0.372056841850281
1.1599999666214 -0.366396188735962
1.16999995708466 -0.360375642776489
1.17999994754791 -0.354004383087158
1.19000005722046 -0.347293257713318
1.20000004768372 -0.340253591537476
1.21000003814697 -0.332897305488586
1.23000001907349 -0.317287445068359
1.25 -0.30057430267334
1.26999998092651 -0.282878994941711
1.28999996185303 -0.264331340789795
1.30999994277954 -0.24506950378418
1.33000004291534 -0.225237607955933
1.36000001430511 -0.194744348526001
1.44000005722046 -0.112576484680176
1.46000003814697 -0.0925986766815186
1.48000001907349 -0.0730980634689331
1.49000000953674 -0.0635608434677124
};
\addplot [ultra thick, red]
table {%
0 0.1720130443573
0.0199999809265137 0.164787292480469
0.0499999523162842 0.154523491859436
0.0800000429153442 0.144828796386719
0.110000014305115 0.135755896568298
0.190000057220459 0.112717151641846
0.220000028610229 0.10397732257843
0.25 0.0946859121322632
0.279999971389771 0.0847444534301758
0.299999952316284 0.077631950378418
0.319999933242798 0.0700103044509888
0.340000033378601 0.0618181228637695
0.360000014305115 0.0528779029846191
0.379999995231628 0.0430694818496704
0.399999976158142 0.032381534576416
0.419999957084656 0.020869255065918
0.440000057220459 0.00843179225921631
0.460000038146973 -0.0049128532409668
0.480000019073486 -0.0191214084625244
0.5 -0.034176230430603
0.519999980926514 -0.05002760887146
0.539999961853027 -0.0666161775588989
0.559999942779541 -0.0839835405349731
0.579999923706055 -0.102072358131409
0.610000014305115 -0.130043983459473
0.639999985694885 -0.158814430236816
0.680000066757202 -0.198253631591797
0.75 -0.267154812812805
0.769999980926514 -0.286407947540283
0.789999961853027 -0.305055618286133
0.809999942779541 -0.322777986526489
0.829999923706055 -0.339400053024292
0.839999914169312 -0.347267985343933
0.850000023841858 -0.354826688766479
0.860000014305115 -0.362074136734009
0.870000004768372 -0.368971586227417
0.879999995231628 -0.375504016876221
0.889999985694885 -0.381661534309387
0.899999976158142 -0.387444615364075
0.910000085830688 -0.392851710319519
0.920000076293945 -0.397881150245667
0.930000066757202 -0.402544021606445
0.940000057220459 -0.406829595565796
0.950000047683716 -0.410747766494751
0.960000038146973 -0.414315342903137
0.970000028610229 -0.417531609535217
0.980000019073486 -0.420383930206299
0.990000009536743 -0.422860622406006
1 -0.424949169158936
1.00999999046326 -0.426622033119202
1.01999998092651 -0.427864551544189
1.02999997138977 -0.428663015365601
1.03999996185303 -0.429016470909119
1.04999995231628 -0.428964734077454
1.05999994277954 -0.428489089012146
1.07000005245209 -0.427588105201721
1.08000004291534 -0.42623233795166
1.0900000333786 -0.424414277076721
1.10000002384186 -0.42213237285614
1.11000001430511 -0.419396042823792
1.12000000476837 -0.416221380233765
1.12999999523163 -0.412630438804626
1.13999998569489 -0.408641934394836
1.14999997615814 -0.404266595840454
1.1599999666214 -0.399503469467163
1.16999995708466 -0.39435613155365
1.17999994754791 -0.388819932937622
1.19000005722046 -0.382902383804321
1.20000004768372 -0.376608371734619
1.21000003814697 -0.369920969009399
1.22000002861023 -0.362843871116638
1.23000001907349 -0.35540759563446
1.24000000953674 -0.347633838653564
1.25 -0.339545249938965
1.26999998092651 -0.322505474090576
1.28999996185303 -0.304490566253662
1.30999994277954 -0.285367965698242
1.33000004291534 -0.265298843383789
1.35000002384186 -0.244558930397034
1.37999999523163 -0.212616205215454
1.45000004768372 -0.137471556663513
1.48000001907349 -0.105811476707458
1.49000000953674 -0.0954482555389404
};
\addplot [ultra thick, blue]
table {%
0 0.1720130443573
0.0199999809265137 0.164616465568542
0.0399999618530273 0.157625555992126
0.059999942779541 0.151007175445557
0.0900000333786011 0.141676068305969
0.120000004768372 0.13288426399231
0.220000028610229 0.104301571846008
0.240000009536743 0.0980798006057739
0.259999990463257 0.0914738178253174
0.279999971389771 0.0843764543533325
0.299999952316284 0.0766818523406982
0.319999933242798 0.0683176517486572
0.340000033378601 0.0592365264892578
0.360000014305115 0.0494033098220825
0.379999995231628 0.0387929677963257
0.399999976158142 0.0273805856704712
0.419999957084656 0.0151405334472656
0.440000057220459 0.00205683708190918
0.460000038146973 -0.0118739604949951
0.480000019073486 -0.0266444683074951
0.5 -0.0422395467758179
0.519999980926514 -0.0586323738098145
0.539999961853027 -0.0757832527160645
0.559999942779541 -0.0936392545700073
0.579999923706055 -0.112123131752014
0.600000023841858 -0.131140828132629
0.629999995231628 -0.160446524620056
0.670000076293945 -0.200391054153442
0.720000028610229 -0.250332117080688
0.75 -0.279478430747986
0.769999980926514 -0.298266410827637
0.789999961853027 -0.316368699073792
0.809999942779541 -0.333640217781067
0.829999923706055 -0.349937677383423
0.839999914169312 -0.357677817344666
0.850000023841858 -0.36512303352356
0.860000014305115 -0.372257471084595
0.870000004768372 -0.379065155982971
0.879999995231628 -0.385531425476074
0.889999985694885 -0.391642093658447
0.899999976158142 -0.397383689880371
0.910000085830688 -0.402743935585022
0.920000076293945 -0.407710790634155
0.930000066757202 -0.412273287773132
0.940000057220459 -0.416421413421631
0.950000047683716 -0.420145988464355
0.960000038146973 -0.423438549041748
0.970000028610229 -0.426291584968567
0.980000019073486 -0.428698301315308
0.990000009536743 -0.430652856826782
1 -0.432150363922119
1.00999999046326 -0.433187007904053
1.01999998092651 -0.433759450912476
1.02999997138977 -0.433865785598755
1.03999996185303 -0.433504462242126
1.04999995231628 -0.432675361633301
1.05999994277954 -0.431378841400146
1.07000005245209 -0.429616570472717
1.08000004291534 -0.427390813827515
1.0900000333786 -0.424704909324646
1.10000002384186 -0.421563148498535
1.11000001430511 -0.417970418930054
1.12000000476837 -0.41393256187439
1.12999999523163 -0.409456729888916
1.13999998569489 -0.404550790786743
1.14999997615814 -0.399223446846008
1.1599999666214 -0.393484354019165
1.16999995708466 -0.387344121932983
1.17999994754791 -0.38081419467926
1.19000005722046 -0.373906970024109
1.20000004768372 -0.366635799407959
1.21000003814697 -0.359014987945557
1.22000002861023 -0.351059913635254
1.23000001907349 -0.342786312103271
1.25 -0.325348854064941
1.26999998092651 -0.306840419769287
1.28999996185303 -0.287407159805298
1.30999994277954 -0.267201781272888
1.33000004291534 -0.246385812759399
1.36000001430511 -0.214376449584961
1.44000005722046 -0.128136396408081
1.47000002861023 -0.0968406200408936
1.49000000953674 -0.0766401290893555
};
\addplot [ultra thick, color0]
table {%
0 0.1720130443573
0.0199999809265137 0.164611101150513
0.0399999618530273 0.157597064971924
0.059999942779541 0.15094780921936
0.0900000333786011 0.141585350036621
0.120000004768372 0.13282299041748
0.159999966621399 0.121732950210571
0.210000038146973 0.107975602149963
0.240000009536743 0.0992509126663208
0.259999990463257 0.0930432081222534
0.279999971389771 0.0864084959030151
0.299999952316284 0.0792520046234131
0.319999933242798 0.071486234664917
0.340000033378601 0.0630265474319458
0.360000014305115 0.0537991523742676
0.379999995231628 0.0437474250793457
0.399999976158142 0.0328261852264404
0.419999957084656 0.0209991931915283
0.440000057220459 0.00824284553527832
0.460000038146973 -0.00544953346252441
0.480000019073486 -0.0200598239898682
0.5 -0.0355559587478638
0.519999980926514 -0.0519064664840698
0.539999961853027 -0.0690622329711914
0.559999942779541 -0.0869650840759277
0.579999923706055 -0.105541110038757
0.600000023841858 -0.12470531463623
0.629999995231628 -0.154332756996155
0.670000076293945 -0.194864273071289
0.720000028610229 -0.245650291442871
0.75 -0.275291323661804
0.769999980926514 -0.294384717941284
0.789999961853027 -0.31276798248291
0.809999942779541 -0.330294370651245
0.829999923706055 -0.346823811531067
0.839999914169312 -0.354672908782959
0.850000023841858 -0.362223744392395
0.860000014305115 -0.369460940361023
0.870000004768372 -0.376369833946228
0.879999995231628 -0.382936477661133
0.889999985694885 -0.389147758483887
0.899999976158142 -0.394991278648376
0.910000085830688 -0.400455474853516
0.920000076293945 -0.405529618263245
0.930000066757202 -0.410203456878662
0.940000057220459 -0.414467573165894
0.950000047683716 -0.41831374168396
0.960000038146973 -0.421733856201172
0.970000028610229 -0.424721121788025
0.980000019073486 -0.427269220352173
0.990000009536743 -0.429372549057007
1 -0.431026697158813
1.00999999046326 -0.432227492332458
1.01999998092651 -0.432971954345703
1.02999997138977 -0.433257937431335
1.03999996185303 -0.433083772659302
1.04999995231628 -0.432448506355286
1.05999994277954 -0.431352019309998
1.07000005245209 -0.429794549942017
1.08000004291534 -0.427777528762817
1.0900000333786 -0.425302624702454
1.10000002384186 -0.422372817993164
1.11000001430511 -0.418991684913635
1.12000000476837 -0.41516387462616
1.12999999523163 -0.410894632339478
1.13999998569489 -0.406190037727356
1.14999997615814 -0.401057124137878
1.1599999666214 -0.395503878593445
1.16999995708466 -0.389539241790771
1.17999994754791 -0.383172631263733
1.19000005722046 -0.376414179801941
1.20000004768372 -0.369274973869324
1.21000003814697 -0.361766576766968
1.22000002861023 -0.353901267051697
1.23000001907349 -0.345692157745361
1.24000000953674 -0.337153077125549
1.25999999046326 -0.31914484500885
1.27999997138977 -0.300002336502075
1.29999995231628 -0.279862642288208
1.32000005245209 -0.258875370025635
1.3400000333786 -0.23720121383667
1.37000000476837 -0.203770041465759
1.46000003814697 -0.102187395095825
1.48000001907349 -0.0803723335266113
1.49000000953674 -0.0696748495101929
};


==> supp_mat/fetch_plots/constraint_loss_data.tex <==
\path [fill=color0, fill opacity=0.4, ultra thick]
(axis cs:0,237.925003051758)
--(axis cs:0,211.867477416992)
--(axis cs:100,261.10009765625)
--(axis cs:200,262.886291503906)
--(axis cs:300,264.170318603516)
--(axis cs:400,250.576416015625)
--(axis cs:500,42.0327339172363)
--(axis cs:600,8.49201679229736)
--(axis cs:700,6.70053720474243)
--(axis cs:800,5.01216506958008)
--(axis cs:900,5.6209602355957)
--(axis cs:1000,1.58914947509766)
--(axis cs:1100,2.20554208755493)
--(axis cs:1200,7.27553176879883)
--(axis cs:1300,18.8865242004395)
--(axis cs:1400,24.5383987426758)
--(axis cs:1500,25.6514453887939)
--(axis cs:1600,27.448802947998)
--(axis cs:1700,27.9536628723145)
--(axis cs:1800,36.5069351196289)
--(axis cs:1900,40.7017097473145)
--(axis cs:2000,51.571533203125)
--(axis cs:2100,57.1563720703125)
--(axis cs:2200,55.919921875)
--(axis cs:2300,49.2231636047363)
--(axis cs:2400,50.0492973327637)
--(axis cs:2500,49.9380569458008)
--(axis cs:2600,74.3858108520508)
--(axis cs:2700,95.0464477539062)
--(axis cs:2800,120.612426757812)
--(axis cs:2900,142.361602783203)
--(axis cs:3000,153.484115600586)
--(axis cs:3100,128.602340698242)
--(axis cs:3200,127.2255859375)
--(axis cs:3300,116.761131286621)
--(axis cs:3400,114.569725036621)
--(axis cs:3500,139.926849365234)
--(axis cs:3600,139.1123046875)
--(axis cs:3700,152.905471801758)
--(axis cs:3800,173.743255615234)
--(axis cs:3900,173.795211791992)
--(axis cs:4000,196.888641357422)
--(axis cs:4100,200.711715698242)
--(axis cs:4200,209.338851928711)
--(axis cs:4300,192.587890625)
--(axis cs:4400,196.642456054688)
--(axis cs:4500,201.365905761719)
--(axis cs:4600,235.114715576172)
--(axis cs:4700,267.549224853516)
--(axis cs:4800,287.324890136719)
--(axis cs:4900,305.640167236328)
--(axis cs:5000,286.992828369141)
--(axis cs:5100,279.767883300781)
--(axis cs:5200,266.716400146484)
--(axis cs:5300,279.102081298828)
--(axis cs:5400,269.178314208984)
--(axis cs:5500,268.493011474609)
--(axis cs:5600,296.209136962891)
--(axis cs:5700,270.897277832031)
--(axis cs:5800,253.700988769531)
--(axis cs:5900,245.279434204102)
--(axis cs:6000,244.083770751953)
--(axis cs:6100,250.990478515625)
--(axis cs:6200,267.476318359375)
--(axis cs:6300,289.775970458984)
--(axis cs:6400,320.691009521484)
--(axis cs:6500,367.428771972656)
--(axis cs:6600,371.674072265625)
--(axis cs:6700,380.967041015625)
--(axis cs:6800,390.760345458984)
--(axis cs:6900,384.492889404297)
--(axis cs:7000,377.940002441406)
--(axis cs:7100,380.7158203125)
--(axis cs:7200,357.402374267578)
--(axis cs:7300,348.420562744141)
--(axis cs:7400,338.81591796875)
--(axis cs:7500,347.926788330078)
--(axis cs:7600,349.229766845703)
--(axis cs:7700,351.05419921875)
--(axis cs:7800,373.931243896484)
--(axis cs:7900,339.962554931641)
--(axis cs:8000,301.172424316406)
--(axis cs:8100,286.989044189453)
--(axis cs:8200,266.140869140625)
--(axis cs:8300,249.476959228516)
--(axis cs:8400,241.918914794922)
--(axis cs:8500,243.216400146484)
--(axis cs:8600,227.677200317383)
--(axis cs:8700,240.705856323242)
--(axis cs:8800,232.158203125)
--(axis cs:8900,250.845336914062)
--(axis cs:9000,251.595260620117)
--(axis cs:9100,252.255874633789)
--(axis cs:9200,254.892929077148)
--(axis cs:9300,248.598831176758)
--(axis cs:9400,265.6015625)
--(axis cs:9500,259.362609863281)
--(axis cs:9600,263.972106933594)
--(axis cs:9700,269.340667724609)
--(axis cs:9800,267.110595703125)
--(axis cs:9900,252.569519042969)
--(axis cs:10000,242.525619506836)
--(axis cs:10100,248.816482543945)
--(axis cs:10200,258.380310058594)
--(axis cs:10300,268.520355224609)
--(axis cs:10400,267.990142822266)
--(axis cs:10500,292.061828613281)
--(axis cs:10600,287.885040283203)
--(axis cs:10700,305.611541748047)
--(axis cs:10800,332.221557617188)
--(axis cs:10900,331.977416992188)
--(axis cs:11000,333.077209472656)
--(axis cs:11100,325.018371582031)
--(axis cs:11200,297.157897949219)
--(axis cs:11300,289.728485107422)
--(axis cs:11400,294.464263916016)
--(axis cs:11500,311.208190917969)
--(axis cs:11600,338.119537353516)
--(axis cs:11700,329.016662597656)
--(axis cs:11800,321.089263916016)
--(axis cs:11900,310.486999511719)
--(axis cs:12000,289.543518066406)
--(axis cs:12100,245.758865356445)
--(axis cs:12200,233.767761230469)
--(axis cs:12300,224.598876953125)
--(axis cs:12400,226.233612060547)
--(axis cs:12500,220.864166259766)
--(axis cs:12600,227.955490112305)
--(axis cs:12700,238.660308837891)
--(axis cs:12800,242.254653930664)
--(axis cs:12900,243.898971557617)
--(axis cs:13000,239.410293579102)
--(axis cs:13100,234.766128540039)
--(axis cs:13200,228.69921875)
--(axis cs:13300,246.186050415039)
--(axis cs:13400,242.430404663086)
--(axis cs:13500,250.6484375)
--(axis cs:13600,245.861877441406)
--(axis cs:13700,227.515487670898)
--(axis cs:13800,235.252349853516)
--(axis cs:13900,228.483596801758)
--(axis cs:14000,228.192962646484)
--(axis cs:14100,246.778121948242)
--(axis cs:14200,247.583587646484)
--(axis cs:14300,268.993743896484)
--(axis cs:14400,269.806060791016)
--(axis cs:14500,263.996887207031)
--(axis cs:14600,232.641876220703)
--(axis cs:14700,211.809677124023)
--(axis cs:14800,210.583709716797)
--(axis cs:14900,215.782806396484)
--(axis cs:15000,208.26513671875)
--(axis cs:15100,202.674713134766)
--(axis cs:15200,223.060623168945)
--(axis cs:15300,234.86003112793)
--(axis cs:15400,252.891403198242)
--(axis cs:15500,252.021881103516)
--(axis cs:15600,252.737503051758)
--(axis cs:15700,243.077346801758)
--(axis cs:15800,240.858596801758)
--(axis cs:15900,240.606262207031)
--(axis cs:16000,253.314056396484)
--(axis cs:16100,247.667190551758)
--(axis cs:16200,245.511352539062)
--(axis cs:16300,239.692123413086)
--(axis cs:16400,239.402252197266)
--(axis cs:16500,268.3828125)
--(axis cs:16600,259.651550292969)
--(axis cs:16700,261.959381103516)
--(axis cs:16800,289.94921875)
--(axis cs:16900,310.45654296875)
--(axis cs:17000,297.407806396484)
--(axis cs:17100,309.493011474609)
--(axis cs:17200,296.561706542969)
--(axis cs:17300,286.059387207031)
--(axis cs:17400,271.989837646484)
--(axis cs:17500,257.9140625)
--(axis cs:17600,246.754531860352)
--(axis cs:17700,246.188720703125)
--(axis cs:17800,236.026473999023)
--(axis cs:17900,227.731918334961)
--(axis cs:18000,216.261016845703)
--(axis cs:18100,204.853118896484)
--(axis cs:18200,215.9599609375)
--(axis cs:18300,231.124389648438)
--(axis cs:18400,232.56591796875)
--(axis cs:18500,261.956451416016)
--(axis cs:18600,285.498809814453)
--(axis cs:18700,305.319702148438)
--(axis cs:18800,303.158935546875)
--(axis cs:18900,285.684265136719)
--(axis cs:19000,255.546615600586)
--(axis cs:19100,246.903244018555)
--(axis cs:19200,252.369934082031)
--(axis cs:19300,282.061706542969)
--(axis cs:19400,286.267913818359)
--(axis cs:19500,286.360931396484)
--(axis cs:19600,271.086700439453)
--(axis cs:19700,238.127166748047)
--(axis cs:19800,203.004486083984)
--(axis cs:19900,194.085052490234)
--(axis cs:20000,206.0341796875)
--(axis cs:20100,211.15234375)
--(axis cs:20200,221.022659301758)
--(axis cs:20300,225.532028198242)
--(axis cs:20400,230.149993896484)
--(axis cs:20500,213.61328125)
--(axis cs:20600,216.249435424805)
--(axis cs:20700,207.887634277344)
--(axis cs:20800,210.308471679688)
--(axis cs:20900,209.821426391602)
--(axis cs:21000,222.740509033203)
--(axis cs:21100,237.649780273438)
--(axis cs:21200,254.386932373047)
--(axis cs:21300,258.989898681641)
--(axis cs:21400,255.463623046875)
--(axis cs:21500,239.509536743164)
--(axis cs:21600,235.169494628906)
--(axis cs:21700,237.678115844727)
--(axis cs:21800,246.940628051758)
--(axis cs:21900,243.8486328125)
--(axis cs:22000,259.929412841797)
--(axis cs:22100,274.756469726562)
--(axis cs:22200,265.448913574219)
--(axis cs:22300,250.444488525391)
--(axis cs:22400,251.248199462891)
--(axis cs:22500,250.243957519531)
--(axis cs:22600,237.177780151367)
--(axis cs:22700,247.9453125)
--(axis cs:22800,252.951370239258)
--(axis cs:22900,260.182800292969)
--(axis cs:23000,258.938201904297)
--(axis cs:23100,257.724700927734)
--(axis cs:23200,263.081573486328)
--(axis cs:23300,266.703857421875)
--(axis cs:23400,263.668273925781)
--(axis cs:23500,261.455932617188)
--(axis cs:23600,284.378601074219)
--(axis cs:23700,285.6875)
--(axis cs:23800,285.6875)
--(axis cs:23900,285.6875)
--(axis cs:24000,285.6875)
--(axis cs:24100,285.6875)
--(axis cs:24200,285.932098388672)
--(axis cs:24300,285.873718261719)
--(axis cs:24400,285.6875)
--(axis cs:24500,285.769714355469)
--(axis cs:24600,285.6875)
--(axis cs:24700,285.6875)
--(axis cs:24800,285.6875)
--(axis cs:24900,285.6875)
--(axis cs:25000,285.6875)
--(axis cs:25100,285.6875)
--(axis cs:25200,285.6875)
--(axis cs:25300,285.6875)
--(axis cs:25400,285.6875)
--(axis cs:25500,285.6875)
--(axis cs:25600,285.6875)
--(axis cs:25700,285.6875)
--(axis cs:25800,285.6875)
--(axis cs:25900,285.6875)
--(axis cs:26000,285.6875)
--(axis cs:26100,285.6875)
--(axis cs:26200,285.6875)
--(axis cs:26300,285.6875)
--(axis cs:26400,285.6875)
--(axis cs:26500,285.6875)
--(axis cs:26600,285.6875)
--(axis cs:26700,285.6875)
--(axis cs:26800,274.797149658203)
--(axis cs:26900,269.342041015625)
--(axis cs:27000,268.369934082031)
--(axis cs:27100,272.777191162109)
--(axis cs:27200,285.6875)
--(axis cs:27300,285.6875)
--(axis cs:27400,285.6875)
--(axis cs:27500,285.6875)
--(axis cs:27600,285.6875)
--(axis cs:27700,285.6875)
--(axis cs:27800,285.6875)
--(axis cs:27900,285.6875)
--(axis cs:28000,285.6875)
--(axis cs:28100,285.6875)
--(axis cs:28200,285.6875)
--(axis cs:28300,285.6875)
--(axis cs:28400,285.6875)
--(axis cs:28500,285.6875)
--(axis cs:28600,285.6875)
--(axis cs:28700,285.6875)
--(axis cs:28800,285.6875)
--(axis cs:28900,285.6875)
--(axis cs:29000,285.6875)
--(axis cs:29100,285.6875)
--(axis cs:29200,285.6875)
--(axis cs:29300,285.6875)
--(axis cs:29400,285.6875)
--(axis cs:29500,285.6875)
--(axis cs:29600,285.6875)
--(axis cs:29700,285.6875)
--(axis cs:29800,285.6875)
--(axis cs:29900,285.6875)
--(axis cs:30000,285.6875)
--(axis cs:30100,285.6875)
--(axis cs:30200,285.6875)
--(axis cs:30300,285.6875)
--(axis cs:30400,285.6875)
--(axis cs:30500,285.6875)
--(axis cs:30600,285.6875)
--(axis cs:30700,285.6875)
--(axis cs:30800,285.6875)
--(axis cs:30900,285.6875)
--(axis cs:31000,285.6875)
--(axis cs:31100,285.6875)
--(axis cs:31200,285.6875)
--(axis cs:31300,285.6875)
--(axis cs:31400,285.6875)
--(axis cs:31500,285.6875)
--(axis cs:31600,285.6875)
--(axis cs:31700,285.6875)
--(axis cs:31800,285.6875)
--(axis cs:31900,285.6875)
--(axis cs:32000,285.6875)
--(axis cs:32100,285.6875)
--(axis cs:32200,285.6875)
--(axis cs:32300,285.6875)
--(axis cs:32400,285.6875)
--(axis cs:32500,285.6875)
--(axis cs:32600,285.6875)
--(axis cs:32700,285.6875)
--(axis cs:32800,285.6875)
--(axis cs:32900,285.6875)
--(axis cs:33000,285.6875)
--(axis cs:33100,285.6875)
--(axis cs:33200,285.6875)
--(axis cs:33300,285.6875)
--(axis cs:33400,285.6875)
--(axis cs:33500,285.6875)
--(axis cs:33600,285.6875)
--(axis cs:33700,285.6875)
--(axis cs:33800,285.6875)
--(axis cs:33900,285.6875)
--(axis cs:34000,285.6875)
--(axis cs:34100,285.6875)
--(axis cs:34200,285.6875)
--(axis cs:34300,285.6875)
--(axis cs:34300,423.303894042969)
--(axis cs:34300,423.303894042969)
--(axis cs:34200,426.1103515625)
--(axis cs:34100,447.194183349609)
--(axis cs:34000,454.480743408203)
--(axis cs:33900,453.176849365234)
--(axis cs:33800,449.891296386719)
--(axis cs:33700,440.137725830078)
--(axis cs:33600,417.440765380859)
--(axis cs:33500,400.848449707031)
--(axis cs:33400,403.414764404297)
--(axis cs:33300,397.858459472656)
--(axis cs:33200,402.381195068359)
--(axis cs:33100,395.231811523438)
--(axis cs:33000,418.085815429688)
--(axis cs:32900,426.741577148438)
--(axis cs:32800,443.639556884766)
--(axis cs:32700,447.576416015625)
--(axis cs:32600,451.904357910156)
--(axis cs:32500,428.763458251953)
--(axis cs:32400,411.598968505859)
--(axis cs:32300,385.782745361328)
--(axis cs:32200,380.465362548828)
--(axis cs:32100,372.159301757812)
--(axis cs:32000,376.937255859375)
--(axis cs:31900,390.487762451172)
--(axis cs:31800,393.432495117188)
--(axis cs:31700,393.844909667969)
--(axis cs:31600,406.589630126953)
--(axis cs:31500,415.806213378906)
--(axis cs:31400,407.352844238281)
--(axis cs:31300,409.271606445312)
--(axis cs:31200,400.725250244141)
--(axis cs:31100,378.241119384766)
--(axis cs:31000,362.846252441406)
--(axis cs:30900,374.049133300781)
--(axis cs:30800,385.992706298828)
--(axis cs:30700,388.165405273438)
--(axis cs:30600,407.340270996094)
--(axis cs:30500,405.955902099609)
--(axis cs:30400,420.927459716797)
--(axis cs:30300,420.116455078125)
--(axis cs:30200,421.469421386719)
--(axis cs:30100,405.439147949219)
--(axis cs:30000,395.42041015625)
--(axis cs:29900,360.395690917969)
--(axis cs:29800,341.53125)
--(axis cs:29700,336.831695556641)
--(axis cs:29600,324.767852783203)
--(axis cs:29500,317.884307861328)
--(axis cs:29400,314.407745361328)
--(axis cs:29300,314.092254638672)
--(axis cs:29200,308.791564941406)
--(axis cs:29100,325.811248779297)
--(axis cs:29000,349.921081542969)
--(axis cs:28900,380.364807128906)
--(axis cs:28800,384.231170654297)
--(axis cs:28700,400.120452880859)
--(axis cs:28600,421.600158691406)
--(axis cs:28500,426.593231201172)
--(axis cs:28400,399.029052734375)
--(axis cs:28300,403.903839111328)
--(axis cs:28200,394.860870361328)
--(axis cs:28100,372.686157226562)
--(axis cs:28000,346.086364746094)
--(axis cs:27900,344.776275634766)
--(axis cs:27800,346.005859375)
--(axis cs:27700,341.035919189453)
--(axis cs:27600,344.290985107422)
--(axis cs:27500,336.118835449219)
--(axis cs:27400,329.934692382812)
--(axis cs:27300,313.548065185547)
--(axis cs:27200,300.628784179688)
--(axis cs:27100,287.2578125)
--(axis cs:27000,287.2578125)
--(axis cs:26900,287.2578125)
--(axis cs:26800,287.2578125)
--(axis cs:26700,295.732971191406)
--(axis cs:26600,321.601257324219)
--(axis cs:26500,340.592132568359)
--(axis cs:26400,338.689880371094)
--(axis cs:26300,340.038909912109)
--(axis cs:26200,335.466339111328)
--(axis cs:26100,315.330261230469)
--(axis cs:26000,302.696563720703)
--(axis cs:25900,306.469696044922)
--(axis cs:25800,309.546752929688)
--(axis cs:25700,310.959197998047)
--(axis cs:25600,325.657867431641)
--(axis cs:25500,342.846374511719)
--(axis cs:25400,345.069213867188)
--(axis cs:25300,349.711120605469)
--(axis cs:25200,347.238037109375)
--(axis cs:25100,361.294708251953)
--(axis cs:25000,358.025665283203)
--(axis cs:24900,343.165710449219)
--(axis cs:24800,328.155792236328)
--(axis cs:24700,321.509490966797)
--(axis cs:24600,300.238403320312)
--(axis cs:24500,290.101135253906)
--(axis cs:24400,298.841796875)
--(axis cs:24300,289.376831054688)
--(axis cs:24200,288.927276611328)
--(axis cs:24100,292.501098632812)
--(axis cs:24000,307.531951904297)
--(axis cs:23900,300.203918457031)
--(axis cs:23800,302.109527587891)
--(axis cs:23700,298.977294921875)
--(axis cs:23600,286.972961425781)
--(axis cs:23500,287.259368896484)
--(axis cs:23400,287.260162353516)
--(axis cs:23300,287.260925292969)
--(axis cs:23200,287.26171875)
--(axis cs:23100,287.26171875)
--(axis cs:23000,284.798797607422)
--(axis cs:22900,282.794311523438)
--(axis cs:22800,285.949157714844)
--(axis cs:22700,287.26171875)
--(axis cs:22600,302.432037353516)
--(axis cs:22500,314.482055664062)
--(axis cs:22400,321.604400634766)
--(axis cs:22300,325.252960205078)
--(axis cs:22200,319.682037353516)
--(axis cs:22100,334.602355957031)
--(axis cs:22000,332.938323974609)
--(axis cs:21900,316.407043457031)
--(axis cs:21800,312.165740966797)
--(axis cs:21700,287.209899902344)
--(axis cs:21600,265.375)
--(axis cs:21500,275.420166015625)
--(axis cs:21400,273.435150146484)
--(axis cs:21300,266.299163818359)
--(axis cs:21200,281.853912353516)
--(axis cs:21100,287.825775146484)
--(axis cs:21000,297.366394042969)
--(axis cs:20900,306.028900146484)
--(axis cs:20800,301.384368896484)
--(axis cs:20700,287.578918457031)
--(axis cs:20600,293.21826171875)
--(axis cs:20500,279.391326904297)
--(axis cs:20400,273.23193359375)
--(axis cs:20300,271.995758056641)
--(axis cs:20200,279.98583984375)
--(axis cs:20100,282.037780761719)
--(axis cs:20000,290.362152099609)
--(axis cs:19900,297.908142089844)
--(axis cs:19800,321.540863037109)
--(axis cs:19700,312.855682373047)
--(axis cs:19600,322.525299072266)
--(axis cs:19500,329.427642822266)
--(axis cs:19400,330.453460693359)
--(axis cs:19300,318.516967773438)
--(axis cs:19200,322.565490722656)
--(axis cs:19100,326.964996337891)
--(axis cs:19000,319.727355957031)
--(axis cs:18900,338.8359375)
--(axis cs:18800,321.98583984375)
--(axis cs:18700,324.135162353516)
--(axis cs:18600,319.84765625)
--(axis cs:18500,322.227355957031)
--(axis cs:18400,328.284118652344)
--(axis cs:18300,307.211547851562)
--(axis cs:18200,295.89892578125)
--(axis cs:18100,297.737945556641)
--(axis cs:18000,299.992645263672)
--(axis cs:17900,294.327453613281)
--(axis cs:17800,304.335021972656)
--(axis cs:17700,331.684753417969)
--(axis cs:17600,349.946472167969)
--(axis cs:17500,333.514007568359)
--(axis cs:17400,323.348358154297)
--(axis cs:17300,332.954315185547)
--(axis cs:17200,331.974945068359)
--(axis cs:17100,318.535125732422)
--(axis cs:17000,317.773529052734)
--(axis cs:16900,332.32421875)
--(axis cs:16800,346.114471435547)
--(axis cs:16700,351.121490478516)
--(axis cs:16600,338.334228515625)
--(axis cs:16500,336.270812988281)
--(axis cs:16400,320.193572998047)
--(axis cs:16300,299.598480224609)
--(axis cs:16200,298.365783691406)
--(axis cs:16100,300.647644042969)
--(axis cs:16000,287.111328125)
--(axis cs:15900,279.617980957031)
--(axis cs:15800,289.385467529297)
--(axis cs:15700,282.564117431641)
--(axis cs:15600,302.230926513672)
--(axis cs:15500,310.106811523438)
--(axis cs:15400,305.464324951172)
--(axis cs:15300,290.171722412109)
--(axis cs:15200,276.847198486328)
--(axis cs:15100,255.845306396484)
--(axis cs:15000,243.896331787109)
--(axis cs:14900,261.492706298828)
--(axis cs:14800,295.735534667969)
--(axis cs:14700,320.909606933594)
--(axis cs:14600,326.273223876953)
--(axis cs:14500,316.463134765625)
--(axis cs:14400,302.500762939453)
--(axis cs:14300,306.286071777344)
--(axis cs:14200,333.935791015625)
--(axis cs:14100,340.712005615234)
--(axis cs:14000,336.438293457031)
--(axis cs:13900,331.115356445312)
--(axis cs:13800,321.774047851562)
--(axis cs:13700,313.203247070312)
--(axis cs:13600,295.786560058594)
--(axis cs:13500,273.373565673828)
--(axis cs:13400,265.134704589844)
--(axis cs:13300,249.544525146484)
--(axis cs:13200,255.209487915039)
--(axis cs:13100,259.443237304688)
--(axis cs:13000,270.556243896484)
--(axis cs:12900,293.8828125)
--(axis cs:12800,299.880859375)
--(axis cs:12700,326.412506103516)
--(axis cs:12600,318.673828125)
--(axis cs:12500,324.419525146484)
--(axis cs:12400,321.278900146484)
--(axis cs:12300,338.112884521484)
--(axis cs:12200,322.028076171875)
--(axis cs:12100,339.405975341797)
--(axis cs:12000,333.503356933594)
--(axis cs:11900,355.829895019531)
--(axis cs:11800,355.744140625)
--(axis cs:11700,380.437744140625)
--(axis cs:11600,361.261627197266)
--(axis cs:11500,358.161529541016)
--(axis cs:11400,350.674835205078)
--(axis cs:11300,356.474395751953)
--(axis cs:11200,348.189453125)
--(axis cs:11100,350.110931396484)
--(axis cs:11000,352.801696777344)
--(axis cs:10900,352.771484375)
--(axis cs:10800,344.261779785156)
--(axis cs:10700,364.205871582031)
--(axis cs:10600,401.819366455078)
--(axis cs:10500,444.548034667969)
--(axis cs:10400,461.614074707031)
--(axis cs:10300,474.380859375)
--(axis cs:10200,522.602355957031)
--(axis cs:10100,534.526245117188)
--(axis cs:10000,492.624206542969)
--(axis cs:9900,468.660949707031)
--(axis cs:9800,460.585144042969)
--(axis cs:9700,383.435943603516)
--(axis cs:9600,361.928527832031)
--(axis cs:9500,327.735168457031)
--(axis cs:9400,325.326568603516)
--(axis cs:9300,301.502502441406)
--(axis cs:9200,312.359161376953)
--(axis cs:9100,318.175964355469)
--(axis cs:9000,312.702911376953)
--(axis cs:8900,297.044006347656)
--(axis cs:8800,297.390197753906)
--(axis cs:8700,257.573120117188)
--(axis cs:8600,237.922271728516)
--(axis cs:8500,258.31640625)
--(axis cs:8400,287.350860595703)
--(axis cs:8300,290.197601318359)
--(axis cs:8200,333.932800292969)
--(axis cs:8100,365.895690917969)
--(axis cs:8000,381.023315429688)
--(axis cs:7900,363.215240478516)
--(axis cs:7800,388.418853759766)
--(axis cs:7700,448.563293457031)
--(axis cs:7600,502.245147705078)
--(axis cs:7500,526.680847167969)
--(axis cs:7400,533.376159667969)
--(axis cs:7300,523.060852050781)
--(axis cs:7200,509.383087158203)
--(axis cs:7100,477.540344238281)
--(axis cs:7000,497.174560546875)
--(axis cs:6900,525.52734375)
--(axis cs:6800,537.726196289062)
--(axis cs:6700,507.900207519531)
--(axis cs:6600,463.028503417969)
--(axis cs:6500,430.086059570312)
--(axis cs:6400,420.608032226562)
--(axis cs:6300,368.781890869141)
--(axis cs:6200,366.047302246094)
--(axis cs:6100,365.952545166016)
--(axis cs:6000,403.075103759766)
--(axis cs:5900,421.165222167969)
--(axis cs:5800,412.1591796875)
--(axis cs:5700,433.427124023438)
--(axis cs:5600,419.231781005859)
--(axis cs:5500,372.352722167969)
--(axis cs:5400,345.239074707031)
--(axis cs:5300,359.612609863281)
--(axis cs:5200,313.469635009766)
--(axis cs:5100,313.383087158203)
--(axis cs:5000,330.706390380859)
--(axis cs:4900,337.056304931641)
--(axis cs:4800,331.103881835938)
--(axis cs:4700,358.553955078125)
--(axis cs:4600,356.223663330078)
--(axis cs:4500,361.139068603516)
--(axis cs:4400,380.112731933594)
--(axis cs:4300,368.809509277344)
--(axis cs:4200,305.40673828125)
--(axis cs:4100,316.763366699219)
--(axis cs:4000,322.122833251953)
--(axis cs:3900,334.707702636719)
--(axis cs:3800,365.058410644531)
--(axis cs:3700,365.880920410156)
--(axis cs:3600,328.037231445312)
--(axis cs:3500,278.644287109375)
--(axis cs:3400,224.760604858398)
--(axis cs:3300,191.840270996094)
--(axis cs:3200,181.021011352539)
--(axis cs:3100,204.642532348633)
--(axis cs:3000,220.413558959961)
--(axis cs:2900,218.617645263672)
--(axis cs:2800,199.951293945312)
--(axis cs:2700,196.722106933594)
--(axis cs:2600,184.029632568359)
--(axis cs:2500,160.153564453125)
--(axis cs:2400,160.087005615234)
--(axis cs:2300,144.508728027344)
--(axis cs:2200,149.102935791016)
--(axis cs:2100,123.597869873047)
--(axis cs:2000,113.937240600586)
--(axis cs:1900,99.9110794067383)
--(axis cs:1800,93.7909088134766)
--(axis cs:1700,79.0804672241211)
--(axis cs:1600,73.0702285766602)
--(axis cs:1500,70.9086151123047)
--(axis cs:1400,94.2665328979492)
--(axis cs:1300,90.9848937988281)
--(axis cs:1200,100.095748901367)
--(axis cs:1100,104.388732910156)
--(axis cs:1000,96.9970092773438)
--(axis cs:900,62.9253273010254)
--(axis cs:800,60.1164665222168)
--(axis cs:700,56.8890686035156)
--(axis cs:600,63.3722305297852)
--(axis cs:500,100.656539916992)
--(axis cs:400,310.820098876953)
--(axis cs:300,322.988311767578)
--(axis cs:200,306.850463867188)
--(axis cs:100,286.942504882812)
--(axis cs:0,237.925003051758)
--cycle;

\path [fill=white!40.1960784313725!black, fill opacity=0.4, ultra thick]
(axis cs:0,0.00546552613377571)
--(axis cs:0,0.00483751576393843)
--(axis cs:100,0.00483698956668377)
--(axis cs:200,0.00271829543635249)
--(axis cs:300,0.000903920852579176)
--(axis cs:400,6.10426059211022e-06)
--(axis cs:500,0)
--(axis cs:600,0)
--(axis cs:700,0)
--(axis cs:800,0)
--(axis cs:900,1.67334255820606e-05)
--(axis cs:1000,8.72332602739334e-05)
--(axis cs:1100,8.72332602739334e-05)
--(axis cs:1200,0.000130596759845503)
--(axis cs:1300,0.000191313039977103)
--(axis cs:1400,0.000166424026247114)
--(axis cs:1500,0.000149114988744259)
--(axis cs:1600,0.000694442540407181)
--(axis cs:1700,0.000593376404140145)
--(axis cs:1800,0.000740136136300862)
--(axis cs:1900,0.000910972594283521)
--(axis cs:2000,0.00115554046351463)
--(axis cs:2100,0.000687542837113142)
--(axis cs:2200,0.0013356547569856)
--(axis cs:2300,0.000495161104481667)
--(axis cs:2400,0.000901719904504716)
--(axis cs:2500,0.000662741076666862)
--(axis cs:2600,0.000930432230234146)
--(axis cs:2700,0.00092057790607214)
--(axis cs:2800,0.00213234964758158)
--(axis cs:2900,0.00220429827459157)
--(axis cs:3000,0.00167833059094846)
--(axis cs:3100,0.00168134330306202)
--(axis cs:3200,0.00222564116120338)
--(axis cs:3300,0.00168862869031727)
--(axis cs:3400,0.00132358376868069)
--(axis cs:3500,0.00168128393124789)
--(axis cs:3600,0.00169371941592544)
--(axis cs:3700,0.00126785563770682)
--(axis cs:3800,0.00104487361386418)
--(axis cs:3900,0.00144222029484808)
--(axis cs:4000,0.00341570097953081)
--(axis cs:4100,0.00186446949373931)
--(axis cs:4200,0.00308691547252238)
--(axis cs:4300,0.002515465952456)
--(axis cs:4400,0.000986131140962243)
--(axis cs:4500,0.000595399062149227)
--(axis cs:4600,0.000737183494493365)
--(axis cs:4700,0.000612314732279629)
--(axis cs:4800,0.000978122581727803)
--(axis cs:4900,0.000997256487607956)
--(axis cs:5000,0.00105053244624287)
--(axis cs:5100,0.0010830641258508)
--(axis cs:5200,0.00166286085732281)
--(axis cs:5300,0.00133092363830656)
--(axis cs:5400,0.00143646053038538)
--(axis cs:5500,0.00201174290850759)
--(axis cs:5600,0.00213901605457067)
--(axis cs:5700,0.00149803597014397)
--(axis cs:5800,0.00236350880004466)
--(axis cs:5900,0.00192027376033366)
--(axis cs:6000,0.00150494265835732)
--(axis cs:6100,0.00276569416746497)
--(axis cs:6200,0.00299112359061837)
--(axis cs:6300,0.00239076768048108)
--(axis cs:6400,0.00338934501633048)
--(axis cs:6500,0.00337997521273792)
--(axis cs:6600,0.00196414301171899)
--(axis cs:6700,0.0019818632863462)
--(axis cs:6800,0.00218252534978092)
--(axis cs:6900,0.0013943666126579)
--(axis cs:7000,0.0027922778390348)
--(axis cs:7100,0.00435074558481574)
--(axis cs:7200,0.00452185655012727)
--(axis cs:7300,0.00533555448055267)
--(axis cs:7400,0.00214294088073075)
--(axis cs:7500,0.00293785729445517)
--(axis cs:7600,0.00284295971505344)
--(axis cs:7700,0.00272319605574012)
--(axis cs:7800,0.00262545933946967)
--(axis cs:7900,0.0018497024429962)
--(axis cs:8000,0.00130684673786163)
--(axis cs:8100,0.00141834549140185)
--(axis cs:8200,0.00184761837590486)
--(axis cs:8300,0.00211975281126797)
--(axis cs:8400,0.00209931377321482)
--(axis cs:8500,0.00178852677345276)
--(axis cs:8600,0.00241603259928524)
--(axis cs:8700,0.00189135072287172)
--(axis cs:8800,0.00188021757639945)
--(axis cs:8900,0.00384205020964146)
--(axis cs:9000,0.00416135555133224)
--(axis cs:9100,0.00387640669941902)
--(axis cs:9200,0.00507509708404541)
--(axis cs:9300,0.0036198329180479)
--(axis cs:9400,0.00233557214960456)
--(axis cs:9500,0.00245482753962278)
--(axis cs:9600,0.00192187773063779)
--(axis cs:9700,0.00183289649430662)
--(axis cs:9800,0.00195123453158885)
--(axis cs:9900,0.00113551015965641)
--(axis cs:10000,0.00103186967317015)
--(axis cs:10100,0.00237001175992191)
--(axis cs:10200,0.00203695590607822)
--(axis cs:10300,0.00358482031151652)
--(axis cs:10400,0.00296826963312924)
--(axis cs:10500,0.00314995343796909)
--(axis cs:10600,0.00276533956639469)
--(axis cs:10700,0.0026103975251317)
--(axis cs:10800,0.00124095077626407)
--(axis cs:10900,0.000994336558505893)
--(axis cs:11000,0.00172268750611693)
--(axis cs:11100,0.00222566118463874)
--(axis cs:11200,0.00243891472928226)
--(axis cs:11300,0.00285938964225352)
--(axis cs:11400,0.00296008097939193)
--(axis cs:11500,0.00243562995456159)
--(axis cs:11600,0.00163811119273305)
--(axis cs:11700,0.00220730691216886)
--(axis cs:11800,0.00183904636651278)
--(axis cs:11900,0.0022596896160394)
--(axis cs:12000,0.00233743595890701)
--(axis cs:12100,0.00299625401385128)
--(axis cs:12200,0.00432268995791674)
--(axis cs:12300,0.00276877102442086)
--(axis cs:12400,0.00276521313935518)
--(axis cs:12500,0.00378331495448947)
--(axis cs:12600,0.00338948960416019)
--(axis cs:12700,0.00293023604899645)
--(axis cs:12800,0.00308385118842125)
--(axis cs:12900,0.00309920916333795)
--(axis cs:13000,0.00258896639570594)
--(axis cs:13100,0.00249582529067993)
--(axis cs:13200,0.00244441628456116)
--(axis cs:13300,0.0023071407340467)
--(axis cs:13400,0.00345491315238178)
--(axis cs:13500,0.00344536988995969)
--(axis cs:13600,0.00355582241900265)
--(axis cs:13700,0.00340813770890236)
--(axis cs:13800,0.00353825464844704)
--(axis cs:13900,0.00303652859292924)
--(axis cs:14000,0.0030118846334517)
--(axis cs:14100,0.00288993725553155)
--(axis cs:14200,0.00419694511219859)
--(axis cs:14300,0.00325419893488288)
--(axis cs:14400,0.00293771037831903)
--(axis cs:14500,0.00266131572425365)
--(axis cs:14600,0.00294919102452695)
--(axis cs:14700,0.00174391525797546)
--(axis cs:14800,0.00249302503652871)
--(axis cs:14900,0.00234586698934436)
--(axis cs:15000,0.00203636894002557)
--(axis cs:15100,0.00197851657867432)
--(axis cs:15200,0.00426848279312253)
--(axis cs:15300,0.00371221313253045)
--(axis cs:15400,0.0042867548763752)
--(axis cs:15500,0.00355703826062381)
--(axis cs:15600,0.0035890459548682)
--(axis cs:15700,0.00240503158420324)
--(axis cs:15800,0.00283912662416697)
--(axis cs:15900,0.00273391371592879)
--(axis cs:16000,0.00262057385407388)
--(axis cs:16100,0.00256977090612054)
--(axis cs:16200,0.0023155331145972)
--(axis cs:16300,0.00133770704269409)
--(axis cs:16400,0.00251871347427368)
--(axis cs:16500,0.00263789901509881)
--(axis cs:16600,0.00264016096480191)
--(axis cs:16700,0.00350009673275054)
--(axis cs:16800,0.00352751603350043)
--(axis cs:16900,0.00253958068788052)
--(axis cs:17000,0.00244067911989987)
--(axis cs:17100,0.00252106273546815)
--(axis cs:17200,0.00220823707059026)
--(axis cs:17300,0.00235371547751129)
--(axis cs:17400,0.00304657546803355)
--(axis cs:17500,0.00237484718672931)
--(axis cs:17600,0.00309207942336798)
--(axis cs:17700,0.00294109573587775)
--(axis cs:17800,0.00393783301115036)
--(axis cs:17900,0.00330180791206658)
--(axis cs:18000,0.00333225727081299)
--(axis cs:18100,0.00196844339370728)
--(axis cs:18200,0.00179911847226322)
--(axis cs:18300,0.00223048916086555)
--(axis cs:18400,0.00258115539327264)
--(axis cs:18500,0.00278441328555346)
--(axis cs:18600,0.00270497403107584)
--(axis cs:18700,0.00227294093929231)
--(axis cs:18800,0.0031800998840481)
--(axis cs:18900,0.00359323644079268)
--(axis cs:19000,0.00362445856444538)
--(axis cs:19100,0.00341089186258614)
--(axis cs:19200,0.00401407293975353)
--(axis cs:19300,0.00493527669459581)
--(axis cs:19400,0.00239985249936581)
--(axis cs:19500,0.00246105180121958)
--(axis cs:19600,0.00270561757497489)
--(axis cs:19700,0.00278289546258748)
--(axis cs:19800,0.00273652328178287)
--(axis cs:19900,0.00338268000632524)
--(axis cs:20000,0.00305422442033887)
--(axis cs:20100,0.00426567438989878)
--(axis cs:20200,0.00390973314642906)
--(axis cs:20300,0.0044286185875535)
--(axis cs:20400,0.00576056260615587)
--(axis cs:20500,0.00591312628239393)
--(axis cs:20600,0.00502048386260867)
--(axis cs:20700,0.00496227154508233)
--(axis cs:20800,0.00416136672720313)
--(axis cs:20900,0.00327011034823954)
--(axis cs:21000,0.00346823898144066)
--(axis cs:21100,0.00350130931474268)
--(axis cs:21200,0.00474364450201392)
--(axis cs:21300,0.00519083021208644)
--(axis cs:21400,0.00467483140528202)
--(axis cs:21500,0.00501247914507985)
--(axis cs:21600,0.00463953753933311)
--(axis cs:21700,0.00341665185987949)
--(axis cs:21800,0.00322266737930477)
--(axis cs:21900,0.00306874443776906)
--(axis cs:22000,0.00245116301812232)
--(axis cs:22100,0.00254172482527792)
--(axis cs:22200,0.0025615612976253)
--(axis cs:22300,0.00225329003296793)
--(axis cs:22400,0.00237437034957111)
--(axis cs:22500,0.00276885414496064)
--(axis cs:22600,0.00316216051578522)
--(axis cs:22700,0.00391185563057661)
--(axis cs:22800,0.0043192645534873)
--(axis cs:22900,0.00515468325465918)
--(axis cs:23000,0.00535854138433933)
--(axis cs:23100,0.00508613279089332)
--(axis cs:23200,0.00438877008855343)
--(axis cs:23300,0.00392786599695683)
--(axis cs:23400,0.0036476687528193)
--(axis cs:23500,0.00331310811452568)
--(axis cs:23600,0.00459592789411545)
--(axis cs:23700,0.00440153665840626)
--(axis cs:23800,0.00555700063705444)
--(axis cs:23900,0.00501228636130691)
--(axis cs:24000,0.00479469262063503)
--(axis cs:24100,0.00347996759228408)
--(axis cs:24200,0.00362211838364601)
--(axis cs:24300,0.00509118940681219)
--(axis cs:24400,0.0051051820628345)
--(axis cs:24500,0.00565676670521498)
--(axis cs:24600,0.00599058857187629)
--(axis cs:24700,0.00592584628611803)
--(axis cs:24800,0.00345480465330184)
--(axis cs:24900,0.00403713714331388)
--(axis cs:25000,0.00415077293291688)
--(axis cs:25100,0.00442524719983339)
--(axis cs:25200,0.00480891577899456)
--(axis cs:25300,0.00457455916330218)
--(axis cs:25400,0.00417455192655325)
--(axis cs:25500,0.00359273934736848)
--(axis cs:25600,0.00308434548787773)
--(axis cs:25700,0.00300519471056759)
--(axis cs:25800,0.00407980522140861)
--(axis cs:25900,0.00405621435493231)
--(axis cs:26000,0.00423480663448572)
--(axis cs:26100,0.00418767239898443)
--(axis cs:26200,0.00416082050651312)
--(axis cs:26300,0.00323889055289328)
--(axis cs:26400,0.0030115032568574)
--(axis cs:26500,0.00272920029237866)
--(axis cs:26600,0.00368376052938402)
--(axis cs:26700,0.00373112084344029)
--(axis cs:26800,0.00444256421178579)
--(axis cs:26900,0.00435787718743086)
--(axis cs:27000,0.00463553983718157)
--(axis cs:27100,0.00424590660259128)
--(axis cs:27200,0.00462279887869954)
--(axis cs:27300,0.00447339378297329)
--(axis cs:27400,0.00480052269995213)
--(axis cs:27500,0.00465881079435349)
--(axis cs:27600,0.00447263568639755)
--(axis cs:27700,0.00361617328599095)
--(axis cs:27800,0.00284483167342842)
--(axis cs:27900,0.00326508423313498)
--(axis cs:28000,0.00357314571738243)
--(axis cs:28100,0.00316453236155212)
--(axis cs:28100,0.00972661748528481)
--(axis cs:28100,0.00972661748528481)
--(axis cs:28000,0.00967986043542624)
--(axis cs:27900,0.00971476547420025)
--(axis cs:27800,0.00976560357958078)
--(axis cs:27700,0.0096751693636179)
--(axis cs:27600,0.00959421973675489)
--(axis cs:27500,0.00958068296313286)
--(axis cs:27400,0.00957168359309435)
--(axis cs:27300,0.00959416013211012)
--(axis cs:27200,0.00958315655589104)
--(axis cs:27100,0.00961296819150448)
--(axis cs:27000,0.0095822736620903)
--(axis cs:26900,0.00960342213511467)
--(axis cs:26800,0.0095965713262558)
--(axis cs:26700,0.00966288521885872)
--(axis cs:26600,0.00966790225356817)
--(axis cs:26500,0.0097801461815834)
--(axis cs:26400,0.009745042771101)
--(axis cs:26300,0.00971783231943846)
--(axis cs:26200,0.00962056778371334)
--(axis cs:26100,0.00961813796311617)
--(axis cs:26000,0.00961394235491753)
--(axis cs:25900,0.00963029079139233)
--(axis cs:25800,0.00962806306779385)
--(axis cs:25700,0.00974581204354763)
--(axis cs:25600,0.00973621569573879)
--(axis cs:25500,0.00967771746218204)
--(axis cs:25400,0.00961932167410851)
--(axis cs:25300,0.00958658382296562)
--(axis cs:25200,0.00957118906080723)
--(axis cs:25100,0.00959794502705336)
--(axis cs:25000,0.00962148420512676)
--(axis cs:24900,0.0096321078017354)
--(axis cs:24800,0.00969300325959921)
--(axis cs:24700,0.00955609232187271)
--(axis cs:24600,0.00955805368721485)
--(axis cs:24500,0.00955090299248695)
--(axis cs:24400,0.00955691747367382)
--(axis cs:24300,0.00955743901431561)
--(axis cs:24200,0.00967452581971884)
--(axis cs:24100,0.0096901785582304)
--(axis cs:24000,0.00957203004509211)
--(axis cs:23900,0.00956068374216557)
--(axis cs:23800,0.00955010950565338)
--(axis cs:23700,0.00959984865039587)
--(axis cs:23600,0.00958504993468523)
--(axis cs:23500,0.00970917940139771)
--(axis cs:23400,0.0096717681735754)
--(axis cs:23300,0.00964275281876326)
--(axis cs:23200,0.00960088428109884)
--(axis cs:23100,0.00955763272941113)
--(axis cs:23000,0.00955055933445692)
--(axis cs:22900,0.00955520290881395)
--(axis cs:22800,0.00960665289312601)
--(axis cs:22700,0.00964434631168842)
--(axis cs:22600,0.00972689967602491)
--(axis cs:22500,0.00977513380348682)
--(axis cs:22400,0.00982604082673788)
--(axis cs:22300,0.00984209775924683)
--(axis cs:22200,0.00980161130428314)
--(axis cs:22100,0.00980418547987938)
--(axis cs:22000,0.00981598254293203)
--(axis cs:21900,0.00973813235759735)
--(axis cs:21800,0.00971978157758713)
--(axis cs:21700,0.00969735626131296)
--(axis cs:21600,0.00958204455673695)
--(axis cs:21500,0.00956072099506855)
--(axis cs:21400,0.00957965198904276)
--(axis cs:21300,0.00955413468182087)
--(axis cs:21200,0.00957519561052322)
--(axis cs:21100,0.00968784000724554)
--(axis cs:21000,0.00969153642654419)
--(axis cs:20900,0.00971422158181667)
--(axis cs:20800,0.00962056219577789)
--(axis cs:20700,0.00956303812563419)
--(axis cs:20600,0.00956036895513535)
--(axis cs:20500,0.00955578871071339)
--(axis cs:20400,0.00955240707844496)
--(axis cs:20300,0.00959772150963545)
--(axis cs:20200,0.00964460149407387)
--(axis cs:20100,0.00961128808557987)
--(axis cs:20000,0.00973989628255367)
--(axis cs:19900,0.00941066257655621)
--(axis cs:19800,0.00918510556221008)
--(axis cs:19700,0.00949182361364365)
--(axis cs:19600,0.00934605859220028)
--(axis cs:19500,0.00908891391009092)
--(axis cs:19400,0.00916974153369665)
--(axis cs:19300,0.00925514288246632)
--(axis cs:19200,0.00988036580383778)
--(axis cs:19100,0.0097278393805027)
--(axis cs:19000,0.0097913546487689)
--(axis cs:18900,0.0102973580360413)
--(axis cs:18800,0.0102973580360413)
--(axis cs:18700,0.0094796409830451)
--(axis cs:18600,0.00809080991894007)
--(axis cs:18500,0.00643750419840217)
--(axis cs:18400,0.00483478838577867)
--(axis cs:18300,0.00341312028467655)
--(axis cs:18200,0.00450510997325182)
--(axis cs:18100,0.00438620056957006)
--(axis cs:18000,0.00480936793610454)
--(axis cs:17900,0.0051271915435791)
--(axis cs:17800,0.0052429111674428)
--(axis cs:17700,0.00556178949773312)
--(axis cs:17600,0.0054587796330452)
--(axis cs:17500,0.00437994860112667)
--(axis cs:17400,0.00360985659062862)
--(axis cs:17300,0.00333795580081642)
--(axis cs:17200,0.00253121857531369)
--(axis cs:17100,0.00323015777394176)
--(axis cs:17000,0.00437927059829235)
--(axis cs:16900,0.00482456665486097)
--(axis cs:16800,0.00451077241450548)
--(axis cs:16700,0.00502599030733109)
--(axis cs:16600,0.00432963250204921)
--(axis cs:16500,0.00432313233613968)
--(axis cs:16400,0.00421633338555694)
--(axis cs:16300,0.00649840990081429)
--(axis cs:16200,0.0067102937027812)
--(axis cs:16100,0.00695659127086401)
--(axis cs:16000,0.0064244382083416)
--(axis cs:15900,0.00421866588294506)
--(axis cs:15800,0.00377162685617805)
--(axis cs:15700,0.00412330636754632)
--(axis cs:15600,0.00850956793874502)
--(axis cs:15500,0.0077411001548171)
--(axis cs:15400,0.00849411729723215)
--(axis cs:15300,0.00793438218533993)
--(axis cs:15200,0.00748604582622647)
--(axis cs:15100,0.00423459988087416)
--(axis cs:15000,0.00463910866528749)
--(axis cs:14900,0.00347792496904731)
--(axis cs:14800,0.00382573087699711)
--(axis cs:14700,0.00324236298911273)
--(axis cs:14600,0.00432484783232212)
--(axis cs:14500,0.00462356396019459)
--(axis cs:14400,0.00480239558964968)
--(axis cs:14300,0.00495634879916906)
--(axis cs:14200,0.00646419962868094)
--(axis cs:14100,0.0062364786863327)
--(axis cs:14000,0.00625646254047751)
--(axis cs:13900,0.00834075827151537)
--(axis cs:13800,0.011661565862596)
--(axis cs:13700,0.00999101530760527)
--(axis cs:13600,0.00961694680154324)
--(axis cs:13500,0.00936242006719112)
--(axis cs:13400,0.00742164626717567)
--(axis cs:13300,0.00408290978521109)
--(axis cs:13200,0.00319207459688187)
--(axis cs:13100,0.00568880699574947)
--(axis cs:13000,0.00653011118993163)
--(axis cs:12900,0.00654194178059697)
--(axis cs:12800,0.00595997367054224)
--(axis cs:12700,0.00567395612597466)
--(axis cs:12600,0.00709152920171618)
--(axis cs:12500,0.00655442243441939)
--(axis cs:12400,0.00599974580109119)
--(axis cs:12300,0.00597625970840454)
--(axis cs:12200,0.00698094163089991)
--(axis cs:12100,0.00429215282201767)
--(axis cs:12000,0.00400269031524658)
--(axis cs:11900,0.00513026677072048)
--(axis cs:11800,0.00548080494627357)
--(axis cs:11700,0.00671393517404795)
--(axis cs:11600,0.00662817480042577)
--(axis cs:11500,0.00740686897188425)
--(axis cs:11400,0.00728370808064938)
--(axis cs:11300,0.0071267606690526)
--(axis cs:11200,0.00680378079414368)
--(axis cs:11100,0.00791123695671558)
--(axis cs:11000,0.00648015318438411)
--(axis cs:10900,0.00594560708850622)
--(axis cs:10800,0.00588031858205795)
--(axis cs:10700,0.00509979343041778)
--(axis cs:10600,0.00481646927073598)
--(axis cs:10500,0.0055448180064559)
--(axis cs:10400,0.00537041295319796)
--(axis cs:10300,0.00728061003610492)
--(axis cs:10200,0.00598663184791803)
--(axis cs:10100,0.00617004372179508)
--(axis cs:10000,0.00780967809259892)
--(axis cs:9900,0.00796798430383205)
--(axis cs:9800,0.00408003805205226)
--(axis cs:9700,0.00583626981824636)
--(axis cs:9600,0.00585760734975338)
--(axis cs:9500,0.00495925499126315)
--(axis cs:9400,0.00532786967232823)
--(axis cs:9300,0.00661035813391209)
--(axis cs:9200,0.00717759039252996)
--(axis cs:9100,0.00727905612438917)
--(axis cs:9000,0.00665484368801117)
--(axis cs:8900,0.00668072886765003)
--(axis cs:8800,0.00563851278275251)
--(axis cs:8700,0.00501798512414098)
--(axis cs:8600,0.00510468473657966)
--(axis cs:8500,0.00419219303876162)
--(axis cs:8400,0.00486432481557131)
--(axis cs:8300,0.00449492828920484)
--(axis cs:8200,0.00402408232912421)
--(axis cs:8100,0.00349775003269315)
--(axis cs:8000,0.00522793829441071)
--(axis cs:7900,0.00482235988602042)
--(axis cs:7800,0.00791468936949968)
--(axis cs:7700,0.00621026521548629)
--(axis cs:7600,0.00635387748479843)
--(axis cs:7500,0.00843485537916422)
--(axis cs:7400,0.00953948777168989)
--(axis cs:7300,0.00693160388618708)
--(axis cs:7200,0.00729643041267991)
--(axis cs:7100,0.00712104002013803)
--(axis cs:7000,0.00513294991105795)
--(axis cs:6900,0.00635908730328083)
--(axis cs:6800,0.00402952311560512)
--(axis cs:6700,0.0038591306656599)
--(axis cs:6600,0.00424620695412159)
--(axis cs:6500,0.00622361246496439)
--(axis cs:6400,0.00481010926887393)
--(axis cs:6300,0.0035680322907865)
--(axis cs:6200,0.00423457426950336)
--(axis cs:6100,0.00370505452156067)
--(axis cs:6000,0.00199205987155437)
--(axis cs:5900,0.00228475616313517)
--(axis cs:5800,0.00276757567189634)
--(axis cs:5700,0.00265825679525733)
--(axis cs:5600,0.00391737837344408)
--(axis cs:5500,0.00302409683354199)
--(axis cs:5400,0.00277384370565414)
--(axis cs:5300,0.00252642622217536)
--(axis cs:5200,0.00240896106697619)
--(axis cs:5100,0.00128835497889668)
--(axis cs:5000,0.00151407637167722)
--(axis cs:4900,0.00186747591942549)
--(axis cs:4800,0.00207759882323444)
--(axis cs:4700,0.00173316267319024)
--(axis cs:4600,0.00303433928638697)
--(axis cs:4500,0.00283001735806465)
--(axis cs:4400,0.00580459740012884)
--(axis cs:4300,0.00590650178492069)
--(axis cs:4200,0.00566292461007833)
--(axis cs:4100,0.00550371734425426)
--(axis cs:4000,0.0055136363953352)
--(axis cs:3900,0.00547897256910801)
--(axis cs:3800,0.00506046507507563)
--(axis cs:3700,0.00447312230244279)
--(axis cs:3600,0.0045601618476212)
--(axis cs:3500,0.0050100376829505)
--(axis cs:3400,0.00476583791896701)
--(axis cs:3300,0.00342303281649947)
--(axis cs:3200,0.00376981263980269)
--(axis cs:3100,0.00458634970709682)
--(axis cs:3000,0.00273564527742565)
--(axis cs:2900,0.002783905249089)
--(axis cs:2800,0.00227103987708688)
--(axis cs:2700,0.00286986422725022)
--(axis cs:2600,0.00293836602941155)
--(axis cs:2500,0.00292103295214474)
--(axis cs:2400,0.00213274220004678)
--(axis cs:2300,0.00220579328015447)
--(axis cs:2200,0.00181057641748339)
--(axis cs:2100,0.00180232245475054)
--(axis cs:2000,0.00171651144046336)
--(axis cs:1900,0.00145908107515424)
--(axis cs:1800,0.00136423006188124)
--(axis cs:1700,0.000751428829971701)
--(axis cs:1600,0.0013703202130273)
--(axis cs:1500,0.00137883971910924)
--(axis cs:1400,0.00143318506889045)
--(axis cs:1300,0.00142068066634238)
--(axis cs:1200,0.00129664211999625)
--(axis cs:1100,0.000266197515884414)
--(axis cs:1000,0.000246120675001293)
--(axis cs:900,9.17654469958507e-05)
--(axis cs:800,7.33741326257586e-05)
--(axis cs:700,5.99576388538026e-10)
--(axis cs:600,5.99576388538026e-10)
--(axis cs:500,5.99576388538026e-10)
--(axis cs:400,0.000154673092765734)
--(axis cs:300,0.00116706255357713)
--(axis cs:200,0.00322034885175526)
--(axis cs:100,0.00546487607061863)
--(axis cs:0,0.00546552613377571)
--cycle;

\addplot [ultra thick, color0]
table {%
0 224.896194458008
100 272.092132568359
200 281.175018310547
300 288.550933837891
400 276.11962890625
500 71.3446426391602
600 32.4839477539062
700 31.3121242523193
800 32.5643119812012
900 34.2731437683105
1000 49.293083190918
1100 53.1637954711914
1200 53.6856422424316
1300 54.9357032775879
1400 59.402458190918
1500 48.5678939819336
1600 47.9450950622559
1700 50.6780242919922
1800 61.2941246032715
1900 67.5493927001953
2000 77.6405639648438
2100 86.8087692260742
2200 101.4970703125
2300 96.8659439086914
2400 105.068138122559
2500 105.04581451416
2600 129.207748413086
2700 145.884246826172
2800 160.281829833984
2900 180.489654541016
3000 186.948852539062
3100 164.702911376953
3200 152.406478881836
3300 149.977005004883
3400 164.423477172852
3500 199.915008544922
3700 252.624710083008
3800 259.022338867188
3900 246.61311340332
4000 259.505706787109
4100 265.581268310547
4200 261.547637939453
4300 280.943756103516
4400 288.377532958984
4500 283.536560058594
4600 295.669219970703
4700 312.109375
4800 307.619750976562
4900 321.348205566406
5000 308.849609375
5100 294.108306884766
5200 293.770080566406
5300 322.961151123047
5400 311.358764648438
5500 325.018127441406
5600 357.720489501953
5700 352.162139892578
5800 332.929992675781
5900 333.222381591797
6000 323.579437255859
6100 318.118377685547
6200 316.761871337891
6300 327.505249023438
6400 368.017608642578
6500 398.757385253906
6600 420.60498046875
6700 447.806976318359
6800 467.347900390625
6900 455.010040283203
7100 422.75927734375
7200 433.392700195312
7500 437.303863525391
7600 425.737396240234
7700 399.808868408203
7800 381.175109863281
7900 353.242401123047
8000 341.097961425781
8100 332.720245361328
8200 300.515167236328
8300 269.408081054688
8400 264.634826660156
8500 250.766403198242
8600 233.633331298828
8700 248.902206420898
8800 263.352508544922
8900 273.944671630859
9000 282.149017333984
9100 285.215911865234
9200 283.626068115234
9300 274.730987548828
9400 292.791961669922
9500 295.114776611328
9600 317.216766357422
9700 335.182189941406
9800 366.11474609375
9900 364.543975830078
10000 371.141326904297
10100 391.671295166016
10200 399.588989257812
10300 388.746398925781
10400 373.124176025391
10500 377.047027587891
10600 344.852142333984
10700 335.624847412109
10800 338.241607666016
10900 343.907043457031
11000 342.939514160156
11100 337.588989257812
11200 325.555999755859
11300 323.101409912109
11400 322.569549560547
11500 330.868530273438
11600 349.310729980469
11700 354.727264404297
11800 339.962646484375
11900 333.158355712891
12100 292.582458496094
12200 277.89794921875
12300 282.622161865234
12400 278.998077392578
12600 277.471405029297
12700 287.135406494141
12800 273.946014404297
12900 270.205413818359
13000 256.417388916016
13100 247.104644775391
13200 241.727355957031
13500 260.538604736328
13600 270.82421875
13700 270.359436035156
13800 274.620300292969
14000 278.190093994141
14100 285.719573974609
14200 286.774169921875
14300 284.7578125
14400 286.153442382812
14500 289.977416992188
14600 279.457489013672
14800 253.159637451172
14900 235.199996948242
15000 226.08073425293
15100 229.932525634766
15200 249.953979492188
15400 275.209350585938
15500 277.589782714844
15600 273.837463378906
15700 260.391906738281
15800 265.088500976562
15900 261.282012939453
16000 268.692474365234
16100 273.015625
16300 269.645263671875
16400 279.797973632812
16500 297.685394287109
16600 295.365692138672
16700 304.633575439453
16800 317.283813476562
16900 321.390380859375
17000 306.805145263672
17100 314.014129638672
17200 313.384704589844
17300 307.532623291016
17400 294.057464599609
17500 295.014831542969
17600 298.350433349609
17700 288.936767578125
17800 270.180786132812
17900 261.029663085938
18000 258.126770019531
18100 250.059936523438
18200 255.929382324219
18300 269.167999267578
18400 280.425079345703
18500 295.785461425781
18700 315.725067138672
18800 312.572326660156
18900 312.462524414062
19000 291.030792236328
19100 286.934173583984
19200 287.467712402344
19300 299.346282958984
19400 308.360656738281
19500 307.894287109375
19600 296.805999755859
19700 275.491424560547
19800 262.272735595703
19900 245.996673583984
20000 248.198135375977
20100 246.179458618164
20200 250.442260742188
20300 246.643035888672
20400 249.870010375977
20500 245.553161621094
20600 254.733871459961
20700 253.540313720703
20800 262.412719726562
20900 259.824157714844
21100 264.274780273438
21200 269.705230712891
21300 262.644470214844
21400 264.512969970703
21500 257.464874267578
21600 252.525024414062
21700 262.444000244141
21800 276.177368164062
21900 280.127807617188
22000 296.433898925781
22100 304.679382324219
22300 287.848785400391
22400 286.426300048828
22500 282.363006591797
22600 271.194976806641
22700 268.724029541016
23000 271.868469238281
23300 278.292419433594
23500 276.116729736328
23600 285.675811767578
23700 291.640625
23800 292.940368652344
23900 292.149749755859
24000 295.188842773438
24100 288.945648193359
24200 287.4296875
24300 287.625244140625
24400 291.584442138672
24500 287.935394287109
24600 292.164001464844
24700 300.981262207031
24800 303.734832763672
25000 316.108856201172
25100 317.463104248047
25200 311.640075683594
25300 312.664672851562
25500 309.82080078125
25700 296.609405517578
26000 293.183807373047
26100 298.420867919922
26200 306.763549804688
26300 308.65771484375
26500 308.887084960938
26600 301.019287109375
26700 290.292633056641
26800 281.649017333984
26900 279.385406494141
27000 278.982299804688
27100 280.810363769531
27200 292.326049804688
27400 304.471893310547
27600 310.419219970703
27700 309.070770263672
27800 311.129638671875
28000 311.163116455078
28100 322.181793212891
28200 331.367156982422
28300 335.113037109375
28400 333.093811035156
28500 344.511566162109
28600 342.443237304688
28700 333.545776367188
28800 326.964141845703
28900 325.362487792969
29000 312.751525878906
29100 302.763610839844
29200 295.7109375
29300 297.907867431641
29500 299.479095458984
29600 302.331268310547
29700 307.329071044922
29800 309.275970458984
29900 317.090515136719
30000 331.598999023438
30100 335.748870849609
30200 342.389099121094
30400 342.16455078125
30500 335.962951660156
30600 336.536468505859
30700 328.593719482422
30800 327.693725585938
31000 318.105804443359
31100 324.482757568359
31200 333.796356201172
31300 337.336456298828
31400 336.541656494141
31500 340.043273925781
31700 330.9462890625
31900 329.555694580078
32000 323.942749023438
32100 321.963592529297
32300 327.606842041016
32400 338.300476074219
32500 345.410339355469
32600 354.995910644531
32800 351.572418212891
32900 344.572845458984
33000 340.987487792969
33100 331.520904541016
33200 334.482238769531
33300 332.608856201172
33400 334.910339355469
33500 333.847320556641
33600 340.720275878906
33700 350.121887207031
33800 354.162017822266
34000 356.062957763672
34100 353.044830322266
34200 344.3115234375
34300 343.14892578125
};
\addplot [ultra thick, white!66.2745098039216!black, dash pattern=on 10pt off 5pt]
table {%
0 0.00515152141451836
100 0.00515093328431249
200 0.00298795290291309
300 0.00103488506283611
400 8.00003545009531e-05
500 2.48352838294608e-10
700 2.48352838294608e-10
800 3.03927809000015e-05
900 5.78296749154106e-05
1000 0.000164446042617783
1100 0.000173289939993992
1200 0.000633029616437852
1300 0.000805997056886554
1400 0.000799804634880275
1500 0.000763977353926748
1600 0.000994294881820679
1700 0.000672402500640601
1800 0.00105218321550637
1900 0.00118502660188824
2000 0.00143602560274303
2100 0.00124493287876248
2200 0.00157311570364982
2300 0.00132322299759835
2400 0.00141520402394235
2500 0.00177029706537724
2600 0.00186610058881342
2700 0.0018952211830765
2800 0.00220169546082616
2900 0.00245455862022936
3000 0.00220698839984834
3100 0.00313384691253304
3200 0.00299772713333368
3300 0.00248759193345904
3400 0.00283817504532635
3500 0.00334566156379879
3600 0.0031269402243197
3700 0.0028704886790365
3800 0.00305266887880862
3900 0.00346059631556273
4000 0.00446466961875558
4100 0.00368409371003509
4200 0.0043749213218689
4300 0.00421098247170448
4400 0.00339536461979151
4500 0.00171270803548396
4600 0.00188576127402484
4700 0.00117273861542344
4800 0.00156451866496354
4900 0.0014323660871014
5000 0.00128230464179069
5100 0.00118127488531172
5200 0.00203591072931886
5300 0.00193080306053162
5400 0.00214729411527514
5500 0.00252287788316607
5600 0.00302819791249931
5700 0.00216047838330269
5800 0.00256554246880114
5900 0.00210251519456506
6000 0.00174850143957883
6100 0.00318082049489021
6200 0.00357732269912958
6300 0.00306223123334348
6400 0.00402462901547551
6500 0.00478911679238081
6600 0.00301301316358149
6700 0.00288524804636836
6800 0.00301765650510788
6900 0.00387672684155405
7000 0.00391104491427541
7100 0.00573589187115431
7200 0.00590914208441973
7300 0.00604609632864594
7400 0.00584121374413371
7500 0.00568635761737823
7600 0.00459841964766383
7700 0.0043972977437079
7800 0.00491735385730863
7900 0.00333603098988533
8000 0.00325876055285335
8100 0.00245804828591645
8200 0.00294238142669201
8300 0.00321975094266236
8400 0.00348181929439306
8500 0.0029171125497669
8600 0.00378416874445975
8700 0.00338901253417134
8800 0.00386511348187923
8900 0.00526138814166188
9000 0.00559398671612144
9100 0.00557773094624281
9200 0.00595642672851682
9300 0.00511509506031871
9400 0.00378898321650922
9500 0.00370704126544297
9600 0.00388974160887301
9700 0.00373165146447718
9800 0.0030156362336129
9900 0.00445743277668953
10000 0.00437084026634693
10100 0.00402471702545881
10200 0.00386106502264738
10300 0.00543271377682686
10400 0.0040701269172132
10500 0.00434738583862782
10600 0.0036601850297302
10700 0.00385509640909731
10900 0.00327993743121624
11000 0.00373714161105454
11100 0.00486401654779911
11200 0.00447667110711336
11300 0.00499307457357645
11400 0.00512189511209726
11500 0.00492125051096082
11600 0.00413314439356327
11700 0.00446062255650759
11800 0.00365992565639317
11900 0.00361040094867349
12000 0.00317006278783083
12100 0.00362234865315259
12200 0.00544229010120034
12300 0.00437251524999738
12400 0.00438247853890061
12500 0.00516886962577701
12600 0.00497969705611467
12700 0.00430209608748555
12800 0.00452191149815917
12900 0.0048200530000031
13000 0.00455953972414136
13100 0.00406061904504895
13200 0.002780357375741
13300 0.00315156020224094
13400 0.00543827889487147
13500 0.00640389462932944
13600 0.00663481885567307
13700 0.00669957743957639
13800 0.00759990839287639
13900 0.00568864308297634
14000 0.00463417312130332
14100 0.00454873917624354
14200 0.00533057097345591
14300 0.00398258771747351
14400 0.00376789621077478
14500 0.00364243914373219
14600 0.00363702024333179
14700 0.00249313982203603
14800 0.00315937818959355
14900 0.00291313091292977
15000 0.00316380569711328
15100 0.00301427231170237
15200 0.00587726524099708
15300 0.00580383464694023
15400 0.00639043701812625
15500 0.0056417933665216
15600 0.00600409274920821
15700 0.00332801719196141
15800 0.0033622863702476
15900 0.00347629003226757
16000 0.00452250754460692
16100 0.00462112482637167
16200 0.00445491820573807
16300 0.00390920741483569
16400 0.00333251827396452
16600 0.00348489615134895
16700 0.00426304340362549
16800 0.00409733178094029
16900 0.00383320590481162
17000 0.00329230213537812
17100 0.00287561002187431
17200 0.00239169597625732
17300 0.00284583563916385
17400 0.00332821626216173
17500 0.00337739684619009
17600 0.00427542999386787
17700 0.0042381682433188
17800 0.00459037162363529
17900 0.0042667118832469
18000 0.00406006863340735
18100 0.00305927218869328
18200 0.00310161500237882
18300 0.00280284858308733
18400 0.00369284930638969
18500 0.00470620766282082
18600 0.00539789255708456
18700 0.00587629107758403
18800 0.00682799005880952
18900 0.0071806930936873
19000 0.00670790579169989
19100 0.00656936643645167
19200 0.00694721844047308
19300 0.00673875119537115
19400 0.00578479655086994
19500 0.00577498227357864
19600 0.00602583680301905
19700 0.00613735895603895
19800 0.00596081325784326
19900 0.00639667036011815
20000 0.00639706011861563
20100 0.0069384821690619
20200 0.00677716778591275
20300 0.00701317004859447
20400 0.00760613149031997
20500 0.00765698868781328
20600 0.00729042617604136
20700 0.00726265506818891
20800 0.00689096376299858
20900 0.00649216584861279
21000 0.0065798875875771
21100 0.00659457314759493
21200 0.00715942168608308
21300 0.00737248314544559
21400 0.00712724169716239
21500 0.00728660076856613
21600 0.00711079221218824
21700 0.00655700406059623
21900 0.00640343734994531
22000 0.00613357266411185
22200 0.00618158746510744
22300 0.00604769308120012
22400 0.00610020384192467
22600 0.00644452963024378
22700 0.00677810190245509
22800 0.00696295686066151
22900 0.00735494261607528
23000 0.0074545512907207
23100 0.00732188392430544
23200 0.00699482904747128
23300 0.00678530987352133
23500 0.00651114387437701
23600 0.00709048705175519
23700 0.0070006912574172
23800 0.00753826089203358
23900 0.00728648481890559
24000 0.00718336226418614
24100 0.00658507319167256
24200 0.00664832023903728
24300 0.00732431607320905
24400 0.0073310500010848
24500 0.00757151562720537
24600 0.00768278678879142
24700 0.00766120571643114
24800 0.00657390477135777
24900 0.00683462060987949
25000 0.00688612693920732
25100 0.00701159564778209
25200 0.00719005381688476
25300 0.00708057172596455
25400 0.0068969358690083
25600 0.00641028210520744
25700 0.00637550232931972
25800 0.00685393344610929
25900 0.00684325210750103
26000 0.00692437263205647
26200 0.0068906950764358
26300 0.00647836271673441
26500 0.0062546725384891
26600 0.00667583104223013
26700 0.00669700372964144
26800 0.0070195677690208
26900 0.00698065059259534
27000 0.00710890674963593
27100 0.00692943762987852
27200 0.00710297748446465
27300 0.00703377509489655
27400 0.00718610361218452
27600 0.00703342771157622
27800 0.00630521681159735
27900 0.00648992462083697
28000 0.00662650121375918
28100 0.00644557364284992
};

==> supp_mat/fetch_plots/geomrelerr.tex <==
% This file was created with tikzplotlib v0.9.12.
\begin{tikzpicture}

\definecolor{color0}{rgb}{1,0,1}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
log basis y={10},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={\(\displaystyle \mathrm{Number \ of \ training \ trajectories }\)},
xmajorgrids,
xmin=-23.95, xmax=524.95,
xtick style={color=black},
y grid style={white!69.0196078431373!black},
ylabel={\(\displaystyle \mathrm{Geometric \ mean \ of \ relative \ error }\)},
ymajorgrids,
ymin=0.06299942014023, ymax=0.517269287287668,
ymode=log,
ytick style={color=black}
]
\path [fill=blue, fill opacity=0.4, semithick]
(axis cs:1,0.450832588657663)
--(axis cs:1,0.342277254094566)
--(axis cs:10,0.193951732104943)
--(axis cs:25,0.150299187024981)
--(axis cs:75,0.139574592806006)
--(axis cs:200,0.127053163665148)
--(axis cs:500,0.12671936290503)
--(axis cs:500,0.173708148227355)
--(axis cs:500,0.173708148227355)
--(axis cs:200,0.153499872891358)
--(axis cs:75,0.175308678055132)
--(axis cs:25,0.200064418380496)
--(axis cs:10,0.242821759343827)
--(axis cs:1,0.450832588657663)
--cycle;

\path [fill=red, fill opacity=0.4, semithick]
(axis cs:1,0.470060717754753)
--(axis cs:1,0.349116601596732)
--(axis cs:10,0.128702420635964)
--(axis cs:25,0.103147952468473)
--(axis cs:75,0.0909859729168512)
--(axis cs:200,0.0821552220450362)
--(axis cs:500,0.0887728774389657)
--(axis cs:500,0.123950443219074)
--(axis cs:500,0.123950443219074)
--(axis cs:200,0.105308444634118)
--(axis cs:75,0.1225136292467)
--(axis cs:25,0.146719670927311)
--(axis cs:10,0.183442881853881)
--(axis cs:1,0.470060717754753)
--cycle;

\path [fill=green!50.1960784313725!black, fill opacity=0.4, semithick]
(axis cs:1,0.460758098853286)
--(axis cs:1,0.332549681437606)
--(axis cs:10,0.104416636058916)
--(axis cs:25,0.0929826811626782)
--(axis cs:75,0.0840021843585121)
--(axis cs:200,0.0737448759121545)
--(axis cs:500,0.0693265017147747)
--(axis cs:500,0.0930321786056807)
--(axis cs:500,0.0930321786056807)
--(axis cs:200,0.0942462047210047)
--(axis cs:75,0.107495555657725)
--(axis cs:25,0.119711127995211)
--(axis cs:10,0.131280766537419)
--(axis cs:1,0.460758098853286)
--cycle;

\path [fill=color0, fill opacity=0.4, semithick]
(axis cs:1,0.457690971213657)
--(axis cs:1,0.329526233032621)
--(axis cs:10,0.103653766848593)
--(axis cs:25,0.0935290442563888)
--(axis cs:75,0.0827389188560648)
--(axis cs:200,0.075193272762717)
--(axis cs:500,0.073899063733729)
--(axis cs:500,0.098851571947577)
--(axis cs:500,0.098851571947577)
--(axis cs:200,0.0969252035812792)
--(axis cs:75,0.100867508333778)
--(axis cs:25,0.134153717115168)
--(axis cs:10,0.131659006313328)
--(axis cs:1,0.457690971213657)
--cycle;

\addplot [semithick, blue, mark=asterisk, mark size=4, mark options={solid}]
table {%
1 0.396554887294769
10 0.218386724591255
25 0.175181820988655
75 0.157441630959511
200 0.140276536345482
500 0.150213733315468
};
\addlegendentry{No si.}
\addplot [semithick, red, mark=asterisk, mark size=4, mark options={solid}]
table {%
1 0.409588694572449
10 0.156072616577148
25 0.124933794140816
75 0.106749795377254
200 0.0937318354845047
500 0.106361664831638
};
\addlegendentry{Si 2}
\addplot [semithick, green!50.1960784313725!black, mark=asterisk, mark size=4, mark options={solid}]
table {%
1 0.396653860807419
10 0.117848709225655
25 0.106346897780895
75 0.0957488790154457
200 0.0839955359697342
500 0.0811793431639671
};
\addlegendentry{si 3}
\addplot [semithick, color0, mark=asterisk, mark size=4, mark options={solid}]
table {%
1 0.393608659505844
10 0.117656394839287
25 0.113841384649277
75 0.0918032079935074
200 0.0860592424869537
500 0.0863753259181976
};
\addlegendentry{si 4}
\end{axis}

\end{tikzpicture}


==> supp_mat/fetch_plots/relerr_500.tex <==
% This file was created with tikzplotlib v0.9.12.
\begin{tikzpicture}

\definecolor{color0}{rgb}{1,0,1}

\begin{axis}[
legend cell align={left},
legend style={
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  at={(0.03,0.97)},
  anchor=north west,
  draw=white!80!black
},
log basis y={10},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={\(\displaystyle \mathrm{Time \ (seconds)}\)},
xmajorgrids,
xmin=0.000499999988824129, xmax=0.0994999977760017,
xtick style={color=black},
y grid style={white!69.0196078431373!black},
ylabel={\(\displaystyle \mathrm{Relative \ error}\) (\(\displaystyle N_{\mathrm{train}}=500\))},
ymajorgrids,
ymin=0.0403423932359269, ymax=0.186214482340161,
ymode=log,
ytick style={color=black}
]
\path [fill=blue, fill opacity=0.4, semithick]
(axis cs:0.00499999988824129,0.0981471371189214)
--(axis cs:0.00499999988824129,0.0693458930148139)
--(axis cs:0.00999999977648258,0.0768913576643062)
--(axis cs:0.0149999996647239,0.0805582154812716)
--(axis cs:0.0199999995529652,0.0845196110592269)
--(axis cs:0.0249999994412065,0.0910616688263388)
--(axis cs:0.0299999993294477,0.0960605583494559)
--(axis cs:0.034999999217689,0.0995347371251724)
--(axis cs:0.0399999991059303,0.102204599471983)
--(axis cs:0.0449999989941716,0.105266256553993)
--(axis cs:0.0499999988824129,0.107840601840457)
--(axis cs:0.0549999987706542,0.11024953719084)
--(axis cs:0.0599999986588955,0.112444513695491)
--(axis cs:0.0649999985471368,0.114894346999308)
--(axis cs:0.0699999984353781,0.117045373991443)
--(axis cs:0.0749999983236194,0.119135580434824)
--(axis cs:0.0799999982118607,0.121087367134153)
--(axis cs:0.0849999981001019,0.123097295652794)
--(axis cs:0.0899999979883432,0.124914798373905)
--(axis cs:0.0949999978765845,0.12671936290503)
--(axis cs:0.0949999978765845,0.173708148227355)
--(axis cs:0.0949999978765845,0.173708148227355)
--(axis cs:0.0899999979883432,0.169887707845062)
--(axis cs:0.0849999981001019,0.165865428211006)
--(axis cs:0.0799999982118607,0.161634229731955)
--(axis cs:0.0749999983236194,0.157497989129546)
--(axis cs:0.0699999984353781,0.153176988531972)
--(axis cs:0.0649999985471368,0.148494744088243)
--(axis cs:0.0599999986588955,0.143608795563009)
--(axis cs:0.0549999987706542,0.139183186266431)
--(axis cs:0.0499999988824129,0.134703444736652)
--(axis cs:0.0449999989941716,0.130206618772106)
--(axis cs:0.0399999991059303,0.125438398773785)
--(axis cs:0.034999999217689,0.121120112118062)
--(axis cs:0.0299999993294477,0.116526519213719)
--(axis cs:0.0249999994412065,0.111403463333061)
--(axis cs:0.0199999995529652,0.108039080407262)
--(axis cs:0.0149999996647239,0.105659266717689)
--(axis cs:0.00999999977648258,0.103238590486459)
--(axis cs:0.00499999988824129,0.0981471371189214)
--cycle;

\path [fill=red, fill opacity=0.4, semithick]
(axis cs:0.00499999988824129,0.0830617524482067)
--(axis cs:0.00499999988824129,0.0577385334961019)
--(axis cs:0.00999999977648258,0.0609472347238716)
--(axis cs:0.0149999996647239,0.062344939486539)
--(axis cs:0.0199999995529652,0.0645523857627769)
--(axis cs:0.0249999994412065,0.0688552481509171)
--(axis cs:0.0299999993294477,0.0721968693716407)
--(axis cs:0.034999999217689,0.0740155351438639)
--(axis cs:0.0399999991059303,0.0747251433342523)
--(axis cs:0.0449999989941716,0.076196688060175)
--(axis cs:0.0499999988824129,0.078265236166539)
--(axis cs:0.0549999987706542,0.0799868066050893)
--(axis cs:0.0599999986588955,0.0811944321399374)
--(axis cs:0.0649999985471368,0.0826790375067071)
--(axis cs:0.0699999984353781,0.0842147872536796)
--(axis cs:0.0749999983236194,0.0852262409253277)
--(axis cs:0.0799999982118607,0.0858964548859035)
--(axis cs:0.0849999981001019,0.0869284669749143)
--(axis cs:0.0899999979883432,0.0880689473886511)
--(axis cs:0.0949999978765845,0.0887728774389657)
--(axis cs:0.0949999978765845,0.123950443219074)
--(axis cs:0.0949999978765845,0.123950443219074)
--(axis cs:0.0899999979883432,0.122065787742204)
--(axis cs:0.0849999981001019,0.119591672074542)
--(axis cs:0.0799999982118607,0.117123474651583)
--(axis cs:0.0749999983236194,0.114965108071722)
--(axis cs:0.0699999984353781,0.112221726189995)
--(axis cs:0.0649999985471368,0.108807137019256)
--(axis cs:0.0599999986588955,0.105237598566073)
--(axis cs:0.0549999987706542,0.102156176573968)
--(axis cs:0.0499999988824129,0.0986413392759387)
--(axis cs:0.0449999989941716,0.0947838197919073)
--(axis cs:0.0399999991059303,0.0911599179141883)
--(axis cs:0.034999999217689,0.0883223634854195)
--(axis cs:0.0299999993294477,0.0853904199404792)
--(axis cs:0.0249999994412065,0.0822060938997066)
--(axis cs:0.0199999995529652,0.0802182975294789)
--(axis cs:0.0149999996647239,0.0799168495767018)
--(axis cs:0.00999999977648258,0.0798972512640844)
--(axis cs:0.00499999988824129,0.0830617524482067)
--cycle;

\path [fill=green!50.1960784313725!black, fill opacity=0.4, semithick]
(axis cs:0.00499999988824129,0.0691418707714119)
--(axis cs:0.00499999988824129,0.0432468939969296)
--(axis cs:0.00999999977648258,0.0516324535170185)
--(axis cs:0.0149999996647239,0.0515130633290674)
--(axis cs:0.0199999995529652,0.0512873514591298)
--(axis cs:0.0249999994412065,0.0531749001829137)
--(axis cs:0.0299999993294477,0.0547475864476341)
--(axis cs:0.034999999217689,0.0563171018417981)
--(axis cs:0.0399999991059303,0.0571659570531023)
--(axis cs:0.0449999989941716,0.0586610050907562)
--(axis cs:0.0499999988824129,0.0600586372681437)
--(axis cs:0.0549999987706542,0.0612916019755903)
--(axis cs:0.0599999986588955,0.0622983017165615)
--(axis cs:0.0649999985471368,0.0635656407422943)
--(axis cs:0.0699999984353781,0.064995355484257)
--(axis cs:0.0749999983236194,0.0661467390966307)
--(axis cs:0.0799999982118607,0.066896883721782)
--(axis cs:0.0849999981001019,0.0678902986932688)
--(axis cs:0.0899999979883432,0.0688010277693822)
--(axis cs:0.0949999978765845,0.0693265017147747)
--(axis cs:0.0949999978765845,0.0930321786056807)
--(axis cs:0.0949999978765845,0.0930321786056807)
--(axis cs:0.0899999979883432,0.0919125371334513)
--(axis cs:0.0849999981001019,0.0902283378317776)
--(axis cs:0.0799999982118607,0.0886564630415355)
--(axis cs:0.0749999983236194,0.0875976061835957)
--(axis cs:0.0699999984353781,0.0861671861597333)
--(axis cs:0.0649999985471368,0.0842818920139673)
--(axis cs:0.0599999986588955,0.0822768049447333)
--(axis cs:0.0549999987706542,0.0810396972361705)
--(axis cs:0.0499999988824129,0.0796091263396972)
--(axis cs:0.0449999989941716,0.0775728662310419)
--(axis cs:0.0399999991059303,0.0749869548046289)
--(axis cs:0.034999999217689,0.0727956040974394)
--(axis cs:0.0299999993294477,0.0707275527701303)
--(axis cs:0.0249999994412065,0.0679617527078296)
--(axis cs:0.0199999995529652,0.0666160932079101)
--(axis cs:0.0149999996647239,0.0669410170690395)
--(axis cs:0.00999999977648258,0.0704492526822372)
--(axis cs:0.00499999988824129,0.0691418707714119)
--cycle;

\path [fill=color0, fill opacity=0.4, semithick]
(axis cs:0.00499999988824129,0.0728660114739282)
--(axis cs:0.00499999988824129,0.0472793839221152)
--(axis cs:0.00999999977648258,0.0522475106476856)
--(axis cs:0.0149999996647239,0.0543423041579315)
--(axis cs:0.0199999995529652,0.0549865341125751)
--(axis cs:0.0249999994412065,0.0575579704268763)
--(axis cs:0.0299999993294477,0.0597066606806348)
--(axis cs:0.034999999217689,0.0611029359784349)
--(axis cs:0.0399999991059303,0.0618320840140064)
--(axis cs:0.0449999989941716,0.0631873537919674)
--(axis cs:0.0499999988824129,0.064806731440754)
--(axis cs:0.0549999987706542,0.0661392594038266)
--(axis cs:0.0599999986588955,0.0671212654631985)
--(axis cs:0.0649999985471368,0.0684943794472619)
--(axis cs:0.0699999984353781,0.0698058700151522)
--(axis cs:0.0749999983236194,0.0707865738041196)
--(axis cs:0.0799999982118607,0.0714254531301117)
--(axis cs:0.0849999981001019,0.0722892435519938)
--(axis cs:0.0899999979883432,0.0731936281646384)
--(axis cs:0.0949999978765845,0.073899063733729)
--(axis cs:0.0949999978765845,0.098851571947577)
--(axis cs:0.0949999978765845,0.098851571947577)
--(axis cs:0.0899999979883432,0.0974827054803171)
--(axis cs:0.0849999981001019,0.0955383551671605)
--(axis cs:0.0799999982118607,0.093652007236664)
--(axis cs:0.0749999983236194,0.0923510896217436)
--(axis cs:0.0699999984353781,0.0907468745546822)
--(axis cs:0.0649999985471368,0.0885441239818889)
--(axis cs:0.0599999986588955,0.0862765882982384)
--(axis cs:0.0549999987706542,0.0849457619405477)
--(axis cs:0.0499999988824129,0.0830950683301027)
--(axis cs:0.0449999989941716,0.0807032698346358)
--(axis cs:0.0399999991059303,0.0778895897794887)
--(axis cs:0.034999999217689,0.0758716613948973)
--(axis cs:0.0299999993294477,0.0730464991303921)
--(axis cs:0.0249999994412065,0.0692151823749083)
--(axis cs:0.0199999995529652,0.0667704042014442)
--(axis cs:0.0149999996647239,0.0689100804883708)
--(axis cs:0.00999999977648258,0.0732407344645434)
--(axis cs:0.00499999988824129,0.0728660114739282)
--cycle;

\addplot [semithick, blue]
table {%
0.00499999523162842 0.0837465077638626
0.00999999046325684 0.0900649651885033
0.0149999856948853 0.0931087359786034
0.0199999809265137 0.0962793454527855
0.0249999761581421 0.101232580840588
0.0299999713897705 0.106293544173241
0.0349999666213989 0.110327422618866
0.0399999618530273 0.113821513950825
0.0449999570846558 0.117736451327801
0.0499999523162842 0.121272020041943
0.0549999475479126 0.124716356396675
0.059999942779541 0.128026649355888
0.065000057220459 0.131694540381432
0.0700000524520874 0.135111182928085
0.0750000476837158 0.138316780328751
0.0850000381469727 0.144481375813484
0.0900000333786011 0.147401243448257
0.0950000286102295 0.150213733315468
};
\addlegendentry{No si.}
\addplot [semithick, red]
table {%
0.00499999523162842 0.0704001411795616
0.00999999046325684 0.0704222470521927
0.0149999856948853 0.0711309015750885
0.0199999809265137 0.0723853409290314
0.0249999761581421 0.0755306631326675
0.0299999713897705 0.0787936374545097
0.0349999666213989 0.081168957054615
0.0399999618530273 0.0829425230622292
0.0449999570846558 0.0854902490973473
0.0499999523162842 0.0884532779455185
0.0549999475479126 0.0910714864730835
0.059999942779541 0.0932160168886185
0.065000057220459 0.0957430973649025
0.0700000524520874 0.0982182696461678
0.0750000476837158 0.100095674395561
0.0800000429153442 0.101509973406792
0.0850000381469727 0.103260084986687
0.0900000333786011 0.105067357420921
0.0950000286102295 0.106361664831638
};
\addlegendentry{Si 2}
\addplot [semithick, green!50.1960784313725!black]
table {%
0.00499999523162842 0.0561943836510181
0.00999999046325684 0.061040848493576
0.0149999856948853 0.0592270456254482
0.0199999809265137 0.0589517205953598
0.0249999761581421 0.0605683177709579
0.0299999713897705 0.0627375692129135
0.0349999666213989 0.0645563378930092
0.0399999618530273 0.0660764425992966
0.0449999570846558 0.0681169256567955
0.0499999523162842 0.0698338747024536
0.0549999475479126 0.071165643632412
0.059999942779541 0.0722875520586967
0.065000057220459 0.0739237666130066
0.0700000524520874 0.0755812674760818
0.0750000476837158 0.0768721699714661
0.0800000429153442 0.0777766704559326
0.0900000333786011 0.080356776714325
0.0950000286102295 0.0811793431639671
};
\addlegendentry{si 3}
\addplot [semithick, color0]
table {%
0.00499999523162842 0.0600726939737797
0.00999999046325684 0.0627441257238388
0.0149999856948853 0.0616261959075928
0.0199999809265137 0.060878474265337
0.0249999761581421 0.0633865743875504
0.0299999713897705 0.0663765668869019
0.0349999666213989 0.0684873014688492
0.0399999618530273 0.0698608309030533
0.0449999570846558 0.0719453096389771
0.0499999523162842 0.0739509016275406
0.0549999475479126 0.0755425170063972
0.059999942779541 0.0766989141702652
0.065000057220459 0.0785192474722862
0.0700000524520874 0.0802763700485229
0.0750000476837158 0.0815688446164131
0.0800000429153442 0.0825387313961983
0.0850000381469727 0.0839137956500053
0.0900000333786011 0.0853381603956223
0.0950000286102295 0.0863753259181976
};
\addlegendentry{si 4}
\end{axis}

\end{tikzpicture}


==> supp_mat/fetch_plots/relerr_data.tex <==
\path [fill=red, fill opacity=0.4, ultra thick]
(axis cs:0.00499999988824129,0.0981471371189214)
--(axis cs:0.00499999988824129,0.0693458930148139)
--(axis cs:0.00999999977648258,0.0768913576643062)
--(axis cs:0.0149999996647239,0.0805582154812716)
--(axis cs:0.0199999995529652,0.0845196110592269)
--(axis cs:0.0249999994412065,0.0910616688263388)
--(axis cs:0.0299999993294477,0.0960605583494559)
--(axis cs:0.034999999217689,0.0995347371251724)
--(axis cs:0.0399999991059303,0.102204599471983)
--(axis cs:0.0449999989941716,0.105266256553993)
--(axis cs:0.0499999988824129,0.107840601840457)
--(axis cs:0.0549999987706542,0.11024953719084)
--(axis cs:0.0599999986588955,0.112444513695491)
--(axis cs:0.0649999985471368,0.114894346999308)
--(axis cs:0.0699999984353781,0.117045373991443)
--(axis cs:0.0749999983236194,0.119135580434824)
--(axis cs:0.0799999982118607,0.121087367134153)
--(axis cs:0.0849999981001019,0.123097295652794)
--(axis cs:0.0899999979883432,0.124914798373905)
--(axis cs:0.0949999978765845,0.12671936290503)
--(axis cs:0.0949999978765845,0.173708148227355)
--(axis cs:0.0949999978765845,0.173708148227355)
--(axis cs:0.0899999979883432,0.169887707845062)
--(axis cs:0.0849999981001019,0.165865428211006)
--(axis cs:0.0799999982118607,0.161634229731955)
--(axis cs:0.0749999983236194,0.157497989129546)
--(axis cs:0.0699999984353781,0.153176988531972)
--(axis cs:0.0649999985471368,0.148494744088243)
--(axis cs:0.0599999986588955,0.143608795563009)
--(axis cs:0.0549999987706542,0.139183186266431)
--(axis cs:0.0499999988824129,0.134703444736652)
--(axis cs:0.0449999989941716,0.130206618772106)
--(axis cs:0.0399999991059303,0.125438398773785)
--(axis cs:0.034999999217689,0.121120112118062)
--(axis cs:0.0299999993294477,0.116526519213719)
--(axis cs:0.0249999994412065,0.111403463333061)
--(axis cs:0.0199999995529652,0.108039080407262)
--(axis cs:0.0149999996647239,0.105659266717689)
--(axis cs:0.00999999977648258,0.103238590486459)
--(axis cs:0.00499999988824129,0.0981471371189214)
--cycle;

\path [fill=green!50.1960784313725!black, fill opacity=0.4, ultra thick]
(axis cs:0.00499999988824129,0.0830617524482067)
--(axis cs:0.00499999988824129,0.0577385334961019)
--(axis cs:0.00999999977648258,0.0609472347238716)
--(axis cs:0.0149999996647239,0.062344939486539)
--(axis cs:0.0199999995529652,0.0645523857627769)
--(axis cs:0.0249999994412065,0.0688552481509171)
--(axis cs:0.0299999993294477,0.0721968693716407)
--(axis cs:0.034999999217689,0.0740155351438639)
--(axis cs:0.0399999991059303,0.0747251433342523)
--(axis cs:0.0449999989941716,0.076196688060175)
--(axis cs:0.0499999988824129,0.078265236166539)
--(axis cs:0.0549999987706542,0.0799868066050893)
--(axis cs:0.0599999986588955,0.0811944321399374)
--(axis cs:0.0649999985471368,0.0826790375067071)
--(axis cs:0.0699999984353781,0.0842147872536796)
--(axis cs:0.0749999983236194,0.0852262409253277)
--(axis cs:0.0799999982118607,0.0858964548859035)
--(axis cs:0.0849999981001019,0.0869284669749143)
--(axis cs:0.0899999979883432,0.0880689473886511)
--(axis cs:0.0949999978765845,0.0887728774389657)
--(axis cs:0.0949999978765845,0.123950443219074)
--(axis cs:0.0949999978765845,0.123950443219074)
--(axis cs:0.0899999979883432,0.122065787742204)
--(axis cs:0.0849999981001019,0.119591672074542)
--(axis cs:0.0799999982118607,0.117123474651583)
--(axis cs:0.0749999983236194,0.114965108071722)
--(axis cs:0.0699999984353781,0.112221726189995)
--(axis cs:0.0649999985471368,0.108807137019256)
--(axis cs:0.0599999986588955,0.105237598566073)
--(axis cs:0.0549999987706542,0.102156176573968)
--(axis cs:0.0499999988824129,0.0986413392759387)
--(axis cs:0.0449999989941716,0.0947838197919073)
--(axis cs:0.0399999991059303,0.0911599179141883)
--(axis cs:0.034999999217689,0.0883223634854195)
--(axis cs:0.0299999993294477,0.0853904199404792)
--(axis cs:0.0249999994412065,0.0822060938997066)
--(axis cs:0.0199999995529652,0.0802182975294789)
--(axis cs:0.0149999996647239,0.0799168495767018)
--(axis cs:0.00999999977648258,0.0798972512640844)
--(axis cs:0.00499999988824129,0.0830617524482067)
--cycle;

\path [fill=color0, fill opacity=0.4, ultra thick]
(axis cs:0.00499999988824129,0.0691418707714119)
--(axis cs:0.00499999988824129,0.0432468939969296)
--(axis cs:0.00999999977648258,0.0516324535170185)
--(axis cs:0.0149999996647239,0.0515130633290674)
--(axis cs:0.0199999995529652,0.0512873514591298)
--(axis cs:0.0249999994412065,0.0531749001829137)
--(axis cs:0.0299999993294477,0.0547475864476341)
--(axis cs:0.034999999217689,0.0563171018417981)
--(axis cs:0.0399999991059303,0.0571659570531023)
--(axis cs:0.0449999989941716,0.0586610050907562)
--(axis cs:0.0499999988824129,0.0600586372681437)
--(axis cs:0.0549999987706542,0.0612916019755903)
--(axis cs:0.0599999986588955,0.0622983017165615)
--(axis cs:0.0649999985471368,0.0635656407422943)
--(axis cs:0.0699999984353781,0.064995355484257)
--(axis cs:0.0749999983236194,0.0661467390966307)
--(axis cs:0.0799999982118607,0.066896883721782)
--(axis cs:0.0849999981001019,0.0678902986932688)
--(axis cs:0.0899999979883432,0.0688010277693822)
--(axis cs:0.0949999978765845,0.0693265017147747)
--(axis cs:0.0949999978765845,0.0930321786056807)
--(axis cs:0.0949999978765845,0.0930321786056807)
--(axis cs:0.0899999979883432,0.0919125371334513)
--(axis cs:0.0849999981001019,0.0902283378317776)
--(axis cs:0.0799999982118607,0.0886564630415355)
--(axis cs:0.0749999983236194,0.0875976061835957)
--(axis cs:0.0699999984353781,0.0861671861597333)
--(axis cs:0.0649999985471368,0.0842818920139673)
--(axis cs:0.0599999986588955,0.0822768049447333)
--(axis cs:0.0549999987706542,0.0810396972361705)
--(axis cs:0.0499999988824129,0.0796091263396972)
--(axis cs:0.0449999989941716,0.0775728662310419)
--(axis cs:0.0399999991059303,0.0749869548046289)
--(axis cs:0.034999999217689,0.0727956040974394)
--(axis cs:0.0299999993294477,0.0707275527701303)
--(axis cs:0.0249999994412065,0.0679617527078296)
--(axis cs:0.0199999995529652,0.0666160932079101)
--(axis cs:0.0149999996647239,0.0669410170690395)
--(axis cs:0.00999999977648258,0.0704492526822372)
--(axis cs:0.00499999988824129,0.0691418707714119)
--cycle;

\path [fill=white!40!black, fill opacity=0.4, ultra thick]
(axis cs:0.00499999988824129,0.0728660114739282)
--(axis cs:0.00499999988824129,0.0472793839221152)
--(axis cs:0.00999999977648258,0.0522475106476856)
--(axis cs:0.0149999996647239,0.0543423041579315)
--(axis cs:0.0199999995529652,0.0549865341125751)
--(axis cs:0.0249999994412065,0.0575579704268763)
--(axis cs:0.0299999993294477,0.0597066606806348)
--(axis cs:0.034999999217689,0.0611029359784349)
--(axis cs:0.0399999991059303,0.0618320840140064)
--(axis cs:0.0449999989941716,0.0631873537919674)
--(axis cs:0.0499999988824129,0.064806731440754)
--(axis cs:0.0549999987706542,0.0661392594038266)
--(axis cs:0.0599999986588955,0.0671212654631985)
--(axis cs:0.0649999985471368,0.0684943794472619)
--(axis cs:0.0699999984353781,0.0698058700151522)
--(axis cs:0.0749999983236194,0.0707865738041196)
--(axis cs:0.0799999982118607,0.0714254531301117)
--(axis cs:0.0849999981001019,0.0722892435519938)
--(axis cs:0.0899999979883432,0.0731936281646384)
--(axis cs:0.0949999978765845,0.073899063733729)
--(axis cs:0.0949999978765845,0.098851571947577)
--(axis cs:0.0949999978765845,0.098851571947577)
--(axis cs:0.0899999979883432,0.0974827054803171)
--(axis cs:0.0849999981001019,0.0955383551671605)
--(axis cs:0.0799999982118607,0.093652007236664)
--(axis cs:0.0749999983236194,0.0923510896217436)
--(axis cs:0.0699999984353781,0.0907468745546822)
--(axis cs:0.0649999985471368,0.0885441239818889)
--(axis cs:0.0599999986588955,0.0862765882982384)
--(axis cs:0.0549999987706542,0.0849457619405477)
--(axis cs:0.0499999988824129,0.0830950683301027)
--(axis cs:0.0449999989941716,0.0807032698346358)
--(axis cs:0.0399999991059303,0.0778895897794887)
--(axis cs:0.034999999217689,0.0758716613948973)
--(axis cs:0.0299999993294477,0.0730464991303921)
--(axis cs:0.0249999994412065,0.0692151823749083)
--(axis cs:0.0199999995529652,0.0667704042014442)
--(axis cs:0.0149999996647239,0.0689100804883708)
--(axis cs:0.00999999977648258,0.0732407344645434)
--(axis cs:0.00499999988824129,0.0728660114739282)
--cycle;

\addplot [ultra thick, red]
table {%
0.00499999523162842 0.0837465077638626
0.00999999046325684 0.0900649651885033
0.0149999856948853 0.0931087359786034
0.0199999809265137 0.0962793454527855
0.0249999761581421 0.101232580840588
0.0299999713897705 0.106293544173241
0.0349999666213989 0.110327422618866
0.0399999618530273 0.113821513950825
0.0449999570846558 0.117736451327801
0.0499999523162842 0.121272020041943
0.0549999475479126 0.124716356396675
0.059999942779541 0.128026649355888
0.065000057220459 0.131694540381432
0.0700000524520874 0.135111182928085
0.0750000476837158 0.138316780328751
0.0850000381469727 0.144481375813484
0.0900000333786011 0.147401243448257
0.0950000286102295 0.150213733315468
};
% \addlegendentry{No si.}
\addplot [ultra thick, green!50.1960784313725!black]
table {%
0.00499999523162842 0.0704001411795616
0.00999999046325684 0.0704222470521927
0.0149999856948853 0.0711309015750885
0.0199999809265137 0.0723853409290314
0.0249999761581421 0.0755306631326675
0.0299999713897705 0.0787936374545097
0.0349999666213989 0.081168957054615
0.0399999618530273 0.0829425230622292
0.0449999570846558 0.0854902490973473
0.0499999523162842 0.0884532779455185
0.0549999475479126 0.0910714864730835
0.059999942779541 0.0932160168886185
0.065000057220459 0.0957430973649025
0.0700000524520874 0.0982182696461678
0.0750000476837158 0.100095674395561
0.0800000429153442 0.101509973406792
0.0850000381469727 0.103260084986687
0.0900000333786011 0.105067357420921
0.0950000286102295 0.106361664831638
};
% \addlegendentry{Si 2}
\addplot [ultra thick, color0]
table {%
0.00499999523162842 0.0561943836510181
0.00999999046325684 0.061040848493576
0.0149999856948853 0.0592270456254482
0.0199999809265137 0.0589517205953598
0.0249999761581421 0.0605683177709579
0.0299999713897705 0.0627375692129135
0.0349999666213989 0.0645563378930092
0.0399999618530273 0.0660764425992966
0.0449999570846558 0.0681169256567955
0.0499999523162842 0.0698338747024536
0.0549999475479126 0.071165643632412
0.059999942779541 0.0722875520586967
0.065000057220459 0.0739237666130066
0.0700000524520874 0.0755812674760818
0.0750000476837158 0.0768721699714661
0.0800000429153442 0.0777766704559326
0.0900000333786011 0.080356776714325
0.0950000286102295 0.0811793431639671
};
% \addlegendentry{si 3}
\addplot [ultra thick, white!40!black]
table {%
0.00499999523162842 0.0600726939737797
0.00999999046325684 0.0627441257238388
0.0149999856948853 0.0616261959075928
0.0199999809265137 0.060878474265337
0.0249999761581421 0.0633865743875504
0.0299999713897705 0.0663765668869019
0.0349999666213989 0.0684873014688492
0.0399999618530273 0.0698608309030533
0.0449999570846558 0.0719453096389771
0.0499999523162842 0.0739509016275406
0.0549999475479126 0.0755425170063972
0.059999942779541 0.0766989141702652
0.065000057220459 0.0785192474722862
0.0700000524520874 0.0802763700485229
0.0750000476837158 0.0815688446164131
0.0800000429153442 0.0825387313961983
0.0850000381469727 0.0839137956500053
0.0900000333786011 0.0853381603956223
0.0950000286102295 0.0863753259181976
};
% \addlegendentry{si 4}




% \path [fill=blue, fill opacity=0.4, ultra thick]
% (axis cs:0.00499999988824129,0.104644967318169)
% --(axis cs:0.00499999988824129,0.0735731940053169)
% --(axis cs:0.00999999977648258,0.0808920605276985)
% --(axis cs:0.0149999996647239,0.0836938807572603)
% --(axis cs:0.0199999995529652,0.0867695519978043)
% --(axis cs:0.0249999994412065,0.0923157700653139)
% --(axis cs:0.0299999993294477,0.0973650951179764)
% --(axis cs:0.034999999217689,0.101662286631509)
% --(axis cs:0.0399999991059303,0.105320288986683)
% --(axis cs:0.0449999989941716,0.108968955728221)
% --(axis cs:0.0499999988824129,0.112164199952017)
% --(axis cs:0.0549999987706542,0.114874582314576)
% --(axis cs:0.0599999986588955,0.117283901268746)
% --(axis cs:0.0649999985471368,0.119674390690466)
% --(axis cs:0.0699999984353781,0.121829861257787)
% --(axis cs:0.0749999983236194,0.123752504517181)
% --(axis cs:0.0799999982118607,0.1256384918868)
% --(axis cs:0.0849999981001019,0.127635494599139)
% --(axis cs:0.0899999979883432,0.129562600113302)
% --(axis cs:0.0949999978765845,0.13142408914452)
% --(axis cs:0.0999999977648258,0.133205876743766)
% --(axis cs:0.104999997653067,0.135073594172048)
% --(axis cs:0.109999997541308,0.136834793923856)
% --(axis cs:0.11499999742955,0.138437898607242)
% --(axis cs:0.119999997317791,0.139934224885507)
% --(axis cs:0.124999997206032,0.141429874370928)
% --(axis cs:0.129999997094274,0.142813579882247)
% --(axis cs:0.134999996982515,0.144077579317613)
% --(axis cs:0.139999996870756,0.145249019510009)
% --(axis cs:0.144999996758997,0.146419907406387)
% --(axis cs:0.149999996647239,0.147562421058272)
% --(axis cs:0.15499999653548,0.148690351919368)
% --(axis cs:0.159999996423721,0.149804332145281)
% --(axis cs:0.164999996311963,0.150995638410959)
% --(axis cs:0.169999996200204,0.152170440940089)
% --(axis cs:0.174999996088445,0.153359390460353)
% --(axis cs:0.179999995976686,0.154604749199006)
% --(axis cs:0.184999995864928,0.15597526650941)
% --(axis cs:0.189999995753169,0.157512710256331)
% --(axis cs:0.19499999564141,0.159211054828558)
% --(axis cs:0.199999995529652,0.161087170455919)
% --(axis cs:0.204999995417893,0.163058040021124)
% --(axis cs:0.209999995306134,0.165098760390318)
% --(axis cs:0.214999995194376,0.167214557386469)
% --(axis cs:0.219999995082617,0.169383305629256)
% --(axis cs:0.224999994970858,0.171670192782016)
% --(axis cs:0.229999994859099,0.174060459585118)
% --(axis cs:0.234999994747341,0.176524598007166)
% --(axis cs:0.239999994635582,0.179035766404665)
% --(axis cs:0.244999994523823,0.181571641720527)
% --(axis cs:0.249999994412065,0.184139903083795)
% --(axis cs:0.254999994300306,0.186705873531486)
% --(axis cs:0.259999994188547,0.189271209372746)
% --(axis cs:0.264999994076788,0.19184850312581)
% --(axis cs:0.26999999396503,0.194425657701666)
% --(axis cs:0.274999993853271,0.196978490692018)
% --(axis cs:0.279999993741512,0.199493515675635)
% --(axis cs:0.284999993629754,0.20196690511764)
% --(axis cs:0.289999993517995,0.204384454027888)
% --(axis cs:0.294999993406236,0.206762409183226)
% --(axis cs:0.299999993294477,0.209077914295185)
% --(axis cs:0.304999993182719,0.211398599946444)
% --(axis cs:0.30999999307096,0.21367382878454)
% --(axis cs:0.314999992959201,0.215896106155777)
% --(axis cs:0.319999992847443,0.218102084808151)
% --(axis cs:0.324999992735684,0.220279090268894)
% --(axis cs:0.329999992623925,0.222426757967953)
% --(axis cs:0.334999992512167,0.224562763561923)
% --(axis cs:0.339999992400408,0.226690720198322)
% --(axis cs:0.344999992288649,0.228828048873333)
% --(axis cs:0.34999999217689,0.230960049781846)
% --(axis cs:0.354999992065132,0.233086611026266)
% --(axis cs:0.359999991953373,0.235212454822518)
% --(axis cs:0.364999991841614,0.237378767508273)
% --(axis cs:0.369999991729856,0.239566018308699)
% --(axis cs:0.374999991618097,0.24175396638904)
% --(axis cs:0.379999991506338,0.243947285350089)
% --(axis cs:0.384999991394579,0.246147274598957)
% --(axis cs:0.389999991282821,0.248327282774095)
% --(axis cs:0.394999991171062,0.250508289601579)
% --(axis cs:0.399999991059303,0.252684933863462)
% --(axis cs:0.404999990947545,0.254852182536972)
% --(axis cs:0.409999990835786,0.257020699377944)
% --(axis cs:0.414999990724027,0.259148981080679)
% --(axis cs:0.419999990612268,0.261252144042803)
% --(axis cs:0.42499999050051,0.26334111823306)
% --(axis cs:0.429999990388751,0.265379620519107)
% --(axis cs:0.434999990276992,0.267365589339461)
% --(axis cs:0.439999990165234,0.269326258130468)
% --(axis cs:0.444999990053475,0.271266364461258)
% --(axis cs:0.449999989941716,0.273167769137577)
% --(axis cs:0.454999989829957,0.275033112195185)
% --(axis cs:0.459999989718199,0.276870047537394)
% --(axis cs:0.46499998960644,0.27870401345168)
% --(axis cs:0.469999989494681,0.280521795208296)
% --(axis cs:0.474999989382923,0.282334225868085)
% --(axis cs:0.479999989271164,0.284138345551925)
% --(axis cs:0.484999989159405,0.285920029945882)
% --(axis cs:0.489999989047647,0.28768411599039)
% --(axis cs:0.494999988935888,0.289442441096964)
% --(axis cs:0.494999988935888,0.385392018376879)
% --(axis cs:0.494999988935888,0.385392018376879)
% --(axis cs:0.489999989047647,0.383232416726784)
% --(axis cs:0.484999989159405,0.381038863322875)
% --(axis cs:0.479999989271164,0.378801498204892)
% --(axis cs:0.474999989382923,0.376548727245794)
% --(axis cs:0.469999989494681,0.374266103938028)
% --(axis cs:0.46499998960644,0.371958947572844)
% --(axis cs:0.459999989718199,0.36964654332137)
% --(axis cs:0.454999989829957,0.367348182077589)
% --(axis cs:0.449999989941716,0.365021707668885)
% --(axis cs:0.444999990053475,0.362655860991412)
% --(axis cs:0.439999990165234,0.360271672254737)
% --(axis cs:0.434999990276992,0.357880713618944)
% --(axis cs:0.429999990388751,0.355472420676185)
% --(axis cs:0.42499999050051,0.353020795716705)
% --(axis cs:0.419999990612268,0.350531423514041)
% --(axis cs:0.414999990724027,0.348029239996762)
% --(axis cs:0.409999990835786,0.345495137006861)
% --(axis cs:0.404999990947545,0.3429348168487)
% --(axis cs:0.399999991059303,0.340354493698975)
% --(axis cs:0.394999991171062,0.337789870303694)
% --(axis cs:0.389999991282821,0.335205801384271)
% --(axis cs:0.384999991394579,0.332578348947944)
% --(axis cs:0.379999991506338,0.32990961709774)
% --(axis cs:0.374999991618097,0.327249707679)
% --(axis cs:0.369999991729856,0.324563048667938)
% --(axis cs:0.364999991841614,0.321866331028157)
% --(axis cs:0.359999991953373,0.319158542574693)
% --(axis cs:0.354999992065132,0.316466704556033)
% --(axis cs:0.34999999217689,0.31374778768912)
% --(axis cs:0.344999992288649,0.311004144993009)
% --(axis cs:0.339999992400408,0.308250753258195)
% --(axis cs:0.334999992512167,0.305521583272315)
% --(axis cs:0.329999992623925,0.302744054759145)
% --(axis cs:0.324999992735684,0.299913996238354)
% --(axis cs:0.319999992847443,0.297069249928117)
% --(axis cs:0.314999992959201,0.294219340450701)
% --(axis cs:0.30999999307096,0.291342974674745)
% --(axis cs:0.304999993182719,0.288448772495865)
% --(axis cs:0.299999993294477,0.285541348061667)
% --(axis cs:0.294999993406236,0.28270302530654)
% --(axis cs:0.289999993517995,0.279841306072054)
% --(axis cs:0.284999993629754,0.276968977459032)
% --(axis cs:0.279999993741512,0.274060557995169)
% --(axis cs:0.274999993853271,0.271133796324603)
% --(axis cs:0.26999999396503,0.268170750674561)
% --(axis cs:0.264999994076788,0.265182288949878)
% --(axis cs:0.259999994188547,0.262184279507878)
% --(axis cs:0.254999994300306,0.25925803369192)
% --(axis cs:0.249999994412065,0.256331025477006)
% --(axis cs:0.244999994523823,0.253402034823111)
% --(axis cs:0.239999994635582,0.250508650220522)
% --(axis cs:0.234999994747341,0.247689148309062)
% --(axis cs:0.229999994859099,0.244880140444648)
% --(axis cs:0.224999994970858,0.242046699387587)
% --(axis cs:0.219999995082617,0.239186093521672)
% --(axis cs:0.214999995194376,0.236397313277547)
% --(axis cs:0.209999995306134,0.233639262380815)
% --(axis cs:0.204999995417893,0.230969664637113)
% --(axis cs:0.199999995529652,0.228355032460781)
% --(axis cs:0.19499999564141,0.22580687581028)
% --(axis cs:0.189999995753169,0.223264714471965)
% --(axis cs:0.184999995864928,0.220692950013391)
% --(axis cs:0.179999995976686,0.218100626073155)
% --(axis cs:0.174999996088445,0.215579089457809)
% --(axis cs:0.169999996200204,0.213054996818397)
% --(axis cs:0.164999996311963,0.210489730287167)
% --(axis cs:0.159999996423721,0.207904919033045)
% --(axis cs:0.15499999653548,0.205351943198339)
% --(axis cs:0.149999996647239,0.202773866407403)
% --(axis cs:0.144999996758997,0.200162856899296)
% --(axis cs:0.139999996870756,0.197499526284553)
% --(axis cs:0.134999996982515,0.194856788489981)
% --(axis cs:0.129999997094274,0.192131576628439)
% --(axis cs:0.124999997206032,0.189313496542394)
% --(axis cs:0.119999997317791,0.186420357989294)
% --(axis cs:0.11499999742955,0.18356440234626)
% --(axis cs:0.109999997541308,0.180589700072097)
% --(axis cs:0.104999997653067,0.17749141917182)
% --(axis cs:0.0999999977648258,0.174274378331976)
% --(axis cs:0.0949999978765845,0.171135413018651)
% --(axis cs:0.0899999979883432,0.1679158439598)
% --(axis cs:0.0849999981001019,0.164660100636731)
% --(axis cs:0.0799999982118607,0.161369633955076)
% --(axis cs:0.0749999983236194,0.158447923434911)
% --(axis cs:0.0699999984353781,0.155508515442735)
% --(axis cs:0.0649999985471368,0.152562822303125)
% --(axis cs:0.0599999986588955,0.149644851810824)
% --(axis cs:0.0549999987706542,0.147344385922198)
% --(axis cs:0.0499999988824129,0.144624422975886)
% --(axis cs:0.0449999989941716,0.141438255943546)
% --(axis cs:0.0399999991059303,0.137329900200645)
% --(axis cs:0.034999999217689,0.132848545513201)
% --(axis cs:0.0299999993294477,0.127554194425302)
% --(axis cs:0.0249999994412065,0.122188839704902)
% --(axis cs:0.0199999995529652,0.117637873483173)
% --(axis cs:0.0149999996647239,0.114162500857339)
% --(axis cs:0.00999999977648258,0.110827012774136)
% --(axis cs:0.00499999988824129,0.104644967318169)
% --cycle;

% \path [fill=red, fill opacity=0.4, ultra thick]
% (axis cs:0.00499999988824129,0.115323148725986)
% --(axis cs:0.00499999988824129,0.0777649893221378)
% --(axis cs:0.00999999977648258,0.0848498704497275)
% --(axis cs:0.0149999996647239,0.0876242482072469)
% --(axis cs:0.0199999995529652,0.0903150550499889)
% --(axis cs:0.0249999994412065,0.0948590644829372)
% --(axis cs:0.0299999993294477,0.0987825867679661)
% --(axis cs:0.034999999217689,0.101518560374524)
% --(axis cs:0.0399999991059303,0.103652610297194)
% --(axis cs:0.0449999989941716,0.105969880028875)
% --(axis cs:0.0499999988824129,0.107956286707888)
% --(axis cs:0.0549999987706542,0.109656123009977)
% --(axis cs:0.0599999986588955,0.111217858392856)
% --(axis cs:0.0649999985471368,0.113106333385324)
% --(axis cs:0.0699999984353781,0.114675728616817)
% --(axis cs:0.0749999983236194,0.115936028405548)
% --(axis cs:0.0799999982118607,0.116997216418278)
% --(axis cs:0.0849999981001019,0.118160586497656)
% --(axis cs:0.0899999979883432,0.119174678313352)
% --(axis cs:0.0949999978765845,0.120074064296149)
% --(axis cs:0.0999999977648258,0.120937919501056)
% --(axis cs:0.104999997653067,0.121911309847295)
% --(axis cs:0.109999997541308,0.122844218669428)
% --(axis cs:0.11499999742955,0.123683973411858)
% --(axis cs:0.119999997317791,0.124510987407826)
% --(axis cs:0.124999997206032,0.125438034955452)
% --(axis cs:0.129999997094274,0.12632974188517)
% --(axis cs:0.134999996982515,0.127174117710089)
% --(axis cs:0.139999996870756,0.127993114756346)
% --(axis cs:0.144999996758997,0.128889133139415)
% --(axis cs:0.149999996647239,0.129824534793162)
% --(axis cs:0.15499999653548,0.130766464833809)
% --(axis cs:0.159999996423721,0.131703411098832)
% --(axis cs:0.164999996311963,0.132769650062524)
% --(axis cs:0.169999996200204,0.133879472519765)
% --(axis cs:0.174999996088445,0.134964031838909)
% --(axis cs:0.179999995976686,0.136000339720473)
% --(axis cs:0.184999995864928,0.137086638445677)
% --(axis cs:0.189999995753169,0.138221114496175)
% --(axis cs:0.19499999564141,0.139378416511888)
% --(axis cs:0.199999995529652,0.140601278382238)
% --(axis cs:0.204999995417893,0.141873633248089)
% --(axis cs:0.209999995306134,0.143158456069269)
% --(axis cs:0.214999995194376,0.144433311498)
% --(axis cs:0.219999995082617,0.145735375410912)
% --(axis cs:0.224999994970858,0.147056177021314)
% --(axis cs:0.229999994859099,0.148393366880473)
% --(axis cs:0.234999994747341,0.149766533633098)
% --(axis cs:0.239999994635582,0.151182438867571)
% --(axis cs:0.244999994523823,0.152603374087243)
% --(axis cs:0.249999994412065,0.15402858502602)
% --(axis cs:0.254999994300306,0.155438285344679)
% --(axis cs:0.259999994188547,0.15681428323794)
% --(axis cs:0.264999994076788,0.158192472258403)
% --(axis cs:0.26999999396503,0.159540307337155)
% --(axis cs:0.274999993853271,0.160855012875347)
% --(axis cs:0.279999993741512,0.162117701960092)
% --(axis cs:0.284999993629754,0.16334837724874)
% --(axis cs:0.289999993517995,0.164537469557674)
% --(axis cs:0.294999993406236,0.165765728361017)
% --(axis cs:0.299999993294477,0.166912601846999)
% --(axis cs:0.304999993182719,0.168086855671557)
% --(axis cs:0.30999999307096,0.169226722341343)
% --(axis cs:0.314999992959201,0.170308198000797)
% --(axis cs:0.319999992847443,0.171380096410684)
% --(axis cs:0.324999992735684,0.17243664785745)
% --(axis cs:0.329999992623925,0.173457349164852)
% --(axis cs:0.334999992512167,0.174462804215311)
% --(axis cs:0.339999992400408,0.175472581807845)
% --(axis cs:0.344999992288649,0.176454656704429)
% --(axis cs:0.34999999217689,0.177412862818855)
% --(axis cs:0.354999992065132,0.178337525799806)
% --(axis cs:0.359999991953373,0.179250928049253)
% --(axis cs:0.364999991841614,0.180240352779148)
% --(axis cs:0.369999991729856,0.18122981942378)
% --(axis cs:0.374999991618097,0.182228511910347)
% --(axis cs:0.379999991506338,0.1832528188409)
% --(axis cs:0.384999991394579,0.184288305595684)
% --(axis cs:0.389999991282821,0.185307995045993)
% --(axis cs:0.394999991171062,0.186342496633504)
% --(axis cs:0.399999991059303,0.187361104642761)
% --(axis cs:0.404999990947545,0.188318019747563)
% --(axis cs:0.409999990835786,0.189283604460759)
% --(axis cs:0.414999990724027,0.190191776510701)
% --(axis cs:0.419999990612268,0.191065816054047)
% --(axis cs:0.42499999050051,0.191926409777511)
% --(axis cs:0.429999990388751,0.192748515305735)
% --(axis cs:0.434999990276992,0.193521901309966)
% --(axis cs:0.439999990165234,0.194260040597891)
% --(axis cs:0.444999990053475,0.194991816688482)
% --(axis cs:0.449999989941716,0.195757637184958)
% --(axis cs:0.454999989829957,0.196460982648037)
% --(axis cs:0.459999989718199,0.197146788064293)
% --(axis cs:0.46499998960644,0.197848506176417)
% --(axis cs:0.469999989494681,0.198537370176233)
% --(axis cs:0.474999989382923,0.199270514545252)
% --(axis cs:0.479999989271164,0.199982059127765)
% --(axis cs:0.484999989159405,0.200772436117638)
% --(axis cs:0.489999989047647,0.201595229414353)
% --(axis cs:0.494999988935888,0.202401563889188)
% --(axis cs:0.494999988935888,0.267334673739007)
% --(axis cs:0.494999988935888,0.267334673739007)
% --(axis cs:0.489999989047647,0.266392663090109)
% --(axis cs:0.484999989159405,0.265431700082125)
% --(axis cs:0.479999989271164,0.26449651625256)
% --(axis cs:0.474999989382923,0.263547774299235)
% --(axis cs:0.469999989494681,0.262567320963961)
% --(axis cs:0.46499998960644,0.261596730645664)
% --(axis cs:0.459999989718199,0.260611383168248)
% --(axis cs:0.454999989829957,0.259621167722351)
% --(axis cs:0.449999989941716,0.258617351136264)
% --(axis cs:0.444999990053475,0.257580110177751)
% --(axis cs:0.439999990165234,0.256514147628608)
% --(axis cs:0.434999990276992,0.255442177868827)
% --(axis cs:0.429999990388751,0.254355594624831)
% --(axis cs:0.42499999050051,0.253220909276357)
% --(axis cs:0.419999990612268,0.252051406436885)
% --(axis cs:0.414999990724027,0.250890784152269)
% --(axis cs:0.409999990835786,0.249696506193748)
% --(axis cs:0.404999990947545,0.248492273800554)
% --(axis cs:0.399999991059303,0.247235360401502)
% --(axis cs:0.394999991171062,0.245983897039866)
% --(axis cs:0.389999991282821,0.244681379229696)
% --(axis cs:0.384999991394579,0.243365549842991)
% --(axis cs:0.379999991506338,0.242016125684251)
% --(axis cs:0.374999991618097,0.240693186273677)
% --(axis cs:0.369999991729856,0.239328290483388)
% --(axis cs:0.364999991841614,0.237969106358381)
% --(axis cs:0.359999991953373,0.23654514483009)
% --(axis cs:0.354999992065132,0.235193980954573)
% --(axis cs:0.34999999217689,0.23381502229776)
% --(axis cs:0.344999992288649,0.232433165480359)
% --(axis cs:0.339999992400408,0.231069015293304)
% --(axis cs:0.334999992512167,0.229701997185493)
% --(axis cs:0.329999992623925,0.228373500181266)
% --(axis cs:0.324999992735684,0.227069038231186)
% --(axis cs:0.319999992847443,0.225790645756163)
% --(axis cs:0.314999992959201,0.224526033075727)
% --(axis cs:0.30999999307096,0.223262333390923)
% --(axis cs:0.304999993182719,0.221957139399408)
% --(axis cs:0.299999993294477,0.220580555586704)
% --(axis cs:0.294999993406236,0.219275543817263)
% --(axis cs:0.289999993517995,0.217955873914347)
% --(axis cs:0.284999993629754,0.216651929831597)
% --(axis cs:0.279999993741512,0.215340723840481)
% --(axis cs:0.274999993853271,0.214109186380535)
% --(axis cs:0.26999999396503,0.212878444754997)
% --(axis cs:0.264999994076788,0.211643588762323)
% --(axis cs:0.259999994188547,0.210439511097812)
% --(axis cs:0.254999994300306,0.20930654830538)
% --(axis cs:0.249999994412065,0.208188499089921)
% --(axis cs:0.244999994523823,0.207043877158112)
% --(axis cs:0.239999994635582,0.205969163880385)
% --(axis cs:0.234999994747341,0.204925208664335)
% --(axis cs:0.229999994859099,0.203932147593429)
% --(axis cs:0.224999994970858,0.202873637206446)
% --(axis cs:0.219999995082617,0.201803304814188)
% --(axis cs:0.214999995194376,0.200756940434422)
% --(axis cs:0.209999995306134,0.199689594290334)
% --(axis cs:0.204999995417893,0.19876871600107)
% --(axis cs:0.199999995529652,0.197834880456701)
% --(axis cs:0.19499999564141,0.196936268207326)
% --(axis cs:0.189999995753169,0.195942748293694)
% --(axis cs:0.184999995864928,0.194896809192459)
% --(axis cs:0.179999995976686,0.193810291666759)
% --(axis cs:0.174999996088445,0.192796912316492)
% --(axis cs:0.169999996200204,0.191724467277622)
% --(axis cs:0.164999996311963,0.19057212449875)
% --(axis cs:0.159999996423721,0.18939432956688)
% --(axis cs:0.15499999653548,0.188285607901092)
% --(axis cs:0.149999996647239,0.187143957677883)
% --(axis cs:0.144999996758997,0.185978488205353)
% --(axis cs:0.139999996870756,0.184764824252658)
% --(axis cs:0.134999996982515,0.183561875698163)
% --(axis cs:0.129999997094274,0.182276828459588)
% --(axis cs:0.124999997206032,0.180852493587045)
% --(axis cs:0.119999997317791,0.179334688886043)
% --(axis cs:0.11499999742955,0.177896907617686)
% --(axis cs:0.109999997541308,0.176234160408414)
% --(axis cs:0.104999997653067,0.174359363712783)
% --(axis cs:0.0999999977648258,0.172277012117884)
% --(axis cs:0.0949999978765845,0.170112583160872)
% --(axis cs:0.0899999979883432,0.167660647011338)
% --(axis cs:0.0849999981001019,0.164889582146963)
% --(axis cs:0.0799999982118607,0.161849751472089)
% --(axis cs:0.0749999983236194,0.158919588601636)
% --(axis cs:0.0699999984353781,0.155732267660274)
% --(axis cs:0.0649999985471368,0.152350414729004)
% --(axis cs:0.0599999986588955,0.148816315729496)
% --(axis cs:0.0549999987706542,0.145846369950568)
% --(axis cs:0.0499999988824129,0.142431785960871)
% --(axis cs:0.0449999989941716,0.139036829363225)
% --(axis cs:0.0399999991059303,0.135173732269162)
% --(axis cs:0.034999999217689,0.131664782662156)
% --(axis cs:0.0299999993294477,0.127698206181957)
% --(axis cs:0.0249999994412065,0.12378645301857)
% --(axis cs:0.0199999995529652,0.120456069490315)
% --(axis cs:0.0149999996647239,0.118911521950235)
% --(axis cs:0.00999999977648258,0.117899680506565)
% --(axis cs:0.00499999988824129,0.115323148725986)
% --cycle;

% \path [fill=green!50.1960784313725!black, fill opacity=0.4, ultra thick]
% (axis cs:0.00499999988824129,0.0905936145398397)
% --(axis cs:0.00499999988824129,0.0619344746316198)
% --(axis cs:0.00999999977648258,0.0643951706717472)
% --(axis cs:0.0149999996647239,0.0653294359239248)
% --(axis cs:0.0199999995529652,0.066889258578383)
% --(axis cs:0.0249999994412065,0.070217011365269)
% --(axis cs:0.0299999993294477,0.0738559794930689)
% --(axis cs:0.034999999217689,0.0770621182568461)
% --(axis cs:0.0399999991059303,0.0795285510342601)
% --(axis cs:0.0449999989941716,0.0819562772393401)
% --(axis cs:0.0499999988824129,0.0846317128454203)
% --(axis cs:0.0549999987706542,0.0866215792615274)
% --(axis cs:0.0599999986588955,0.0879249477371107)
% --(axis cs:0.0649999985471368,0.089615614995606)
% --(axis cs:0.0699999984353781,0.0915062668902724)
% --(axis cs:0.0749999983236194,0.0928340885431344)
% --(axis cs:0.0799999982118607,0.0935478286933084)
% --(axis cs:0.0849999981001019,0.0946570942411352)
% --(axis cs:0.0899999979883432,0.0960547828902234)
% --(axis cs:0.0949999978765845,0.0970455563206244)
% --(axis cs:0.0999999977648258,0.0976856848693922)
% --(axis cs:0.104999997653067,0.0988120199618261)
% --(axis cs:0.109999997541308,0.100077116232881)
% --(axis cs:0.11499999742955,0.10081090440166)
% --(axis cs:0.119999997317791,0.101369310139692)
% --(axis cs:0.124999997206032,0.102470062699565)
% --(axis cs:0.129999997094274,0.103678925529724)
% --(axis cs:0.134999996982515,0.104503430747126)
% --(axis cs:0.139999996870756,0.10527489014677)
% --(axis cs:0.144999996758997,0.106557498751393)
% --(axis cs:0.149999996647239,0.107900738740209)
% --(axis cs:0.15499999653548,0.10883821729714)
% --(axis cs:0.159999996423721,0.109888269938818)
% --(axis cs:0.164999996311963,0.111501055981534)
% --(axis cs:0.169999996200204,0.113144602110863)
% --(axis cs:0.174999996088445,0.114368129569538)
% --(axis cs:0.179999995976686,0.115903736671615)
% --(axis cs:0.184999995864928,0.117974529655571)
% --(axis cs:0.189999995753169,0.11995925349499)
% --(axis cs:0.19499999564141,0.12161329930135)
% --(axis cs:0.199999995529652,0.12374732758748)
% --(axis cs:0.204999995417893,0.126334951915038)
% --(axis cs:0.209999995306134,0.128740577060067)
% --(axis cs:0.214999995194376,0.130913732113491)
% --(axis cs:0.219999995082617,0.133632685206692)
% --(axis cs:0.224999994970858,0.136677889548922)
% --(axis cs:0.229999994859099,0.139437646968747)
% --(axis cs:0.234999994747341,0.142045095562463)
% --(axis cs:0.239999994635582,0.145220930955307)
% --(axis cs:0.244999994523823,0.148591642267018)
% --(axis cs:0.249999994412065,0.151690540837371)
% --(axis cs:0.254999994300306,0.154706347173512)
% --(axis cs:0.259999994188547,0.158191905295761)
% --(axis cs:0.264999994076788,0.161801702369791)
% --(axis cs:0.26999999396503,0.165162325427477)
% --(axis cs:0.274999993853271,0.168490306013928)
% --(axis cs:0.279999993741512,0.172220027384902)
% --(axis cs:0.284999993629754,0.176040929434169)
% --(axis cs:0.289999993517995,0.179646676320252)
% --(axis cs:0.294999993406236,0.183271356702235)
% --(axis cs:0.299999993294477,0.18720170566392)
% --(axis cs:0.304999993182719,0.19119806081624)
% --(axis cs:0.30999999307096,0.195065083762147)
% --(axis cs:0.314999992959201,0.19892778263886)
% --(axis cs:0.319999992847443,0.203016479622035)
% --(axis cs:0.324999992735684,0.207153527058704)
% --(axis cs:0.329999992623925,0.211187850040957)
% --(axis cs:0.334999992512167,0.21521023986656)
% --(axis cs:0.339999992400408,0.219360471671798)
% --(axis cs:0.344999992288649,0.223534655355488)
% --(axis cs:0.34999999217689,0.227639825365903)
% --(axis cs:0.354999992065132,0.231717608236221)
% --(axis cs:0.359999991953373,0.235873744249659)
% --(axis cs:0.364999991841614,0.240057808639197)
% --(axis cs:0.369999991729856,0.244180670116588)
% --(axis cs:0.374999991618097,0.248259982864188)
% --(axis cs:0.379999991506338,0.252382722043005)
% --(axis cs:0.384999991394579,0.256504301834792)
% --(axis cs:0.389999991282821,0.260562441872667)
% --(axis cs:0.394999991171062,0.264574062216608)
% --(axis cs:0.399999991059303,0.268600965216978)
% --(axis cs:0.404999990947545,0.272627398714064)
% --(axis cs:0.409999990835786,0.276605664682336)
% --(axis cs:0.414999990724027,0.280524440081107)
% --(axis cs:0.419999990612268,0.284431321079858)
% --(axis cs:0.42499999050051,0.288328906086199)
% --(axis cs:0.429999990388751,0.292179750519874)
% --(axis cs:0.434999990276992,0.295960383406113)
% --(axis cs:0.439999990165234,0.299711016105431)
% --(axis cs:0.444999990053475,0.303457807739307)
% --(axis cs:0.449999989941716,0.307180385472404)
% --(axis cs:0.454999989829957,0.310837229203332)
% --(axis cs:0.459999989718199,0.314452361436014)
% --(axis cs:0.46499998960644,0.318058200395016)
% --(axis cs:0.469999989494681,0.321645320655308)
% --(axis cs:0.474999989382923,0.325177329576675)
% --(axis cs:0.479999989271164,0.328657164928547)
% --(axis cs:0.484999989159405,0.33212724566744)
% --(axis cs:0.489999989047647,0.335585535055852)
% --(axis cs:0.494999988935888,0.339012015787009)
% --(axis cs:0.494999988935888,0.423174016440028)
% --(axis cs:0.494999988935888,0.423174016440028)
% --(axis cs:0.489999989047647,0.419759463528283)
% --(axis cs:0.484999989159405,0.416317490283102)
% --(axis cs:0.479999989271164,0.412858982173539)
% --(axis cs:0.474999989382923,0.409357781168524)
% --(axis cs:0.469999989494681,0.405791279764874)
% --(axis cs:0.46499998960644,0.402177130713504)
% --(axis cs:0.459999989718199,0.398556507571238)
% --(axis cs:0.454999989829957,0.394919299467151)
% --(axis cs:0.449999989941716,0.391190949706465)
% --(axis cs:0.444999990053475,0.387412097059352)
% --(axis cs:0.439999990165234,0.383616123636629)
% --(axis cs:0.434999990276992,0.379805317071009)
% --(axis cs:0.429999990388751,0.375919802399306)
% --(axis cs:0.42499999050051,0.371953023372403)
% --(axis cs:0.419999990612268,0.367963560465907)
% --(axis cs:0.414999990724027,0.363970716732445)
% --(axis cs:0.409999990835786,0.35989908220315)
% --(axis cs:0.404999990947545,0.355742462386361)
% --(axis cs:0.399999991059303,0.351545364876176)
% --(axis cs:0.394999991171062,0.347353337732869)
% --(axis cs:0.389999991282821,0.343109011586739)
% --(axis cs:0.384999991394579,0.338768689848453)
% --(axis cs:0.379999991506338,0.334387266326286)
% --(axis cs:0.374999991618097,0.329998260998805)
% --(axis cs:0.369999991729856,0.325577518838651)
% --(axis cs:0.364999991841614,0.321069897028989)
% --(axis cs:0.359999991953373,0.316507100068982)
% --(axis cs:0.354999992065132,0.311954876900811)
% --(axis cs:0.34999999217689,0.307406588197479)
% --(axis cs:0.344999992288649,0.302773026542977)
% --(axis cs:0.339999992400408,0.298087564223247)
% --(axis cs:0.334999992512167,0.293378937834227)
% --(axis cs:0.329999992623925,0.288746056057768)
% --(axis cs:0.324999992735684,0.284049694797799)
% --(axis cs:0.319999992847443,0.279261448915349)
% --(axis cs:0.314999992959201,0.274471284377216)
% --(axis cs:0.30999999307096,0.269775059475637)
% --(axis cs:0.304999993182719,0.265048965685354)
% --(axis cs:0.299999993294477,0.260192919307162)
% --(axis cs:0.294999993406236,0.255329638241039)
% --(axis cs:0.289999993517995,0.250674088490193)
% --(axis cs:0.284999993629754,0.245957231738513)
% --(axis cs:0.279999993741512,0.241119209438786)
% --(axis cs:0.274999993853271,0.236259484595615)
% --(axis cs:0.26999999396503,0.23166762701484)
% --(axis cs:0.264999994076788,0.227155098158826)
% --(axis cs:0.259999994188547,0.222385497861896)
% --(axis cs:0.254999994300306,0.217734842144771)
% --(axis cs:0.249999994412065,0.21357792776023)
% --(axis cs:0.244999994523823,0.209439746624466)
% --(axis cs:0.239999994635582,0.205044221603139)
% --(axis cs:0.234999994747341,0.200774445671174)
% --(axis cs:0.229999994859099,0.19720343831519)
% --(axis cs:0.224999994970858,0.193577620014021)
% --(axis cs:0.219999995082617,0.189537076352577)
% --(axis cs:0.214999995194376,0.185866844768108)
% --(axis cs:0.209999995306134,0.182953097505703)
% --(axis cs:0.204999995417893,0.180004656083975)
% --(axis cs:0.199999995529652,0.176574702263556)
% --(axis cs:0.19499999564141,0.173618403888439)
% --(axis cs:0.189999995753169,0.171530429454806)
% --(axis cs:0.184999995864928,0.16897502876134)
% --(axis cs:0.179999995976686,0.166068018225678)
% --(axis cs:0.174999996088445,0.163722713872973)
% --(axis cs:0.169999996200204,0.1619771403708)
% --(axis cs:0.164999996311963,0.159892748969577)
% --(axis cs:0.159999996423721,0.157498667698726)
% --(axis cs:0.15499999653548,0.155816834776973)
% --(axis cs:0.149999996647239,0.154719875326475)
% --(axis cs:0.144999996758997,0.153007838280282)
% --(axis cs:0.139999996870756,0.151022497238454)
% --(axis cs:0.134999996982515,0.149646427987025)
% --(axis cs:0.129999997094274,0.148754034290532)
% --(axis cs:0.124999997206032,0.147201628289117)
% --(axis cs:0.119999997317791,0.145505880028255)
% --(axis cs:0.11499999742955,0.144562323745085)
% --(axis cs:0.109999997541308,0.143760930331894)
% --(axis cs:0.104999997653067,0.142221298716994)
% --(axis cs:0.0999999977648258,0.14050204433664)
% --(axis cs:0.0949999978765845,0.139287454897502)
% --(axis cs:0.0899999979883432,0.13769892538765)
% --(axis cs:0.0849999981001019,0.135321896426039)
% --(axis cs:0.0799999982118607,0.132861408165901)
% --(axis cs:0.0749999983236194,0.130649481806007)
% --(axis cs:0.0699999984353781,0.12791689037287)
% --(axis cs:0.0649999985471368,0.12474647528303)
% --(axis cs:0.0599999986588955,0.121533834934194)
% --(axis cs:0.0549999987706542,0.119088036008425)
% --(axis cs:0.0499999988824129,0.116099491437273)
% --(axis cs:0.0449999989941716,0.113040665141123)
% --(axis cs:0.0399999991059303,0.110558637406503)
% --(axis cs:0.034999999217689,0.109022654615685)
% --(axis cs:0.0299999993294477,0.106104931973609)
% --(axis cs:0.0249999994412065,0.102545191119572)
% --(axis cs:0.0199999995529652,0.0997331082189722)
% --(axis cs:0.0149999996647239,0.0963579984910028)
% --(axis cs:0.00999999977648258,0.0926075090910755)
% --(axis cs:0.00499999988824129,0.0905936145398397)
% --cycle;

% \path [fill=color0, fill opacity=0.4, ultra thick]
% (axis cs:0.00499999988824129,0.0723257914846999)
% --(axis cs:0.00499999988824129,0.044429407423608)
% --(axis cs:0.00999999977648258,0.0539409375767771)
% --(axis cs:0.0149999996647239,0.053225250659491)
% --(axis cs:0.0199999995529652,0.0531345400969327)
% --(axis cs:0.0249999994412065,0.0551293052876465)
% --(axis cs:0.0299999993294477,0.0571697549564637)
% --(axis cs:0.034999999217689,0.0588305271295207)
% --(axis cs:0.0399999991059303,0.0599630955190938)
% --(axis cs:0.0449999989941716,0.0617028736620725)
% --(axis cs:0.0499999988824129,0.0634576459598399)
% --(axis cs:0.0549999987706542,0.0646482099618023)
% --(axis cs:0.0599999986588955,0.0654319256960148)
% --(axis cs:0.0649999985471368,0.0664430674285895)
% --(axis cs:0.0699999984353781,0.0677677144711779)
% --(axis cs:0.0749999983236194,0.0687458842516745)
% --(axis cs:0.0799999982118607,0.0694806170757633)
% --(axis cs:0.0849999981001019,0.070411033322479)
% --(axis cs:0.0899999979883432,0.071418889230684)
% --(axis cs:0.0949999978765845,0.0720862912562898)
% --(axis cs:0.0999999977648258,0.0727198262668881)
% --(axis cs:0.104999997653067,0.0735291859354889)
% --(axis cs:0.109999997541308,0.0743550325112774)
% --(axis cs:0.11499999742955,0.0748841847476781)
% --(axis cs:0.119999997317791,0.0753862491825369)
% --(axis cs:0.124999997206032,0.0761232292564328)
% --(axis cs:0.129999997094274,0.0768467600382069)
% --(axis cs:0.134999996982515,0.077428795486793)
% --(axis cs:0.139999996870756,0.0780102705271391)
% --(axis cs:0.144999996758997,0.0788065685103195)
% --(axis cs:0.149999996647239,0.0796340660563939)
% --(axis cs:0.15499999653548,0.0802784814557429)
% --(axis cs:0.159999996423721,0.0810320538343023)
% --(axis cs:0.164999996311963,0.0819777925142018)
% --(axis cs:0.169999996200204,0.0828753442214418)
% --(axis cs:0.174999996088445,0.0836859806752981)
% --(axis cs:0.179999995976686,0.0847211183128134)
% --(axis cs:0.184999995864928,0.0859697191411594)
% --(axis cs:0.189999995753169,0.0871684657718662)
% --(axis cs:0.19499999564141,0.0884106620521939)
% --(axis cs:0.199999995529652,0.0899353354768147)
% --(axis cs:0.204999995417893,0.0915776381551231)
% --(axis cs:0.209999995306134,0.0931094477164975)
% --(axis cs:0.214999995194376,0.0947679461792401)
% --(axis cs:0.219999995082617,0.0966536621453462)
% --(axis cs:0.224999994970858,0.0985770539479435)
% --(axis cs:0.229999994859099,0.100382971438614)
% --(axis cs:0.234999994747341,0.102384216571466)
% --(axis cs:0.239999994635582,0.104543701349481)
% --(axis cs:0.244999994523823,0.106716009165406)
% --(axis cs:0.249999994412065,0.108803642419831)
% --(axis cs:0.254999994300306,0.111045089737367)
% --(axis cs:0.259999994188547,0.113373893624675)
% --(axis cs:0.264999994076788,0.115722334162695)
% --(axis cs:0.26999999396503,0.118004115494962)
% --(axis cs:0.274999993853271,0.120463270142621)
% --(axis cs:0.279999993741512,0.12298102677754)
% --(axis cs:0.284999993629754,0.125502318493234)
% --(axis cs:0.289999993517995,0.128012918856024)
% --(axis cs:0.294999993406236,0.130686107903321)
% --(axis cs:0.299999993294477,0.133411083929857)
% --(axis cs:0.304999993182719,0.136173687226338)
% --(axis cs:0.30999999307096,0.138994660887709)
% --(axis cs:0.314999992959201,0.141929352248594)
% --(axis cs:0.319999992847443,0.144883022930397)
% --(axis cs:0.324999992735684,0.147866996680735)
% --(axis cs:0.329999992623925,0.150922012172414)
% --(axis cs:0.334999992512167,0.154015413803879)
% --(axis cs:0.339999992400408,0.157138003742365)
% --(axis cs:0.344999992288649,0.160320700672981)
% --(axis cs:0.34999999217689,0.163569127166642)
% --(axis cs:0.354999992065132,0.166803792500647)
% --(axis cs:0.359999991953373,0.17005880902664)
% --(axis cs:0.364999991841614,0.17337841714836)
% --(axis cs:0.369999991729856,0.176740578104524)
% --(axis cs:0.374999991618097,0.180065008068346)
% --(axis cs:0.379999991506338,0.183420187240154)
% --(axis cs:0.384999991394579,0.186842993798051)
% --(axis cs:0.389999991282821,0.19027679098263)
% --(axis cs:0.394999991171062,0.19365692335345)
% --(axis cs:0.399999991059303,0.197066645103535)
% --(axis cs:0.404999990947545,0.200532693225683)
% --(axis cs:0.409999990835786,0.203987211326878)
% --(axis cs:0.414999990724027,0.207390076622503)
% --(axis cs:0.419999990612268,0.210809042670906)
% --(axis cs:0.42499999050051,0.214265009620529)
% --(axis cs:0.429999990388751,0.217692004672694)
% --(axis cs:0.434999990276992,0.221060653173686)
% --(axis cs:0.439999990165234,0.22443459767659)
% --(axis cs:0.444999990053475,0.227842566772114)
% --(axis cs:0.449999989941716,0.231219303613149)
% --(axis cs:0.454999989829957,0.234539028396446)
% --(axis cs:0.459999989718199,0.237856219059607)
% --(axis cs:0.46499998960644,0.241199396628021)
% --(axis cs:0.469999989494681,0.244511696995495)
% --(axis cs:0.474999989382923,0.247775942063147)
% --(axis cs:0.479999989271164,0.251032512736893)
% --(axis cs:0.484999989159405,0.254305697231816)
% --(axis cs:0.489999989047647,0.257556838628418)
% --(axis cs:0.494999988935888,0.260755094948821)
% --(axis cs:0.494999988935888,0.341926402429029)
% --(axis cs:0.494999988935888,0.341926402429029)
% --(axis cs:0.489999989047647,0.338510900062983)
% --(axis cs:0.484999989159405,0.335035267459041)
% --(axis cs:0.479999989271164,0.331522407498773)
% --(axis cs:0.474999989382923,0.328003349630812)
% --(axis cs:0.469999989494681,0.324464654707762)
% --(axis cs:0.46499998960644,0.320864120864743)
% --(axis cs:0.459999989718199,0.317215283600589)
% --(axis cs:0.454999989829957,0.313567078846323)
% --(axis cs:0.449999989941716,0.30990457170794)
% --(axis cs:0.444999990053475,0.306189159276113)
% --(axis cs:0.439999990165234,0.30241491981555)
% --(axis cs:0.434999990276992,0.298633194248247)
% --(axis cs:0.429999990388751,0.294848089913116)
% --(axis cs:0.42499999050051,0.291014252387845)
% --(axis cs:0.419999990612268,0.287098815666206)
% --(axis cs:0.414999990724027,0.283173509660718)
% --(axis cs:0.409999990835786,0.279255053703552)
% --(axis cs:0.404999990947545,0.275307974699719)
% --(axis cs:0.399999991059303,0.27127141985542)
% --(axis cs:0.394999991171062,0.267225978365104)
% --(axis cs:0.389999991282821,0.26320793646448)
% --(axis cs:0.384999991394579,0.259174470227904)
% --(axis cs:0.379999991506338,0.25503223149251)
% --(axis cs:0.374999991618097,0.250877183710329)
% --(axis cs:0.369999991729856,0.246779445665621)
% --(axis cs:0.364999991841614,0.242696043935185)
% --(axis cs:0.359999991953373,0.238493908006504)
% --(axis cs:0.354999992065132,0.234279346372542)
% --(axis cs:0.34999999217689,0.230167962374849)
% --(axis cs:0.344999992288649,0.226099440006191)
% --(axis cs:0.339999992400408,0.221904005637417)
% --(axis cs:0.334999992512167,0.217678284378716)
% --(axis cs:0.329999992623925,0.213619485493408)
% --(axis cs:0.324999992735684,0.209624210894439)
% --(axis cs:0.319999992847443,0.205471327670699)
% --(axis cs:0.314999992959201,0.201280285624445)
% --(axis cs:0.30999999307096,0.197330456073162)
% --(axis cs:0.304999993182719,0.193441526603557)
% --(axis cs:0.299999993294477,0.18937817683882)
% --(axis cs:0.294999993406236,0.185264514245044)
% --(axis cs:0.289999993517995,0.181489606882163)
% --(axis cs:0.284999993629754,0.177750759890497)
% --(axis cs:0.279999993741512,0.173790036493232)
% --(axis cs:0.274999993853271,0.169789573569113)
% --(axis cs:0.26999999396503,0.166247751478426)
% --(axis cs:0.264999994076788,0.162768793100849)
% --(axis cs:0.259999994188547,0.159025680721607)
% --(axis cs:0.254999994300306,0.155347280358988)
% --(axis cs:0.249999994412065,0.152260099835455)
% --(axis cs:0.244999994523823,0.149190273958979)
% --(axis cs:0.239999994635582,0.145793489695186)
% --(axis cs:0.234999994747341,0.142542096644207)
% --(axis cs:0.229999994859099,0.139972099925327)
% --(axis cs:0.224999994970858,0.137322382463338)
% --(axis cs:0.219999995082617,0.134265362729042)
% --(axis cs:0.214999995194376,0.131470875989588)
% --(axis cs:0.209999995306134,0.129378018955632)
% --(axis cs:0.204999995417893,0.127174460606692)
% --(axis cs:0.199999995529652,0.124619924665411)
% --(axis cs:0.19499999564141,0.122422455832414)
% --(axis cs:0.189999995753169,0.120822463074719)
% --(axis cs:0.184999995864928,0.118911104789816)
% --(axis cs:0.179999995976686,0.116699219552803)
% --(axis cs:0.174999996088445,0.114935753558584)
% --(axis cs:0.169999996200204,0.113652990706122)
% --(axis cs:0.164999996311963,0.111993708139155)
% --(axis cs:0.159999996423721,0.110143421155643)
% --(axis cs:0.15499999653548,0.108778230390167)
% --(axis cs:0.149999996647239,0.107700326071263)
% --(axis cs:0.144999996758997,0.106186066160169)
% --(axis cs:0.139999996870756,0.104582624039567)
% --(axis cs:0.134999996982515,0.103534719472137)
% --(axis cs:0.129999997094274,0.102617021948427)
% --(axis cs:0.124999997206032,0.101249202477253)
% --(axis cs:0.119999997317791,0.0998579215377418)
% --(axis cs:0.11499999742955,0.0989267083577865)
% --(axis cs:0.109999997541308,0.0980004719223629)
% --(axis cs:0.104999997653067,0.0966184984930541)
% --(axis cs:0.0999999977648258,0.0952158256202922)
% --(axis cs:0.0949999978765845,0.0942467591825453)
% --(axis cs:0.0899999979883432,0.0931020253564953)
% --(axis cs:0.0849999981001019,0.0915806693264902)
% --(axis cs:0.0799999982118607,0.0902212214304113)
% --(axis cs:0.0749999983236194,0.089241773372161)
% --(axis cs:0.0699999984353781,0.0879697340637059)
% --(axis cs:0.0649999985471368,0.0863133557983032)
% --(axis cs:0.0599999986588955,0.0846183247504366)
% --(axis cs:0.0549999987706542,0.0837984260853516)
% --(axis cs:0.0499999988824129,0.0825995808862086)
% --(axis cs:0.0449999989941716,0.0811211853611831)
% --(axis cs:0.0399999991059303,0.0795671275704294)
% --(axis cs:0.034999999217689,0.0787810339459002)
% --(axis cs:0.0299999993294477,0.0769930293466132)
% --(axis cs:0.0249999994412065,0.0748628587053995)
% --(axis cs:0.0199999995529652,0.0735565321982417)
% --(axis cs:0.0149999996647239,0.0748216554187491)
% --(axis cs:0.00999999977648258,0.0777360300409083)
% --(axis cs:0.00499999988824129,0.0723257914846999)
% --cycle;

% \path [fill=white!50.1960784313725!black, fill opacity=0.4, ultra thick]
% (axis cs:0.00499999988824129,0.0717130428605083)
% --(axis cs:0.00499999988824129,0.0479423620231686)
% --(axis cs:0.00999999977648258,0.0545217469628543)
% --(axis cs:0.0149999996647239,0.0550003746788291)
% --(axis cs:0.0199999995529652,0.0544554062637262)
% --(axis cs:0.0249999994412065,0.0563242272400719)
% --(axis cs:0.0299999993294477,0.0585527093342239)
% --(axis cs:0.034999999217689,0.0598958804710367)
% --(axis cs:0.0399999991059303,0.0609020837733752)
% --(axis cs:0.0449999989941716,0.0622297278214893)
% --(axis cs:0.0499999988824129,0.0635801774965467)
% --(axis cs:0.0549999987706542,0.0644275561573345)
% --(axis cs:0.0599999986588955,0.0650691824181672)
% --(axis cs:0.0649999985471368,0.0661175948923066)
% --(axis cs:0.0699999984353781,0.0674021507333243)
% --(axis cs:0.0749999983236194,0.0682795717863606)
% --(axis cs:0.0799999982118607,0.0689160373934828)
% --(axis cs:0.0849999981001019,0.0698269230203977)
% --(axis cs:0.0899999979883432,0.0709013929213666)
% --(axis cs:0.0949999978765845,0.0718145240580949)
% --(axis cs:0.0999999977648258,0.0725894509359476)
% --(axis cs:0.104999997653067,0.0735822090961512)
% --(axis cs:0.109999997541308,0.0745890059825799)
% --(axis cs:0.11499999742955,0.0753541678872109)
% --(axis cs:0.119999997317791,0.0760601799340242)
% --(axis cs:0.124999997206032,0.0769474359961481)
% --(axis cs:0.129999997094274,0.0778587237631285)
% --(axis cs:0.134999996982515,0.0786547537650245)
% --(axis cs:0.139999996870756,0.0793650287638424)
% --(axis cs:0.144999996758997,0.0802308613670677)
% --(axis cs:0.149999996647239,0.0811935689325096)
% --(axis cs:0.15499999653548,0.0820134393549197)
% --(axis cs:0.159999996423721,0.0827706081734575)
% --(axis cs:0.164999996311963,0.0837738538613493)
% --(axis cs:0.169999996200204,0.0848324726039726)
% --(axis cs:0.174999996088445,0.0857808426125378)
% --(axis cs:0.179999995976686,0.0867567227984275)
% --(axis cs:0.184999995864928,0.0880742980425841)
% --(axis cs:0.189999995753169,0.0894710984513577)
% --(axis cs:0.19499999564141,0.0908225610703488)
% --(axis cs:0.199999995529652,0.0923327849656376)
% --(axis cs:0.204999995417893,0.0941165061536277)
% --(axis cs:0.209999995306134,0.0959291803023438)
% --(axis cs:0.214999995194376,0.0976681712591969)
% --(axis cs:0.219999995082617,0.099592106606057)
% --(axis cs:0.224999994970858,0.101733079106683)
% --(axis cs:0.229999994859099,0.103862121802528)
% --(axis cs:0.234999994747341,0.10585240012953)
% --(axis cs:0.239999994635582,0.108132051708598)
% --(axis cs:0.244999994523823,0.110536660945738)
% --(axis cs:0.249999994412065,0.112951932752745)
% --(axis cs:0.254999994300306,0.115204100610966)
% --(axis cs:0.259999994188547,0.117763382724385)
% --(axis cs:0.264999994076788,0.120400274598243)
% --(axis cs:0.26999999396503,0.123051609098941)
% --(axis cs:0.274999993853271,0.125579609739125)
% --(axis cs:0.279999993741512,0.128408085479573)
% --(axis cs:0.284999993629754,0.131261065036432)
% --(axis cs:0.289999993517995,0.134129989205288)
% --(axis cs:0.294999993406236,0.13688267540486)
% --(axis cs:0.299999993294477,0.139913443167068)
% --(axis cs:0.304999993182719,0.142999359302441)
% --(axis cs:0.30999999307096,0.146096264125586)
% --(axis cs:0.314999992959201,0.149126074335531)
% --(axis cs:0.319999992847443,0.152378719109889)
% --(axis cs:0.324999992735684,0.155682578173698)
% --(axis cs:0.329999992623925,0.15897858085942)
% --(axis cs:0.334999992512167,0.162239120484111)
% --(axis cs:0.339999992400408,0.165653774406453)
% --(axis cs:0.344999992288649,0.169117883750487)
% --(axis cs:0.34999999217689,0.172558855076731)
% --(axis cs:0.354999992065132,0.175973118870107)
% --(axis cs:0.359999991953373,0.179484344402664)
% --(axis cs:0.364999991841614,0.183032952829621)
% --(axis cs:0.369999991729856,0.18656258677443)
% --(axis cs:0.374999991618097,0.190071425919554)
% --(axis cs:0.379999991506338,0.193633851851779)
% --(axis cs:0.384999991394579,0.197228757175838)
% --(axis cs:0.389999991282821,0.200806622830147)
% --(axis cs:0.394999991171062,0.204351485806873)
% --(axis cs:0.399999991059303,0.207929588215637)
% --(axis cs:0.404999990947545,0.211528693336554)
% --(axis cs:0.409999990835786,0.215119514108756)
% --(axis cs:0.414999990724027,0.218666949895898)
% --(axis cs:0.419999990612268,0.222214109143622)
% --(axis cs:0.42499999050051,0.225766267661877)
% --(axis cs:0.429999990388751,0.229314162847539)
% --(axis cs:0.434999990276992,0.232810772764882)
% --(axis cs:0.439999990165234,0.236291532488447)
% --(axis cs:0.444999990053475,0.239765927455225)
% --(axis cs:0.449999989941716,0.243247528144637)
% --(axis cs:0.454999989829957,0.246680589819622)
% --(axis cs:0.459999989718199,0.250073234763564)
% --(axis cs:0.46499998960644,0.253462744299809)
% --(axis cs:0.469999989494681,0.25685844865005)
% --(axis cs:0.474999989382923,0.260207185306575)
% --(axis cs:0.479999989271164,0.263519132805804)
% --(axis cs:0.484999989159405,0.266830835836301)
% --(axis cs:0.489999989047647,0.270152339463855)
% --(axis cs:0.494999988935888,0.273426411991371)
% --(axis cs:0.494999988935888,0.349083688898173)
% --(axis cs:0.494999988935888,0.349083688898173)
% --(axis cs:0.489999989047647,0.345670997645619)
% --(axis cs:0.484999989159405,0.342226387022885)
% --(axis cs:0.479999989271164,0.33874835703001)
% --(axis cs:0.474999989382923,0.335247415517636)
% --(axis cs:0.469999989494681,0.331701272603454)
% --(axis cs:0.46499998960644,0.328122944434829)
% --(axis cs:0.459999989718199,0.324506155452288)
% --(axis cs:0.454999989829957,0.320888767586842)
% --(axis cs:0.449999989941716,0.317223707342547)
% --(axis cs:0.444999990053475,0.313515463006913)
% --(axis cs:0.439999990165234,0.309774295233777)
% --(axis cs:0.434999990276992,0.306025274830068)
% --(axis cs:0.429999990388751,0.302226545148903)
% --(axis cs:0.42499999050051,0.29837651404755)
% --(axis cs:0.419999990612268,0.294491827579123)
% --(axis cs:0.414999990724027,0.290596686974282)
% --(axis cs:0.409999990835786,0.286672087604551)
% --(axis cs:0.404999990947545,0.282690339648468)
% --(axis cs:0.399999991059303,0.278674479889772)
% --(axis cs:0.394999991171062,0.274638871434317)
% --(axis cs:0.389999991282821,0.270589285872698)
% --(axis cs:0.384999991394579,0.266487781900841)
% --(axis cs:0.379999991506338,0.262365852605217)
% --(axis cs:0.374999991618097,0.258220544620302)
% --(axis cs:0.369999991729856,0.254079846352938)
% --(axis cs:0.364999991841614,0.249902609588789)
% --(axis cs:0.359999991953373,0.245721374016094)
% --(axis cs:0.354999992065132,0.24150687159973)
% --(axis cs:0.34999999217689,0.237330055455407)
% --(axis cs:0.344999992288649,0.233147742249853)
% --(axis cs:0.339999992400408,0.228981961207176)
% --(axis cs:0.334999992512167,0.224763729696106)
% --(axis cs:0.329999992623925,0.220613444180788)
% --(axis cs:0.324999992735684,0.216525358412039)
% --(axis cs:0.319999992847443,0.212433986269763)
% --(axis cs:0.314999992959201,0.208240605728379)
% --(axis cs:0.30999999307096,0.204141408887456)
% --(axis cs:0.304999993182719,0.200151170579539)
% --(axis cs:0.299999993294477,0.196131415591675)
% --(axis cs:0.294999993406236,0.192012039335615)
% --(axis cs:0.289999993517995,0.1880386661517)
% --(axis cs:0.284999993629754,0.184291709820745)
% --(axis cs:0.279999993741512,0.18039816794208)
% --(axis cs:0.274999993853271,0.176341350610355)
% --(axis cs:0.26999999396503,0.172505554402672)
% --(axis cs:0.264999994076788,0.1689867837134)
% --(axis cs:0.259999994188547,0.165278824728154)
% --(axis cs:0.254999994300306,0.161475135822998)
% --(axis cs:0.249999994412065,0.158038054083306)
% --(axis cs:0.244999994523823,0.154993651136215)
% --(axis cs:0.239999994635582,0.151595511597343)
% --(axis cs:0.234999994747341,0.148153450009759)
% --(axis cs:0.229999994859099,0.145255843126663)
% --(axis cs:0.224999994970858,0.142697694914994)
% --(axis cs:0.219999995082617,0.139637457711652)
% --(axis cs:0.214999995194376,0.136618011644152)
% --(axis cs:0.209999995306134,0.134338425813371)
% --(axis cs:0.204999995417893,0.132196205095746)
% --(axis cs:0.199999995529652,0.129554138709648)
% --(axis cs:0.19499999564141,0.12709280731082)
% --(axis cs:0.189999995753169,0.125415317579282)
% --(axis cs:0.184999995864928,0.123567233546952)
% --(axis cs:0.179999995976686,0.121274711674759)
% --(axis cs:0.174999996088445,0.119327692575696)
% --(axis cs:0.169999996200204,0.118109646300884)
% --(axis cs:0.164999996311963,0.116463362822477)
% --(axis cs:0.159999996423721,0.114493584065053)
% --(axis cs:0.15499999653548,0.112963372538152)
% --(axis cs:0.149999996647239,0.111993262722908)
% --(axis cs:0.144999996758997,0.110506304616588)
% --(axis cs:0.139999996870756,0.108849474354826)
% --(axis cs:0.134999996982515,0.107768637398986)
% --(axis cs:0.129999997094274,0.107013481427831)
% --(axis cs:0.124999997206032,0.105702644121307)
% --(axis cs:0.119999997317791,0.10433527759536)
% --(axis cs:0.11499999742955,0.10353048258254)
% --(axis cs:0.109999997541308,0.102744199304688)
% --(axis cs:0.104999997653067,0.101416892564622)
% --(axis cs:0.0999999977648258,0.100046001683656)
% --(axis cs:0.0949999978765845,0.0991062162541207)
% --(axis cs:0.0899999979883432,0.0979210694992463)
% --(axis cs:0.0849999981001019,0.0962776138187348)
% --(axis cs:0.0799999982118607,0.0946657160670327)
% --(axis cs:0.0749999983236194,0.0933097306728568)
% --(axis cs:0.0699999984353781,0.0916069767012315)
% --(axis cs:0.0649999985471368,0.0896009924358052)
% --(axis cs:0.0599999986588955,0.0876074121237368)
% --(axis cs:0.0549999987706542,0.0865720318094755)
% --(axis cs:0.0499999988824129,0.0850385253058287)
% --(axis cs:0.0449999989941716,0.0835224054091462)
% --(axis cs:0.0399999991059303,0.0815473239455492)
% --(axis cs:0.034999999217689,0.0802732282341523)
% --(axis cs:0.0299999993294477,0.077842820206363)
% --(axis cs:0.0249999994412065,0.075286150444266)
% --(axis cs:0.0199999995529652,0.0739858239094146)
% --(axis cs:0.0149999996647239,0.0748448027177378)
% --(axis cs:0.00999999977648258,0.077868551452679)
% --(axis cs:0.00499999988824129,0.0717130428605083)
% --cycle;

% \addplot [ultra thick, blue]
% table {%
% 0.00499999523162842 0.0891090780496597
% 0.00999999046325684 0.0958595350384712
% 0.0149999856948853 0.098928190767765
% 0.0199999809265137 0.102203704416752
% 0.0299999713897705 0.112459667026997
% 0.0349999666213989 0.117255419492722
% 0.0399999618530273 0.121325097978115
% 0.0449999570846558 0.125203624367714
% 0.0499999523162842 0.128394305706024
% 0.0549999475479126 0.131109476089478
% 0.059999942779541 0.133464381098747
% 0.065000057220459 0.136118590831757
% 0.0700000524520874 0.138669177889824
% 0.0850000381469727 0.146147802472115
% 0.0900000333786011 0.148739218711853
% 0.0950000286102295 0.151279717683792
% 0.110000014305115 0.158712238073349
% 0.115000009536743 0.161001145839691
% 0.125 0.165371686220169
% 0.129999995231628 0.167472586035728
% 0.134999990463257 0.16946716606617
% 0.144999980926514 0.173291370272636
% 0.154999971389771 0.177021160721779
% 0.184999942779541 0.188334137201309
% 0.194999933242798 0.192508980631828
% 0.205000042915344 0.197013854980469
% 0.215000033378601 0.201805919408798
% 0.225000023841858 0.206858426332474
% 0.254999995231628 0.222981944680214
% 0.269999980926514 0.231298178434372
% 0.279999971389771 0.236777037382126
% 0.289999961853027 0.242112904787064
% 0.299999952316284 0.247309640049934
% 0.309999942779541 0.252508372068405
% 0.319999933242798 0.257585674524307
% 0.329999923706055 0.262585371732712
% 0.345000028610229 0.269916087388992
% 0.360000014305115 0.277185469865799
% 0.375 0.284501850605011
% 0.389999985694885 0.291766494512558
% 0.404999971389771 0.298893481492996
% 0.414999961853027 0.303589135408401
% 0.424999952316284 0.308180928230286
% 0.434999942779541 0.312623143196106
% 0.450000047683716 0.319094717502594
% 0.465000033378601 0.325331509113312
% 0.480000019073486 0.33146995306015
% 0.495000004768372 0.337417215108871
% };
% \addlegendentry{No si.}
% \addplot [ultra thick, red]
% table {%
% 0.00499999523162842 0.0965440645813942
% 0.00999999046325684 0.101374782621861
% 0.0149999856948853 0.103267908096313
% 0.0199999809265137 0.105385564267635
% 0.0249999761581421 0.109322763979435
% 0.0299999713897705 0.113240383565426
% 0.0349999666213989 0.116591677069664
% 0.0399999618530273 0.119413174688816
% 0.0449999570846558 0.122503362596035
% 0.0499999523162842 0.125194042921066
% 0.0549999475479126 0.127751260995865
% 0.059999942779541 0.130017086863518
% 0.065000057220459 0.132728382945061
% 0.0700000524520874 0.135204002261162
% 0.0750000476837158 0.137427806854248
% 0.0800000429153442 0.139423504471779
% 0.0850000381469727 0.141525059938431
% 0.0900000333786011 0.143417656421661
% 0.0950000286102295 0.145093321800232
% 0.105000019073486 0.148135304450989
% 0.110000014305115 0.149539217352867
% 0.115000009536743 0.150790438055992
% 0.120000004768372 0.151922807097435
% 0.125 0.153145298361778
% 0.129999995231628 0.154303312301636
% 0.134999990463257 0.155367985367775
% 0.144999980926514 0.157433807849884
% 0.190000057220459 0.167081922292709
% 0.210000038146973 0.171424046158791
% 0.245000004768372 0.179823651909828
% 0.254999995231628 0.18237242102623
% 0.284999966621399 0.190000176429749
% 0.309999942779541 0.196244537830353
% 0.329999923706055 0.200915440917015
% 0.355000019073486 0.206765726208687
% 0.365000009536743 0.209104746580124
% 0.389999985694885 0.214994698762894
% 0.399999976158142 0.217298209667206
% 0.409999966621399 0.21949003636837
% 0.419999957084656 0.221558630466461
% 0.429999947547913 0.223552018404007
% 0.444999933242798 0.226285979151726
% 0.454999923706055 0.228041112422943
% 0.495000004768372 0.234868139028549
% };
% \addlegendentry{Si 1}
% \addplot [ultra thick, green!50.1960784313725!black]
% table {%
% 0.00499999523162842 0.0762640386819839
% 0.0149999856948853 0.0808437243103981
% 0.0199999809265137 0.0833111777901649
% 0.0249999761581421 0.0863811075687408
% 0.0299999713897705 0.0899804532527924
% 0.0349999666213989 0.0930423885583878
% 0.0399999618530273 0.0950435847043991
% 0.0449999570846558 0.0974984765052795
% 0.0499999523162842 0.100365601480007
% 0.0549999475479126 0.102854825556278
% 0.059999942779541 0.104729406535625
% 0.0700000524520874 0.109711572527885
% 0.0750000476837158 0.111741788685322
% 0.0800000429153442 0.113204643130302
% 0.0850000381469727 0.114989511668682
% 0.0900000333786011 0.116876855492592
% 0.0950000286102295 0.118166506290436
% 0.100000023841858 0.119093850255013
% 0.110000014305115 0.121919028460979
% 0.120000004768372 0.123437598347664
% 0.129999995231628 0.126216486096382
% 0.134999990463257 0.12707494199276
% 0.139999985694885 0.128148689866066
% 0.144999980926514 0.129782646894455
% 0.149999976158142 0.131310299038887
% 0.154999971389771 0.132327526807785
% 0.159999966621399 0.133693471550941
% 0.164999961853027 0.135696887969971
% 0.169999957084656 0.13756088912487
% 0.174999952316284 0.139045402407646
% 0.179999947547913 0.140985891222954
% 0.184999942779541 0.143474742770195
% 0.190000057220459 0.145744830369949
% 0.194999933242798 0.14761583507061
% 0.200000047683716 0.150161013007164
% 0.205000042915344 0.153169795870781
% 0.210000038146973 0.155846834182739
% 0.215000033378601 0.158390268683434
% 0.220000028610229 0.161584883928299
% 0.225000023841858 0.165127739310265
% 0.230000019073486 0.168320551514626
% 0.235000014305115 0.171409741044044
% 0.245000004768372 0.179015681147575
% 0.254999995231628 0.186220556497574
% 0.264999985694885 0.194478422403336
% 0.274999976158142 0.202374890446663
% 0.284999966621399 0.210999056696892
% 0.305000066757202 0.228123500943184
% 0.319999933242798 0.241139009594917
% 0.325000047683716 0.245601564645767
% 0.335000038146973 0.254294574260712
% 0.345000028610229 0.263153791427612
% 0.355000019073486 0.271836221218109
% 0.365000009536743 0.280563831329346
% 0.375 0.289129078388214
% 0.384999990463257 0.29763650894165
% 0.394999980926514 0.305963665246964
% 0.404999971389771 0.314184933900833
% 0.414999961853027 0.322247594594955
% 0.424999952316284 0.330140948295593
% 0.434999942779541 0.337882846593857
% 0.444999933242798 0.345434993505478
% 0.454999923706055 0.352878302335739
% 0.470000028610229 0.363718301057816
% 0.480000019073486 0.370758056640625
% 0.495000004768372 0.381092995405197
% };
% \addlegendentry{Si 2}
% \addplot [ultra thick, color0]
% table {%
% 0.00499999523162842 0.058377593755722
% 0.00999999046325684 0.0658384785056114
% 0.0149999856948853 0.0640234425663948
% 0.0199999809265137 0.0633455291390419
% 0.0249999761581421 0.0649960860610008
% 0.0299999713897705 0.0670813769102097
% 0.0349999666213989 0.0688057765364647
% 0.0399999618530273 0.0697651132941246
% 0.0449999570846558 0.071412019431591
% 0.0499999523162842 0.0730286166071892
% 0.0549999475479126 0.0742233172059059
% 0.059999942779541 0.0750251188874245
% 0.065000057220459 0.0763782113790512
% 0.0700000524520874 0.077868714928627
% 0.0750000476837158 0.0789938271045685
% 0.0800000429153442 0.0798509269952774
% 0.0850000381469727 0.0809958502650261
% 0.0900000333786011 0.0822604671120644
% 0.0950000286102295 0.0831665322184563
% 0.100000023841858 0.0839678272604942
% 0.110000014305115 0.0861777439713478
% 0.120000004768372 0.0876220911741257
% 0.129999995231628 0.0897318795323372
% 0.134999990463257 0.090481773018837
% 0.139999985694885 0.0912964418530464
% 0.149999976158142 0.0936672016978264
% 0.154999971389771 0.09452835470438
% 0.159999966621399 0.095587745308876
% 0.164999961853027 0.096985749900341
% 0.169999957084656 0.0982641652226448
% 0.174999952316284 0.0993108674883842
% 0.179999947547913 0.100710168480873
% 0.184999942779541 0.102440416812897
% 0.190000057220459 0.103995457291603
% 0.194999933242798 0.105416551232338
% 0.200000047683716 0.107277646660805
% 0.205000042915344 0.109376065433025
% 0.215000033378601 0.113119408488274
% 0.220000028610229 0.115459501743317
% 0.225000023841858 0.117949709296227
% 0.235000014305115 0.122463181614876
% 0.245000004768372 0.127953127026558
% 0.254999995231628 0.13319618999958
% 0.264999985694885 0.139245584607124
% 0.274999976158142 0.145126432180405
% 0.284999966621399 0.151626512408257
% 0.294999957084656 0.157975301146507
% 0.305000066757202 0.164807602763176
% 0.329999923706055 0.182270720601082
% 0.345000028610229 0.19321009516716
% 0.360000014305115 0.204276353120804
% 0.370000004768372 0.211759999394417
% 0.384999990463257 0.223008751869202
% 0.394999980926514 0.230441465973854
% 0.404999971389771 0.23792028427124
% 0.414999961853027 0.24528181552887
% 0.424999952316284 0.252639621496201
% 0.434999942779541 0.259846895933151
% 0.444999933242798 0.267015844583511
% 0.454999923706055 0.274053037166595
% 0.465000033378601 0.281031757593155
% 0.475000023841858 0.287889689207077
% 0.485000014305115 0.29467049241066
% 0.495000004768372 0.301340788602829
% };
% \addlegendentry{Si 3}
% \addplot [ultra thick, white!50.1960784313725!black]
% table {%
% 0.00499999523162842 0.0598277002573013
% 0.00999999046325684 0.0661951526999474
% 0.0149999856948853 0.0649225860834122
% 0.0199999809265137 0.0642206072807312
% 0.0249999761581421 0.065805196762085
% 0.0299999713897705 0.0681977644562721
% 0.0349999666213989 0.0700845494866371
% 0.0399999618530273 0.0712246969342232
% 0.0449999570846558 0.0728760734200478
% 0.0499999523162842 0.0743093490600586
% 0.0549999475479126 0.0754997953772545
% 0.059999942779541 0.0763383060693741
% 0.065000057220459 0.0778592899441719
% 0.0700000524520874 0.0795045644044876
% 0.0750000476837158 0.0807946473360062
% 0.0800000429153442 0.0817908719182014
% 0.0850000381469727 0.0830522626638412
% 0.0900000333786011 0.0844112187623978
% 0.0950000286102295 0.0854603871703148
% 0.100000023841858 0.0863177254796028
% 0.110000014305115 0.0886666104197502
% 0.120000004768372 0.0901977196335793
% 0.129999995231628 0.0924361050128937
% 0.134999990463257 0.0932116881012917
% 0.139999985694885 0.0941072404384613
% 0.144999980926514 0.0953686013817787
% 0.149999976158142 0.0965934246778488
% 0.154999971389771 0.0974884107708931
% 0.159999966621399 0.0986321046948433
% 0.164999961853027 0.100118592381477
% 0.169999957084656 0.101471051573753
% 0.174999952316284 0.102554246783257
% 0.179999947547913 0.104015700519085
% 0.184999942779541 0.105820775032043
% 0.190000057220459 0.107443206012249
% 0.194999933242798 0.108957692980766
% 0.200000047683716 0.1109434440732
% 0.205000042915344 0.113156363368034
% 0.215000033378601 0.117143116891384
% 0.225000023841858 0.122215390205383
% 0.235000014305115 0.127002909779549
% 0.245000004768372 0.132765144109726
% 0.254999995231628 0.138339638710022
% 0.264999985694885 0.14469350874424
% 0.274999976158142 0.150960490107536
% 0.279999971389771 0.154403120279312
% 0.284999966621399 0.157776355743408
% 0.294999957084656 0.164447352290154
% 0.305000066757202 0.171575248241425
% 0.325000047683716 0.186103954911232
% 0.340000033378601 0.197317898273468
% 0.350000023841858 0.204944476485252
% 0.365000009536743 0.21646773815155
% 0.375 0.224145993590355
% 0.384999990463257 0.231858253479004
% 0.394999980926514 0.239495187997818
% 0.404999971389771 0.247109532356262
% 0.414999961853027 0.254631787538528
% 0.424999952316284 0.262071371078491
% 0.434999942779541 0.269418001174927
% 0.444999933242798 0.276640653610229
% 0.454999923706055 0.283784717321396
% 0.465000033378601 0.290792852640152
% 0.475000023841858 0.297727286815643
% 0.485000014305115 0.304528564214706
% 0.495000004768372 0.311255037784576
% };
% \addlegendentry{Si 4}

==> supp_mat/fetch_plots/traj_err_data.tex <==
\path [fill=red, fill opacity=0.4, ultra thick]
(axis cs:1,0.450832588657663)
--(axis cs:1,0.342277254094566)
--(axis cs:10,0.193951732104943)
--(axis cs:25,0.150299187024981)
--(axis cs:75,0.139574592806006)
--(axis cs:200,0.127053163665148)
--(axis cs:500,0.12671936290503)
--(axis cs:500,0.173708148227355)
--(axis cs:500,0.173708148227355)
--(axis cs:200,0.153499872891358)
--(axis cs:75,0.175308678055132)
--(axis cs:25,0.200064418380496)
--(axis cs:10,0.242821759343827)
--(axis cs:1,0.450832588657663)
--cycle;

\path [fill=green!50.1960784313725!black, fill opacity=0.4, ultra thick]
(axis cs:1,0.470060717754753)
--(axis cs:1,0.349116601596732)
--(axis cs:10,0.128702420635964)
--(axis cs:25,0.103147952468473)
--(axis cs:75,0.0909859729168512)
--(axis cs:200,0.0821552220450362)
--(axis cs:500,0.0887728774389657)
--(axis cs:500,0.123950443219074)
--(axis cs:500,0.123950443219074)
--(axis cs:200,0.105308444634118)
--(axis cs:75,0.1225136292467)
--(axis cs:25,0.146719670927311)
--(axis cs:10,0.183442881853881)
--(axis cs:1,0.470060717754753)
--cycle;

\path [fill=color0, fill opacity=0.4, ultra thick]
(axis cs:1,0.460758098853286)
--(axis cs:1,0.332549681437606)
--(axis cs:10,0.104416636058916)
--(axis cs:25,0.0929826811626782)
--(axis cs:75,0.0840021843585121)
--(axis cs:200,0.0737448759121545)
--(axis cs:500,0.0693265017147747)
--(axis cs:500,0.0930321786056807)
--(axis cs:500,0.0930321786056807)
--(axis cs:200,0.0942462047210047)
--(axis cs:75,0.107495555657725)
--(axis cs:25,0.119711127995211)
--(axis cs:10,0.131280766537419)
--(axis cs:1,0.460758098853286)
--cycle;

\path [fill=white!40!black, fill opacity=0.4, ultra thick]
(axis cs:1,0.457690971213657)
--(axis cs:1,0.329526233032621)
--(axis cs:10,0.103653766848593)
--(axis cs:25,0.0935290442563888)
--(axis cs:75,0.0827389188560648)
--(axis cs:200,0.075193272762717)
--(axis cs:500,0.073899063733729)
--(axis cs:500,0.098851571947577)
--(axis cs:500,0.098851571947577)
--(axis cs:200,0.0969252035812792)
--(axis cs:75,0.100867508333778)
--(axis cs:25,0.134153717115168)
--(axis cs:10,0.131659006313328)
--(axis cs:1,0.457690971213657)
--cycle;

\addplot [ultra thick, red, mark=*, mark size=1.5, mark options={solid}]
table {%
1 0.396554887294769
10 0.218386724591255
25 0.175181820988655
75 0.157441630959511
200 0.140276536345482
500 0.150213733315468
};
% \addlegendentry{No si.}
\addplot [ultra thick, green!50.1960784313725!black, mark=asterisk, mark size=1.5, mark options={solid}]
table {%
1 0.409588694572449
10 0.156072616577148
25 0.124933794140816
75 0.106749795377254
200 0.0937318354845047
500 0.106361664831638
};
% \addlegendentry{Si 2}
\addplot [ultra thick, color0, mark=*, mark size=1.5, mark options={solid}]
table {%
1 0.396653860807419
10 0.117848709225655
25 0.106346897780895
75 0.0957488790154457
200 0.0839955359697342
500 0.0811793431639671
};
% \addlegendentry{si 3}
\addplot [ultra thick, white!40!black, mark=*, mark size=1.5, mark options={solid}]
table {%
1 0.393608659505844
10 0.117656394839287
25 0.113841384649277
75 0.0918032079935074
200 0.0860592424869537
500 0.0863753259181976
};
% \addlegendentry{si 4}

==> supp_mat/humanoid_plots/constraint_loss_data.tex <==
\path [fill=color0, fill opacity=0.4, ultra thick]
(axis cs:0,5223.42333984375)
--(axis cs:0,1456.70703125)
--(axis cs:100,1457.14331054688)
--(axis cs:200,1455.37463378906)
--(axis cs:300,557.868896484375)
--(axis cs:400,617.975952148438)
--(axis cs:500,695.533813476562)
--(axis cs:600,57.2175788879395)
--(axis cs:700,617.562866210938)
--(axis cs:800,683.730834960938)
--(axis cs:900,717.829711914062)
--(axis cs:1000,898.556640625)
--(axis cs:1100,1187.13903808594)
--(axis cs:1200,1202.84143066406)
--(axis cs:1300,1389.24645996094)
--(axis cs:1400,1409.875)
--(axis cs:1500,1507.22302246094)
--(axis cs:1600,2015.07971191406)
--(axis cs:1600,5391.03759765625)
--(axis cs:1600,5391.03759765625)
--(axis cs:1500,8856.5546875)
--(axis cs:1400,8659.91796875)
--(axis cs:1300,8451.9052734375)
--(axis cs:1200,8276.607421875)
--(axis cs:1100,8233.419921875)
--(axis cs:1000,7407.00146484375)
--(axis cs:900,7061.953125)
--(axis cs:800,4261.2734375)
--(axis cs:700,4154.76220703125)
--(axis cs:600,4034.8134765625)
--(axis cs:500,4255.35595703125)
--(axis cs:400,4237.27294921875)
--(axis cs:300,4240.666015625)
--(axis cs:200,5221.0107421875)
--(axis cs:100,5223.4228515625)
--(axis cs:0,5223.42333984375)
--cycle;

\path [fill=white!40.1960784313725!black, fill opacity=0.4, ultra thick]
(axis cs:0,14.111156463623)
--(axis cs:0,7.47982849134132e-05)
--(axis cs:100,7.2385802923236e-05)
--(axis cs:200,7.23291959729977e-05)
--(axis cs:300,7.23291959729977e-05)
--(axis cs:400,7.23291959729977e-05)
--(axis cs:500,7.23291959729977e-05)
--(axis cs:600,7.23291959729977e-05)
--(axis cs:700,7.23291595932096e-05)
--(axis cs:800,7.19058007234707e-05)
--(axis cs:900,7.19058007234707e-05)
--(axis cs:1000,0)
--(axis cs:1100,0)
--(axis cs:1200,0)
--(axis cs:1300,0)
--(axis cs:1400,0)
--(axis cs:1500,0)
--(axis cs:1600,0)
--(axis cs:1600,0.000755777466110885)
--(axis cs:1600,0.000755777466110885)
--(axis cs:1500,0.000755777466110885)
--(axis cs:1400,0.000755777466110885)
--(axis cs:1300,0.000777501205448061)
--(axis cs:1200,0.000858554907608777)
--(axis cs:1100,0.102439239621162)
--(axis cs:1000,0.102252602577209)
--(axis cs:900,0.102258905768394)
--(axis cs:800,0.102342382073402)
--(axis cs:700,0.102342419326305)
--(axis cs:600,0.101785019040108)
--(axis cs:500,0.101785019040108)
--(axis cs:400,14.2128505706787)
--(axis cs:300,14.2128276824951)
--(axis cs:200,14.2127466201782)
--(axis cs:100,14.1111545562744)
--(axis cs:0,14.111156463623)
--cycle;

\addplot [ultra thick, color0]
table {%
0 3340.064453125
200 3338.19287109375
300 2399.26806640625
400 2427.6240234375
500 2475.4443359375
600 1772.1611328125
700 2114.14135742188
800 2240.84790039062
900 3416.64111328125
1000 3819.67358398438
1100 4368.2060546875
1200 4427.52783203125
1300 4642.56591796875
1500 4868.39208984375
1600 3703.05883789062
};
\addplot [ultra thick, white!66.2745098039216!black]
table {%
0 5.84526538848877
100 5.84526348114014
200 5.8873438835144
400 5.8873872756958
500 0.04239222407341
600 0.04239222407341
700 0.0426875613629818
800 0.0426874347031116
900 0.0424427315592766
1100 0.0424983836710453
1200 0.000418209296185523
1300 0.000384131184546277
1400 0.000374975992599502
1600 0.000374975992599502
};


==> supp_mat/humanoid_plots/geomrelerr.tex <==
% This file was created with tikzplotlib v0.9.12.
\begin{tikzpicture}

\definecolor{color0}{rgb}{1,0,1}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
log basis y={10},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={\(\displaystyle \mathrm{Number \ of \ training \ trajectories }\)},
xmajorgrids,
xmin=-23.95, xmax=524.95,
xtick style={color=black},
y grid style={white!69.0196078431373!black},
ylabel={\(\displaystyle \mathrm{Geometric \ mean \ of \ relative \ error }\)},
ymajorgrids,
ymin=0.112838589141192, ymax=0.684740490837029,
ymode=log,
ytick style={color=black}
]
\path [fill=blue, fill opacity=0.4, semithick]
(axis cs:1,0.541743363602843)
--(axis cs:1,0.449112071455718)
--(axis cs:10,0.222851933182839)
--(axis cs:25,0.218278809800564)
--(axis cs:75,0.203373653824151)
--(axis cs:200,0.202344693428683)
--(axis cs:500,0.205319745054706)
--(axis cs:500,0.24492664882946)
--(axis cs:500,0.24492664882946)
--(axis cs:200,0.239061668396655)
--(axis cs:75,0.260088453237498)
--(axis cs:25,0.255254397050033)
--(axis cs:10,0.273922619095674)
--(axis cs:1,0.541743363602843)
--cycle;

\path [fill=red, fill opacity=0.4, semithick]
(axis cs:1,0.531010585830433)
--(axis cs:1,0.459758101681661)
--(axis cs:10,0.229730335009316)
--(axis cs:25,0.191273754876949)
--(axis cs:75,0.175796832901461)
--(axis cs:200,0.164071554922007)
--(axis cs:500,0.170048621804538)
--(axis cs:500,0.202470236594375)
--(axis cs:500,0.202470236594375)
--(axis cs:200,0.206555843340007)
--(axis cs:75,0.231836704110698)
--(axis cs:25,0.224161883102382)
--(axis cs:10,0.27300405791108)
--(axis cs:1,0.531010585830433)
--cycle;

\path [fill=green!50.1960784313725!black, fill opacity=0.4, semithick]
(axis cs:1,0.327037261321266)
--(axis cs:1,0.271321338504818)
--(axis cs:10,0.153216160419598)
--(axis cs:25,0.162110887475575)
--(axis cs:75,0.14101120413756)
--(axis cs:200,0.131378655409453)
--(axis cs:500,0.133331697770542)
--(axis cs:500,0.172200606977037)
--(axis cs:500,0.172200606977037)
--(axis cs:200,0.160043838253535)
--(axis cs:75,0.165050957437437)
--(axis cs:25,0.196078888437663)
--(axis cs:10,0.187416813983647)
--(axis cs:1,0.327037261321266)
--cycle;

\path [fill=color0, fill opacity=0.4, semithick]
(axis cs:1,0.282463641182809)
--(axis cs:1,0.246882484426964)
--(axis cs:10,0.161905684649898)
--(axis cs:25,0.148348927125901)
--(axis cs:75,0.129090951546991)
--(axis cs:200,0.124358420615673)
--(axis cs:500,0.122476188880835)
--(axis cs:500,0.152916463115796)
--(axis cs:500,0.152916463115796)
--(axis cs:200,0.18128134913412)
--(axis cs:75,0.160261962288737)
--(axis cs:25,0.189036696377846)
--(axis cs:10,0.189963946263115)
--(axis cs:1,0.282463641182809)
--cycle;

\path [fill=white!50.1960784313725!black, fill opacity=0.4, semithick]
(axis cs:1,0.281672105413093)
--(axis cs:1,0.24446312947722)
--(axis cs:10,0.162119355053934)
--(axis cs:25,0.159594768858239)
--(axis cs:75,0.166204760461526)
--(axis cs:200,0.145110190962717)
--(axis cs:500,0.162198415650703)
--(axis cs:500,0.630858549893925)
--(axis cs:500,0.630858549893925)
--(axis cs:200,0.175752334968792)
--(axis cs:75,0.194949935788108)
--(axis cs:25,0.191690811891073)
--(axis cs:10,0.202372520726317)
--(axis cs:1,0.281672105413093)
--cycle;

\addplot [semithick, blue, mark=asterisk, mark size=4, mark options={solid}]
table {%
1 0.495427817106247
10 0.248387262225151
25 0.236766636371613
75 0.231731072068214
200 0.220703214406967
500 0.22512324154377
};
\addlegendentry{No si.}
\addplot [semithick, red, mark=asterisk, mark size=4, mark options={solid}]
table {%
1 0.495384305715561
10 0.251367211341858
25 0.207717821002007
75 0.203816741704941
200 0.185313686728477
500 0.186259418725967
};
\addlegendentry{Si 1}
\addplot [semithick, green!50.1960784313725!black, mark=asterisk, mark size=4, mark options={solid}]
table {%
1 0.299179285764694
10 0.170316502451897
25 0.179094910621643
75 0.153031080961227
200 0.145711228251457
500 0.152766168117523
};
\addlegendentry{Si 2}
\addplot [semithick, color0, mark=asterisk, mark size=4, mark options={solid}]
table {%
1 0.26467302441597
10 0.175934821367264
25 0.168692797422409
75 0.144676461815834
200 0.152819901704788
500 0.137696325778961
};
\addlegendentry{Si 3}
\addplot [semithick, white!50.1960784313725!black, mark=asterisk, mark size=4, mark options={solid}]
table {%
1 0.263067573308945
10 0.182245910167694
25 0.175642788410187
75 0.180577367544174
200 0.160431265830994
500 0.160534837245941
};
\addlegendentry{Si 4}
\end{axis}

\end{tikzpicture}


==> supp_mat/humanoid_plots/relerr_data.tex <==
\path [fill=red, fill opacity=0.4, ultra thick]
(axis cs:0.00187499995809048,0.223284651023948)
--(axis cs:0.00187499995809048,0.187695007463598)
--(axis cs:0.00374999991618097,0.238073378583014)
--(axis cs:0.00562499987427145,0.272915417762303)
--(axis cs:0.00749999983236194,0.296941764426831)
--(axis cs:0.00937499979045242,0.31378301041161)
--(axis cs:0.0112499997485429,0.326169058022026)
--(axis cs:0.0131249997066334,0.33603125434734)
--(axis cs:0.0149999996647239,0.344396583523761)
--(axis cs:0.0168749996228144,0.350577990730298)
--(axis cs:0.0187499995809048,0.355902759398283)
--(axis cs:0.0206249995389953,0.360659122884723)
--(axis cs:0.0224999994970858,0.364959140525023)
--(axis cs:0.0243749994551763,0.369079666832317)
--(axis cs:0.0262499994132668,0.373418755106175)
--(axis cs:0.0281249993713573,0.378105818071183)
--(axis cs:0.0299999993294477,0.383109354021729)
--(axis cs:0.0318749992875382,0.387992539662234)
--(axis cs:0.0337499992456287,0.392863938891101)
--(axis cs:0.0356249992037192,0.397422771456937)
--(axis cs:0.0374999991618097,0.40157376413107)
--(axis cs:0.0393749991199002,0.405325760221273)
--(axis cs:0.0412499990779907,0.408780934590834)
--(axis cs:0.0431249990360811,0.411984581000991)
--(axis cs:0.0449999989941716,0.415001821315762)
--(axis cs:0.0468749989522621,0.417721495614524)
--(axis cs:0.0487499989103526,0.420274014769265)
--(axis cs:0.0506249988684431,0.422661631274987)
--(axis cs:0.0524999988265336,0.424919836282206)
--(axis cs:0.054374998784624,0.427128184097617)
--(axis cs:0.0562499987427145,0.429352510089324)
--(axis cs:0.058124998700805,0.43160122785948)
--(axis cs:0.0599999986588955,0.433904146684153)
--(axis cs:0.061874998616986,0.436364983593702)
--(axis cs:0.0637499985750765,0.43889829952594)
--(axis cs:0.0656249985331669,0.441331483302928)
--(axis cs:0.0674999984912574,0.443539617436761)
--(axis cs:0.0693749984493479,0.445540446356029)
--(axis cs:0.0712499984074384,0.447387163250341)
--(axis cs:0.0731249983655289,0.449112071455718)
--(axis cs:0.0731249983655289,0.541743363602843)
--(axis cs:0.0731249983655289,0.541743363602843)
--(axis cs:0.0712499984074384,0.539869819107963)
--(axis cs:0.0693749984493479,0.537857723342209)
--(axis cs:0.0674999984912574,0.535690275685537)
--(axis cs:0.0656249985331669,0.533342389927295)
--(axis cs:0.0637499985750765,0.530805451220647)
--(axis cs:0.061874998616986,0.528177473863705)
--(axis cs:0.0599999986588955,0.525507110434785)
--(axis cs:0.058124998700805,0.522819855880136)
--(axis cs:0.0562499987427145,0.520140647615703)
--(axis cs:0.054374998784624,0.517448198944522)
--(axis cs:0.0524999988265336,0.514722708497198)
--(axis cs:0.0506249988684431,0.511921049201876)
--(axis cs:0.0487499989103526,0.509019604200708)
--(axis cs:0.0468749989522621,0.506061053914449)
--(axis cs:0.0449999989941716,0.503107116256956)
--(axis cs:0.0431249990360811,0.500062132028918)
--(axis cs:0.0412499990779907,0.496999294073496)
--(axis cs:0.0393749991199002,0.493914921542748)
--(axis cs:0.0374999991618097,0.490837674689559)
--(axis cs:0.0356249992037192,0.487716660234649)
--(axis cs:0.0337499992456287,0.484548615123408)
--(axis cs:0.0318749992875382,0.481389369746183)
--(axis cs:0.0299999993294477,0.478257875172665)
--(axis cs:0.0281249993713573,0.474712558954193)
--(axis cs:0.0262499994132668,0.47126126845787)
--(axis cs:0.0243749994551763,0.467746910053326)
--(axis cs:0.0224999994970858,0.463758677179827)
--(axis cs:0.0206249995389953,0.458758689862794)
--(axis cs:0.0187499995809048,0.452237133988835)
--(axis cs:0.0168749996228144,0.44391572654426)
--(axis cs:0.0149999996647239,0.433191093951257)
--(axis cs:0.0131249997066334,0.418590449681734)
--(axis cs:0.0112499997485429,0.401780542791275)
--(axis cs:0.00937499979045242,0.38194061610734)
--(axis cs:0.00749999983236194,0.357533872117525)
--(axis cs:0.00562499987427145,0.325905423696999)
--(axis cs:0.00374999991618097,0.283117501415678)
--(axis cs:0.00187499995809048,0.223284651023948)
--cycle;

\path [fill=blue, fill opacity=0.4, ultra thick]
(axis cs:0.00187499995809048,0.214541418636306)
--(axis cs:0.00187499995809048,0.185881351688115)
--(axis cs:0.00374999991618097,0.236092069616369)
--(axis cs:0.00562499987427145,0.271175634381049)
--(axis cs:0.00749999983236194,0.296051392355213)
--(axis cs:0.00937499979045242,0.314141038170178)
--(axis cs:0.0112499997485429,0.3280265826775)
--(axis cs:0.0131249997066334,0.339346058426552)
--(axis cs:0.0149999996647239,0.34899721967944)
--(axis cs:0.0168749996228144,0.356445171778196)
--(axis cs:0.0187499995809048,0.362689152513271)
--(axis cs:0.0206249995389953,0.367938546340262)
--(axis cs:0.0224999994970858,0.372345878750611)
--(axis cs:0.0243749994551763,0.376289462166616)
--(axis cs:0.0262499994132668,0.380256637769328)
--(axis cs:0.0281249993713573,0.384495361509867)
--(axis cs:0.0299999993294477,0.389011506668433)
--(axis cs:0.0318749992875382,0.39352650055273)
--(axis cs:0.0337499992456287,0.39812376351268)
--(axis cs:0.0356249992037192,0.402566676493214)
--(axis cs:0.0374999991618097,0.406716369576053)
--(axis cs:0.0393749991199002,0.410544983942511)
--(axis cs:0.0412499990779907,0.414152290405695)
--(axis cs:0.0431249990360811,0.417577750791763)
--(axis cs:0.0449999989941716,0.420872654527487)
--(axis cs:0.0468749989522621,0.42399662833414)
--(axis cs:0.0487499989103526,0.427030362276816)
--(axis cs:0.0506249988684431,0.429913438051283)
--(axis cs:0.0524999988265336,0.432640506463098)
--(axis cs:0.054374998784624,0.435272782940318)
--(axis cs:0.0562499987427145,0.437885461904852)
--(axis cs:0.058124998700805,0.440479101953634)
--(axis cs:0.0599999986588955,0.443074451307937)
--(axis cs:0.061874998616986,0.445799145197709)
--(axis cs:0.0637499985750765,0.448588006041982)
--(axis cs:0.0656249985331669,0.451279282940277)
--(axis cs:0.0674999984912574,0.453746066072114)
--(axis cs:0.0693749984493479,0.455947271603313)
--(axis cs:0.0712499984074384,0.457936324876151)
--(axis cs:0.0731249983655289,0.459758101681661)
--(axis cs:0.0731249983655289,0.531010585830433)
--(axis cs:0.0731249983655289,0.531010585830433)
--(axis cs:0.0712499984074384,0.529213091286003)
--(axis cs:0.0693749984493479,0.527306959496213)
--(axis cs:0.0674999984912574,0.525269641013705)
--(axis cs:0.0656249985331669,0.523073621225886)
--(axis cs:0.0637499985750765,0.520718964308791)
--(axis cs:0.061874998616986,0.51832670763358)
--(axis cs:0.0599999986588955,0.51601151724239)
--(axis cs:0.058124998700805,0.513819501844797)
--(axis cs:0.0562499987427145,0.511618501072789)
--(axis cs:0.054374998784624,0.509336496679038)
--(axis cs:0.0524999988265336,0.506909567254102)
--(axis cs:0.0506249988684431,0.504237280426706)
--(axis cs:0.0487499989103526,0.501272665257261)
--(axis cs:0.0468749989522621,0.498086043918768)
--(axis cs:0.0449999989941716,0.494759610080264)
--(axis cs:0.0431249990360811,0.491254702194686)
--(axis cs:0.0412499990779907,0.487655851538596)
--(axis cs:0.0393749991199002,0.483947944470614)
--(axis cs:0.0374999991618097,0.480127945177385)
--(axis cs:0.0356249992037192,0.476048111458795)
--(axis cs:0.0337499992456287,0.471695563026587)
--(axis cs:0.0318749992875382,0.467160454267312)
--(axis cs:0.0299999993294477,0.462623765795768)
--(axis cs:0.0281249993713573,0.457876112381823)
--(axis cs:0.0262499994132668,0.453198691698332)
--(axis cs:0.0243749994551763,0.448520028145378)
--(axis cs:0.0224999994970858,0.443587264911232)
--(axis cs:0.0206249995389953,0.437967936147307)
--(axis cs:0.0187499995809048,0.431224243438415)
--(axis cs:0.0168749996228144,0.423152576787881)
--(axis cs:0.0149999996647239,0.413234024557788)
--(axis cs:0.0131249997066334,0.399866766466688)
--(axis cs:0.0112499997485429,0.384516966802067)
--(axis cs:0.00937499979045242,0.366280408742227)
--(axis cs:0.00749999983236194,0.343492654281299)
--(axis cs:0.00562499987427145,0.313434715046863)
--(axis cs:0.00374999991618097,0.272308633158595)
--(axis cs:0.00187499995809048,0.214541418636306)
--cycle;

\path [fill=green!50.1960784313725!black, fill opacity=0.4, ultra thick]
(axis cs:0.00187499995809048,0.139223652861534)
--(axis cs:0.00187499995809048,0.105741159496303)
--(axis cs:0.00374999991618097,0.130081037698578)
--(axis cs:0.00562499987427145,0.145344502749689)
--(axis cs:0.00749999983236194,0.155538276775949)
--(axis cs:0.00937499979045242,0.162851166227453)
--(axis cs:0.0112499997485429,0.16854483471046)
--(axis cs:0.0131249997066334,0.17323162891121)
--(axis cs:0.0149999996647239,0.17710652105921)
--(axis cs:0.0168749996228144,0.179192809077768)
--(axis cs:0.0187499995809048,0.180742702540436)
--(axis cs:0.0206249995389953,0.182042745454178)
--(axis cs:0.0224999994970858,0.183330904036916)
--(axis cs:0.0243749994551763,0.185059589750292)
--(axis cs:0.0262499994132668,0.18762430784414)
--(axis cs:0.0281249993713573,0.191170815435446)
--(axis cs:0.0299999993294477,0.19535752526746)
--(axis cs:0.0318749992875382,0.200197318555072)
--(axis cs:0.0337499992456287,0.205232080108991)
--(axis cs:0.0356249992037192,0.20991473089874)
--(axis cs:0.0374999991618097,0.213931126117727)
--(axis cs:0.0393749991199002,0.217303303752117)
--(axis cs:0.0412499990779907,0.220375086672446)
--(axis cs:0.0431249990360811,0.223513034823706)
--(axis cs:0.0449999989941716,0.226709565601887)
--(axis cs:0.0468749989522621,0.229841097745072)
--(axis cs:0.0487499989103526,0.23264512668181)
--(axis cs:0.0506249988684431,0.235163623049129)
--(axis cs:0.0524999988265336,0.237790583013786)
--(axis cs:0.054374998784624,0.240892445845379)
--(axis cs:0.0562499987427145,0.24437878226566)
--(axis cs:0.058124998700805,0.247946664915851)
--(axis cs:0.0599999986588955,0.251236190330465)
--(axis cs:0.061874998616986,0.254082495381524)
--(axis cs:0.0637499985750765,0.256574401815768)
--(axis cs:0.0656249985331669,0.259223628749858)
--(axis cs:0.0674999984912574,0.262275033318818)
--(axis cs:0.0693749984493479,0.265598345626652)
--(axis cs:0.0712499984074384,0.26876608361511)
--(axis cs:0.0731249983655289,0.271321338504818)
--(axis cs:0.0731249983655289,0.327037261321266)
--(axis cs:0.0731249983655289,0.327037261321266)
--(axis cs:0.0712499984074384,0.324144004961088)
--(axis cs:0.0693749984493479,0.320903415497655)
--(axis cs:0.0674999984912574,0.317652840440192)
--(axis cs:0.0656249985331669,0.314767869357176)
--(axis cs:0.0637499985750765,0.312341667669991)
--(axis cs:0.061874998616986,0.310126103779903)
--(axis cs:0.0599999986588955,0.307741916582576)
--(axis cs:0.058124998700805,0.305010713663764)
--(axis cs:0.0562499987427145,0.302126260144018)
--(axis cs:0.054374998784624,0.29944380865218)
--(axis cs:0.0524999988265336,0.297301963275048)
--(axis cs:0.0506249988684431,0.295602584773287)
--(axis cs:0.0487499989103526,0.293733062814552)
--(axis cs:0.0468749989522621,0.291290218401913)
--(axis cs:0.0449999989941716,0.288283273457827)
--(axis cs:0.0431249990360811,0.284950308630874)
--(axis cs:0.0412499990779907,0.28149293622296)
--(axis cs:0.0393749991199002,0.277974996359727)
--(axis cs:0.0374999991618097,0.274133549937828)
--(axis cs:0.0356249992037192,0.269673038143413)
--(axis cs:0.0337499992456287,0.264654724215236)
--(axis cs:0.0318749992875382,0.259418435072314)
--(axis cs:0.0299999993294477,0.25433494525116)
--(axis cs:0.0281249993713573,0.249593491941907)
--(axis cs:0.0262499994132668,0.245551320257324)
--(axis cs:0.0243749994551763,0.242392477243696)
--(axis cs:0.0224999994970858,0.239940114478288)
--(axis cs:0.0206249995389953,0.237501059915317)
--(axis cs:0.0187499995809048,0.234658085927116)
--(axis cs:0.0168749996228144,0.231387851935076)
--(axis cs:0.0149999996647239,0.227544491887659)
--(axis cs:0.0131249997066334,0.221702686322528)
--(axis cs:0.0112499997485429,0.215498548701432)
--(axis cs:0.00937499979045242,0.208935629761116)
--(axis cs:0.00749999983236194,0.201164197886453)
--(axis cs:0.00562499987427145,0.18970785286867)
--(axis cs:0.00374999991618097,0.17097152676592)
--(axis cs:0.00187499995809048,0.139223652861534)
--cycle;

\path [fill=color0, fill opacity=0.4, ultra thick]
(axis cs:0.00187499995809048,0.117463438879036)
--(axis cs:0.00187499995809048,0.0912719625240553)
--(axis cs:0.00374999991618097,0.113974005292587)
--(axis cs:0.00562499987427145,0.126456958104897)
--(axis cs:0.00749999983236194,0.134376362646999)
--(axis cs:0.00937499979045242,0.139649923252697)
--(axis cs:0.0112499997485429,0.143570466878104)
--(axis cs:0.0131249997066334,0.14692980482776)
--(axis cs:0.0149999996647239,0.149992049360603)
--(axis cs:0.0168749996228144,0.152569900447804)
--(axis cs:0.0187499995809048,0.155193620709437)
--(axis cs:0.0206249995389953,0.157404737589173)
--(axis cs:0.0224999994970858,0.15904492845752)
--(axis cs:0.0243749994551763,0.160577645881319)
--(axis cs:0.0262499994132668,0.162770347610003)
--(axis cs:0.0281249993713573,0.165986073421327)
--(axis cs:0.0299999993294477,0.169972610874701)
--(axis cs:0.0318749992875382,0.174787893912113)
--(axis cs:0.0337499992456287,0.179844558135913)
--(axis cs:0.0356249992037192,0.184497631220257)
--(axis cs:0.0374999991618097,0.188472614381626)
--(axis cs:0.0393749991199002,0.191930809201438)
--(axis cs:0.0412499990779907,0.195221413537243)
--(axis cs:0.0431249990360811,0.198535490173261)
--(axis cs:0.0449999989941716,0.201646595313717)
--(axis cs:0.0468749989522621,0.204421541246067)
--(axis cs:0.0487499989103526,0.206635196416506)
--(axis cs:0.0506249988684431,0.208624619831706)
--(axis cs:0.0524999988265336,0.211077499334522)
--(axis cs:0.054374998784624,0.214279868504342)
--(axis cs:0.0562499987427145,0.21790023147521)
--(axis cs:0.058124998700805,0.221502920183717)
--(axis cs:0.0599999986588955,0.224698767143723)
--(axis cs:0.061874998616986,0.227365984709238)
--(axis cs:0.0637499985750765,0.229800577682563)
--(axis cs:0.0656249985331669,0.232709447289886)
--(axis cs:0.0674999984912574,0.236307066992831)
--(axis cs:0.0693749984493479,0.240244046008091)
--(axis cs:0.0712499984074384,0.243962185196731)
--(axis cs:0.0731249983655289,0.246882484426964)
--(axis cs:0.0731249983655289,0.282463641182809)
--(axis cs:0.0731249983655289,0.282463641182809)
--(axis cs:0.0712499984074384,0.27993067975894)
--(axis cs:0.0693749984493479,0.276753552462606)
--(axis cs:0.0674999984912574,0.273378836622982)
--(axis cs:0.0656249985331669,0.270310353610835)
--(axis cs:0.0637499985750765,0.267897293959115)
--(axis cs:0.061874998616986,0.266007466769658)
--(axis cs:0.0599999986588955,0.264001024058852)
--(axis cs:0.058124998700805,0.261471338385212)
--(axis cs:0.0562499987427145,0.258527813714269)
--(axis cs:0.054374998784624,0.255592067583558)
--(axis cs:0.0524999988265336,0.253133966377224)
--(axis cs:0.0506249988684431,0.251335330752219)
--(axis cs:0.0487499989103526,0.249766818085744)
--(axis cs:0.0468749989522621,0.247874916102284)
--(axis cs:0.0449999989941716,0.245406628222752)
--(axis cs:0.0431249990360811,0.24259799748098)
--(axis cs:0.0412499990779907,0.239590833706201)
--(axis cs:0.0393749991199002,0.236640348914503)
--(axis cs:0.0374999991618097,0.233622114574902)
--(axis cs:0.0356249992037192,0.230256881082203)
--(axis cs:0.0337499992456287,0.226397797422095)
--(axis cs:0.0318749992875382,0.222264566381443)
--(axis cs:0.0299999993294477,0.218287332357348)
--(axis cs:0.0281249993713573,0.214733950275605)
--(axis cs:0.0262499994132668,0.212118548550569)
--(axis cs:0.0243749994551763,0.210731919357376)
--(axis cs:0.0224999994970858,0.210172821623505)
--(axis cs:0.0206249995389953,0.209504963358523)
--(axis cs:0.0187499995809048,0.207966222939919)
--(axis cs:0.0168749996228144,0.205569037212601)
--(axis cs:0.0149999996647239,0.202258655362648)
--(axis cs:0.0131249997066334,0.196733665161906)
--(axis cs:0.0112499997485429,0.190600388473145)
--(axis cs:0.00937499979045242,0.183650578860782)
--(axis cs:0.00749999983236194,0.175254160782464)
--(axis cs:0.00562499987427145,0.163919504748079)
--(axis cs:0.00374999991618097,0.146870469800431)
--(axis cs:0.00187499995809048,0.117463438879036)
--cycle;

\path [fill=white!50.1960784313725!black, fill opacity=0.4, ultra thick]
(axis cs:0.00187499995809048,0.117603619176082)
--(axis cs:0.00187499995809048,0.0888441738299863)
--(axis cs:0.00374999991618097,0.11137469706396)
--(axis cs:0.00562499987427145,0.123780651602935)
--(axis cs:0.00749999983236194,0.131747545180364)
--(axis cs:0.00937499979045242,0.137328273856982)
--(axis cs:0.0112499997485429,0.141557728839315)
--(axis cs:0.0131249997066334,0.145191110209191)
--(axis cs:0.0149999996647239,0.148601741457914)
--(axis cs:0.0168749996228144,0.151641514377504)
--(axis cs:0.0187499995809048,0.154778988535269)
--(axis cs:0.0206249995389953,0.157511837005123)
--(axis cs:0.0224999994970858,0.15963717738536)
--(axis cs:0.0243749994551763,0.161476834422451)
--(axis cs:0.0262499994132668,0.163769501583791)
--(axis cs:0.0281249993713573,0.166942267589799)
--(axis cs:0.0299999993294477,0.170762495499165)
--(axis cs:0.0318749992875382,0.175384745806747)
--(axis cs:0.0337499992456287,0.180229647992369)
--(axis cs:0.0356249992037192,0.184684989126684)
--(axis cs:0.0374999991618097,0.188495082444062)
--(axis cs:0.0393749991199002,0.191838485302774)
--(axis cs:0.0412499990779907,0.195097590847782)
--(axis cs:0.0431249990360811,0.198361967564248)
--(axis cs:0.0449999989941716,0.201384174581453)
--(axis cs:0.0468749989522621,0.204059307945596)
--(axis cs:0.0487499989103526,0.206216849448362)
--(axis cs:0.0506249988684431,0.208184822026091)
--(axis cs:0.0524999988265336,0.210663466691116)
--(axis cs:0.054374998784624,0.213854682628959)
--(axis cs:0.0562499987427145,0.217381772425103)
--(axis cs:0.058124998700805,0.220810076721044)
--(axis cs:0.0599999986588955,0.223743002878156)
--(axis cs:0.061874998616986,0.226132402915462)
--(axis cs:0.0637499985750765,0.228378979529105)
--(axis cs:0.0656249985331669,0.23121383084439)
--(axis cs:0.0674999984912574,0.234711256629856)
--(axis cs:0.0693749984493479,0.238442252490448)
--(axis cs:0.0712499984074384,0.241875778707065)
--(axis cs:0.0731249983655289,0.24446312947722)
--(axis cs:0.0731249983655289,0.281672105413093)
--(axis cs:0.0731249983655289,0.281672105413093)
--(axis cs:0.0712499984074384,0.278987435559975)
--(axis cs:0.0693749984493479,0.275733615839314)
--(axis cs:0.0674999984912574,0.272356431467571)
--(axis cs:0.0656249985331669,0.269324097082861)
--(axis cs:0.0637499985750765,0.266926629429727)
--(axis cs:0.061874998616986,0.264977610749758)
--(axis cs:0.0599999986588955,0.262791811651001)
--(axis cs:0.058124998700805,0.260098198197488)
--(axis cs:0.0562499987427145,0.257039281191368)
--(axis cs:0.054374998784624,0.254000338592551)
--(axis cs:0.0524999988265336,0.25145098051572)
--(axis cs:0.0506249988684431,0.249482763107709)
--(axis cs:0.0487499989103526,0.247715881087006)
--(axis cs:0.0468749989522621,0.245619917228538)
--(axis cs:0.0449999989941716,0.242986635613337)
--(axis cs:0.0431249990360811,0.240025822840973)
--(axis cs:0.0412499990779907,0.236915183477949)
--(axis cs:0.0393749991199002,0.233907749917004)
--(axis cs:0.0374999991618097,0.230888977148963)
--(axis cs:0.0356249992037192,0.227593341939591)
--(axis cs:0.0337499992456287,0.223821108825077)
--(axis cs:0.0318749992875382,0.219775673376735)
--(axis cs:0.0299999993294477,0.21591848966033)
--(axis cs:0.0281249993713573,0.212530340667989)
--(axis cs:0.0262499994132668,0.210113049145438)
--(axis cs:0.0243749994551763,0.20886632358114)
--(axis cs:0.0224999994970858,0.208346137249713)
--(axis cs:0.0206249995389953,0.207610912135445)
--(axis cs:0.0187499995809048,0.206043567551835)
--(axis cs:0.0168749996228144,0.20377580072798)
--(axis cs:0.0149999996647239,0.200675237237315)
--(axis cs:0.0131249997066334,0.195232168191872)
--(axis cs:0.0112499997485429,0.18925342768493)
--(axis cs:0.00937499979045242,0.182536833705559)
--(axis cs:0.00749999983236194,0.174442184109951)
--(axis cs:0.00562499987427145,0.163246432102678)
--(axis cs:0.00374999991618097,0.146761480506058)
--(axis cs:0.00187499995809048,0.117603619176082)
--cycle;

\addplot [ultra thick, red]
table {%
0.00187504291534424 0.205489858984947
0.00374996662139893 0.260595411062241
0.00562500953674316 0.299410372972488
0.0075000524520874 0.327237814664841
0.00937497615814209 0.347861796617508
0.0112500190734863 0.363974869251251
0.013124942779541 0.377310812473297
0.0149999856948853 0.388793766498566
0.0168750286102295 0.397246927022934
0.0187499523162842 0.404069930315018
0.0206249952316284 0.409708887338638
0.0225000381469727 0.414358913898468
0.0243749618530273 0.41841322183609
0.0262500047683716 0.422340005636215
0.0281250476837158 0.426409184932709
0.0299999713897705 0.430683642625809
0.033750057220459 0.438706308603287
0.0356249809265137 0.442569702863693
0.0375000238418579 0.446205765008926
0.0393749475479126 0.449620366096497
0.0412499904632568 0.452890127897263
0.0431250333786011 0.456023305654526
0.0449999570846558 0.459054529666901
0.046875 0.461891323328018
0.0487500429153442 0.464646816253662
0.0506249666213989 0.467291325330734
0.0525000095367432 0.46982130408287
0.0562499761581421 0.474746555089951
0.059999942779541 0.479705661535263
0.0637500286102295 0.484851896762848
0.0656249523162842 0.487336844205856
0.0674999952316284 0.489614903926849
0.0693750381469727 0.491699069738388
0.0712499618530273 0.493628531694412
0.0731250047683716 0.495427817106247
};
\addplot [ultra thick, blue]
table {%
0.00187504291534424 0.200211375951767
0.00374996662139893 0.254200369119644
0.00562500953674316 0.292305201292038
0.0075000524520874 0.319772034883499
0.00937497615814209 0.340210765600204
0.0112500190734863 0.356271773576736
0.013124942779541 0.369606405496597
0.0149999856948853 0.381115585565567
0.0168750286102295 0.389798879623413
0.0187499523162842 0.396956771612167
0.0206249952316284 0.402953237295151
0.0225000381469727 0.407966554164886
0.0243749618530273 0.412404745817184
0.0262500047683716 0.416727632284164
0.0281250476837158 0.42118564248085
0.0299999713897705 0.425817579030991
0.033750057220459 0.434909731149673
0.0356249809265137 0.439307391643524
0.0375000238418579 0.443422228097916
0.0393749475479126 0.447246462106705
0.0412499904632568 0.450904130935669
0.0431250333786011 0.454416155815125
0.0449999570846558 0.457816064357758
0.046875 0.461041390895844
0.0487500429153442 0.464151591062546
0.0506249666213989 0.467075377702713
0.0525000095367432 0.469775140285492
0.0543750524520874 0.472304672002792
0.0562499761581421 0.474752008914948
0.059999942779541 0.479542940855026
0.0618749856948853 0.482062995433807
0.0637500286102295 0.484653502702713
0.0656249523162842 0.487176477909088
0.0674999952316284 0.4895079433918
0.0693750381469727 0.491627126932144
0.0712499618530273 0.493574768304825
0.0731250047683716 0.495384305715561
};
\addplot [ultra thick, green!50.1960784313725!black]
table {%
0.00187504291534424 0.122482411563396
0.00374996662139893 0.150526270270348
0.00562500953674316 0.167526185512543
0.0075000524520874 0.178351238369942
0.00937497615814209 0.185893401503563
0.0112500190734863 0.192021667957306
0.013124942779541 0.197467178106308
0.0149999856948853 0.202325522899628
0.0168750286102295 0.205290332436562
0.0187499523162842 0.207700431346893
0.0206249952316284 0.209771901369095
0.0225000381469727 0.211635529994965
0.0243749618530273 0.213725998997688
0.0262500047683716 0.216587796807289
0.0281250476837158 0.220382124185562
0.0299999713897705 0.224846199154854
0.0318750143051147 0.229807838797569
0.033750057220459 0.234943449497223
0.0356249809265137 0.239793881773949
0.0375000238418579 0.244032323360443
0.0393749475479126 0.247639164328575
0.0412499904632568 0.25093400478363
0.0431250333786011 0.254231631755829
0.0449999570846558 0.257496386766434
0.046875 0.260565638542175
0.0487500429153442 0.263189047574997
0.0506249666213989 0.265383064746857
0.0525000095367432 0.26754629611969
0.0543750524520874 0.270168095827103
0.0562499761581421 0.273252546787262
0.0581250190734863 0.27647864818573
0.059999942779541 0.279489040374756
0.0618749856948853 0.282104253768921
0.0637500286102295 0.284458041191101
0.0656249523162842 0.286995768547058
0.0674999952316284 0.289963901042938
0.0693750381469727 0.293250918388367
0.0712499618530273 0.296455055475235
0.0731250047683716 0.299179285764694
};
\addplot [ultra thick, color0]
table {%
0.00187504291534424 0.104367703199387
0.00374996662139893 0.130422249436378
0.00562500953674316 0.145188227295876
0.0075000524520874 0.15481524169445
0.00937497615814209 0.161650270223618
0.0112500190734863 0.167085409164429
0.013124942779541 0.171831727027893
0.0149999856948853 0.176125332713127
0.0168750286102295 0.179069444537163
0.0187499523162842 0.181579902768135
0.0206249952316284 0.183454841375351
0.0225000381469727 0.184608846902847
0.0243749618530273 0.185654759407043
0.0262500047683716 0.187444448471069
0.0281250476837158 0.190360009670258
0.0299999713897705 0.19412998855114
0.0318750143051147 0.198526248335838
0.033750057220459 0.203121185302734
0.0356249809265137 0.207377254962921
0.0375000238418579 0.211047351360321
0.0393749475479126 0.214285582304001
0.0431250333786011 0.220566764473915
0.0449999570846558 0.223526611924171
0.046875 0.226148262619972
0.0487500429153442 0.228201031684875
0.0506249666213989 0.229979991912842
0.0525000095367432 0.232105776667595
0.0543750524520874 0.234935969114304
0.0562499761581421 0.238214015960693
0.0581250190734863 0.24148716032505
0.059999942779541 0.244349896907806
0.0618749856948853 0.246686711907387
0.0637500286102295 0.248848930001259
0.0656249523162842 0.251509934663773
0.0674999952316284 0.254842966794968
0.0693750381469727 0.258498817682266
0.0712499618530273 0.261946380138397
0.0731250047683716 0.26467302441597
};
\addplot [ultra thick, white!40.1960784313725!black]
table {%
0.00187504291534424 0.103223890066147
0.00374996662139893 0.129068076610565
0.00562500953674316 0.143513545393944
0.0075000524520874 0.153094857931137
0.00937497615814209 0.159932538866997
0.0112500190734863 0.165405601263046
0.013124942779541 0.170211628079414
0.0149999856948853 0.174638524651527
0.0168750286102295 0.177708685398102
0.0187499523162842 0.180411294102669
0.0206249952316284 0.182561337947845
0.0225000381469727 0.183991670608521
0.0243749618530273 0.185171574354172
0.0262500047683716 0.186941251158714
0.0281250476837158 0.189736306667328
0.0299999713897705 0.193340495228767
0.0318750143051147 0.197580218315125
0.033750057220459 0.202025398612022
0.0356249809265137 0.206139206886292
0.0375000238418579 0.209692046046257
0.0393749475479126 0.212873116135597
0.0431250333786011 0.219193875789642
0.0449999570846558 0.222185358405113
0.046875 0.224839597940445
0.0487500429153442 0.226966395974159
0.0506249666213989 0.228833809494972
0.0525000095367432 0.231057241559029
0.0543750524520874 0.233927488327026
0.0562499761581421 0.237210541963577
0.0581250190734863 0.240454122424126
0.059999942779541 0.243267357349396
0.0618749856948853 0.245555058121681
0.0637500286102295 0.247652754187584
0.0656249523162842 0.250268965959549
0.0674999952316284 0.253533840179443
0.0693750381469727 0.257087886333466
0.0712499618530273 0.26043164730072
0.0731250047683716 0.263067573308945
};


==> supp_mat/humanoid_plots/train_test_loss_data.tex <==
\path [fill=red, fill opacity=0.4, ultra thick]
(axis cs:0,0.157891631126404)
--(axis cs:0,0.156707122921944)
--(axis cs:100,0.152500689029694)
--(axis cs:200,0.147555321455002)
--(axis cs:300,0.142711475491524)
--(axis cs:400,0.13894097507)
--(axis cs:500,0.136075586080551)
--(axis cs:600,0.133588179945946)
--(axis cs:700,0.13145424425602)
--(axis cs:800,0.130239441990852)
--(axis cs:900,0.129831120371819)
--(axis cs:1000,0.129790559411049)
--(axis cs:1100,0.129808112978935)
--(axis cs:1200,0.130750745534897)
--(axis cs:1300,0.131993338465691)
--(axis cs:1400,0.133178263902664)
--(axis cs:1500,0.13405454158783)
--(axis cs:1600,0.135351493954659)
--(axis cs:1700,0.136895939707756)
--(axis cs:1800,0.138367012143135)
--(axis cs:1800,0.140710845589638)
--(axis cs:1800,0.140710845589638)
--(axis cs:1700,0.1396644115448)
--(axis cs:1600,0.137976124882698)
--(axis cs:1500,0.136463105678558)
--(axis cs:1400,0.134592816233635)
--(axis cs:1300,0.133277282118797)
--(axis cs:1200,0.131870120763779)
--(axis cs:1100,0.131040781736374)
--(axis cs:1000,0.1307003647089)
--(axis cs:900,0.130977004766464)
--(axis cs:800,0.131350114941597)
--(axis cs:700,0.132590159773827)
--(axis cs:600,0.134512767195702)
--(axis cs:500,0.136909961700439)
--(axis cs:400,0.139808893203735)
--(axis cs:300,0.143705025315285)
--(axis cs:200,0.14826825261116)
--(axis cs:100,0.153138846158981)
--(axis cs:0,0.157891631126404)
--cycle;

\path [fill=blue, fill opacity=0.4, ultra thick]
(axis cs:0,0.16883285343647)
--(axis cs:0,0.168774530291557)
--(axis cs:100,0.166224166750908)
--(axis cs:200,0.163298755884171)
--(axis cs:300,0.160059332847595)
--(axis cs:400,0.15654131770134)
--(axis cs:500,0.152967691421509)
--(axis cs:600,0.149806439876556)
--(axis cs:700,0.147015690803528)
--(axis cs:800,0.14439769089222)
--(axis cs:900,0.141728043556213)
--(axis cs:1000,0.139089226722717)
--(axis cs:1100,0.136542022228241)
--(axis cs:1200,0.134253308176994)
--(axis cs:1300,0.13244840502739)
--(axis cs:1400,0.130785629153252)
--(axis cs:1500,0.129413813352585)
--(axis cs:1600,0.128441333770752)
--(axis cs:1700,0.12728314101696)
--(axis cs:1800,0.126819714903831)
--(axis cs:1900,0.126506358385086)
--(axis cs:2000,0.126513361930847)
--(axis cs:2100,0.126674488186836)
--(axis cs:2200,0.126767784357071)
--(axis cs:2300,0.126931846141815)
--(axis cs:2400,0.12742093205452)
--(axis cs:2500,0.128065273165703)
--(axis cs:2600,0.128324285149574)
--(axis cs:2700,0.129224315285683)
--(axis cs:2800,0.129832699894905)
--(axis cs:2900,0.130365759134293)
--(axis cs:3000,0.130714654922485)
--(axis cs:3100,0.131480172276497)
--(axis cs:3200,0.132055059075356)
--(axis cs:3200,0.137156561017036)
--(axis cs:3200,0.137156561017036)
--(axis cs:3100,0.136083915829659)
--(axis cs:3000,0.134891837835312)
--(axis cs:2900,0.133804440498352)
--(axis cs:2800,0.132485538721085)
--(axis cs:2700,0.131375342607498)
--(axis cs:2600,0.130737736821175)
--(axis cs:2500,0.129947856068611)
--(axis cs:2400,0.128819033503532)
--(axis cs:2300,0.128465577960014)
--(axis cs:2200,0.128268837928772)
--(axis cs:2100,0.127889558672905)
--(axis cs:2000,0.12802392244339)
--(axis cs:1900,0.127600520849228)
--(axis cs:1800,0.127773091197014)
--(axis cs:1700,0.128536894917488)
--(axis cs:1600,0.129573613405228)
--(axis cs:1500,0.130521804094315)
--(axis cs:1400,0.131793335080147)
--(axis cs:1300,0.133387237787247)
--(axis cs:1200,0.135041922330856)
--(axis cs:1100,0.137195900082588)
--(axis cs:1000,0.139632970094681)
--(axis cs:900,0.142248421907425)
--(axis cs:800,0.144854798913002)
--(axis cs:700,0.147579938173294)
--(axis cs:600,0.150275200605392)
--(axis cs:500,0.153362989425659)
--(axis cs:400,0.156814098358154)
--(axis cs:300,0.160316914319992)
--(axis cs:200,0.163508355617523)
--(axis cs:100,0.16631506383419)
--(axis cs:0,0.16883285343647)
--cycle;

\path [fill=green!50.1960784313725!black, fill opacity=0.4, ultra thick]
(axis cs:0,0.115993812680244)
--(axis cs:0,0.115573808550835)
--(axis cs:100,0.108277775347233)
--(axis cs:200,0.101100146770477)
--(axis cs:300,0.0948384553194046)
--(axis cs:400,0.0887349992990494)
--(axis cs:500,0.0835918784141541)
--(axis cs:600,0.0803125351667404)
--(axis cs:700,0.0779219642281532)
--(axis cs:800,0.0763957276940346)
--(axis cs:900,0.0757012367248535)
--(axis cs:1000,0.0756266117095947)
--(axis cs:1100,0.0761700719594955)
--(axis cs:1200,0.0771142095327377)
--(axis cs:1300,0.0775865316390991)
--(axis cs:1400,0.0780411511659622)
--(axis cs:1500,0.0787514299154282)
--(axis cs:1600,0.0792547017335892)
--(axis cs:1600,0.0813008844852448)
--(axis cs:1600,0.0813008844852448)
--(axis cs:1500,0.0810655206441879)
--(axis cs:1400,0.0807349681854248)
--(axis cs:1300,0.0793756246566772)
--(axis cs:1200,0.0779962241649628)
--(axis cs:1100,0.0770085155963898)
--(axis cs:1000,0.0768293887376785)
--(axis cs:900,0.0770425051450729)
--(axis cs:800,0.0773364081978798)
--(axis cs:700,0.0786337628960609)
--(axis cs:600,0.0811715871095657)
--(axis cs:500,0.0843863561749458)
--(axis cs:400,0.0890617370605469)
--(axis cs:300,0.0950746387243271)
--(axis cs:200,0.101643040776253)
--(axis cs:100,0.108931817114353)
--(axis cs:0,0.115993812680244)
--cycle;

\path [fill=color0, fill opacity=0.4, ultra thick]
(axis cs:0,0.0974255204200745)
--(axis cs:0,0.0967491120100021)
--(axis cs:100,0.0878203138709068)
--(axis cs:200,0.0793911516666412)
--(axis cs:300,0.0724547430872917)
--(axis cs:400,0.0675220042467117)
--(axis cs:500,0.0640111118555069)
--(axis cs:600,0.0615299679338932)
--(axis cs:700,0.0598497688770294)
--(axis cs:800,0.0589690469205379)
--(axis cs:900,0.0585705898702145)
--(axis cs:1000,0.058612909168005)
--(axis cs:1100,0.0590603426098824)
--(axis cs:1200,0.0596427395939827)
--(axis cs:1300,0.0601931884884834)
--(axis cs:1400,0.0610491149127483)
--(axis cs:1500,0.0618468336760998)
--(axis cs:1600,0.0621525123715401)
--(axis cs:1600,0.063120000064373)
--(axis cs:1600,0.063120000064373)
--(axis cs:1500,0.062134362757206)
--(axis cs:1400,0.0614040978252888)
--(axis cs:1300,0.0610441267490387)
--(axis cs:1200,0.0601691231131554)
--(axis cs:1100,0.0597608983516693)
--(axis cs:1000,0.0595056377351284)
--(axis cs:900,0.0595943070948124)
--(axis cs:800,0.0598804466426373)
--(axis cs:700,0.0609363839030266)
--(axis cs:600,0.0625469014048576)
--(axis cs:500,0.0650931745767593)
--(axis cs:400,0.0685819536447525)
--(axis cs:300,0.0733053311705589)
--(axis cs:200,0.0803433060646057)
--(axis cs:100,0.0886920019984245)
--(axis cs:0,0.0974255204200745)
--cycle;

\path [fill=white!40.1960784313725!black, fill opacity=0.4, ultra thick]
(axis cs:0,0.0974728986620903)
--(axis cs:0,0.0966551229357719)
--(axis cs:100,0.087830938398838)
--(axis cs:200,0.079444631934166)
--(axis cs:300,0.0724884644150734)
--(axis cs:400,0.0676380023360252)
--(axis cs:500,0.0641438663005829)
--(axis cs:600,0.0616008266806602)
--(axis cs:700,0.0600851774215698)
--(axis cs:800,0.0592496693134308)
--(axis cs:900,0.0586629025638103)
--(axis cs:1000,0.0587406978011131)
--(axis cs:1100,0.0591305866837502)
--(axis cs:1200,0.0600960850715637)
--(axis cs:1300,0.0608675964176655)
--(axis cs:1400,0.0614956505596638)
--(axis cs:1500,0.0622464530169964)
--(axis cs:1600,0.0631800815463066)
--(axis cs:1600,0.0636094138026237)
--(axis cs:1600,0.0636094138026237)
--(axis cs:1500,0.0632269307971001)
--(axis cs:1400,0.0628291890025139)
--(axis cs:1300,0.0619762763381004)
--(axis cs:1200,0.0609938502311707)
--(axis cs:1100,0.0602083057165146)
--(axis cs:1000,0.0598639845848083)
--(axis cs:900,0.0598933361470699)
--(axis cs:800,0.060356643050909)
--(axis cs:700,0.061256542801857)
--(axis cs:600,0.0628817081451416)
--(axis cs:500,0.0653250515460968)
--(axis cs:400,0.0686143413186073)
--(axis cs:300,0.0734104439616203)
--(axis cs:200,0.0804402083158493)
--(axis cs:100,0.0887273177504539)
--(axis cs:0,0.0974728986620903)
--cycle;

\addplot [ultra thick, red  ]
table {%
0 0.157305002212524
100 0.152832016348839
200 0.147967681288719
300 0.143208265304565
400 0.139409884810448
500 0.136492773890495
600 0.134050458669662
700 0.132003650069237
800 0.130794763565063
900 0.13043338060379
1000 0.130187004804611
1100 0.130454942584038
1200 0.131313025951385
1400 0.133978575468063
1500 0.135258823633194
1600 0.136663794517517
1700 0.138177812099457
1800 0.139382258057594
};
\addlegendentry{Baseline}
\addplot [ultra thick, blue  ]
table {%
0 0.168808653950691
100 0.166276067495346
200 0.163403555750847
300 0.160191714763641
400 0.156698480248451
500 0.153174802660942
600 0.150040820240974
1000 0.139361098408699
1100 0.136889770627022
1200 0.134687200188637
1300 0.13292770087719
1400 0.131289467215538
1500 0.12996780872345
1600 0.129007488489151
1700 0.127900809049606
1800 0.127296417951584
1900 0.127019703388214
2100 0.127282023429871
2200 0.127518326044083
2300 0.127727806568146
2400 0.128180429339409
2500 0.129006564617157
2600 0.129530996084213
2700 0.130361154675484
2800 0.131262004375458
2900 0.132085114717484
3000 0.132803231477737
3100 0.133782044053078
3200 0.134605824947357
};
\addlegendentry{K1}
\addplot [ultra thick, green!39.2156862745098!black,  ]
table {%
0 0.11578381806612
100 0.108604818582535
200 0.101371616125107
300 0.0949505195021629
400 0.0889095664024353
500 0.0839678272604942
600 0.0807565152645111
700 0.0783044919371605
800 0.0768660679459572
900 0.0763718634843826
1000 0.0762280002236366
1100 0.0765892863273621
1200 0.0775552168488503
1300 0.0784810706973076
1400 0.0793880671262741
1500 0.0798000916838646
1600 0.0802777856588364
};
\addlegendentry{K2}
\addplot [ultra thick, color0 ]
table {%
0 0.0970873087644577
100 0.0882561504840851
200 0.0798672139644623
300 0.0728800296783447
400 0.0680519640445709
500 0.0645295530557632
600 0.0620384365320206
700 0.060393076390028
800 0.0594247542321682
900 0.0590824522078037
1000 0.0590592809021473
1100 0.0594106130301952
1200 0.0599059388041496
1300 0.0606186650693417
1400 0.0612562485039234
1500 0.0620062239468098
1600 0.0626362562179565
};
\addlegendentry{K3}
\addplot [ultra thick, white!60.2745098039216!black,  ]
table {%
0 0.0970640182495117
100 0.0882791206240654
200 0.0799424275755882
300 0.0729494616389275
400 0.0681261643767357
500 0.0647266060113907
600 0.0622388310730457
700 0.0606431774795055
800 0.0597685612738132
900 0.0592781156301498
1000 0.0593023486435413
1100 0.059669453650713
1200 0.0605449639260769
1300 0.0614907294511795
1400 0.0621624104678631
1500 0.0627366900444031
1600 0.0633947402238846
};
\addlegendentry{K4}

==> supp_mat/humanoid_plots/traj_err_data.tex <==
\path [fill=red, fill opacity=0.4, ultra thick]
(axis cs:1,0.541743363602843)
--(axis cs:1,0.449112071455718)
--(axis cs:10,0.222851933182839)
--(axis cs:25,0.218278809800564)
--(axis cs:75,0.203373653824151)
--(axis cs:200,0.202344693428683)
--(axis cs:500,0.205319745054706)
--(axis cs:500,0.24492664882946)
--(axis cs:500,0.24492664882946)
--(axis cs:200,0.239061668396655)
--(axis cs:75,0.260088453237498)
--(axis cs:25,0.255254397050033)
--(axis cs:10,0.273922619095674)
--(axis cs:1,0.541743363602843)
--cycle;

\path [fill=blue, fill opacity=0.4, ultra thick]
(axis cs:1,0.531010585830433)
--(axis cs:1,0.459758101681661)
--(axis cs:10,0.229730335009316)
--(axis cs:25,0.191273754876949)
--(axis cs:75,0.175796832901461)
--(axis cs:200,0.164071554922007)
--(axis cs:500,0.170048621804538)
--(axis cs:500,0.202470236594375)
--(axis cs:500,0.202470236594375)
--(axis cs:200,0.206555843340007)
--(axis cs:75,0.231836704110698)
--(axis cs:25,0.224161883102382)
--(axis cs:10,0.27300405791108)
--(axis cs:1,0.531010585830433)
--cycle;

\path [fill=green!50.1960784313725!black, fill opacity=0.4, ultra thick]
(axis cs:1,0.327037261321266)
--(axis cs:1,0.271321338504818)
--(axis cs:10,0.153216160419598)
--(axis cs:25,0.162110887475575)
--(axis cs:75,0.14101120413756)
--(axis cs:200,0.131378655409453)
--(axis cs:500,0.133331697770542)
--(axis cs:500,0.172200606977037)
--(axis cs:500,0.172200606977037)
--(axis cs:200,0.160043838253535)
--(axis cs:75,0.165050957437437)
--(axis cs:25,0.196078888437663)
--(axis cs:10,0.187416813983647)
--(axis cs:1,0.327037261321266)
--cycle;

\path [fill=color0, fill opacity=0.4, ultra thick]
(axis cs:1,0.282463641182809)
--(axis cs:1,0.246882484426964)
--(axis cs:10,0.161905684649898)
--(axis cs:25,0.148348927125901)
--(axis cs:75,0.129090951546991)
--(axis cs:200,0.124358420615673)
--(axis cs:500,0.122476188880835)
--(axis cs:500,0.152916463115796)
--(axis cs:500,0.152916463115796)
--(axis cs:200,0.18128134913412)
--(axis cs:75,0.160261962288737)
--(axis cs:25,0.189036696377846)
--(axis cs:10,0.189963946263115)
--(axis cs:1,0.282463641182809)
--cycle;

\path [fill=white!50.1960784313725!black, fill opacity=0.4, ultra thick]
(axis cs:1,0.281672105413093)
--(axis cs:1,0.24446312947722)
--(axis cs:10,0.162119355053934)
--(axis cs:25,0.159594768858239)
--(axis cs:75,0.166204760461526)
--(axis cs:200,0.145110190962717)
--(axis cs:500,0.162198415650703)
--(axis cs:500,0.630858549893925)
--(axis cs:500,0.630858549893925)
--(axis cs:200,0.175752334968792)
--(axis cs:75,0.194949935788108)
--(axis cs:25,0.191690811891073)
--(axis cs:10,0.202372520726317)
--(axis cs:1,0.281672105413093)
--cycle;

\addplot [ultra thick, red, mark=*, mark size=1.5, mark options={solid}]
table {%
1 0.495427817106247
10 0.248387262225151
25 0.236766636371613
75 0.231731072068214
200 0.220703214406967
500 0.22512324154377
};
\addplot [ultra thick, blue,  mark=*, mark size=1.5, mark options={solid}]
table {%
1 0.495384305715561
10 0.251367211341858
25 0.207717821002007
75 0.203816741704941
200 0.185313686728477
500 0.186259418725967
};
\addplot [ultra thick, green!50.1960784313725!black,  mark=*, mark size=1.5, mark options={solid}]
table {%
1 0.299179285764694
10 0.170316502451897
25 0.179094910621643
75 0.153031080961227
200 0.145711228251457
500 0.152766168117523
};
\addplot [ultra thick, color0,  mark=*, mark size=1.5, mark options={solid}]
table {%
1 0.26467302441597
10 0.175934821367264
25 0.168692797422409
75 0.144676461815834
200 0.152819901704788
500 0.137696325778961
};
\addplot [ultra thick, white!40.1960784313725!black,  mark=*, mark size=1.5, mark options={solid}]
table {%
1 0.263067573308945
10 0.182245910167694
25 0.175642788410187
75 0.180577367544174
200 0.160431265830994
500 0.160534837245941
};

==> supp_mat/reacher_plots/train_test_loss_data.tex <==

% \path [fill=red, fill opacity=0.4, semithick]
% (axis cs:0,0.00179141961788069)
% --(axis cs:0,0.00155390987509309)
% --(axis cs:100,0.00124288381603113)
% --(axis cs:200,0.000992787645182912)
% --(axis cs:300,0.000578928659580938)
% --(axis cs:400,0.000262216404495599)
% --(axis cs:500,0.000128483936284261)
% --(axis cs:600,6.54250871837533e-05)
% --(axis cs:700,3.28227910577115e-05)
% --(axis cs:800,2.48945142645617e-05)
% --(axis cs:900,2.23920803690911e-05)
% --(axis cs:1000,2.15313664244051e-05)
% --(axis cs:1100,2.01580041546788e-05)
% --(axis cs:1200,1.80578071888529e-05)
% --(axis cs:1300,1.59432045958022e-05)
% --(axis cs:1400,1.55720563751308e-05)
% --(axis cs:1500,1.45986058277272e-05)
% --(axis cs:1600,1.54774000777758e-05)
% --(axis cs:1700,1.62177838499839e-05)
% --(axis cs:1800,1.54583277165291e-05)
% --(axis cs:1900,1.48908435452109e-05)
% --(axis cs:2000,1.57364521097621e-05)
% --(axis cs:2100,1.40675310781236e-05)
% --(axis cs:2200,1.24606531301863e-05)
% --(axis cs:2300,1.3361158045593e-05)
% --(axis cs:2400,1.3862862566117e-05)
% --(axis cs:2500,1.3172536524843e-05)
% --(axis cs:2600,1.3114163904623e-05)
% --(axis cs:2700,1.23647319149993e-05)
% --(axis cs:2800,1.26129727657457e-05)
% --(axis cs:2900,1.32218202174885e-05)
% --(axis cs:3000,1.32690503875569e-05)
% --(axis cs:3100,1.20050982100505e-05)
% --(axis cs:3200,1.19915452743054e-05)
% --(axis cs:3300,1.15875422990156e-05)
% --(axis cs:3400,1.25157086879547e-05)
% --(axis cs:3500,1.23324500008155e-05)
% --(axis cs:3600,1.22186410376493e-05)
% --(axis cs:3700,1.25331829310045e-05)
% --(axis cs:3800,1.15938687950607e-05)
% --(axis cs:3900,1.14944163821677e-05)
% --(axis cs:4000,1.15520449515552e-05)
% --(axis cs:4100,1.1904701635748e-05)
% --(axis cs:4200,1.16343733525235e-05)
% --(axis cs:4300,1.11896355800138e-05)
% --(axis cs:4400,1.13267729595196e-05)
% --(axis cs:4500,1.05409037888614e-05)
% --(axis cs:4600,1.06515699549389e-05)
% --(axis cs:4700,1.05963658577107e-05)
% --(axis cs:4800,1.07885188632418e-05)
% --(axis cs:4900,1.01431548859058e-05)
% --(axis cs:5000,9.57233358950686e-06)
% --(axis cs:5100,9.48006391444127e-06)
% --(axis cs:5200,9.79624038822544e-06)
% --(axis cs:5300,1.02281537573377e-05)
% --(axis cs:5400,9.73854242995412e-06)
% --(axis cs:5500,9.87581551662812e-06)
% --(axis cs:5600,9.677632057973e-06)
% --(axis cs:5700,9.77448085195009e-06)
% --(axis cs:5800,8.98970001301987e-06)
% --(axis cs:5900,9.18956370896465e-06)
% --(axis cs:6000,7.86368937616282e-06)
% --(axis cs:6100,8.20754295131139e-06)
% --(axis cs:6200,8.38318663112827e-06)
% --(axis cs:6300,8.93882922950056e-06)
% --(axis cs:6400,9.07510228724685e-06)
% --(axis cs:6500,8.83938409139333e-06)
% --(axis cs:6600,9.45071255367461e-06)
% --(axis cs:6700,9.3052876897137e-06)
% --(axis cs:6800,9.3912944040536e-06)
% --(axis cs:6900,9.43556189623782e-06)
% --(axis cs:7000,8.94813282520618e-06)
% --(axis cs:7100,8.92868328090217e-06)
% --(axis cs:7200,8.34722830108808e-06)
% --(axis cs:7300,8.69815090264179e-06)
% --(axis cs:7400,8.25798338692432e-06)
% --(axis cs:7500,8.07539720349436e-06)
% --(axis cs:7600,7.23401902401581e-06)
% --(axis cs:7700,7.70646359589829e-06)
% --(axis cs:7800,7.35209750493716e-06)
% --(axis cs:7900,7.1815924615284e-06)
% --(axis cs:8000,7.15512768846787e-06)
% --(axis cs:8100,7.5309005138227e-06)
% --(axis cs:8200,7.38776904466764e-06)
% --(axis cs:8300,7.20528430707263e-06)
% --(axis cs:8400,7.1499775937406e-06)
% --(axis cs:8500,7.20104680109622e-06)
% --(axis cs:8600,7.04369540666817e-06)
% --(axis cs:8700,6.28065718866066e-06)
% --(axis cs:8800,6.23452887422801e-06)
% --(axis cs:8900,6.63669005724983e-06)
% --(axis cs:9000,6.66542749726179e-06)
% --(axis cs:9100,6.0017504827027e-06)
% --(axis cs:9200,5.9089429481219e-06)
% --(axis cs:9300,6.20514575769934e-06)
% --(axis cs:9400,6.51332593749193e-06)
% --(axis cs:9500,6.28504935961126e-06)
% --(axis cs:9600,6.42938111726686e-06)
% --(axis cs:9700,6.28576867019246e-06)
% --(axis cs:9800,6.39352506432907e-06)
% --(axis cs:9900,6.01307415082145e-06)
% --(axis cs:10000,5.50734466777552e-06)
% --(axis cs:10100,5.76963240463989e-06)
% --(axis cs:10200,5.7969726038842e-06)
% --(axis cs:10300,6.01876169624183e-06)
% --(axis cs:10400,6.14794195847521e-06)
% --(axis cs:10500,6.31768714555274e-06)
% --(axis cs:10600,6.52132057221935e-06)
% --(axis cs:10700,6.24952239427851e-06)
% --(axis cs:10800,6.05455224915807e-06)
% --(axis cs:10900,5.95458843576812e-06)
% --(axis cs:11000,5.77203749418608e-06)
% --(axis cs:11100,5.42393736836482e-06)
% --(axis cs:11200,5.21222138980143e-06)
% --(axis cs:11300,5.21195763193625e-06)
% --(axis cs:11400,5.43418534274969e-06)
% --(axis cs:11500,5.59891022527712e-06)
% --(axis cs:11600,5.92916822374395e-06)
% --(axis cs:11700,6.04746936670912e-06)
% --(axis cs:11800,5.73491133060755e-06)
% --(axis cs:11900,5.75031021809988e-06)
% --(axis cs:12000,5.3380986177752e-06)
% --(axis cs:12100,5.17248595529025e-06)
% --(axis cs:12200,5.1039148667098e-06)
% --(axis cs:12300,4.76388023553704e-06)
% --(axis cs:12400,4.608638987619e-06)
% --(axis cs:12500,4.80806932989428e-06)
% --(axis cs:12600,4.71689956807827e-06)
% --(axis cs:12700,4.9017618258173e-06)
% --(axis cs:12800,4.97649337973459e-06)
% --(axis cs:12900,4.92305587458384e-06)
% --(axis cs:13000,4.98579913695962e-06)
% --(axis cs:13100,4.99310509386163e-06)
% --(axis cs:13200,4.88844260774946e-06)
% --(axis cs:13300,4.80112132242542e-06)
% --(axis cs:13400,5.05857166627454e-06)
% --(axis cs:13500,4.89613548004226e-06)
% --(axis cs:13600,4.7774998285649e-06)
% --(axis cs:13700,4.58238276396091e-06)
% --(axis cs:13800,4.45506884325851e-06)
% --(axis cs:13900,4.28919389910541e-06)
% --(axis cs:14000,4.26344600284871e-06)
% --(axis cs:14100,4.10752542851911e-06)
% --(axis cs:14200,4.10384488750238e-06)
% --(axis cs:14300,4.23149930002907e-06)
% --(axis cs:14400,4.36061515980916e-06)
% --(axis cs:14500,4.59278692305698e-06)
% --(axis cs:14600,4.44254912848744e-06)
% --(axis cs:14700,4.50534872288351e-06)
% --(axis cs:14800,4.17311649794375e-06)
% --(axis cs:14900,4.05186141079554e-06)
% --(axis cs:15000,4.04181665999651e-06)
% --(axis cs:15100,3.96611995629393e-06)
% --(axis cs:15200,3.85993848540781e-06)
% --(axis cs:15300,4.00613822159587e-06)
% --(axis cs:15400,3.90096232806042e-06)
% --(axis cs:15500,4.0044800582331e-06)
% --(axis cs:15600,3.84961275799291e-06)
% --(axis cs:15700,3.77631340441077e-06)
% --(axis cs:15800,3.59753355490293e-06)
% --(axis cs:15900,3.61362920379213e-06)
% --(axis cs:16000,3.6671870856577e-06)
% --(axis cs:16100,3.60380964734401e-06)
% --(axis cs:16200,3.73511269506217e-06)
% --(axis cs:16300,3.54627919421237e-06)
% --(axis cs:16400,3.65543993717726e-06)
% --(axis cs:16500,3.45649204776041e-06)
% --(axis cs:16600,3.42737669270519e-06)
% --(axis cs:16700,3.43788130475439e-06)
% --(axis cs:16800,3.57725920927742e-06)
% --(axis cs:16900,3.66800727355236e-06)
% --(axis cs:17000,3.43829515602411e-06)
% --(axis cs:17100,3.44643088329279e-06)
% --(axis cs:17200,3.49938617839972e-06)
% --(axis cs:17300,3.31374976269096e-06)
% --(axis cs:17400,3.4742660092826e-06)
% --(axis cs:17500,3.60217669388881e-06)
% --(axis cs:17600,3.81223885621414e-06)
% --(axis cs:17700,3.73446963697789e-06)
% --(axis cs:17800,3.65846111000355e-06)
% --(axis cs:17900,3.64335091257184e-06)
% --(axis cs:18000,3.63857040891158e-06)
% --(axis cs:18100,3.58268647352018e-06)
% --(axis cs:18200,3.54460273722364e-06)
% --(axis cs:18300,3.50898761405074e-06)
% --(axis cs:18400,3.4080078110777e-06)
% --(axis cs:18500,3.32267738408082e-06)
% --(axis cs:18600,3.30208092878528e-06)
% --(axis cs:18700,3.17597568309426e-06)
% --(axis cs:18800,3.11936198313309e-06)
% --(axis cs:18900,3.09936105219979e-06)
% --(axis cs:19000,3.13759269535947e-06)
% --(axis cs:19100,3.13299742175323e-06)
% --(axis cs:19200,3.12968589681454e-06)
% --(axis cs:19300,3.08786959103885e-06)
% --(axis cs:19400,3.01645053729994e-06)
% --(axis cs:19500,3.13085503509814e-06)
% --(axis cs:19600,3.09394806829675e-06)
% --(axis cs:19700,3.02668243347314e-06)
% --(axis cs:19800,3.08501728952604e-06)
% --(axis cs:19900,3.15939129364763e-06)
% --(axis cs:20000,3.05706174448033e-06)
% --(axis cs:20100,2.97106128547151e-06)
% --(axis cs:20200,2.95579635916221e-06)
% --(axis cs:20300,2.96441830440425e-06)
% --(axis cs:20400,2.96981151215086e-06)
% --(axis cs:20500,2.93938193046446e-06)
% --(axis cs:20600,2.97663533129562e-06)
% --(axis cs:20700,3.05273116279124e-06)
% --(axis cs:20800,2.86278452887578e-06)
% --(axis cs:20900,2.92385691995633e-06)
% --(axis cs:21000,2.62516413143858e-06)
% --(axis cs:21100,2.61549925514742e-06)
% --(axis cs:21200,2.58630307110612e-06)
% --(axis cs:21300,2.58647435300836e-06)
% --(axis cs:21400,2.56204986927808e-06)
% --(axis cs:21500,2.49080575175947e-06)
% --(axis cs:21600,2.42466785970823e-06)
% --(axis cs:21700,2.37490080109095e-06)
% --(axis cs:21800,2.3595368363157e-06)
% --(axis cs:21900,2.47005171486735e-06)
% --(axis cs:22000,2.44907676972573e-06)
% --(axis cs:22100,2.40465030712265e-06)
% --(axis cs:22200,2.33962948798377e-06)
% --(axis cs:22300,2.34508680933195e-06)
% --(axis cs:22400,2.275753154773e-06)
% --(axis cs:22500,2.2829746061002e-06)
% --(axis cs:22600,2.27471057685185e-06)
% --(axis cs:22700,2.29887331868391e-06)
% --(axis cs:22800,2.34516064464188e-06)
% --(axis cs:22900,2.42358451050467e-06)
% --(axis cs:23000,2.34426760487073e-06)
% --(axis cs:23100,2.3691906594401e-06)
% --(axis cs:23200,2.31272559711173e-06)
% --(axis cs:23300,2.25238495404517e-06)
% --(axis cs:23400,2.13924635151827e-06)
% --(axis cs:23500,2.05865157834008e-06)
% --(axis cs:23600,2.09538321491864e-06)
% --(axis cs:23700,2.01821876396566e-06)
% --(axis cs:23800,1.95603010478188e-06)
% --(axis cs:23900,2.05753516817903e-06)
% --(axis cs:24000,2.12862013061847e-06)
% --(axis cs:24100,2.11967686446033e-06)
% --(axis cs:24200,2.20741081579973e-06)
% --(axis cs:24300,2.2363223679421e-06)
% --(axis cs:24400,2.14411836978511e-06)
% --(axis cs:24500,2.06693066055474e-06)
% --(axis cs:24600,2.04586500557262e-06)
% --(axis cs:24700,1.93788973416736e-06)
% --(axis cs:24800,2.01806197128052e-06)
% --(axis cs:24900,2.02661362646642e-06)
% --(axis cs:25000,1.99883079363906e-06)
% --(axis cs:25100,2.11099169372207e-06)
% --(axis cs:25200,1.99964830224719e-06)
% --(axis cs:25300,1.95012818028076e-06)
% --(axis cs:25400,1.93599273379551e-06)
% --(axis cs:25500,1.94415984816236e-06)
% --(axis cs:25600,1.90234969065031e-06)
% --(axis cs:25700,1.89523263736534e-06)
% --(axis cs:25800,1.82024442462467e-06)
% --(axis cs:25900,1.79120576167134e-06)
% --(axis cs:26000,1.77335670989632e-06)
% --(axis cs:26100,1.78818545351202e-06)
% --(axis cs:26200,1.78189434938162e-06)
% --(axis cs:26300,1.74621534330804e-06)
% --(axis cs:26400,1.72966232615458e-06)
% --(axis cs:26500,1.71637818150428e-06)
% --(axis cs:26600,1.73118561194646e-06)
% --(axis cs:26700,1.75677825712739e-06)
% --(axis cs:26800,1.70134495092585e-06)
% --(axis cs:26900,1.67684125948197e-06)
% --(axis cs:27000,1.65291768447658e-06)
% --(axis cs:27100,1.64440019045589e-06)
% --(axis cs:27200,1.6327290297619e-06)
% --(axis cs:27300,1.62289886350989e-06)
% --(axis cs:27400,1.60268346424718e-06)
% --(axis cs:27500,1.66571827575673e-06)
% --(axis cs:27600,1.69046237381047e-06)
% --(axis cs:27700,1.65754867363525e-06)
% --(axis cs:27800,1.6409161237469e-06)
% --(axis cs:27900,1.62865150904399e-06)
% --(axis cs:28000,1.60371486919198e-06)
% --(axis cs:28100,1.57370394451883e-06)
% --(axis cs:28200,1.62385545830406e-06)
% --(axis cs:28300,1.57072118747107e-06)
% --(axis cs:28400,1.53576943039904e-06)
% --(axis cs:28500,1.57560172463148e-06)
% --(axis cs:28600,1.57232930071612e-06)
% --(axis cs:28700,1.49194142728533e-06)
% --(axis cs:28800,1.47990780496501e-06)
% --(axis cs:28900,1.46326263348337e-06)
% --(axis cs:29000,1.44552001094037e-06)
% --(axis cs:29100,1.44188249540353e-06)
% --(axis cs:29200,1.4457550839875e-06)
% --(axis cs:29300,1.42475821091264e-06)
% --(axis cs:29400,1.42195905533973e-06)
% --(axis cs:29500,1.4285715685467e-06)
% --(axis cs:29500,1.57704545557806e-06)
% --(axis cs:29500,1.57704545557806e-06)
% --(axis cs:29400,1.55136534379616e-06)
% --(axis cs:29300,1.54224965656996e-06)
% --(axis cs:29200,1.531082981188e-06)
% --(axis cs:29100,1.53433286906615e-06)
% --(axis cs:29000,1.52063303763029e-06)
% --(axis cs:28900,1.55177761977172e-06)
% --(axis cs:28800,1.6078541136611e-06)
% --(axis cs:28700,1.62061757637796e-06)
% --(axis cs:28600,1.60351730104265e-06)
% --(axis cs:28500,1.64316009706797e-06)
% --(axis cs:28400,1.69693308061444e-06)
% --(axis cs:28300,1.67554167733042e-06)
% --(axis cs:28200,1.70607529535163e-06)
% --(axis cs:28100,1.70639294173384e-06)
% --(axis cs:28000,1.72409527630057e-06)
% --(axis cs:27900,1.74611029998341e-06)
% --(axis cs:27800,1.72689227996231e-06)
% --(axis cs:27700,1.7603254731512e-06)
% --(axis cs:27600,1.73881497207207e-06)
% --(axis cs:27500,1.73202828337388e-06)
% --(axis cs:27400,1.75265655532946e-06)
% --(axis cs:27300,1.75087691683659e-06)
% --(axis cs:27200,1.68724644036292e-06)
% --(axis cs:27100,1.74752134311652e-06)
% --(axis cs:27000,1.76094951666051e-06)
% --(axis cs:26900,1.78487999067482e-06)
% --(axis cs:26800,1.78992737370728e-06)
% --(axis cs:26700,1.77196577975735e-06)
% --(axis cs:26600,1.76250340684997e-06)
% --(axis cs:26500,1.86112374507655e-06)
% --(axis cs:26400,1.86847485286637e-06)
% --(axis cs:26300,1.86967829488999e-06)
% --(axis cs:26200,1.87244279615688e-06)
% --(axis cs:26100,1.90838450293417e-06)
% --(axis cs:26000,1.91015701051681e-06)
% --(axis cs:25900,1.95785384734002e-06)
% --(axis cs:25800,1.979382392526e-06)
% --(axis cs:25700,1.9925218517009e-06)
% --(axis cs:25600,2.03151073798584e-06)
% --(axis cs:25500,2.12120354022493e-06)
% --(axis cs:25400,2.11457500994159e-06)
% --(axis cs:25300,2.09193007333639e-06)
% --(axis cs:25200,2.16820467984084e-06)
% --(axis cs:25100,2.12669826391663e-06)
% --(axis cs:25000,2.14725240200137e-06)
% --(axis cs:24900,2.15659937205075e-06)
% --(axis cs:24800,2.20676592744395e-06)
% --(axis cs:24700,2.1439204865012e-06)
% --(axis cs:24600,2.22002345633842e-06)
% --(axis cs:24500,2.26622339285313e-06)
% --(axis cs:24400,2.31627346186222e-06)
% --(axis cs:24300,2.36793195623138e-06)
% --(axis cs:24200,2.40982207355927e-06)
% --(axis cs:24100,2.37626293140368e-06)
% --(axis cs:24000,2.35992501857278e-06)
% --(axis cs:23900,2.30022641641193e-06)
% --(axis cs:23800,2.30621040419684e-06)
% --(axis cs:23700,2.20557244722299e-06)
% --(axis cs:23600,2.16468028206719e-06)
% --(axis cs:23500,2.21844305579816e-06)
% --(axis cs:23400,2.25119621229922e-06)
% --(axis cs:23300,2.32016315700665e-06)
% --(axis cs:23200,2.45738319559113e-06)
% --(axis cs:23100,2.39456376662988e-06)
% --(axis cs:23000,2.51596132010737e-06)
% --(axis cs:22900,2.47178169635752e-06)
% --(axis cs:22800,2.38714683492944e-06)
% --(axis cs:22700,2.52394279898275e-06)
% --(axis cs:22600,2.52450345602454e-06)
% --(axis cs:22500,2.53497923162483e-06)
% --(axis cs:22400,2.42508408007704e-06)
% --(axis cs:22300,2.49867136365423e-06)
% --(axis cs:22200,2.4110133744588e-06)
% --(axis cs:22100,2.48893465436612e-06)
% --(axis cs:22000,2.55315752023048e-06)
% --(axis cs:21900,2.59897319813593e-06)
% --(axis cs:21800,2.68562498207614e-06)
% --(axis cs:21700,2.72300061416836e-06)
% --(axis cs:21600,2.66187748343878e-06)
% --(axis cs:21500,2.63980391240916e-06)
% --(axis cs:21400,2.58182380498823e-06)
% --(axis cs:21300,2.63857698330222e-06)
% --(axis cs:21200,2.65228803409571e-06)
% --(axis cs:21100,2.82285020438631e-06)
% --(axis cs:21000,2.84848081658262e-06)
% --(axis cs:20900,3.05481946138998e-06)
% --(axis cs:20800,3.35467486609909e-06)
% --(axis cs:20700,3.44223010267362e-06)
% --(axis cs:20600,3.41697633144419e-06)
% --(axis cs:20500,3.3779789394548e-06)
% --(axis cs:20400,3.13768336438483e-06)
% --(axis cs:20300,3.05288389249549e-06)
% --(axis cs:20200,3.01581743202694e-06)
% --(axis cs:20100,3.16766885267101e-06)
% --(axis cs:20000,3.2762483883271e-06)
% --(axis cs:19900,3.30157827430125e-06)
% --(axis cs:19800,3.35977749116511e-06)
% --(axis cs:19700,3.44690382687767e-06)
% --(axis cs:19600,3.45783178682356e-06)
% --(axis cs:19500,3.45668775846985e-06)
% --(axis cs:19400,3.59340980105803e-06)
% --(axis cs:19300,3.53650464566896e-06)
% --(axis cs:19200,3.56876083227009e-06)
% --(axis cs:19100,3.42240958918722e-06)
% --(axis cs:19000,3.45500716159879e-06)
% --(axis cs:18900,3.4827673375096e-06)
% --(axis cs:18800,3.50636082200202e-06)
% --(axis cs:18700,3.57821021701726e-06)
% --(axis cs:18600,3.58073695946879e-06)
% --(axis cs:18500,3.63252139703775e-06)
% --(axis cs:18400,3.67285185120815e-06)
% --(axis cs:18300,3.82757966687003e-06)
% --(axis cs:18200,3.63365825970441e-06)
% --(axis cs:18100,3.81174734716791e-06)
% --(axis cs:18000,4.12155992330861e-06)
% --(axis cs:17900,4.06749860081524e-06)
% --(axis cs:17800,4.12248331163161e-06)
% --(axis cs:17700,4.52917169595796e-06)
% --(axis cs:17600,4.33107596387928e-06)
% --(axis cs:17500,4.29447188534948e-06)
% --(axis cs:17400,4.2800702353575e-06)
% --(axis cs:17300,4.50822445089336e-06)
% --(axis cs:17200,3.99831054901753e-06)
% --(axis cs:17100,4.09180857134434e-06)
% --(axis cs:17000,3.8268642397806e-06)
% --(axis cs:16900,3.86976145694362e-06)
% --(axis cs:16800,3.84226059743987e-06)
% --(axis cs:16700,3.90745984123789e-06)
% --(axis cs:16600,3.96115420420349e-06)
% --(axis cs:16500,3.95482645111662e-06)
% --(axis cs:16400,3.75686281686603e-06)
% --(axis cs:16300,3.82579985303594e-06)
% --(axis cs:16200,3.82001459067887e-06)
% --(axis cs:16100,4.05376236369247e-06)
% --(axis cs:16000,4.12853453304346e-06)
% --(axis cs:15900,4.20748793230174e-06)
% --(axis cs:15800,4.34140825600774e-06)
% --(axis cs:15700,4.22572978555519e-06)
% --(axis cs:15600,4.15346986315122e-06)
% --(axis cs:15500,4.46105354613695e-06)
% --(axis cs:15400,4.56261167902519e-06)
% --(axis cs:15300,4.5711773747924e-06)
% --(axis cs:15200,4.37210315139421e-06)
% --(axis cs:15100,4.27593867325448e-06)
% --(axis cs:15000,4.19022952427902e-06)
% --(axis cs:14900,4.55945337128175e-06)
% --(axis cs:14800,4.56553657669579e-06)
% --(axis cs:14700,4.82336971981916e-06)
% --(axis cs:14600,4.81845843411241e-06)
% --(axis cs:14500,4.76642196572474e-06)
% --(axis cs:14400,4.66433472035247e-06)
% --(axis cs:14300,4.62938567885312e-06)
% --(axis cs:14200,4.47842421114611e-06)
% --(axis cs:14100,4.62902031657993e-06)
% --(axis cs:14000,4.36651160162552e-06)
% --(axis cs:13900,4.52468129953048e-06)
% --(axis cs:13800,4.75343313546063e-06)
% --(axis cs:13700,4.87619399922368e-06)
% --(axis cs:13600,5.07448086875991e-06)
% --(axis cs:13500,5.17124751713124e-06)
% --(axis cs:13400,5.22293542689379e-06)
% --(axis cs:13300,5.53815275115688e-06)
% --(axis cs:13200,5.60384958383157e-06)
% --(axis cs:13100,5.51447503669341e-06)
% --(axis cs:13000,5.59925914951602e-06)
% --(axis cs:12900,5.48781992775195e-06)
% --(axis cs:12800,5.10943269858356e-06)
% --(axis cs:12700,5.15160464534228e-06)
% --(axis cs:12600,5.45208199083665e-06)
% --(axis cs:12500,5.32256102023415e-06)
% --(axis cs:12400,5.48501127761886e-06)
% --(axis cs:12300,5.76114748979437e-06)
% --(axis cs:12200,5.71436159911213e-06)
% --(axis cs:12100,5.44559653855412e-06)
% --(axis cs:12000,5.73851902985659e-06)
% --(axis cs:11900,6.12747873542204e-06)
% --(axis cs:11800,6.41818336686447e-06)
% --(axis cs:11700,6.33810309047248e-06)
% --(axis cs:11600,6.54155021792293e-06)
% --(axis cs:11500,6.63267853369737e-06)
% --(axis cs:11400,6.25830473669049e-06)
% --(axis cs:11300,6.12313922848464e-06)
% --(axis cs:11200,5.97980692149323e-06)
% --(axis cs:11100,6.11746593539233e-06)
% --(axis cs:11000,6.62635477588085e-06)
% --(axis cs:10900,7.1826972782696e-06)
% --(axis cs:10800,7.2741404447455e-06)
% --(axis cs:10700,7.51108909096511e-06)
% --(axis cs:10600,7.405010912762e-06)
% --(axis cs:10500,7.57368578841167e-06)
% --(axis cs:10400,7.31064337417704e-06)
% --(axis cs:10300,7.31852839044462e-06)
% --(axis cs:10200,7.5089578629532e-06)
% --(axis cs:10100,7.25992681488779e-06)
% --(axis cs:10000,6.46235084751485e-06)
% --(axis cs:9900,6.21754714832227e-06)
% --(axis cs:9800,6.46661354278533e-06)
% --(axis cs:9700,6.5925403071378e-06)
% --(axis cs:9600,6.88782835716512e-06)
% --(axis cs:9500,7.65219618305731e-06)
% --(axis cs:9400,7.79697050308272e-06)
% --(axis cs:9300,8.14129388105781e-06)
% --(axis cs:9200,8.15514897174123e-06)
% --(axis cs:9100,7.88430281675103e-06)
% --(axis cs:9000,7.37222589668464e-06)
% --(axis cs:8900,7.1073082946063e-06)
% --(axis cs:8800,7.52402606159596e-06)
% --(axis cs:8700,7.81982658523644e-06)
% --(axis cs:8600,8.23116321455256e-06)
% --(axis cs:8500,9.52780644793366e-06)
% --(axis cs:8400,9.75346541115657e-06)
% --(axis cs:8300,9.69945199929046e-06)
% --(axis cs:8200,9.63114334693364e-06)
% --(axis cs:8100,9.31546612030406e-06)
% --(axis cs:8000,8.16266369078302e-06)
% --(axis cs:7900,8.22500040394612e-06)
% --(axis cs:7800,8.07821686198198e-06)
% --(axis cs:7700,8.40403839351352e-06)
% --(axis cs:7600,8.19224906160812e-06)
% --(axis cs:7500,8.67576467727743e-06)
% --(axis cs:7400,8.81227040502291e-06)
% --(axis cs:7300,9.08616524829544e-06)
% --(axis cs:7200,9.83814008873446e-06)
% --(axis cs:7100,1.00370142220092e-05)
% --(axis cs:7000,9.96279466423254e-06)
% --(axis cs:6900,9.77557063423442e-06)
% --(axis cs:6800,1.0022283522214e-05)
% --(axis cs:6700,9.66911173723831e-06)
% --(axis cs:6600,9.82038793438989e-06)
% --(axis cs:6500,9.90536598310565e-06)
% --(axis cs:6400,9.65221823078735e-06)
% --(axis cs:6300,9.64766003574079e-06)
% --(axis cs:6200,9.74058150064426e-06)
% --(axis cs:6100,9.48133888980815e-06)
% --(axis cs:6000,9.54189523359405e-06)
% --(axis cs:5900,9.95802654973737e-06)
% --(axis cs:5800,1.00270389388848e-05)
% --(axis cs:5700,1.03874063350368e-05)
% --(axis cs:5600,1.15257438267274e-05)
% --(axis cs:5500,1.21803099370452e-05)
% --(axis cs:5400,1.10601498460487e-05)
% --(axis cs:5300,1.25309835734331e-05)
% --(axis cs:5200,1.26897185673357e-05)
% --(axis cs:5100,1.19834937268135e-05)
% --(axis cs:5000,1.26500385219695e-05)
% --(axis cs:4900,1.26658295454159e-05)
% --(axis cs:4800,1.14895886600167e-05)
% --(axis cs:4700,1.20241065153809e-05)
% --(axis cs:4600,1.29300244047729e-05)
% --(axis cs:4500,1.32277014777587e-05)
% --(axis cs:4400,1.30701330749581e-05)
% --(axis cs:4300,1.36368770677401e-05)
% --(axis cs:4200,1.31816573081595e-05)
% --(axis cs:4100,1.40971653244903e-05)
% --(axis cs:4000,1.39432913036586e-05)
% --(axis cs:3900,1.37051421309549e-05)
% --(axis cs:3800,1.34937795479237e-05)
% --(axis cs:3700,1.41005513502479e-05)
% --(axis cs:3600,1.31985202674364e-05)
% --(axis cs:3500,1.30964359036357e-05)
% --(axis cs:3400,1.39103931673193e-05)
% --(axis cs:3300,1.52915115646035e-05)
% --(axis cs:3200,1.52942723336602e-05)
% --(axis cs:3100,1.55582571631293e-05)
% --(axis cs:3000,1.63983353644067e-05)
% --(axis cs:2900,1.5569379924128e-05)
% --(axis cs:2800,1.59390212956235e-05)
% --(axis cs:2700,1.53757932686179e-05)
% --(axis cs:2600,1.49195536308131e-05)
% --(axis cs:2500,1.51989621283954e-05)
% --(axis cs:2400,1.56792618760183e-05)
% --(axis cs:2300,1.55426899269977e-05)
% --(axis cs:2200,1.60667617762344e-05)
% --(axis cs:2100,1.70792518524676e-05)
% --(axis cs:2000,1.67513704509866e-05)
% --(axis cs:1900,1.71282698295855e-05)
% --(axis cs:1800,1.74121229032342e-05)
% --(axis cs:1700,1.75919975058771e-05)
% --(axis cs:1600,1.63920627347376e-05)
% --(axis cs:1500,1.70930051745885e-05)
% --(axis cs:1400,1.72079385694454e-05)
% --(axis cs:1300,1.82146886462794e-05)
% --(axis cs:1200,2.11823259545653e-05)
% --(axis cs:1100,2.20883515544366e-05)
% --(axis cs:1000,2.17442610432598e-05)
% --(axis cs:900,2.33411927766516e-05)
% --(axis cs:800,2.7443793167803e-05)
% --(axis cs:700,3.34040970992502e-05)
% --(axis cs:600,7.66322221896838e-05)
% --(axis cs:500,0.000140631195190227)
% --(axis cs:400,0.000299285981233704)
% --(axis cs:300,0.000662737839536917)
% --(axis cs:200,0.00107441084856785)
% --(axis cs:100,0.00138377895130589)
% --(axis cs:0,0.00179141961788069)
% --cycle;

\path [fill=red, fill opacity=0.2, semithick]
(axis cs:0,0.00794493036430928)
--(axis cs:0,0.00792317748604364)
--(axis cs:100,0.0065848743385515)
--(axis cs:200,0.00505695469397237)
--(axis cs:300,0.00338619162290507)
--(axis cs:400,0.00178837855409415)
--(axis cs:500,0.000985278690901584)
--(axis cs:600,0.000611077999596422)
--(axis cs:700,0.000411842297425804)
--(axis cs:800,0.000362620296763487)
--(axis cs:900,0.00032752720172402)
--(axis cs:1000,0.000298620624552315)
--(axis cs:1100,0.000274931584658309)
--(axis cs:1200,0.000256637012007072)
--(axis cs:1300,0.000239079197735861)
--(axis cs:1400,0.000227048416274827)
--(axis cs:1500,0.000220975328405741)
--(axis cs:1600,0.000218077592382846)
--(axis cs:1700,0.000218268167210757)
--(axis cs:1800,0.000223572788044673)
--(axis cs:1900,0.000216262209326544)
--(axis cs:2000,0.000216134550285422)
--(axis cs:2100,0.000206434984208891)
--(axis cs:2200,0.000196638351471821)
--(axis cs:2300,0.000192853864107725)
--(axis cs:2400,0.000192488475725672)
--(axis cs:2500,0.000181977671597006)
--(axis cs:2600,0.000193789453890256)
--(axis cs:2700,0.000191861720970051)
--(axis cs:2800,0.000189198273112381)
--(axis cs:2900,0.000186987592602992)
--(axis cs:3000,0.000188927373928458)
--(axis cs:3100,0.000178195244880903)
--(axis cs:3200,0.000177978741144972)
--(axis cs:3300,0.000168760374247822)
--(axis cs:3400,0.000172218884219902)
--(axis cs:3500,0.000173278593058551)
--(axis cs:3600,0.000173642177965453)
--(axis cs:3700,0.000175903710590367)
--(axis cs:3800,0.000175616518978398)
--(axis cs:3900,0.000171243987413393)
--(axis cs:4000,0.000169711803702109)
--(axis cs:4100,0.000172825859043403)
--(axis cs:4200,0.00017236576936298)
--(axis cs:4300,0.000167693011248602)
--(axis cs:4400,0.000165745695194825)
--(axis cs:4500,0.000157824339609176)
--(axis cs:4600,0.000155564772431313)
--(axis cs:4700,0.000148252324687529)
--(axis cs:4800,0.000149367310081661)
--(axis cs:4900,0.000152981530923669)
--(axis cs:5000,0.000152889420849398)
--(axis cs:5100,0.000147283398922225)
--(axis cs:5200,0.000145814326850031)
--(axis cs:5300,0.000147103999147593)
--(axis cs:5400,0.00014019135093937)
--(axis cs:5500,0.000138729337938435)
--(axis cs:5600,0.000135316352496103)
--(axis cs:5700,0.000134348546188495)
--(axis cs:5800,0.000132778985794949)
--(axis cs:5900,0.000127986694617333)
--(axis cs:6000,0.000122391485642451)
--(axis cs:6100,0.000119164870861333)
--(axis cs:6200,0.00011835470386704)
--(axis cs:6300,0.000118808475676171)
--(axis cs:6400,0.000127250914921902)
--(axis cs:6500,0.000131158108964106)
--(axis cs:6600,0.000130498443353996)
--(axis cs:6700,0.000129413847596205)
--(axis cs:6800,0.000125474108149665)
--(axis cs:6900,0.000120387282425768)
--(axis cs:7000,0.000119421465560608)
--(axis cs:7100,0.000115416109527837)
--(axis cs:7200,0.00011377626160185)
--(axis cs:7300,0.000110506571396613)
--(axis cs:7400,0.000109320596650683)
--(axis cs:7500,0.000110172643009107)
--(axis cs:7600,0.000108654176890762)
--(axis cs:7700,0.000110822891665448)
--(axis cs:7800,0.000111526415500908)
--(axis cs:7900,0.000107629612079876)
--(axis cs:8000,0.000106519207011028)
--(axis cs:8100,0.000114105240695766)
--(axis cs:8200,0.00011192825895394)
--(axis cs:8300,0.000110275823562246)
--(axis cs:8400,0.00010731690121422)
--(axis cs:8500,0.000104498582287293)
--(axis cs:8600,0.000101130344683152)
--(axis cs:8700,9.7064374837615e-05)
--(axis cs:8800,9.55297146709891e-05)
--(axis cs:8900,9.49607405595845e-05)
--(axis cs:9000,9.60820538784582e-05)
--(axis cs:9100,9.53089628301208e-05)
--(axis cs:9200,9.67427625011389e-05)
--(axis cs:9300,9.72594501880651e-05)
--(axis cs:9400,9.68474497851896e-05)
--(axis cs:9500,9.65894041970606e-05)
--(axis cs:9600,9.21167071537533e-05)
--(axis cs:9700,9.26127978979672e-05)
--(axis cs:9800,9.19084957854828e-05)
--(axis cs:9900,9.12098430058818e-05)
--(axis cs:10000,9.03305944269132e-05)
--(axis cs:10100,9.28310957138549e-05)
--(axis cs:10200,9.29976050804488e-05)
--(axis cs:10300,9.49488040776608e-05)
--(axis cs:10400,9.47096782704783e-05)
--(axis cs:10500,9.61527941204935e-05)
--(axis cs:10600,9.43855082559888e-05)
--(axis cs:10700,9.36486474895074e-05)
--(axis cs:10800,9.33742647764567e-05)
--(axis cs:10900,9.2190950556113e-05)
--(axis cs:11000,8.92080258762501e-05)
--(axis cs:11100,8.5679747917207e-05)
--(axis cs:11200,8.63538395311443e-05)
--(axis cs:11300,8.70492305019831e-05)
--(axis cs:11400,8.98741150221174e-05)
--(axis cs:11500,9.27909559756554e-05)
--(axis cs:11600,9.39604507751447e-05)
--(axis cs:11700,9.34806069832737e-05)
--(axis cs:11800,9.17766170002406e-05)
--(axis cs:11900,8.9181388285441e-05)
--(axis cs:12000,8.84940236975647e-05)
--(axis cs:12100,8.80666981372847e-05)
--(axis cs:12200,8.86013060442862e-05)
--(axis cs:12300,8.59349481294773e-05)
--(axis cs:12400,8.71945962378165e-05)
--(axis cs:12500,8.84944876808836e-05)
--(axis cs:12600,8.8029088221035e-05)
--(axis cs:12700,8.82447335970224e-05)
--(axis cs:12800,8.83636920626717e-05)
--(axis cs:12900,8.56956435743977e-05)
--(axis cs:13000,8.63622709150731e-05)
--(axis cs:13100,8.66251762703017e-05)
--(axis cs:13200,8.54606810729679e-05)
--(axis cs:13300,8.50161033227789e-05)
--(axis cs:13400,8.60783544904851e-05)
--(axis cs:13500,8.67805893501232e-05)
--(axis cs:13600,8.4347776174095e-05)
--(axis cs:13700,8.46066353589163e-05)
--(axis cs:13800,8.35187667107613e-05)
--(axis cs:13900,8.36384131956795e-05)
--(axis cs:14000,8.20011899932928e-05)
--(axis cs:14100,8.20695569435454e-05)
--(axis cs:14200,8.15318789526242e-05)
--(axis cs:14300,8.32358559580136e-05)
--(axis cs:14400,8.32642403535338e-05)
--(axis cs:14500,8.25459769360737e-05)
--(axis cs:14600,8.23704208177882e-05)
--(axis cs:14700,8.36477270763379e-05)
--(axis cs:14800,8.04299475858256e-05)
--(axis cs:14900,7.91436596050231e-05)
--(axis cs:15000,7.79270213966436e-05)
--(axis cs:15100,7.75396331603952e-05)
--(axis cs:15200,7.55497428870005e-05)
--(axis cs:15300,7.67525877888417e-05)
--(axis cs:15400,7.84932585196413e-05)
--(axis cs:15500,7.94264469060556e-05)
--(axis cs:15600,7.8085255372489e-05)
--(axis cs:15700,7.82438081586132e-05)
--(axis cs:15800,7.80856239388613e-05)
--(axis cs:15900,7.63595080269357e-05)
--(axis cs:16000,7.5460649638751e-05)
--(axis cs:16100,7.46196097397629e-05)
--(axis cs:16200,7.5903055897795e-05)
--(axis cs:16300,7.58335417131963e-05)
--(axis cs:16400,7.70768168157377e-05)
--(axis cs:16500,7.54256031061275e-05)
--(axis cs:16600,7.63348006004477e-05)
--(axis cs:16700,7.54307535155135e-05)
--(axis cs:16800,7.43807592522468e-05)
--(axis cs:16900,7.3736714129013e-05)
--(axis cs:17000,7.42769088927572e-05)
--(axis cs:17100,7.34832200798359e-05)
--(axis cs:17200,7.28710887031161e-05)
--(axis cs:17300,7.4204123397513e-05)
--(axis cs:17400,7.49344799023913e-05)
--(axis cs:17500,7.46213388153844e-05)
--(axis cs:17600,7.52874054039201e-05)
--(axis cs:17700,7.48927131702648e-05)
--(axis cs:17800,7.40453719209013e-05)
--(axis cs:17900,7.19245245512281e-05)
--(axis cs:18000,7.33578404874997e-05)
--(axis cs:18100,7.42160416268778e-05)
--(axis cs:18200,7.40627210928966e-05)
--(axis cs:18300,7.45572609541029e-05)
--(axis cs:18400,7.47634906466555e-05)
--(axis cs:18500,7.35666419237113e-05)
--(axis cs:18600,7.14857202751341e-05)
--(axis cs:18700,7.09770022904407e-05)
--(axis cs:18800,7.16626408077917e-05)
--(axis cs:18900,7.14616258339688e-05)
--(axis cs:19000,7.20721489187934e-05)
--(axis cs:19100,7.34633483038463e-05)
--(axis cs:19200,7.37075197535939e-05)
--(axis cs:19300,7.42347211622872e-05)
--(axis cs:19400,7.46640853860299e-05)
--(axis cs:19500,7.42388061509685e-05)
--(axis cs:19600,7.27306758206246e-05)
--(axis cs:19700,7.29040922719206e-05)
--(axis cs:19800,7.16890926129019e-05)
--(axis cs:19900,7.10565889017966e-05)
--(axis cs:20000,7.03462727306229e-05)
--(axis cs:20100,7.14104196090918e-05)
--(axis cs:20200,7.16507847541647e-05)
--(axis cs:20300,7.36060615740641e-05)
--(axis cs:20400,7.42676700619262e-05)
--(axis cs:20500,7.40111675739607e-05)
--(axis cs:20600,7.31077953366388e-05)
--(axis cs:20700,7.31965385373868e-05)
--(axis cs:20800,7.12968702897036e-05)
--(axis cs:20900,7.14124880913654e-05)
--(axis cs:21000,7.16170533260604e-05)
--(axis cs:21100,7.13899477860111e-05)
--(axis cs:21200,7.09489684907658e-05)
--(axis cs:21300,7.02368598766867e-05)
--(axis cs:21400,6.98624675983925e-05)
--(axis cs:21500,6.96665501465548e-05)
--(axis cs:21600,7.04190586709522e-05)
--(axis cs:21700,7.07105144436147e-05)
--(axis cs:21800,7.07483719544172e-05)
--(axis cs:21900,7.19195168427021e-05)
--(axis cs:22000,7.10528053734549e-05)
--(axis cs:22100,7.12202407139552e-05)
--(axis cs:22200,6.95015629673265e-05)
--(axis cs:22300,6.97350830707862e-05)
--(axis cs:22400,6.89426750344256e-05)
--(axis cs:22500,6.89246765286983e-05)
--(axis cs:22600,6.76330911186871e-05)
--(axis cs:22700,6.78451532285383e-05)
--(axis cs:22800,6.70843058416883e-05)
--(axis cs:22900,6.67929934421954e-05)
--(axis cs:23000,6.70843289817083e-05)
--(axis cs:23100,6.78242036725681e-05)
--(axis cs:23200,6.90571766078277e-05)
--(axis cs:23300,6.89457622451572e-05)
--(axis cs:23400,6.98363685248496e-05)
--(axis cs:23500,6.96262648772451e-05)
--(axis cs:23600,7.01659608131377e-05)
--(axis cs:23700,6.86628355803345e-05)
--(axis cs:23800,6.87498834435233e-05)
--(axis cs:23900,6.84284833825952e-05)
--(axis cs:24000,6.82793248242338e-05)
--(axis cs:24100,6.79880178527122e-05)
--(axis cs:24200,6.92752146496692e-05)
--(axis cs:24300,6.8843109935723e-05)
--(axis cs:24400,6.85384142048596e-05)
--(axis cs:24500,6.83184156041719e-05)
--(axis cs:24600,6.73594546287464e-05)
--(axis cs:24700,6.73095012931081e-05)
--(axis cs:24800,6.73684105802712e-05)
--(axis cs:24900,6.64009526094589e-05)
--(axis cs:25000,6.55053337791316e-05)
--(axis cs:25100,6.58480979859444e-05)
--(axis cs:25200,6.57219587425822e-05)
--(axis cs:25300,6.57552460248583e-05)
--(axis cs:25400,6.57391665638293e-05)
--(axis cs:25500,6.64376728685177e-05)
--(axis cs:25600,6.56948340151946e-05)
--(axis cs:25700,6.58319944352881e-05)
--(axis cs:25800,6.61122446801713e-05)
--(axis cs:25900,6.626389214239e-05)
--(axis cs:26000,6.59013438419499e-05)
--(axis cs:26100,6.61835691913976e-05)
--(axis cs:26200,6.58787345647683e-05)
--(axis cs:26300,6.60659145475971e-05)
--(axis cs:26400,6.59565868945148e-05)
--(axis cs:26500,6.57882429986464e-05)
--(axis cs:26600,6.5244260908148e-05)
--(axis cs:26700,6.51380424601179e-05)
--(axis cs:26800,6.51656649538671e-05)
--(axis cs:26900,6.51529735151676e-05)
--(axis cs:27000,6.45814763201072e-05)
--(axis cs:27100,6.42804429928451e-05)
--(axis cs:27200,6.41661852927335e-05)
--(axis cs:27300,6.38788239454142e-05)
--(axis cs:27400,6.41202570635051e-05)
--(axis cs:27500,6.48989302683124e-05)
--(axis cs:27600,6.52201841775685e-05)
--(axis cs:27700,6.53009780458412e-05)
--(axis cs:27800,6.49674332740775e-05)
--(axis cs:27900,6.46572846144236e-05)
--(axis cs:28000,6.46290614645067e-05)
--(axis cs:28100,6.46342242204233e-05)
--(axis cs:28200,6.45448333388738e-05)
--(axis cs:28300,6.49180989119943e-05)
--(axis cs:28400,6.49763207367949e-05)
--(axis cs:28500,6.53680924184854e-05)
--(axis cs:28600,6.56755132748502e-05)
--(axis cs:28700,6.54337871336116e-05)
--(axis cs:28800,6.50589041017106e-05)
--(axis cs:28900,6.48777925701976e-05)
--(axis cs:29000,6.42724983886354e-05)
--(axis cs:29100,6.40650955277576e-05)
--(axis cs:29200,6.41449436048882e-05)
--(axis cs:29300,6.48019684853355e-05)
--(axis cs:29400,6.50493228966052e-05)
--(axis cs:29500,6.47546491567011e-05)
--(axis cs:29500,6.91619904497673e-05)
--(axis cs:29500,6.91619904497673e-05)
--(axis cs:29400,6.93031252281437e-05)
--(axis cs:29300,6.96568240657747e-05)
--(axis cs:29200,6.98749593024238e-05)
--(axis cs:29100,7.0252898512369e-05)
--(axis cs:29000,7.03048573469894e-05)
--(axis cs:28900,7.03708866706574e-05)
--(axis cs:28800,6.99189339227865e-05)
--(axis cs:28700,6.96442408272327e-05)
--(axis cs:28600,6.9209126523503e-05)
--(axis cs:28500,6.91665796393916e-05)
--(axis cs:28400,6.90388760811321e-05)
--(axis cs:28300,6.93251390292212e-05)
--(axis cs:28200,6.9099871717339e-05)
--(axis cs:28100,6.91869839259775e-05)
--(axis cs:28000,6.89130380374309e-05)
--(axis cs:27900,6.8741163231018e-05)
--(axis cs:27800,6.87219801163553e-05)
--(axis cs:27700,6.89914987258687e-05)
--(axis cs:27600,6.8952917412757e-05)
--(axis cs:27500,6.88829372603323e-05)
--(axis cs:27400,6.89959874301681e-05)
--(axis cs:27300,6.92185137298667e-05)
--(axis cs:27200,6.89500145750664e-05)
--(axis cs:27100,6.962891192486e-05)
--(axis cs:27000,7.00201461893524e-05)
--(axis cs:26900,7.05470391972613e-05)
--(axis cs:26800,7.0141827307575e-05)
--(axis cs:26700,7.04632801333599e-05)
--(axis cs:26600,6.9588373255562e-05)
--(axis cs:26500,6.92868124909806e-05)
--(axis cs:26400,6.84054858669663e-05)
--(axis cs:26300,6.86043571070162e-05)
--(axis cs:26200,6.84492915657168e-05)
--(axis cs:26100,6.90382540048397e-05)
--(axis cs:26000,6.8978203756201e-05)
--(axis cs:25900,6.95363153570247e-05)
--(axis cs:25800,6.95054303855126e-05)
--(axis cs:25700,7.03898713000391e-05)
--(axis cs:25600,6.98537572881341e-05)
--(axis cs:25500,7.03163990923289e-05)
--(axis cs:25400,7.03759599031702e-05)
--(axis cs:25300,7.01766553372454e-05)
--(axis cs:25200,6.98380373817747e-05)
--(axis cs:25100,7.01521498414763e-05)
--(axis cs:25000,6.97261809926478e-05)
--(axis cs:24900,6.95579687488408e-05)
--(axis cs:24800,6.96263083429622e-05)
--(axis cs:24700,6.97302354350758e-05)
--(axis cs:24600,7.06168860491531e-05)
--(axis cs:24500,7.10122456305844e-05)
--(axis cs:24400,7.0802675902477e-05)
--(axis cs:24300,7.08978716527276e-05)
--(axis cs:24200,7.06873935778371e-05)
--(axis cs:24100,7.1554361136957e-05)
--(axis cs:24000,7.18045095882739e-05)
--(axis cs:23900,7.27557096219484e-05)
--(axis cs:23800,7.26332701369163e-05)
--(axis cs:23700,7.28456633472439e-05)
--(axis cs:23600,7.30108948226916e-05)
--(axis cs:23500,7.23178708560141e-05)
--(axis cs:23400,7.06909937119035e-05)
--(axis cs:23300,7.08533406628431e-05)
--(axis cs:23200,7.13172760439611e-05)
--(axis cs:23100,7.02004134691655e-05)
--(axis cs:23000,7.00795937910345e-05)
--(axis cs:22900,7.08855403503003e-05)
--(axis cs:22800,7.14441791258489e-05)
--(axis cs:22700,7.19818088361029e-05)
--(axis cs:22600,7.29256528083198e-05)
--(axis cs:22500,7.43890156166616e-05)
--(axis cs:22400,7.44422002295931e-05)
--(axis cs:22300,7.47949406102136e-05)
--(axis cs:22200,7.41654913952686e-05)
--(axis cs:22100,7.38757486657662e-05)
--(axis cs:22000,7.3356216222038e-05)
--(axis cs:21900,7.35241401047616e-05)
--(axis cs:21800,7.32776568140527e-05)
--(axis cs:21700,7.27547727637006e-05)
--(axis cs:21600,7.26289737099987e-05)
--(axis cs:21500,7.30937617665009e-05)
--(axis cs:21400,7.29121789212908e-05)
--(axis cs:21300,7.38453344339263e-05)
--(axis cs:21200,7.37480490888841e-05)
--(axis cs:21100,7.3278517965833e-05)
--(axis cs:21000,7.34776690669084e-05)
--(axis cs:20900,7.48121992502352e-05)
--(axis cs:20800,7.71818543936209e-05)
--(axis cs:20700,7.74985010428789e-05)
--(axis cs:20600,7.8283045040399e-05)
--(axis cs:20500,7.86529052376428e-05)
--(axis cs:20400,7.81492462305449e-05)
--(axis cs:20300,7.59295347578278e-05)
--(axis cs:20200,7.69959417904712e-05)
--(axis cs:20100,7.76766886357172e-05)
--(axis cs:20000,7.7841823042016e-05)
--(axis cs:19900,7.7932574282121e-05)
--(axis cs:19800,7.75639326888302e-05)
--(axis cs:19700,7.71267241676186e-05)
--(axis cs:19600,7.65657976194687e-05)
--(axis cs:19500,7.66572109006438e-05)
--(axis cs:19400,7.69232533828472e-05)
--(axis cs:19300,7.76938493472906e-05)
--(axis cs:19200,7.80679626675261e-05)
--(axis cs:19100,7.87813955484089e-05)
--(axis cs:19000,7.85902720584241e-05)
--(axis cs:18900,7.78911683686967e-05)
--(axis cs:18800,7.8636883537333e-05)
--(axis cs:18700,7.82909755892524e-05)
--(axis cs:18600,7.75761122630509e-05)
--(axis cs:18500,7.78622740245853e-05)
--(axis cs:18400,7.76135922031973e-05)
--(axis cs:18300,7.66414504861747e-05)
--(axis cs:18200,7.65465902443758e-05)
--(axis cs:18100,7.62305783280137e-05)
--(axis cs:18000,7.66674219710606e-05)
--(axis cs:17900,7.73792141750749e-05)
--(axis cs:17800,7.79882352829225e-05)
--(axis cs:17700,8.1604125535039e-05)
--(axis cs:17600,8.22660983127549e-05)
--(axis cs:17500,8.31279512194114e-05)
--(axis cs:17400,8.34596229584717e-05)
--(axis cs:17300,8.36190263382159e-05)
--(axis cs:17200,8.23526989814983e-05)
--(axis cs:17100,8.20951065868918e-05)
--(axis cs:17000,8.09267049867124e-05)
--(axis cs:16900,8.1084149455354e-05)
--(axis cs:16800,8.10379600680008e-05)
--(axis cs:16700,8.07754378466787e-05)
--(axis cs:16600,8.18477358454209e-05)
--(axis cs:16500,8.25109817191896e-05)
--(axis cs:16400,8.27559407714964e-05)
--(axis cs:16300,8.46424726153033e-05)
--(axis cs:16200,8.57161927857694e-05)
--(axis cs:16100,8.65288340395244e-05)
--(axis cs:16000,8.70853523180471e-05)
--(axis cs:15900,8.76210877017572e-05)
--(axis cs:15800,8.67758777989469e-05)
--(axis cs:15700,8.62128214625622e-05)
--(axis cs:15600,8.60368703434596e-05)
--(axis cs:15500,8.67120077059785e-05)
--(axis cs:15400,8.51255824172405e-05)
--(axis cs:15300,8.51943351010689e-05)
--(axis cs:15200,8.44609060431344e-05)
--(axis cs:15100,8.37985831155128e-05)
--(axis cs:15000,8.38048833639804e-05)
--(axis cs:14900,8.38162046416359e-05)
--(axis cs:14800,8.43295083613798e-05)
--(axis cs:14700,8.5107807028665e-05)
--(axis cs:14600,8.55294111952749e-05)
--(axis cs:14500,8.51578310775865e-05)
--(axis cs:14400,8.79181011320609e-05)
--(axis cs:14300,8.79159061329202e-05)
--(axis cs:14200,8.90919968913577e-05)
--(axis cs:14100,8.95045657557426e-05)
--(axis cs:14000,8.91202080713255e-05)
--(axis cs:13900,8.88254203915646e-05)
--(axis cs:13800,9.08230584755137e-05)
--(axis cs:13700,9.11135928337907e-05)
--(axis cs:13600,9.50887230400153e-05)
--(axis cs:13500,9.56267842511371e-05)
--(axis cs:13400,9.35233991833415e-05)
--(axis cs:13300,9.26955816325051e-05)
--(axis cs:13200,9.28609221857933e-05)
--(axis cs:13100,9.04664942627196e-05)
--(axis cs:13000,8.93851984629413e-05)
--(axis cs:12900,8.98846213872598e-05)
--(axis cs:12800,8.99240847840774e-05)
--(axis cs:12700,8.98435665659039e-05)
--(axis cs:12600,9.04488113384281e-05)
--(axis cs:12500,8.89450987725666e-05)
--(axis cs:12400,9.0823362877279e-05)
--(axis cs:12300,9.2780443537151e-05)
--(axis cs:12200,9.13512913953134e-05)
--(axis cs:12100,9.30159079066923e-05)
--(axis cs:12000,9.36248504232718e-05)
--(axis cs:11900,9.53062601780565e-05)
--(axis cs:11800,9.55877986146251e-05)
--(axis cs:11700,9.68399516298925e-05)
--(axis cs:11600,9.68284602595188e-05)
--(axis cs:11500,9.87916126350525e-05)
--(axis cs:11400,0.000100291295921522)
--(axis cs:11300,9.93126765092253e-05)
--(axis cs:11200,9.77097622420879e-05)
--(axis cs:11100,9.79798936594134e-05)
--(axis cs:11000,0.000101270247364289)
--(axis cs:10900,0.000103350020333738)
--(axis cs:10800,0.000102261975562139)
--(axis cs:10700,0.000105462992808611)
--(axis cs:10600,0.000104946542141072)
--(axis cs:10500,0.00010309171777532)
--(axis cs:10400,0.000101618817048213)
--(axis cs:10300,0.00010442035467336)
--(axis cs:10200,0.000105192919356395)
--(axis cs:10100,0.000105976663729443)
--(axis cs:10000,0.000102889131585796)
--(axis cs:9900,0.000100706984067749)
--(axis cs:9800,0.000101071154670044)
--(axis cs:9700,0.000100728794584013)
--(axis cs:9600,0.000101813803277775)
--(axis cs:9500,0.000100794071021218)
--(axis cs:9400,0.000102762088172978)
--(axis cs:9300,0.000103140569148116)
--(axis cs:9200,0.000104656016865337)
--(axis cs:9100,0.000107681648602931)
--(axis cs:9000,0.000107483620140588)
--(axis cs:8900,0.000106798393704457)
--(axis cs:8800,0.0001051147302749)
--(axis cs:8700,0.000106148314343864)
--(axis cs:8600,0.000106449966036246)
--(axis cs:8500,0.000114142248235731)
--(axis cs:8400,0.000115653796387726)
--(axis cs:8300,0.00011626685215021)
--(axis cs:8200,0.000118023586101196)
--(axis cs:8100,0.000118395520741153)
--(axis cs:8000,0.000116107462942239)
--(axis cs:7900,0.00011755555135565)
--(axis cs:7800,0.000115459865646008)
--(axis cs:7700,0.000115909083121321)
--(axis cs:7600,0.000114017379900218)
--(axis cs:7500,0.000120457840313981)
--(axis cs:7400,0.000121880895094816)
--(axis cs:7300,0.000122250096141002)
--(axis cs:7200,0.000123237601720164)
--(axis cs:7100,0.000124571133051002)
--(axis cs:7000,0.000121984774047384)
--(axis cs:6900,0.000136805625700783)
--(axis cs:6800,0.000150518503661521)
--(axis cs:6700,0.000148748587683023)
--(axis cs:6600,0.000150864835079374)
--(axis cs:6500,0.000147152632644236)
--(axis cs:6400,0.000145773039243887)
--(axis cs:6300,0.000140859944121113)
--(axis cs:6200,0.00014010768521033)
--(axis cs:6100,0.000142531782268821)
--(axis cs:6000,0.000144817633792639)
--(axis cs:5900,0.000143207791795818)
--(axis cs:5800,0.000140155969827431)
--(axis cs:5700,0.0001450835679476)
--(axis cs:5600,0.000155043374921327)
--(axis cs:5500,0.000155513180006611)
--(axis cs:5400,0.000153316120663661)
--(axis cs:5300,0.000160129250232971)
--(axis cs:5200,0.000159388779016257)
--(axis cs:5100,0.000152628706236988)
--(axis cs:5000,0.00015620427925158)
--(axis cs:4900,0.000158546074012022)
--(axis cs:4800,0.000161689020407954)
--(axis cs:4700,0.000170593690649705)
--(axis cs:4600,0.000171985255631423)
--(axis cs:4500,0.000173564966814389)
--(axis cs:4400,0.00018204455295394)
--(axis cs:4300,0.000184299546740831)
--(axis cs:4200,0.000183282939865283)
--(axis cs:4100,0.00018467234622349)
--(axis cs:4000,0.00018381312140751)
--(axis cs:3900,0.000181656276362368)
--(axis cs:3800,0.000183107974244534)
--(axis cs:3700,0.000183286917342181)
--(axis cs:3600,0.000189150277936249)
--(axis cs:3500,0.000190583405329372)
--(axis cs:3400,0.000186250201547963)
--(axis cs:3300,0.000192229863817698)
--(axis cs:3200,0.000190940866572572)
--(axis cs:3100,0.000197574587678648)
--(axis cs:3000,0.000207758539509519)
--(axis cs:2900,0.000214278501228518)
--(axis cs:2800,0.000213409303576371)
--(axis cs:2700,0.000218547457614763)
--(axis cs:2600,0.000217739182190267)
--(axis cs:2500,0.000216569751940814)
--(axis cs:2400,0.000209891373191033)
--(axis cs:2300,0.000211435046687278)
--(axis cs:2200,0.000211742117447431)
--(axis cs:2100,0.0002152653824086)
--(axis cs:2000,0.000226381764511681)
--(axis cs:1900,0.000238366702551749)
--(axis cs:1800,0.000234648231123401)
--(axis cs:1700,0.000244962568023539)
--(axis cs:1600,0.000247852969385046)
--(axis cs:1500,0.000246498755010423)
--(axis cs:1400,0.000250404794349108)
--(axis cs:1300,0.000263884536977211)
--(axis cs:1200,0.00027354119651791)
--(axis cs:1100,0.000287363608815189)
--(axis cs:1000,0.000316635532918552)
--(axis cs:900,0.000336890663030776)
--(axis cs:800,0.000370540757322453)
--(axis cs:700,0.000442363081526322)
--(axis cs:600,0.000663961720752591)
--(axis cs:500,0.00103819168757927)
--(axis cs:400,0.00186996323304045)
--(axis cs:300,0.00346133319078174)
--(axis cs:200,0.00511083696938624)
--(axis cs:100,0.0066082193052827)
--(axis cs:0,0.00794493036430928)
--cycle;

% \path [fill=blue, fill opacity=0.4, semithick]
% (axis cs:0,0.00157419282920996)
% --(axis cs:0,0.00133076806807553)
% --(axis cs:100,0.00105293332777753)
% --(axis cs:200,0.000835445680698698)
% --(axis cs:300,0.000471442362512845)
% --(axis cs:400,0.000194163656672847)
% --(axis cs:500,0.000104072299877457)
% --(axis cs:600,5.62409077843989e-05)
% --(axis cs:700,2.31242849896771e-05)
% --(axis cs:800,2.08354464675608e-05)
% --(axis cs:900,2.0242977187108e-05)
% --(axis cs:1000,1.86737172838088e-05)
% --(axis cs:1100,1.8473350857836e-05)
% --(axis cs:1200,1.65190368294836e-05)
% --(axis cs:1300,1.46007929226268e-05)
% --(axis cs:1400,1.45595014449124e-05)
% --(axis cs:1500,1.39987305625565e-05)
% --(axis cs:1600,1.31470811509501e-05)
% --(axis cs:1700,1.23771706300203e-05)
% --(axis cs:1800,1.2035628126418e-05)
% --(axis cs:1900,1.1564137462496e-05)
% --(axis cs:2000,1.21898054728434e-05)
% --(axis cs:2100,1.16470080345494e-05)
% --(axis cs:2200,1.09459750996755e-05)
% --(axis cs:2300,1.15052853607579e-05)
% --(axis cs:2400,1.21716046810303e-05)
% --(axis cs:2500,1.16514703436143e-05)
% --(axis cs:2600,1.12045463620562e-05)
% --(axis cs:2700,1.08253308790665e-05)
% --(axis cs:2800,1.2218136819482e-05)
% --(axis cs:2900,1.14846883223336e-05)
% --(axis cs:3000,1.13691679837163e-05)
% --(axis cs:3100,1.06839009951026e-05)
% --(axis cs:3200,1.10233227846716e-05)
% --(axis cs:3300,1.04278367311103e-05)
% --(axis cs:3400,1.04058192632113e-05)
% --(axis cs:3500,9.63624357737949e-06)
% --(axis cs:3600,9.10047577231e-06)
% --(axis cs:3700,9.5343355281848e-06)
% --(axis cs:3800,9.37487115134702e-06)
% --(axis cs:3900,8.91762182493274e-06)
% --(axis cs:4000,9.07643546023538e-06)
% --(axis cs:4100,8.97059176356568e-06)
% --(axis cs:4200,8.88943616715981e-06)
% --(axis cs:4300,8.56012299280805e-06)
% --(axis cs:4400,8.57573468093313e-06)
% --(axis cs:4500,8.29416708025767e-06)
% --(axis cs:4600,8.24257812777846e-06)
% --(axis cs:4700,8.42871746101428e-06)
% --(axis cs:4800,8.4245594437946e-06)
% --(axis cs:4900,8.38055161580665e-06)
% --(axis cs:5000,7.89089250355638e-06)
% --(axis cs:5100,7.48138527147456e-06)
% --(axis cs:5200,7.62778874151625e-06)
% --(axis cs:5300,7.50897569846769e-06)
% --(axis cs:5400,7.27513685235156e-06)
% --(axis cs:5500,7.02867680176686e-06)
% --(axis cs:5600,7.70901409397964e-06)
% --(axis cs:5700,7.68945708642909e-06)
% --(axis cs:5800,7.34685461730445e-06)
% --(axis cs:5900,6.98265228087463e-06)
% --(axis cs:6000,6.41061145648107e-06)
% --(axis cs:6100,6.4713640542875e-06)
% --(axis cs:6200,6.41454235797881e-06)
% --(axis cs:6300,6.52682489769626e-06)
% --(axis cs:6400,6.41065046100906e-06)
% --(axis cs:6500,6.26631980958736e-06)
% --(axis cs:6600,6.20882394761043e-06)
% --(axis cs:6700,6.84763625424222e-06)
% --(axis cs:6800,6.75222215658097e-06)
% --(axis cs:6900,6.9491915145061e-06)
% --(axis cs:7000,7.11487048509731e-06)
% --(axis cs:7100,7.22533548147336e-06)
% --(axis cs:7200,6.75108759187364e-06)
% --(axis cs:7300,6.47179599942322e-06)
% --(axis cs:7400,6.01174488981778e-06)
% --(axis cs:7500,6.14563050017196e-06)
% --(axis cs:7600,5.52937366449794e-06)
% --(axis cs:7700,5.83082362285183e-06)
% --(axis cs:7800,5.96219492482279e-06)
% --(axis cs:7900,5.79999557947903e-06)
% --(axis cs:8000,5.96087959349111e-06)
% --(axis cs:8100,5.82236059405093e-06)
% --(axis cs:8200,5.98329964898762e-06)
% --(axis cs:8300,6.2124961218276e-06)
% --(axis cs:8400,6.18702649479812e-06)
% --(axis cs:8500,6.03851492696033e-06)
% --(axis cs:8600,6.18080258594938e-06)
% --(axis cs:8700,5.90023861011906e-06)
% --(axis cs:8800,5.51684139806199e-06)
% --(axis cs:8900,5.38168866751086e-06)
% --(axis cs:9000,5.30333257654161e-06)
% --(axis cs:9100,5.12931489501202e-06)
% --(axis cs:9200,4.94082928964035e-06)
% --(axis cs:9300,5.59608125206238e-06)
% --(axis cs:9400,5.45823576867349e-06)
% --(axis cs:9500,5.17551565720891e-06)
% --(axis cs:9600,5.14677633371604e-06)
% --(axis cs:9700,4.93805581257798e-06)
% --(axis cs:9800,4.41815024160211e-06)
% --(axis cs:9900,4.34978837972918e-06)
% --(axis cs:10000,4.48925128989008e-06)
% --(axis cs:10100,4.88479956162697e-06)
% --(axis cs:10200,4.82986088613207e-06)
% --(axis cs:10300,4.75232133351308e-06)
% --(axis cs:10400,4.91382739176767e-06)
% --(axis cs:10500,4.74645490566272e-06)
% --(axis cs:10600,5.31777827673816e-06)
% --(axis cs:10700,5.35614677817898e-06)
% --(axis cs:10800,5.14136443704612e-06)
% --(axis cs:10900,5.23742130072448e-06)
% --(axis cs:11000,4.99155065312772e-06)
% --(axis cs:11100,4.49621797846624e-06)
% --(axis cs:11200,4.28577609435795e-06)
% --(axis cs:11300,4.26603205429515e-06)
% --(axis cs:11400,4.17942519347321e-06)
% --(axis cs:11500,4.32250675190568e-06)
% --(axis cs:11600,4.39899932618509e-06)
% --(axis cs:11700,4.43108289984513e-06)
% --(axis cs:11800,4.68693743957599e-06)
% --(axis cs:11900,4.76454462231271e-06)
% --(axis cs:12000,4.43808607702983e-06)
% --(axis cs:12100,4.28329482121784e-06)
% --(axis cs:12200,4.21369470758731e-06)
% --(axis cs:12300,3.86055035455103e-06)
% --(axis cs:12400,3.7286421997507e-06)
% --(axis cs:12500,3.84083710535097e-06)
% --(axis cs:12600,3.91305387524031e-06)
% --(axis cs:12700,4.01111268946884e-06)
% --(axis cs:12800,3.91774033742321e-06)
% --(axis cs:12900,3.98815678896883e-06)
% --(axis cs:13000,3.99431144676484e-06)
% --(axis cs:13100,4.15440630506347e-06)
% --(axis cs:13200,4.15080585948066e-06)
% --(axis cs:13300,4.03955264363309e-06)
% --(axis cs:13400,4.04972219228132e-06)
% --(axis cs:13500,3.80861373773618e-06)
% --(axis cs:13600,3.8826833444146e-06)
% --(axis cs:13700,3.86781120027029e-06)
% --(axis cs:13800,3.61897649477471e-06)
% --(axis cs:13900,3.51280823780378e-06)
% --(axis cs:14000,3.37834019441461e-06)
% --(axis cs:14100,3.25098593093718e-06)
% --(axis cs:14200,3.25224294856887e-06)
% --(axis cs:14300,3.40953464631249e-06)
% --(axis cs:14400,3.3066744793037e-06)
% --(axis cs:14500,3.54750512751695e-06)
% --(axis cs:14600,3.59588529398404e-06)
% --(axis cs:14700,3.73433841722689e-06)
% --(axis cs:14800,3.6658348935794e-06)
% --(axis cs:14900,3.54089996370769e-06)
% --(axis cs:15000,3.69051037552825e-06)
% --(axis cs:15100,3.44877198728392e-06)
% --(axis cs:15200,3.21731262562637e-06)
% --(axis cs:15300,3.21182894287698e-06)
% --(axis cs:15400,3.18144330276225e-06)
% --(axis cs:15500,3.16813256777914e-06)
% --(axis cs:15600,3.18006037752674e-06)
% --(axis cs:15700,3.14037673121331e-06)
% --(axis cs:15800,3.14356725309215e-06)
% --(axis cs:15900,3.04659074572869e-06)
% --(axis cs:16000,3.08352764579607e-06)
% --(axis cs:16100,3.08232378401229e-06)
% --(axis cs:16200,3.08188429372695e-06)
% --(axis cs:16300,3.05720233116446e-06)
% --(axis cs:16400,3.0711570301514e-06)
% --(axis cs:16500,2.99250998039412e-06)
% --(axis cs:16600,2.8875703913583e-06)
% --(axis cs:16700,2.9206417255753e-06)
% --(axis cs:16800,2.96753379830219e-06)
% --(axis cs:16900,2.9718237117206e-06)
% --(axis cs:17000,2.90250171813797e-06)
% --(axis cs:17100,3.0000466535696e-06)
% --(axis cs:17200,2.88995742950898e-06)
% --(axis cs:17300,2.7920941398384e-06)
% --(axis cs:17400,2.83262703663102e-06)
% --(axis cs:17500,2.79703399524746e-06)
% --(axis cs:17600,2.86472107654224e-06)
% --(axis cs:17700,2.85594937451433e-06)
% --(axis cs:17800,2.73068234413077e-06)
% --(axis cs:17900,2.69651995900461e-06)
% --(axis cs:18000,2.83904681803697e-06)
% --(axis cs:18100,2.84358609865107e-06)
% --(axis cs:18200,2.8557629644217e-06)
% --(axis cs:18300,2.74414931075294e-06)
% --(axis cs:18400,2.73673723699551e-06)
% --(axis cs:18500,2.64552995457592e-06)
% --(axis cs:18600,2.52703515797541e-06)
% --(axis cs:18700,2.47485852544385e-06)
% --(axis cs:18800,2.60106765141391e-06)
% --(axis cs:18900,2.49024702496056e-06)
% --(axis cs:19000,2.54103108203255e-06)
% --(axis cs:19100,2.48236463668325e-06)
% --(axis cs:19200,2.46087684396799e-06)
% --(axis cs:19300,2.42637966302463e-06)
% --(axis cs:19400,2.2927052781204e-06)
% --(axis cs:19500,2.46268380139286e-06)
% --(axis cs:19600,2.46981544457893e-06)
% --(axis cs:19700,2.56175901631618e-06)
% --(axis cs:19800,2.49264610254694e-06)
% --(axis cs:19900,2.60178109996574e-06)
% --(axis cs:20000,2.40488411740484e-06)
% --(axis cs:20100,2.34387672271082e-06)
% --(axis cs:20200,2.38885297377273e-06)
% --(axis cs:20300,2.48003173988337e-06)
% --(axis cs:20400,2.19198622227634e-06)
% --(axis cs:20500,2.22917394880468e-06)
% --(axis cs:20600,2.19721099590793e-06)
% --(axis cs:20700,2.16128865166867e-06)
% --(axis cs:20800,2.1100146746023e-06)
% --(axis cs:20900,2.01080908393167e-06)
% --(axis cs:21000,1.92942686350274e-06)
% --(axis cs:21100,1.92338501788069e-06)
% --(axis cs:21200,2.00464251067162e-06)
% --(axis cs:21300,1.99233302561525e-06)
% --(axis cs:21400,2.03352212487112e-06)
% --(axis cs:21500,1.99477857750733e-06)
% --(axis cs:21600,1.98342690027391e-06)
% --(axis cs:21700,1.94366735806634e-06)
% --(axis cs:21800,1.96267399050476e-06)
% --(axis cs:21900,2.00676390716296e-06)
% --(axis cs:22000,1.93886025295355e-06)
% --(axis cs:22100,1.95362734802814e-06)
% --(axis cs:22200,1.9032135036398e-06)
% --(axis cs:22300,1.93355131081978e-06)
% --(axis cs:22400,1.89900103493357e-06)
% --(axis cs:22500,1.8895193008118e-06)
% --(axis cs:22600,1.91385242765112e-06)
% --(axis cs:22700,1.8786684477634e-06)
% --(axis cs:22800,1.88887036552321e-06)
% --(axis cs:22900,1.85622066019678e-06)
% --(axis cs:23000,1.77965673986735e-06)
% --(axis cs:23100,1.80348296329682e-06)
% --(axis cs:23200,1.67152211953715e-06)
% --(axis cs:23300,1.68180557206933e-06)
% --(axis cs:23400,1.68147980956998e-06)
% --(axis cs:23500,1.6357788257961e-06)
% --(axis cs:23600,1.56757898827163e-06)
% --(axis cs:23700,1.59095231734281e-06)
% --(axis cs:23800,1.5889384122818e-06)
% --(axis cs:23900,1.62056271062339e-06)
% --(axis cs:24000,1.67059273102961e-06)
% --(axis cs:24100,1.61733432375546e-06)
% --(axis cs:24200,1.67006371236708e-06)
% --(axis cs:24300,1.70534808522356e-06)
% --(axis cs:24400,1.59784514365305e-06)
% --(axis cs:24500,1.57266048059742e-06)
% --(axis cs:24600,1.5919696593556e-06)
% --(axis cs:24700,1.51476288519094e-06)
% --(axis cs:24800,1.59301228918147e-06)
% --(axis cs:24900,1.63686818128756e-06)
% --(axis cs:25000,1.596692403553e-06)
% --(axis cs:25100,1.69733818947323e-06)
% --(axis cs:25200,1.58246429615636e-06)
% --(axis cs:25300,1.54501273360777e-06)
% --(axis cs:25400,1.56520922199759e-06)
% --(axis cs:25500,1.5602557474434e-06)
% --(axis cs:25600,1.48110439102189e-06)
% --(axis cs:25700,1.49639777084721e-06)
% --(axis cs:25800,1.37402280049419e-06)
% --(axis cs:25900,1.31728207393745e-06)
% --(axis cs:26000,1.34237306459456e-06)
% --(axis cs:26100,1.42595294009859e-06)
% --(axis cs:26200,1.45442498680875e-06)
% --(axis cs:26300,1.51442976287615e-06)
% --(axis cs:26400,1.50315675387672e-06)
% --(axis cs:26500,1.42294100321743e-06)
% --(axis cs:26600,1.39031692003857e-06)
% --(axis cs:26700,1.36626897935375e-06)
% --(axis cs:26800,1.31428347714626e-06)
% --(axis cs:26900,1.32841947924321e-06)
% --(axis cs:27000,1.32212732256651e-06)
% --(axis cs:27100,1.35816888778705e-06)
% --(axis cs:27200,1.37622905837535e-06)
% --(axis cs:27300,1.38056392255915e-06)
% --(axis cs:27400,1.34306155722937e-06)
% --(axis cs:27500,1.36211208997261e-06)
% --(axis cs:27600,1.31569096096278e-06)
% --(axis cs:27700,1.27892260413938e-06)
% --(axis cs:27800,1.33387641668026e-06)
% --(axis cs:27900,1.35642988431191e-06)
% --(axis cs:28000,1.30809081236079e-06)
% --(axis cs:28100,1.29562355708987e-06)
% --(axis cs:28200,1.27777710829185e-06)
% --(axis cs:28300,1.25844267048726e-06)
% --(axis cs:28400,1.24429815197824e-06)
% --(axis cs:28500,1.25810460196156e-06)
% --(axis cs:28600,1.23557496055899e-06)
% --(axis cs:28700,1.22265117877809e-06)
% --(axis cs:28800,1.23662097284231e-06)
% --(axis cs:28900,1.22900046714047e-06)
% --(axis cs:29000,1.22403465126932e-06)
% --(axis cs:29100,1.21471808886239e-06)
% --(axis cs:29200,1.20129641454041e-06)
% --(axis cs:29300,1.18747505687547e-06)
% --(axis cs:29400,1.19095163719305e-06)
% --(axis cs:29500,1.20634965388578e-06)
% --(axis cs:29500,1.27206900444649e-06)
% --(axis cs:29500,1.27206900444649e-06)
% --(axis cs:29400,1.22796872661097e-06)
% --(axis cs:29300,1.26175549115771e-06)
% --(axis cs:29200,1.24359922405395e-06)
% --(axis cs:29100,1.26262480397839e-06)
% --(axis cs:29000,1.28147053279642e-06)
% --(axis cs:28900,1.34565402353193e-06)
% --(axis cs:28800,1.34096695656645e-06)
% --(axis cs:28700,1.36176513074387e-06)
% --(axis cs:28600,1.32571773417705e-06)
% --(axis cs:28500,1.30959763541926e-06)
% --(axis cs:28400,1.25843263365799e-06)
% --(axis cs:28300,1.27103411090784e-06)
% --(axis cs:28200,1.34898716932528e-06)
% --(axis cs:28100,1.32836503364693e-06)
% --(axis cs:28000,1.36245528206536e-06)
% --(axis cs:27900,1.39080118054717e-06)
% --(axis cs:27800,1.36181180991468e-06)
% --(axis cs:27700,1.3738047610391e-06)
% --(axis cs:27600,1.37745945709107e-06)
% --(axis cs:27500,1.36952297489872e-06)
% --(axis cs:27400,1.38162807556063e-06)
% --(axis cs:27300,1.4193766803675e-06)
% --(axis cs:27200,1.43527908934001e-06)
% --(axis cs:27100,1.44568772647703e-06)
% --(axis cs:27000,1.43863758431002e-06)
% --(axis cs:26900,1.46288967032398e-06)
% --(axis cs:26800,1.50175433314005e-06)
% --(axis cs:26700,1.54289222082077e-06)
% --(axis cs:26600,1.53842368501854e-06)
% --(axis cs:26500,1.54373027543429e-06)
% --(axis cs:26400,1.5762799685725e-06)
% --(axis cs:26300,1.55084127642806e-06)
% --(axis cs:26200,1.47637436561353e-06)
% --(axis cs:26100,1.53421945321215e-06)
% --(axis cs:26000,1.59683717356376e-06)
% --(axis cs:25900,1.53231308951177e-06)
% --(axis cs:25800,1.50933362483007e-06)
% --(axis cs:25700,1.59529278593442e-06)
% --(axis cs:25600,1.55259035647881e-06)
% --(axis cs:25500,1.61276625177833e-06)
% --(axis cs:25400,1.63289859651264e-06)
% --(axis cs:25300,1.63686604628578e-06)
% --(axis cs:25200,1.65872793862556e-06)
% --(axis cs:25100,1.71773172745748e-06)
% --(axis cs:25000,1.73227715062712e-06)
% --(axis cs:24900,1.7355269103104e-06)
% --(axis cs:24800,1.77276583434673e-06)
% --(axis cs:24700,1.76237533900564e-06)
% --(axis cs:24600,1.71750170781881e-06)
% --(axis cs:24500,1.75492967328501e-06)
% --(axis cs:24400,1.85086372327356e-06)
% --(axis cs:24300,1.89310085342291e-06)
% --(axis cs:24200,1.86627991066323e-06)
% --(axis cs:24100,1.86328355845305e-06)
% --(axis cs:24000,1.82331468776121e-06)
% --(axis cs:23900,1.73742486318836e-06)
% --(axis cs:23800,1.69067083322827e-06)
% --(axis cs:23700,1.74992268922422e-06)
% --(axis cs:23600,1.75916519911395e-06)
% --(axis cs:23500,1.79139811786392e-06)
% --(axis cs:23400,1.76715860183373e-06)
% --(axis cs:23300,1.84425601630026e-06)
% --(axis cs:23200,1.89274720482971e-06)
% --(axis cs:23100,1.89973171596578e-06)
% --(axis cs:23000,1.90795960503776e-06)
% --(axis cs:22900,1.9061479485835e-06)
% --(axis cs:22800,1.93558182194986e-06)
% --(axis cs:22700,2.04951089800936e-06)
% --(axis cs:22600,2.01035001611393e-06)
% --(axis cs:22500,2.09621567396448e-06)
% --(axis cs:22400,2.09673882115132e-06)
% --(axis cs:22300,2.04281104820632e-06)
% --(axis cs:22200,2.12249721935926e-06)
% --(axis cs:22100,2.06684353346209e-06)
% --(axis cs:22000,2.1442392219295e-06)
% --(axis cs:21900,2.11560040940924e-06)
% --(axis cs:21800,2.16993613252255e-06)
% --(axis cs:21700,2.1598381462755e-06)
% --(axis cs:21600,2.19304358958815e-06)
% --(axis cs:21500,2.13338637500682e-06)
% --(axis cs:21400,2.08841594185085e-06)
% --(axis cs:21300,2.13623071000913e-06)
% --(axis cs:21200,2.14127767320176e-06)
% --(axis cs:21100,2.21062569667086e-06)
% --(axis cs:21000,2.22807997970633e-06)
% --(axis cs:20900,2.38520369534507e-06)
% --(axis cs:20800,2.53305612553059e-06)
% --(axis cs:20700,2.58283843914794e-06)
% --(axis cs:20600,2.65891900318997e-06)
% --(axis cs:20500,2.65517515462056e-06)
% --(axis cs:20400,2.58385519132302e-06)
% --(axis cs:20300,2.50885898950525e-06)
% --(axis cs:20200,2.58395212915543e-06)
% --(axis cs:20100,2.82704094325341e-06)
% --(axis cs:20000,2.8716104220253e-06)
% --(axis cs:19900,2.89727561508684e-06)
% --(axis cs:19800,2.72751982234008e-06)
% --(axis cs:19700,2.7827360469628e-06)
% --(axis cs:19600,2.81244568537481e-06)
% --(axis cs:19500,2.85428795132212e-06)
% --(axis cs:19400,2.96966832530405e-06)
% --(axis cs:19300,2.85734711764102e-06)
% --(axis cs:19200,2.93816201113485e-06)
% --(axis cs:19100,2.80318492294721e-06)
% --(axis cs:19000,2.73220196392229e-06)
% --(axis cs:18900,2.8649888827397e-06)
% --(axis cs:18800,3.05808712798509e-06)
% --(axis cs:18700,3.1996640162475e-06)
% --(axis cs:18600,3.184418750007e-06)
% --(axis cs:18500,3.22964468673253e-06)
% --(axis cs:18400,3.27600811859994e-06)
% --(axis cs:18300,3.12550503119714e-06)
% --(axis cs:18200,2.89853319170981e-06)
% --(axis cs:18100,3.02834943791e-06)
% --(axis cs:18000,3.21410969121149e-06)
% --(axis cs:17900,3.09678293937792e-06)
% --(axis cs:17800,3.14076151959452e-06)
% --(axis cs:17700,3.09288284768799e-06)
% --(axis cs:17600,3.10493348116036e-06)
% --(axis cs:17500,2.98610126774959e-06)
% --(axis cs:17400,2.96997759754793e-06)
% --(axis cs:17300,3.19373863088529e-06)
% --(axis cs:17200,3.23376753156229e-06)
% --(axis cs:17100,3.38816573324015e-06)
% --(axis cs:17000,3.35382617589325e-06)
% --(axis cs:16900,3.3271816754945e-06)
% --(axis cs:16800,3.12970352413849e-06)
% --(axis cs:16700,3.06363101920293e-06)
% --(axis cs:16600,2.9562614254366e-06)
% --(axis cs:16500,3.06758460918682e-06)
% --(axis cs:16400,3.18988077314243e-06)
% --(axis cs:16300,3.25994320072591e-06)
% --(axis cs:16200,3.39095360406675e-06)
% --(axis cs:16100,3.45569956962933e-06)
% --(axis cs:16000,3.49415489127914e-06)
% --(axis cs:15900,3.47310062048856e-06)
% --(axis cs:15800,3.53595170890547e-06)
% --(axis cs:15700,3.5642276408002e-06)
% --(axis cs:15600,3.41421628449669e-06)
% --(axis cs:15500,3.59454261651172e-06)
% --(axis cs:15400,3.67417341795119e-06)
% --(axis cs:15300,3.56893005805062e-06)
% --(axis cs:15200,3.62188131894067e-06)
% --(axis cs:15100,3.90183871037745e-06)
% --(axis cs:15000,3.80676498299367e-06)
% --(axis cs:14900,4.48428607685714e-06)
% --(axis cs:14800,4.36475660747946e-06)
% --(axis cs:14700,4.43303647887213e-06)
% --(axis cs:14600,4.19121119234583e-06)
% --(axis cs:14500,4.11719101615151e-06)
% --(axis cs:14400,3.77220430352169e-06)
% --(axis cs:14300,3.78187934172664e-06)
% --(axis cs:14200,3.70277860234882e-06)
% --(axis cs:14100,3.92508415388728e-06)
% --(axis cs:14000,4.08968438962327e-06)
% --(axis cs:13900,4.15548686734906e-06)
% --(axis cs:13800,4.12330412474498e-06)
% --(axis cs:13700,4.08292220944887e-06)
% --(axis cs:13600,3.93791301501303e-06)
% --(axis cs:13500,4.00709081348849e-06)
% --(axis cs:13400,4.18803007080367e-06)
% --(axis cs:13300,4.29225774251984e-06)
% --(axis cs:13200,4.37403792559683e-06)
% --(axis cs:13100,4.60318366192658e-06)
% --(axis cs:13000,4.57646527683205e-06)
% --(axis cs:12900,4.39185433042589e-06)
% --(axis cs:12800,4.29517674795483e-06)
% --(axis cs:12700,4.11188489816518e-06)
% --(axis cs:12600,4.49969508195804e-06)
% --(axis cs:12500,4.71177312854078e-06)
% --(axis cs:12400,4.66658688815899e-06)
% --(axis cs:12300,4.89113435428989e-06)
% --(axis cs:12200,4.93344533101016e-06)
% --(axis cs:12100,4.87728651831117e-06)
% --(axis cs:12000,5.29919927421506e-06)
% --(axis cs:11900,5.25149169944558e-06)
% --(axis cs:11800,5.47619594714056e-06)
% --(axis cs:11700,5.50383455870137e-06)
% --(axis cs:11600,5.18487558136322e-06)
% --(axis cs:11500,4.89392626314484e-06)
% --(axis cs:11400,5.04628912405943e-06)
% --(axis cs:11300,4.90384074374016e-06)
% --(axis cs:11200,4.83034356591424e-06)
% --(axis cs:11100,4.96499274200766e-06)
% --(axis cs:11000,5.47808945119551e-06)
% --(axis cs:10900,5.92948015791237e-06)
% --(axis cs:10800,6.03979389673785e-06)
% --(axis cs:10700,6.10816751212398e-06)
% --(axis cs:10600,6.06860614194233e-06)
% --(axis cs:10500,6.12301528888208e-06)
% --(axis cs:10400,5.4220457779598e-06)
% --(axis cs:10300,5.46803436755704e-06)
% --(axis cs:10200,5.41860881199436e-06)
% --(axis cs:10100,5.47834280584481e-06)
% --(axis cs:10000,5.44241411876778e-06)
% --(axis cs:9900,5.58809863965159e-06)
% --(axis cs:9800,5.51217639085474e-06)
% --(axis cs:9700,5.7398264126553e-06)
% --(axis cs:9600,5.69671074922573e-06)
% --(axis cs:9500,5.81993513620733e-06)
% --(axis cs:9400,5.78904962082314e-06)
% --(axis cs:9300,6.08640414312638e-06)
% --(axis cs:9200,5.90053630596007e-06)
% --(axis cs:9100,5.68935674625783e-06)
% --(axis cs:9000,5.63965074082193e-06)
% --(axis cs:8900,5.49478142268964e-06)
% --(axis cs:8800,5.63220273843536e-06)
% --(axis cs:8700,6.39213004268445e-06)
% --(axis cs:8600,6.34290592742583e-06)
% --(axis cs:8500,6.77638080558139e-06)
% --(axis cs:8400,7.00543304835987e-06)
% --(axis cs:8300,7.14166315132138e-06)
% --(axis cs:8200,6.54206899538323e-06)
% --(axis cs:8100,6.81495848075691e-06)
% --(axis cs:8000,6.41446068449766e-06)
% --(axis cs:7900,6.29581932357427e-06)
% --(axis cs:7800,6.12246399495261e-06)
% --(axis cs:7700,6.59542368081332e-06)
% --(axis cs:7600,6.80285116829157e-06)
% --(axis cs:7500,7.21454465599839e-06)
% --(axis cs:7400,7.57504045131015e-06)
% --(axis cs:7300,7.53580641628405e-06)
% --(axis cs:7200,7.73472228738743e-06)
% --(axis cs:7100,8.42293801743308e-06)
% --(axis cs:7000,7.58972319531365e-06)
% --(axis cs:6900,7.82561582384451e-06)
% --(axis cs:6800,7.71033145809192e-06)
% --(axis cs:6700,7.19363444266508e-06)
% --(axis cs:6600,7.40023698028524e-06)
% --(axis cs:6500,7.46868933916837e-06)
% --(axis cs:6400,7.48238284648289e-06)
% --(axis cs:6300,7.55226574182573e-06)
% --(axis cs:6200,7.37884889277419e-06)
% --(axis cs:6100,7.00675213138849e-06)
% --(axis cs:6000,7.72202040853853e-06)
% --(axis cs:5900,7.89403580510686e-06)
% --(axis cs:5800,7.57438433904763e-06)
% --(axis cs:5700,7.8574293385706e-06)
% --(axis cs:5600,8.24278276769624e-06)
% --(axis cs:5500,8.69724298831405e-06)
% --(axis cs:5400,8.49424223255887e-06)
% --(axis cs:5300,8.49103893431738e-06)
% --(axis cs:5200,8.91938796893012e-06)
% --(axis cs:5100,9.02816224771258e-06)
% --(axis cs:5000,8.95915952436791e-06)
% --(axis cs:4900,9.2997319230353e-06)
% --(axis cs:4800,1.14018786304384e-05)
% --(axis cs:4700,1.13490101385131e-05)
% --(axis cs:4600,1.19895632199788e-05)
% --(axis cs:4500,1.19637921542318e-05)
% --(axis cs:4400,1.14816076059094e-05)
% --(axis cs:4300,9.78488427264424e-06)
% --(axis cs:4200,9.97744607032952e-06)
% --(axis cs:4100,1.0523137384184e-05)
% --(axis cs:4000,1.06049582179483e-05)
% --(axis cs:3900,1.00765055728614e-05)
% --(axis cs:3800,9.8729822277093e-06)
% --(axis cs:3700,1.02928236540808e-05)
% --(axis cs:3600,1.01460579299341e-05)
% --(axis cs:3500,1.04580505090684e-05)
% --(axis cs:3400,1.09173191263505e-05)
% --(axis cs:3300,1.13056050349113e-05)
% --(axis cs:3200,1.19568886368071e-05)
% --(axis cs:3100,1.29246778298788e-05)
% --(axis cs:3000,1.27859573729123e-05)
% --(axis cs:2900,1.22597691323586e-05)
% --(axis cs:2800,1.29178441334759e-05)
% --(axis cs:2700,1.24622616785417e-05)
% --(axis cs:2600,1.27660822948176e-05)
% --(axis cs:2500,1.21267144488006e-05)
% --(axis cs:2400,1.23179832291327e-05)
% --(axis cs:2300,1.19127299497441e-05)
% --(axis cs:2200,1.24804245393172e-05)
% --(axis cs:2100,1.21567167030169e-05)
% --(axis cs:2000,1.29481003347014e-05)
% --(axis cs:1900,1.39245509927777e-05)
% --(axis cs:1800,1.48755818318771e-05)
% --(axis cs:1700,1.54607592533695e-05)
% --(axis cs:1600,1.50044395952279e-05)
% --(axis cs:1500,1.54449300429095e-05)
% --(axis cs:1400,1.5691543194435e-05)
% --(axis cs:1300,1.64842018483089e-05)
% --(axis cs:1200,1.89975511539064e-05)
% --(axis cs:1100,2.00631112067248e-05)
% --(axis cs:1000,2.09462149050376e-05)
% --(axis cs:900,2.1736087851699e-05)
% --(axis cs:800,2.40629411009763e-05)
% --(axis cs:700,2.81510157066598e-05)
% --(axis cs:600,6.72703647078764e-05)
% --(axis cs:500,0.000114086218086727)
% --(axis cs:400,0.000242060592606047)
% --(axis cs:300,0.000553222363479052)
% --(axis cs:200,0.000929543821951678)
% --(axis cs:100,0.00120436939387436)
% --(axis cs:0,0.00157419282920996)
% --cycle;

\path [fill=blue, fill opacity=0.2, semithick]
(axis cs:0,0.00720213678466435)
--(axis cs:0,0.00706319136433646)
--(axis cs:100,0.00577221439616148)
--(axis cs:200,0.00437417259646036)
--(axis cs:300,0.00282089913568673)
--(axis cs:400,0.00136047739749201)
--(axis cs:500,0.00077469900148994)
--(axis cs:600,0.000496558219041754)
--(axis cs:700,0.00030810862638953)
--(axis cs:800,0.000285933100774087)
--(axis cs:900,0.000265588027901413)
--(axis cs:1000,0.000242055493928945)
--(axis cs:1100,0.000211403978837982)
--(axis cs:1200,0.000198701190636847)
--(axis cs:1300,0.000188256568195119)
--(axis cs:1400,0.000182206979851282)
--(axis cs:1500,0.00017908389568628)
--(axis cs:1600,0.000169238035150954)
--(axis cs:1700,0.000163385214052475)
--(axis cs:1800,0.000160370126617323)
--(axis cs:1900,0.000155548191553739)
--(axis cs:2000,0.000154881252626218)
--(axis cs:2100,0.000153664180802631)
--(axis cs:2200,0.000144987952941353)
--(axis cs:2300,0.000136861704128159)
--(axis cs:2400,0.000130871424616827)
--(axis cs:2500,0.000132241600212644)
--(axis cs:2600,0.000132929589784729)
--(axis cs:2700,0.00013109479561135)
--(axis cs:2800,0.000133114026358595)
--(axis cs:2900,0.000123390086199334)
--(axis cs:3000,0.000125517524186516)
--(axis cs:3100,0.000126149054528304)
--(axis cs:3200,0.000121162026848257)
--(axis cs:3300,0.000112764267625281)
--(axis cs:3400,0.000116631922919917)
--(axis cs:3500,0.000111669668139284)
--(axis cs:3600,0.000105183232985002)
--(axis cs:3700,9.7802978012536e-05)
--(axis cs:3800,9.77233266676977e-05)
--(axis cs:3900,9.91469780786126e-05)
--(axis cs:4000,0.000100614156694267)
--(axis cs:4100,9.79694216878478e-05)
--(axis cs:4200,9.91715470346761e-05)
--(axis cs:4300,9.6317229487025e-05)
--(axis cs:4400,9.40337711327546e-05)
--(axis cs:4500,9.00317882660934e-05)
--(axis cs:4600,9.4740007765207e-05)
--(axis cs:4700,9.20050667851291e-05)
--(axis cs:4800,8.80454828334114e-05)
--(axis cs:4900,8.29170278520576e-05)
--(axis cs:5000,7.82815912057926e-05)
--(axis cs:5100,7.87812087001077e-05)
--(axis cs:5200,7.82469831003933e-05)
--(axis cs:5300,7.85129213016319e-05)
--(axis cs:5400,7.47607263862246e-05)
--(axis cs:5500,7.41085851649445e-05)
--(axis cs:5600,7.37033814928695e-05)
--(axis cs:5700,7.0544428886813e-05)
--(axis cs:5800,7.08079930139044e-05)
--(axis cs:5900,6.91807208571154e-05)
--(axis cs:6000,6.91162982179064e-05)
--(axis cs:6100,6.60846709223607e-05)
--(axis cs:6200,6.49503448796098e-05)
--(axis cs:6300,6.25422492970282e-05)
--(axis cs:6400,6.56521623567763e-05)
--(axis cs:6500,6.66362198326674e-05)
--(axis cs:6600,6.88057136976539e-05)
--(axis cs:6700,6.92103519582625e-05)
--(axis cs:6800,6.80141312091571e-05)
--(axis cs:6900,6.51011834458477e-05)
--(axis cs:7000,6.65326936615343e-05)
--(axis cs:7100,6.7397650247664e-05)
--(axis cs:7200,6.52705484436963e-05)
--(axis cs:7300,6.36224732986686e-05)
--(axis cs:7400,6.26280954158098e-05)
--(axis cs:7500,6.10055686207734e-05)
--(axis cs:7600,6.10377387396744e-05)
--(axis cs:7700,6.280401568195e-05)
--(axis cs:7800,6.24553621242084e-05)
--(axis cs:7900,6.08046810681856e-05)
--(axis cs:8000,6.20443091752337e-05)
--(axis cs:8100,6.20841647410181e-05)
--(axis cs:8200,6.10104611950603e-05)
--(axis cs:8300,6.10349664206641e-05)
--(axis cs:8400,6.05256270235834e-05)
--(axis cs:8500,5.77774128819773e-05)
--(axis cs:8600,5.95845166465777e-05)
--(axis cs:8700,5.84384282610086e-05)
--(axis cs:8800,5.4735706419128e-05)
--(axis cs:8900,5.40258237078303e-05)
--(axis cs:9000,5.5526856524376e-05)
--(axis cs:9100,5.42293906217722e-05)
--(axis cs:9200,5.4841631987728e-05)
--(axis cs:9300,5.70718487677459e-05)
--(axis cs:9400,5.49419563023293e-05)
--(axis cs:9500,5.54033201597231e-05)
--(axis cs:9600,5.49950598664233e-05)
--(axis cs:9700,5.60037581940378e-05)
--(axis cs:9800,5.63077568048105e-05)
--(axis cs:9900,5.60716843123014e-05)
--(axis cs:10000,5.63102866784549e-05)
--(axis cs:10100,5.75382788069966e-05)
--(axis cs:10200,5.52797739673536e-05)
--(axis cs:10300,5.52897748716874e-05)
--(axis cs:10400,5.40251794142322e-05)
--(axis cs:10500,5.30424289663948e-05)
--(axis cs:10600,5.5465258790601e-05)
--(axis cs:10700,5.41210931723209e-05)
--(axis cs:10800,5.43041570537651e-05)
--(axis cs:10900,5.37592554503919e-05)
--(axis cs:11000,5.16405348140156e-05)
--(axis cs:11100,4.82689686671494e-05)
--(axis cs:11200,4.98641667624403e-05)
--(axis cs:11300,5.0602842958679e-05)
--(axis cs:11400,5.17053538030205e-05)
--(axis cs:11500,5.25023035117707e-05)
--(axis cs:11600,5.20464327593676e-05)
--(axis cs:11700,5.30923157407788e-05)
--(axis cs:11800,5.25839820329661e-05)
--(axis cs:11900,5.15252053025331e-05)
--(axis cs:12000,4.97656534430524e-05)
--(axis cs:12100,5.06811755202665e-05)
--(axis cs:12200,5.00071348003669e-05)
--(axis cs:12300,4.82671777861011e-05)
--(axis cs:12400,4.82424257567556e-05)
--(axis cs:12500,4.87852536057573e-05)
--(axis cs:12600,4.86974927147951e-05)
--(axis cs:12700,4.91464950191291e-05)
--(axis cs:12800,4.91397908869691e-05)
--(axis cs:12900,4.93310022679003e-05)
--(axis cs:13000,4.72517338884877e-05)
--(axis cs:13100,5.00814928860332e-05)
--(axis cs:13200,4.8717069447104e-05)
--(axis cs:13300,4.74390614446605e-05)
--(axis cs:13400,4.8964915507706e-05)
--(axis cs:13500,4.68144138326579e-05)
--(axis cs:13600,4.58292159908577e-05)
--(axis cs:13700,4.51842287095966e-05)
--(axis cs:13800,4.56782587143971e-05)
--(axis cs:13900,4.73403977355977e-05)
--(axis cs:14000,4.73536003036408e-05)
--(axis cs:14100,4.64808062224246e-05)
--(axis cs:14200,4.60850053050127e-05)
--(axis cs:14300,4.60878014381667e-05)
--(axis cs:14400,4.40438263077243e-05)
--(axis cs:14500,4.54394970399111e-05)
--(axis cs:14600,4.74550721312535e-05)
--(axis cs:14700,4.84666334895731e-05)
--(axis cs:14800,4.72641356234924e-05)
--(axis cs:14900,4.80943371609573e-05)
--(axis cs:15000,4.64693051589498e-05)
--(axis cs:15100,4.54545903720093e-05)
--(axis cs:15200,4.45208684711475e-05)
--(axis cs:15300,4.50445274389382e-05)
--(axis cs:15400,4.41609335396579e-05)
--(axis cs:15500,4.37829478946518e-05)
--(axis cs:15600,4.26522150698282e-05)
--(axis cs:15700,4.22515689190656e-05)
--(axis cs:15800,4.15713976657436e-05)
--(axis cs:15900,4.12029642459861e-05)
--(axis cs:16000,4.13976885467813e-05)
--(axis cs:16100,4.20190708337453e-05)
--(axis cs:16200,4.24673091498373e-05)
--(axis cs:16300,4.3292515840797e-05)
--(axis cs:16400,4.23728882992894e-05)
--(axis cs:16500,4.23943805797954e-05)
--(axis cs:16600,4.07719897851463e-05)
--(axis cs:16700,4.0481905602146e-05)
--(axis cs:16800,4.10341376556345e-05)
--(axis cs:16900,4.06161416936638e-05)
--(axis cs:17000,4.12047184201416e-05)
--(axis cs:17100,4.16022295710486e-05)
--(axis cs:17200,4.09656989023333e-05)
--(axis cs:17300,4.05614785059299e-05)
--(axis cs:17400,4.12486373995452e-05)
--(axis cs:17500,3.97352641970383e-05)
--(axis cs:17600,4.03139910517701e-05)
--(axis cs:17700,3.99391260841412e-05)
--(axis cs:17800,3.87285037624204e-05)
--(axis cs:17900,3.81054293074747e-05)
--(axis cs:18000,3.91568350246911e-05)
--(axis cs:18100,3.88519784507477e-05)
--(axis cs:18200,3.90312253710471e-05)
--(axis cs:18300,3.97602238213474e-05)
--(axis cs:18400,3.99829663506013e-05)
--(axis cs:18500,3.99041829071979e-05)
--(axis cs:18600,3.93868875260377e-05)
--(axis cs:18700,3.99190818865908e-05)
--(axis cs:18800,3.96964898896059e-05)
--(axis cs:18900,3.9010189283625e-05)
--(axis cs:19000,3.97541330383624e-05)
--(axis cs:19100,4.06890009303233e-05)
--(axis cs:19200,4.08721090363477e-05)
--(axis cs:19300,4.09115275098928e-05)
--(axis cs:19400,3.96158693614142e-05)
--(axis cs:19500,3.83522701816274e-05)
--(axis cs:19600,3.7608433293249e-05)
--(axis cs:19700,3.67386779706204e-05)
--(axis cs:19800,3.62074605933528e-05)
--(axis cs:19900,3.66512574263734e-05)
--(axis cs:20000,3.71565481036511e-05)
--(axis cs:20100,3.73322432799091e-05)
--(axis cs:20200,3.6917290051917e-05)
--(axis cs:20300,3.65120793586581e-05)
--(axis cs:20400,3.66685380628456e-05)
--(axis cs:20500,3.72314685755394e-05)
--(axis cs:20600,3.76741962450594e-05)
--(axis cs:20700,3.73901974692333e-05)
--(axis cs:20800,3.79194220655756e-05)
--(axis cs:20900,3.73744950129641e-05)
--(axis cs:21000,3.62831093868596e-05)
--(axis cs:21100,3.57933518126519e-05)
--(axis cs:21200,3.6485979004698e-05)
--(axis cs:21300,3.52353525150885e-05)
--(axis cs:21400,3.50850485614013e-05)
--(axis cs:21500,3.66351549544233e-05)
--(axis cs:21600,3.66028227632385e-05)
--(axis cs:21700,3.6605132446809e-05)
--(axis cs:21800,3.69052376857737e-05)
--(axis cs:21900,3.73105573865435e-05)
--(axis cs:22000,3.61963174956502e-05)
--(axis cs:22100,3.693090463107e-05)
--(axis cs:22200,3.52409326390055e-05)
--(axis cs:22300,3.54268641151968e-05)
--(axis cs:22400,3.44003287108338e-05)
--(axis cs:22500,3.4695980468063e-05)
--(axis cs:22600,3.34461610766644e-05)
--(axis cs:22700,3.42714972141682e-05)
--(axis cs:22800,3.32913099413783e-05)
--(axis cs:22900,3.31488524010863e-05)
--(axis cs:23000,3.2931827101704e-05)
--(axis cs:23100,3.34058686720704e-05)
--(axis cs:23200,3.34250374584675e-05)
--(axis cs:23300,3.39521514719616e-05)
--(axis cs:23400,3.37477290105011e-05)
--(axis cs:23500,3.35166731431999e-05)
--(axis cs:23600,3.40363471992204e-05)
--(axis cs:23700,3.3942291150978e-05)
--(axis cs:23800,3.35693091152037e-05)
--(axis cs:23900,3.37868478020123e-05)
--(axis cs:24000,3.41911919908111e-05)
--(axis cs:24100,3.37967035296673e-05)
--(axis cs:24200,3.29314938724174e-05)
--(axis cs:24300,3.28876295980991e-05)
--(axis cs:24400,3.23736112183717e-05)
--(axis cs:24500,3.21912815269417e-05)
--(axis cs:24600,3.20948335801269e-05)
--(axis cs:24700,3.20475478394499e-05)
--(axis cs:24800,3.2165695284819e-05)
--(axis cs:24900,3.21732907499491e-05)
--(axis cs:25000,3.14864657747581e-05)
--(axis cs:25100,3.16565075859894e-05)
--(axis cs:25200,3.21920901055323e-05)
--(axis cs:25300,3.20012925374529e-05)
--(axis cs:25400,3.203463643662e-05)
--(axis cs:25500,3.19545111949365e-05)
--(axis cs:25600,3.19728481944439e-05)
--(axis cs:25700,3.20102585702372e-05)
--(axis cs:25800,3.2071952875533e-05)
--(axis cs:25900,3.21948850331592e-05)
--(axis cs:26000,3.25313008421233e-05)
--(axis cs:26100,3.23180512302583e-05)
--(axis cs:26200,3.27070065634908e-05)
--(axis cs:26300,3.29213744416118e-05)
--(axis cs:26400,3.21702513720013e-05)
--(axis cs:26500,3.19943125588622e-05)
--(axis cs:26600,3.16706324249326e-05)
--(axis cs:26700,3.08080753536871e-05)
--(axis cs:26800,3.03615977898636e-05)
--(axis cs:26900,3.02972637328791e-05)
--(axis cs:27000,3.00350565439973e-05)
--(axis cs:27100,2.98849284695719e-05)
--(axis cs:27200,2.96830704151674e-05)
--(axis cs:27300,2.97293066915623e-05)
--(axis cs:27400,3.01253529303379e-05)
--(axis cs:27500,3.01355754066362e-05)
--(axis cs:27600,2.99782098715779e-05)
--(axis cs:27700,3.01719873345313e-05)
--(axis cs:27800,2.98428551620278e-05)
--(axis cs:27900,2.95494862050136e-05)
--(axis cs:28000,2.97255455095266e-05)
--(axis cs:28100,2.97177266101585e-05)
--(axis cs:28200,2.96837146462982e-05)
--(axis cs:28300,2.99967285577377e-05)
--(axis cs:28400,3.01990492702662e-05)
--(axis cs:28500,3.00986949263421e-05)
--(axis cs:28600,3.00345980058584e-05)
--(axis cs:28700,2.99414323676473e-05)
--(axis cs:28800,2.97716036075847e-05)
--(axis cs:28900,2.97758136596494e-05)
--(axis cs:29000,2.95766487138792e-05)
--(axis cs:29100,2.97845818149107e-05)
--(axis cs:29200,2.99098398131834e-05)
--(axis cs:29300,3.01235356853252e-05)
--(axis cs:29400,2.98650407819179e-05)
--(axis cs:29500,2.96251221720614e-05)
--(axis cs:29500,3.52258680906748e-05)
--(axis cs:29500,3.52258680906748e-05)
--(axis cs:29400,3.52264123614776e-05)
--(axis cs:29300,3.54372669282927e-05)
--(axis cs:29200,3.55091044249584e-05)
--(axis cs:29100,3.51494450715655e-05)
--(axis cs:29000,3.55821812522151e-05)
--(axis cs:28900,3.51811511682694e-05)
--(axis cs:28800,3.46270515267461e-05)
--(axis cs:28700,3.48478347339882e-05)
--(axis cs:28600,3.53014694370791e-05)
--(axis cs:28500,3.50085424369696e-05)
--(axis cs:28400,3.54898463346174e-05)
--(axis cs:28300,3.59386881326466e-05)
--(axis cs:28200,3.58825735542969e-05)
--(axis cs:28100,3.57745665566919e-05)
--(axis cs:28000,3.60997956434319e-05)
--(axis cs:27900,3.60175630607479e-05)
--(axis cs:27800,3.62507342985271e-05)
--(axis cs:27700,3.57993226248915e-05)
--(axis cs:27600,3.53317611367167e-05)
--(axis cs:27500,3.49072694892581e-05)
--(axis cs:27400,3.49251571869029e-05)
--(axis cs:27300,3.51125304164953e-05)
--(axis cs:27200,3.50779477810311e-05)
--(axis cs:27100,3.53049060496399e-05)
--(axis cs:27000,3.46449424089757e-05)
--(axis cs:26900,3.44998502465114e-05)
--(axis cs:26800,3.3914549378266e-05)
--(axis cs:26700,3.42092406322583e-05)
--(axis cs:26600,3.43102973205838e-05)
--(axis cs:26500,3.48555018585993e-05)
--(axis cs:26400,3.50308385180516e-05)
--(axis cs:26300,3.52104258724893e-05)
--(axis cs:26200,3.51779321502933e-05)
--(axis cs:26100,3.58490258367394e-05)
--(axis cs:26000,3.58410290489152e-05)
--(axis cs:25900,3.55667679145547e-05)
--(axis cs:25800,3.53759399221122e-05)
--(axis cs:25700,3.58583616258097e-05)
--(axis cs:25600,3.47759633196729e-05)
--(axis cs:25500,3.44734645428637e-05)
--(axis cs:25400,3.51704809385042e-05)
--(axis cs:25300,3.57895321496555e-05)
--(axis cs:25200,3.54645533115107e-05)
--(axis cs:25100,3.56770260754507e-05)
--(axis cs:25000,3.61978418032617e-05)
--(axis cs:24900,3.61536832466417e-05)
--(axis cs:24800,3.60269553180011e-05)
--(axis cs:24700,3.57855870262488e-05)
--(axis cs:24600,3.6346762214739e-05)
--(axis cs:24500,3.61358159183966e-05)
--(axis cs:24400,3.57921991044054e-05)
--(axis cs:24300,3.58649187973241e-05)
--(axis cs:24200,3.60491737415726e-05)
--(axis cs:24100,3.59796970060106e-05)
--(axis cs:24000,3.65151748809829e-05)
--(axis cs:23900,3.6885624263768e-05)
--(axis cs:23800,3.66397116141282e-05)
--(axis cs:23700,3.75814994848115e-05)
--(axis cs:23600,3.77432069284951e-05)
--(axis cs:23500,3.76120839258427e-05)
--(axis cs:23400,3.70752952299766e-05)
--(axis cs:23300,3.71439166597758e-05)
--(axis cs:23200,3.64862321678022e-05)
--(axis cs:23100,3.61548210631559e-05)
--(axis cs:23000,3.6457365402173e-05)
--(axis cs:22900,3.67605710722048e-05)
--(axis cs:22800,3.71738118843131e-05)
--(axis cs:22700,3.78443439134535e-05)
--(axis cs:22600,3.8746559759364e-05)
--(axis cs:22500,3.8992352745732e-05)
--(axis cs:22400,3.90799281223023e-05)
--(axis cs:22300,3.86903043391013e-05)
--(axis cs:22200,3.80372145837792e-05)
--(axis cs:22100,3.79687207901213e-05)
--(axis cs:22000,3.75923341964099e-05)
--(axis cs:21900,3.86825396902699e-05)
--(axis cs:21800,3.80599150096908e-05)
--(axis cs:21700,3.80512708080639e-05)
--(axis cs:21600,3.85255660413003e-05)
--(axis cs:21500,3.89647556787495e-05)
--(axis cs:21400,3.90787616915868e-05)
--(axis cs:21300,3.91018704863568e-05)
--(axis cs:21200,3.91590318942782e-05)
--(axis cs:21100,3.84042334355812e-05)
--(axis cs:21000,3.93887672580112e-05)
--(axis cs:20900,3.87019297258938e-05)
--(axis cs:20800,4.05295639093497e-05)
--(axis cs:20700,4.14261220167378e-05)
--(axis cs:20600,4.19541899598477e-05)
--(axis cs:20500,4.18539531729199e-05)
--(axis cs:20400,4.21244309348862e-05)
--(axis cs:20300,4.11868625853537e-05)
--(axis cs:20200,4.09879849533094e-05)
--(axis cs:20100,4.08369045145362e-05)
--(axis cs:20000,4.0926346608725e-05)
--(axis cs:19900,4.12468114704318e-05)
--(axis cs:19800,4.03968528177762e-05)
--(axis cs:19700,4.07349484238253e-05)
--(axis cs:19600,4.03560602459353e-05)
--(axis cs:19500,4.03595078602793e-05)
--(axis cs:19400,4.13417232199846e-05)
--(axis cs:19300,4.21217711174253e-05)
--(axis cs:19200,4.22156152091161e-05)
--(axis cs:19100,4.22207655184936e-05)
--(axis cs:19000,4.30120976842165e-05)
--(axis cs:18900,4.30596139396993e-05)
--(axis cs:18800,4.43323028331657e-05)
--(axis cs:18700,4.52526808314522e-05)
--(axis cs:18600,4.5862914202992e-05)
--(axis cs:18500,4.61763454616651e-05)
--(axis cs:18400,4.56244472399739e-05)
--(axis cs:18300,4.33254355073455e-05)
--(axis cs:18200,4.1195973115635e-05)
--(axis cs:18100,4.08775489006987e-05)
--(axis cs:18000,4.01458007370629e-05)
--(axis cs:17900,4.02180774426917e-05)
--(axis cs:17800,4.10999872839834e-05)
--(axis cs:17700,4.1431808798681e-05)
--(axis cs:17600,4.15220589364749e-05)
--(axis cs:17500,4.19084608886548e-05)
--(axis cs:17400,4.29479466668309e-05)
--(axis cs:17300,4.35811446334602e-05)
--(axis cs:17200,4.42497811645026e-05)
--(axis cs:17100,4.58451698964917e-05)
--(axis cs:17000,4.65855843180953e-05)
--(axis cs:16900,4.63951276582694e-05)
--(axis cs:16800,4.60762942674309e-05)
--(axis cs:16700,4.63567600878166e-05)
--(axis cs:16600,4.50573526392575e-05)
--(axis cs:16500,4.43965587087289e-05)
--(axis cs:16400,4.49466871448849e-05)
--(axis cs:16300,4.39344463642256e-05)
--(axis cs:16200,4.45990164032347e-05)
--(axis cs:16100,4.53005385648979e-05)
--(axis cs:16000,4.66941740157969e-05)
--(axis cs:15900,4.73498719469409e-05)
--(axis cs:15800,4.79374576421968e-05)
--(axis cs:15700,4.87939070338825e-05)
--(axis cs:15600,4.8602824954579e-05)
--(axis cs:15500,5.01036711510578e-05)
--(axis cs:15400,4.98913018233934e-05)
--(axis cs:15300,5.00072644292344e-05)
--(axis cs:15200,5.01897673262836e-05)
--(axis cs:15100,5.08280422614135e-05)
--(axis cs:15000,4.94069904650406e-05)
--(axis cs:14900,5.00181634027723e-05)
--(axis cs:14800,5.11542796677424e-05)
--(axis cs:14700,5.01189299506132e-05)
--(axis cs:14600,4.89092079030688e-05)
--(axis cs:14500,4.79702649599779e-05)
--(axis cs:14400,4.82928808586718e-05)
--(axis cs:14300,4.76636448669866e-05)
--(axis cs:14200,4.73194185673066e-05)
--(axis cs:14100,4.81499313143174e-05)
--(axis cs:14000,4.88650577448635e-05)
--(axis cs:13900,4.84382914020623e-05)
--(axis cs:13800,4.82666174687377e-05)
--(axis cs:13700,4.86191456199853e-05)
--(axis cs:13600,4.82314429908555e-05)
--(axis cs:13500,5.08873273946014e-05)
--(axis cs:13400,5.05172302348072e-05)
--(axis cs:13300,5.18381312432657e-05)
--(axis cs:13200,5.32705367778104e-05)
--(axis cs:13100,5.47239830685541e-05)
--(axis cs:13000,5.31102157980942e-05)
--(axis cs:12900,5.11645679549469e-05)
--(axis cs:12800,5.23811121335072e-05)
--(axis cs:12700,5.19918560973556e-05)
--(axis cs:12600,5.12818478302619e-05)
--(axis cs:12500,5.17402280788418e-05)
--(axis cs:12400,5.06805204425535e-05)
--(axis cs:12300,5.05172754106604e-05)
--(axis cs:12200,5.06229048204672e-05)
--(axis cs:12100,5.1787851716148e-05)
--(axis cs:12000,5.48671878054785e-05)
--(axis cs:11900,5.67454052055102e-05)
--(axis cs:11800,5.7493489827408e-05)
--(axis cs:11700,5.63875123566131e-05)
--(axis cs:11600,5.61296839170126e-05)
--(axis cs:11500,5.66999991895349e-05)
--(axis cs:11400,5.55459357886384e-05)
--(axis cs:11300,5.3919011317469e-05)
--(axis cs:11200,5.26194099638834e-05)
--(axis cs:11100,5.24149096445828e-05)
--(axis cs:11000,5.66514068614971e-05)
--(axis cs:10900,5.90040037408294e-05)
--(axis cs:10800,6.08327654385701e-05)
--(axis cs:10700,6.25288588851177e-05)
--(axis cs:10600,6.19282088235158e-05)
--(axis cs:10500,6.00052740864761e-05)
--(axis cs:10400,5.68773006683542e-05)
--(axis cs:10300,5.65235571212989e-05)
--(axis cs:10200,5.98337951263593e-05)
--(axis cs:10100,6.10873581622307e-05)
--(axis cs:10000,6.13929606518518e-05)
--(axis cs:9900,6.01620267022004e-05)
--(axis cs:9800,6.03484724637938e-05)
--(axis cs:9700,6.21695601389547e-05)
--(axis cs:9600,6.1119339995121e-05)
--(axis cs:9500,5.83959301369044e-05)
--(axis cs:9400,6.01851198790986e-05)
--(axis cs:9300,5.85909634487719e-05)
--(axis cs:9200,5.7390902848008e-05)
--(axis cs:9100,5.76553878795385e-05)
--(axis cs:9000,5.85478702586736e-05)
--(axis cs:8900,5.83001111406074e-05)
--(axis cs:8800,5.77998279104292e-05)
--(axis cs:8700,5.89545770872678e-05)
--(axis cs:8600,6.02451908995819e-05)
--(axis cs:8500,6.27622986152811e-05)
--(axis cs:8400,6.49630569652225e-05)
--(axis cs:8300,6.62792975340945e-05)
--(axis cs:8200,6.38595854677274e-05)
--(axis cs:8100,6.73654671419686e-05)
--(axis cs:8000,6.72054618533682e-05)
--(axis cs:7900,6.56651953937871e-05)
--(axis cs:7800,6.56937772214151e-05)
--(axis cs:7700,6.65257118150018e-05)
--(axis cs:7600,6.45381713692657e-05)
--(axis cs:7500,6.93051505329152e-05)
--(axis cs:7400,6.9704034162762e-05)
--(axis cs:7300,6.93117592347751e-05)
--(axis cs:7200,6.92929766666317e-05)
--(axis cs:7100,7.07249648269196e-05)
--(axis cs:7000,6.99428056503934e-05)
--(axis cs:6900,7.56039158835047e-05)
--(axis cs:6800,7.94906386385712e-05)
--(axis cs:6700,7.69414778243005e-05)
--(axis cs:6600,7.73126044793297e-05)
--(axis cs:6500,7.59698830093941e-05)
--(axis cs:6400,7.55309261574014e-05)
--(axis cs:6300,7.24992548117845e-05)
--(axis cs:6200,7.09441294415904e-05)
--(axis cs:6100,6.97511751875759e-05)
--(axis cs:6000,7.39075149254661e-05)
--(axis cs:5900,7.76214020027897e-05)
--(axis cs:5800,7.6667530394598e-05)
--(axis cs:5700,7.71926603472809e-05)
--(axis cs:5600,7.84601995372633e-05)
--(axis cs:5500,7.99338499077284e-05)
--(axis cs:5400,8.20192528141882e-05)
--(axis cs:5300,8.50702800546003e-05)
--(axis cs:5200,8.88243938268036e-05)
--(axis cs:5100,8.94076670350088e-05)
--(axis cs:5000,9.48983188467752e-05)
--(axis cs:4900,9.55010070684113e-05)
--(axis cs:4800,9.92151271792366e-05)
--(axis cs:4700,0.000101165263236401)
--(axis cs:4600,0.00010816631121382)
--(axis cs:4500,0.000111570544260725)
--(axis cs:4400,0.000109140962773298)
--(axis cs:4300,0.000103356775395859)
--(axis cs:4200,0.000104631785953497)
--(axis cs:4100,0.000103370446675145)
--(axis cs:4000,0.000105538947775534)
--(axis cs:3900,0.000107561824258525)
--(axis cs:3800,0.000111813005930569)
--(axis cs:3700,0.000111566569264532)
--(axis cs:3600,0.000112784911973526)
--(axis cs:3500,0.000115898386936931)
--(axis cs:3400,0.000117767426896847)
--(axis cs:3300,0.000130722811459259)
--(axis cs:3200,0.000135836618060633)
--(axis cs:3100,0.000140923699879308)
--(axis cs:3000,0.000149643347686472)
--(axis cs:2900,0.000153332140208977)
--(axis cs:2800,0.000153309726191441)
--(axis cs:2700,0.000152838796339955)
--(axis cs:2600,0.000147734518598429)
--(axis cs:2500,0.00014053650807651)
--(axis cs:2400,0.000154731657151862)
--(axis cs:2300,0.000150816833878571)
--(axis cs:2200,0.000156231594264872)
--(axis cs:2100,0.000156670534762726)
--(axis cs:2000,0.000167734768134591)
--(axis cs:1900,0.000171919730722768)
--(axis cs:1800,0.000177243061112989)
--(axis cs:1700,0.000189536650586251)
--(axis cs:1600,0.00019663661922965)
--(axis cs:1500,0.000197576977806279)
--(axis cs:1400,0.000204715766502191)
--(axis cs:1300,0.000216412745185997)
--(axis cs:1200,0.000222121371469727)
--(axis cs:1100,0.000232344064391201)
--(axis cs:1000,0.000248391880442246)
--(axis cs:900,0.000274278822499551)
--(axis cs:800,0.000289193789163781)
--(axis cs:700,0.000346820978302233)
--(axis cs:600,0.000558749793250035)
--(axis cs:500,0.000872374700310218)
--(axis cs:400,0.00158550812338741)
--(axis cs:300,0.00303829922734546)
--(axis cs:200,0.00456458383344036)
--(axis cs:100,0.00593542234886424)
--(axis cs:0,0.00720213678466435)
--cycle;

% \path [fill=green!50.1960784313725!black, fill opacity=0.4, semithick]
% (axis cs:0,0.00118464536959966)
% --(axis cs:0,0.00097466535638357)
% --(axis cs:100,0.000784483804778959)
% --(axis cs:200,0.000591896450660173)
% --(axis cs:300,0.000315121278128499)
% --(axis cs:400,9.14883226721666e-05)
% --(axis cs:500,4.46406695206031e-05)
% --(axis cs:600,1.02843224743784e-05)
% --(axis cs:700,5.29838703217433e-06)
% --(axis cs:800,5.35557318862625e-06)
% --(axis cs:900,4.71908551842616e-06)
% --(axis cs:1000,4.49350902761194e-06)
% --(axis cs:1100,4.00285680356436e-06)
% --(axis cs:1200,3.68902778221341e-06)
% --(axis cs:1300,3.74756805223592e-06)
% --(axis cs:1400,3.40687299851253e-06)
% --(axis cs:1500,3.54020987264732e-06)
% --(axis cs:1600,3.31735173988412e-06)
% --(axis cs:1700,2.52894749826654e-06)
% --(axis cs:1800,2.04479385129744e-06)
% --(axis cs:1900,1.46819049233621e-06)
% --(axis cs:2000,1.20937839183694e-06)
% --(axis cs:2100,8.83959440466475e-07)
% --(axis cs:2200,1.13156227700457e-06)
% --(axis cs:2300,1.3841504999451e-06)
% --(axis cs:2400,1.43339024241268e-06)
% --(axis cs:2500,1.18004535433364e-06)
% --(axis cs:2600,1.33810817642407e-06)
% --(axis cs:2700,1.37241162055263e-06)
% --(axis cs:2800,1.21200256156368e-06)
% --(axis cs:2900,1.01234042086355e-06)
% --(axis cs:3000,7.68999874265997e-07)
% --(axis cs:3100,9.95689618810181e-07)
% --(axis cs:3200,9.36700210101438e-07)
% --(axis cs:3300,6.98299071599222e-07)
% --(axis cs:3400,6.79344142003069e-07)
% --(axis cs:3500,7.59825713253006e-07)
% --(axis cs:3600,9.18450335488926e-07)
% --(axis cs:3700,7.26726995394247e-07)
% --(axis cs:3800,1.0123530323837e-06)
% --(axis cs:3900,1.56940697711807e-06)
% --(axis cs:4000,1.73876949576774e-06)
% --(axis cs:4100,1.54146916924032e-06)
% --(axis cs:4200,1.31533423897182e-06)
% --(axis cs:4300,9.95238338441506e-07)
% --(axis cs:4400,5.41651739167894e-07)
% --(axis cs:4500,6.32367272627878e-07)
% --(axis cs:4600,5.04291186074788e-07)
% --(axis cs:4700,4.55202218275634e-07)
% --(axis cs:4800,7.46787726061518e-07)
% --(axis cs:4900,1.07691324851694e-06)
% --(axis cs:5000,1.03945674675542e-06)
% --(axis cs:5100,1.07404358989069e-06)
% --(axis cs:5200,8.10099696640482e-07)
% --(axis cs:5300,6.2965401890077e-07)
% --(axis cs:5400,5.73445066416441e-07)
% --(axis cs:5500,5.48310194796345e-07)
% --(axis cs:5600,5.3077689470012e-07)
% --(axis cs:5700,6.26564664872692e-07)
% --(axis cs:5800,8.28362582941074e-07)
% --(axis cs:5900,5.63954254088894e-07)
% --(axis cs:6000,4.88812407194329e-07)
% --(axis cs:6100,3.40299444848859e-07)
% --(axis cs:6200,3.23935931102097e-07)
% --(axis cs:6300,3.47125250016586e-07)
% --(axis cs:6400,4.79411478673294e-07)
% --(axis cs:6500,7.78318424539115e-07)
% --(axis cs:6600,8.7573665970425e-07)
% --(axis cs:6700,7.064255961975e-07)
% --(axis cs:6800,6.03133991937097e-07)
% --(axis cs:6900,5.77965967785852e-07)
% --(axis cs:7000,5.87279443682352e-07)
% --(axis cs:7100,6.1074356908896e-07)
% --(axis cs:7200,5.19969258281661e-07)
% --(axis cs:7300,3.38732196508627e-07)
% --(axis cs:7400,2.51549331892079e-07)
% --(axis cs:7500,1.8487425036272e-07)
% --(axis cs:7600,8.65769065775067e-07)
% --(axis cs:7700,8.79369455834476e-07)
% --(axis cs:7800,7.7165238097928e-07)
% --(axis cs:7900,4.12884339349456e-07)
% --(axis cs:8000,3.59925667551361e-07)
% --(axis cs:8100,2.78561197770499e-07)
% --(axis cs:8200,3.01857639487925e-07)
% --(axis cs:8300,3.19167889529139e-07)
% --(axis cs:8400,3.81851432113196e-07)
% --(axis cs:8500,4.02930722251624e-07)
% --(axis cs:8600,4.55073170792999e-07)
% --(axis cs:8700,3.73132947326872e-07)
% --(axis cs:8800,3.16944519117131e-07)
% --(axis cs:8900,3.46004635615711e-07)
% --(axis cs:9000,3.80488085915583e-07)
% --(axis cs:9100,4.2618779365994e-07)
% --(axis cs:9200,3.18021476813527e-07)
% --(axis cs:9300,1.97785553694165e-07)
% --(axis cs:9400,2.28291634324844e-07)
% --(axis cs:9500,2.06776105554434e-07)
% --(axis cs:9600,1.18431999680602e-07)
% --(axis cs:9700,1.51185544835599e-07)
% --(axis cs:9800,2.03042492160781e-07)
% --(axis cs:9900,1.75055725009698e-07)
% --(axis cs:10000,1.19691803578709e-07)
% --(axis cs:10100,2.3917625277176e-07)
% --(axis cs:10200,1.56405588321065e-07)
% --(axis cs:10300,9.70476644267384e-08)
% --(axis cs:10400,1.23556166534091e-07)
% --(axis cs:10500,8.98920598124252e-07)
% --(axis cs:10600,4.59067657400785e-07)
% --(axis cs:10700,3.84408714894547e-07)
% --(axis cs:10800,4.20438747684732e-07)
% --(axis cs:10900,4.63843797849816e-07)
% --(axis cs:11000,2.87379120192118e-07)
% --(axis cs:11100,1.50064380954449e-07)
% --(axis cs:11200,1.15921360355968e-07)
% --(axis cs:11300,1.22304685479995e-07)
% --(axis cs:11400,1.59657699931405e-07)
% --(axis cs:11500,1.8387101403527e-07)
% --(axis cs:11600,2.18867908867593e-07)
% --(axis cs:11700,2.54487984681877e-07)
% --(axis cs:11800,2.41406594115005e-07)
% --(axis cs:11900,2.0246756910613e-07)
% --(axis cs:12000,1.98657743197251e-07)
% --(axis cs:12100,2.20250979588355e-07)
% --(axis cs:12200,1.87585345032911e-07)
% --(axis cs:12300,1.40267040167681e-07)
% --(axis cs:12400,2.04395235230092e-07)
% --(axis cs:12500,2.95810943672461e-07)
% --(axis cs:12600,4.01024863339297e-07)
% --(axis cs:12700,2.88739734739371e-07)
% --(axis cs:12800,2.41619197233638e-07)
% --(axis cs:12900,1.79975121579748e-07)
% --(axis cs:13000,1.37457440375164e-07)
% --(axis cs:13100,1.79532397242409e-07)
% --(axis cs:13200,1.43345095303038e-07)
% --(axis cs:13300,1.79639838693268e-07)
% --(axis cs:13400,1.85593786333157e-07)
% --(axis cs:13500,1.83219763416472e-07)
% --(axis cs:13600,2.1506923836685e-07)
% --(axis cs:13700,1.86733255327257e-07)
% --(axis cs:13800,1.82760050488427e-07)
% --(axis cs:13900,1.97214641156312e-07)
% --(axis cs:14000,1.90530533868613e-07)
% --(axis cs:14100,1.85232214991068e-07)
% --(axis cs:14200,9.04868913665956e-08)
% --(axis cs:14300,1.00202052461735e-07)
% --(axis cs:14400,1.03065238475555e-07)
% --(axis cs:14500,8.49441046546309e-08)
% --(axis cs:14600,6.37015906135568e-08)
% --(axis cs:14700,7.78574297751062e-08)
% --(axis cs:14800,1.25848667112552e-07)
% --(axis cs:14900,1.62181360672863e-07)
% --(axis cs:15000,1.82365723417208e-07)
% --(axis cs:15100,1.51444658334205e-07)
% --(axis cs:15200,1.47105747773509e-07)
% --(axis cs:15300,1.58538247025757e-07)
% --(axis cs:15400,1.3218640804372e-07)
% --(axis cs:15500,1.54298763647474e-07)
% --(axis cs:15600,1.58119590692589e-07)
% --(axis cs:15700,1.77811016782455e-07)
% --(axis cs:15800,1.09538931297841e-07)
% --(axis cs:15900,1.06247262508113e-07)
% --(axis cs:16000,1.18726528502596e-07)
% --(axis cs:16100,1.15560663777059e-07)
% --(axis cs:16200,1.23678627765331e-07)
% --(axis cs:16300,1.28838918570817e-07)
% --(axis cs:16400,1.51389845446309e-07)
% --(axis cs:16500,9.02434029282274e-08)
% --(axis cs:16600,1.04844999061501e-07)
% --(axis cs:16700,1.15261403248943e-07)
% --(axis cs:16800,1.18071855111216e-07)
% --(axis cs:16900,1.37745028441778e-07)
% --(axis cs:17000,9.98670314511615e-08)
% --(axis cs:17100,9.08813276005738e-08)
% --(axis cs:17200,6.51170741261846e-08)
% --(axis cs:17300,6.20167533026171e-08)
% --(axis cs:17400,5.99842460284918e-08)
% --(axis cs:17500,7.2427020768037e-08)
% --(axis cs:17600,1.34730488419317e-07)
% --(axis cs:17700,1.91083853983198e-07)
% --(axis cs:17800,1.94515463006321e-07)
% --(axis cs:17900,1.70826180127376e-07)
% --(axis cs:18000,1.64133675124854e-07)
% --(axis cs:18100,1.14779206942172e-07)
% --(axis cs:18200,7.91653137284243e-08)
% --(axis cs:18300,7.51629293251699e-08)
% --(axis cs:18400,1.22895241222491e-07)
% --(axis cs:18500,1.45933769665644e-07)
% --(axis cs:18600,1.64797266032573e-07)
% --(axis cs:18700,1.61815452523992e-07)
% --(axis cs:18800,1.31348880838222e-07)
% --(axis cs:18900,9.00868993384896e-08)
% --(axis cs:19000,9.93642096223723e-08)
% --(axis cs:19100,1.11611364914039e-07)
% --(axis cs:19200,1.11929010231541e-07)
% --(axis cs:19300,9.53764275134729e-08)
% --(axis cs:19400,9.78673292858818e-08)
% --(axis cs:19500,1.07521050891307e-07)
% --(axis cs:19600,1.31596411828329e-07)
% --(axis cs:19700,1.60046232811471e-07)
% --(axis cs:19800,1.0023600947716e-07)
% --(axis cs:19900,9.40272100443918e-08)
% --(axis cs:20000,8.99486333663286e-08)
% --(axis cs:20100,7.55255826399129e-08)
% --(axis cs:20200,7.49217924141428e-08)
% --(axis cs:20300,7.5776411450244e-08)
% --(axis cs:20400,7.06546116293956e-08)
% --(axis cs:20500,8.14985556374027e-08)
% --(axis cs:20600,9.30987497218909e-08)
% --(axis cs:20700,9.71810007950387e-08)
% --(axis cs:20800,1.285210169101e-07)
% --(axis cs:20900,1.52903900085207e-07)
% --(axis cs:21000,1.51626420490319e-07)
% --(axis cs:21100,1.3538094613682e-07)
% --(axis cs:21200,8.97272241218025e-08)
% --(axis cs:21300,6.19345540659784e-08)
% --(axis cs:21400,6.17418875261403e-08)
% --(axis cs:21500,6.8650885214555e-08)
% --(axis cs:21600,7.06565961647565e-08)
% --(axis cs:21700,6.91924239377453e-08)
% --(axis cs:21800,7.93055700161606e-08)
% --(axis cs:21900,8.47239546863942e-08)
% --(axis cs:22000,9.66936656234662e-08)
% --(axis cs:22100,8.97755559938677e-08)
% --(axis cs:22200,8.3072202025465e-08)
% --(axis cs:22300,7.58240625881376e-08)
% --(axis cs:22400,8.31646873179629e-08)
% --(axis cs:22500,6.53350024764034e-08)
% --(axis cs:22600,6.39574827365831e-08)
% --(axis cs:22700,6.6878026360919e-08)
% --(axis cs:22800,7.11112040537786e-08)
% --(axis cs:22900,7.43568674976957e-08)
% --(axis cs:23000,7.50888242627201e-08)
% --(axis cs:23100,6.90552909803336e-08)
% --(axis cs:23200,7.06320202698839e-08)
% --(axis cs:23300,6.32707414374113e-08)
% --(axis cs:23400,6.37156469646599e-08)
% --(axis cs:23500,6.693251434724e-08)
% --(axis cs:23600,6.84976308646538e-08)
% --(axis cs:23700,6.46089049438707e-08)
% --(axis cs:23800,5.64810821300323e-08)
% --(axis cs:23900,5.9155493944885e-08)
% --(axis cs:24000,5.91516438516394e-08)
% --(axis cs:24100,5.14710185418025e-08)
% --(axis cs:24200,5.28151672093938e-08)
% --(axis cs:24300,5.51261578227021e-08)
% --(axis cs:24400,5.49525602837249e-08)
% --(axis cs:24500,5.71382162242482e-08)
% --(axis cs:24600,5.75162436810462e-08)
% --(axis cs:24700,5.7571254479616e-08)
% --(axis cs:24800,5.9621675372547e-08)
% --(axis cs:24900,5.70751873275797e-08)
% --(axis cs:25000,5.11720833025534e-08)
% --(axis cs:25100,4.84046104001374e-08)
% --(axis cs:25200,5.09419211198294e-08)
% --(axis cs:25300,5.92823026466326e-08)
% --(axis cs:25400,6.43974100282108e-08)
% --(axis cs:25500,6.06597082024409e-08)
% --(axis cs:25600,5.21233155989196e-08)
% --(axis cs:25700,5.22309142420273e-08)
% --(axis cs:25800,5.54433669058994e-08)
% --(axis cs:25900,5.22084639431098e-08)
% --(axis cs:26000,5.78177968215687e-08)
% --(axis cs:26100,6.04059956189445e-08)
% --(axis cs:26200,6.59539852970111e-08)
% --(axis cs:26300,6.80669157469955e-08)
% --(axis cs:26400,5.0206283536039e-08)
% --(axis cs:26500,4.63090425714954e-08)
% --(axis cs:26600,4.77610960876925e-08)
% --(axis cs:26700,4.73235331028316e-08)
% --(axis cs:26800,4.75759854639227e-08)
% --(axis cs:26900,4.78838093559873e-08)
% --(axis cs:27000,4.79800461879012e-08)
% --(axis cs:27100,4.74734666953783e-08)
% --(axis cs:27200,5.07813887854256e-08)
% --(axis cs:27300,4.69159066868671e-08)
% --(axis cs:27400,4.55229380454569e-08)
% --(axis cs:27500,4.92032748748411e-08)
% --(axis cs:27600,5.06620021980735e-08)
% --(axis cs:27700,4.94613917313396e-08)
% --(axis cs:27800,5.16044203483205e-08)
% --(axis cs:27900,5.03406464332689e-08)
% --(axis cs:28000,4.62699926487458e-08)
% --(axis cs:28100,4.5112300289396e-08)
% --(axis cs:28200,4.49963680341189e-08)
% --(axis cs:28300,4.35720893505885e-08)
% --(axis cs:28400,4.41378713211847e-08)
% --(axis cs:28500,4.46048777727566e-08)
% --(axis cs:28600,4.35246628705318e-08)
% --(axis cs:28700,4.36973416340254e-08)
% --(axis cs:28800,4.41672620814289e-08)
% --(axis cs:28900,4.55690771079946e-08)
% --(axis cs:29000,4.50573677805153e-08)
% --(axis cs:29100,4.52931017665489e-08)
% --(axis cs:29200,4.51177590576931e-08)
% --(axis cs:29300,4.62542791731245e-08)
% --(axis cs:29400,4.52196049149175e-08)
% --(axis cs:29500,4.76437205340858e-08)
% --(axis cs:29500,5.26885583657796e-08)
% --(axis cs:29500,5.26885583657796e-08)
% --(axis cs:29400,5.12635787202071e-08)
% --(axis cs:29300,5.18282850011192e-08)
% --(axis cs:29200,5.27324325361138e-08)
% --(axis cs:29100,5.20447984623732e-08)
% --(axis cs:29000,5.07186472494538e-08)
% --(axis cs:28900,5.38596846492863e-08)
% --(axis cs:28800,5.16915614937463e-08)
% --(axis cs:28700,5.07352123498295e-08)
% --(axis cs:28600,5.22339144933115e-08)
% --(axis cs:28500,5.12124572120776e-08)
% --(axis cs:28400,7.2890112190098e-08)
% --(axis cs:28300,7.61719413996615e-08)
% --(axis cs:28200,7.95299611252612e-08)
% --(axis cs:28100,8.00297885206599e-08)
% --(axis cs:28000,7.84788368103006e-08)
% --(axis cs:27900,5.39765190798732e-08)
% --(axis cs:27800,5.35281531133913e-08)
% --(axis cs:27700,5.52017280396362e-08)
% --(axis cs:27600,5.5444838567508e-08)
% --(axis cs:27500,5.56555989461414e-08)
% --(axis cs:27400,5.59623873423276e-08)
% --(axis cs:27300,5.31437341231162e-08)
% --(axis cs:27200,5.4194401053165e-08)
% --(axis cs:27100,5.97634946599054e-08)
% --(axis cs:27000,6.33629114214938e-08)
% --(axis cs:26900,6.3519808707845e-08)
% --(axis cs:26800,6.83101312388454e-08)
% --(axis cs:26700,6.47798923434137e-08)
% --(axis cs:26600,6.78444519208721e-08)
% --(axis cs:26500,1.02358318516933e-07)
% --(axis cs:26400,1.06909541525244e-07)
% --(axis cs:26300,1.03212895209553e-07)
% --(axis cs:26200,1.09260680590313e-07)
% --(axis cs:26100,1.08628400816619e-07)
% --(axis cs:26000,7.96413101494439e-08)
% --(axis cs:25900,7.57623357620955e-08)
% --(axis cs:25800,7.53056558435181e-08)
% --(axis cs:25700,8.50630128592031e-08)
% --(axis cs:25600,8.62982191392042e-08)
% --(axis cs:25500,8.90531445199943e-08)
% --(axis cs:25400,9.50251962879733e-08)
% --(axis cs:25300,8.60851288677546e-08)
% --(axis cs:25200,8.86590335577843e-08)
% --(axis cs:25100,9.95223452624321e-08)
% --(axis cs:25000,8.17839316062604e-08)
% --(axis cs:24900,7.18449140519316e-08)
% --(axis cs:24800,6.76903484247596e-08)
% --(axis cs:24700,6.7859551055042e-08)
% --(axis cs:24600,6.35156633044897e-08)
% --(axis cs:24500,7.50876174949794e-08)
% --(axis cs:24400,8.38492327681247e-08)
% --(axis cs:24300,8.84615763540364e-08)
% --(axis cs:24200,8.78264393588061e-08)
% --(axis cs:24100,8.78299961518503e-08)
% --(axis cs:24000,7.51358277206155e-08)
% --(axis cs:23900,7.01604128971056e-08)
% --(axis cs:23800,7.49108302127978e-08)
% --(axis cs:23700,7.70409769246179e-08)
% --(axis cs:23600,8.40582383466774e-08)
% --(axis cs:23500,1.4099966971625e-07)
% --(axis cs:23400,1.47876997951776e-07)
% --(axis cs:23300,1.52630989426347e-07)
% --(axis cs:23200,1.50224422671532e-07)
% --(axis cs:23100,1.42769071869832e-07)
% --(axis cs:23000,8.31748622192911e-08)
% --(axis cs:22900,8.3014649209221e-08)
% --(axis cs:22800,1.02191651863952e-07)
% --(axis cs:22700,9.43662334203749e-08)
% --(axis cs:22600,9.5527859766217e-08)
% --(axis cs:22500,9.81370683664446e-08)
% --(axis cs:22400,1.00121420040109e-07)
% --(axis cs:22300,9.28634383573149e-08)
% --(axis cs:22200,1.0592516920925e-07)
% --(axis cs:22100,1.10085313549177e-07)
% --(axis cs:22000,1.10105117511358e-07)
% --(axis cs:21900,1.15648709315315e-07)
% --(axis cs:21800,1.11600815913026e-07)
% --(axis cs:21700,1.02458239641488e-07)
% --(axis cs:21600,9.7771883531802e-08)
% --(axis cs:21500,9.05774653494045e-08)
% --(axis cs:21400,9.29730832641969e-08)
% --(axis cs:21300,1.25525012736794e-07)
% --(axis cs:21200,1.89772569854099e-07)
% --(axis cs:21100,1.95234963031529e-07)
% --(axis cs:21000,1.99211599360303e-07)
% --(axis cs:20900,2.02799838733895e-07)
% --(axis cs:20800,2.13050893756871e-07)
% --(axis cs:20700,1.59427332128216e-07)
% --(axis cs:20600,1.09560000266999e-07)
% --(axis cs:20500,1.01479062960207e-07)
% --(axis cs:20400,9.70433491329297e-08)
% --(axis cs:20300,8.06849923827197e-08)
% --(axis cs:20200,9.61217446086541e-08)
% --(axis cs:20100,1.54200730591606e-07)
% --(axis cs:20000,1.79921543920344e-07)
% --(axis cs:19900,1.90758904882861e-07)
% --(axis cs:19800,1.89203467827002e-07)
% --(axis cs:19700,1.79617281333209e-07)
% --(axis cs:19600,1.67900444523929e-07)
% --(axis cs:19500,1.71251537174291e-07)
% --(axis cs:19400,1.82558358244439e-07)
% --(axis cs:19300,1.77256129609185e-07)
% --(axis cs:19200,1.48050029427663e-07)
% --(axis cs:19100,1.85256597950135e-07)
% --(axis cs:19000,2.44637690883576e-07)
% --(axis cs:18900,2.71489320767048e-07)
% --(axis cs:18800,3.18291400555012e-07)
% --(axis cs:18700,2.61981720712085e-07)
% --(axis cs:18600,2.10506470144984e-07)
% --(axis cs:18500,1.94892220816449e-07)
% --(axis cs:18400,2.03188461631909e-07)
% --(axis cs:18300,1.7402737059541e-07)
% --(axis cs:18200,1.71334279606583e-07)
% --(axis cs:18100,2.25643775068881e-07)
% --(axis cs:18000,2.35466310094987e-07)
% --(axis cs:17900,2.33407500593839e-07)
% --(axis cs:17800,2.44043058403184e-07)
% --(axis cs:17700,2.42967949701375e-07)
% --(axis cs:17600,2.41458336738125e-07)
% --(axis cs:17500,2.59349815754561e-07)
% --(axis cs:17400,2.57605122108814e-07)
% --(axis cs:17300,2.62195262509392e-07)
% --(axis cs:17200,2.49068229662203e-07)
% --(axis cs:17100,2.181129025428e-07)
% --(axis cs:17000,1.99302781027633e-07)
% --(axis cs:16900,6.70705887252184e-07)
% --(axis cs:16800,7.19223437780603e-07)
% --(axis cs:16700,7.24961598562618e-07)
% --(axis cs:16600,7.24144841267586e-07)
% --(axis cs:16500,7.52616486450891e-07)
% --(axis cs:16400,1.97998219107744e-07)
% --(axis cs:16300,1.76586419309358e-07)
% --(axis cs:16200,1.8927125536839e-07)
% --(axis cs:16100,2.12092369343079e-07)
% --(axis cs:16000,2.06525929353044e-07)
% --(axis cs:15900,2.52865802465713e-07)
% --(axis cs:15800,2.34983494815909e-07)
% --(axis cs:15700,2.74979420776329e-07)
% --(axis cs:15600,3.02265953750354e-07)
% --(axis cs:15500,3.00907185731505e-07)
% --(axis cs:15400,3.05392401883474e-07)
% --(axis cs:15300,3.12853655553186e-07)
% --(axis cs:15200,2.63121652720059e-07)
% --(axis cs:15100,2.59541476745633e-07)
% --(axis cs:15000,3.00263573584135e-07)
% --(axis cs:14900,3.18946182466474e-07)
% --(axis cs:14800,3.11898769764082e-07)
% --(axis cs:14700,3.4305685368222e-07)
% --(axis cs:14600,3.19518720929622e-07)
% --(axis cs:14500,1.94811804450375e-07)
% --(axis cs:14400,1.86839151677566e-07)
% --(axis cs:14300,3.25179935187379e-07)
% --(axis cs:14200,3.61273040378174e-07)
% --(axis cs:14100,5.03144865383805e-07)
% --(axis cs:14000,5.57134995974676e-07)
% --(axis cs:13900,5.47623618298801e-07)
% --(axis cs:13800,5.57451796054659e-07)
% --(axis cs:13700,5.73723939487733e-07)
% --(axis cs:13600,4.11507137957463e-07)
% --(axis cs:13500,4.23257646860797e-07)
% --(axis cs:13400,4.26498781705098e-07)
% --(axis cs:13300,3.04361453803067e-07)
% --(axis cs:13200,2.73723978137226e-07)
% --(axis cs:13100,2.1335512959571e-07)
% --(axis cs:13000,4.01625934068623e-07)
% --(axis cs:12900,5.10120777778564e-07)
% --(axis cs:12800,6.119353257094e-07)
% --(axis cs:12700,6.09861945200862e-07)
% --(axis cs:12600,5.36964784924895e-07)
% --(axis cs:12500,5.40402644537975e-07)
% --(axis cs:12400,4.61262739496157e-07)
% --(axis cs:12300,4.28364786376046e-07)
% --(axis cs:12200,4.1320034887207e-07)
% --(axis cs:12100,4.36927232231225e-07)
% --(axis cs:12000,4.46908820919711e-07)
% --(axis cs:11900,4.70892678454465e-07)
% --(axis cs:11800,4.27874182225499e-07)
% --(axis cs:11700,3.72089897045645e-07)
% --(axis cs:11600,3.06199184936361e-07)
% --(axis cs:11500,3.05498010083214e-07)
% --(axis cs:11400,3.20137412627248e-07)
% --(axis cs:11300,3.45095578434901e-07)
% --(axis cs:11200,3.9407320829408e-07)
% --(axis cs:11100,3.84068457508186e-07)
% --(axis cs:11000,3.73043595552247e-07)
% --(axis cs:10900,1.08753983810616e-06)
% --(axis cs:10800,1.17114449440401e-06)
% --(axis cs:10700,1.19348892082752e-06)
% --(axis cs:10600,1.13259698067421e-06)
% --(axis cs:10500,9.7001254641633e-07)
% --(axis cs:10400,8.57609802441407e-07)
% --(axis cs:10300,8.53898488092119e-07)
% --(axis cs:10200,8.30417842235125e-07)
% --(axis cs:10100,7.62368320607697e-07)
% --(axis cs:10000,4.8790232124162e-07)
% --(axis cs:9900,5.31194413657806e-07)
% --(axis cs:9800,6.20447544651995e-07)
% --(axis cs:9700,6.36179142628204e-07)
% --(axis cs:9600,6.10198184063315e-07)
% --(axis cs:9500,6.98871099201214e-07)
% --(axis cs:9400,6.40919128419088e-07)
% --(axis cs:9300,7.36890815792763e-07)
% --(axis cs:9200,8.33371354575348e-07)
% --(axis cs:9100,8.96821104034974e-07)
% --(axis cs:9000,8.72599372592579e-07)
% --(axis cs:8900,8.91266910875367e-07)
% --(axis cs:8800,8.1288085428924e-07)
% --(axis cs:8700,5.82354391818724e-07)
% --(axis cs:8600,5.47265219036069e-07)
% --(axis cs:8500,6.96842733104396e-07)
% --(axis cs:8400,6.64242819819832e-07)
% --(axis cs:8300,5.96586506162554e-07)
% --(axis cs:8200,5.34872527502264e-07)
% --(axis cs:8100,4.16880596810605e-07)
% --(axis cs:8000,1.00303974065862e-06)
% --(axis cs:7900,1.03754549365961e-06)
% --(axis cs:7800,1.02820146815149e-06)
% --(axis cs:7700,1.0355163471549e-06)
% --(axis cs:7600,9.55408312964406e-07)
% --(axis cs:7500,8.30754894392598e-07)
% --(axis cs:7400,8.32478735181856e-07)
% --(axis cs:7300,7.33859825447016e-07)
% --(axis cs:7200,8.06731467885812e-07)
% --(axis cs:7100,9.57861232516074e-07)
% --(axis cs:7000,1.07223899400873e-06)
% --(axis cs:6900,1.31385608980113e-06)
% --(axis cs:6800,1.31568161070834e-06)
% --(axis cs:6700,1.12365014985904e-06)
% --(axis cs:6600,1.09977268360623e-06)
% --(axis cs:6500,1.25936255360431e-06)
% --(axis cs:6400,1.23671331050545e-06)
% --(axis cs:6300,1.04801598321996e-06)
% --(axis cs:6200,1.03121686267101e-06)
% --(axis cs:6100,8.41412400446912e-07)
% --(axis cs:6000,7.27502552904593e-07)
% --(axis cs:5900,8.25606321552357e-07)
% --(axis cs:5800,9.62671295421139e-07)
% --(axis cs:5700,1.21738414577725e-06)
% --(axis cs:5600,1.97296362711227e-06)
% --(axis cs:5500,1.90584687761047e-06)
% --(axis cs:5400,1.88325593088334e-06)
% --(axis cs:5300,1.81215891771843e-06)
% --(axis cs:5200,1.94847277472883e-06)
% --(axis cs:5100,1.60622923204777e-06)
% --(axis cs:5000,1.59200503310077e-06)
% --(axis cs:4900,1.55001410907935e-06)
% --(axis cs:4800,1.74352166600174e-06)
% --(axis cs:4700,1.82446264157065e-06)
% --(axis cs:4600,1.16670724048692e-06)
% --(axis cs:4500,1.28398985783617e-06)
% --(axis cs:4400,1.45039370711839e-06)
% --(axis cs:4300,1.55624965287501e-06)
% --(axis cs:4200,2.13661210508561e-06)
% --(axis cs:4100,2.09136513980902e-06)
% --(axis cs:4000,2.22017556981381e-06)
% --(axis cs:3900,2.31515287391258e-06)
% --(axis cs:3800,2.32350574710517e-06)
% --(axis cs:3700,1.48891899851027e-06)
% --(axis cs:3600,1.32209960908024e-06)
% --(axis cs:3500,1.18442920653415e-06)
% --(axis cs:3400,1.33830124008405e-06)
% --(axis cs:3300,1.28198757263648e-06)
% --(axis cs:3200,1.46805331095182e-06)
% --(axis cs:3100,1.74143164694732e-06)
% --(axis cs:3000,2.05959257814622e-06)
% --(axis cs:2900,2.29075769250468e-06)
% --(axis cs:2800,2.28869677418191e-06)
% --(axis cs:2700,2.14072557062004e-06)
% --(axis cs:2600,2.23885992982068e-06)
% --(axis cs:2500,2.27828032009145e-06)
% --(axis cs:2400,2.07053447228943e-06)
% --(axis cs:2300,2.15492101601898e-06)
% --(axis cs:2200,2.04767882425051e-06)
% --(axis cs:2100,1.96049255318158e-06)
% --(axis cs:2000,1.98253263757662e-06)
% --(axis cs:1900,2.06774312290342e-06)
% --(axis cs:1800,2.71481060350221e-06)
% --(axis cs:1700,4.10527864274104e-06)
% --(axis cs:1600,4.40051281224545e-06)
% --(axis cs:1500,4.89623727261479e-06)
% --(axis cs:1400,5.09826112688284e-06)
% --(axis cs:1300,5.13004441383426e-06)
% --(axis cs:1200,5.88082314146442e-06)
% --(axis cs:1100,6.26057189961895e-06)
% --(axis cs:1000,6.36549779418684e-06)
% --(axis cs:900,7.58061911864185e-06)
% --(axis cs:800,7.05881879096831e-06)
% --(axis cs:700,7.48210324339509e-06)
% --(axis cs:600,2.15491547250679e-05)
% --(axis cs:500,5.9453852182188e-05)
% --(axis cs:400,0.000102723626650517)
% --(axis cs:300,0.000341219213264364)
% --(axis cs:200,0.000655921135991287)
% --(axis cs:100,0.000921005287494679)
% --(axis cs:0,0.00118464536959966)
% --cycle;

\path [fill=green!50.1960784313725!black, fill opacity=0.2, semithick]
(axis cs:0,0.00449837547693887)
--(axis cs:0,0.00445945200232925)
--(axis cs:100,0.00352351291189394)
--(axis cs:200,0.00246974431810779)
--(axis cs:300,0.00139723591805478)
--(axis cs:400,0.000421370500234841)
--(axis cs:500,0.000216971571399304)
--(axis cs:600,6.91006405808362e-05)
--(axis cs:700,4.63637142932481e-05)
--(axis cs:800,4.24799811598135e-05)
--(axis cs:900,4.15213910157181e-05)
--(axis cs:1000,4.0478461836091e-05)
--(axis cs:1100,3.75924312312409e-05)
--(axis cs:1200,3.56021672569982e-05)
--(axis cs:1300,3.31457199784438e-05)
--(axis cs:1400,3.06518838320572e-05)
--(axis cs:1500,2.83983358201886e-05)
--(axis cs:1600,2.40241218088796e-05)
--(axis cs:1700,1.9745692758179e-05)
--(axis cs:1800,1.64624814564277e-05)
--(axis cs:1900,1.32978115518751e-05)
--(axis cs:2000,1.03327662406265e-05)
--(axis cs:2100,8.07260090997263e-06)
--(axis cs:2200,8.29290126586312e-06)
--(axis cs:2300,9.27048956268279e-06)
--(axis cs:2400,9.44797900827402e-06)
--(axis cs:2500,8.63404210434559e-06)
--(axis cs:2600,8.29023022485574e-06)
--(axis cs:2700,8.41399354215724e-06)
--(axis cs:2800,7.64645779037612e-06)
--(axis cs:2900,6.62409801876726e-06)
--(axis cs:3000,5.86446345196679e-06)
--(axis cs:3100,6.33813767931426e-06)
--(axis cs:3200,6.09676840364437e-06)
--(axis cs:3300,5.38150144945564e-06)
--(axis cs:3400,5.0792154161001e-06)
--(axis cs:3500,5.4248875683209e-06)
--(axis cs:3600,5.60523339300165e-06)
--(axis cs:3700,4.65859504124485e-06)
--(axis cs:3800,5.54493732410941e-06)
--(axis cs:3900,7.29823998768081e-06)
--(axis cs:4000,7.55405075732103e-06)
--(axis cs:4100,7.57265195803507e-06)
--(axis cs:4200,6.62052326989399e-06)
--(axis cs:4300,4.89903037206679e-06)
--(axis cs:4400,3.32889378724159e-06)
--(axis cs:4500,3.39908289013855e-06)
--(axis cs:4600,2.98309937301594e-06)
--(axis cs:4700,3.11471838510394e-06)
--(axis cs:4800,4.19249322204491e-06)
--(axis cs:4900,5.09647022836376e-06)
--(axis cs:5000,5.01127723360426e-06)
--(axis cs:5100,4.94662450645089e-06)
--(axis cs:5200,3.8242925326116e-06)
--(axis cs:5300,3.36871805104896e-06)
--(axis cs:5400,3.25021855352917e-06)
--(axis cs:5500,2.98221489541751e-06)
--(axis cs:5600,2.94823781695411e-06)
--(axis cs:5700,2.90812043008226e-06)
--(axis cs:5800,3.86406425158883e-06)
--(axis cs:5900,2.86888852941347e-06)
--(axis cs:6000,2.66851615026582e-06)
--(axis cs:6100,2.0374045103609e-06)
--(axis cs:6200,1.95796915001008e-06)
--(axis cs:6300,2.06477645195743e-06)
--(axis cs:6400,2.60072651227414e-06)
--(axis cs:6500,3.61788715636313e-06)
--(axis cs:6600,4.38730125413529e-06)
--(axis cs:6700,3.5657669463309e-06)
--(axis cs:6800,2.88221395862267e-06)
--(axis cs:6900,2.85906968151521e-06)
--(axis cs:7000,2.68281896679848e-06)
--(axis cs:7100,2.45430058717989e-06)
--(axis cs:7200,2.07947565340931e-06)
--(axis cs:7300,1.63675386567432e-06)
--(axis cs:7400,1.64192193274382e-06)
--(axis cs:7500,1.44037692334462e-06)
--(axis cs:7600,3.7303380778439e-06)
--(axis cs:7700,3.76095979882007e-06)
--(axis cs:7800,3.33871441927903e-06)
--(axis cs:7900,2.04856485380417e-06)
--(axis cs:8000,1.79411681769998e-06)
--(axis cs:8100,1.63503915025145e-06)
--(axis cs:8200,1.72032580391565e-06)
--(axis cs:8300,1.7874774206667e-06)
--(axis cs:8400,1.97885601696949e-06)
--(axis cs:8500,2.14917846547462e-06)
--(axis cs:8600,2.39335736076688e-06)
--(axis cs:8700,2.09123897783466e-06)
--(axis cs:8800,1.90677128411918e-06)
--(axis cs:8900,1.94973716737513e-06)
--(axis cs:9000,2.01249387171979e-06)
--(axis cs:9100,2.15883856467456e-06)
--(axis cs:9200,1.7498822738093e-06)
--(axis cs:9300,1.19981254579661e-06)
--(axis cs:9400,1.38425716381686e-06)
--(axis cs:9500,1.26674987447627e-06)
--(axis cs:9600,1.00581652064655e-06)
--(axis cs:9700,1.14706576725308e-06)
--(axis cs:9800,1.33568486205104e-06)
--(axis cs:9900,1.1340092784812e-06)
--(axis cs:10000,9.64580993404274e-07)
--(axis cs:10100,1.4964353281989e-06)
--(axis cs:10200,1.08938301606765e-06)
--(axis cs:10300,7.89977619845803e-07)
--(axis cs:10400,9.63297112332554e-07)
--(axis cs:10500,3.16080095406717e-06)
--(axis cs:10600,2.11524423124246e-06)
--(axis cs:10700,1.84692817842832e-06)
--(axis cs:10800,1.91939513547296e-06)
--(axis cs:10900,2.17579439588671e-06)
--(axis cs:11000,1.73914009933789e-06)
--(axis cs:11100,1.08151008724651e-06)
--(axis cs:11200,1.01987991716817e-06)
--(axis cs:11300,1.05871913284336e-06)
--(axis cs:11400,1.18119814472279e-06)
--(axis cs:11500,1.32081721643084e-06)
--(axis cs:11600,1.44070107052567e-06)
--(axis cs:11700,1.60393920776416e-06)
--(axis cs:11800,1.38865207437599e-06)
--(axis cs:11900,1.28274418224753e-06)
--(axis cs:12000,1.28447879527369e-06)
--(axis cs:12100,1.3611302145807e-06)
--(axis cs:12200,1.29062446651353e-06)
--(axis cs:12300,1.09106861162727e-06)
--(axis cs:12400,1.4898247830599e-06)
--(axis cs:12500,1.84846577030112e-06)
--(axis cs:12600,2.14017433299595e-06)
--(axis cs:12700,1.79835494820691e-06)
--(axis cs:12800,1.52634928469357e-06)
--(axis cs:12900,1.16920145212692e-06)
--(axis cs:13000,1.0363116150529e-06)
--(axis cs:13100,1.2189664101681e-06)
--(axis cs:13200,1.02901454194821e-06)
--(axis cs:13300,1.13029670642714e-06)
--(axis cs:13400,1.18069721664129e-06)
--(axis cs:13500,1.17416440260043e-06)
--(axis cs:13600,1.30959653594775e-06)
--(axis cs:13700,1.08750432740075e-06)
--(axis cs:13800,1.13198490658828e-06)
--(axis cs:13900,1.19216911399216e-06)
--(axis cs:14000,1.17536917526159e-06)
--(axis cs:14100,1.1764806912782e-06)
--(axis cs:14200,9.33928595951547e-07)
--(axis cs:14300,8.95431794781332e-07)
--(axis cs:14400,8.96653418112718e-07)
--(axis cs:14500,8.17962215314668e-07)
--(axis cs:14600,7.48350548697843e-07)
--(axis cs:14700,7.49843657966543e-07)
--(axis cs:14800,9.06537027758013e-07)
--(axis cs:14900,1.05878452241717e-06)
--(axis cs:15000,1.16693563474571e-06)
--(axis cs:15100,1.1202556632813e-06)
--(axis cs:15200,1.06783214657186e-06)
--(axis cs:15300,1.15694915625948e-06)
--(axis cs:15400,1.1336248534076e-06)
--(axis cs:15500,1.14860615727918e-06)
--(axis cs:15600,1.15545360029924e-06)
--(axis cs:15700,1.17784168862599e-06)
--(axis cs:15800,8.91993920469887e-07)
--(axis cs:15900,8.72812258874893e-07)
--(axis cs:16000,9.2726008512246e-07)
--(axis cs:16100,9.22806993191877e-07)
--(axis cs:16200,9.89536219783453e-07)
--(axis cs:16300,1.01789984919965e-06)
--(axis cs:16400,1.13888275730859e-06)
--(axis cs:16500,1.09271618544443e-06)
--(axis cs:16600,1.15272084037823e-06)
--(axis cs:16700,1.16111347291579e-06)
--(axis cs:16800,1.16643964728845e-06)
--(axis cs:16900,1.17694745111674e-06)
--(axis cs:17000,9.2225779297503e-07)
--(axis cs:17100,8.68480498694259e-07)
--(axis cs:17200,7.50128619257662e-07)
--(axis cs:17300,7.21676023189354e-07)
--(axis cs:17400,6.88200420964277e-07)
--(axis cs:17500,7.21302507223292e-07)
--(axis cs:17600,9.67895674190774e-07)
--(axis cs:17700,1.25651267156862e-06)
--(axis cs:17800,1.25932682884233e-06)
--(axis cs:17900,1.12851759439886e-06)
--(axis cs:18000,1.10385384400018e-06)
--(axis cs:18100,9.81499530024514e-07)
--(axis cs:18200,7.86068978843684e-07)
--(axis cs:18300,7.62663657789036e-07)
--(axis cs:18400,8.64752885536999e-07)
--(axis cs:18500,9.17892168856732e-07)
--(axis cs:18600,1.08026046420359e-06)
--(axis cs:18700,1.15645968556931e-06)
--(axis cs:18800,9.66568223626273e-07)
--(axis cs:18900,8.16289166475721e-07)
--(axis cs:19000,8.81218332408752e-07)
--(axis cs:19100,9.13682890642854e-07)
--(axis cs:19200,8.69407958111729e-07)
--(axis cs:19300,8.75135654400552e-07)
--(axis cs:19400,8.8016426792582e-07)
--(axis cs:19500,8.78864402996416e-07)
--(axis cs:19600,9.4109696885563e-07)
--(axis cs:19700,1.13467412881162e-06)
--(axis cs:19800,8.88583413228817e-07)
--(axis cs:19900,8.50456678732006e-07)
--(axis cs:20000,8.30955843575499e-07)
--(axis cs:20100,7.62059729339421e-07)
--(axis cs:20200,7.45455258382823e-07)
--(axis cs:20300,7.43392132456848e-07)
--(axis cs:20400,7.41484944209227e-07)
--(axis cs:20500,7.85318216632383e-07)
--(axis cs:20600,8.26704986907649e-07)
--(axis cs:20700,8.6156122463453e-07)
--(axis cs:20800,9.40350047196766e-07)
--(axis cs:20900,1.04589411351445e-06)
--(axis cs:21000,1.02801791918053e-06)
--(axis cs:21100,9.85953472655906e-07)
--(axis cs:21200,8.51849874204178e-07)
--(axis cs:21300,6.92058664301961e-07)
--(axis cs:21400,6.96528797418244e-07)
--(axis cs:21500,7.50293746110954e-07)
--(axis cs:21600,7.52624525249565e-07)
--(axis cs:21700,7.37993228552054e-07)
--(axis cs:21800,7.86783628401386e-07)
--(axis cs:21900,8.08500205891203e-07)
--(axis cs:22000,8.30197691384983e-07)
--(axis cs:22100,8.09689607603351e-07)
--(axis cs:22200,7.74563721434166e-07)
--(axis cs:22300,7.38805985695783e-07)
--(axis cs:22400,7.5686096417335e-07)
--(axis cs:22500,7.08669161387273e-07)
--(axis cs:22600,7.00556281926737e-07)
--(axis cs:22700,7.20375852049946e-07)
--(axis cs:22800,7.34747689829762e-07)
--(axis cs:22900,7.44516696567714e-07)
--(axis cs:23000,7.48417041480538e-07)
--(axis cs:23100,7.44362294661131e-07)
--(axis cs:23200,7.43339319616696e-07)
--(axis cs:23300,7.04413875259323e-07)
--(axis cs:23400,6.96482909035663e-07)
--(axis cs:23500,7.15576916664534e-07)
--(axis cs:23600,7.01943419844788e-07)
--(axis cs:23700,6.89241940548449e-07)
--(axis cs:23800,6.78289604885683e-07)
--(axis cs:23900,6.76664719078444e-07)
--(axis cs:24000,6.75618145123006e-07)
--(axis cs:24100,6.52205592196682e-07)
--(axis cs:24200,6.51264262979963e-07)
--(axis cs:24300,6.52336179876227e-07)
--(axis cs:24400,6.57396116609503e-07)
--(axis cs:24500,6.71039983455245e-07)
--(axis cs:24600,6.81025202583525e-07)
--(axis cs:24700,6.86328362581838e-07)
--(axis cs:24800,6.92713636219897e-07)
--(axis cs:24900,6.88766045498569e-07)
--(axis cs:25000,6.58902087501817e-07)
--(axis cs:25100,6.52223718092291e-07)
--(axis cs:25200,6.58080766591838e-07)
--(axis cs:25300,6.69998120240141e-07)
--(axis cs:25400,6.78555736302025e-07)
--(axis cs:25500,6.45330933887989e-07)
--(axis cs:25600,6.28560536826791e-07)
--(axis cs:25700,6.23585294005598e-07)
--(axis cs:25800,6.40790121215028e-07)
--(axis cs:25900,6.55680734698577e-07)
--(axis cs:26000,6.656685871104e-07)
--(axis cs:26100,6.75138779025977e-07)
--(axis cs:26200,6.82958176267104e-07)
--(axis cs:26300,6.87832627067779e-07)
--(axis cs:26400,6.27604226880886e-07)
--(axis cs:26500,6.24671495204417e-07)
--(axis cs:26600,6.15967672639773e-07)
--(axis cs:26700,6.20228189855352e-07)
--(axis cs:26800,6.22344903600859e-07)
--(axis cs:26900,6.24896461230576e-07)
--(axis cs:27000,6.22154168692314e-07)
--(axis cs:27100,6.23391673505881e-07)
--(axis cs:27200,6.28321679936884e-07)
--(axis cs:27300,6.23109631903793e-07)
--(axis cs:27400,6.20127382330595e-07)
--(axis cs:27500,6.19483361916895e-07)
--(axis cs:27600,6.20820352091082e-07)
--(axis cs:27700,6.24596320926956e-07)
--(axis cs:27800,6.16587829768518e-07)
--(axis cs:27900,6.20374478223586e-07)
--(axis cs:28000,6.13044793506284e-07)
--(axis cs:28100,6.08137308263284e-07)
--(axis cs:28200,6.01015315178087e-07)
--(axis cs:28300,5.99848913815914e-07)
--(axis cs:28400,5.93979597285368e-07)
--(axis cs:28500,5.95352882744806e-07)
--(axis cs:28600,5.91386179061839e-07)
--(axis cs:28700,5.89659418042565e-07)
--(axis cs:28800,5.92259216720724e-07)
--(axis cs:28900,5.9142527519535e-07)
--(axis cs:29000,5.88848052361848e-07)
--(axis cs:29100,5.9146064865902e-07)
--(axis cs:29200,5.88905003916932e-07)
--(axis cs:29300,5.86003464254472e-07)
--(axis cs:29400,5.83239884529111e-07)
--(axis cs:29500,5.84348976688852e-07)
--(axis cs:29500,6.04817286134616e-07)
--(axis cs:29500,6.04817286134616e-07)
--(axis cs:29400,6.06831916694177e-07)
--(axis cs:29300,6.08622608950576e-07)
--(axis cs:29200,6.08594147892771e-07)
--(axis cs:29100,6.10892734064211e-07)
--(axis cs:29000,6.11591101704316e-07)
--(axis cs:28900,6.13002573993155e-07)
--(axis cs:28800,6.10038717142189e-07)
--(axis cs:28700,6.12776387638014e-07)
--(axis cs:28600,6.16021750782986e-07)
--(axis cs:28500,6.1942385654413e-07)
--(axis cs:28400,7.23076316525929e-07)
--(axis cs:28300,7.27595422798852e-07)
--(axis cs:28200,7.28486616775234e-07)
--(axis cs:28100,7.29521631559196e-07)
--(axis cs:28000,7.30585934002772e-07)
--(axis cs:27900,6.41570278231513e-07)
--(axis cs:27800,6.48708907305577e-07)
--(axis cs:27700,6.49687193928337e-07)
--(axis cs:27600,6.46208434272192e-07)
--(axis cs:27500,6.45249344438773e-07)
--(axis cs:27400,6.31955177376359e-07)
--(axis cs:27300,6.35182176977248e-07)
--(axis cs:27200,6.43874067093123e-07)
--(axis cs:27100,6.65985125719887e-07)
--(axis cs:27000,6.79161923702386e-07)
--(axis cs:26900,6.83013452593732e-07)
--(axis cs:26800,6.75496229332919e-07)
--(axis cs:26700,6.75009143117599e-07)
--(axis cs:26600,6.85815369493063e-07)
--(axis cs:26500,7.85026867696788e-07)
--(axis cs:26400,7.91631794742382e-07)
--(axis cs:26300,8.0508887419934e-07)
--(axis cs:26200,8.17877846423436e-07)
--(axis cs:26100,8.1797780127555e-07)
--(axis cs:26000,7.31848140179464e-07)
--(axis cs:25900,7.31437701770305e-07)
--(axis cs:25800,7.33557493816458e-07)
--(axis cs:25700,7.64702002316635e-07)
--(axis cs:25600,7.70694447053592e-07)
--(axis cs:25500,7.71535050650173e-07)
--(axis cs:25400,8.23948807472776e-07)
--(axis cs:25300,7.93918458119062e-07)
--(axis cs:25200,8.11048557913209e-07)
--(axis cs:25100,8.39118453204322e-07)
--(axis cs:25000,8.08155188278039e-07)
--(axis cs:24900,7.13491339553939e-07)
--(axis cs:24800,7.11837267096807e-07)
--(axis cs:24700,6.9660360156268e-07)
--(axis cs:24600,6.86504355099631e-07)
--(axis cs:24500,7.3037852157996e-07)
--(axis cs:24400,7.70758303951635e-07)
--(axis cs:24300,7.85027041281057e-07)
--(axis cs:24200,7.95592536722837e-07)
--(axis cs:24100,7.89154009313173e-07)
--(axis cs:24000,7.46513919846137e-07)
--(axis cs:23900,7.34411391871742e-07)
--(axis cs:23800,7.54587624604576e-07)
--(axis cs:23700,7.52295239801927e-07)
--(axis cs:23600,7.63116135664379e-07)
--(axis cs:23500,8.58524429434129e-07)
--(axis cs:23400,8.89725562320898e-07)
--(axis cs:23300,8.93245248079397e-07)
--(axis cs:23200,8.95799295326478e-07)
--(axis cs:23100,8.93264489976653e-07)
--(axis cs:23000,7.97213035305597e-07)
--(axis cs:22900,8.08748989933297e-07)
--(axis cs:22800,8.64801909196063e-07)
--(axis cs:22700,8.33509617194712e-07)
--(axis cs:22600,8.38634769428031e-07)
--(axis cs:22500,8.44508220757319e-07)
--(axis cs:22400,8.04007893398175e-07)
--(axis cs:22300,7.85920340656028e-07)
--(axis cs:22200,8.35344870662403e-07)
--(axis cs:22100,8.49547733697117e-07)
--(axis cs:22000,8.4213882925671e-07)
--(axis cs:21900,9.12248293295002e-07)
--(axis cs:21800,8.91068159061328e-07)
--(axis cs:21700,8.52026055921426e-07)
--(axis cs:21600,8.06350491504458e-07)
--(axis cs:21500,7.94084706803968e-07)
--(axis cs:21400,8.06027723978762e-07)
--(axis cs:21300,9.5940837869742e-07)
--(axis cs:21200,1.27884557046823e-06)
--(axis cs:21100,1.32145947558035e-06)
--(axis cs:21000,1.32329029774966e-06)
--(axis cs:20900,1.33757887618691e-06)
--(axis cs:20800,1.36910109382441e-06)
--(axis cs:20700,9.94992780888489e-07)
--(axis cs:20600,8.56827026977621e-07)
--(axis cs:20500,8.51859990060242e-07)
--(axis cs:20400,8.29981383522969e-07)
--(axis cs:20300,8.16271485473255e-07)
--(axis cs:20200,8.95950901171688e-07)
--(axis cs:20100,1.11340082172756e-06)
--(axis cs:20000,1.22762864625989e-06)
--(axis cs:19900,1.26209012506879e-06)
--(axis cs:19800,1.22826896122754e-06)
--(axis cs:19700,1.20833685890377e-06)
--(axis cs:19600,1.18178350616759e-06)
--(axis cs:19500,1.15354191135978e-06)
--(axis cs:19400,1.20144281457149e-06)
--(axis cs:19300,1.18292558797466e-06)
--(axis cs:19200,1.0383925419851e-06)
--(axis cs:19100,1.17335654307516e-06)
--(axis cs:19000,1.2887435683059e-06)
--(axis cs:18900,1.35071629286573e-06)
--(axis cs:18800,1.44844099463697e-06)
--(axis cs:18700,1.26830619774019e-06)
--(axis cs:18600,1.18690206083083e-06)
--(axis cs:18500,1.29423661197885e-06)
--(axis cs:18400,1.30971393949272e-06)
--(axis cs:18300,1.20511607005523e-06)
--(axis cs:18200,1.11533656084008e-06)
--(axis cs:18100,1.29413677230456e-06)
--(axis cs:18000,1.35165925090093e-06)
--(axis cs:17900,1.36617718405916e-06)
--(axis cs:17800,1.34864034575996e-06)
--(axis cs:17700,1.35723996557234e-06)
--(axis cs:17600,1.43770323734603e-06)
--(axis cs:17500,1.55538054013718e-06)
--(axis cs:17400,1.55626909712989e-06)
--(axis cs:17300,1.56394858490739e-06)
--(axis cs:17200,1.51858016803572e-06)
--(axis cs:17100,1.32958915387974e-06)
--(axis cs:17000,1.30602667572953e-06)
--(axis cs:16900,2.24305478442677e-06)
--(axis cs:16800,2.37747090344851e-06)
--(axis cs:16700,2.3776580765374e-06)
--(axis cs:16600,2.3646253406918e-06)
--(axis cs:16500,2.44682835113491e-06)
--(axis cs:16400,1.2424552769507e-06)
--(axis cs:16300,1.15628025004621e-06)
--(axis cs:16200,1.19635500314803e-06)
--(axis cs:16100,1.27878377569916e-06)
--(axis cs:16000,1.26760115057122e-06)
--(axis cs:15900,1.53713716751398e-06)
--(axis cs:15800,1.59668336061367e-06)
--(axis cs:15700,1.63672736350818e-06)
--(axis cs:15600,1.72335823158271e-06)
--(axis cs:15500,1.73973625442441e-06)
--(axis cs:15400,1.61406940952397e-06)
--(axis cs:15300,1.6218061242523e-06)
--(axis cs:15200,1.54932273592862e-06)
--(axis cs:15100,1.48078674750676e-06)
--(axis cs:15000,1.59082414247458e-06)
--(axis cs:14900,1.64440357938753e-06)
--(axis cs:14800,1.62011059604741e-06)
--(axis cs:14700,1.67634083244141e-06)
--(axis cs:14600,1.55026098435656e-06)
--(axis cs:14500,1.14816864411002e-06)
--(axis cs:14400,1.12840435337297e-06)
--(axis cs:14300,1.53728311769639e-06)
--(axis cs:14200,1.72322293041249e-06)
--(axis cs:14100,2.28017649995824e-06)
--(axis cs:14000,2.53679374194422e-06)
--(axis cs:13900,2.52459662705424e-06)
--(axis cs:13800,2.56923831275883e-06)
--(axis cs:13700,2.52727410355221e-06)
--(axis cs:13600,1.88625601612962e-06)
--(axis cs:13500,1.95303587414567e-06)
--(axis cs:13400,1.97262392983867e-06)
--(axis cs:13300,1.6412481683011e-06)
--(axis cs:13200,1.59421542409959e-06)
--(axis cs:13100,1.30874731574762e-06)
--(axis cs:13000,2.09197976732868e-06)
--(axis cs:12900,2.70297615149854e-06)
--(axis cs:12800,3.60540692639174e-06)
--(axis cs:12700,3.5994387404371e-06)
--(axis cs:12600,3.40509531609909e-06)
--(axis cs:12500,3.21752741790502e-06)
--(axis cs:12400,2.76462939019449e-06)
--(axis cs:12300,2.09152528879204e-06)
--(axis cs:12200,1.95107173444089e-06)
--(axis cs:12100,1.96377015419598e-06)
--(axis cs:12000,2.0341909133078e-06)
--(axis cs:11900,2.15171569181938e-06)
--(axis cs:11800,2.05000742179284e-06)
--(axis cs:11700,1.6992992254783e-06)
--(axis cs:11600,1.57668934735529e-06)
--(axis cs:11500,1.6047538071697e-06)
--(axis cs:11400,1.70819407397769e-06)
--(axis cs:11300,1.91465308297647e-06)
--(axis cs:11200,2.050361063513e-06)
--(axis cs:11100,2.05851969608262e-06)
--(axis cs:11000,1.95170602799391e-06)
--(axis cs:10900,4.07745529816812e-06)
--(axis cs:10800,4.47497509132286e-06)
--(axis cs:10700,4.50802397197936e-06)
--(axis cs:10600,4.34127663432216e-06)
--(axis cs:10500,4.67438764152061e-06)
--(axis cs:10400,4.31094545758301e-06)
--(axis cs:10300,4.34380228516305e-06)
--(axis cs:10200,4.22946611561073e-06)
--(axis cs:10100,3.97931162881879e-06)
--(axis cs:10000,2.56323804189403e-06)
--(axis cs:9900,2.6782195578902e-06)
--(axis cs:9800,3.18944271063067e-06)
--(axis cs:9700,3.06477712403172e-06)
--(axis cs:9600,2.88245841160453e-06)
--(axis cs:9500,3.11380442041162e-06)
--(axis cs:9400,2.96116873191853e-06)
--(axis cs:9300,3.195310141332e-06)
--(axis cs:9200,3.75575795506627e-06)
--(axis cs:9100,4.11603298651462e-06)
--(axis cs:9000,4.25423439739111e-06)
--(axis cs:8900,4.31851276216306e-06)
--(axis cs:8800,3.87195141374977e-06)
--(axis cs:8700,2.93184714556664e-06)
--(axis cs:8600,2.71982573311125e-06)
--(axis cs:8500,3.04193584910979e-06)
--(axis cs:8400,2.95234647908808e-06)
--(axis cs:8300,2.61671971953236e-06)
--(axis cs:8200,2.3312325917671e-06)
--(axis cs:8100,1.8842893124167e-06)
--(axis cs:8000,4.71714903507478e-06)
--(axis cs:7900,4.85269075063334e-06)
--(axis cs:7800,4.85133793897995e-06)
--(axis cs:7700,4.87280273737201e-06)
--(axis cs:7600,4.58362294424817e-06)
--(axis cs:7500,3.56574935213063e-06)
--(axis cs:7400,3.57389703189959e-06)
--(axis cs:7300,4.14065567342771e-06)
--(axis cs:7200,4.36689998065598e-06)
--(axis cs:7100,4.75496879790164e-06)
--(axis cs:7000,5.06589034022946e-06)
--(axis cs:6900,5.75781014705978e-06)
--(axis cs:6800,5.37227505333802e-06)
--(axis cs:6700,5.00199217995322e-06)
--(axis cs:6600,4.74586491374977e-06)
--(axis cs:6500,5.5039383098701e-06)
--(axis cs:6400,5.41773075300558e-06)
--(axis cs:6300,4.70672039135151e-06)
--(axis cs:6200,4.62987256414989e-06)
--(axis cs:6100,3.76013592089438e-06)
--(axis cs:6000,3.47458932435501e-06)
--(axis cs:5900,3.74045879329973e-06)
--(axis cs:5800,4.11534884573288e-06)
--(axis cs:5700,5.32758677353281e-06)
--(axis cs:5600,7.80671010835251e-06)
--(axis cs:5500,7.47421113006718e-06)
--(axis cs:5400,7.44840099976627e-06)
--(axis cs:5300,7.13161383116382e-06)
--(axis cs:5200,7.38178674422969e-06)
--(axis cs:5100,6.61684380573406e-06)
--(axis cs:5000,6.49056499088113e-06)
--(axis cs:4900,6.37542078945126e-06)
--(axis cs:4800,7.04862624812106e-06)
--(axis cs:4700,7.60686075560795e-06)
--(axis cs:4600,5.10633767822371e-06)
--(axis cs:4500,5.27298304573519e-06)
--(axis cs:4400,5.59832509676495e-06)
--(axis cs:4300,6.2558092465692e-06)
--(axis cs:4200,8.37733640109034e-06)
--(axis cs:4100,8.66518741444429e-06)
--(axis cs:4000,1.00811280591934e-05)
--(axis cs:3900,1.08441817591591e-05)
--(axis cs:3800,1.09638078085353e-05)
--(axis cs:3700,7.84404918072293e-06)
--(axis cs:3600,6.99824365680163e-06)
--(axis cs:3500,6.76591386999192e-06)
--(axis cs:3400,7.51909318752844e-06)
--(axis cs:3300,7.4413810108097e-06)
--(axis cs:3200,8.20191042445825e-06)
--(axis cs:3100,8.814398482308e-06)
--(axis cs:3000,9.51176756997951e-06)
--(axis cs:2900,1.03466451687419e-05)
--(axis cs:2800,1.07658964057158e-05)
--(axis cs:2700,1.10564136754868e-05)
--(axis cs:2600,1.1758444274314e-05)
--(axis cs:2500,1.20280649251961e-05)
--(axis cs:2400,1.16522659980114e-05)
--(axis cs:2300,1.1812078443946e-05)
--(axis cs:2200,1.17667810902141e-05)
--(axis cs:2100,1.25679719528822e-05)
--(axis cs:2000,1.29472639291694e-05)
--(axis cs:1900,1.47786087606976e-05)
--(axis cs:1800,1.88480951843402e-05)
--(axis cs:1700,2.56473911703232e-05)
--(axis cs:1600,2.92669402588489e-05)
--(axis cs:1500,3.31754268301802e-05)
--(axis cs:1400,3.61268503002799e-05)
--(axis cs:1300,3.89621663447182e-05)
--(axis cs:1200,3.89650742304832e-05)
--(axis cs:1100,4.0758197863592e-05)
--(axis cs:1000,4.3458086296048e-05)
--(axis cs:900,4.91640433909052e-05)
--(axis cs:800,5.05134214415614e-05)
--(axis cs:700,5.43925651324475e-05)
--(axis cs:600,0.000135188613841153)
--(axis cs:500,0.000283869671890263)
--(axis cs:400,0.000497289821387315)
--(axis cs:300,0.00147499705103882)
--(axis cs:200,0.00255209079266337)
--(axis cs:100,0.00356445703881679)
--(axis cs:0,0.00449837547693887)
--cycle;

% \addplot [semithick, red]
% table {%
% 0 0.00167266489006579
% 200 0.00103359902277589
% 300 0.000620833248831332
% 400 0.000280751177342609
% 500 0.000134557572891936
% 600 7.10286840330809e-05
% 700 3.31134397129063e-05
% 800 2.61691402556607e-05
% 900 2.28666413022438e-05
% 1000 2.16378048207844e-05
% 1100 2.1123189071659e-05
% 1200 1.96200580830919e-05
% 1300 1.70789426192641e-05
% 1400 1.63899876497453e-05
% 1500 1.58458096848335e-05
% 1600 1.59347364387941e-05
% 1700 1.69048980751541e-05
% 1900 1.60095478349831e-05
% 2000 1.62439064297359e-05
% 2100 1.55733941937797e-05
% 2200 1.42637099997955e-05
% 2300 1.44519171954016e-05
% 2400 1.47710597957484e-05
% 2500 1.41857444759808e-05
% 2700 1.38702598633245e-05
% 2800 1.42759936352377e-05
% 2900 1.43956021929625e-05
% 3000 1.48336966958595e-05
% 3100 1.37816832648241e-05
% 3200 1.36429025587859e-05
% 3400 1.32130526253604e-05
% 3500 1.27144376165234e-05
% 3600 1.27085759231704e-05
% 3700 1.33168668980943e-05
% 3800 1.25438300528913e-05
% 3900 1.25997748909867e-05
% 4000 1.27476641864632e-05
% 4100 1.30009348140447e-05
% 4200 1.24080152090755e-05
% 4300 1.24132611745154e-05
% 4400 1.21984503493877e-05
% 4500 1.18842990559642e-05
% 4600 1.17907984531485e-05
% 4700 1.13102332761628e-05
% 4800 1.11390536403633e-05
% 4900 1.14044923975598e-05
% 5000 1.11111794467433e-05
% 5100 1.07317755464464e-05
% 5200 1.12429788714508e-05
% 5300 1.13795640572789e-05
% 5400 1.03993434095173e-05
% 5500 1.10280589069589e-05
% 5600 1.06016850622837e-05
% 5700 1.00809493233101e-05
% 5800 9.50836874835659e-06
% 5900 9.57378961174982e-06
% 6000 8.70279291120823e-06
% 6100 8.84444398252526e-06
% 6300 9.29324323806213e-06
% 6400 9.3636581368628e-06
% 6500 9.37237018661108e-06
% 6600 9.63555430644192e-06
% 6700 9.48719934967812e-06
% 6800 9.70679411693709e-06
% 6900 9.60556644713506e-06
% 7000 9.45546162256505e-06
% 7100 9.48284650803544e-06
% 7200 9.09268328541657e-06
% 7300 8.89215516508557e-06
% 7400 8.5351284724311e-06
% 7500 8.37558400235139e-06
% 7600 7.71313352743164e-06
% 7700 8.05525542091345e-06
% 7800 7.71515806263778e-06
% 8000 7.65889762988081e-06
% 8100 8.42317967908457e-06
% 8200 8.50945252750535e-06
% 8300 8.45237173052737e-06
% 8400 8.45172235131031e-06
% 8500 8.36442814033944e-06
% 8600 7.63742536946665e-06
% 8700 7.05024376657093e-06
% 8800 6.87928059051046e-06
% 8900 6.87199553794926e-06
% 9000 7.01882436260348e-06
% 9100 6.94302798365243e-06
% 9200 7.0320452323358e-06
% 9300 7.17322291166056e-06
% 9400 7.15514670446282e-06
% 9500 6.96862025506562e-06
% 9600 6.65860625304049e-06
% 9700 6.4391542764497e-06
% 9800 6.43006887912634e-06
% 9900 6.11530958849471e-06
% 10000 5.98484439251479e-06
% 10100 6.51477648716536e-06
% 10200 6.65296465740539e-06
% 10300 6.66864434606396e-06
% 10400 6.72929490974639e-06
% 10500 6.94568916514982e-06
% 10600 6.96316692483379e-06
% 10700 6.88030786477611e-06
% 10800 6.66434789309278e-06
% 10900 6.56864494885667e-06
% 11000 6.19919819655479e-06
% 11100 5.7707006817509e-06
% 11200 5.59601721761283e-06
% 11300 5.66754624742316e-06
% 11400 5.84624740440631e-06
% 11500 6.1157929849287e-06
% 11600 6.23535697741318e-06
% 11700 6.19278944213875e-06
% 11900 5.93889262745506e-06
% 12000 5.53830932403798e-06
% 12100 5.30904162587831e-06
% 12200 5.40913833901868e-06
% 12300 5.26251460541971e-06
% 12400 5.04682429891545e-06
% 12600 5.08448920299998e-06
% 12700 5.02668353874469e-06
% 12800 5.04296349390643e-06
% 12900 5.20543926540995e-06
% 13000 5.29253020431497e-06
% 13100 5.25379118698766e-06
% 13200 5.24614779351396e-06
% 13300 5.16963609697996e-06
% 13400 5.14075236424105e-06
% 13600 4.9259888328379e-06
% 13700 4.72928650196991e-06
% 13800 4.60425007986487e-06
% 13900 4.40693747805199e-06
% 14000 4.31497983299778e-06
% 14100 4.36827349403757e-06
% 14200 4.29113515565405e-06
% 14300 4.43044336861931e-06
% 14400 4.51247342425631e-06
% 14500 4.67960217065411e-06
% 14600 4.630505827663e-06
% 14700 4.66435676571564e-06
% 14800 4.36932850789162e-06
% 14900 4.3056566028099e-06
% 15000 4.11602150052204e-06
% 15200 4.11602150052204e-06
% 15300 4.28865723733907e-06
% 15400 4.23178880737396e-06
% 15500 4.23276469518896e-06
% 15600 4.00154067392577e-06
% 15700 4.00102226194576e-06
% 15800 3.96946961700451e-06
% 15900 3.91055937143392e-06
% 16000 3.89786237064982e-06
% 16300 3.68603787137545e-06
% 16400 3.7061499824631e-06
% 16600 3.69426675206341e-06
% 16700 3.67267034562246e-06
% 16800 3.70976113117649e-06
% 16900 3.76888488062832e-06
% 17000 3.63257845492626e-06
% 17100 3.76912089450343e-06
% 17200 3.74884803022724e-06
% 17300 3.91098910768051e-06
% 17400 3.87716954719508e-06
% 17500 3.94832295569358e-06
% 17600 4.07165771321161e-06
% 17700 4.13181942349183e-06
% 17800 3.89046999771381e-06
% 17900 3.85542671210715e-06
% 18000 3.88006537832553e-06
% 18100 3.69721669812861e-06
% 18200 3.58913121090154e-06
% 18300 3.66828567166522e-06
% 18400 3.54043027073203e-06
% 18500 3.47760123986518e-06
% 18600 3.44141062669223e-06
% 18800 3.31286014443322e-06
% 18900 3.2910643312789e-06
% 19000 3.29630074702436e-06
% 19100 3.27770362673618e-06
% 19200 3.34922492584155e-06
% 19300 3.31218734572758e-06
% 19600 3.27589032167452e-06
% 19700 3.23679455505044e-06
% 19800 3.22239816341607e-06
% 19900 3.23048561767791e-06
% 20000 3.16665546051809e-06
% 20200 2.98580812341243e-06
% 20300 3.0086496281001e-06
% 20400 3.05374828712957e-06
% 20500 3.15867919198354e-06
% 20700 3.24748089042259e-06
% 20800 3.10872860609379e-06
% 20900 2.98933764497633e-06
% 21000 2.73682348961302e-06
% 21100 2.71917565441981e-06
% 21200 2.61929426415008e-06
% 21300 2.61252444033744e-06
% 21400 2.57193619290774e-06
% 21500 2.56530597653182e-06
% 21600 2.54327392212872e-06
% 21700 2.54895144280454e-06
% 21800 2.52258018917928e-06
% 21900 2.53451253229287e-06
% 22000 2.50111838795419e-06
% 22100 2.44679176830687e-06
% 22200 2.37532162827847e-06
% 22300 2.4218788894359e-06
% 22400 2.35041875384923e-06
% 22500 2.40897679759655e-06
% 22600 2.39960809267359e-06
% 22700 2.41140855905542e-06
% 22800 2.3661539216846e-06
% 22900 2.44768375523563e-06
% 23000 2.43011481870781e-06
% 23100 2.38187658396782e-06
% 23200 2.38505367633479e-06
% 23400 2.19522144107032e-06
% 23500 2.13854855246609e-06
% 23600 2.13003295357339e-06
% 23700 2.11189444598858e-06
% 23800 2.13112070923671e-06
% 23900 2.17888077713724e-06
% 24000 2.24427276407368e-06
% 24100 2.24796963266272e-06
% 24200 2.30861655836634e-06
% 24300 2.30212663154816e-06
% 24500 2.16657599594328e-06
% 24600 2.13294424611377e-06
% 24700 2.04090611077845e-06
% 24800 2.11241399483697e-06
% 25000 2.07304128707619e-06
% 25100 2.11884594136791e-06
% 25200 2.08392680178804e-06
% 25300 2.02102887669753e-06
% 25500 2.03268109544297e-06
% 25600 1.966930085473e-06
% 25700 1.94387644114613e-06
% 25800 1.89981290077412e-06
% 26000 1.84175598860747e-06
% 26100 1.84828502369783e-06
% 26300 1.80794597781642e-06
% 26500 1.78874995526712e-06
% 26600 1.74684453213558e-06
% 26700 1.76437197296764e-06
% 27100 1.69596114574233e-06
% 27200 1.6599869923084e-06
% 27300 1.68688734447642e-06
% 27400 1.67767041148181e-06
% 27600 1.71463943843264e-06
% 27700 1.7089371340262e-06
% 27800 1.68390431554144e-06
% 27900 1.6873800632311e-06
% 28100 1.64004825364827e-06
% 28200 1.66496465681121e-06
% 28300 1.62313199325581e-06
% 28500 1.60938088811236e-06
% 28600 1.58792329330026e-06
% 28700 1.55627969888883e-06
% 28800 1.54388123974059e-06
% 28900 1.50752032368473e-06
% 29000 1.48307651670621e-06
% 29200 1.48841900227126e-06
% 29300 1.48350318340817e-06
% 29400 1.48666163113376e-06
% 29500 1.50280880006903e-06
% };\addlegendentry{nosi}
\addplot [ultra thick, red]
table {%
0 0.00793405342847109
100 0.00659654662013054
200 0.00508389482274652
300 0.00342376297339797
400 0.00182917073834687
500 0.00101173517759889
600 0.000637519755400717
700 0.000427102640969679
800 0.00036658052704297
900 0.000332209019688889
1000 0.000307628040900454
1100 0.000281147571513429
1200 0.000265089067397639
1400 0.000238726614043117
1500 0.000233736995141953
1700 0.000231615340453573
1900 0.000227314420044422
2000 0.000221258102101274
2100 0.000210850135772489
2200 0.000204190248041414
2300 0.000202144496142864
2400 0.000201189948711544
2500 0.000199273665202782
2600 0.00020576428505592
2700 0.000205204531084746
2800 0.00020130374468863
2900 0.00020063306146767
3000 0.00019834291015286
3100 0.00018788491433952
3300 0.00018049510254059
3400 0.000179234571987763
3500 0.000181931027327664
3600 0.000181396273546852
3700 0.00017959535762202
3800 0.000179362235940062
3900 0.000176450164872222
4000 0.000176762463524938
4100 0.000178749149199575
4200 0.000177824331331067
4400 0.000173895081388764
4500 0.000165694698807783
4600 0.000163775039254688
4800 0.000155528119648807
4900 0.00015576378791593
5000 0.000154546869453043
5100 0.000149956016684882
5200 0.000152601554873399
5300 0.0001536166673759
5400 0.000146753765875474
5500 0.000147121274494566
5600 0.000145179888932034
5700 0.000139716037665494
5800 0.000136467526317574
5900 0.000135597219923511
6000 0.000133604582515545
6100 0.00013084830425214
6200 0.000129231149912812
6300 0.00012983416672796
6400 0.000136511953314766
6500 0.00013915533781983
6600 0.000140681659104303
6800 0.000137996335979551
6900 0.000128596482682042
7000 0.000120703109132592
7100 0.000119993594125845
7200 0.000118506948638242
7300 0.000116378352686297
7500 0.000115315262519289
7600 0.000111335757537745
7700 0.000113365967990831
7800 0.000113493122626096
8000 0.000111313333036378
8100 0.000116250383143779
8300 0.000113271344162058
8500 0.000109320419142023
8600 0.000103790160210337
8700 0.000101606339740101
8800 0.000100322220532689
9000 0.000101782818092033
9100 0.000101495286799036
9300 0.000100200028100517
9400 9.98047544271685e-05
9500 9.86917439149693e-05
9600 9.69652537605725e-05
9900 9.59583630901761e-05
10000 9.66098887147382e-05
10100 9.94038346107118e-05
10200 9.90952248685062e-05
10300 9.96846138150431e-05
10400 9.81642515398562e-05
10500 9.9622251582332e-05
10700 9.95557711576112e-05
10800 9.78181342361495e-05
10900 9.77704621618614e-05
11000 9.52391565078869e-05
11100 9.18297955649905e-05
11200 9.20317688724026e-05
11300 9.31809190660715e-05
11400 9.50827525230125e-05
11500 9.57913071033545e-05
11700 9.51602414716035e-05
12000 9.10594098968431e-05
12500 8.87197820702568e-05
12600 8.9238936197944e-05
12800 8.91438467078842e-05
12900 8.77901256899349e-05
13000 8.78737409948371e-05
13200 8.91607778612524e-05
13300 8.88558715814725e-05
13400 8.98008511285298e-05
13500 9.12036921363324e-05
13600 8.97182617336512e-05
13700 8.78601349540986e-05
14000 8.5560699517373e-05
14100 8.57870254549198e-05
14200 8.53119272505865e-05
14400 8.55911421240307e-05
14500 8.38519044918939e-05
14700 8.43777670525014e-05
14800 8.23796872282401e-05
15000 8.08659824542701e-05
15100 8.06691168691032e-05
15200 8.00053603597917e-05
15500 8.30692442832515e-05
15600 8.20611021481454e-05
15800 8.24307135189883e-05
16000 8.1273028627038e-05
16100 8.0574223829899e-05
16200 8.08096228865907e-05
16500 7.89683108450845e-05
16600 7.9091259976849e-05
16700 7.81030976213515e-05
16900 7.74104628362693e-05
17100 7.77891837060452e-05
17200 7.76119049987756e-05
17300 7.8911536547821e-05
17400 7.91970160207711e-05
17700 7.8248413046822e-05
17800 7.60167749831453e-05
17900 7.4651870818343e-05
18100 7.52232881495729e-05
18300 7.55993605707772e-05
18400 7.61885676183738e-05
18500 7.57144880481064e-05
18600 7.45309007470496e-05
18700 7.46340010664426e-05
18800 7.51497354940511e-05
18900 7.46763762435876e-05
19100 7.61223491281271e-05
19300 7.59642935008742e-05
19500 7.54480279283598e-05
19600 7.46482619433664e-05
19700 7.50154431443661e-05
20000 7.40940595278516e-05
20100 7.45435900171287e-05
20200 7.43233395041898e-05
20300 7.4767776823137e-05
20400 7.62084819143638e-05
20500 7.63319985708222e-05
20800 7.4239338573534e-05
20900 7.31123582227156e-05
21000 7.25473364582285e-05
21600 7.15240530553274e-05
21800 7.20129974070005e-05
21900 7.27218284737319e-05
22000 7.2204515163321e-05
22100 7.2547969466541e-05
22200 7.18335068086162e-05
22300 7.22650293027982e-05
22400 7.16924623702653e-05
22500 7.16568174539134e-05
22600 7.02793913660571e-05
22800 6.92642206558958e-05
23000 6.85819395584986e-05
23100 6.90122687956318e-05
23200 7.01872413628735e-05
23300 6.9899542722851e-05
23400 7.02636534697376e-05
23600 7.15884016244672e-05
23700 7.07542349118739e-05
23900 7.05920538166538e-05
24100 6.97711802786216e-05
24200 6.99813244864345e-05
24500 6.96653150953352e-05
24700 6.85198465362191e-05
24800 6.84973565512337e-05
25000 6.7615786974784e-05
25100 6.80000957800075e-05
25200 6.77799762343056e-05
25500 6.83770558680408e-05
25600 6.77743228152394e-05
25700 6.81109086144716e-05
25800 6.78088545100763e-05
25900 6.79001241223887e-05
26000 6.74397670081817e-05
26100 6.7610882979352e-05
26200 6.71639936626889e-05
26300 6.73351460136473e-05
26400 6.71810339554213e-05
26500 6.7537504946813e-05
26600 6.74163020448759e-05
26700 6.78006690577604e-05
26800 6.7653731093742e-05
26900 6.78499709465541e-05
27100 6.69546716380864e-05
27200 6.65581392240711e-05
27400 6.65581392240711e-05
27600 6.70865338179283e-05
27700 6.7146225774195e-05
27900 6.66992564219981e-05
29000 6.72886599204503e-05
29200 6.70099761919118e-05
29400 6.71762390993536e-05
29500 6.69583459966816e-05
}; \addlegendentry{Baseline}

\addplot [ultra thick, blue]
table {%
0 0.00713266292586923
100 0.00585381686687469
200 0.00446937792003155
300 0.00292959995567799
400 0.0014729923568666
500 0.00082353682955727
600 0.000527653901372105
700 0.000327464804286137
800 0.000287563510937616
900 0.000269933487288654
1100 0.00022187405556906
1200 0.000210411322768778
1300 0.000202334675122984
1400 0.000193461324670352
1600 0.000182937350473367
1700 0.000176460918737575
1800 0.000168806567671709
1900 0.000163733959197998
2000 0.000161307994858362
2100 0.000155167377670296
2200 0.000150609761476517
2300 0.000143839264637791
2400 0.000142801553010941
2500 0.000136389033286832
2600 0.000140332078444771
2800 0.000143211844260804
2900 0.000138361123390496
3000 0.000137580442242324
3100 0.000133536392240785
3200 0.000128499304992147
3300 0.000121743527415674
3400 0.000117199655505829
3500 0.000113784022687469
3700 0.00010468480468262
3800 0.000104768165329006
3900 0.000103354395832866
4000 0.000103076519735623
4100 0.000100669960374944
4200 0.000101901678135619
4300 9.98369796434417e-05
4400 0.000101587378594559
4500 0.000100801189546473
4600 0.000101453173556365
4700 9.65851795626804e-05
4800 9.36303113121539e-05
4900 8.92090538400225e-05
5100 8.40944776427932e-05
5200 8.35357059258968e-05
5300 8.17916079540737e-05
5400 7.83899522502907e-05
5500 7.70212427596562e-05
5600 7.60818220442161e-05
5700 7.38685703254305e-05
5900 7.34010318410583e-05
6000 7.15118876541965e-05
6100 6.79179429425858e-05
6200 6.79472577758133e-05
6300 6.75207484164275e-05
6400 7.05915153957903e-05
6500 7.13030240149237e-05
6600 7.30591564206406e-05
6700 7.30759202269837e-05
6800 7.37523587304167e-05
6900 7.03525802236982e-05
7000 6.82377067278139e-05
7100 6.9061316025909e-05
7200 6.72817914164625e-05
7300 6.64671460981481e-05
7400 6.61660669720732e-05
7500 6.51553491479717e-05
7600 6.27879562671296e-05
7700 6.46648768451996e-05
7900 6.3234954723157e-05
8000 6.46249172859825e-05
8100 6.47248307359405e-05
8200 6.24350213911384e-05
8300 6.36571712675504e-05
8400 6.27443369012326e-05
8500 6.02698819420766e-05
8600 5.99148515902925e-05
8700 5.86965252296068e-05
8800 5.62677923880983e-05
8900 5.61629894946236e-05
9000 5.70373449590988e-05
9100 5.59424152015708e-05
9200 5.61162669328041e-05
9300 5.78313920414075e-05
9400 5.75635494897142e-05
9500 5.68996110814624e-05
9700 5.90866839047521e-05
9800 5.83280852879398e-05
9900 5.81168751523364e-05
10000 5.88515940762591e-05
10100 5.93128133914433e-05
10300 5.59066793357488e-05
10400 5.5451240768889e-05
10500 5.65238333365414e-05
10600 5.86967180424836e-05
10700 5.8324949350208e-05
10800 5.75684789509978e-05
10900 5.63816429348662e-05
11000 5.41459885425866e-05
11100 5.03419505548663e-05
11300 5.2260951633798e-05
11400 5.36256411578506e-05
11500 5.46011360711418e-05
11600 5.40880537300836e-05
11700 5.47399176866747e-05
11800 5.50387158000376e-05
11900 5.41352892469149e-05
12000 5.23164126207121e-05
12200 5.03150404256303e-05
12300 4.93922525492962e-05
12400 4.94614978379104e-05
12500 5.0262751756236e-05
12600 4.99896632391028e-05
12700 5.05691932630725e-05
12800 5.07604418089613e-05
12900 5.02477996633388e-05
13000 5.01809772686101e-05
13100 5.24027600476984e-05
13300 4.96385837323032e-05
13400 4.97410983371083e-05
13500 4.88508740090765e-05
13600 4.70303348265588e-05
13800 4.69724327558652e-05
13900 4.78893271065317e-05
14000 4.81093520647846e-05
14200 4.6702192776138e-05
14300 4.6875728003215e-05
14400 4.61683448520489e-05
14500 4.67048594146036e-05
14600 4.81821443827357e-05
14700 4.92927865707316e-05
14900 4.90562488266733e-05
15000 4.79381451441441e-05
15100 4.81413226225413e-05
15200 4.73553227493539e-05
15300 4.75259075756185e-05
15400 4.70261002192274e-05
15500 4.69433034595568e-05
15600 4.56275229225866e-05
15700 4.55227418569848e-05
15800 4.47544261987787e-05
15900 4.42764212493785e-05
16200 4.3533156713238e-05
16400 4.36597656516824e-05
16500 4.33954810432624e-05
16600 4.29146493843291e-05
16700 4.34193098044489e-05
17000 4.38951428805012e-05
17100 4.37237140431534e-05
17200 4.26077385782264e-05
17300 4.20713295170572e-05
17400 4.20982687501237e-05
17500 4.08218584198039e-05
17600 4.09180211136118e-05
17700 4.06854742323048e-05
17900 3.9161754102679e-05
18000 3.96513096347917e-05
18200 4.01135876018088e-05
18300 4.15428185078781e-05
18400 4.2803687392734e-05
18500 4.30402615165804e-05
18600 4.26249098381959e-05
18700 4.25858961534686e-05
18800 4.20144133386202e-05
18900 4.10349057347048e-05
19000 4.13831185142044e-05
19300 4.15166432503611e-05
19500 3.93558948417194e-05
19800 3.83021651941817e-05
19900 3.89490196539555e-05
20100 3.90845634683501e-05
20300 3.88494627259206e-05
20400 3.93964910472278e-05
20600 3.9814203773858e-05
20700 3.94081725971773e-05
20800 3.92244946851861e-05
20900 3.80382225557696e-05
21000 3.78359545720741e-05
21100 3.70987945643719e-05
21200 3.78224976884667e-05
21300 3.71685928257648e-05
21400 3.70818925148342e-05
21500 3.77999567717779e-05
21700 3.73282164218836e-05
21800 3.74825940525625e-05
21900 3.79965640604496e-05
22000 3.68943074136041e-05
22100 3.7449808587553e-05
22200 3.66390631825197e-05
22300 3.70585694327019e-05
22400 3.67401335097384e-05
22500 3.68441542377695e-05
22600 3.60963385901414e-05
22700 3.60579178959597e-05
22800 3.52325550920796e-05
23000 3.46945889759809e-05
23200 3.49556285073049e-05
23300 3.55480333382729e-05
23400 3.5411496355664e-05
23500 3.55643896909896e-05
23600 3.58897741534747e-05
23700 3.57618955604266e-05
23800 3.51045127899852e-05
23900 3.53362265741453e-05
24000 3.53531831933651e-05
24200 3.44903273798991e-05
24300 3.43762658303604e-05
24400 3.40828955813777e-05
24600 3.42208113579545e-05
24700 3.39165526384022e-05
24900 3.41634877258912e-05
25100 3.36667471856344e-05
25300 3.38954087055754e-05
25500 3.32139716192614e-05
25600 3.33744137606118e-05
25700 3.3934320526896e-05
25800 3.37239434884395e-05
26100 3.40835322276689e-05
26200 3.39424805133604e-05
26300 3.40659134963062e-05
26400 3.36005359713454e-05
26500 3.3424912544433e-05
26800 3.21380866807885e-05
26900 3.23985586874187e-05
27000 3.23399908666033e-05
27100 3.25949076795951e-05
27200 3.23804924846627e-05
27600 3.26549779856578e-05
27700 3.29856702592224e-05
27800 3.30467883031815e-05
27900 3.27835150528699e-05
28000 3.29126669385005e-05
28100 3.27461384586059e-05
28200 3.2783154892968e-05
28300 3.29677131958306e-05
28400 3.28444402839523e-05
28500 3.25536348100286e-05
28600 3.26680310536176e-05
28800 3.21993284160271e-05
28900 3.24784814438317e-05
29000 3.25794135278556e-05
29100 3.24669999827165e-05
29200 3.27094858221244e-05
29300 3.27804191329051e-05
29500 3.24254979204852e-05
}; \addlegendentry{K1}

\addplot [ultra thick,  green!50.1960784313725!black]
table {%
0 0.00447891326621175
100 0.00354398507624865
200 0.00251091783866286
300 0.00143611629027873
400 0.000459330069134012
500 0.000250420678639784
600 0.000102144644188229
700 5.03781120642088e-05
800 4.64967160951346e-05
900 4.53427128377371e-05
1000 4.19682619394735e-05
1100 3.91753019357566e-05
1200 3.7283607525751e-05
1300 3.60539597750176e-05
1500 3.0786879506195e-05
1600 2.66455299424706e-05
1700 2.26965530600864e-05
1800 1.76552875927882e-05
1900 1.40382080644486e-05
2000 1.16400196930044e-05
2100 1.03202901300392e-05
2200 1.0029842997028e-05
2300 1.05412818811601e-05
2400 1.05501167126931e-05
2500 1.03310485428665e-05
2700 9.73520582192577e-06
2800 9.20617821975611e-06
2900 8.4853718362865e-06
3000 7.68811605666997e-06
3100 7.5762723099615e-06
3200 7.14933548806584e-06
3300 6.41144333712873e-06
3400 6.29915166427963e-06
3500 6.09540029472555e-06
3600 6.30173917670618e-06
3700 6.25132179266075e-06
3800 8.25437382445671e-06
3900 9.07121466298122e-06
4000 8.81758569448721e-06
4200 7.49893388274359e-06
4300 5.57741896045627e-06
4400 4.46361082140356e-06
4500 4.33603327110177e-06
4600 4.04471848014509e-06
4700 5.36079232915654e-06
4800 5.62056129638222e-06
4900 5.73594525121734e-06
5100 5.78173603571486e-06
5200 5.60303806196316e-06
5300 5.25016412211698e-06
5400 5.3493095037993e-06
5500 5.22821301274234e-06
5600 5.37747519047116e-06
5700 4.11785231335671e-06
5800 3.98970405512955e-06
5900 3.30467537423829e-06
6000 3.07155346490617e-06
6100 2.89877152681584e-06
6200 3.29392014464247e-06
6300 3.3857470498333e-06
6400 4.00922772314516e-06
6500 4.56091402156744e-06
6600 4.56658153780154e-06
6700 4.28388057116535e-06
6800 4.12724421039457e-06
6900 4.30844193033408e-06
7000 3.87435693482985e-06
7100 3.60463582183002e-06
7300 2.88870614895131e-06
7400 2.60791034634167e-06
7500 2.50306334237393e-06
7600 4.15698286815314e-06
7700 4.31688022217713e-06
7800 4.09502490583691e-06
7900 3.450627446e-06
8000 3.25563132719253e-06
8100 1.75966499682545e-06
8200 2.02577871277754e-06
8300 2.20209904000512e-06
8400 2.46560193772893e-06
8500 2.59555577031279e-06
8700 2.51154233410489e-06
8800 2.88936280412599e-06
8900 3.13412397190405e-06
9100 3.13743612423423e-06
9200 2.75282013717515e-06
9300 2.19756066144328e-06
9400 2.17271258406981e-06
9500 2.1902762910031e-06
9600 1.94413678400451e-06
9700 2.10592065741366e-06
9800 2.26256406676839e-06
9900 1.90611444850219e-06
10000 1.76390904016444e-06
10100 2.73787236437784e-06
10200 2.65942367150274e-06
10300 2.5668894068076e-06
10400 2.63712172454689e-06
10500 3.91759431295213e-06
10600 3.2282589472743e-06
10700 3.17747640110611e-06
10800 3.19718583341455e-06
10900 3.12662427859323e-06
11000 1.84542375336605e-06
11100 1.570014887875e-06
11200 1.53512041833892e-06
11400 1.44469674978609e-06
11500 1.46278557622281e-06
11600 1.50869436765788e-06
11700 1.65161873155739e-06
11800 1.71932981629652e-06
11900 1.7172300204038e-06
12000 1.65933465723356e-06
12100 1.66244933552662e-06
12200 1.62084893418069e-06
12300 1.59129695020965e-06
12400 2.1272282992868e-06
12500 2.53299617725133e-06
12600 2.77263393400062e-06
12700 2.69889619630703e-06
12800 2.56587782132556e-06
12900 1.9360888927622e-06
13100 1.26385691601172e-06
13200 1.31161516492284e-06
13300 1.3857717249266e-06
13400 1.57666045197402e-06
13500 1.56359999436972e-06
13600 1.59792557496985e-06
13700 1.80738834387739e-06
13800 1.85061207957915e-06
13900 1.85838200650323e-06
14000 1.85608189440245e-06
14100 1.72832767475484e-06
14200 1.32857599055569e-06
14300 1.21635707728274e-06
14400 1.01252862805268e-06
14500 9.83065206128231e-07
14600 1.14930628569709e-06
14700 1.21309210499021e-06
14800 1.26332417949016e-06
14900 1.35159325509449e-06
15000 1.3788796877634e-06
15100 1.3005217169848e-06
15200 1.30857722524524e-06
15300 1.38937775773229e-06
15400 1.37384745357849e-06
15500 1.44417174396949e-06
15600 1.43940530961117e-06
15700 1.4072838894208e-06
15800 1.24433915971167e-06
15900 1.20497463740321e-06
16000 1.09743075427104e-06
16100 1.10079531623342e-06
16300 1.08708968582505e-06
16400 1.190668513118e-06
16500 1.76977141563839e-06
16600 1.75867216967163e-06
16700 1.76938669937954e-06
16800 1.77195488504367e-06
16900 1.71000135651411e-06
17000 1.11414260572928e-06
17100 1.09903453449078e-06
17200 1.13435385173943e-06
17300 1.14281203877908e-06
17400 1.12223460746463e-06
17500 1.13834130388568e-06
17600 1.20279901238973e-06
17700 1.3068757880319e-06
17800 1.30398336750659e-06
17900 1.24734708606411e-06
18000 1.22775657018792e-06
18100 1.13781777599797e-06
18200 9.50703281432652e-07
18300 9.83890231509577e-07
18400 1.08723293124058e-06
18500 1.10606413272762e-06
18600 1.13358066755609e-06
18700 1.21238235806231e-06
18800 1.20750428322935e-06
18900 1.08350297978177e-06
19000 1.08498034023796e-06
19100 1.04352011476294e-06
19200 9.53900666900154e-07
19300 1.02903061360848e-06
19400 1.04080356777558e-06
19500 1.016202872961e-06
19600 1.06144034361932e-06
19700 1.17150511869113e-06
19800 1.05842616449081e-06
19900 1.05627384527907e-06
20000 1.02929277545627e-06
20100 9.37730078476307e-07
20200 8.20702950932173e-07
20300 7.79832191710739e-07
20400 7.85733220709517e-07
20500 8.18589001028158e-07
20600 8.4176605241737e-07
20700 9.28277017919754e-07
20800 1.15472619199863e-06
20900 1.19173705570574e-06
21000 1.17565423352062e-06
21100 1.15370608000376e-06
21200 1.06534821497917e-06
21300 8.2573382087503e-07
21400 7.51277866584132e-07
21500 7.72189537201484e-07
21600 7.79487209001672e-07
21700 7.95009839293925e-07
21800 8.38926098367665e-07
21900 8.60374655076157e-07
22000 8.36168226214795e-07
22100 8.29618727493653e-07
22200 8.04954368049948e-07
22300 7.62363470130367e-07
22400 7.80434334046731e-07
22600 7.69595317251515e-07
22700 7.76942670199787e-07
22800 7.99775193627283e-07
22900 7.76633044097252e-07
23000 7.72814644278697e-07
23100 8.18813759906334e-07
23200 8.19569265786413e-07
23300 7.98829148607183e-07
23500 7.87050794315292e-07
23600 7.32529713332042e-07
23700 7.2076835522239e-07
23800 7.16438364634087e-07
23900 7.05537786416244e-07
24000 7.11066320491227e-07
24100 7.20679736332386e-07
24200 7.23428343007981e-07
24400 7.14076918484352e-07
24500 7.00708937984018e-07
24600 6.83764540099219e-07
24800 7.02275542607822e-07
24900 7.01128385571792e-07
25000 7.33528509044845e-07
25100 7.45670831747702e-07
25200 7.34564991944353e-07
25300 7.31958095911978e-07
25400 7.51252343889064e-07
25500 7.08433162799338e-07
25600 6.99627321409935e-07
25800 6.87173894675652e-07
26000 6.98758299222391e-07
26100 7.46558043829282e-07
26200 7.50418053030444e-07
26300 7.46460500522517e-07
26400 7.09618007022073e-07
26500 7.04849469457258e-07
26600 6.50891365694406e-07
26700 6.47618662696914e-07
26800 6.48920490675664e-07
26900 6.53955112284166e-07
27100 6.44688611828315e-07
27300 6.29145858965785e-07
27400 6.26041639861796e-07
27500 6.32366209174506e-07
27700 6.37141567949584e-07
27900 6.30972181170364e-07
28000 6.71815485020488e-07
28400 6.5852754005391e-07
28500 6.07388187745528e-07
28700 6.01217720941349e-07
29200 5.98749352320738e-07
29500 5.94582843405078e-07
}; \addlegendentry{K2}

==> supp_mat/reacher_plots/traj_err_data.tex <==
\path [fill=red, fill opacity=0.4, ultra thick]
(axis cs:1,0.321317324899372)
--(axis cs:1,0.154270957373277)
--(axis cs:2,0.0849194177170999)
--(axis cs:5,0.0480576647863629)
--(axis cs:10,0.0409580701297988)
--(axis cs:15,0.0377832687809504)
--(axis cs:25,0.0386983208442786)
--(axis cs:50,0.0325164114609333)
--(axis cs:50,0.069386282212959)
--(axis cs:50,0.069386282212959)
--(axis cs:25,0.106018718582589)
--(axis cs:15,0.0704285062923213)
--(axis cs:10,0.0723070156297636)
--(axis cs:5,0.301779308324021)
--(axis cs:2,0.19897611581381)
--(axis cs:1,0.321317324899372)
--cycle;

\path [fill=blue, fill opacity=0.4, ultra thick]
(axis cs:1,0.302775857204024)
--(axis cs:1,0.103822736962633)
--(axis cs:2,0.0828076115162474)
--(axis cs:5,0.0381229520179212)
--(axis cs:10,0.0304438363374599)
--(axis cs:15,0.0287823142787306)
--(axis cs:25,0.0217575984727216)
--(axis cs:50,0.00758026968939714)
--(axis cs:50,0.0199793722874369)
--(axis cs:50,0.0199793722874369)
--(axis cs:25,0.0927208561785352)
--(axis cs:15,0.0612113714019699)
--(axis cs:10,0.0660780928106958)
--(axis cs:5,0.127245395091526)
--(axis cs:2,0.253844151062908)
--(axis cs:1,0.302775857204024)
--cycle;

\path [fill=green!50.1960784313725!black, fill opacity=0.4, ultra thick]
(axis cs:1,0.109159357055561)
--(axis cs:1,0.0352173188407961)
--(axis cs:2,0.0230413231588501)
--(axis cs:5,0.00408155118403199)
--(axis cs:10,0.00418598635894365)
--(axis cs:15,0.00292412662244513)
--(axis cs:25,0.00205979541594006)
--(axis cs:50,0.00211097925347557)
--(axis cs:50,0.00372017678820147)
--(axis cs:50,0.00372017678820147)
--(axis cs:25,0.00529417726546357)
--(axis cs:15,0.00918405285446757)
--(axis cs:10,0.00746139809075942)
--(axis cs:5,0.0118184691689693)
--(axis cs:2,0.0495833337870229)
--(axis cs:1,0.109159357055561)
--cycle;

\addplot [ultra thick, red, mark=*, mark size=1.5, mark options={solid}]
table {%
1 0.237794145941734
2 0.141947731375694
5 0.174918502569199
10 0.0566325411200523
15 0.0541058890521526
25 0.0723585188388824
50 0.0509513504803181
};
\addplot [ultra thick, blue, mark=*, mark size=1.5, mark options={solid}]
table {%
1 0.203299298882484
2 0.168325915932655
5 0.0826841816306114
10 0.0482609681785107
15 0.0449968427419662
25 0.0572392269968987
50 0.013779821805656
};
\addplot [ultra thick, green!50.1960784313725!black, mark=*, mark size=1.5, mark options={solid}]
table {%
1 0.0721883475780487
2 0.0363123267889023
5 0.00795001070946455
10 0.00582369277253747
15 0.00605409080162644
25 0.00367698539048433
50 0.00291557726450264
};


==> supp_mat/ur5e_plots/relerr_data.tex <==
\path [fill=red, fill opacity=0.4, ultra thick]
(axis cs:0.00249999994412065,0.0689658270143467)
--(axis cs:0.00249999994412065,0.0531844783785417)
--(axis cs:0.00499999988824129,0.121054991611039)
--(axis cs:0.00749999983236194,0.155841647124411)
--(axis cs:0.00999999977648258,0.172703943711814)
--(axis cs:0.0124999997206032,0.178783057636422)
--(axis cs:0.0149999996647239,0.177486678264227)
--(axis cs:0.0174999996088445,0.17083760919769)
--(axis cs:0.0199999995529652,0.161057367041059)
--(axis cs:0.0224999994970858,0.152197561112275)
--(axis cs:0.0249999994412065,0.144804222324234)
--(axis cs:0.0274999993853271,0.139459077829965)
--(axis cs:0.0299999993294477,0.13583599336393)
--(axis cs:0.0324999992735684,0.133164537800093)
--(axis cs:0.034999999217689,0.131114131822622)
--(axis cs:0.0374999991618097,0.129275945723534)
--(axis cs:0.0399999991059303,0.12738670854117)
--(axis cs:0.042499999050051,0.125778200673116)
--(axis cs:0.0449999989941716,0.123990100061176)
--(axis cs:0.0474999989382923,0.122246150710438)
--(axis cs:0.0474999989382923,0.199646389379003)
--(axis cs:0.0474999989382923,0.199646389379003)
--(axis cs:0.0449999989941716,0.200053703773677)
--(axis cs:0.042499999050051,0.199554924583593)
--(axis cs:0.0399999991059303,0.198168396253103)
--(axis cs:0.0374999991618097,0.196248734925689)
--(axis cs:0.034999999217689,0.193641740875607)
--(axis cs:0.0324999992735684,0.19053577357241)
--(axis cs:0.0299999993294477,0.187199321883119)
--(axis cs:0.0274999993853271,0.183927610912632)
--(axis cs:0.0249999994412065,0.181258996344638)
--(axis cs:0.0224999994970858,0.179796104601694)
--(axis cs:0.0199999995529652,0.180095394566163)
--(axis cs:0.0174999996088445,0.183503645726392)
--(axis cs:0.0149999996647239,0.18851445621452)
--(axis cs:0.0124999997206032,0.190844855725787)
--(axis cs:0.00999999977648258,0.186267640070446)
--(axis cs:0.00749999983236194,0.171175461000425)
--(axis cs:0.00499999988824129,0.138424700253303)
--(axis cs:0.00249999994412065,0.0689658270143467)
--cycle;

\path [fill=blue, fill opacity=0.4, ultra thick]
(axis cs:0.00249999994412065,0.0726684754483229)
--(axis cs:0.00249999994412065,0.0629908674400216)
--(axis cs:0.00499999988824129,0.130448017158423)
--(axis cs:0.00749999983236194,0.161931135940525)
--(axis cs:0.00999999977648258,0.17535600350848)
--(axis cs:0.0124999997206032,0.177927099875836)
--(axis cs:0.0149999996647239,0.172931752225648)
--(axis cs:0.0174999996088445,0.16325949220645)
--(axis cs:0.0199999995529652,0.151936152179457)
--(axis cs:0.0224999994970858,0.143145878421694)
--(axis cs:0.0249999994412065,0.136098680540765)
--(axis cs:0.0274999993853271,0.131196805360052)
--(axis cs:0.0299999993294477,0.128047998382747)
--(axis cs:0.0324999992735684,0.125937898407024)
--(axis cs:0.034999999217689,0.124609995601403)
--(axis cs:0.0374999991618097,0.123723705501436)
--(axis cs:0.0399999991059303,0.123039506919892)
--(axis cs:0.042499999050051,0.122807293909428)
--(axis cs:0.0449999989941716,0.122531057774966)
--(axis cs:0.0474999989382923,0.122139999108882)
--(axis cs:0.0474999989382923,0.158075039864172)
--(axis cs:0.0474999989382923,0.158075039864172)
--(axis cs:0.0449999989941716,0.157368925227393)
--(axis cs:0.042499999050051,0.156572898265892)
--(axis cs:0.0399999991059303,0.155674570582542)
--(axis cs:0.0374999991618097,0.155012172587297)
--(axis cs:0.034999999217689,0.154325606658226)
--(axis cs:0.0324999992735684,0.153702067746465)
--(axis cs:0.0299999993294477,0.153330257249883)
--(axis cs:0.0274999993853271,0.153433313373949)
--(axis cs:0.0249999994412065,0.154671439713784)
--(axis cs:0.0224999994970858,0.157854108030984)
--(axis cs:0.0199999995529652,0.164163753565803)
--(axis cs:0.0174999996088445,0.174803511538032)
--(axis cs:0.0149999996647239,0.184520161100352)
--(axis cs:0.0124999997206032,0.189238514662264)
--(axis cs:0.00999999977648258,0.18620157612975)
--(axis cs:0.00749999983236194,0.172437983768483)
--(axis cs:0.00499999988824129,0.141055640944796)
--(axis cs:0.00249999994412065,0.0726684754483229)
--cycle;

\path [fill=green!50.1960784313725!black, fill opacity=0.4, ultra thick]
(axis cs:0.00249999994412065,0.471913191838826)
--(axis cs:0.00249999994412065,0.437153809486613)
--(axis cs:0.00499999988824129,0.219158749494758)
--(axis cs:0.00749999983236194,0.177177089333213)
--(axis cs:0.00999999977648258,0.145233073077855)
--(axis cs:0.0124999997206032,0.122410101653298)
--(axis cs:0.0149999996647239,0.110397619244634)
--(axis cs:0.0174999996088445,0.102158190788989)
--(axis cs:0.0199999995529652,0.0952824755533037)
--(axis cs:0.0224999994970858,0.0911564229729691)
--(axis cs:0.0249999994412065,0.0858726084418683)
--(axis cs:0.0274999993853271,0.0809500503208644)
--(axis cs:0.0299999993294477,0.0763872380003592)
--(axis cs:0.0324999992735684,0.0722664109215401)
--(axis cs:0.034999999217689,0.068748196808696)
--(axis cs:0.0374999991618097,0.0659604106854848)
--(axis cs:0.0399999991059303,0.0637998019686118)
--(axis cs:0.042499999050051,0.0630988197218866)
--(axis cs:0.0449999989941716,0.0622103631230509)
--(axis cs:0.0474999989382923,0.0616857911404033)
--(axis cs:0.0474999989382923,0.0796748887686242)
--(axis cs:0.0474999989382923,0.0796748887686242)
--(axis cs:0.0449999989941716,0.0798146604925229)
--(axis cs:0.042499999050051,0.0805947647236089)
--(axis cs:0.0399999991059303,0.0812660419526536)
--(axis cs:0.0374999991618097,0.0835235403113978)
--(axis cs:0.034999999217689,0.086565955604915)
--(axis cs:0.0324999992735684,0.0904555890040852)
--(axis cs:0.0299999993294477,0.0951122465604369)
--(axis cs:0.0274999993853271,0.10039108533724)
--(axis cs:0.0249999994412065,0.106230996340122)
--(axis cs:0.0224999994970858,0.112553883092556)
--(axis cs:0.0199999995529652,0.117247302752853)
--(axis cs:0.0174999996088445,0.125849984192497)
--(axis cs:0.0149999996647239,0.134816606194019)
--(axis cs:0.0124999997206032,0.145047126714834)
--(axis cs:0.00999999977648258,0.161566977215666)
--(axis cs:0.00749999983236194,0.195604350057738)
--(axis cs:0.00499999988824129,0.274533340443556)
--(axis cs:0.00249999994412065,0.471913191838826)
--cycle;

\addplot [ultra thick, red]
table {%
0.00250005722045898 0.0610751584172249
0.00499999523162842 0.129739835858345
0.0075000524520874 0.163508534431458
0.00999999046325684 0.179485812783241
0.0125000476837158 0.184813991189003
0.0149999856948853 0.183000534772873
0.0175000429153442 0.177170634269714
0.0199999809265137 0.170576348900795
0.0225000381469727 0.165996834635735
0.0249999761581421 0.163031607866287
0.0275000333786011 0.16169336438179
0.0299999713897705 0.161517649888992
0.0325000286102295 0.161850154399872
0.0349999666213989 0.162377908825874
0.0375000238418579 0.162762343883514
0.0399999618530273 0.162777572870255
0.0425000190734863 0.162666544318199
0.0449999570846558 0.162021905183792
0.0475000143051147 0.160946264863014
};
\addplot [ultra thick, blue]
table {%
0.00250005722045898 0.0678296685218811
0.00499999523162842 0.135751843452454
0.0075000524520874 0.167184546589851
0.00999999046325684 0.18077877163887
0.0125000476837158 0.183582842350006
0.0149999856948853 0.178725942969322
0.0175000429153442 0.169031485915184
0.0199999809265137 0.158049955964088
0.0225000381469727 0.150499999523163
0.0249999761581421 0.145385026931763
0.0275000333786011 0.142315044999123
0.0299999713897705 0.14068914949894
0.0325000286102295 0.139819964766502
0.0349999666213989 0.139467820525169
0.0375000238418579 0.139367938041687
0.0399999618530273 0.139357045292854
0.0425000190734863 0.139690116047859
0.0449999570846558 0.139949977397919
0.0475000143051147 0.140107527375221
};
\addplot [ultra thick, green!50.1960784313725!black]
table {%
0.00250005722045898 0.45453342795372
0.00499999523162842 0.246846094727516
0.0075000524520874 0.186390697956085
0.00999999046325684 0.153399989008904
0.0125000476837158 0.133728593587875
0.0149999856948853 0.122607104480267
0.0175000429153442 0.114004082977772
0.0199999809265137 0.106264896690845
0.0225000381469727 0.101855143904686
0.0249999761581421 0.096051812171936
0.0275000333786011 0.090670570731163
0.0299999713897705 0.0857497379183769
0.0325000286102295 0.0813609957695007
0.0349999666213989 0.0776570811867714
0.0375000238418579 0.0747419819235802
0.0399999618530273 0.0725329145789146
0.0425000190734863 0.0718467980623245
0.0449999570846558 0.0710125043988228
0.0475000143051147 0.0706803351640701
};

==> supp_mat/ur5e_plots/train_test_loss_data.tex <==
\path [fill=red, fill opacity=0.2, ultra thick]
(axis cs:0,0.0390019230544567)
--(axis cs:0,0.0390019230544567)
--(axis cs:100,0.0389935377607013)
--(axis cs:200,0.038820221300711)
--(axis cs:300,0.0374572107230414)
--(axis cs:400,0.035111146594165)
--(axis cs:500,0.0337754504536296)
--(axis cs:600,0.0327751579160007)
--(axis cs:700,0.0319456771890674)
--(axis cs:800,0.0304680000034032)
--(axis cs:900,0.0287133572675713)
--(axis cs:1000,0.0263532021837723)
--(axis cs:1100,0.0238966970479016)
--(axis cs:1200,0.0218216087100045)
--(axis cs:1300,0.0203481754139741)
--(axis cs:1400,0.0193295853171039)
--(axis cs:1500,0.0187712700380581)
--(axis cs:1600,0.0182842418278811)
--(axis cs:1700,0.0179887703582524)
--(axis cs:1800,0.0174107043169788)
--(axis cs:1900,0.0172072858140255)
--(axis cs:2000,0.0171278444714557)
--(axis cs:2100,0.0167495554083363)
--(axis cs:2200,0.0166856293560179)
--(axis cs:2300,0.0163993936321127)
--(axis cs:2400,0.0160135925717717)
--(axis cs:2500,0.0160705142018792)
--(axis cs:2600,0.015687067451869)
--(axis cs:2700,0.0155677251933654)
--(axis cs:2800,0.0153582092513127)
--(axis cs:2900,0.0152240493458081)
--(axis cs:3000,0.0150642342156459)
--(axis cs:3100,0.0148986713960833)
--(axis cs:3200,0.0147004178557138)
--(axis cs:3300,0.0143914025990864)
--(axis cs:3400,0.0141314140739747)
--(axis cs:3500,0.0138679086936188)
--(axis cs:3600,0.0136463374360309)
--(axis cs:3700,0.0135596232803747)
--(axis cs:3800,0.0133855260270621)
--(axis cs:3900,0.0130769345013418)
--(axis cs:4000,0.0130295029215585)
--(axis cs:4100,0.0126933634329218)
--(axis cs:4200,0.0124905470682182)
--(axis cs:4300,0.0124153131944128)
--(axis cs:4400,0.0124932617899268)
--(axis cs:4500,0.0121981834095788)
--(axis cs:4600,0.0120714540766274)
--(axis cs:4700,0.012112222163656)
--(axis cs:4800,0.0118186145916696)
--(axis cs:4900,0.0118592825138282)
--(axis cs:5000,0.0116095313186105)
--(axis cs:5100,0.0115649135029901)
--(axis cs:5200,0.0117047003214234)
--(axis cs:5300,0.0112487156849648)
--(axis cs:5400,0.0114230507394669)
--(axis cs:5500,0.0114000885954949)
--(axis cs:5600,0.011242422503022)
--(axis cs:5700,0.0109979109148537)
--(axis cs:5800,0.0110227020665706)
--(axis cs:5900,0.0113258599659133)
--(axis cs:6000,0.0110731459589566)
--(axis cs:6100,0.0109757591315358)
--(axis cs:6200,0.0108897253214146)
--(axis cs:6300,0.0109392678172291)
--(axis cs:6400,0.0108540003111364)
--(axis cs:6500,0.0106986108349984)
--(axis cs:6600,0.0104886898854216)
--(axis cs:6700,0.0105874528853446)
--(axis cs:6800,0.010589931894156)
--(axis cs:6900,0.0105021855651666)
--(axis cs:7000,0.0104933879271097)
--(axis cs:7100,0.0104874764774217)
--(axis cs:7200,0.0104466151104123)
--(axis cs:7300,0.0101978540003754)
--(axis cs:7400,0.0102253445844202)
--(axis cs:7500,0.0102641770055587)
--(axis cs:7600,0.0100156815841977)
--(axis cs:7700,0.0102918812925402)
--(axis cs:7800,0.0101722741298809)
--(axis cs:7900,0.0100752079581922)
--(axis cs:8000,0.0100742407043751)
--(axis cs:8100,0.00993030350670319)
--(axis cs:8200,0.0101399599634939)
--(axis cs:8300,0.00990401156249051)
--(axis cs:8400,0.00986824440778013)
--(axis cs:8500,0.0100807580725781)
--(axis cs:8600,0.00984426893009472)
--(axis cs:8700,0.00978200393536158)
--(axis cs:8800,0.0098957208040605)
--(axis cs:8900,0.00985134296544564)
--(axis cs:9000,0.00956138011118001)
--(axis cs:9100,0.00974494757994635)
--(axis cs:9200,0.00966957228431847)
--(axis cs:9300,0.00968610239147603)
--(axis cs:9400,0.00942433481852649)
--(axis cs:9500,0.00945873166574525)
--(axis cs:9600,0.00961692750765235)
--(axis cs:9700,0.00951288025889301)
--(axis cs:9800,0.00951084617814242)
--(axis cs:9900,0.00940022947421289)
--(axis cs:10000,0.00930521063777677)
--(axis cs:10100,0.00956620548676755)
--(axis cs:10200,0.00919848294011048)
--(axis cs:10300,0.00925913271811572)
--(axis cs:10400,0.00926735389766136)
--(axis cs:10500,0.00921621579480726)
--(axis cs:10600,0.00913554999404355)
--(axis cs:10700,0.00915666492010604)
--(axis cs:10800,0.00906463629858183)
--(axis cs:10900,0.00892522726758842)
--(axis cs:11000,0.00904680362973168)
--(axis cs:11100,0.00891162097254798)
--(axis cs:11200,0.00904375286613435)
--(axis cs:11300,0.00902139866044665)
--(axis cs:11400,0.0091464407591103)
--(axis cs:11500,0.00913317560390981)
--(axis cs:11600,0.00900773778476909)
--(axis cs:11700,0.00881875193035082)
--(axis cs:11800,0.00894772454291747)
--(axis cs:11900,0.00890308476985161)
--(axis cs:12000,0.0088918730606556)
--(axis cs:12100,0.00875854685392737)
--(axis cs:12200,0.0087886762856131)
--(axis cs:12300,0.00870813260688227)
--(axis cs:12400,0.00876822482892754)
--(axis cs:12500,0.00872705711636747)
--(axis cs:12600,0.00844241337050077)
--(axis cs:12700,0.00858775839734778)
--(axis cs:12800,0.00869631322190546)
--(axis cs:12900,0.00852511492234635)
--(axis cs:13000,0.00862470241674096)
--(axis cs:13100,0.00855684281157158)
--(axis cs:13200,0.00849748396239164)
--(axis cs:13300,0.00847296703056671)
--(axis cs:13400,0.00857985105092882)
--(axis cs:13500,0.00860978579817038)
--(axis cs:13600,0.0085171372593455)
--(axis cs:13700,0.00847827441763168)
--(axis cs:13800,0.00845297603993865)
--(axis cs:13900,0.00841286057663339)
--(axis cs:14000,0.00851908722302513)
--(axis cs:14100,0.00843923603366369)
--(axis cs:14200,0.00836468332273902)
--(axis cs:14300,0.00834230592489208)
--(axis cs:14400,0.00828220070166768)
--(axis cs:14500,0.00840020743556755)
--(axis cs:14600,0.00809642957247223)
--(axis cs:14700,0.00817862713847061)
--(axis cs:14800,0.00828825786729658)
--(axis cs:14900,0.00823762768116255)
--(axis cs:15000,0.00810482894566643)
--(axis cs:15100,0.00820295153444956)
--(axis cs:15200,0.00821836663425745)
--(axis cs:15300,0.00831141557665537)
--(axis cs:15400,0.00819623478996619)
--(axis cs:15500,0.00804897649605054)
--(axis cs:15600,0.00791164237865653)
--(axis cs:15700,0.00788106313789754)
--(axis cs:15800,0.00798870882063932)
--(axis cs:15900,0.00793909059815781)
--(axis cs:16000,0.00801860862503443)
--(axis cs:16100,0.00808516503598333)
--(axis cs:16200,0.00811777314866733)
--(axis cs:16300,0.00787014450993398)
--(axis cs:16400,0.00796453540891239)
--(axis cs:16500,0.00783531820941225)
--(axis cs:16600,0.00783880155870226)
--(axis cs:16700,0.0079092997486794)
--(axis cs:16800,0.00794334274554502)
--(axis cs:16900,0.00810734208059149)
--(axis cs:17000,0.00785580026397593)
--(axis cs:17100,0.00804709377977169)
--(axis cs:17200,0.00786014504959882)
--(axis cs:17300,0.00789820331957385)
--(axis cs:17400,0.00809562585048097)
--(axis cs:17500,0.00789633376190455)
--(axis cs:17600,0.00790698543359649)
--(axis cs:17700,0.00805270701066)
--(axis cs:17800,0.00784721246763646)
--(axis cs:17900,0.00779746951263744)
--(axis cs:18000,0.00785846147230269)
--(axis cs:18100,0.00790799847281275)
--(axis cs:18200,0.0077795116392026)
--(axis cs:18300,0.00789274469109758)
--(axis cs:18400,0.00791085653691805)
--(axis cs:18500,0.00780632440726103)
--(axis cs:18600,0.00782029891908889)
--(axis cs:18700,0.00782565188222422)
--(axis cs:18800,0.00774952120416009)
--(axis cs:18900,0.0078251347800603)
--(axis cs:19000,0.00768757253261497)
--(axis cs:19100,0.00771380361548724)
--(axis cs:19200,0.00759052524803289)
--(axis cs:19300,0.00774001797214972)
--(axis cs:19400,0.00783912518808262)
--(axis cs:19500,0.00787840328723618)
--(axis cs:19600,0.00760576595893871)
--(axis cs:19700,0.00783620519297671)
--(axis cs:19800,0.00777783850355871)
--(axis cs:19900,0.00765096498542813)
--(axis cs:20000,0.00771298951788669)
--(axis cs:20100,0.00758096477966604)
--(axis cs:20200,0.00793066135964605)
--(axis cs:20300,0.00776740483038818)
--(axis cs:20400,0.00763139482291003)
--(axis cs:20500,0.00765562133347785)
--(axis cs:20600,0.00767951223348876)
--(axis cs:20700,0.00759920155890349)
--(axis cs:20800,0.00752264660583358)
--(axis cs:20900,0.00747395022208779)
--(axis cs:21000,0.00758517559496483)
--(axis cs:21100,0.00752126068821471)
--(axis cs:21200,0.00755554419978906)
--(axis cs:21300,0.00761459309123421)
--(axis cs:21400,0.00764059626312338)
--(axis cs:21500,0.00772170446355137)
--(axis cs:21600,0.00741617273869792)
--(axis cs:21700,0.00757151021847276)
--(axis cs:21800,0.0077398232236092)
--(axis cs:21900,0.00741727590322288)
--(axis cs:22000,0.00759938032392324)
--(axis cs:22100,0.00762857381525359)
--(axis cs:22200,0.00755934063593784)
--(axis cs:22300,0.00760354587697724)
--(axis cs:22400,0.00756494789618983)
--(axis cs:22500,0.0074590032550326)
--(axis cs:22600,0.00766536267280333)
--(axis cs:22700,0.007575873584747)
--(axis cs:22700,0.00852821395923725)
--(axis cs:22700,0.00852821395923725)
--(axis cs:22600,0.00851400708973653)
--(axis cs:22500,0.00854710480793009)
--(axis cs:22400,0.0085299658099936)
--(axis cs:22300,0.00852379244552315)
--(axis cs:22200,0.00853086616595349)
--(axis cs:22100,0.00851981426007826)
--(axis cs:22000,0.00852445653613745)
--(axis cs:21900,0.00855391811818091)
--(axis cs:21800,0.00850243223313642)
--(axis cs:21700,0.0085289131920621)
--(axis cs:21600,0.00855409865247528)
--(axis cs:21500,0.00850522359670209)
--(axis cs:21400,0.00851791094242252)
--(axis cs:21300,0.00852203393218453)
--(axis cs:21200,0.00853147623713365)
--(axis cs:21100,0.00853700205980817)
--(axis cs:21000,0.00852672512453874)
--(axis cs:20900,0.00854467202231001)
--(axis cs:20800,0.00853677812232156)
--(axis cs:20700,0.00852448504778183)
--(axis cs:20600,0.00851178777123193)
--(axis cs:20500,0.00851553975188935)
--(axis cs:20400,0.00851936719366451)
--(axis cs:20300,0.0084982193723997)
--(axis cs:20200,0.00847460690218396)
--(axis cs:20100,0.00852739877669913)
--(axis cs:20000,0.00850657240168328)
--(axis cs:19900,0.00851627367969565)
--(axis cs:19800,0.00849663823074175)
--(axis cs:19700,0.00848794269951828)
--(axis cs:19600,0.00852343873400121)
--(axis cs:19500,0.0084818494979498)
--(axis cs:19400,0.00848751523406291)
--(axis cs:19300,0.00850240232869161)
--(axis cs:19200,0.00852587003421577)
--(axis cs:19100,0.00850644624102451)
--(axis cs:19000,0.00851052736866384)
--(axis cs:18900,0.00848957043285067)
--(axis cs:18800,0.00850094572372592)
--(axis cs:18700,0.0084894941567054)
--(axis cs:18600,0.00849028488098854)
--(axis cs:18500,0.00849236050516226)
--(axis cs:18400,0.00847730581274314)
--(axis cs:18300,0.00847982452469682)
--(axis cs:18200,0.00849638536202415)
--(axis cs:18100,0.00847770021819773)
--(axis cs:18000,0.00848470557937025)
--(axis cs:17900,0.00849368379412493)
--(axis cs:17800,0.00848633557404499)
--(axis cs:17700,0.00845989307348586)
--(axis cs:17600,0.00847784029772072)
--(axis cs:17500,0.00847932185690213)
--(axis cs:17400,0.00845603762773456)
--(axis cs:17300,0.00847906069331919)
--(axis cs:17200,0.00848446275809704)
--(axis cs:17100,0.00846046660748207)
--(axis cs:17000,0.00848509001444293)
--(axis cs:16900,0.00845518620677951)
--(axis cs:16800,0.00847291263913859)
--(axis cs:16700,0.00844037662690838)
--(axis cs:16600,0.00840402790319018)
--(axis cs:16500,0.0084073752793843)
--(axis cs:16400,0.00842647057900996)
--(axis cs:16300,0.00839681179457645)
--(axis cs:16200,0.00851360719576328)
--(axis cs:16100,0.00850046191388328)
--(axis cs:16000,0.00845512488454587)
--(axis cs:15900,0.00845222210533245)
--(axis cs:15800,0.00844608360856944)
--(axis cs:15700,0.00845295925741525)
--(axis cs:15600,0.00840490250678016)
--(axis cs:15500,0.00843070568125468)
--(axis cs:15400,0.0085227817669723)
--(axis cs:15300,0.00858073819307615)
--(axis cs:15200,0.00849682156601766)
--(axis cs:15100,0.00848399958624492)
--(axis cs:15000,0.00843696748031191)
--(axis cs:14900,0.00847256490482232)
--(axis cs:14800,0.00853539402266339)
--(axis cs:14700,0.00863410778826972)
--(axis cs:14600,0.00855669591231221)
--(axis cs:14500,0.00864330736251735)
--(axis cs:14400,0.00852071746425449)
--(axis cs:14300,0.00852016162733272)
--(axis cs:14200,0.00860455601649342)
--(axis cs:14100,0.00852340457468674)
--(axis cs:14000,0.00871133842784965)
--(axis cs:13900,0.0085958233780426)
--(axis cs:13800,0.00875096528044093)
--(axis cs:13700,0.0086427897485963)
--(axis cs:13600,0.00863826539109026)
--(axis cs:13500,0.00898183841210782)
--(axis cs:13400,0.00883680434549292)
--(axis cs:13300,0.00857401911719464)
--(axis cs:13200,0.00863820879795668)
--(axis cs:13100,0.00882062501443721)
--(axis cs:13000,0.0088118317495951)
--(axis cs:12900,0.00866310443121028)
--(axis cs:12800,0.00895445493891455)
--(axis cs:12700,0.00886710481813843)
--(axis cs:12600,0.00888762840560002)
--(axis cs:12500,0.00877532776481107)
--(axis cs:12400,0.00879215412985401)
--(axis cs:12300,0.00897497852430898)
--(axis cs:12200,0.00900164311243244)
--(axis cs:12100,0.00898484133693815)
--(axis cs:12000,0.00936606588563123)
--(axis cs:11900,0.00918494989473954)
--(axis cs:11800,0.00896314462830458)
--(axis cs:11700,0.00906422475064321)
--(axis cs:11600,0.00916905564647322)
--(axis cs:11500,0.00916659276449331)
--(axis cs:11400,0.00958263627210473)
--(axis cs:11300,0.00918483139385239)
--(axis cs:11200,0.00925321905101805)
--(axis cs:11100,0.00908139147063687)
--(axis cs:11000,0.00932396194206124)
--(axis cs:10900,0.00919033542966322)
--(axis cs:10800,0.00942002816144142)
--(axis cs:10700,0.00938779789978811)
--(axis cs:10600,0.00926109144416249)
--(axis cs:10500,0.00947963723488094)
--(axis cs:10400,0.0096596949941214)
--(axis cs:10300,0.00936210212601258)
--(axis cs:10200,0.00956413536318847)
--(axis cs:10100,0.0096797152160475)
--(axis cs:10000,0.00965273705350486)
--(axis cs:9900,0.00952052678137406)
--(axis cs:9800,0.00964103515902342)
--(axis cs:9700,0.00970604512777424)
--(axis cs:9600,0.010059750375019)
--(axis cs:9500,0.00972544793830824)
--(axis cs:9400,0.0097313134080128)
--(axis cs:9300,0.00975118150691729)
--(axis cs:9200,0.00979559727460398)
--(axis cs:9100,0.010041680383239)
--(axis cs:9000,0.0100112206111329)
--(axis cs:8900,0.0101727399684174)
--(axis cs:8800,0.00997791814374427)
--(axis cs:8700,0.010040242149249)
--(axis cs:8600,0.0100072424142189)
--(axis cs:8500,0.0102405943347582)
--(axis cs:8400,0.0101050566104977)
--(axis cs:8300,0.00998221017417903)
--(axis cs:8200,0.0103157071646717)
--(axis cs:8100,0.0100755900763959)
--(axis cs:8000,0.0104169868032162)
--(axis cs:7900,0.0102898948792909)
--(axis cs:7800,0.0103158533153004)
--(axis cs:7700,0.0103478878195302)
--(axis cs:7600,0.0102646646901783)
--(axis cs:7500,0.0104970253943706)
--(axis cs:7400,0.0106071244815639)
--(axis cs:7300,0.0106653164247217)
--(axis cs:7200,0.010934640128836)
--(axis cs:7100,0.0108335849003023)
--(axis cs:7000,0.0108945467576437)
--(axis cs:6900,0.0106327888698052)
--(axis cs:6800,0.0106896750740085)
--(axis cs:6700,0.0108020867786457)
--(axis cs:6600,0.0108178099534075)
--(axis cs:6500,0.0110615262958183)
--(axis cs:6400,0.0114355471372206)
--(axis cs:6300,0.0111486700245837)
--(axis cs:6200,0.0112242504369392)
--(axis cs:6100,0.0112935432266942)
--(axis cs:6000,0.0115619774230554)
--(axis cs:5900,0.0115284868160557)
--(axis cs:5800,0.0110447690303424)
--(axis cs:5700,0.0112602360615776)
--(axis cs:5600,0.0113096219382806)
--(axis cs:5500,0.0116192593652554)
--(axis cs:5400,0.0114529710232221)
--(axis cs:5300,0.011527771288003)
--(axis cs:5200,0.0117419812773989)
--(axis cs:5100,0.0118656506273559)
--(axis cs:5000,0.0121325459326649)
--(axis cs:4900,0.0120196196830559)
--(axis cs:4800,0.0121390377585972)
--(axis cs:4700,0.0123337368927611)
--(axis cs:4600,0.0121886291368212)
--(axis cs:4500,0.0126026871579814)
--(axis cs:4400,0.012760267560036)
--(axis cs:4300,0.0128665420212161)
--(axis cs:4200,0.0129199405587715)
--(axis cs:4100,0.0132699591370048)
--(axis cs:4000,0.0131105716345141)
--(axis cs:3900,0.0134690464438878)
--(axis cs:3800,0.0137955740732167)
--(axis cs:3700,0.0138610794204389)
--(axis cs:3600,0.0140495425250227)
--(axis cs:3500,0.0140949758616416)
--(axis cs:3400,0.0141659655389479)
--(axis cs:3300,0.014597876422733)
--(axis cs:3200,0.0150502037114561)
--(axis cs:3100,0.0149925711875094)
--(axis cs:3000,0.015092295603326)
--(axis cs:2900,0.0153364453651936)
--(axis cs:2800,0.0155164714764075)
--(axis cs:2700,0.0157650557241201)
--(axis cs:2600,0.0159194800825968)
--(axis cs:2500,0.0161309423250361)
--(axis cs:2400,0.0163668753298556)
--(axis cs:2300,0.01667861625145)
--(axis cs:2200,0.0168888834932335)
--(axis cs:2100,0.016997188787284)
--(axis cs:2000,0.0172256042274623)
--(axis cs:1900,0.0174184033746138)
--(axis cs:1800,0.0176467609184135)
--(axis cs:1700,0.0182706809019169)
--(axis cs:1600,0.0183582226707977)
--(axis cs:1500,0.0189357607351048)
--(axis cs:1400,0.0195207395321838)
--(axis cs:1300,0.0208439116204103)
--(axis cs:1200,0.0221191241664553)
--(axis cs:1100,0.0242660252913312)
--(axis cs:1000,0.0269350464942761)
--(axis cs:900,0.0288973531943631)
--(axis cs:800,0.0307619814786258)
--(axis cs:700,0.0324469863493886)
--(axis cs:600,0.0331448051060724)
--(axis cs:500,0.0342312066103315)
--(axis cs:400,0.0353095805395859)
--(axis cs:300,0.0375690133338382)
--(axis cs:200,0.0388255995752516)
--(axis cs:100,0.0389938276639317)
--(axis cs:0,0.0390019230544567)
--cycle;

\path [fill=blue, fill opacity=0.2, ultra thick]
(axis cs:0,0.038980360346801)
--(axis cs:0,0.0389803568345637)
--(axis cs:100,0.0389721848099988)
--(axis cs:200,0.0387978504297354)
--(axis cs:300,0.037416131816138)
--(axis cs:400,0.0351344817768292)
--(axis cs:500,0.0336935621386484)
--(axis cs:600,0.0327247050193857)
--(axis cs:700,0.0319627263859943)
--(axis cs:800,0.0303625192061382)
--(axis cs:900,0.0283576864043883)
--(axis cs:1000,0.0260043408975868)
--(axis cs:1100,0.0234878884424759)
--(axis cs:1200,0.0214170939421079)
--(axis cs:1300,0.0202215421845153)
--(axis cs:1400,0.0192905561711082)
--(axis cs:1500,0.018568268183964)
--(axis cs:1600,0.0180824703411802)
--(axis cs:1700,0.0176455662925474)
--(axis cs:1800,0.0171719887525245)
--(axis cs:1900,0.0168443696723664)
--(axis cs:2000,0.0163694674161094)
--(axis cs:2100,0.0158459593809483)
--(axis cs:2200,0.0154668718878377)
--(axis cs:2300,0.0149198261708462)
--(axis cs:2400,0.0141955985261853)
--(axis cs:2500,0.0142092102276979)
--(axis cs:2600,0.0137411311458298)
--(axis cs:2700,0.0136212100073159)
--(axis cs:2800,0.0132749232272979)
--(axis cs:2900,0.0131564389878724)
--(axis cs:3000,0.0129516400876213)
--(axis cs:3100,0.0128067363169031)
--(axis cs:3200,0.0127304952225964)
--(axis cs:3300,0.0124568400099384)
--(axis cs:3400,0.0125115983962562)
--(axis cs:3500,0.0121923084621607)
--(axis cs:3600,0.0122234976383133)
--(axis cs:3700,0.0121354270499735)
--(axis cs:3800,0.011882547837733)
--(axis cs:3900,0.0119184152480948)
--(axis cs:4000,0.0118032223081315)
--(axis cs:4100,0.0119024465824155)
--(axis cs:4200,0.0116873125650591)
--(axis cs:4300,0.0117222575913396)
--(axis cs:4400,0.0116457164775315)
--(axis cs:4500,0.0114728227144562)
--(axis cs:4600,0.0113898960957961)
--(axis cs:4700,0.0114035357242036)
--(axis cs:4800,0.0113699003676702)
--(axis cs:4900,0.0112372807627182)
--(axis cs:5000,0.0111406086964914)
--(axis cs:5100,0.0110891127488941)
--(axis cs:5200,0.0110954118913194)
--(axis cs:5300,0.0108640509765671)
--(axis cs:5400,0.0108781974035263)
--(axis cs:5500,0.0111339849469059)
--(axis cs:5600,0.0109519955586202)
--(axis cs:5700,0.0106666206095436)
--(axis cs:5800,0.0107454282936472)
--(axis cs:5900,0.0108044403928586)
--(axis cs:6000,0.0107194096838028)
--(axis cs:6100,0.010597745589222)
--(axis cs:6200,0.0107401374215122)
--(axis cs:6300,0.0105291358947433)
--(axis cs:6400,0.0103793072275857)
--(axis cs:6500,0.0102338978412076)
--(axis cs:6600,0.0101838031956194)
--(axis cs:6700,0.0104625614751282)
--(axis cs:6800,0.0101029542470737)
--(axis cs:6900,0.00989806233169144)
--(axis cs:7000,0.0100067357010927)
--(axis cs:7100,0.0102067653008396)
--(axis cs:7200,0.0100081847327594)
--(axis cs:7300,0.00988462787603704)
--(axis cs:7400,0.00977607490814138)
--(axis cs:7500,0.00956886383740498)
--(axis cs:7600,0.00965966469205192)
--(axis cs:7700,0.00950330992030682)
--(axis cs:7800,0.00955123298993774)
--(axis cs:7900,0.0094522805693688)
--(axis cs:8000,0.00931912498732138)
--(axis cs:8100,0.00950747856645895)
--(axis cs:8200,0.00931660340577969)
--(axis cs:8300,0.00911405457891658)
--(axis cs:8400,0.0092207814061763)
--(axis cs:8500,0.00913149880302797)
--(axis cs:8600,0.0091987051461474)
--(axis cs:8700,0.00906780558604704)
--(axis cs:8800,0.00896956344587149)
--(axis cs:8900,0.00899653767674365)
--(axis cs:9000,0.00893033980424356)
--(axis cs:9100,0.0089215929134014)
--(axis cs:9200,0.00888550623348204)
--(axis cs:9300,0.00886176494480199)
--(axis cs:9400,0.00849689186354955)
--(axis cs:9500,0.00868439716808915)
--(axis cs:9600,0.00867833022524581)
--(axis cs:9700,0.0083988752378818)
--(axis cs:9800,0.00856478470075495)
--(axis cs:9900,0.00849520308787294)
--(axis cs:10000,0.00838825828897466)
--(axis cs:10100,0.00866240942720303)
--(axis cs:10200,0.00819942787740677)
--(axis cs:10300,0.00848647863103921)
--(axis cs:10400,0.00827440098847979)
--(axis cs:10500,0.00828305876315057)
--(axis cs:10600,0.00809241686160554)
--(axis cs:10700,0.00797315661509834)
--(axis cs:10800,0.00800735487681699)
--(axis cs:10900,0.00777791655004944)
--(axis cs:11000,0.00791165344409051)
--(axis cs:11100,0.00773609681103695)
--(axis cs:11200,0.00784543908309972)
--(axis cs:11300,0.00761609665838511)
--(axis cs:11400,0.00794606767211969)
--(axis cs:11500,0.00760464704590356)
--(axis cs:11600,0.00760642208449722)
--(axis cs:11700,0.00777880064906505)
--(axis cs:11800,0.007705969625634)
--(axis cs:11900,0.00770212091396891)
--(axis cs:12000,0.00762178288261719)
--(axis cs:12100,0.00743533161715177)
--(axis cs:12200,0.00725828843871519)
--(axis cs:12300,0.00730049838585498)
--(axis cs:12400,0.00726049048835554)
--(axis cs:12500,0.00744890649412878)
--(axis cs:12600,0.00723177190805919)
--(axis cs:12700,0.00743024244721573)
--(axis cs:12800,0.00716151818236276)
--(axis cs:12900,0.00717142691343633)
--(axis cs:13000,0.00706647175747577)
--(axis cs:13100,0.00729899610664002)
--(axis cs:13200,0.00693629834888316)
--(axis cs:13300,0.00694568735613641)
--(axis cs:13400,0.00696144878839016)
--(axis cs:13500,0.00708887565391173)
--(axis cs:13600,0.00709457720270843)
--(axis cs:13700,0.00691325231660435)
--(axis cs:13800,0.00688392193197541)
--(axis cs:13900,0.00679142768582729)
--(axis cs:14000,0.00675322766270128)
--(axis cs:14100,0.0068470827387971)
--(axis cs:14200,0.00680981983088893)
--(axis cs:14300,0.00656805376546546)
--(axis cs:14400,0.00668084678094104)
--(axis cs:14500,0.00660636573296926)
--(axis cs:14600,0.00669499299108831)
--(axis cs:14700,0.00656764966842501)
--(axis cs:14800,0.00660066955185303)
--(axis cs:14900,0.0065216203205995)
--(axis cs:15000,0.0067054257270076)
--(axis cs:15100,0.00644700803819003)
--(axis cs:15200,0.00657660024364443)
--(axis cs:15300,0.00647662395437266)
--(axis cs:15400,0.00653311396626778)
--(axis cs:15500,0.00627659959432214)
--(axis cs:15600,0.00630108807038502)
--(axis cs:15700,0.00623155433442663)
--(axis cs:15800,0.00632928979543296)
--(axis cs:15900,0.00623340804685052)
--(axis cs:16000,0.00621633208266651)
--(axis cs:16100,0.00634656439186504)
--(axis cs:16200,0.00620301784558253)
--(axis cs:16300,0.00612101827533021)
--(axis cs:16400,0.00608617525561459)
--(axis cs:16500,0.00628151758046672)
--(axis cs:16600,0.0064018964828007)
--(axis cs:16700,0.00602537345592028)
--(axis cs:16800,0.00607406861764413)
--(axis cs:16900,0.00603267125946271)
--(axis cs:17000,0.00599511593603545)
--(axis cs:17100,0.00603225232076827)
--(axis cs:17200,0.00604644357890509)
--(axis cs:17300,0.006129523967479)
--(axis cs:17400,0.00605193265427383)
--(axis cs:17500,0.0061461732439221)
--(axis cs:17600,0.00594677277434289)
--(axis cs:17700,0.00579436420948821)
--(axis cs:17800,0.00595430883462606)
--(axis cs:17900,0.00589069862388415)
--(axis cs:18000,0.00584553950173259)
--(axis cs:18100,0.00586802476801412)
--(axis cs:18200,0.00581697877415387)
--(axis cs:18300,0.00583165936548952)
--(axis cs:18400,0.00573803728088986)
--(axis cs:18500,0.0057443358420666)
--(axis cs:18600,0.00582729756128459)
--(axis cs:18700,0.00581481694696823)
--(axis cs:18800,0.00570845378929767)
--(axis cs:18900,0.00570043654715355)
--(axis cs:19000,0.00585628529869073)
--(axis cs:19100,0.00563092633216951)
--(axis cs:19200,0.00583227470401506)
--(axis cs:19300,0.00576280173593403)
--(axis cs:19400,0.00562517856011497)
--(axis cs:19500,0.00563887668270049)
--(axis cs:19600,0.00562185692928885)
--(axis cs:19700,0.00558684199721526)
--(axis cs:19800,0.00576467033891056)
--(axis cs:19900,0.0057120508071795)
--(axis cs:20000,0.00564121735563552)
--(axis cs:20100,0.00551094827399823)
--(axis cs:20200,0.00559778378070519)
--(axis cs:20300,0.00548548837794752)
--(axis cs:20400,0.00563609031572937)
--(axis cs:20500,0.00564888849976819)
--(axis cs:20600,0.00563948451894676)
--(axis cs:20700,0.00536918796828598)
--(axis cs:20800,0.00547037206451498)
--(axis cs:20900,0.00536696785608402)
--(axis cs:21000,0.00549672290580982)
--(axis cs:21100,0.00545821540817292)
--(axis cs:21200,0.00538335488955533)
--(axis cs:21300,0.00557010000013288)
--(axis cs:21400,0.00558686984527378)
--(axis cs:21500,0.00546788175377224)
--(axis cs:21600,0.0054015255020328)
--(axis cs:21700,0.00533397649438218)
--(axis cs:21800,0.00541972499123919)
--(axis cs:21900,0.00542409663302114)
--(axis cs:22000,0.00538981594098939)
--(axis cs:22100,0.00541585406440399)
--(axis cs:22200,0.00535599354803356)
--(axis cs:22300,0.00542055997996261)
--(axis cs:22400,0.00540709929058687)
--(axis cs:22500,0.00535037656099055)
--(axis cs:22600,0.005420318017853)
--(axis cs:22700,0.00527054074815825)
--(axis cs:22800,0.00537088338243734)
--(axis cs:22900,0.00538343561876557)
--(axis cs:23000,0.00536328469756404)
--(axis cs:23100,0.00540891740492364)
--(axis cs:23200,0.00541321184283982)
--(axis cs:23300,0.00536481179112321)
--(axis cs:23400,0.00533050647498585)
--(axis cs:23500,0.00541125038294635)
--(axis cs:23600,0.00540632652328542)
--(axis cs:23700,0.00536690474105718)
--(axis cs:23800,0.00538605910576488)
--(axis cs:23800,0.00551867522759135)
--(axis cs:23800,0.00551867522759135)
--(axis cs:23700,0.00551488304582395)
--(axis cs:23600,0.00579368270103006)
--(axis cs:23500,0.00553422682952243)
--(axis cs:23400,0.00551362918196701)
--(axis cs:23300,0.00551465110417082)
--(axis cs:23200,0.00550527502053489)
--(axis cs:23100,0.00549176877964159)
--(axis cs:23000,0.00550916161345283)
--(axis cs:22900,0.00566255396168687)
--(axis cs:22800,0.00564474197767405)
--(axis cs:22700,0.00542863392917399)
--(axis cs:22600,0.00554399084751536)
--(axis cs:22500,0.00560977394908216)
--(axis cs:22400,0.00547726391365393)
--(axis cs:22300,0.00560324953249365)
--(axis cs:22200,0.00564785151283153)
--(axis cs:22100,0.00575206644060312)
--(axis cs:22000,0.00555151812778578)
--(axis cs:21900,0.00564477461176703)
--(axis cs:21800,0.00575257831780406)
--(axis cs:21700,0.00557527226993406)
--(axis cs:21600,0.00568719626255158)
--(axis cs:21500,0.005678911077748)
--(axis cs:21400,0.00566650571477146)
--(axis cs:21300,0.00593596137997532)
--(axis cs:21200,0.00567478565652812)
--(axis cs:21100,0.00572245117759038)
--(axis cs:21000,0.00595984395695216)
--(axis cs:20900,0.0056058067314876)
--(axis cs:20800,0.00578586948553322)
--(axis cs:20700,0.00580655440458446)
--(axis cs:20600,0.00579496250134552)
--(axis cs:20500,0.00573675814893681)
--(axis cs:20400,0.00585715979104242)
--(axis cs:20300,0.00574874446745821)
--(axis cs:20200,0.00590125853159899)
--(axis cs:20100,0.00576871510747897)
--(axis cs:20000,0.00589547863880122)
--(axis cs:19900,0.00600961205939304)
--(axis cs:19800,0.0058800410686118)
--(axis cs:19700,0.00588680159627487)
--(axis cs:19600,0.00591503619509285)
--(axis cs:19500,0.00598863195510529)
--(axis cs:19400,0.0059891726627975)
--(axis cs:19300,0.00597439745382824)
--(axis cs:19200,0.00591664580123047)
--(axis cs:19100,0.00606764159719772)
--(axis cs:19000,0.00601759044595009)
--(axis cs:18900,0.00592792269860372)
--(axis cs:18800,0.0059550333917698)
--(axis cs:18700,0.0058542153287085)
--(axis cs:18600,0.00593775003610384)
--(axis cs:18500,0.00610777520444632)
--(axis cs:18400,0.00607427152231086)
--(axis cs:18300,0.00612353605151729)
--(axis cs:18200,0.00592862560184431)
--(axis cs:18100,0.00619468470009231)
--(axis cs:18000,0.00612346680817405)
--(axis cs:17900,0.00605720360604084)
--(axis cs:17800,0.00606712348565084)
--(axis cs:17700,0.00614390783457441)
--(axis cs:17600,0.00610594919047336)
--(axis cs:17500,0.00632934123009234)
--(axis cs:17400,0.00645696166257826)
--(axis cs:17300,0.0062854057999707)
--(axis cs:17200,0.00625053542623299)
--(axis cs:17100,0.0062157928232135)
--(axis cs:17000,0.00638786139564262)
--(axis cs:16900,0.00629929598259938)
--(axis cs:16800,0.00641318641918677)
--(axis cs:16700,0.00639522092586909)
--(axis cs:16600,0.00654432580511247)
--(axis cs:16500,0.00663062264738754)
--(axis cs:16400,0.0064469424509624)
--(axis cs:16300,0.00635090346663223)
--(axis cs:16200,0.00645934601393187)
--(axis cs:16100,0.00644531384148825)
--(axis cs:16000,0.00653298408814515)
--(axis cs:15900,0.00640805258791749)
--(axis cs:15800,0.00661823851717067)
--(axis cs:15700,0.00688658047709394)
--(axis cs:15600,0.00655010082025095)
--(axis cs:15500,0.00666010488731931)
--(axis cs:15400,0.00670149049422992)
--(axis cs:15300,0.00684649495582078)
--(axis cs:15200,0.00667010954767812)
--(axis cs:15100,0.00681016423093575)
--(axis cs:15000,0.00684804650879124)
--(axis cs:14900,0.00677172762173292)
--(axis cs:14800,0.00696906357609859)
--(axis cs:14700,0.00682615817738604)
--(axis cs:14600,0.00693172838608575)
--(axis cs:14500,0.00699019258953987)
--(axis cs:14400,0.00708341231405223)
--(axis cs:14300,0.0070538306326969)
--(axis cs:14200,0.00693903798268793)
--(axis cs:14100,0.00727181530026572)
--(axis cs:14000,0.00705841246827556)
--(axis cs:13900,0.00710914009162757)
--(axis cs:13800,0.00733804743906525)
--(axis cs:13700,0.00718670945098967)
--(axis cs:13600,0.00719263566085606)
--(axis cs:13500,0.0071657989719817)
--(axis cs:13400,0.00718919927900473)
--(axis cs:13300,0.00731712050980114)
--(axis cs:13200,0.00735545936884546)
--(axis cs:13100,0.00744886380349048)
--(axis cs:13000,0.00753517826946155)
--(axis cs:12900,0.00735966238995783)
--(axis cs:12800,0.00756918335109389)
--(axis cs:12700,0.00768315567507504)
--(axis cs:12600,0.00746226531827999)
--(axis cs:12500,0.00763615365530245)
--(axis cs:12400,0.0079444703024177)
--(axis cs:12300,0.0077030881125446)
--(axis cs:12200,0.00777596433898047)
--(axis cs:12100,0.00765860620950155)
--(axis cs:12000,0.00796956936408453)
--(axis cs:11900,0.00781449455876506)
--(axis cs:11800,0.00787988347170548)
--(axis cs:11700,0.00795816077776922)
--(axis cs:11600,0.0080005788649849)
--(axis cs:11500,0.0079115421915321)
--(axis cs:11400,0.00825299770022814)
--(axis cs:11300,0.00823121407590676)
--(axis cs:11200,0.00833820762314363)
--(axis cs:11100,0.00827164820657105)
--(axis cs:11000,0.00825672174501516)
--(axis cs:10900,0.00824148396957988)
--(axis cs:10800,0.00833370800671903)
--(axis cs:10700,0.0084237626502911)
--(axis cs:10600,0.0083907658468168)
--(axis cs:10500,0.0085466883226194)
--(axis cs:10400,0.00849632197691963)
--(axis cs:10300,0.00860916663771893)
--(axis cs:10200,0.00862148157801182)
--(axis cs:10100,0.00888745676235627)
--(axis cs:10000,0.00919481327565998)
--(axis cs:9900,0.0087295042423937)
--(axis cs:9800,0.00875703722230229)
--(axis cs:9700,0.00901998801392351)
--(axis cs:9600,0.00891482507934506)
--(axis cs:9500,0.00893482088831146)
--(axis cs:9400,0.00884268976012388)
--(axis cs:9300,0.00897325234888965)
--(axis cs:9200,0.00936557879953735)
--(axis cs:9100,0.00923410233623557)
--(axis cs:9000,0.00915430546705771)
--(axis cs:8900,0.0091454720981002)
--(axis cs:8800,0.00950734185534178)
--(axis cs:8700,0.00966434108437392)
--(axis cs:8600,0.00948043188508988)
--(axis cs:8500,0.00961469159093649)
--(axis cs:8400,0.00977868029930968)
--(axis cs:8300,0.00949431497516598)
--(axis cs:8200,0.00961785943457872)
--(axis cs:8100,0.00980114870618669)
--(axis cs:8000,0.00975633760730696)
--(axis cs:7900,0.00951577445537428)
--(axis cs:7800,0.00983036526907416)
--(axis cs:7700,0.00994602342955687)
--(axis cs:7600,0.00988701732300946)
--(axis cs:7500,0.00983184267731117)
--(axis cs:7400,0.0100666906963149)
--(axis cs:7300,0.0102170075303776)
--(axis cs:7200,0.0103337592167016)
--(axis cs:7100,0.0103674827845798)
--(axis cs:7000,0.0103921027444515)
--(axis cs:6900,0.0103644137251228)
--(axis cs:6800,0.0102929443235433)
--(axis cs:6700,0.0105352856448389)
--(axis cs:6600,0.0103832941950721)
--(axis cs:6500,0.0107622884201681)
--(axis cs:6400,0.0110378927168708)
--(axis cs:6300,0.0106655859877987)
--(axis cs:6200,0.0108357064938311)
--(axis cs:6100,0.0108784759920781)
--(axis cs:6000,0.0109503121679435)
--(axis cs:5900,0.0110906329613856)
--(axis cs:5800,0.0108595424247763)
--(axis cs:5700,0.0107211973494471)
--(axis cs:5600,0.011028309954126)
--(axis cs:5500,0.0113493881139166)
--(axis cs:5400,0.0112124350649357)
--(axis cs:5300,0.011178669291603)
--(axis cs:5200,0.0113400986397484)
--(axis cs:5100,0.0115137154706389)
--(axis cs:5000,0.0115810494538636)
--(axis cs:4900,0.0113814544463892)
--(axis cs:4800,0.0114849251141022)
--(axis cs:4700,0.011684244577566)
--(axis cs:4600,0.0116603630820874)
--(axis cs:4500,0.0119545562926846)
--(axis cs:4400,0.011891256224018)
--(axis cs:4300,0.0117566129991883)
--(axis cs:4200,0.0119003905188932)
--(axis cs:4100,0.0119863555734368)
--(axis cs:4000,0.0119033032560622)
--(axis cs:3900,0.0121107632967842)
--(axis cs:3800,0.0121817639199507)
--(axis cs:3700,0.0123087674606057)
--(axis cs:3600,0.012243868798804)
--(axis cs:3500,0.0123426167354009)
--(axis cs:3400,0.0126116966675176)
--(axis cs:3300,0.0125983983462545)
--(axis cs:3200,0.0128530395893375)
--(axis cs:3100,0.0130794919911785)
--(axis cs:3000,0.0130228987105123)
--(axis cs:2900,0.0133204614158259)
--(axis cs:2800,0.0133883360653444)
--(axis cs:2700,0.0141489087805688)
--(axis cs:2600,0.013888425609395)
--(axis cs:2500,0.0143933128806255)
--(axis cs:2400,0.0145572872326915)
--(axis cs:2300,0.0152544323046561)
--(axis cs:2200,0.0157980180974853)
--(axis cs:2100,0.0162056672119262)
--(axis cs:2000,0.016494140834906)
--(axis cs:1900,0.0170010140015399)
--(axis cs:1800,0.0172474075187838)
--(axis cs:1700,0.0179972885768183)
--(axis cs:1600,0.0182401916447734)
--(axis cs:1500,0.0188074774900103)
--(axis cs:1400,0.0193273043547383)
--(axis cs:1300,0.020423161869284)
--(axis cs:1200,0.0219590376620072)
--(axis cs:1100,0.0239195747504638)
--(axis cs:1000,0.0265207162493598)
--(axis cs:900,0.028694050457079)
--(axis cs:800,0.0307005965893152)
--(axis cs:700,0.0322308948918148)
--(axis cs:600,0.0330829280825545)
--(axis cs:500,0.0342243212575003)
--(axis cs:400,0.0353059844284499)
--(axis cs:300,0.0374776705882657)
--(axis cs:200,0.0388021791778785)
--(axis cs:100,0.0389724788537064)
--(axis cs:0,0.038980360346801)
--cycle;

\path [fill=green!50.1960784313725!black, fill opacity=0.2, ultra thick]
(axis cs:0,0.0574927553534508)
--(axis cs:0,0.0574927553534508)
--(axis cs:100,0.0574398323094995)
--(axis cs:200,0.0563991881086609)
--(axis cs:300,0.0523909474641775)
--(axis cs:400,0.0436406503344025)
--(axis cs:500,0.0385023750332377)
--(axis cs:600,0.037651315161948)
--(axis cs:700,0.0373019520434192)
--(axis cs:800,0.0364657131109171)
--(axis cs:900,0.0347989297400964)
--(axis cs:1000,0.0342157445924293)
--(axis cs:1100,0.0337431832079807)
--(axis cs:1200,0.0325821984786356)
--(axis cs:1300,0.0302271483511611)
--(axis cs:1400,0.0274892540903305)
--(axis cs:1500,0.0236997992574177)
--(axis cs:1600,0.0190136311119597)
--(axis cs:1700,0.0158657616125858)
--(axis cs:1800,0.0130195795652949)
--(axis cs:1900,0.0108368017797645)
--(axis cs:2000,0.00967926016292388)
--(axis cs:2100,0.00895624320031587)
--(axis cs:2200,0.00830202486666007)
--(axis cs:2300,0.00802377392365909)
--(axis cs:2400,0.00756239412250593)
--(axis cs:2500,0.00725581998975785)
--(axis cs:2600,0.00705759761986934)
--(axis cs:2700,0.00672410837629789)
--(axis cs:2800,0.00660251940527448)
--(axis cs:2900,0.00643624548207266)
--(axis cs:3000,0.0063785414956291)
--(axis cs:3100,0.00618853762073734)
--(axis cs:3200,0.00603176230732301)
--(axis cs:3300,0.00607485187707195)
--(axis cs:3400,0.00589666125938017)
--(axis cs:3500,0.0057840881000999)
--(axis cs:3600,0.00575743244126428)
--(axis cs:3700,0.00548745148047913)
--(axis cs:3800,0.00550193740326262)
--(axis cs:3900,0.00540350220548376)
--(axis cs:4000,0.00536310874848743)
--(axis cs:4100,0.00537538443499439)
--(axis cs:4200,0.00526290261699403)
--(axis cs:4300,0.00513957142066924)
--(axis cs:4400,0.00498894239818718)
--(axis cs:4500,0.0049644915066338)
--(axis cs:4600,0.00486604764061657)
--(axis cs:4700,0.00483501374457394)
--(axis cs:4800,0.00464911614254584)
--(axis cs:4900,0.00475488219397346)
--(axis cs:5000,0.0046803856785804)
--(axis cs:5100,0.00459886784477667)
--(axis cs:5200,0.00451916193782644)
--(axis cs:5300,0.00438402450545458)
--(axis cs:5400,0.00434502094534958)
--(axis cs:5500,0.00420185405675307)
--(axis cs:5600,0.00419464309442004)
--(axis cs:5700,0.00415376400983838)
--(axis cs:5800,0.00419456178156951)
--(axis cs:5900,0.0040516090345773)
--(axis cs:6000,0.00397977203318683)
--(axis cs:6100,0.00390457263832518)
--(axis cs:6200,0.00393980429653285)
--(axis cs:6300,0.00388658414080813)
--(axis cs:6400,0.00378568302883886)
--(axis cs:6500,0.0038974358418345)
--(axis cs:6600,0.00374189224500883)
--(axis cs:6700,0.00368783240425656)
--(axis cs:6800,0.00360360615701652)
--(axis cs:6900,0.00351975973118442)
--(axis cs:7000,0.00356356159235256)
--(axis cs:7100,0.00355335472379002)
--(axis cs:7200,0.00356858310341571)
--(axis cs:7300,0.00352944144576628)
--(axis cs:7400,0.00339610554475564)
--(axis cs:7500,0.00343882356805005)
--(axis cs:7600,0.0033903580711612)
--(axis cs:7700,0.00337631645582562)
--(axis cs:7800,0.00336384556796734)
--(axis cs:7900,0.00338933067496195)
--(axis cs:8000,0.00328717716787304)
--(axis cs:8100,0.00330344313968388)
--(axis cs:8200,0.00319484943963583)
--(axis cs:8300,0.00329678070589538)
--(axis cs:8400,0.00316306813276715)
--(axis cs:8500,0.0031883282392319)
--(axis cs:8600,0.00314854921959609)
--(axis cs:8700,0.00313843947499677)
--(axis cs:8800,0.00314055295118974)
--(axis cs:8900,0.00309746360519006)
--(axis cs:9000,0.00308585928031348)
--(axis cs:9100,0.0030630458173316)
--(axis cs:9200,0.00310510912508572)
--(axis cs:9300,0.0030208764110315)
--(axis cs:9400,0.00305738914492321)
--(axis cs:9500,0.00303580912832017)
--(axis cs:9600,0.00303640560959866)
--(axis cs:9700,0.00302146828939068)
--(axis cs:9800,0.00302254309751515)
--(axis cs:9900,0.00298186013404566)
--(axis cs:10000,0.00297436451393183)
--(axis cs:10100,0.00298347594339993)
--(axis cs:10200,0.0029145140971962)
--(axis cs:10300,0.00296134084544412)
--(axis cs:10400,0.00287271819317)
--(axis cs:10500,0.00291190251002215)
--(axis cs:10600,0.00286245950750932)
--(axis cs:10700,0.00289253700825415)
--(axis cs:10800,0.00283302903483228)
--(axis cs:10900,0.00284892455584192)
--(axis cs:11000,0.00289913787428177)
--(axis cs:11100,0.00282868989433339)
--(axis cs:11200,0.00285093792260446)
--(axis cs:11300,0.00282676906755292)
--(axis cs:11400,0.00282031945035925)
--(axis cs:11500,0.00279546957378494)
--(axis cs:11600,0.00278755206559797)
--(axis cs:11700,0.00279952027369041)
--(axis cs:11800,0.00278749613198058)
--(axis cs:11900,0.00277580899163854)
--(axis cs:12000,0.00272635423474712)
--(axis cs:12100,0.00275848021636245)
--(axis cs:12200,0.00276132622682162)
--(axis cs:12300,0.00270913885691506)
--(axis cs:12400,0.00268529107986946)
--(axis cs:12500,0.0026606823870683)
--(axis cs:12600,0.00268922332422041)
--(axis cs:12700,0.00270070295349551)
--(axis cs:12800,0.00263753361679908)
--(axis cs:12900,0.00269554873018744)
--(axis cs:13000,0.00264939232614243)
--(axis cs:13100,0.00267358035453497)
--(axis cs:13200,0.00260228182833258)
--(axis cs:13300,0.0026012575501849)
--(axis cs:13400,0.00259584605655915)
--(axis cs:13500,0.00258682430238121)
--(axis cs:13600,0.00257792812973971)
--(axis cs:13700,0.00266199596468644)
--(axis cs:13800,0.00259685989299156)
--(axis cs:13900,0.00261539077296135)
--(axis cs:14000,0.00255323239020712)
--(axis cs:14100,0.00254425387263483)
--(axis cs:14200,0.00251745482382591)
--(axis cs:14300,0.00252255024781303)
--(axis cs:14400,0.00250737768907652)
--(axis cs:14500,0.0024866776061413)
--(axis cs:14600,0.00251389887196295)
--(axis cs:14700,0.00253186219724647)
--(axis cs:14800,0.00247536179743562)
--(axis cs:14900,0.00246446270102361)
--(axis cs:15000,0.00245139955477073)
--(axis cs:15100,0.0024640071841481)
--(axis cs:15200,0.00247728550736303)
--(axis cs:15300,0.00246617142568105)
--(axis cs:15400,0.00245606735780731)
--(axis cs:15500,0.0024044939213219)
--(axis cs:15600,0.00242717445755324)
--(axis cs:15700,0.0024650787121936)
--(axis cs:15800,0.00242970733507119)
--(axis cs:15900,0.00239470289017186)
--(axis cs:16000,0.00239440214628934)
--(axis cs:16100,0.00245976207314404)
--(axis cs:16200,0.00246074993386205)
--(axis cs:16300,0.00242224203622883)
--(axis cs:16400,0.00246222251992883)
--(axis cs:16500,0.00239864531535138)
--(axis cs:16600,0.00235370263261714)
--(axis cs:16700,0.00235248345394131)
--(axis cs:16800,0.00244819159369603)
--(axis cs:16900,0.00234651148568928)
--(axis cs:17000,0.00238102360967895)
--(axis cs:17100,0.00248087553342339)
--(axis cs:17200,0.0023208446960262)
--(axis cs:17300,0.00237260049709953)
--(axis cs:17400,0.00237273561909024)
--(axis cs:17500,0.00229228056251799)
--(axis cs:17600,0.00230433497218091)
--(axis cs:17700,0.00229306913334434)
--(axis cs:17800,0.0022924052957772)
--(axis cs:17900,0.00230430628257357)
--(axis cs:18000,0.00227996609640185)
--(axis cs:18100,0.00236565145292991)
--(axis cs:18200,0.00228075652415216)
--(axis cs:18300,0.00230192295749275)
--(axis cs:18400,0.00224867240426361)
--(axis cs:18500,0.00225365130372409)
--(axis cs:18600,0.00230889891806977)
--(axis cs:18700,0.00231714625709217)
--(axis cs:18800,0.00223408808565062)
--(axis cs:18900,0.00228259123640209)
--(axis cs:19000,0.00229423495742668)
--(axis cs:19100,0.00223361311534969)
--(axis cs:19200,0.00227049994633992)
--(axis cs:19300,0.00224840837270605)
--(axis cs:19400,0.00221888900264166)
--(axis cs:19500,0.00223300107225086)
--(axis cs:19600,0.00219846103298763)
--(axis cs:19700,0.0022162170204979)
--(axis cs:19800,0.00224015208724876)
--(axis cs:19900,0.00220916164368035)
--(axis cs:20000,0.0022426420262222)
--(axis cs:20100,0.00220846788330132)
--(axis cs:20200,0.0022573019006563)
--(axis cs:20300,0.00227880008622362)
--(axis cs:20400,0.00225922659707393)
--(axis cs:20500,0.00223127316565127)
--(axis cs:20600,0.0021849147996661)
--(axis cs:20700,0.00218527252869171)
--(axis cs:20800,0.00215941015303199)
--(axis cs:20900,0.00223217222135763)
--(axis cs:21000,0.0021795323114389)
--(axis cs:21100,0.00218254749033367)
--(axis cs:21200,0.00222667095117489)
--(axis cs:21300,0.00218396005447646)
--(axis cs:21400,0.00219648367558879)
--(axis cs:21500,0.00215373729538639)
--(axis cs:21600,0.00215062662044993)
--(axis cs:21700,0.00216776895711523)
--(axis cs:21800,0.00216631967830252)
--(axis cs:21900,0.00218755615577619)
--(axis cs:22000,0.00217865970123537)
--(axis cs:22100,0.00219655721337103)
--(axis cs:22200,0.00212227347903391)
--(axis cs:22300,0.00214030589963905)
--(axis cs:22400,0.00221684915068995)
--(axis cs:22500,0.00220701884489582)
--(axis cs:22600,0.00216535496963465)
--(axis cs:22700,0.00218442436081818)
--(axis cs:22800,0.00216903765641537)
--(axis cs:22900,0.00215598303987088)
--(axis cs:23000,0.00216182080568759)
--(axis cs:23100,0.00213334526995943)
--(axis cs:23200,0.00219626565264362)
--(axis cs:23300,0.00215878533676516)
--(axis cs:23300,0.00256254095107068)
--(axis cs:23300,0.00256254095107068)
--(axis cs:23200,0.002560023105525)
--(axis cs:23100,0.00256475554029022)
--(axis cs:23000,0.00256230084685596)
--(axis cs:22900,0.00256276752016443)
--(axis cs:22800,0.00256175319708499)
--(axis cs:22700,0.0025607048246001)
--(axis cs:22600,0.00256202848500606)
--(axis cs:22500,0.00255951259894842)
--(axis cs:22400,0.00255914856624354)
--(axis cs:22300,0.00256411610736537)
--(axis cs:22200,0.00256581902838806)
--(axis cs:22100,0.00256000783716139)
--(axis cs:22000,0.00256107743691676)
--(axis cs:21900,0.00256051321501016)
--(axis cs:21800,0.00256195551770338)
--(axis cs:21700,0.00256184703295725)
--(axis cs:21600,0.00256321323086986)
--(axis cs:21500,0.00256295240301172)
--(axis cs:21400,0.00256001168097096)
--(axis cs:21300,0.00256073389285862)
--(axis cs:21200,0.00255889579477191)
--(axis cs:21100,0.00256082335806374)
--(axis cs:21000,0.00256101942352515)
--(axis cs:20900,0.00255880814749498)
--(axis cs:20800,0.00256249107127324)
--(axis cs:20700,0.00256065216142572)
--(axis cs:20600,0.00256067430388362)
--(axis cs:20500,0.00255881965278774)
--(axis cs:20400,0.00255906371973628)
--(axis cs:20300,0.00256017506018923)
--(axis cs:20200,0.00255900190510225)
--(axis cs:20100,0.00255945247294253)
--(axis cs:20000,0.00255876139444466)
--(axis cs:19900,0.00255942445298392)
--(axis cs:19800,0.00256044310064376)
--(axis cs:19700,0.00255200927521171)
--(axis cs:19600,0.0025488839240561)
--(axis cs:19500,0.00255515738920067)
--(axis cs:19400,0.00256195904226043)
--(axis cs:19300,0.0025655256827614)
--(axis cs:19200,0.00257206839778622)
--(axis cs:19100,0.00255656957571777)
--(axis cs:19000,0.00256454150390636)
--(axis cs:18900,0.00259202469361872)
--(axis cs:18800,0.00255150225380141)
--(axis cs:18700,0.00257245667101978)
--(axis cs:18600,0.00256465933994714)
--(axis cs:18500,0.00256520386022763)
--(axis cs:18400,0.00256861549901545)
--(axis cs:18300,0.00256580568686835)
--(axis cs:18200,0.0025786121031179)
--(axis cs:18100,0.00257859791379061)
--(axis cs:18000,0.00257235955911811)
--(axis cs:17900,0.00257781719394165)
--(axis cs:17800,0.00256164501393052)
--(axis cs:17700,0.00257931534778769)
--(axis cs:17600,0.00258573532464307)
--(axis cs:17500,0.0025758469983459)
--(axis cs:17400,0.00259683361446635)
--(axis cs:17300,0.00257510423159324)
--(axis cs:17200,0.00257298503959064)
--(axis cs:17100,0.00261293818518364)
--(axis cs:17000,0.00257961035987635)
--(axis cs:16900,0.00257306062677165)
--(axis cs:16800,0.00259811365295515)
--(axis cs:16700,0.00258072337623243)
--(axis cs:16600,0.00260260674056293)
--(axis cs:16500,0.00261734134576491)
--(axis cs:16400,0.00261054206672845)
--(axis cs:16300,0.00258630739324743)
--(axis cs:16200,0.00259277973722084)
--(axis cs:16100,0.00259986217286714)
--(axis cs:16000,0.00259550406788827)
--(axis cs:15900,0.00260115835576827)
--(axis cs:15800,0.00260872109568474)
--(axis cs:15700,0.00263904614429828)
--(axis cs:15600,0.00258457732459584)
--(axis cs:15500,0.00261595470624937)
--(axis cs:15400,0.00263572896088268)
--(axis cs:15300,0.00262049252952066)
--(axis cs:15200,0.00259569825054015)
--(axis cs:15100,0.00260659580281351)
--(axis cs:15000,0.00260180570561533)
--(axis cs:14900,0.00262375982250671)
--(axis cs:14800,0.00262634550087299)
--(axis cs:14700,0.00264517357530563)
--(axis cs:14600,0.00269674988451131)
--(axis cs:14500,0.00262846355464485)
--(axis cs:14400,0.00264643803860441)
--(axis cs:14300,0.00265920515710635)
--(axis cs:14200,0.00263852110656683)
--(axis cs:14100,0.00267023736556186)
--(axis cs:14000,0.00268490838778807)
--(axis cs:13900,0.00266824666500809)
--(axis cs:13800,0.00271787719971202)
--(axis cs:13700,0.00274313700453404)
--(axis cs:13600,0.00270379528511848)
--(axis cs:13500,0.00268067704066045)
--(axis cs:13400,0.00271290744382296)
--(axis cs:13300,0.00269017474729322)
--(axis cs:13200,0.00276328079689678)
--(axis cs:13100,0.0027444832525319)
--(axis cs:13000,0.00271902278491254)
--(axis cs:12900,0.00273635619298337)
--(axis cs:12800,0.00278724575735334)
--(axis cs:12700,0.00275354377735861)
--(axis cs:12600,0.00279054816443619)
--(axis cs:12500,0.00276770819036719)
--(axis cs:12400,0.00280604712472301)
--(axis cs:12300,0.00282804044178384)
--(axis cs:12200,0.00286510730213813)
--(axis cs:12100,0.00279503587727907)
--(axis cs:12000,0.00284282685981986)
--(axis cs:11900,0.00280394649466105)
--(axis cs:11800,0.00289069828781072)
--(axis cs:11700,0.00282247286445401)
--(axis cs:11600,0.00289203949327569)
--(axis cs:11500,0.00284984403684828)
--(axis cs:11400,0.00283912930865019)
--(axis cs:11300,0.00285811721537786)
--(axis cs:11200,0.00294929685214403)
--(axis cs:11100,0.00290955636028954)
--(axis cs:11000,0.00292867631108924)
--(axis cs:10900,0.00287641046348826)
--(axis cs:10800,0.00289895593812151)
--(axis cs:10700,0.00296897242786644)
--(axis cs:10600,0.00293089481127834)
--(axis cs:10500,0.0029776031035731)
--(axis cs:10400,0.00296675428819004)
--(axis cs:10300,0.00302367391604352)
--(axis cs:10200,0.00295501682025955)
--(axis cs:10100,0.00304813257605486)
--(axis cs:10000,0.00306774156314317)
--(axis cs:9900,0.00302715512063068)
--(axis cs:9800,0.00309464791295007)
--(axis cs:9700,0.00305936699217014)
--(axis cs:9600,0.00313932818268647)
--(axis cs:9500,0.00312450972315078)
--(axis cs:9400,0.00310468323173531)
--(axis cs:9300,0.00305465545412817)
--(axis cs:9200,0.00314790767708615)
--(axis cs:9100,0.00308113538700727)
--(axis cs:9000,0.00322625459583061)
--(axis cs:8900,0.00321906179076956)
--(axis cs:8800,0.00321944999740237)
--(axis cs:8700,0.00321506454944924)
--(axis cs:8600,0.00323056617565185)
--(axis cs:8500,0.0033205829444929)
--(axis cs:8400,0.003326864869973)
--(axis cs:8300,0.00330754742478693)
--(axis cs:8200,0.00344677288266524)
--(axis cs:8100,0.00337299434876275)
--(axis cs:8000,0.00335969921073273)
--(axis cs:7900,0.00347060328249559)
--(axis cs:7800,0.00345837417139029)
--(axis cs:7700,0.00340963183932061)
--(axis cs:7600,0.00343471182571562)
--(axis cs:7500,0.00349075639896196)
--(axis cs:7400,0.00357024117485704)
--(axis cs:7300,0.00357692791551512)
--(axis cs:7200,0.0036060900763697)
--(axis cs:7100,0.00362693200281388)
--(axis cs:7000,0.00362533008917951)
--(axis cs:6900,0.0036996866261552)
--(axis cs:6800,0.00380391629287425)
--(axis cs:6700,0.00374776103935569)
--(axis cs:6600,0.00381985241140496)
--(axis cs:6500,0.00392106699782019)
--(axis cs:6400,0.00390168276261109)
--(axis cs:6300,0.00409497077469951)
--(axis cs:6200,0.00395674849714877)
--(axis cs:6100,0.00402094583963127)
--(axis cs:6000,0.0041363704806645)
--(axis cs:5900,0.00407264529889892)
--(axis cs:5800,0.00424698856514276)
--(axis cs:5700,0.00428949531379831)
--(axis cs:5600,0.0044416061348919)
--(axis cs:5500,0.00436941928005482)
--(axis cs:5400,0.00449551264894084)
--(axis cs:5300,0.00449712468719654)
--(axis cs:5200,0.00461846293688459)
--(axis cs:5100,0.0047546081108487)
--(axis cs:5000,0.00482224376045566)
--(axis cs:4900,0.00482200811319471)
--(axis cs:4800,0.00497885534519483)
--(axis cs:4700,0.00498675106978302)
--(axis cs:4600,0.00502386328828844)
--(axis cs:4500,0.00502994299658374)
--(axis cs:4400,0.00521293862059051)
--(axis cs:4300,0.0051954542673432)
--(axis cs:4200,0.00535342253542299)
--(axis cs:4100,0.00549806584175793)
--(axis cs:4000,0.00553104234557171)
--(axis cs:3900,0.00562463143768644)
--(axis cs:3800,0.00579799714537366)
--(axis cs:3700,0.00577194042339813)
--(axis cs:3600,0.00586719158008705)
--(axis cs:3500,0.00594751197834379)
--(axis cs:3400,0.00599099122966608)
--(axis cs:3300,0.00616958252928804)
--(axis cs:3200,0.00636461675620377)
--(axis cs:3100,0.00630860682007254)
--(axis cs:3000,0.00646943588432874)
--(axis cs:2900,0.00665419831533688)
--(axis cs:2800,0.00681588777414074)
--(axis cs:2700,0.00712447049151507)
--(axis cs:2600,0.00714183684927421)
--(axis cs:2500,0.00750111441709885)
--(axis cs:2400,0.00762264381575113)
--(axis cs:2300,0.00812546941623711)
--(axis cs:2200,0.00856174902069605)
--(axis cs:2100,0.00903626260338839)
--(axis cs:2000,0.00994691333828951)
--(axis cs:1900,0.0114469944412533)
--(axis cs:1800,0.0140522540452398)
--(axis cs:1700,0.0168517730387731)
--(axis cs:1600,0.0201794241700767)
--(axis cs:1500,0.0241990260005989)
--(axis cs:1400,0.0279663486151482)
--(axis cs:1300,0.0311468553373333)
--(axis cs:1200,0.0331320614637371)
--(axis cs:1100,0.0339162867342711)
--(axis cs:1000,0.0343155724230596)
--(axis cs:900,0.0358465267726726)
--(axis cs:800,0.0369442589805988)
--(axis cs:700,0.0375177195675719)
--(axis cs:600,0.0377604019350165)
--(axis cs:500,0.0388990345132966)
--(axis cs:400,0.0439598217383578)
--(axis cs:300,0.0528053199022318)
--(axis cs:200,0.0564248942659119)
--(axis cs:100,0.0574415192806571)
--(axis cs:0,0.0574927553534508)
--cycle;

\addplot [ultra thick, red]
table {%
0 0.0390019230544567
100 0.0389936827123165
200 0.0388229079544544
300 0.0375131145119667
400 0.0352103672921658
500 0.0340033285319805
600 0.0329599864780903
700 0.0321963354945183
800 0.0306149907410145
900 0.0288053564727306
1000 0.0266441255807877
1100 0.0240813568234444
1200 0.0219703651964664
1300 0.0205960422754288
1400 0.0194251611828804
1600 0.0183212328702211
1700 0.0181297268718481
1800 0.017528735101223
1900 0.0173128470778465
2000 0.0171767212450504
2100 0.016873374581337
2200 0.0167872570455074
2300 0.0165390074253082
2400 0.0161902327090502
2500 0.0161007288843393
2600 0.0158032737672329
2700 0.0156663898378611
2800 0.0154373422265053
2900 0.0152802485972643
3000 0.0150782661512494
3100 0.0149456197395921
3200 0.0148753104731441
3400 0.0141486888751388
3500 0.0139814401045442
3800 0.0135905491188169
3900 0.0132729904726148
4000 0.0130700385197997
4100 0.0129816606640816
4200 0.0127052450552583
4300 0.0126409288495779
4400 0.0126267662271857
4500 0.0124004362151027
4600 0.0121300416067243
4700 0.0122229782864451
4800 0.0119788274168968
4900 0.0119394520297647
5000 0.0118710398674011
5100 0.0117152826860547
5200 0.0117233404889703
5300 0.0113882422447205
5400 0.0114380121231079
5500 0.0115096746012568
5600 0.0112760234624147
5700 0.0111290719360113
5800 0.0110337361693382
5900 0.0114271733909845
6000 0.0113175623118877
6100 0.0111346514895558
6200 0.0110569866374135
6300 0.0110439686104655
6400 0.0111447731032968
6500 0.0108800670132041
6600 0.0106532508507371
6700 0.010694770142436
6900 0.0105674890801311
7000 0.0106939664110541
7100 0.0106605319306254
7200 0.010690625756979
7300 0.0104315839707851
7400 0.0104162357747555
7500 0.010380600579083
7600 0.0101401722058654
7700 0.0103198848664761
7900 0.0101825511083007
8000 0.0102456137537956
8100 0.0100029455497861
8200 0.0102278329432011
8300 0.00994311273097992
8400 0.00998665206134319
8500 0.0101606762036681
8600 0.00992575846612453
8700 0.00991112273186445
8800 0.00993682071566582
8900 0.0100120408460498
9000 0.00978629849851131
9100 0.00989331398159266
9200 0.00973258260637522
9300 0.0097186416387558
9400 0.00957782100886106
9500 0.0095920916646719
9600 0.00983833987265825
9700 0.0096094636246562
9800 0.00957593880593777
9900 0.00946037843823433
10000 0.00947897415608168
10100 0.00962296221405268
10200 0.00938130635768175
10300 0.00931061618030071
10400 0.00946352630853653
10500 0.00934792682528496
10600 0.00919832289218903
10700 0.00927223265171051
10800 0.00924233440309763
10900 0.00905777886509895
11000 0.00918538402765989
11100 0.00899650622159243
11200 0.00914848688989878
11300 0.00910311751067638
11400 0.0093645378947258
11500 0.00914988294243813
11600 0.00908839702606201
11700 0.00894148834049702
11800 0.00895543489605188
12000 0.00912897009402514
12100 0.00887169595807791
12200 0.00889515783637762
12400 0.00878018885850906
12500 0.00875119026750326
12600 0.00866502150893211
12700 0.00872743222862482
12800 0.00882538314908743
12900 0.00859410688281059
13000 0.00871826708316803
13100 0.0086887339130044
13200 0.00856784451752901
13300 0.0085234921425581
13400 0.00870832707732916
13500 0.00879580993205309
13600 0.00857770442962646
13700 0.00856053363531828
13800 0.00860197097063065
13900 0.00850434321910143
14000 0.00861521251499653
14100 0.00848131999373436
14200 0.0084846168756485
14300 0.00843123439699411
14400 0.00840146094560623
14500 0.00852175615727901
14600 0.00832656212151051
14700 0.00840636435896158
14800 0.00841182563453913
14900 0.00835509784519672
15000 0.00827089883387089
15100 0.00834347866475582
15200 0.00835759285837412
15300 0.00844607688486576
15400 0.00835950672626495
15500 0.00823984108865261
15600 0.00815827213227749
15700 0.00816701073199511
15800 0.0082173990085721
15900 0.00819565635174513
16200 0.00831568986177444
16300 0.00813348032534122
16400 0.00819550361484289
16500 0.00812134891748428
16600 0.00812141504138708
16700 0.00817483849823475
16800 0.00820812862366438
16900 0.00828126259148121
17000 0.00817044544965029
17100 0.00825378019362688
17200 0.00817230250686407
17300 0.0081886313855648
17400 0.00827583111822605
17500 0.00818782765418291
17600 0.00819241348654032
17700 0.00825630035251379
17800 0.00816677324473858
17900 0.00814557634294033
18100 0.00819284934550524
18200 0.00813794694840908
18300 0.00818628538399935
18400 0.00819408241659403
18500 0.00814934261143208
18700 0.00815757364034653
18800 0.00812523253262043
18900 0.00815735477954149
19000 0.00809905119240284
19100 0.00811012554913759
19200 0.00805819593369961
19300 0.00812121015042067
19400 0.00816332176327705
19500 0.00818012654781342
19600 0.00806459970772266
19700 0.00816207565367222
19800 0.00813724100589752
19900 0.00808362010866404
20000 0.00810977816581726
20100 0.00805418007075787
20200 0.00820263382047415
20400 0.00807537883520126
20600 0.00809565093368292
20800 0.00802971329540014
20900 0.00800931174308062
21000 0.00805594958364964
21100 0.00802913121879101
21400 0.00807925406843424
21500 0.00811346527189016
21600 0.0079851346090436
21800 0.00812112540006638
21900 0.00798559933900833
22000 0.00806191749870777
22100 0.00807419512420893
22200 0.00804510340094566
22300 0.0080636702477932
22400 0.00804745778441429
22500 0.0080030532553792
22600 0.00808968394994736
22700 0.00805204547941685
};\addlegendentry{Baseline}


\addplot [ultra thick, blue]
table {%
0 0.0389803573489189
100 0.038972333073616
200 0.0388000160455704
300 0.0374469012022018
400 0.0352202355861664
500 0.033958937972784
600 0.0329038128256798
700 0.0320968106389046
800 0.030531557276845
900 0.0285258647054434
1000 0.026262529194355
1100 0.0237037353217602
1200 0.0216880682855844
1300 0.0203223526477814
1400 0.0193089321255684
1500 0.0186878722161055
1600 0.0181613303720951
1700 0.0178214274346828
1800 0.0172096956521273
1900 0.0169226881116629
2000 0.0164318047463894
2200 0.0156324468553066
2300 0.015087129548192
2400 0.0143764419481158
2500 0.0143012637272477
2600 0.0138147780671716
2700 0.0138850584626198
2800 0.0133316274732351
2900 0.0132384495809674
3000 0.0129872700199485
3100 0.0129431122913957
3200 0.0127917695790529
3300 0.0125276194885373
3400 0.012561647221446
3500 0.0122674638405442
3600 0.0122336819767952
3700 0.012222096323967
3800 0.0120321568101645
3900 0.0120145892724395
4000 0.0118532618507743
4100 0.0119444020092487
4200 0.0117938509210944
4300 0.0117394346743822
4400 0.0117684882134199
4500 0.0117136873304844
4600 0.0115251308307052
4700 0.0115438904613256
4900 0.0113093676045537
5000 0.0113608287647367
5100 0.0113014141097665
5200 0.0112177571281791
5300 0.0110213588923216
5400 0.0110453171655536
5500 0.0112416855990887
5600 0.0109901521354914
5700 0.0106939077377319
5800 0.0108024850487709
5900 0.0109475366771221
6100 0.0107381111010909
6200 0.0107879210263491
6300 0.0105973612517118
6400 0.0107086002826691
6600 0.0102835493162274
6700 0.0104989232495427
6800 0.0101979495957494
6900 0.0101312389597297
7000 0.0101994192227721
7100 0.0102871228009462
7300 0.0100508155301213
7400 0.00992138404399157
7500 0.00970035325735807
7600 0.00977334380149841
7800 0.00969079881906509
7900 0.00948402844369411
8000 0.00953772943466902
8100 0.00965431425720453
8200 0.00946723110973835
8300 0.00930418260395527
8400 0.00949972867965698
8500 0.00937309581786394
8600 0.00933957006782293
8700 0.00936607457697392
8800 0.00923845358192921
8900 0.00907100550830364
9000 0.00904232263565063
9200 0.00912554282695055
9300 0.00891750771552324
9400 0.00866978894919157
9500 0.00880960747599602
9600 0.00879657827317715
9700 0.00870943162590265
9900 0.00861235242336988
10000 0.00879153795540333
10100 0.00877493154257536
10200 0.00841045472770929
10300 0.00854782108217478
10400 0.00838536117225885
10500 0.00841487478464842
10600 0.00824159197509289
10700 0.0081984605640173
10800 0.00817053113132715
10900 0.00800969917327166
11000 0.00808418821543455
11100 0.00800387468189001
11200 0.0080918250605464
11300 0.00792365428060293
11400 0.00809953175485134
11500 0.00775809353217483
11600 0.00780349923297763
11700 0.00786848179996014
11800 0.00779292499646544
11900 0.00775830633938313
12000 0.00779567658901215
12100 0.00754696922376752
12200 0.0075171273201704
12300 0.00750179123133421
12400 0.00760247884318233
12500 0.00754252914339304
12600 0.0073470170609653
12700 0.00755669921636581
12800 0.00736535107716918
12900 0.0072655463591218
13000 0.00730082346126437
13100 0.0073739280924201
13200 0.00714587885886431
13300 0.0071314019151032
13400 0.00707532232627273
13500 0.00712733576074243
13600 0.00714360782876611
13700 0.00704998057335615
13800 0.00711098359897733
13900 0.00695028528571129
14000 0.00690582022070885
14100 0.00705944979563355
14200 0.00687442906200886
14300 0.00681094126775861
14400 0.0068821283057332
14500 0.00679827760905027
14600 0.00681336084380746
14700 0.00669690407812595
14800 0.00678486656397581
14900 0.00664667459204793
15000 0.00677673658356071
15100 0.00662858597934246
15200 0.00662335567176342
15300 0.0066615603864193
15400 0.00661730067804456
15500 0.00646835193037987
15600 0.00642559444531798
15700 0.00655906740576029
15800 0.00647376570850611
15900 0.00632072938606143
16000 0.0063746590167284
16100 0.00639594020321965
16200 0.00633118255063891
16300 0.00623595947399735
16400 0.00626655714586377
16500 0.00645607011392713
16600 0.00647311192005873
16700 0.00621029548346996
16800 0.0062436256557703
16900 0.00616598315536976
17000 0.00619148788973689
17100 0.0061240210197866
17200 0.00614849105477333
17300 0.00620746333152056
17400 0.00625444576144218
17500 0.00623775692656636
17600 0.00602635974064469
17700 0.00596913741901517
17800 0.00601071491837502
17900 0.00597394956275821
18000 0.00598450284451246
18100 0.00603135395795107
18200 0.00587280141189694
18300 0.00597759801894426
18400 0.00590615486726165
18500 0.00592605443671346
18700 0.00583451567217708
18800 0.00583174219354987
18900 0.00581417977809906
19000 0.00593693694099784
19100 0.00584928411990404
19200 0.00587445870041847
19300 0.00586859881877899
19400 0.00580717483535409
19500 0.00581375509500504
19600 0.00576844578608871
19700 0.00573682086542249
19800 0.00582235679030418
19900 0.00586082972586155
20000 0.00576834753155708
20100 0.00563983293250203
20200 0.00574952038004994
20300 0.00561711611226201
20400 0.00574662396684289
20500 0.0056928233243525
20600 0.00571722397580743
20700 0.00558786978945136
20800 0.00562812015414238
20900 0.00548638682812452
21000 0.0057282829657197
21100 0.00559033360332251
21200 0.0055290712043643
21300 0.00575303146615624
21400 0.00562668638303876
21500 0.00557339703664184
21600 0.00554435979574919
21700 0.00545462500303984
21800 0.00558615196496248
21900 0.00553443701937795
22000 0.00547066610306501
22100 0.00558395963162184
22200 0.00550192315131426
22300 0.00551190553233027
22400 0.00544218253344297
22500 0.00548007432371378
22600 0.00548215350136161
22700 0.00534958811476827
22800 0.00550781330093741
22900 0.00552299479022622
23000 0.00543622206896544
23200 0.00545924436300993
23400 0.00542206782847643
23500 0.00547273876145482
23600 0.00560000585392118
23700 0.00544089497998357
23800 0.00545236794278026
};\addlegendentry{K1}

\addplot [ultra thick, green!50.2156862745098!black]
table {%
0 0.0574927590787411
100 0.0574406757950783
200 0.056412048637867
300 0.0525981411337852
400 0.0438002310693264
500 0.0387007035315037
600 0.0377058610320091
700 0.0374098345637321
800 0.0367049835622311
900 0.0353227257728577
1000 0.0342656560242176
1100 0.0338297300040722
1200 0.0328571349382401
1300 0.0306870006024837
1400 0.0277278013527393
1500 0.0239494126290083
1600 0.0195965263992548
1700 0.0163587685674429
1800 0.0135359186679125
1900 0.0111418971791863
2000 0.0098130851984024
2100 0.00899625476449728
2200 0.00843188725411892
2300 0.00807462073862553
2400 0.0075925188139081
2500 0.00737846782431006
2600 0.00709971832111478
2700 0.00692428881302476
2800 0.00670920219272375
2900 0.00654522236436605
3000 0.00642398931086063
3100 0.00624857377260923
3200 0.0061981906183064
3300 0.0061222156509757
3400 0.00594382779672742
3500 0.00586579972878098
3600 0.00581231294199824
3700 0.00562969595193863
3800 0.00564996665343642
3900 0.00551406666636467
4000 0.00544707523658872
4100 0.00543672358617187
4200 0.00530816148966551
4300 0.00516751362010837
4400 0.00510093942284584
4500 0.0049972184933722
4600 0.00494495546445251
4700 0.00491088163107634
4800 0.00481398683041334
4900 0.00478844624012709
5000 0.00475131534039974
5100 0.00467673875391483
5200 0.00456881290301681
5300 0.0044405753724277
5400 0.00442026648670435
5500 0.00428563542664051
5600 0.00431812461465597
5700 0.00422163028270006
5800 0.00422077486291528
5900 0.00406212639063597
6000 0.00405807187780738
6100 0.00396275892853737
6200 0.00394827499985695
6300 0.00399077776819468
6400 0.00384368281811476
6500 0.00390925258398056
6600 0.00378087139688432
6700 0.00371779594570398
6800 0.0037037602160126
6900 0.00360972317866981
7000 0.00359444529749453
7200 0.00358733674511313
7300 0.00355318398214877
7400 0.00348317273892462
7500 0.00346478982828557
7600 0.00341253401711583
7700 0.00339297391474247
7900 0.00342996744439006
8000 0.00332343811169267
8100 0.00333821843378246
8300 0.00330216367729008
8400 0.00324496650137007
8500 0.00325445551425219
8600 0.00318955816328526
8700 0.00317675271071494
8800 0.00318000162951648
8900 0.0031582631636411
9000 0.00315605662763119
9100 0.00307208974845707
9200 0.00312650762498379
9300 0.00303776515647769
9400 0.00308103626593947
9500 0.0030801584944129
9600 0.00308786705136299
9700 0.00304041802883148
9800 0.00305859535001218
9900 0.0030045066960156
10000 0.00302105280570686
10100 0.00301580503582954
10200 0.00293476553633809
10300 0.00299250660464168
10400 0.00291973678395152
10500 0.00294475210830569
10600 0.00289667816832662
10700 0.00293075502850115
10800 0.00286599318496883
10900 0.00286266743205488
11000 0.00291390670463443
11100 0.00286912266165018
11200 0.0029001166112721
11300 0.00284244283102453
11400 0.00282972399145365
11500 0.00282265688292682
11600 0.00283979577943683
11700 0.00281099718995392
11800 0.00283909752033651
11900 0.0027898782864213
12100 0.00277675758115947
12200 0.00281321723014116
12300 0.00276858964934945
12400 0.00274566933512688
12500 0.00271419598720968
12600 0.00273988582193851
12800 0.00271238922141492
12900 0.00271595316007733
13000 0.00268420740030706
13100 0.00270903180353343
13200 0.00268278131261468
13300 0.00264571630395949
13400 0.00265437690541148
13500 0.00263375067152083
13600 0.00264086248353124
13700 0.00270256726071239
13800 0.00265736877918243
13900 0.00264181941747665
14000 0.00261907000094652
14100 0.00260724616236985
14200 0.00257798796519637
14300 0.00259087770245969
14400 0.00257690832950175
14500 0.00255757058039308
14600 0.00260532461106777
14700 0.00258851773105562
14800 0.00255085388198495
14900 0.00254411180503666
15000 0.00252660224214196
15100 0.0025353014934808
15200 0.00253649172373116
15400 0.00254589854739606
15500 0.00251022446900606
15600 0.00250587635673583
15700 0.0025520627386868
15800 0.00251921452581882
15900 0.00249793077819049
16000 0.00249495264142752
16100 0.00252981251105666
16200 0.00252676452510059
16300 0.00250427424907684
16400 0.00253638182766736
16600 0.00247815414331853
16700 0.00246660364791751
16800 0.0025231521576643
16900 0.00245978566817939
17000 0.00248031690716743
17100 0.00254690647125244
17200 0.00244691525585949
17300 0.00247385213151574
17400 0.00248478446155787
17500 0.00243406416848302
17600 0.00244503538124263
17800 0.00242702569812536
17900 0.00244106142781675
18000 0.00242616236209869
18100 0.00247212522663176
18200 0.00242968392558396
18300 0.00243386370129883
18400 0.00240864348597825
18500 0.00240942765958607
18600 0.00243677967227995
18700 0.00244480185210705
18800 0.00239279516972601
18900 0.00243730819784105
19000 0.00242938776500523
19100 0.00239509111270308
19200 0.00242128456011415
19400 0.00239042402245104
19500 0.00239407899789512
19600 0.00237367255613208
19700 0.00238411361351609
19800 0.00240029697306454
19900 0.00238429312594235
20000 0.00240070163272321
20100 0.00238396064378321
20200 0.00240815151482821
20300 0.00241948803886771
20500 0.0023950464092195
20600 0.00237279431894422
20700 0.00237296242266893
20800 0.00236095068976283
20900 0.00239548971876502
21000 0.00237027532421052
21100 0.00237168488092721
21200 0.00239278329536319
21300 0.00237234774976969
21400 0.00237824814394116
21500 0.00235834438353777
21600 0.00235691945999861
21700 0.00236480846069753
21800 0.00236413744278252
21900 0.0023740348406136
22000 0.00236986787058413
22100 0.00237828213721514
22200 0.00234404671937227
22300 0.00235221046023071
22400 0.00238799885846674
22500 0.0023832656443119
22600 0.00236369227059186
22700 0.002372563816607
22900 0.00235937512479722
23000 0.00236206059344113
23100 0.00234905024990439
23200 0.00237814383581281
23300 0.00236066314391792
}; \addlegendentry{K2}

==> supp_mat/ur5e_plots/traj_err_data.tex <==
\path [fill=red, fill opacity=0.4, ultra thick]
(axis cs:1,0.425842757042726)
--(axis cs:1,0.369011197968586)
--(axis cs:5,0.340659076055574)
--(axis cs:15,0.215481461951959)
--(axis cs:25,0.161485036747361)
--(axis cs:50,0.121269717837292)
--(axis cs:100,0.122246150710438)
--(axis cs:100,0.199646389379003)
--(axis cs:100,0.199646389379003)
--(axis cs:50,0.204837884818649)
--(axis cs:25,0.260791318943091)
--(axis cs:15,0.310860167617414)
--(axis cs:5,0.379305355618416)
--(axis cs:1,0.425842757042726)
--cycle;

\path [fill=blue, fill opacity=0.4, ultra thick]
(axis cs:1,0.425728743098355)
--(axis cs:1,0.368476143608182)
--(axis cs:5,0.340969836179182)
--(axis cs:15,0.198690673072993)
--(axis cs:25,0.164320584402678)
--(axis cs:50,0.115447289735228)
--(axis cs:100,0.122139999108882)
--(axis cs:100,0.158075039864172)
--(axis cs:100,0.158075039864172)
--(axis cs:50,0.158764253051484)
--(axis cs:25,0.259565857354428)
--(axis cs:15,0.300096100030564)
--(axis cs:5,0.38032091498312)
--(axis cs:1,0.425728743098355)
--cycle;

\path [fill=green!50.1960784313725!black, fill opacity=0.4, ultra thick]
(axis cs:1,0.403154509634611)
--(axis cs:1,0.360432041582331)
--(axis cs:5,0.0947917792092252)
--(axis cs:15,0.0874259090992881)
--(axis cs:25,0.0684932792479964)
--(axis cs:50,0.0639969877720852)
--(axis cs:100,0.0616857911404033)
--(axis cs:100,0.0796748887686242)
--(axis cs:100,0.0796748887686242)
--(axis cs:50,0.0856512706605412)
--(axis cs:25,0.0920321341262693)
--(axis cs:15,0.121028934402069)
--(axis cs:5,0.146313848306424)
--(axis cs:1,0.403154509634611)
--cycle;

\addplot [ultra thick, red, mark=*, mark size=1.5, mark options={solid}]
table {%
1 0.3974269926548
5 0.359982252120972
15 0.263170778751373
25 0.211138218641281
50 0.163053810596466
100 0.160946264863014
};
\addplot [ultra thick, blue, mark=*, mark size=1.5, mark options={solid}]
table {%
1 0.397102475166321
5 0.36064538359642
15 0.249393373727798
25 0.211943238973618
50 0.137105777859688
100 0.140107527375221
};
\addplot [ultra thick, green!50.1960784313725!black, mark=*, mark size=1.5, mark options={solid}]
table {%
1 0.381793349981308
5 0.120552815496922
15 0.104227423667908
25 0.0802627131342888
50 0.0748241320252419
100 0.0706803351640701
};
